Regret Lower Bounds for Decentralized Multi-Agent Stochastic Shortest Path Problems

Multi-agent systems (MAS) are central to applications such as swarm robotics and traffic routing, where agents must coordinate in a decentralized manner to achieve a common objective. Stochastic Shortest Path (SSP) problems provide a natural framework for modeling decentralized control in such settings. While the problem of learning in SSP has been extensively studied in single-agent settings, the decentralized multi-agent variant remains largely unexplored. In this work, we take a step towards addressing that gap. We study decentralized multi-agent SSPs (Dec-MASSPs) under linear function approximation, where the transition dynamics and costs are represented using linear models. Applying novel symmetry-based arguments, we identify the structure of optimal policies. Our main contribution is the first regret lower bound for this setting based on the construction of hard-to-learn instances for any number of agents, $n$. Our regret lower bound of $\Omega(\sqrt{K})$, over $K$ episodes, highlights the inherent learning difficulty in Dec-MASSPs. These insights clarify the learning complexity of decentralized control and can further guide the design of efficient learning algorithms in multi-agent systems.

==> CR_Sections/all_updated_7_4_25.tex <==
\section{Experiments}
\label{sec:experiment}
In this section, we provide the details of the MDP network that we use to prove that lower bound. Consider a network with two nodes $\{s_{init}, g\}$. Thus, the number of states is $2^n$, where $n$ is the number of agents.
In each state the actions available to each agent are $\mathcal{A}^i = \{-1, 1\}^{d-1}$, for some given $d\geq 2$. So, the total number of actions is $2^{nd}$. 
Since the number of states and actions is exponentially large, we parameterize the transition probability. For each $(\tb{\ti{s}}^{\prime}, \tb{\ti{a}}, \tb{\ti{s}}) \in \mathcal{S} \times \mathcal{A} \times \mathcal{S}$, the global transition probability is parameterized as $\mathbb{P}_{\boldsymbol{\theta}}(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}) = \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},\tb{\ti{a}}), {\boldsymbol{\theta}} \rangle$.  The global features  are described below.


\textcolor{red}{Below are the updated features that match Min et al at n=1. The proof for this is in the appendix below proof for previous features.}

\pt{These are the final updated features, right? If this is the case. The first result we need to write is -- the features are valid and hence satisfy all the properties. These features will reduce to the Min paper when $n=1$.}
\textcolor{red}{yes these are the final ones from my side as of now, i would remove the 4th case in $\phi^i(.)$ definition}

\begin{equation}
\label{eqn:features_global_new}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  \tb{\ti{a}}) = 
\begin{cases} (\phi(s^{\prime^1} | s^1, \tb{\ti{a}}^1), \dots, \phi(s^{\prime^n} | s^n, \tb{\ti{a}}^n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}} ~\text{and}~  s^{i'} = g ~\text{if} ~ s^i = g,~ \forall~ i\in N
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}}, \text{or },  \exists~ i \in N,~ s.t. ~ s^i \neq s_{init}, s^{i'} = s_{init}
\\
(\mb{0}_{nd-1}, 1), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}}, 
\end{cases}
\end{equation}

Here $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i)$ are defined as 
\begin{equation*}
\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) = \begin{cases}  
\left(-\tb{\ti{a}}^i, \frac{1-\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}^i = s^{\prime^{i}} = s_{init}
\\
\left(\tb{\ti{a}}^i, \frac{\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}^i = s_{init},~s^{\prime^{i}} = g
\\
\left(\mathbf{0}_{d-1}, \frac{1}{n 2^{r}} \right)^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = g
\\
\mathbf{0}_d^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = s_{init}.
\end{cases}
\end{equation*}

==> CR_Sections/experiments.tex <==
\section{\textit{Transition Probability Model} Experiments}
\label{sec:experiment}
In this section, we provide the details of the MDP network that we use to prove that lower bound. Consider a network with two nodes $\{s_{init}, g\}$. Thus, the number of states is $2^n$, where $n$ is the number of agents.
In each state the actions available to each agent are $\mathcal{A}^i = \{-1, 1\}^{d-1}$, for some given $d\geq 2$. So, the total number of actions is $2^{nd}$. 
Since the number of states and actions is exponentially large, we parameterize the transition probability. For each $(\tb{\ti{s}}^{\prime}, \tb{\ti{a}}, \tb{\ti{s}}) \in \mathcal{S} \times \mathcal{A} \times \mathcal{S}$, the global transition probability is parameterized as $\mathbb{P}_{\boldsymbol{\theta}}(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}) = \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},\tb{\ti{a}}), {\boldsymbol{\theta}} \rangle$.  The global features  are described below. \\
\textcolor{red}{in the above, total # actions need to be $2^{n(d-1)}$}


\textcolor{red}{Below are the updated features that match Min et al at n=1. The proof for this is in the appendix below proof for previous features.}

\pt{These are the final updated features, right? If this is the case. The first result we need to write is -- the features are valid and hence satisfy all the properties. These features will reduce to the Min paper when $n=1$.}
\textcolor{red}{yes these are the final ones from my side as of now, i would remove the 4th case in $\phi^i(.)$ definition}

\begin{equation}
\label{eqn:features_global_new}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  \tb{\ti{a}}) = 
\begin{cases} (\phi(s^{\prime^1} | s^1, \tb{\ti{a}}^1), \dots, \phi(s^{\prime^n} | s^n, \tb{\ti{a}}^n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}} ~\text{and}~  s^{i'} = g ~\text{if} ~ s^i = g,~ \forall~ i\in N
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}}, \text{or },  \exists~ i \in N,~ s.t. ~ s^i \neq s_{init}, s^{i'} = s_{init}
\\
(\mb{0}_{nd-1}, 1), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}}, 
\end{cases}
\end{equation}

Here $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i)$ are defined as 
\begin{equation*}
\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) = \begin{cases}  
\left(-\tb{\ti{a}}^i, \frac{1-\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}^i = s^{\prime^{i}} = s_{init}
\\
\left(\tb{\ti{a}}^i, \frac{\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}^i = s_{init},~s^{\prime^{i}} = g
\\
\left(\mathbf{0}_{d-1}, \frac{1}{n 2^{r}} \right)^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = g
\\
\mathbf{0}_d^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = s_{init}.
\end{cases}
\end{equation*}
\\

In the above, $r$ represents the number of agents at $s_{init}$ and $\theta$ is an $nd$- dimensional vector of the form $\theta = (\theta_1,1, \theta_2,1,\dots,\theta_n,1)$ where for every $i \in [n]$, $\theta_i$ is a d-1 dimensional vector each of whose component is $(+/-) \frac{\Delta}{n(d-1)}$. To prove lower bound, we will further impose that for our instances, none of the two $\theta_i's$ are equal.


==> CR_Sections/extra-appedix.tex <==
\section*{Appendix}

\section{Proofs}
\label{app:proofs}

In this section, we provide the details and proofs of the main results we stated in the paper.

\subsection{Proof of Lemma \ref{lemma: feature_properties}}
\label{app-proof:features_properties}

Recall, the global features  are given by
\begin{equation}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  \tb{\ti{a}}) = 
\begin{cases} (\phi(s^{\prime^1} | s^1, \tb{\ti{a}}^1), \dots, \phi(s^{\prime^n} | s^n, \tb{\ti{a}}^n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}}, ~\tb{\ti{s}}' \neq \tb{\ti{g}}, ~\text{and}~  s^{i'} = g ~\text{if} ~ s^i = g,~ \forall~ i\in N
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}}, \text{or },  \exists~ i \in N,~ s.t. ~ s^i \neq s_{init}, s^{i'} = g
\\
(\mb{0}_{nd-1}, 1), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}}, 
\end{cases}
\end{equation}
the first condition ensures that if an agent is at $g$, it should remain at $g$. The second condition make sure that the probability of the infeasible transitions is zero.

Here $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i)$ are defined as 
\begin{equation*}
\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) = \begin{cases}  
\left(-\tb{\ti{a}}^i, \frac{1-\delta}{r 2^r} \right)^{\top}, & if ~ {s}^i = s^{\prime^{i}} = s_{init}
\\
\left(\tb{\ti{a}}^i, \frac{\delta}{r 2^r} \right)^{\top}, & if ~ {s}^i = s_{init},~s^{\prime^{i}} = g
\\
\left(\mathbf{0}_{d-1}, \frac{1}{(n-r) 2^{r+1}} \right)^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = g
\\
\mathbf{0}_d^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = s_{init}.
\end{cases}
\end{equation*}
Here $r$ denotes the number of agent in $s_{init}$ in the global state $\tb{\ti{s}}$. The vector $\mathbf{0}_d^{\top} = (0,0, \dots, 0)^{\top}$ is a vector of $d$ dimension with all zeros. 
Thus, the features $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) \in \mathbb{R}^{nd}$. Moreover, the transition probability parameters are taken as $\boldsymbol{\theta} = \left( \boldsymbol{\theta}^1, 1,  \boldsymbol{\theta}^2, 1 \dots, \boldsymbol{\theta}^n, 1 \right)$ where $\boldsymbol{\theta}^i \in \left\lbrace -\frac{\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}  \right\rbrace^{d-1} $, and $\Delta < \delta$. 

\textbf{Recall the Lemma.}
    \textit{The features $\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},\tb{\ti{a}})$ satisfy the following: (a) $\sum_{\tb{\ti{s}}^{\prime}} \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = 1, ~ \forall ~\tb{\ti{s}}, \tb{\ti{a}}$; (b) $\langle \phi(\tb{\ti{s}}^{\prime} = \tb{\ti{g}} | \tb{\ti{s}} = \tb{\ti{g}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = 1, ~\forall~\tb{\ti{a}}$; (c) $\langle \phi(\tb{\ti{s}}^{\prime} \neq \tb{\ti{g}} | \tb{\ti{s}} = \tb{\ti{g}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = 0,~ \forall ~\tb{\ti{a}}$.}


\begin{proof}
   
    We will prove part (a), proof of the other parts follow directly from the feature design. 

\textbf{Case 1.} $\tb{\ti{s}}\neq \ti{\ti{g}}$

    Without loss of generality let us assume that $\tb{\ti{s}}$ is such that $r$ agents are at $s_{init}$, and remaining $n-r$ agents are at $g$. 

    The inner product in the summation can be rewritten as
    \begin{equation}
    \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle.
    \end{equation}
    Thus, proving the original equation reduces to proving
    \begin{equation}
        \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}} \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle = 1.
    \end{equation}
    We first note that out of $2^n$ total number of states, there are $2^r$ feasible states. For the remaining states, the features are zero by design,  and hence the above summation reduces to 
    \begin{equation}
        \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}_F} \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle = 1,
    \end{equation}
    where $\mathcal{S}_F$ is the set of all feasible state space. 
    
    Consider an agent $i$, who is at $s_{init}$. Out of total $2^r$ next possible states, there are exactly $\frac{2^r}{2}$ states in which agent $i$ will remain at $s_{init}$, and in remaining $\frac{2^r}{2}$ states in which the agents move to goal node. 
    The probability that the next node of agent $i$ is $s_{init}$ given that the current node of agent $i$ is $s_{init}$ is given by $- \langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{1-\delta}{r 2^r}$. And the probability that the next node of agent $i$ is $g$ given that the current node of agent $i$ is $s_{init}$ is  $ \langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{\delta}{r 2^r}$.
    Since, this is true for all the $r$ agents which are at $s_{init}$ so the contribution to the probability term from these $r$ agents who are at $s_{init}$ is
    \begin{eqnarray*}
        \sum_{i=1}^r \left\lbrace \left( -\langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{1-\delta}{r 2^r} \right) \times \frac{2^r}{2} \right\rbrace + \sum_{i=1}^r  \left\lbrace \left(\langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{\delta}{r 2^r} \right) \times \frac{2^r}{2} \right\rbrace = \frac{1}{2}.
    \end{eqnarray*}
    Next, consider an agent whose state is $g$; for this agent, there is only only possibility, the agent should stay at $g$. This is because it any agent tries to move to $s_{init}$, that state space is no more belong to the set of feasible state spaces. Therefore, the total number of such cases are  transitions are $2^r$. The probability that agent will stay at $g$ is  $\frac{1}{(n-r)} \times \frac{1}{2^{r+1}}$.  So the total probability in this case is  
    \begin{equation*}
        \sum_{i = r+1}^n  \frac{1}{(n-r) 2^{r+1}} \times 2^r = \frac{1}{2}.
    \end{equation*}
    So, the sum of these linearly approximated probabilities is
	\begin{eqnarray*}
		\sum_{\tb{\ti{s}}^{\prime}\in \mathcal{S}} \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \sum_{\tb{\ti{s}}^{\prime}\in \mathcal{S}_F} \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \frac{1}{2} + \frac{1}{2} = 1.
	\end{eqnarray*}

\textbf{Case 2.} $\tb{\ti{s}} =  \ti{\ti{g}}$

\begin{align}
    \sum_{\tb{\ti{s}}'\in \mathcal{S}} \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle &=  \langle \phi(\tb{\ti{s}}^{\prime} = \tb{\ti{g}}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle + \sum_{\tb{\ti{s}}' \neq \tb{\ti{g}}} \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle 
    \\
    & = 0 +  \langle (\tb{0}_{nd-1}, 1), (\theta^1, 1, \theta^2, 1,\dots, \theta^n, 1) \rangle \\ 
    &= 1.
\end{align}
This completes the proof. 
\end{proof}


\begin{proof} 
% 
\textcolor{red}{THIS IS FOR UPDATED FEATURES WHICH MATCH MIN ET AL FOR n=1. I HAVEN'T VERIFIED THE EXPLANATIONS IN ENGLISH BUT ONLY MODIFIED THE RESPECTIVE MATHEMATICAL EXPRESSIONS} 

We will prove part (a), proof of the other parts follow directly from the feature design. 

\textbf{Case 1.} $\tb{\ti{s}}\neq \ti{\ti{g}}$

    Without loss of generality let us assume that $\tb{\ti{s}}$ is such that $r$ agents are at $s_{init}$, and remaining $n-r$ agents are at $g$. 

    The inner product in the summation can be rewritten as
    \begin{equation}
    \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle.
    \end{equation}
    Thus, proving the original equation reduces to proving
    \begin{equation}
        \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}} \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle = 1.
    \end{equation}
    We first note that out of $2^n$ total number of states, there are $2^r$ feasible states. For the remaining states, the features are zero by design,  and hence the above summation reduces to 
    \begin{equation}
        \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}_F} \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle = 1,
    \end{equation}
    where $\mathcal{S}_F$ is the set of all feasible state space. 
    
    Consider an agent $i$, who is at $s_{init}$. Out of total $2^r$ next possible states, there are exactly $\frac{2^r}{2}$ states in which agent $i$ will remain at $s_{init}$, and in remaining $\frac{2^r}{2}$ states in which the agents move to goal node. 
    The probability that the next node of agent $i$ is $s_{init}$ given that the current node of agent $i$ is $s_{init}$ is given by $- \langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{1-\delta}{n 2^{r-1}}$. And the probability that the next node of agent $i$ is $g$ given that the current node of agent $i$ is $s_{init}$ is  $ \langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{\delta}{n 2^{r-1}}$.
    Since, this is true for all the $r$ agents which are at $s_{init}$ so the contribution to the probability term from these $r$ agents who are at $s_{init}$ is
    \begin{eqnarray*}
        \sum_{i=1}^r \left\lbrace \left( -\langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{1-\delta}{n 2^{r-1}} \right) \times \frac{2^r}{2} \right\rbrace + \sum_{i=1}^r  \left\lbrace \left(\langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{\delta}{n 2^{r-1}} \right) \times \frac{2^r}{2} \right\rbrace = \frac{r}{n}.
    \end{eqnarray*}
    Next, consider an agent whose state is $g$; for this agent, there is only only possibility, the agent should stay at $g$. This is because it any agent tries to move to $s_{init}$, that state space is no more belong to the set of feasible state spaces. Therefore, the total number of such cases are  transitions are $2^r$. The probability that agent will stay at $g$ is  $\frac{1}{n} \times \frac{1}{2^{r}}$.  So the total probability in this case is  
    \begin{equation*}
        \sum_{i = r+1}^n  \frac{1}{n 2^{r}} \times 2^r = \frac{n-r}{n}.
    \end{equation*}
    So, the sum of these linearly approximated probabilities is
	\begin{eqnarray*}
		\sum_{\tb{\ti{s}}^{\prime}\in \mathcal{S}} \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \sum_{\tb{\ti{s}}^{\prime}\in \mathcal{S}_F} \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \frac{r}{n} + \frac{n-r}{n} = 1.
	\end{eqnarray*}

\textbf{Case 2.} $\tb{\ti{s}} =  \ti{\ti{g}}$

\begin{align}
    \sum_{\tb{\ti{s}}'\in \mathcal{S}} \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle &=  \langle \phi(\tb{\ti{s}}^{\prime} = \tb{\ti{g}}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle + \sum_{\tb{\ti{s}}' \neq \tb{\ti{g}}} \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle 
    \\
    & = 0 +  \langle (\tb{0}_{nd-1}, 1), (\theta^1, 1, \theta^2, 1,\dots, \theta^n, 1) \rangle \\ 
    &= 1.
\end{align}
This completes the proof. 
\end{proof}







==> CR_Sections/extras1.tex <==
\begin{subsection}{Proposed Model}
    


Hey, I had come up with the following feature design
\begin{equation*}
\label{eqn: features_global}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  \tb{\ti{a}}) = 
\begin{cases} (\phi(s^{\prime^1} | s^1, \tb{\ti{a}}^1), \dots, \phi(s^{\prime^n} | s^n, \tb{\ti{a}}^n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}} and s^{i}=g \implies s^{\prime^i} = g  \forall i \in [N]
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}},   or if ~\tb{\ti{s}} \neq \tb{\ti{g}} but \exists i \in [N] s.t. s^{i}=g but s^{\prime^i} \neq g
\\
(\mb{0}_{nd-1}, 1), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}},
\end{cases}
\end{equation*}

where $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i)$ is defined as 
\begin{equation*}
\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) = \begin{cases}  
\left(-\tb{\ti{a}}^i, \frac{1-\delta}{k.2^k} \right)^{\top}, & if ~ {s}^i = s^{\prime^{i}} = s_{init}
\\
\left(\tb{\ti{a}}^i, \frac{\delta}{k.2^k} \right)^{\top}, & if ~ {s}^i = s_{init},~s^{\prime^{i}} = g
\\
\left(\mathbf{0}_{d-1}, \frac{1}{(n-k).2^{k+1}} \right)^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = g.
\end{cases}
\end{equation*}
Here $\mathbf{0}_d^{\top} = (0,0, \dots, 0)^{\top}$ is a vector of $d$ dimension with all zeros.
Thus, the features $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) \in \mathbb{R}^{nd}$. Moreover, the transition probability parameters are taken as $\boldsymbol{\theta} = \left( \boldsymbol{\theta}^1, 1,  \boldsymbol{\theta}^2, 1 \dots, \boldsymbol{\theta}^n, 1 \right)$ where $\boldsymbol{\theta}^i \in \left\lbrace -\frac{\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}  \right\rbrace^{d-1} $, and $\Delta < \delta$. Also, k represents the number of agents at $s_{init}$ in s. \\
\end{subsection}
\begin{subsection}{Why the above Model works}
Let's partition the set of all global transitions $( \tb{s}, \tb{\ti{a}}, \tb{s}^{\prime}) \in \mathcal{S}\times\mathcal{A}\times\mathcal{S}$ into the following: \pt{Note that the entire thing is true irrespective of the agent's action.}
\\
\begin{enumerate}
    \item When $\tb{s} = \tb{g}$ 
    \begin{enumerate}
        \item $\tb{s}^{\prime} = \tb{g}$ \\
        Corresponds to the third case in the definition of global $\phi(.|.,.)$
        \\
    Then, 
    \begin{align}
    \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
    \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
    & =\langle \phi((g,g,g,...,g)|(s,g,g,...,g),(a_1, a_2,...a_n)),\theta \rangle \\
    &= \langle (\tb{0}_{nd-1}, 1), (\theta_1, 1, \theta_2, 1, ..., \theta_n, 1) \rangle \\ 
    &= 1.
\end{align}   
        \item When $\tb{s}^{\prime} \neq \tb{g}$ \\ (This implies that there is at least one agent that moves back to $s_{init}$. Corresponds to first part of the second condition in the definition of global $\phi(.|.,.)$. This takes care of the $2^{n}-1$ impossible transitions for any global action)
        \begin{align}
    \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
    \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
    & =\langle \tb{0}_{nd},\theta \rangle \\
    &= 0.
    \end{align}
    \end{enumerate}
    \item When $\tb{s} \neq \tb{g}$
    \begin{enumerate}
        
        \item When there exists some agent who transits from g to $s_{init}$. \pt{This case was not considered in the previous feature design. And hence this probability was non-zero.} \\
        This corresponds to the "or" part of the second case in the definition of global $\phi(.|.,.)$

        \begin{align}
    \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
    \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
    & =\langle \tb{0}_{nd},\theta \rangle \\
    &= 0.
    \end{align}

        \item When there exists no agent who transits from g to $s_{init}$. \\ That means all agents either remain put in their original state or only transit from $s_{init}$ to $g$. This is the most general case and the most interesting one too. Takes care of all but the corner cases mentioned above.\\
        Consider a general initial state: $\tb{s} = (s_1,s_2,\dots,s_n)$ where agents $i_1, i_2, \dots, i_r$ are at $s_{init}$ while agents $j_1, j_2, \dots, j_{n-r}$ are already at g. We consider $r \geq 1$ as $r = 0$ is taken care of above. Let $\mathcal{I} := \{i_1, i_2, \dots, i_r\}$ and $\mathcal{J} := \{j_1, j_2, \dots, j_{n-r}\}$. Agents in $\mathcal{I}$ can transit to $s_{init}$ or g while those in $\mathcal{J}$ remain at g. Then, (where $\tb{s}^{\prime}$ denotes only a possible state i.e., not one of those discussed above with 0 probability of transition)
\begin{lalign}    \sum_{\tb{s}^{\prime}}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
 \\ &&\text{Just expand the notation} \\
&= \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})}\mathbb{P}((\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})| (\ti{s}^1, \ti{s}^2,...,\ti{s}^n), (\ti{a}^1, \ti{a}^2,...,\ti{a}^n))

\\ &&\text{Using Model} 

    \\ &=\sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2}, \dots ,\ti{s}^{\prime^n})}
    \langle \phi((\ti{s}^{\prime^1}, \ti{s}^{\prime^2}, \dots ,\ti{s}^{\prime^n})|(\ti{s}^1, \ti{s}^2,...,\ti{s}^n), (\ti{a}^1, \ti{a}^2,...,\ti{a}^n)),(\theta_1, 1, \theta_2, 1, ..., \theta_n, 1) \rangle \\
   \\&& \text{Using Features} \\ &=\sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})}
    \langle (\phi(\ti{s}^{\prime^1}|\ti{s}^1,\ti{a}^1), \phi(\ti{s}^{\prime^2}|\ti{s}^2,\ti{a}^2),...,\phi(\ti{s}^{\prime^n}|\ti{s}^n,\ti{a}^n)),(\theta_1, 1, \theta_2, 1, ..., \theta_n, 1) \rangle \\
    \\ &&\text{Individual Dot Products} \\
    &= \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})} \sum_{m = 1, 2,\dots,n}
    \langle \phi(\ti{s}^{\prime^m}|\ti{s}^m,\ti{a}^m),(\theta_m, 1) \rangle 
    \\ 
     &&\text{Sum over all agents broken into sum over two partition sets} \\
    &= \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})} \{(\sum_{i \in \mathcal{I}}
    \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle) + (\sum_{j \in \mathcal{J}}
    \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle)\}  \\ &&\text{Distributing the outer sum }\\
    &= \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},\dots ,\ti{s}^{\prime^n})} \sum_{i \in \mathcal{I}}
    \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle +  \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2}, \dots ,\ti{s}^{\prime^n})} \sum_{j \in \mathcal{J}}
    \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle
    \\ &&\text{Switching summations }\\
    &= \sum_{i \in \mathcal{I}} \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})}
    \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle +  \sum_{j \in \mathcal{J}} \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})} 
    \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle
    \\&&\text{Property of Summations }\\
&= \sum_{i \in \mathcal{I}} \Big\{  \sum_{\ti{s}^{\prime^1}} \sum_{\ti{s}^{\prime^2}} \dots \sum_{\ti{s}^{\prime^n}} \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle \Big \} + \sum_{j \in \mathcal{J}}  \Big \{  \sum_{\ti{s}^{\prime^1}} \sum_{\ti{s}^{\prime^2}} \dots \sum_{\ti{s}^{\prime^n}} \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle \Big \}
\\&&\text{'j' summations have only one choice (again according to property of summations)}\\
&= \sum_{i \in \mathcal{I}}
 \Big \{     \sum_{\ti{s}^{\prime^{i_1}}} \sum_{\ti{s}^{\prime^{i_2}}} \dots \sum_{\ti{s}^{\prime^{i_r}}} \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle \Big \} +  \sum_{j \in \mathcal{J}}  \Big \{  \sum_{\ti{s}^{\prime^{i_1}}}     \sum_{\ti{s}^{\prime^{i_2}}} \dots
\sum_{\ti{s}^{\prime^{i_r}}} 
    \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle \}
    \\
\\&& \text{Fixing an outer 'i', every other i has two choices hence $2^{r-1}$ but fixing outer 'j' every other 'i' still has 2 choices hence $2^r$.}
    \\
    &=  \sum_{i \in \mathcal{I}} \{2^{r-1}. \sum_{\ti{s}^{\prime^i}}
    \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle \} +  \sum_{j \in \mathcal{J}} \{  2^r. 
    \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle \}
    \\
    & \text{\pt{This is not clear, why we get $2^{r-1}$ and $2^r$? }}
    \\ 
     &= 
     \sum_{i \in \mathcal{I}} \{2^{r-1}. 
    \langle (0_{d-1}, \frac{1}{r.2^r})),(\theta_i, 1) \rangle \} +  \sum_{j \in \mathcal{J}} \{  2^r.  
    \langle (0_{d-1}, \frac{1}{(n-r).2^{r+1}}),(\theta_j, 1) \rangle \} 
     \\
     &= 
     \sum_{i \in \mathcal{I}} \frac{1}{2.r} +  \sum_{j \in \mathcal{J}} \frac{1}{2.(n-r)} 
     \\
     &= \frac{1}{2} + \frac{1}{2}
    \\
    & = 1.
\end{lalign}
\\

    \textcolor{brown}{Also need to show that all probabilities lie between 0 and 1. This leads to $\delta = O(2^n.\Delta) = o(1)$. But I haven't shown so far. } \\

\pt{Surprisingly, there are no terms involving $\delta$ in your entire proof. What happen to such terms?}\\
\textcolor{blue}{DOUBT ON POWERS OF 2 - I think maybe now it's clearer, I added a couple of intermediate steps. It's just mathematical simplification. 
}\\
\textcolor{blue}{ The sum over all global s' can be written as nested summations (standard technique in such summations). These summations can be permuted freely. If you permute such that the i fixed from the outer sum is the innermost summation, you will observe that this summation remains constant for all outside summations over each possibility of state. As there are 2 possibilities for $s^{\prime^l}$ for every l and as there are r-1 such states outside, factor of 2 from each of those results in $2^{r-1}$. In the sum over j, there are r states (outer summations) with the constant inner term hence $2^r$. A standard doubt may be why it is multiplying and not adding. Try to expand any nested summation and you will see why!}
\textcolor{blue}{WHY NO $\delta$ - When you add, over possible $s^{\prime^i}$ (i.e. s and g) in the first summation, you can observe that the $\delta$ terms in the corresponding features add in such a way that they cancel each other. I just haven't written explicitly that step, but it's too trivial.}
\pt{we should write the proof in more details and clean it with more readability?}
\textcolor{blue}{Absolutely, there are plenty many things I've to add. Once I add them all, we can make it more detailed.}

\pt{Still it is not clear to me. Is there a way to simplify this proof. These notations, etc are very complicated. }

\textcolor{blue}{I don't think it can be simplified. The notations were meant to simplify the transitions between steps.}
        
    \end{enumerate}
\end{enumerate}
    
\end{subsection}


Recall, the global features defined in the MACCM paper are given by
\begin{equation*}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  \tb{\ti{a}}) = 
\begin{cases} (\phi(s^{\prime^1} | s^1, \tb{\ti{a}}^1), \dots, \phi(s^{\prime^n} | s^n, \tb{\ti{a}}^n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}},
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}},
\\
(\mb{0}_{nd-1}, 2^{n-1}), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}},
\end{cases}
\end{equation*}
where $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i)$ is defined as 
\begin{equation*}
\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) = \begin{cases}  
\left(-\tb{\ti{a}}^i, \frac{1-\delta}{n} \right)^{\top}, & if ~ {s}^i = s^{\prime^{i}} = s_{init}
\\
\left(\tb{\ti{a}}^i, \frac{\delta}{n} \right)^{\top}, & if ~ {s}^i = s_{init},~s^{\prime^{i}} = g
\\
\mathbf{0}_{d}^{\top}, & if ~ {s}^i = g,~s^{\prime^{i}} = s_{init}
\\
\left(\mathbf{0}_{d-1}, \frac{1}{n} \right)^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = g.
\end{cases}
\end{equation*}
Here $\mathbf{0}_d^{\top} = (0,0, \dots, 0)^{\top}$ is a vector of $d$ dimension with all zeros.
Thus, the features $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) \in \mathbb{R}^{nd}$. Moreover, the transition probability parameters are taken as $\boldsymbol{\theta} = \left( \boldsymbol{\theta}^1, \frac{1}{2^{n-1}},  \boldsymbol{\theta}^2, \frac{1}{2^{n-1}} \dots, \boldsymbol{\theta}^n, \frac{1}{2^{n-1}} \right)$ where $\boldsymbol{\theta}^i \in \left\lbrace -\frac{\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}  \right\rbrace^{d-1} $, and $\Delta < \delta$. 

However, these features doesn't capture the following case.

Let $\tb{\ti{s}} = (s, g, g,..., g)$ and  $\tb{\ti{s}}^{\prime} =(s, g, g, ..., s)$. Let's check the probability of transition under an arbitrary global action $\tb{\ti{a}} = (a_1, a_2,...,a_n)$ using the given model: 
\begin{align}
    \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
    \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
    & =\langle \phi((s,g,g,...,s)|(s,g,g,...,g),(a_1, a_2,...a_n)),\theta \rangle \\
    &= \langle (\phi(s|s,a_1), \phi(g|g,a_2),...\phi(s|g,a_n)), (\theta_1, \frac{1}{2^{n-1}}, \theta_2, \frac{1}{2^{n-1}}, ..., \theta_n, \frac{1}{2^{n-1}}) \rangle \\ 
    &= \langle ((-a_1, \frac{1-\delta}{n}), (0_{d-1}, \frac{1}{n}), ..., (0_d)), ( \theta_1, \frac{1}{2^{n-1}}, \theta_2, \frac{1}{2^{n-1}}, ..., \theta_n ,  \frac{1}{2^{n-1}})  \rangle \\
    &= \langle -a_1, \theta_1 \rangle + \frac{1-\delta}{n} . \frac{1}{2^{n-1}} + \frac{1}{n} . \frac{1}{2^{n-1}} . (n-2) + 0 
    \\
    & \neq 0.
\end{align}

Therefore, the above feature design is not capturing the transition probabilities correctly. 

Note that if we use the above feature design along with the condition that $\mathbb{P}(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}) = 0$, if any agent $i$ is transitioning from $s^i = g$ to  $s^{\prime^i} = s_{\text{init}}$. Then, we get the following

\begin{align}
    \sum_{\tb{\ti{s}}^{\prime}} \mathbb{P}(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}) = \frac{r  2^{r-1} 
    + (n-r) 2^r}{n \cdot 2^{n-1}} \neq 1,
\end{align}
where $r$ is total number of agent at $s_{\text{init}}$ in the current state $\tb{\ti{s}}$.

\pt{Utkarsh -- try to see if you can proof the above result, and using this you can adjust your features or the $\boldsymbol{\theta}$ vector.}



..... 

\pt{Here I am copying what you have written Utkarsh in the proofs.}



\dots

\begin{enumerate}
    \item When $\tb{\ti{s}} = \tb{g}$ 
    \begin{enumerate}
        \item $\tb{\ti{s}}^{\prime} = \tb{g}$ \\
        Corresponds to the third case in the definition of global $\phi(.|.,.)$(\ref{eqn:features_global_new})
        \\
        Then, using Assumption \ref{assm:lfa_prob} and features (\ref{eqn:features_global_new}, \ref{eqn:features_global_new_gen}), for any $\tb{\ti{a}} \in \mathcal{A}$
        \begin{align}
        \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
        \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
         & =\langle \phi((g,g,g,\dots,g)|(g,g,g,\dots,g),(a_1, a_2,\dotsa_n)),\boldsymbol{\theta} \rangle \\
         &= \langle (\tb{0}_{nd-1}, 1), (\theta_1, 1, \theta_2, 1, \dots, \theta_n, 1) \rangle \\ 
         &= 1.
        \end{align}   
        \item When $\tb{\ti{s}}^{\prime} \neq \tb{g}$ \\ This implies that there is at least one agent that moves back to node $s$. Corresponds to first part of the second condition in the definition of global $\phi(.|.,.)$ (\ref{eqn:features_global_new}). This takes care of the $2^{n}-1$ impossible transitions for any global action. Using Assumption \ref{assm:lfa_prob} and features (\ref{eqn:features_global_new}, \ref{eqn:features_global_new_gen}) for any global action $\tb{\ti{a}} \in \mathcal{A}$
        \begin{align}
        \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
        \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
        & =\langle \tb{0}_{nd},\theta \rangle \\
        &= 0.
        \end{align}
    \end{enumerate}
    \item When $\tb{\ti{s}} \neq \tb{g}$
        \begin{enumerate}
        \item When there exists some agent who transits from node $g$ to node $s$. This captures all the remaining impossible transitions for any action.
        This corresponds to the "or" part of the second case in the definition of global $\phi(.|.,.)$ (\ref{eqn:features_global_new}). Using Assumption \ref{assm:lfa_prob} and features (\ref{eqn:features_global_new}, \ref{eqn:features_global_new_gen}), for any global action $\tb{\ti{a}} \in \mathcal{A}$
        \begin{align}
        \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
        \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
        & =\langle \tb{0}_{nd},\theta \rangle \\
        &= 0.
        \end{align}
        \item When there exists no agent who transits from node $g$ to node $s$. \\ That means any agent either remains put in its original node (either $s$ or $g$) or only transit from node $s$ to node $g$. This is the most general and the most interesting case. Corner cases are taken care of above.\\
        Consider a general initial state: $\tb{\ti{s}} = (s_1,s_2,\dots,s_n)$ where agents in $\mathcal{I}:=\{i_1, i_2, \dots, i_r \}$ are at node $s$ while agents in $\mathcal{J}:= \{j_1, j_2, \dots, j_{n-r} \}$ are already at node g. Here, we only consider $r \geq 1$ since $r = 0$ is taken care of above. Agents in $\mathcal{I}$ can either stay at node $s$ itself or transit to $g$ while those in $\mathcal{J}$ remain at $g$. Let $\mathcal{S}(\tb{\ti{s}})$ represent the set of all possible next states from $\tb{\ti{s}}$. \\
        Then, using Assumption \ref{assm:lfa_prob} and features (\ref{eqn:features_global_new}), for any $\tb{\ti{a}} = \{a_1,a_2,\dots,a_n\} \in \mathcal{A}$: 
    \begin{align}    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
    &= \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)}\mathbb{P}(({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)| ({s}_1, {s}_2,\dots,{s}_n), ({a}_1, {a}_2,\dots,{a}_n))
    \\ &=\sum_{({s}^{\prime}_1, {s}^{\prime}_2, \dots ,{s}^{\prime}_n)}
    \langle \phi((\ti{s}^{\prime}_1, {s}^{\prime}_2, \dots ,{s}^{\prime}_n)|({s}_1, {s}_2,\dots,{s}_n), ({a}_1, {a}_2,\dots,{a}_n)),(\theta_1, 1, \theta_2, 1, \dots, \theta_n, 1) \rangle \\
    &=\sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)}
    \langle (\phi({s}^{\prime}_1|{s}_1,{a}_1), \phi({s}^{\prime}_2|{s}_2,{a}_2),\dots,\phi({s}^{\prime}_n|{s}_n,{a}_n)),(\theta_1, 1, \theta_2, 1, \dots, \theta_n, 1) \rangle \\
    &= \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)} \sum_{m \in [n]}
    \langle \phi({s}^{\prime}_m|{s}_m,{a}_m),(\theta_m, 1) \rangle 
    \end{align}
    In the below step, we split the summation into two set of agents based on which node they are present at. This helps us later to exploit the similarity in the number of times the local inner product $\langle \phi(s'_i|s_i,a_i),(\theta_i,1)\rangle$ appears in the entire sum. 
    \begin{align}
    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
    &= \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)} \Bigg\{\sum_{i \in \mathcal{I}}
    \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}}
    \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \Bigg \}  \\ 
    &= \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots ,{s}^{\prime}_n)} \sum_{i \in \mathcal{I}}
    \langle \phi(\ti{s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle +  \sum_{({s}^{\prime}_1, {s}^{\prime}_2, \dots ,{s}^{\prime}_n)} \sum_{j \in \mathcal{J}}
    \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle
    \\ 
    &= \sum_{i \in \mathcal{I}} \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)}
    \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle +  \sum_{j \in \mathcal{J}} \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)} 
    \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle
    \\
    &= \sum_{i \in \mathcal{I}} \Big\{  \sum_{{s}^{\prime}_1} \sum_{{s}^{\prime}_2} \dots \sum_{{s}^{\prime}_n} \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle \Big \} + \sum_{j \in \mathcal{J}}  \Big \{  \sum_{{s}^{\prime}_1} \sum_{{s}^{\prime}_2} \dots \sum_{{s}^{\prime}_n} \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \Big \}
    \end{align}
    Since for any $j \in \mathcal{J}, s'_j \equiv g$, 
    \begin{align}
    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
&= \sum_{i \in \mathcal{I}}
 \Big \{     \sum_{{s}^{\prime}_{i_1}} \sum_{{s}^{\prime}_{i_2}} \dots \sum_{{s}^{\prime}_{i_r}} \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle \Big \} +  \sum_{j \in \mathcal{J}}  \Big \{  \sum_{{s}^{\prime}_{i_1}}     \sum_{{s}^{\prime}_{i_2}} \dots
\sum_{{s}^{\prime}_{i_r}} 
    \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \Big \}
    \end{align}
    For any fixed $i \in \mathcal{I},$ the $\sum_{{s}^{\prime}_i}
    \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle $ doesn't depend on next state of other agents in $\mathcal{I}$. Similarly for any $j \in \mathcal{J}, \langle \phi(\ti{s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle $ doesn't depend on next state of any agent in $\mathcal{I}$. Hence,
    \begin{align}
    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
    &=  \sum_{i \in \mathcal{I}} \{2^{r-1}. \sum_{{s}^{\prime}_i}
    \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle \} +  \sum_{j \in \mathcal{J}} \{  2^r. 
    \langle \phi(\ti{s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \}
    \end{align}
    Using features (\ref{eqn:features_global_new_gen})
    \begin{align}
    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
     &= 
     \sum_{i \in \mathcal{I}} \{2^{r-1}. 
    \langle (0_{d-1}, \frac{1}{n.2^{r-1}})),(\theta_i, 1) \rangle \} +  \sum_{j \in \mathcal{J}} \{  2^r.  
    \langle (0_{d-1}, \frac{1}{n.2^{r}}),(\theta_j, 1) \rangle \} 
     \\
     &= 
     \sum_{i \in \mathcal{I}} \frac{1}{n} +  \sum_{j \in \mathcal{J}} \frac{1}{n} 
     \\
     &= \frac{r}{n} + \frac{n-r}{n}
    \\
    & = 1.
    \end{align}
\end{enumerate}


    Since for any $j \in \mathcal{J}, s'_j \equiv g$, 
    \begin{align}
    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
    &= \sum_{i \in \mathcal{I}}
     \Big \{     \sum_{{s}^{\prime}_{i_1}} \sum_{{s}^{\prime}_{i_2}} \dots \sum_{{s}^{\prime}_{i_r}} \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle \Big \} +  \sum_{j \in \mathcal{J}}  \Big \{  \sum_{{s}^{\prime}_{i_1}}     \sum_{{s}^{\prime}_{i_2}} \dots
    \sum_{{s}^{\prime}_{i_r}} 
    \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \Big \}
\end{align}

For any fixed $i \in \mathcal{I},$ the $\sum_{{s}^{\prime}_i}
\langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle $ doesn't depend on next state of other agents in $\mathcal{I}$. Similarly for any $j \in \mathcal{J}, \langle \phi(\ti{s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle $ doesn't depend on next state of any agent in $\mathcal{I}$. Hence,
\begin{align}
    \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) 
    & =  \sum_{i \in \mathcal{I}} \bigg\{2^{r-1} \sum_{{s}^{\prime}_i}
    \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle \bigg\} +  \sum_{j \in \mathcal{J}} \bigg\{  2^r  
    \langle \phi(\ti{s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \bigg\}
\end{align}
Using features in Equation (\ref{eqn:features_global_new_gen})
\begin{align}
    \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \nonumber
     &= 
     \sum_{i \in \mathcal{I}} \bigg\{2^{r-1}. 
    \langle (0_{d-1}, \frac{1}{n.2^{r-1}})),(\theta_i, 1) \rangle \bigg\} +  \sum_{j \in \mathcal{J}} \bigg\{  2^r.  
    \langle (0_{d-1}, \frac{1}{n.2^{r}}),(\theta_j, 1) \rangle \bigg\} 
     \\
     &= 
     \sum_{i \in \mathcal{I}} \frac{1}{n} +  \sum_{j \in \mathcal{J}} \frac{1}{n} 
     \\
     &= \frac{r}{n} + \frac{n-r}{n}
    \\
    & = 1.
\end{align}

It remains to check that individual transition probabilities also lie in $[0,1]$. \\
For the transitions from $\tb{\ti{s}}=\tb{g}$ and other impossible transitions, we saw above that this holds. \\
For general transitions, we check below. \\
Consider any instance $n\geq1,\theta \in \Theta, \delta \in (2/5,1/2), \Delta < 2^{-n}\frac{1-2\delta}{1+n+n^2}$. \\
For any $r \in [n], r' \in [r] \cup \{0\}$, consider any $\tb{\ti{s}} \in \mathcal{S}(r)$, $\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})$ and any action $\tb{\ti{a}} \in \mathcal{A}$.  

\begin{align}
    \Delta & <  \frac{2^{-n} (1-2\delta)}{1+n+n^2} <  \frac{2^{-n} \cdot 2  \delta}{3}
\end{align}

    The above follows since for $\delta \in (2/5,1/2)$, $1-2\delta<2\delta$ and for $n\geq 1, 1+n+n^2 \geq 3$. \\ Further as $r \leq n$, \\
    \begin{align}
    &\delta > 3.2^{n-1}.\Delta \\
    &\implies \delta > 3.2^{r-1}.\Delta \\
    &\Longleftrightarrow \frac{\delta}{2^{r-1}} - 3\Delta>0 \\
    &\Longleftrightarrow \frac{( -0.5n)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta > 0 
    \end{align} 

    Since for any $r \in [n], 0\leq r' \leq r, \delta \in (2/5,1/2)$ we have $r'-0.5r \geq -0.5n$, the above implies: 
    \begin{align}
     &\frac{( r'-0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta > 0 \\
    &\Longleftrightarrow \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} - 3\Delta > 0 
    \end{align}
    Since $r' \leq r \leq n$ we have $\frac{\Delta}{n}(r-2r') \geq -\Delta$. Hence,
    \begin{align}
    &\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') -  \frac{2 \Delta}{1} > 0 \end{align}


    As indicator function can take only $0$ and $1$ values, \\ $\sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \geq -(r-r') \geq -r \geq -n $. \\ Thus, we have, along with the general transition probability expression from \ref{lemma:general_tp},
    \begin{align}
    &\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') \\
    &\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{   \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} > 0 \\
    &\quad \Longleftrightarrow p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'} > 0
\end{align}



Similarly, 
\begin{align}
    &2/5 < \delta < 1/2, \Delta < 2^{-n}.\frac{1-2\delta}{1+n+n^2}, n\geq 1 \\
    &\implies \Delta < 2^{-n} . \frac{2\delta}{3} \\
    &\Longleftrightarrow \delta > 3.2^{n-1}.\Delta \\
    &\implies \delta > 3\Delta \\
    &\Longleftrightarrow 1>1-\delta+3\Delta \\
    &\implies 1> \frac{0.5n(2-2\delta)}{n.2^{r-1}} + 3\Delta \\
    &\implies 1> \frac{(r'-0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} +    3\Delta \\
    &\Longleftrightarrow 1>  \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} +    3\Delta  \\
    &\implies 1> \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{1} \\ 
    &\implies 1>  \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') + \\
    &\quad \frac{2 \Delta}{n(d-1)}\sum_{p \in [d-1]}  \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \\
    &\Longleftrightarrow 1>p^{\tb{\ti{a}}}_{\tb{\ti{s}},{s^\prime}}
\end{align}

Hence, the features described in Equation \eqref{eqn:features_global_new},\ref{eqn:features_global_new_gen} along with the transition probability  (Assumption \ref{assm:lfa_prob}) define valid instances.

\subsection{Proof of Lemma \ref{lemma:general_tp}}

Suppose $\tb{\ti{s}} \in \mathcal{S}\setminus\{\goal\}$ is such that agents at index in $\mathcal{I}:= \{i_1,i_2,\dots, i_r\}$ are at node $s$ and those at $\mathcal{J} := \{j_1,j_2,\dots, j_{n-r}\}$ are already at node $g$. Let agents in $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ be the ones transiting from node $s$ to node $g$ i.e., $\tb{\ti{s}} \in \mathcal{S}(r)$ and $s' \in \mathcal{S}(r')$ where $n \geq r \geq r' \geq 0$ and $n \geq 1$. 

Then using \ref{assm:lfa_prob}: 
\begin{align} 
\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) &= \langle \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}), \theta \rangle \\
&= \langle \phi((s'_1,s'_2,\dots,s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n) ), (\theta_1,1,\theta_2,1,\dots,\theta_n,1)\rangle
\end{align} 
Using Equation \eqref{eqn:features_global_new}, 
\begin{align}
&\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \\
&= \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots, \theta_n,1) \rangle  \\
&= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle \phi(s|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle \phi(g|s,a_t), (\theta_t,1) \rangle \\
\end{align}

Using Equation \eqref{eqn:features_global_new_gen}
\begin{align}
&\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \\
&= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle (-a_i, \frac{1-\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j, 1) \rangle  + \sum_{t \in \mathcal{T}} \langle (a_t, \frac{\delta}{n.2^{r-1}}), (\theta_t,1) \rangle \\
&= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \Big \{ \frac{1-\delta}{n.2^{r-1}} + \langle -a_i, \theta_i \rangle \Big \} + \sum_{j \in \mathcal{J}}   \frac{1}{n.2^{r}}  + \sum_{t \in \mathcal{T}} \Big \{ \langle a_t,\theta_t  \rangle + \frac{\delta}{n.2^{r-1}} \Big \}   \\
&=  r'. \frac{1-\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}  + (r-r'). \frac{\delta}{n.2^{r-1}} + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\
&= \frac{r' + (r-2r')\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}   + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle 
\end{align} 



Since for any $i \in [n], a_i \in \{-1,1\}^{d-1}, \theta_i \in \Big \{ \frac{-\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)} \Big \}^{d-1}$, we have:
\begin{align}
&\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \\
&= \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} a_{i,p}. \theta_{i,p}      + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   a_{t,p} .\theta_{t,p}  \\
&= \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} \\
&\quad - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{\sgn(a_{i,p}) = \sgn(\theta_{i,p})\} -  \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Big \}     \\
&\quad + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{\sgn(a_{t,p}) = \sgn(\theta_{t,p})\} -  \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}  \\
&= \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} \\
&\quad - \sum_{i \in \mathcal{I} \cap \mathcal{T'}}  \frac{\Delta}{n(d-1)} \Big \{  d-1 -  2 \sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Big \}   \\
&\quad + \sum_{t \in \mathcal{T}}    \frac{\Delta}{n(d-1)} \Big \{  d-1 - 2\sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}  \\
&= \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}   \\
&\quad - \frac{\Delta}{n(d-1)} \Big \{  r'(d-1) -  2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Big \}  \\
&\quad +    \frac{\Delta}{n(d-1)} \Big \{  (r-r').(d-1) - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \\
&=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}      \\
&\quad +    \frac{\Delta}{n(d-1)} \Big \{  (r-2r').(d-1) \Big \} + \frac{2\Delta}{n(d-1)}. \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \\
&\quad - \frac{2\Delta}{n(d-1)} . \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \\
&=  \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')  + \\
&\quad \frac{2 \Delta}{n(d-1)}\sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}  -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} 
\end{align}

  


Proof of Claim \ref{claim:probability_inequality}


For any of our instances ($n \geq 1, 2/5< \delta <1/2, \Delta<2^{-n}\frac{1-2\delta}{1+n+n^2}$ ), consider any $r \in [n]$. 

\tb{For $0 \leq r'\leq \lfloor\frac{r+1}{2}\rfloor$}, \\

For any of our instances, 
\begin{align}
& \Delta < \frac{1-2\delta}{2^{n}(1+n+n^2)} 
\\
&\implies \Delta < \frac{1-2\delta}{2^{n} (1+n+\frac{n^2}{8})} \\
&\Longleftrightarrow \Delta (\frac{n^2}{8}+n+1)<\frac{1-2\delta}{2^{n}} 
\end{align}
Since $0 \leq r \leq n,$ we have $\frac{n^2}{8}+n+1 \geq \frac{r^2}{8}+r+1$. \\
Also, $\frac{(r+1)}{2^{r+1}} \geq \frac{1}{2^n}$. \\
As $2/5 < \delta < 1/2$, we have:
\begin{align}
& \frac{\Delta}{n}(\frac{r^2}{8}+r+1)<(r+1)\frac{1-2\delta}{n2^{r+1}} \\
&\Longleftrightarrow \frac{\Delta}{n}\frac{r^2}{8} + (r+1) \frac{\Delta}{n}<(r+1)\frac{1-2\delta}{n2^{r+1}} 
\end{align}
As $0\leq r' \leq r, r'(r-2r') \leq r^2/8$. Thus, \\
\begin{align}
&(r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0 
\end{align}
Since we are considering $0 \leq r' \leq \lfloor\frac{r+1}{2}\rfloor$, we have $\frac{2r'-(r+1)}{2} \leq 0$. \\
Also, since $0 \leq r' \leq r \leq n, \delta \in (2/5,1/2)$, we have $0.5n + (1-2\delta)(r'-0.5r) \geq 0.5n + (1-2\delta)(-0.5r) \geq 0.5n + (1-2\delta)(-0.5n) = n(1-\delta) > 0.$\\
Using above,
\begin{align}
&\Big \{\frac{2r'-(r+1)}{2} \Big \}. \Big \{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}} \Big \} +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0 \\
& \Longleftrightarrow (r+1).\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}\Big\}  + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')< \\
& \quad (r+1-r').\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}} \Big \}    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\
& \Longleftrightarrow  (r+1).\Big \{\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r') \Big \} \\
&  
\quad < (r+1-r').\Big \{ \frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')\Big \}
\\
& \Longleftrightarrow (r+1).\Big\{\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r')\Big\}
\\ 
& \quad < (r+1-r').\Big \{\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n \cdot 2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')\Big \} \\
& \Longleftrightarrow (r+1).\Big \{\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r') \Big \}
\\
& \quad < (r+1-r').\Big \{\frac{r' + (r-2r')\delta}{n \cdot 2^{r-1}} +   \frac{n-r}{n \cdot 2^r}        +    \frac{\Delta}{n}  (r-2r') \Big \} 
\\
& \Longleftrightarrow  \frac{r+1}{r+1-r'}p^*_{r+1,r'}<p^*_{r,r'} \\
& \Longleftrightarrow  \binom{r+1}{r'} p^*_{r+1,r'}
 < \binom{r}{r'}p^*_{r,r'} 
\end{align}
In the last second step, we use the expression for $p^*_{r+1,r'}$ and $p^*_{r,r'}$ from the general transition probability expression in Lemma \ref{lemma:general_tp}. 

Similarly, \\ \tb{For $r' > \lfloor \frac{r+1}{2} \rfloor$}, \\
Again, for any of our instances, we have:
\begin{align}
     \Delta  < \frac{1-2\delta}{(n^2+n+1).2^{n}},  1/2>\delta>2/5 
\end{align}
Since for this range of $\delta$ we have, $1-2\delta < 3\delta-1,$ we obtain:
\begin{align}
      \Delta & < \frac{3\delta-1}{(n^2+n+1).2^{n}} 
      \\
      \Longleftrightarrow & \Delta  (n^2+n+1)  (2^{n})
      < 3\delta-1 
      \end{align}
As $n \geq 1$, using above and $\delta \in (2/5,1/2)$, we have:
\begin{align}
      &n > \frac{0.5-\delta}{2\delta-0.5}+ \frac{\Delta  (n^2+n+1)  (2^{n})}{2\delta-0.5} 
      \\
      \Longleftrightarrow  & (2\delta-0.5)n > 0.5-\delta +  \Delta  (n^2+n+1)  (2^{n}) 
      \\
      \Longleftrightarrow  & 0.5n-n+2n\delta-0.5+\delta >   \Delta  (n^2+n+1)  (2^{n}) 
      \end{align}
      Since for $n \geq 1$ we have $n^2+n+1 \geq n^2-n-1$. Thus:
      \begin{align}
      & (-n-0.5)(1-2\delta)+0.5n    >   \Delta  (n^2-n-1)  (2^{n}) 
      \end{align}
      As $n \geq r, \delta \in (2/5,1/2),$ we have:
      \begin{align}
      & \frac{(-r-0.5)(1-2\delta)+0.5n }{1}   >   \frac{\Delta}{1}  (r^2-r-1)  (2^{r}) \\
      \Longleftrightarrow & \frac{(-r-0.5)(1-2\delta)+0.5n }{n.2^{r}}   >   \frac{\Delta}{n}  (r^2-r-1) 
      \end{align}


     Further since $r \geq r'\geq \lfloor \frac{r+1}{2}\rfloor$, we have $r \cdot r'-2r'^2 \geq -r^2$. \\
      Also, using $\delta \in (2/5,1/2)$,
      \begin{align}
      & \frac{(r'-r-0.5)(1-2\delta)+0.5n }{n \cdot 2^r} +  \frac{\Delta}{n}  (1+r+r \cdot r'-2r'^2)  >0 \\
      \Longleftrightarrow & \frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^r} \\
      & \quad +  \frac{\Delta}{n}  (1+r+r \cdot r'-2r'^2) - 0.5(r+1)(\frac{1-2\delta}{n \cdot 2^r}) >0 \\
      \Longleftrightarrow  & (\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^r}) \\
      & \quad +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n \cdot 2^r} + \frac{\Delta}{n}) >0  \label{}
      \end{align}

      As $r' \geq \lfloor \frac{r+1}{2} \rfloor$, we have $\frac{2r'-(r+1)}{2} \geq 1/2$. Hence, \textcolor{blue}{we can simplify the above,}

      \begin{align}
        & \Big\{\frac{2r'-(r+1)}{2}\Big\}.\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}}\Big\}  \\
      & \quad + (r')\frac{\Delta}{n}  (r-2r') + (r+1)\Big \{\frac{\delta-0.5}{n \cdot 2^r} + \frac{\Delta}{n} \Big\}>0 \\
      \Longleftrightarrow  &  (r+1).\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^r}\Big\} \\
      & \quad + (r+1)\Big\{\frac{\delta-0.5}{n \cdot 2^r} + \frac{\Delta}{n}\Big\}     +    (r+1)\frac{\Delta}{n}  (r-2r')
      \\
      & \quad > (r+1-r').\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}}\Big\}    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\
      \Longleftrightarrow &   (r+1).\Big\{\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n \cdot 2^r}    +    \frac{\Delta}{n}  (r+1-2r')\Big\}
      \\
      & \quad >(r+1-r').\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')\Big\}   \\
      \Longleftrightarrow & (r+1).\Big\{\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n \cdot 2^r}    +    \frac{\Delta}{n}  (r+1-2r')\Big\}
      \\
      & \quad >(r+1-r').\Big\{\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n \cdot 2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')\Big\}  \\
      \Longleftrightarrow &  (r+1).\Big \{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r')\Big\}
      \\
      & \quad >(r+1-r').\Big\{\frac{r' + (r-2r')\delta}{n \cdot 2^{r-1}} +   \frac{n-r}{n \cdot 2^r}        +    \frac{\Delta}{n}  (r-2r')\Big\}
      \\
      \Longleftrightarrow & \frac{r+1}{r+1-r'}p^*_{r+1,r'}>p^*_{r,r'} \\
      \Longleftrightarrow &  \binom{r+1}{r'}p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'} 
\end{align}


\subsection{Proof of Lemma \ref{lemma:probability_inequality}}

\textbf{Recall Lemma \ref{lemma:probability_inequality}:}
\textit{ If for every $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.}

\begin{proof} 
By definition of $V^*,$
\begin{align}
    V^*_r & = 1+\sum_{r'=0}^{r} \binom{r}{r'} p^*_{r,r'} V^*_{r'}, \quad \text{and}
    \\
    V^*_{r+1} &= 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r'=0}^{r}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'}
\end{align}
From the lemma hypothesis, we have
\begin{align}
    \binom{r+1}{r'} p^*_{r+1,r'} 
    &= \binom{r}{r'}p^*_{r,r'}-\delta_{r'}, \quad \forall
    ~~r' \in \{0,1,2,\dots,\lfloor\frac{r+1}{2}\rfloor\},
    \\
    \binom{r+1}{r'} p^*_{r+1,r'}
    & =
    \binom{r}{r'}p^*_{r,r'}+\delta_{r'}, \quad \forall ~~ r' \in \{\lfloor \frac{r+1}{2} \rfloor\ +1 , \lfloor\frac{r+1}{2}\rfloor+2,\dots,r-1,r\}
\end{align}
As Claim \ref{claim:probability_inequality} holds for our instances, \\
suppose for every $r' \in \{0,1,2,\dots,\lfloor\frac{r+1}{2}\rfloor\}$, 
\begin{align}
    \binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}-\delta_{r'} 
\end{align}
and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor\ +1 , \lfloor\frac{r+1}{2}\rfloor+2,\dots,r-1,r\}$, 
\begin{align}
\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}+\delta_{r'}
\end{align}
where $\delta_{r'}>0$ for every $r' \in \{0,1,\dots,r\}$\\ 

Note that, 
\begin{align}
&\sum_{r'=0}^{r+1} \binom{r+1}{r'}p^*_{r+1,r'} = 1 \\
    &\Longleftrightarrow\sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \binom{r+1}{r'}p^*_{r+1,r'} + \sum_{r'=\lfloor \frac{r+1}{2} \rfloor +1}^{r} \binom{r+1}{r'}p^*_{r+1,r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1\\
    &\Longleftrightarrow \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \Big\{\binom{r}{r'}p^*_{r,r'}-\delta_{r'} \Big\} + \sum_{ r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \Big \{ \binom{r}{r'}p^*_{r,r'} + \delta_{r'} \Big\} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\
    &\Longleftrightarrow \sum_{r'=0}^{ \lfloor \frac{r+1}{2} \rfloor} \binom{r}{r'}p^*_{r,r'}-\sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'} + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \binom{r}{r'}p^*_{r,r'} + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\
    &\Longleftrightarrow p^*_{r+1,r+1} = \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'}  -  \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1 }^{ r } \delta_{r'} + 1 -  \sum_{0 \leq r' \leq r} \binom{r}{r'}p^*_{r,r'} \\
    &\Longleftrightarrow p^*_{r+1,r+1} = \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'}  -  \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'} \label{eqn:p_r_r}
\end{align}
Now, going back: 
\begin{align}
&V^*_{r+1}  \\
&=1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' = 0}^r \binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'}  \\
&= 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' = 0}^ {\lfloor \frac{r+1}{2} \rfloor} \binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'}  +  \sum_{r'= \lfloor \frac{r+1}{2} \rfloor +1}^{r}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} \\
&= 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \Big\{\binom{r}{r'}p^*_{r,r'} - \delta_{r'}\Big\}V^*_{r'}  +  \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{ r}\Big\{\binom{r}{r'}p^*_{r,r'}+\delta_{r'} \Big\}V^*_{r'} \\
&= 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' =0}^{ \lfloor \frac{r+1}{2} \rfloor}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' =0}^{ \lfloor \frac{r+1}{2} \rfloor} \delta_{r'} V^*_{r'}  + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \binom{r}{r'}p^*_{r,r'} V^*_{r'}+ \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'}V^*_{r'} \\
&= 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' = 0}^{r} \binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'} V^*_{r'}  +  \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'}V^*_{r'} \\
&=   p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' = 0}^{ \lfloor \frac{r+1}{2} \rfloor} \delta_{r'} V^*_{r'}  +   \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'}V^*_{r'} \\
&> p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'} V^*_{\lfloor \frac{r+1}{2} \rfloor + 1}  +   \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r } \delta_{r'}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} 
\end{align}
The above inequality holds due to induction assumption on monotonicity of $V^*$'s. Thus,
\begin{align}
&V^*_{r+1} \\
&> p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  \Big\{  \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'} - \sum_{r' =  \lfloor \frac{r+1}{2} \rfloor +1}^r \delta_{r'}  \Big\}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\
&= p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ &>  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r 
\end{align}
In the last second step we use the expression for $p^*_{r+1,r+1}$ obtained above \ref{eqn:p_r_r}. The inequality in the last step is due to assumption on monotonicity of $V^*$'s.\\
Thus, combining above with the fact that for our instances for any $r \in [n] \cup \{0\}, p^*_{r+1,r+1} < 1$:
\begin{align}
V^*_{r+1} >   p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r \Longleftrightarrow (1-p^*_{r+1,r+1})(V^*_{r+1}-V^*_r)>0 \Longleftrightarrow V^*_{r+1} > V^*_r
\end{align}

\end{proof}


 \subsection{Proof of Theorem \ref{thm:all_in_one}}

\textbf{Recall the Theorem \ref{thm:all_in_one}:} \pt{To improve the statement. The current statement doesn't look good.} \textit{Consider any instance defined as in (ref). Define global action $\tb{\ti{a}}_{\theta}$ as the action whose $\{(d-1)\times (i-1)+j\}^{th}$ element for every $i \in [n]$ and every $j \in [d-1]$ is given by $\sgn(\theta_{i,j})$. \pt{The following holds simultaneously.}
\begin{itemize}
    \item Then the policy of taking action $\tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$, is optimal. 
    \item Further, optimal value function for each state with the same number of agents at node $s$ takes the same value, i.e., suppose for every $r \in [n]$, $\mathcal{S}(r)$ denotes the set of all states with any $r$ agents at node $s$ and remaining $n-r$ agents at $g$. Then, $V^*(s) = V^*_r(constant)$ for all $s \in \mathcal{S}(r)$. We define $V^*_0=0$.
    \item There exists increasing monotonicity of optimal value function with the number of agents at node $s$ i.e., $0=V^*_0<V^*_1<V^*_2\dots<V^*_n = B^*$. 
\end{itemize}}
    

\begin{proof}
\tb{Base Case}  \\ By definition, $V^*_0 = 0$. \\
Take any $\tb{\ti{s}} \in \mathcal{S}(1)$. \\
We wish to find the optimal action in this state.\\
From $\tb{\ti{s}}$, only possible next global states are $\tb{\ti{s}}$ itself and the global goal state ($goal =\tb{g} = (g,g,g,\dots,g)$). This is akin to the single agent problem. But now, any transition probability also depends on actions of others. \\
Suppose $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$ denotes the transition probability from \tb{\ti{s}} to \tb{g} for any $\tb{\ti{a}} \in \mathcal{A}$. Then the value of this action at $\tb{\ti{s}}$ can be expressed as:  \\
$V^{\tb{\ti{a}}}(\tb{\ti{s}}) = (1-p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}).(1+V^{\tb{\ti{a}}}(\tb{\ti{s}})) + p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}.(1+V_0) \implies V^{\tb{a}}(\tb{\ti{s}}) = \frac{1}{p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}}$ \\
Thus, the optimal action at \tb{\ti{s}} is the one that minimizes $V^{\tb{a}}_1(\tb{\ti{s}})$ i.e., maximizes $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$. From the expression of general transition probability in Lemma \ref{lemma:general_tp}, the transition probability is maximum when $\tb{\ti{a}}$ is such that it matches all signs with $\theta$ at the respective components of agent who was initially at node $s$ in $\tb{\ti{s}}$. The signs of other components do not matter. Hence, there could be multiple optimal actions $\tb{\ti{a}}^*$ for any particular $\tb{\ti{s}} \in \mathcal{S}(1)$. \\
Notice that the above analysis holds for any $\tb{\ti{s}} \in \mathcal{S}(1)$. Note that the particular action $\tb{\ti{a}}_{\theta}$ each of whose components' sign matches with respective components of $\theta$ (as defined in theorem \ref{thm:all_in_one}), is common for possible optimal actions for every $\tb{\ti{s}} \in \mathcal{S}(1)$. We consider this $\tb{\ti{a}}^*=\tb{\ti{a}}_{\theta}$ in particular. \\
From Corollary \ref{corollary:p_star}, $p^{\tb{\ti{a}}^*}_{\tb{\ti{s}},\tb{g}} = p^{\tb{\ti{a}}^*} \forall \tb{\ti{s}} \in \mathcal{S}(1)$. Thus $V^*(\tb{\ti{s}}) = V^*_1 \forall \tb{\ti{s}} \in \mathcal{S}(1)$ \\
Clearly, $V^*_1 = \frac{1}{p^*_{\tb{\ti{s}},\tb{g}}}>0= V^*_0$ \\
Hence, all the three claims of Theorem \ref{thm:all_in_one} hold for the base case.\\
\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:
\begin{itemize}
    \item The optimal action $\tb{\ti{a}}^*$ is the one that matches sign at all components with $\theta$ (i.e., $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$) for any state in $\mathcal{S}(k)$. This implies from Corollary \ref{corollary:p_star} that, $p^*(\tb{\ti{s}} \in \mathcal{S}(k)  \xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})) = p^*_{k,k'}$, where $\tb{\ti{s}}' \in \mathcal{S}(k')$ for any $k' \in \{0,1,2,\dots,k\}$.
    \item $V^*_k(\tb{\ti{s}})=V^*_k$ for all $\tb{\ti{s}} \in \mathcal{S}(k)$
    \item $V^*_k>V^*_{k-1}>\dots>V^*_0 = 0$
\end{itemize}
Now, we need to show the same three claims hold for $r+1$. \\
Consider any $\tb{\ti{s}} \in S(r+1)$. \\
We again want to know what's the optimal action in this state. We know the optimal action in all the other states that can be reached from $\tb{\ti{s}}$. Hence, we consider the value of any action $\tb{a} \in \mathcal{A}$ in $\tb{\ti{s}}$ as follows (This is the same as $Q^*(\tb{\ti{s}},\tb{a})$ in most literature):
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}}) \\
&= \sum_{\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}}) \setminus \{\tb{\ti{s}},\tb{g}\}} \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}})\{1+V^*(\tb{\ti{s}}')\} + \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^{\tb{\ti{a}}}(\tb{\ti{s}})\} + \mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^*(\tb{g})\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +\sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'}V^*_{r'} 
\end{align}
Using general expression for transition probability from Lemma \ref{lemma:general_tp}:
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}})\\
&= 1+ \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) \\
&\quad +  \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Bigg\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^\tb{\ti{a}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}  \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} + \\
&\quad   \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \sum_{i \in [n]} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)} \times \\
&\quad  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{ \Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'} \Bigg \}  +  \\ 
&\quad \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  + \frac{\Delta}{n(d-1)} 
 \times \\
&\quad \Bigg\{  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Big \} + \\
&\quad \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \} \Bigg\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^a({\tb{\ti{s}}} +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
 &\quad \sum_{r' \in [r]}  \Bigg\{\Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}.V^*_{r'} \Bigg \}  \\
&\quad +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Big \} \\
&\quad + \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{  \{ \binom{r}{r'}  - \binom{r}{r'-1} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        + \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  +   \\
&\quad \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Big  \}
\end{align}

Observe that the term inside the summation is always non negative since when $r' \geq r/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} \geq V^*_{r+1-r'}$ while for $r' \leq r/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_{r+1-r'}$ due to property of Binomial coefficients and the Induction assumption of monotonicity of $V^*$ . Note that the above argument is for $r' \in [r]$. \\
To minimize $V^{\tb{\ti{a}}}(\tb{\ti{s}})$, we need to minimize $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well (check after rearrangement as it will appear in denominator as $1-\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$). \\
Clearly, the action that matches sign with all components of $\theta$ (i.e., $\tb{\ti{a}}_{\theta}$) minimizes $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well as makes the sum of non-negative terms the minimum i.e., $0$. Hence, it minimizes $V^\tb{\ti{a}}(\tb{\ti{s}})$. Hence this action $\tb{\ti{a}}_{\theta}$ is the optimal action $\tb{\ti{a}}^*$. \\
Notice the above argument holds for any $ \tb{\ti{s}} \in \mathcal{S}(r+1)$. Hence $\tb{\ti{a}}^*$ is the same for each of them. \\
Again, by Corollary \ref{corollary:p_star}, $p^*(\tb{\ti{s}} \in \mathcal{S}(\tb{\ti{s}})\xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})) = p^*_{r+1,r'}$ for any $r' \in [r] \cup \{0\}$. \\
Thus, $V^*(\tb{\ti{s}}) = V^*_{r+1}$ for any $\tb{\ti{s}} \in \mathcal{S}(r+1)$. \\
Using the induction assumption combined with this result, Claim \ref{claim:probability_inequality} and Lemma \ref{lemma:probability_inequality}, we have $V^*_{r+1}>V^*_r$. \\
Hence by induction, all three claims of the theorem hold.
\end{proof}


\begin{proof}
\tb{Base Case}  

By definition, $V^*_0 = 0$.

Take any $\tb{\ti{s}} \in \mathcal{S}(1)$. \\
We wish to find the optimal action in this state.\\
From $\tb{\ti{s}}$, only possible next global states are $\tb{\ti{s}}$ itself and the global goal state ($goal =\tb{g} = (g,g,g,\dots,g)$). This is akin to the single agent problem. But now, any transition probability also depends on actions of others. \\
Suppose $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$ denotes the transition probability from \tb{\ti{s}} to \tb{g} for any $\tb{\ti{a}} \in \mathcal{A}$. Then the value of this action at $\tb{\ti{s}}$ can be expressed as:  \\
$V^{\tb{\ti{a}}}(\tb{\ti{s}}) = (1-p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}).(1+V^{\tb{\ti{a}}}(\tb{\ti{s}})) + p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}.(1+V_0) \implies V^{\tb{a}}(\tb{\ti{s}}) = \frac{1}{p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}}$ \\
Thus, the optimal action at \tb{\ti{s}} is the one that minimizes $V^{\tb{a}}_1(\tb{\ti{s}})$ i.e., maximizes $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$. From the expression of general transition probability in Lemma \ref{lemma:general_tp}, the transition probability is maximum when $\tb{\ti{a}}$ is such that it matches all signs with $\theta$ at the respective components of agent who was initially at node $s$ in $\tb{\ti{s}}$. The signs of other components do not matter. Hence, there could be multiple optimal actions $\tb{\ti{a}}^*$ for any particular $\tb{\ti{s}} \in \mathcal{S}(1)$. \\
Notice that the above analysis holds for any $\tb{\ti{s}} \in \mathcal{S}(1)$. Note that the particular action $\tb{\ti{a}}_{\theta}$ each of whose components' sign matches with respective components of $\theta$ (as defined in theorem \ref{thm:all_in_one}), is common for possible optimal actions for every $\tb{\ti{s}} \in \mathcal{S}(1)$. We consider this $\tb{\ti{a}}^*=\tb{\ti{a}}_{\theta}$ in particular. \\
From Corollary \ref{corollary:p_star}, $p^{\tb{\ti{a}}^*}_{\tb{\ti{s}},\tb{g}} = p^{\tb{\ti{a}}^*} \forall \tb{\ti{s}} \in \mathcal{S}(1)$. Thus $V^*(\tb{\ti{s}}) = V^*_1 \forall \tb{\ti{s}} \in \mathcal{S}(1)$ \\
Clearly, $V^*_1 = \frac{1}{p^*_{\tb{\ti{s}},\tb{g}}}>0= V^*_0$ \\
Hence, all the three claims of Theorem \ref{thm:all_in_one} hold for the base case.\\
\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:
\begin{itemize}
    \item The optimal action $\tb{\ti{a}}^*$ is the one that matches sign at all components with $\theta$ (i.e., $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$) for any state in $\mathcal{S}(k)$. This implies from Corollary \ref{corollary:p_star} that, $p^*(\tb{\ti{s}} \in \mathcal{S}(k)  \xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})) = p^*_{k,k'}$, where $\tb{\ti{s}}' \in \mathcal{S}(k')$ for any $k' \in \{0,1,2,\dots,k\}$.
    \item $V^*_k(\tb{\ti{s}})=V^*_k$ for all $\tb{\ti{s}} \in \mathcal{S}(k)$
    \item $V^*_k>V^*_{k-1}>\dots>V^*_0 = 0$
\end{itemize}
Now, we need to show the same three claims hold for $r+1$. \\
Consider any $\tb{\ti{s}} \in S(r+1)$. \\
We again want to know what's the optimal action in this state. We know the optimal action in all the other states that can be reached from $\tb{\ti{s}}$. Hence, we consider the value of any action $\tb{a} \in \mathcal{A}$ in $\tb{\ti{s}}$ as follows (This is the same as $Q^*(\tb{\ti{s}},\tb{a})$ in most literature):
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}}) \\
&= \sum_{\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}}) \setminus \{\tb{\ti{s}},\tb{g}\}} \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}})\{1+V^*(\tb{\ti{s}}')\} + \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^{\tb{\ti{a}}}(\tb{\ti{s}})\} + \mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^*(\tb{g})\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +\sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'}V^*_{r'} 
\end{align}
Using general expression for transition probability from Lemma \ref{lemma:general_tp}:
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}})\\
&= 1+ \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) \\
&\quad +  \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Bigg\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^\tb{\ti{a}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}  \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} + \\
&\quad   \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \sum_{i \in [n]} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)} \times \\
&\quad  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{ \Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'} \Bigg \}  +  \\ 
&\quad \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  + \frac{\Delta}{n(d-1)} 
 \times \\
&\quad \Bigg\{  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Big \} + \\
&\quad \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \} \Bigg\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^a({\tb{\ti{s}}} +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
 &\quad \sum_{r' \in [r]}  \Bigg\{\Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}.V^*_{r'} \Bigg \}  \\
&\quad +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Big \} \\
&\quad + \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{  \{ \binom{r}{r'}  - \binom{r}{r'-1} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        + \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  +   \\
&\quad \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Big  \}
\end{align}

Observe that the term inside the summation is always non negative since when $r' \geq r/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} \geq V^*_{r+1-r'}$ while for $r' \leq r/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_{r+1-r'}$ due to property of Binomial coefficients and the Induction assumption of monotonicity of $V^*$ . Note that the above argument is for $r' \in [r]$. \\
To minimize $V^{\tb{\ti{a}}}(\tb{\ti{s}})$, we need to minimize $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well (check after rearrangement as it will appear in denominator as $1-\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$). \\
Clearly, the action that matches sign with all components of $\theta$ (i.e., $\tb{\ti{a}}_{\theta}$) minimizes $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well as makes the sum of non-negative terms the minimum i.e., $0$. Hence, it minimizes $V^\tb{\ti{a}}(\tb{\ti{s}})$. Hence this action $\tb{\ti{a}}_{\theta}$ is the optimal action $\tb{\ti{a}}^*$. \\
Notice the above argument holds for any $ \tb{\ti{s}} \in \mathcal{S}(r+1)$. Hence $\tb{\ti{a}}^*$ is the same for each of them. \\
Again, by Corollary \ref{corollary:p_star}, $p^*(\tb{\ti{s}} \in \mathcal{S}(\tb{\ti{s}})\xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})) = p^*_{r+1,r'}$ for any $r' \in [r] \cup \{0\}$. \\
Thus, $V^*(\tb{\ti{s}}) = V^*_{r+1}$ for any $\tb{\ti{s}} \in \mathcal{S}(r+1)$. \\
Using the induction assumption combined with this result, Claim \ref{claim:probability_inequality} and Lemma \ref{lemma:probability_inequality}, we have $V^*_{r+1}>V^*_r$. \\
Hence by induction, all three claims of the theorem hold.
\end{proof}


\section{Notations and Prelims}

..... \pt{Your writeup starts here.}

A general Multi-Agent Stochastic Shortest Path (MA-SSP) problem is defined as $(\mathcal{V}, N, \mathbb{P}, \mathcal{A})$. Here $\mathcal{V} \coloneqq
\{v_1,v_2,v_3,\dots,v_q\}$ is the set of nodes. $N=\{1,2,\dots,n\} = [n]$ is the set of agents.  
At any instant, each agent can be at exactly one node in $\mathcal{V}$. We represent the global state of the system by $\tb{\ti{s}} = \{s_1,s_2,\dots,s_{n}\}$ where for every agent $i \in N$, $s_i \in \mathcal{V}$ represents the node where the agent $i$ is present. 
Hence, the set of all possible states $\mathcal{S}$ is $\Pi_{i=1}^{n}\mathcal{V}= \mathcal{V}^n$. At time step, each agent can take an action. We assume that the set of actions available for any agent $i \in [n]$, namely $\mathcal{A}^i$ is independent of the node at which it is present.
We represent the global action $\tb{\ti{a}} = \{a_1,a_2,\dots,a_n\}$ where for every $i \in N,a^i \in \mathcal{A}^i$ represents the action taken by the agent $i$. 
Hence, the set of all actions possible at any state $\tb{\ti{s}} \in \mathcal{S}$ is $\mathcal{A}=\Pi_{i=1}^n \mathcal{A}^i$. At any state $\tb{\ti{s}} \in \mathcal{S}$, if action $\tb{\ti{a}}$ is taken, then each agent $i \in N$ incurs a cost $c^i(\tb{\ti{s}},\tb{\ti{a}})$ which in general is a random variable, in that instant where,  $0<c_{\min} \leq c^i(\tb{\ti{s}},\tb{\ti{a}})\leq 1$. Note that individual cost depends on global state and global action. This model encapsulates complexities arising due to multi-agent setup. 

We show below how congestion can be modeled and incorporated in this framework. Suppose for any agent $i \in N, \tb{\ti{s}} = (s_1,s_2,\dots,s_n) \in \mathcal{S}, \tb{\ti{a}} = (a_1,a_2,\dots,a_n) \in \mathcal{A}$, $K^i(\tb{\ti{s}},\tb{\ti{a}})$ denotes the cost to the agent $i$ due to private efficiency and all other complex multi-agent interdependencies except congestion. Congestion can be modeled by considering the total number of agents who take the same actions. We define Congestion Factor:
\begin{align}
    c_f^i(\tb{\ti{s}},\tb{\ti{a}}) = \sum_{j=1}^n \mathbbm{1}\{a_j = a_i\}
\end{align}
Thus, we model the cost to agent $i \in N$  as 
\begin{align} \label{eqn:ind_cost}
    c^i(\tb{\ti{s}},\tb{\ti{a}}) = c_f^i(\tb{\ti{s}},\tb{\ti{a}}) \times K^i(\tb{\ti{s}},\tb{\ti{a}})=\sum_{j=1}^n \mathbbm{1}\{a_j = a_i\}.K^i(\tb{\ti{s}},\tb{\ti{a}})
\end{align}
We define the global cost (to the system) as the average of individual costs i.e., 
\begin{align} \label{eqn:glb_cost}
c(\tb{\ti{s}},\tb{\ti{a}}) = \frac{1}{n}\sum_{i=1}^n c^i(\tb{\ti{s}},\tb{\ti{a}}) = \frac{1}{n}\sum_{i=1}^n c^i_f(\tb{\ti{s}}, \tb{\ti{a}}) \times K^i(\tb{\ti{s}},\tb{\ti{a}})  = \frac{1}{n}\sum_{i=1}^n \Bigg \{\sum_{j=1}^n \mathbbm{1}\{a_j = a_i\} \Bigg \}\times K^i(\tb{\ti{s}},\tb{\ti{a}}) 
\end{align}
\pt{congestion} \textcolor{red}{i've added some discussion on congestion above}
The environment also responds with a next state $\tb{\ti{s}}^\prime$ sampled according to a probability distribution depending on $\tb{\ti{s}}$ and $\tb{\ti{a}}$ i.e., $\tb{\ti{s}}^\prime \sim \mathbb{P}(.|\tb{\ti{s}},\tb{\ti{a}})$. 
This captures that in the multi-agent set up, the next state of any agent is also influenced by state and action of other players. 
In planning setting, the cost function and the transition probability function is known. While in learning setting, atleast one of the two is unknown. \\
Finally, we define a policy($\pi$) as a \ti{scheme} of taking actions in various states. 

\pt{In our setup} -- Given an ordered pair of states $(\tb{\ti{s}}_\init, \tb{g}) \in \mathcal{S} \times \mathcal{S}\setminus\tb{g}$, the problem is to find the best policy ($\pi^*$) to reach state $\tb{g}$ starting from  $\tb{\ti{s}}_\init$ in a cumulative global cost minimization sense. Due to stochastic costs and transition dynamics, one can only evaluate policies in terms of their expected behavior. The most general way is to consider the set of all history-dependent randomized policies $\Pi = \{\pi:\mathcal{H}\xrightarrow{}\Delta(\mathcal{A})\}$, where each policy $\pi$ is a mapping from the set of all histories $\mathcal{H}$ to the set of all probability distributions over global actions $\Delta(\mathcal{A})$. 

Due to Markovian and stationary transition and cost structure,
it is sufficient to consider policies in the Markov and Deterministic space to find the optimal policy(\textcolor{red}{can this statement be made better?}cite). Even then, there may be "bad" policies which do not lead to \tb{g} almost surely. We call these as improper policies. On the other hand, those policies that lead to \tb{g} almost surely are said to be proper. We further assume that the set of proper policies ($\Pi_p$) is non-empty (\textcolor{red}{should this be written under begin assumption? or this is ok?}). 
For any policy $\pi \in \Pi$, we define for any state $\tb{\ti{s}} \in \mathcal{S}$, the expected long-term cost as:
\begin{align}
    V^{\pi}(\tb{\ti{s}}) = \mathbb{E}[c(\tb{\ti{s}}_1,\pi(\tb{\ti{s}}_1))+c(\tb{\ti{s}}_2,\pi(\tb{\ti{s}}_2))+\dots|\tb{\ti{s}}_1=\tb{\ti{s}}]
\end{align}
where $\tb{\ti{s}}_{t+1} \sim \mathbb{P}(.|s_t,\pi(s_t))$  for time steps $t=1,2, \cdots$. In general, the expectation is due to randomized action due to policy, stochastic cost and transition dynamics. For an improper policy \pt{what is improper policy?}, the above becomes unbounded for at least one state. However, for any proper policy the summation inside the expectation almost surely has random but finite bounded terms and thus the expectation becomes overall bounded.  
Restricting to proper policies ($\Pi_{p}$), planning version of the MASSP problem can be expressed as the following: 
\begin{align}
    \pi^* = \arg \min_{\pi \in \Pi_p} V^\pi(\tb{\ti{s}}_{init})
\end{align}
We define diameter $B^*$ of any MA-SSP problem as: 
\begin{align}
    B^* = \max_{\tb{\ti{s}}\in \mathcal{S}}V^*(\tb{\ti{s}})
\end{align}
In learning setting, due to the lack of knowledge of cost and transition probability functions, one needs to \textit{sufficiently} explore all state-action pairs while ensuring that the best policy is learned over time and actions are taken according to it. 
As we wish to learn the best policy to navigate from one state to the another, any MASSP learning algorithm is run over multiple episodes all starting at $\tb{\ti{s}}_{init}$ and ending at $goal$. 

The learnability of an MASSP learning algorithm $\mathfrak{A}$ is thus characterized by the notion of cumulative regret over $K$ episodes in hindsight. It is a measure of the difference between the expected long term cost of chosing actions as prescribed by the algorithm and that by choosing actions according to the optimal policy.  Suppose, $h_1,h_2,\dots,h_k$ represent the random variables representing the length of episodes $1,2,\dots,K$ respectively. Then, expected cumulative regret of the algorithm is defined as: \pt{regret of policy}
\begin{align}\label{eqn:regret}
    \mathbb{E}_{\mathfrak{A}}[R(K)] = \mathbb{E} \Bigg \{ \sum_{k=1}
^{K}\sum_{h=1}^{h_k} c(\tb{\ti{s}}_{k,h},\tb{\ti{a}}_{k,h}) \Bigg \} - K.V^*(s_{init}) \end{align}
where $\tb{\ti{s}}_{k,h}$ and $\tb{\ti{a}}_{k,h}$ respectively denote the random variables associated with state and action at the $h^{th}$ step in the $k^{th}$ episode. 

... \pt{Your writeup ends here}



\subsection{Related Works}\label{subsec:relatedwork}

\begin{itemize}
    \item Planning SSP: Bertsekas, Tsitsiklis, Guillot,..
    \item Learning SSP 1 agent - \\Tabular: Tarbouriech, Cohen, Rosenberg, \\Linear Mixture SSP: Min et al (Closest to our work), Vial .
    \item Learning SSP Multi-Agent : Trivedi and Hemachandra.
    \item Dec-MARL : Zhang
\end{itemize}


\section{Proof of Thm 1}

\pt{the above thing is not for the induction -- want to show for the types of r=1 to n -- need to mention though about r=0. the episode ends at g. eqn 120 is for r=1, not from r=0. thus, we have that eqn for r=1. by defn we have V=0. base case to be taken as r=1,}
    



This completes the base case.
        

=== 

\pt{Now assume that it is true for all r upto k. , and then prove it for r = k+1. }


for r=1 , claim 1,2,3, holds,  ==>  r=2, claim 1,2,3 holds, ==-=> r=k, claim 1, 2, 3 holds.. Then first we need to prove that claim 1 holds for r= k+1, then using this claim, --- prove claim 2, and then prove claim 3...



===

   

\end{proof}



\begin{proof}
    We will prove this result using the principle of Mathematical induction on $r$.  First we consider the base case $r = 0$.

\paragraph{Base case: $r=0, \mathcal{S}(0)$. -- better to start from $\mathcal{S}(1)$.} 


\pt{All the agents are at goal  node. Hence, any policy is optimal. so claim 1 holds be default. since their is only one state of type $r=0$, the second claim holds. The third claim holds by definition. }




By definition, we have $V^*_0 = 0$. For any state $\tb{\ti{s}} \in \mathcal{S}(1)$, we would like to find the optimal action in this state.  From $\tb{\ti{s}}$ the only possible next global states are $\tb{\ti{s}}$ itself and the global goal state $\tb{\ti{g}} = (g, \dots ,g)$. This is akin to the single agent problem, however, the transition probability  depends on actions of others. Suppose $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$ denotes the transition probability from \tb{\ti{s}} to \tb{g} for any $\tb{\ti{a}} \in \mathcal{A}$. Then the value of this action at $\tb{\ti{s}}$ can be expressed as
% 
\begin{align}
    V^{\tb{\ti{a}}}(\tb{\ti{s}}) = (1-p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}) \cdot (1+V^{\tb{\ti{a}}}(\tb{\ti{s}})) + p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}} \cdot (1+V_0)
    \quad \implies V^{\tb{a}}(\tb{\ti{s}}) = \frac{1}{p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}}.
\end{align}
\pt{this is $Q(s,a)$. }

Thus, the optimal action at $\tb{\ti{s}}$ is the one that minimizes $V^{\tb{a}}_1(\tb{\ti{s}})$ i.e., maximizes $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$.

From the expression of general transition probability in Lemma \ref{lemma:general_tp}, the transition probability is maximum when $\tb{\ti{a}}$ is such that it matches all signs with $\theta$ at the respective components of agent who was initially at node $s$ in $\tb{\ti{s}}$. The sign of other components do not matter. Hence, there could be multiple optimal actions $\tb{\ti{a}}^*$ for any particular $\tb{\ti{s}} \in \mathcal{S}(1)$.

\pt{we can write the exact expression of the probability again here. This will make it more clear. Explain this part abut indicators.}



Notice that the above analysis holds for any $\tb{\ti{s}} \in \mathcal{S}(1)$. Note that the particular action $\tb{\ti{a}}_{\theta}$ each of whose components' sign matches with respective components of $\theta$ (as defined in theorem \ref{thm:all_in_one}), is common for possible optimal actions for every $\tb{\ti{s}} \in \mathcal{S}(1)$.

We consider this as $\tb{\ti{a}}^*=\tb{\ti{a}}_{\theta}$ in particular. 



\pt{all the states of same type has the same optimal action. This is equivalent to the threshold type policies -- to think and write more in this direction. We  partition the state space, and in each partition we have clarity about what is optimal action -- sign mathcing property.}

From Corollary \ref{corollary:p_star}, $p^{\tb{\ti{a}}^*}_{\tb{\ti{s}},\tb{g}} = p^{\tb{\ti{a}}^*} \forall \tb{\ti{s}} \in \mathcal{S}(1)$. Thus 
\begin{align}
    V^*(\tb{\ti{s}}) = V^*_1, \quad ~ \forall ~ \tb{\ti{s}} \in \mathcal{S}(1)
\end{align}
Clearly, $V^*_1 = \frac{1}{p^*_{\tb{\ti{s}},\tb{g}}}>0= V^*_0$. \pt{So, the vlues are same for all states in $\mathcal{S}(1)$. }

\pt{I do not understand the above proof. Can you explain it in more details. }

\pt{Why we suddenly mentioned that all the claims are true? It's not clear to me.}

This proves that all the three claims of Theorem \ref{thm:all_in_one} hold for the base case. 



\end{proof}

...

\begin{proof}
\tb{Base Case}  

\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:
\begin{itemize}
    \item The optimal action $\tb{\ti{a}}^*$ is the one that matches sign at all components with $\theta$ (i.e., $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$) for any state in $\mathcal{S}(k)$. This implies from Corollary \ref{corollary:p_star} that, $p^*(\tb{\ti{s}} \in \mathcal{S}(k)  \xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})) = p^*_{k,k'}$, where $\tb{\ti{s}}' \in \mathcal{S}(k')$ for any $k' \in \{0,1,2,\dots,k\}$.
    \item $V^*_k(\tb{\ti{s}})=V^*_k$ for all $\tb{\ti{s}} \in \mathcal{S}(k)$
    \item $V^*_k>V^*_{k-1}>\dots>V^*_0 = 0$
\end{itemize}
Now, we need to show the same three claims hold for $r+1$. \\
Consider any $\tb{\ti{s}} \in S(r+1)$. \\
We again want to know what's the optimal action in this state. We know the optimal action in all the other states that can be reached from $\tb{\ti{s}}$.

\pt{upto $r$, reachable ... }

Hence, we consider the value of any action $\tb{a} \in \mathcal{A}$ in $\tb{\ti{s}}$ as follows (This is the same as $Q^*(\tb{\ti{s}},\tb{a})$ in most literature):
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}}) \\
&= \sum_{\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}}) \setminus \{\tb{\ti{s}},\tb{g}\}} \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}})\{1+V^*(\tb{\ti{s}}')\} + \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^{\tb{\ti{a}}}(\tb{\ti{s}})\} + \mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^*(\tb{g})\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +\sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'}V^*_{r'} 
\end{align}

\pt{let us write the english explanation of the last term.. Now focus on third term.}


Using general expression for transition probability from Lemma \ref{lemma:general_tp}:
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}})\\
&= 1+ \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) \\
&\quad +  \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Bigg\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^\tb{\ti{a}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}  \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} 
\end{align}
The last line follows from observing that for fixed $r'$, the inner summation over $s'$ in line 127 is just the sum of $|\mathcal{S}(
r')(\tb{\ti{s}})| = \binom{r+1}{r'}$ terms and the outer summations are taken in side for the term in eqn128.\\
In the below, we alternatively represent the summation over sets $\mathcal{I} \cap \mathcal{T}$ and $\mathcal{T}$ as an appropriate summation over $\mathcal{I}$ and in the next step, we take the $V^*(.)$ factor inside and take the summation over two terms:
\begin{align}
&V^a(\tb{\ti{s}})  \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} + \\
&\quad   \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \sum_{i \in \mathcal{I}} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)} \times \\
&\quad  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{ \Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'} \Bigg \}  +  \\ 
&\quad \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} 
\end{align}
In the last step, we identified that for every agent $i \in \mathcal{I}$ for a fixed $r'$ the number of states in $\mathcal{S}(r')(\tb{\ti{s}})$ in which it stays at node $s$ itself is $\binom{r}{r'-1}$ and those in which it transits to node $g$ is $\binom{r}{r'}$. \\
In the immediate below step, we use $\sum_{a \in [m]} f(a) = \sum_{a \in [m]} f(1+m-a)$ for any function $f(.)$ and natural number $m$. (Here, the part of eqn 141 inside the summations over $p$ and $i$ is our $f$, $ a$ is $r'$ and $m$ is $r$.) In the next few steps, we simplify the expression using properties of binomial coefficients and simplify: 
\begin{align} 
&V^a(\tb{\ti{s}}) \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  + \frac{\Delta}{n(d-1)} 
 \times \\
&\quad \Bigg\{  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Big \} + \\
&\quad \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \} \Bigg\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^a({\tb{\ti{s}}} +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
 &\quad \sum_{r' \in [r]}  \Bigg\{\Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}.V^*_{r'} \Bigg \}  \\
&\quad +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Bigg \{ \Big \{ \binom{r}{r'-1}  - \binom{r}{r'} \Big \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Bigg \} \\
&\quad + \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Bigg \{ \Big \{ \binom{r}{r'}  - \binom{r}{r'-1} \Big \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Bigg  \}  \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        + \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  +   \\
&\quad \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Bigg \{ \Big\{ \binom{r}{r'-1}  - \binom{r}{r'} \Big \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Bigg \}
\end{align}
\pt{We identified the partitions based on the type, the action is common. }

\pt{Sum over r' is written in terms of binomials -- in how many states of type r', reach from s, agent i is not transiting or transiting, respectively.}

\pt{sum backward.. rather than forward.}

Observe that the term inside the summation is always non negative since when $r' \geq r/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} \geq V^*_{r+1-r'}$ while for $r' \leq r/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_{r+1-r'}$ due to property of Binomial coefficients and the Induction assumption of monotonicity of $V^*$ . Note that the above argument is for $r' \in [r]$. \\
To minimize $V^{\tb{\ti{a}}}(\tb{\ti{s}})$, we need to minimize $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well (check after rearrangement as it will appear in denominator as $1-\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$). \\
Clearly, the action that matches sign with all components of $\theta$ (i.e., $\tb{\ti{a}}_{\theta}$) minimizes $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well as makes the sum of non-negative terms the minimum i.e., $0$. Hence, it minimizes $V^\tb{\ti{a}}(\tb{\ti{s}})$. Hence this action $\tb{\ti{a}}_{\theta}$ is the optimal action $\tb{\ti{a}}^*$. \\
Notice the above argument holds for any $ \tb{\ti{s}} \in \mathcal{S}(r+1)$. Hence $\tb{\ti{a}}^*$ is the same for each of them. \\
Again, by Corollary \ref{corollary:p_star}, $p^*(\tb{\ti{s}} \in \mathcal{S}(\tb{\ti{s}})\xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})) = p^*_{r+1,r'}$ for any $r' \in [r] \cup \{0\}$. \\
Thus, $V^*(\tb{\ti{s}}) = V^*_{r+1}$ for any $\tb{\ti{s}} \in \mathcal{S}(r+1)$. \\
Using the induction assumption combined with this result, Claim \ref{claim:probability_inequality} and Lemma \ref{lemma:probability_inequality}, we have $V^*_{r+1}>V^*_r$. \\
Hence by induction, all three claims of the theorem hold.





\pt{Why this part is written here, need to be written in prelims or the introduction.} \textcolor{red}{removed from here and placed into introduction}
\textcolor{red}{The transition from single agent SSP to Multi-Agent SSP, leads to the following complications: 
\begin{itemize}
    \item The state and action space explodes 
    \item Next state transition probabilities and costs of individual agents depends not only on individual current state and action but also on that of others.
    \item Information needs to be shared to meet global objective however there may be privacy and scaling issues. 
    \item Tractable closed form expression of optimal value function is no longer easy to obtain to use it in lower-bound regret analysis. This is because at $n=1$, the number of states for single agent instances are only 2 and these are the same as nodes themselves $(s,g)$. But with $n>1$, this is exponential in $n$ and it's quite challenging to obtain closed form expressions for $V^*$ for these states and use them in regret lower bound analysis. We circumvent this issue by ignoring a non-exactly simplifiable summation of not neccesarily all positive terms, by showing that the entire summation is itself positive (\ref{lemma:sum_diff_prob_v}).
    \item In our analysis, we observe another similar challenge when simplifying a KL-divergence term that arises due to information theoretic bound on difference between expectations over different measures of the same random variable (\ref{eqn:exp_diff}). Instead of direct simplification, a suitable upper bounding technique that exploits symmetry of state-space for KL-divergence works for us.
 \end{itemize}
 }

\textcolor{red}{We conjecture that the decentralised MASSP problem is harder to solve compared to the single agent SSP learning problem. (Open problem, would require to prove that a lower bound for D-MASSP is higher compared to an upper bound on SASSP).} \textcolor{red}{have moved this to conclusion} \pt{conclusion}


\subsection{Proof of Theorem \ref{thm:lower_bound}}

\textbf{Recall Theorem \ref{thm:lower_bound}. }
    \textit{For any MASSP learning algorithm $\mathfrak{A}$ as defined in \ref{subsec:problem_formulation}, there exists a LM-MASSP instance ($\theta \in \Theta$) for every $n \geq 1$, $\delta \in (2/5,1/2)$, $\Delta < 2^{-n}.\frac{1-2\delta}{1+n+n^2}$, such that the expected cumulative regret upon running the algorithm on this instance for $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.\{\frac{1-2\delta}{1+n+n^2}\}^2} $ episodes at least matches the reported $\widetilde{O}(\sqrt{K})$ upper bound by \citep{trivedi2023massp} in terms of number of training episodes $K$. Here $V^*_1 = \frac{2n}{n-1+2(\delta+\Delta)}$. 
    Specifically for this instance, we have $\mathbb{E}_{\theta,\mathfrak{A}}[R(K)] \geq \frac{d.\sqrt{\delta}\sqrt{K.V^*_1}}{2^{n+9}}$  }   



\begin{proof}
We construct and analyze a family of hard to learn instances based on the discussion in \ref{sec:approach}.  Recall that for our instances, we  restricted $\theta$ (global theta) such that (no two local theta are same) $\theta_{i} \neq \theta_{j}$ $ \forall$ $ i \neq j \in [n]$ i.e., no two $\theta_i$ are the same. We denoted the set of all $\theta$ as $\Theta$. 
\\
In Theorem $\ref{thm:all_in_one}$, we characterized the optimal policy. The restriction on $\theta$ ensures that for the optimal global action, the individual actions for each agent are all different.
To further reduce complexity of the analysis, we let our instances be such that the cost of any global action in any non-goal state is equal to 1 (see Remark \ref{rem:cost_one}) and that in goal state equal to 0.  \\
Consider any instance parameters $(n\geq 1, \delta \in (2/5,1/2), \Delta < 2^{-n} . \frac{1-2\delta}{1+n+n^2})$. We want to analyze regrets for any policy for instances that are defined by above fixed parameters $(n,\delta, \Delta)$ and any  $\theta \in \Theta$. \\
Suppose in episode \textit{k}, agents take actions according to policy $\pi^k_{\theta}$. Let, $\tb{\ti{s}}_t$ represent the global state and $\tb{\ti{a}}_t$ the global action at time $t$. Then, the expected regret for the \textit{k-th} episode is:

\begin{align}
    & R_{\theta,k}  \\
    &= V^{\pi^k_\theta}(\tb{\ti{s}}_1) - V^*(\tb{\ti{s}}_1)  \label{regret}
    \\
    &=  V^{\pi^k_\theta}(\tb{\ti{s}}_1) - \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}[Q^{\pi^*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] + \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}[Q^{\pi^*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^{\pi^*}(\tb{\ti{s}}_1) 
    \end{align}
    In the above, we add and subtract $\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}[Q^{\pi^*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)]$. \\
    Below, we expand using the definitions of $V^{\pi^k_{\theta}}(.)$ and $Q^{\pi^*}(.,.)$ and rearrange:
    \begin{align}
    R_{\theta,k}
    &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}\{c(\tb{\ti{s}}_1, \tb{\ti{a}}_1) + \mathbb{E}_{\tb{\ti{s}}_2 \sim \mathbb{P}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)}[V^{\pi^k_\theta}(\tb{\ti{s}}_2)]\}  
    \\ 
    & \quad -\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}\{c(\tb{\ti{s}}_1, \tb{\ti{a}}_1) + \mathbb{E}_{\tb{\ti{s}}_2 \sim \mathbb{P}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)}[V^*(\tb{\ti{s}}_2)] \} + \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}[Q^{\pi^*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^{\pi^*}(\tb{\ti{s}}_1) \\
    &= \mathbb{E}_{\tb{\ti{a}}_1 \sim\ \pi^k_\theta(\tb{\ti{s}}_1), \tb{\ti{s}}_2 \sim\ \mathbb{P}(.|\tb{\ti{s}}_1,\tb{\ti{a}}_1)}[V^{\pi^k_\theta}(\tb{\ti{s}}_2) - V^*(\tb{\ti{s}}_2)] + \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}[Q^{\pi^*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^{\pi^*}(\tb{\ti{s}}_1) \label{eq_Q_V}
\end{align}
In the above expression, there appears to be a recursive relation from the first term but it its unclear how to deal with the second term. \\ 
We expand upon it below where $Q^* (.,.)= Q^{\pi^*}, V^*(.)=V^{\pi^*}$:
\begin{align}
  &\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[Q^{*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^*(\tb{\ti{s}}_1) \\
    &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[c(\tb{\ti{s}}_1, \tb{\ti{a}}_1) + \mathbb{E}_{\tb{\ti{s}}_2 \sim \mathbb{P}(.|\tb{\ti{s}}_1,\tb{\ti{a}}_1)}\{V^*(\tb{\ti{s}}_2)\}] - V^*(\tb{\ti{s}}_1) 
    \end{align}
    Above, we use the definition of $Q^*(.,.)$. \\
    Below, we use that the cost $c(\tb{\ti{s}}, \tb{\ti{a}}) \equiv 1 \forall (\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S}\backslash\{\tb{\ti{g}}\} \times \mathcal{A}$ and then expand the expectation:
    \begin{align}
    &\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[Q^{*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^*(\tb{\ti{s}}_1) \\
    &=  \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{  1 + \mathbb{E}_{\tb{\ti{s}}_2 \sim \mathbb{P}(.,\tb{\ti{s}}_1,\tb{\ti{a}}_1)}[V^*(\tb{\ti{s}}_2)] - V^*(\tb{\ti{s}}_1) \Big \} \\
    &=   \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k(\tb{\ti{s}}_1)} \Big\{ 1 +  \mathbb{P}(\tb{\ti{s}}_1|\tb{\ti{s}}_1,\tb{\ti{a}}_1) V^*(\tb{\ti{s}}_1) + \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)V^*(\tb{\ti{s}}_2) - V^*(\tb{\ti{s}}_1) \Big \} \end{align}
   To simplify above, we use the general transition probability expression from Lemma \ref{lemma:general_tp} and then rearrange:
    \begin{align}
   &\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[Q^{*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^*(\tb{\ti{s}}_1) \\
    &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi_{\theta}^k(\tb{\ti{s}}_1)} \Bigg\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Big \}  V^*(\tb{\ti{s}}_1) \\
  &+ \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)V^*(\tb{\ti{s}}_2)  - V^*(\tb{\ti{s}}_1) \Bigg \} \\
  &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta \Big \}  V^*(\tb{\ti{s}}_1) + \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)V^*(\tb{\ti{s}}_2) - V^*(\tb{\ti{s}}_1)  \Big \} \\
  &+ \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi_{\theta}^k(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*(\tb{\ti{s}}_1) \Big\} \\
  &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ 1 +\mathbb{P}(\tb{\ti{s}}_1|\tb{\ti{s}}_1,a_1^*) V^*(\tb{\ti{s}}_1) + \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)V^*(\tb{\ti{s}}_2) - V^*(\tb{\ti{s}}_1) \Big \} \\
  &+ \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}_1) \Big\}  
  \end{align}
The last step follows from transition probability expression in Lemma \ref{lemma:general_tp} since $\tb{\ti{s}} = (s,s,\dots,s)$.\\  
Below, we expand $V^*(\tb{\ti{s}}_1)$ and simplify:
  \begin{align}
  &\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[Q^{*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^*(\tb{\ti{s}}_1) \\    
  &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Bigg\{ 1 + \mathbb{P}(\tb{\ti{s}}_1|\tb{\ti{s}}_1,\tb{\ti{a}}_1^*)  V^*(\tb{\ti{s}}_1) + \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)V^*(\tb{\ti{s}}_2) - \Big\{ 1 +  \mathbb{P}(\tb{\ti{s}}_1|\tb{\ti{s}}_1,\tb{\ti{a}}_1^*) V^*(\tb{\ti{s}}_1) \\
  &+ \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1, \tb{\ti{a}}_1^*) V^*(\tb{\ti{s}}_2) \Big\} \Bigg \} + \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p})\neq \sgn(\theta_{i,p})\} V^*(\tb{\ti{s}}_1) \Big\} \\
  &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{\sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} [\mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)-\mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1, \tb{\ti{a}}_1^*)] V^*(\tb{\ti{s}}_2)  \Big \} \\
  &+ \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}_1) \Big\}
\end{align}

Using Lemma \ref{lemma:sum_diff_prob_v}, 
\begin{align}
    \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[Q^*(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^*(\tb{\ti{s}}_1) \geq \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}_1) \Big\} \label{eqn:final_qv}
\end{align}
Using Equation \eqref{eqn:final_qv} in Equation \eqref{eq_Q_V}, 
\begin{align}
    &R_{\theta,k} \geq  \mathbb{E}_{\tb{\ti{a}}_1 \sim\ \pi^k_{\theta}(\tb{\ti{s}}_1), \tb{\ti{s}}_2 \sim\ \mathbb{P}(.|\tb{\ti{s}}_1,\tb{\ti{a}}_1)}[V^{\pi^k_{\theta}}(\tb{\ti{s}}_2) - V^*(\tb{\ti{s}}_2)] \\
 &+ \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\tb{\ti{s}}_1 \neq goal \} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}_1) \Big\}
\end{align}

By recursion, Lemma \ref{lemma:sum_diff_prob_v} and since $V^*(\tb{\ti{s}}) \geq V^*_1$ for any $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$: \\
\begin{align}
    R_{\theta,k}  \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{k} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\tb{\ti{s}}_h \neq goal \} \mathbbm{1}\{\sgn(a^h_{i,p}) \neq \sgn(\theta_{i,p})\} \Big\}
\end{align}
 where, the expectation is taken with respect to trajectory induced in the $k^{th}$ episode by the interaction of policy $\pi^k_{\theta}$ and transition kernel $\mathbb{P}_{\theta}(.|.,.)$. Now, the total expected regret over $K$ episodes is: 
 \begin{align}
     R_{\theta}(K) \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{t=1}^{\infty} \mathbb{E}_{\theta, \pi_{\theta}} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\tb{\ti{s}}_t \neq goal \} \mathbbm{1}\{\sgn(a^t_{i,p}) \neq \sgn(\theta_{i,p})\} \Big\}
 \end{align}
 Analogous to \cite{min2022learning}, \cite{cohen2021minimax}, we define: 
 \begin{align}
     N = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq \goal\}
 \end{align}
\textcolor{red}{Remark:we need to deal with same notation as $[n]$} representing the random variable for total number of time steps over K episodes and for agent $i \in [n]$, $j \in [d-1]$,
 \begin{align}
     N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\}
 \end{align}
that represents the number of times in the entire duration of $K$ episodes that the agent $i$ chose $j^{th}$ component of its action as same as that of the optimal. Thus, 
\begin{align}
    R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi_{\theta}}  [ \sum_{i=1}^{n} \sum_{j=1}^{d-1} N_{i,j}(\theta) ]
\end{align}
To use the standard Pinsker's Inequality, we need $N_{i,j}(\theta)$ to be bounded almost surely which is known to not hold for SSPs (\cite{min2022learning},\cite{cohen2021minimax}). Hence, we use the capping trick introduced by \cite{cohen2021minimax} and also used by \cite{min2022learning}. In this trick, we cap the learning process to a predetermined $T$. 
If the learning process (i.e. $K^{th}$ episode) ends before this, the agents continue to remain at $goal$. In this case the summation for the actual process and the capped process is the same. On the other hand when $K$ episodes end beyond $T$, we have a truncated sum. Due to non-negativity of each part (Indicator function), the sum for the capped process lower bounds the actual sum. \\ Define 
\begin{align}
    N^- = \sum_{t=1}^T\mathbbm{1}\{\tb{\ti{s}}_t \neq \goal\}
\end{align} 
and for any agent $i \in [n] $ and $ j \in [d-1],$
\begin{align}
    N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{\tb{\ti{s}}_t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\}
\end{align} 
It is easy to see that (since any component of action has to match corresponding of $\theta$ or $\theta^j$) for any $i \in [n]$ and $j \in [d-1]$, 
\begin{align}\label{eqn:ntotal}
    N^- =   N^-_{i,j}(\theta) + N^-_{i,j}(\theta^{j}) 
\end{align}
 where for every $\theta \in \Theta$, $\theta^j$ represents the vector that only differs from $\theta$ at the $j^{th}$ index of every $\theta_i$ in $\theta = \{\theta_1,1,\theta_2,1,\dots,\theta_n,1\}$, where each $\theta_i \in \{\frac{-\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}\}^{d-1}$. \\  
Thus,  
\begin{align}
    R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi_{\theta}}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}
\end{align}
  Notice that $\theta \in \Theta \iff \theta^{j} \in \Theta$. This follows from definition of $\Theta$. Fixing $\pi_{\theta} = \pi$, this helps us write as follows: 
  \begin{align}
      2 \sum_{\theta \in \Theta} &R_{\theta}(K)\\
      &\geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \{ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \} \\
      &= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^- - N^-_{i,j}(\theta)] \}
      \end{align}
    Above, we use \eqref{eqn:ntotal}
      \begin{align}
       &2 \sum_{\theta \in \Theta} R_{\theta}(K)\\
          &= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^-] - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}\\
      &= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}
  \end{align}
  The above step is due to for any $j \in [d-1]$, for any $f(.)$, we have $\sum_{\theta \in \Theta} f(\theta^j) = \sum_{\theta \in \Theta} f(\theta) $
Using Lemma \ref{lemma:pinsk} and Lemma \ref{lemma:gen_co}, \\
\begin{align}
    &2 \sum_{\theta \in \Theta} R_{\theta}(K) \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  \mathbb{E}_{\theta, \pi}  [N^-] +  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] - \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] \} \Big \} \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV^*_1/4 -  \{  \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] - \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] \} \Big \} \label{eqn:exp_diff} \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV^*_1/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \}
\end{align}
Using Lemma \ref{lemma:kl_d}, 
\begin{align}
    &2 \sum_{\theta \in \Theta} R_{\theta}(K) \\
    &\geq \frac{2 \Delta V_1^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{1/2} \sqrt{3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]}  \} \Big \}  \\
    &= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{\mathbb{E}_{\theta}[N^-]} \Big \} \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{T} \Big \} \\
    &= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \}
\end{align}
In the last second step we used the fact that $N^- \leq T$ \\
Further, notice that the term inside the bracket is independent of $\theta, i$ or $j$. Thus, we have: 
\begin{align}
    \sum_{\theta \in \Theta} R_{\theta}(K) \geq  \Delta V_1^* |\Theta| \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \}
\end{align}
Thus by rearranging and using $\sqrt{3}<2$,
\begin{align}
    \frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq   V_1^*  \Big \{ \Delta  KV_1^*/4 -   (KV_1^*)^{3/2}  \frac{2^{n+2}.\Delta^2}{\sqrt{\delta} (d-1)} \Big \}
\end{align}
Pick, 
\begin{align}
    \Delta^* = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}
\end{align}
At this value of $\Delta$,
\begin{align}
    &\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \\
    &\geq V_1^* \Bigg \{  \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}. \frac{KV_1^*}{4} - \frac{(KV_1^*)^{3/2}.2^{n+2}}{\sqrt{\delta}(d-1)}. \Big \{\frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}\Big\}^2 \Bigg \} \\
    &= V_1^* \Bigg\{\frac{(d-1) \sqrt{\delta.K.V_1^*}}{2^{n+7}} - \frac{(d-1)\sqrt{\delta.K.V_1^*}}{2^{n+8}}\Bigg\} \\
    &\geq  \frac{(d-1).\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+8}} \\
    &\geq \frac{d.\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+9}}
\end{align}
In the last second line, we use that $V^*_1>1$ and in the last line, we use $d-1 \geq d/2$ for any natural number $d\geq 2$ which holds for our instances. Since the average over entire set is lower bounded by the RHS, there must exist some parameter in the set for which the RHS is a lower bound. Hence proved. \\
It remains to show that the $\Delta$ picked above is valid. \\ Hence, need to ensure that: 
\begin{align}
    \Delta = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}} < 2^{-n}.\Bigg \{\frac{1-2\delta}{1+n+n^2} \Bigg \} 
\end{align}
which gives: 
\begin{align}
    K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.\{\frac{1-2\delta}{1+n+n^2}\}^2} 
\end{align}
\end{proof}


\subsection{Proof of Lemma \ref{lemma:gen_co}}

\textbf{Recall the Lemma  \ref{lemma:gen_co}.}  \textit{If $T \geq 2KV^*_1$, then, $\mathbb{E}_{\theta}[N^-] \geq KV^*_1/4$,  for any $\theta \in \Theta$.} 

\begin{proof}
If capped process finishes before $T$, then $N^-=N$. Else, number of visits to $goal$ state is less than $K$ due to which $N^- \geq T-K$. Therefore, we have
% 
\begin{align}
    \mathbb{E}[N^-] \geq \mathbb{E}[\min\{T-K,N\}] \geq \mathbb{E}[\sum_{i=1}^K\min\{T/K-1, N_k\}]
\end{align}
% 
In the above, $N_k$ is the random variable representing the length of episode $k$. Since $T\geq2KV^*_1,$ and $V^*_1\geq1$ the lemma will hold for any policy if $N_k \geq V^*_1$ with probability $\geq 1/4$ for any policy. Consider any policy.  
\begin{align}
    \mathbb{P}[N_k \geq V^*_1] &= \mathbb{P}(\tb{\ti{s}}_2 \neq \tb{\ti{g}}|\tb{\ti{s}}_1=\tb{\ti{s}}).\mathbb{P}(\tb{\ti{s}}_3 \neq \tb{\ti{g}}|\tb{\ti{s}}_2).\mathbb{P}(\tb{\ti{s}}_4 \neq \tb{\ti{g}}|\tb{\ti{s}}_3) \dots \mathbb{P}(\tb{\ti{s}}_{\lceil V^*_1\rceil} \neq \tb{\ti{g}}|\tb{\ti{s}}_{\lfloor V^*_1\rfloor-1}) 
    \\ 
    &= (1-p^{a(\tb{\ti{s}}_1)}_{\tb{\ti{s}}_1,goal}).(1-p^{a(\tb{\ti{s}}_2)}_{\tb{\ti{s}}_2,goal})\dots(1-p^{a(\tb{\ti{s}}_{\lfloor V^*_1\rfloor-1})}_{\tb{\ti{s}}_{\lfloor V^*_1\rfloor-1},goal}) 
\end{align}
For any state $\tb{\ti{s}}$, $1-p^{a(\tb{\ti{s}})}_{\tb{\ti{s}},goal}$ is minimum when $p^{a(\tb{\ti{s}})}_{\tb{\ti{s}},goal}$ is maximum. Check from Lemma \ref{lemma:general_tp} that this happens at $a^*$ which matches all signs with $\theta$, i.e., $a^* = a_{\theta}$ and at any $\tb{\ti{s}} \in \mathcal{S}_{n,1}$(i.e., $p^*_{1,0}$). Thus, we can lower bound the above product as: 
\begin{align}
    \mathbb{P}[N_k \geq V^*_1]  & \geq 
    (1-p^*_{\tb{\ti{s}}_1,goal}).(1-p^*_{\tb{\ti{s}}_2,goal})\dots(1-p^*_{s_{\lfloor V^*_1 \rfloor -1},goal}) 
    \\
    & \geq (1-p^*_{1,0})^{\lfloor V^*_1 \rfloor -1} 
    \\
    & \geq (1-p^*_{1,0})^{ V^*_1 } 
    \\
    &= (1-p^*_{1,0})^{ 1/{p^*_{1,0}} }
    \\
    & \geq 1/4
\end{align}
For the last second inequality, we use for $x\geq 2$, $(1-1/x)^{x}\geq 1/4$ 
Why here $x = 1/p^*_{1,0}\geq 2$ is shown at the end of the alternate proof below. \\
\textcolor{red}{can someone comment if there's any issue with above proof?}
Thus, 
 \begin{align}
     \mathbb{E}[N^-]  \geq \mathbb{E}[\sum_{i=1}^K min  \{T/K-1, N_k\}] \geq KV^*_1/4
 \end{align}

\subsubsection{Alternate proof for showing $\mathbb{P}[N_k \geq V^*_1] \ge \frac{1}{4}$}
 
Using Lemma \ref{lemma:episodelength}, for some $\tb{\ti{s}}_1 \in \mathcal{S}(1)$, we have, 
\begin{align}
    \mathbb{P}^{\pi}[N_k \geq V^*_1](\tb{\ti{s}}) 
    &\geq 
    \mathbb{P}^{\pi^*}[N_k \geq V^*_1](\tb{\ti{s}})  
    \\
    &\geq \mathbb{P}^{\pi^*}[N_k \geq V^*_1](\tb{\ti{s}}_1) 
    \\
    &= (1-p^*(goal|\tb{\ti{s}}_1,\tb{\ti{a}}^*))^{\lfloor V^*_1 \rfloor  } 
    \\
    &\geq (1-p^*(goal|\tb{\ti{s}}_1,\tb{\ti{a}}^*))^{ V^*_1 }  
    \\
    &\geq 1/4
\end{align}
% 
Here, the last inequality comes from the fact $V^*_1 = 1/p^*(goal|\tb{\ti{s}}_1, \tb{\ti{a}}^*)$ (see proof of Theorem \ref{thm:all_in_one}) that for $x>2$, $(1-1/x)^x \geq 1/4$. \\Note that $V^*_1 = \frac{2n}{n-1+2(\delta+\Delta)} > 2$ since 
\begin{align}
    \frac{1}{V^*_1} & = \frac{n-1}{2n} + \frac{2(\delta+\Delta)}{2n} 
    \\
    & < \frac{n-1}{2n} + \frac{2(\delta+2^{-n}.\frac{1-2\delta}{1+n+n^2})}{2n} 
    \\
    & < \frac{n-1}{2n} + \frac{2(\delta+\frac{1-2\delta}{6})}{2n} 
    \\
    &= \frac{n-1}{2n} + \frac{(\frac{1+4\delta}{3})}{2n} 
    \\
    & < 1/2
\end{align}
Above, the first inequality arises due to $\Delta < \frac{1-2\delta}{1+n+n^2}$ for our instances, the second inequality arises due to $n \geq 1$ and the final step is due to $\delta < 1/2$.
\end{proof}


\section{Preliminaries and Problem Formulation} 
\label{sec:problem}




\subsection{Notations and Preliminaries}
\label{subsec:prelims}


\begin{itemize}
    \item Directly start with our setup --- multi-agent ssp -- what it is -- 
\end{itemize}



\paragraph{General MA-SSP.} We consider a general \emph{Multi-Agent Stochastic Shortest Path (MA-SSP)} problem, defined by the tuple $(\mathcal{V}, N, \mathbb{P}, \mathcal{A})$. Here $\mathcal{V} = \{v_1, v_2, \dots, v_q\}$ denotes the set of nodes, and $N = \{1,2,\dots,n\}$ is the set of $n$ agents. At any given time, each agent occupies exactly one node. The global state of the system is represented as $\tb{\ti{s}} = (s_1, s_2, \dots, s_n) \in \mathcal{S}$, where $s_i \in \mathcal{V}$ denotes the node occupied by agent $i$. Thus, the overall state space is $\mathcal{S} = \mathcal{V}^n$.
\\
\textcolor{red}{Need to mention definition of $r$ and the partition}

Each agent $i \in N$ has an action space $\mathcal{A}^i$, assumed to be independent of its current location. \textcolor{red}{reframing the prev sentence as: "The set of actions $\mathcal{A}^i$ available to any agent $i \in N$ is the same at every node." Also we missed to emphasize that each agent takes action independently. So we can add this line: "Agents take these actions independently."} A global action is denoted as $\tb{\ti{a}} = (a_1, a_2, \dots, a_n) \in \mathcal{A}$, where $\mathcal{A} = \mathcal{A}^1 \times \cdots \times \mathcal{A}^n$. The transition dynamics of the system are governed by a probability distribution $\mathbb{P}$ such that, given a state-action pair $(\tb{\ti{s}}, \tb{\ti{a}})$, the next state $\tb{\ti{s}}'$ is drawn from $\mathbb{P}(\cdot \mid \tb{\ti{s}}, \tb{a})$. This formulation naturally captures the coupling among agents: the future state of each agent may depend on the joint configuration and action of all agents.

Each agent $i$ incurs a \textcolor{red}{an instantaneous} random cost $c^i(\tb{\ti{s}}, \tb{a}) \in [c_{\min}, 1]$ upon taking action $\tb{a}$ in state $\tb{\ti{s}}$, where $c_{\min} > 0$. \textcolor{red}{prev statement sounds like agent i is taking the action $\tb{\ti{a}}$. We can reframe it as: "When global action $\tb{\ti{a}} \in \mathcal{A}$ is taken in global state $\tb{\ti{s}} \in \mathcal{S}$, agent $i \in N$ recieves cost $c^i(\tb{\ti{s}},\tb{\ti{a}})$". I'm also thinking do we need to write the range of cost because it is nowhere used in lower bound analysis. I have used cost as 1 but that doesn't require specific condition on costs. In upper bound, I think there are some steps that need this. But we don't need it for lower bound.}
This individual cost can depend on the full joint state and joint action, encapsulating complex multi-agent interdependencies. \textcolor{red}{Reframing previous sentence: Notice that, in general, the individual costs depends on the location and action of other agents as well as of itself encapsulating complex multi-agent interdependencies. } \\
\\
\textcolor{red}{I personally think there is no need to even talk anything in detail about congestion: basically we can get rid of the next two equations to reduce this section. The last line of the previous paragraph suggests a broad generalisation. Or we can push the discussion on how congestion can be modelled into into appendix and reference here in one line. }

We consider the notion of \emph{congestion-aware costs} to model multi-agent interference. Let $K^i(\tb{\ti{s}}, \tb{a})$ denote a private cost component for agent $i$, capturing all factors other than congestion. The congestion factor for agent $i$ is modeled as:
\begin{align}
    c_f^i(\tb{\ti{s}}, \tb{a}) = \sum_{j=1}^n \mathbbm{1}\{a_j = a_i\},
\end{align}
which counts how many agents (including $i$ itself) are taking the same action. The total cost to agent $i$ is then given by:
\begin{align}\label{eqn:ind_cost}
    c^i(\tb{\ti{s}}, \tb{a}) = c_f^i(\tb{\ti{s}}, \tb{a}) \cdot K^i(\tb{\ti{s}}, \tb{a}).
\end{align}
The global cost is defined as the average of individual costs:
\begin{align}\label{eqn:glb_cost}
    c(\tb{\ti{s}}, \tb{a}) = \frac{1}{n} \sum_{i=1}^n c^i(\tb{\ti{s}}, \tb{a}) = \frac{1}{n} \sum_{i=1}^n \left( \sum_{j=1}^n \mathbbm{1}\{a_j = a_i\} \cdot K^i(\tb{\ti{s}}, \tb{a}) \right).
\end{align}

The goal is to design policies that \textcolor{red}{instead reframe as : The goal is to identify a policy i.e., a \emph{scheme} of taking actions to} minimize the expected cumulative global cost incurred in reaching a target state $\tb{g}$ from a fixed initial state $\tb{\ti{s}}_{\init}$. 
Let $\Pi_{\textcolor{red}{HR}}$ denote the set of all history-dependent randomized policies mapping past trajectories to \textcolor{red}{probability} distributions over actions. Due to the Markovian and stationary nature of the system's $\textcolor{red}{transition}$ dynamics and cost structure, it suffices to consider deterministic Markovian  policies ($\textcolor{red}{\Pi_{MD}}$) without loss of optimality (see, e.g., \cite{puterman2014markov}).

\textcolor{red}{Further,} Not all \textcolor{red}{such} policies ensure successful completion of the task. \textcolor{red}{we didn't define what the task is so better to say "termination of the navigation process to \tb{\ti{g}}"} 
A policy is termed \emph{proper} if it leads to the goal state $\tb{g}$ almost surely, from any initial state. Otherwise, it is termed \emph{improper}, and its expected cumulative cost may be \textcolor{red}{why may be? replace with : is for at least one state?} unbounded. We assume the existence of at least one proper policy and denote the set of all proper policies as $\Pi_p$ \citep{tarbouriech2020no, tarbouriech2021stochastic, cohen2021minimax,min2022learning}.

For any policy $\pi \in \Pi_p$, we define the value function at state $\tb{\ti{s}}$ \textcolor{red}{for any state} as the expected cumulative cost until reaching $\tb{g}$:
\begin{align}
    V^\pi(\tb{\ti{s}}) = \mathbb{E} \left[ \sum_{t=1}^{\tau^\pi} c(\tb{\ti{s}}_t, \pi(\tb{\ti{s}}_t)) \,\middle|\, \tb{\ti{s}}_1 = \tb{\ti{s}} \right],
\end{align}
where $\tau^\pi$ denotes the (random) hitting time of the goal under policy $\pi$. The optimal value function is defined as $V^*(\tb{\ti{s}}) = \min_{\pi \in \Pi_p} V^\pi(\tb{\ti{s}})$, and the optimal policy $\pi^*$ achieves this minimum. We define the \emph{diameter} $B^*$ of the MA-SSP problem as the worst-case \textcolor{red}{worst-case sounds informal, replace with maximum expected} cost-to-go from any state under the optimal policy:
\begin{align}
    B^* = \max_{\tb{\ti{s}} \in \mathcal{S}} V^*(\tb{\ti{s}}).
\end{align}

In the \emph{learning} setting, the transition function $\mathbb{P}$ and/or the cost function $c(.,.)$ are initially unknown. The agent must interact with the environment over $K$ episodes, each beginning at $\tb{\ti{s}}$ and terminating upon reaching $\tb{\ti{g}}$. The agent must balance exploration and exploitation to learn the optimal policy efficiently.

Let $h_k$ be the random episode length for episode $k$ 
 \textcolor{red}{replace as: be the random length of episode $k$}, and let $(\tb{\ti{s}}_{k,h}, \tb{a}_{k,h})$ denote the state and action at step $h$ of episode $k$. Then, the expected cumulative regret of a learning algorithm $\mathfrak{A}$ over $K$ episodes is defined as:
\begin{align}\label{eqn:regret}
    \mathbb{E}_{\mathfrak{A}}[R(K)] = \mathbb{E} \left[ \sum_{k=1}^K \sum_{h=1}^{h_k} c(\tb{\ti{s}}_{k,h}, \tb{a}_{k,h}) \right] - K \cdot V^*(\tb{\ti{s}}_{\init}).
\end{align}
This regret quantifies the performance gap between the learning agent \textcolor{red}{we have multiple learning agents} and an oracle that follows the optimal policy from the start. The goal in MA-SSP learning is to design algorithms that minimize regret, ideally achieving sublinear growth in $K$. 


Recall that the best policy must minimize the cumulative global cost to go from $s_{init}$ to $goal$ and not just the cumulative cost to a particular agent. However, the actions are taken by individual agents. But these agents directly receive only their individual costs and do not have a direct access to others' costs or to the global cost. 
This problem could be solved by the use of a central controller who may coordinate actions and receive signals (individual costs from each agent). However, this significantly increases computation and transmission costs for higher number of agents and would degrade robustness to malicious attacks \citep{zhang2018fully}. Further, agents may be unwilling to share their individual costs to preserve privacy. \pt{As opposed to the central controller approach we consider a decentralized setting where the agents action and thus the reward are preserved.} 
Hence mechanism that ensure agents learn the best policy independently is desirable which takes us into the purview of Decentralized Multi-Agent Reinforcement Learning. But a common goal cannot be achieved without sharing of any information (\textcolor{red}{why? cite?}). For this, (\textcolor{red}{cost parametrisation was motivated from which papers? or was completely new in maccm paper?})(cite) proposes parametrizing the expected costs, namely for all $(\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S} \times \mathcal{A}$, there exist known features $\psi(\tb{\ti{s}},\tb{\ti{a}}) \in R^{nd}$ and an unknown parameter $\tb{w} \in R^{nd}$ for the instance such that $\mathbb{E}[c(\tb{\ti{s}},\tb{\ti{a}})]=\langle \psi(\tb{\ti{s}},\tb{\ti{a}}),\tb{w} \rangle$.
Hence, instead of sharing actual costs, agents can now share their estimate of the unknown parameter. 
Further, since the state and action space is explosively large, we assume the following linear function approximation of transition probabilities to hold:
\begin{assumption} \label{assm:lfa_prob}
    For every pair $(\tb{\ti{s}},\tb{\ti{a}},\tb{\ti{s}}') \in \mathcal{S}\times\mathcal{A}\times\mathcal{S}$,  there exists known features $\phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \in \mathbb{R}^{nd}$ and unknown $\theta \in \mathbb{R}^{nd}$ such that, for any $\tb{\ti{s}}' \in \mathcal{S}$, $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) = \langle \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}),\theta \rangle$. 
\end{assumption}


\pt{We can directly write this thing after defining the features, no need to write it here.}

Due to the above two linear function approximations we will refer to these MASSPs as Linear Mixture MASSPs, LM-MASSPs. They are in general able to capture complex transition interdependencies. We describe a possible feature design for transition probabilities in \ref{subsec:features}. 


\subsection{Problem Formulation}
\label{subsec:problem_formulation}
% 
In the above-described setting, \citep{trivedi2023massp} provided an algorithm whose expected cumulative regret scales as $\widetilde{O}(\sqrt{K})$. To obtain a lower bound in this setting, we need to construct difficult-to-learn instances with tractable optimal policy and analyze its difference from any policy in terms of value function. Similar to arguments in the lower bound proof in \citep{auer2002nonstochastic}, it is sufficient to consider deterministic policies just for notational convenience and the proposed proof can be extended for randomized policies as well. 



Similar to \cite{osband2016lowerboundsregretreinforcement}, we define a Decentralized Multi-Agent Reinforcement Learning algorithm as a deterministic sequence of $\{\pi_t|t=1,2\dots\}$ functions. Here each function $\pi_t$ maps history $\mathcal{H}_t$ till time $t$ to a map in the set of all maps from the set of agents to the set of all possible probability distributions over actions i.e., $\pi_t \in \{(\pi^1,\pi^2,\dots,\pi^n) : \pi^i \in \Delta(\mathcal{A}^i) \forall i \in [n] \}$ where $\Delta(\mathcal{A}^i)$ denotes the probability simplex over individual actions, $\pi^i$ for $i \in [n]$ denotes the independent strategy of choosing actions by agent $i$. \\
In the below section, we demonstrate how to construct these hard to learn instances.

\pt{This section is vey loose as of now. we need to handle the cases.}



\subsection{Construction of the Problem Instances}
\label{subsec:problem_instance}

All instances in our consideration have only two nodes i.e., $\mathcal{V} = \{s,g\}$. Hence, $\mathcal{S} = \Pi_{i \in [n]} \{s,g\} = \{s,g\}^{n}$. Thus, the total number of states, $|\mathcal{S}| = 2^n$. Also, we fix $\tb{\ti{s}}_{\init} = (s,s,\dots,s)$ and $goal = \tb{g} = (g,g,\dots, g)$. At every node, we let the actions available to any agent $i \in [n]$ be the same as $\mathcal{A}^i = \{-1,1\}^{d-1}$ for some $d \geq 2$. Thus the global action space $\mathcal{A}=\{-1,1\}^{n(d-1)}$. Hence, $|\mathcal{A}| = 2^{n(d-1)}$. Further, we assume that once an agent reaches node $g$, it cannot go back to node $s$. Hence, transitions like $\tb{\ti{s}} = (s,s,\dots,g,g) \rightarrow \tb{\ti{s}}'=(s,s,\dots ,g,s)$ are impossible.

\pt{partitioning of the state space- -- we partition the state space based on r, the number of agents at the state s. $\mathcal{S}_r$ -- of type r... $\mathcal{S}(s)$ -- reachable from $s$. $\mathcal{S}_r(s)$ -- reachable from s of type r. }

Any of our instance is parametrized by a tuple $(n,\delta, \Delta, \theta)$ where $n \geq 1$ is the number of agents, $2/5 < \delta < 1/2$ and $\Delta < 2^{-n} \cdot \frac{1-2\delta}{1+n+n^2}$ are parameters of our proposed features \pt{ref this section .. that the detailed feature design in given in the next subsection. The features are defiend for a given instance. }

, and $\theta$ is an $nd$- dimensional vector of the form $\theta = (\theta_1,1, \theta_2,1,\dots,\theta_n,1)$ where for every $i \in [n]$, $\theta_i$ is a $(d-1)$ dimensional vector each of whose component is $\pm \frac{\Delta}{n(d-1)}$. Let the set of all such $\theta$'s be $\Theta$. $\theta$ is a parameter related to the transition probability model mentioned in Assumption \ref{assm:lfa_prob}. For convenience, we will sometimes use $\widetilde{\theta} = (\theta_1,\theta_2,\dots,\theta_n)$ wherever required.

\pt{This is an additional challenge -- and this is very common in MARL Setting. so, to avoid that the instance is suitably chosen -- via cost -- then comes remark 2 -- why such  is possible -- here we need to the cost eqn from previous section. }

\begin{remark}
    For a general cost and transition probability function, there may in general be a trade-off between policy that takes the system ``closer'' to the goal (hence minimizing the number of time steps to reach the goal) and another that takes more time but may be (in an overall sense) cost efficient \citep{tarbouriech2020no}. 
\end{remark}




To avoid this complication in the analysis of our instances, we let for all $\tb{\ti{s}} \in \mathcal{S}\backslash\{\tb{\ti{g}}\}$ and $\tb{\ti{a}} \in \mathcal{A}$, $c(\tb{\ti{s}},\tb{\ti{a}}) = 1$ while for any $\tb{a} \in \mathcal{A}, c(\tb{\ti{g}}, \tb{\ti{a}}) =0$. Hence, the policy that takes us "nearer" to $goal$ is better. This leads to optimum policy being directly influenced by transition probabilities. 

The following justifies how such instances are possible.
\begin{remark} \label{rem:cost_one}
    One class of such instances is the one for whom for all $i \in [n], \tb{\ti{a}} \in \mathcal{A}, K^i(\tb{\ti{s}},\tb{\ti{a}}) = \frac{1}{\sum_{j=1}^n \mathbbm{1}\{a_j=a_i\}}$ for all $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$ and $ K^i(\tb{\ti{g}},\tb{\ti{a}}) = 0$ . From Equation \ref{eqn:ind_cost} and Equation \ref{eqn:glb_cost} one observes that for such instances for all $(\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S}\backslash\tb{\ti{g}} \times \mathcal{A}$, $c(\tb{\ti{s}},\tb{\ti{a}}) = 1$ and $c(\tb{\ti{g}}, \tb{\ti{a}}) = 0$. 
\end{remark}

 


\subsection{Features} 
\label{subsec:features}


For the type of instances mentioned in the previous subsection, we now provide the valid features for the transition probability model mentioned in Assumption \ref{assm:lfa_prob}.


Note that there can be many possible feature designs but all of them must satisfy the following requirements to produce valid transition probabilities in any instance defined above in \ref{subsec:problem_formulation}:
\begin{requirements}
    For any $(\tb{\ti{s}},\tb{\ti{a}},\tb{\ti{s}}') \in \mathcal{S}\times\mathcal{A}\times\mathcal{S}$, the transition probability $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \geq 0$ and for any $(\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S}\times \mathcal{A}$, $\sum_{\tb{\ti{s}}' \in \mathcal{S}}\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) = 1$ \label{reqm:1}
\end{requirements}
\begin{requirements}
   If there is a physically impossible transition to some $\tb{\ti{s}}' \in \mathcal{S}$ from some $\tb{\ti{s}} \in \mathcal{S}$, under action $\tb{\ti{a}} \in \mathcal{A}$, then $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) = 0$ and if there's a certain transition to some $\tb{\ti{s}}' \in \mathcal{S}$ from some $\tb{\ti{s}} \in \mathcal{S}$ under action $\tb{\ti{a}} \in \mathcal{A}$, then $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) = 1$. \label{reqm:2}
\end{requirements}
For our instances, we consider the following feature design :
\begin{equation}
\label{eqn:features_global_new}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  {\ti{a}}) = 
\begin{cases} (\phi(s^{\prime}_1 | s_1, {\ti{a}}_1), \dots, \phi(s^{\prime}_n | s_n, {\ti{a}}_n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}} ~\text{and}~  s^\prime_{i} = g ~\text{if} ~ s_i = g,~ \forall~ i\in [n]
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}}, \text{or } \tb{\ti{s}} \neq \tb{\ti{g}} ,  \exists~ i \in [n],~ s.t. ~ s_i = g, s^\prime_i = s
\\
(\mb{0}_{nd-1}, 1), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}} 
\end{cases}
\end{equation}

Recall that, in the above, $a_i$, $s_i$ and $s^{\prime}_i$ represent the individual action, current node and next node, respectively, of agent $i \in [n]$. Also, observe that the first case corresponds to the most general transitions that are allowed, the second case represents all impossible transitions and the third case takes care of the only \textit{certain} transition.\\
Further, $\phi(s^{\prime}_i | s_i, {\ti{a}}_i)$ are defined as 
\begin{equation} \label{eqn:features_global_new_gen}
\phi(s^{\prime}_i | s_i, {\ti{a}}_i) = \begin{cases}  
\left(-{\ti{a}}_i, \frac{1-\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}_i = s^{\prime}_i = s
\\
\left({\ti{a}}_i, \frac{\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}_i = s,~s^{\prime}_i = g
\\
\left(\mathbf{0}_{d-1}, \frac{1}{n 2^{r}} \right)^{\top}, & if ~ {s}_i = g,~ s^{\prime}_i = g
\end{cases}
\end{equation}

In the above, $r$ represents the number of agents at node $s$ in the current global state $\tb{\ti{s}}$. 

\begin{lemma}\label{lemma:valid_features}
    Features defined above in equations \ref{eqn:features_global_new} and \ref{eqn:features_global_new_gen}, produce valid transition probabilities for any instance $(n,\delta,\Delta,\theta)$ as defined in \ref{subsec:problem_instance}. Specifically they satisfy both requirements \ref{reqm:1} and \ref{reqm:2}.
\end{lemma}
We refer the reader to Appendix \ref{proof:lemma:valid_features} for the proof.

In the following lemma, we derive a general expression for the probability of any valid transition for any instance $(n, \delta, \Delta, \theta)$ as defined in \ref{subsec:problem_instance}. 
\textcolor{red}{the below lemma statement will simplify depending on if these definitions are incorporated in \ref{subsec:prelims}}
\begin{lemma}
\label{lemma:general_tp} 
Consider any state $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$. In this state $\tb{\ti{s}}$, let $\mathcal{I}:=\{i_1,i_2,\dots,i_{r}\}$ denote the set of agents at node $s$ and $\mathcal{J}:=\{j_1,j_2,\dots,j_{n-r}\}$ be those at node $g$. 
Under a valid transition, either the next state is the same as $\tb{\ti{s}}$ or possibly some agents from $\mathcal{I}$ transit to node $g$. Let the set of all valid next states from $\tb{\ti{s}}$ be denoted as $\mathcal{S}(\tb{\ti{s}})$. To study a particular transition to $\tb{\ti{s}}'\in \mathcal{S}(\tb{\ti{s}})$, we define $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ as the set of all agents moving from node $s$ to node $g$. Here, $r'$ denotes the number of agents in state $\tb{\ti{s}}'$ that are at node $s$. For any action $\tb{\ti{a}} \in \mathcal{A}$, the transition probability is given as: 
\begin{align}
    &p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'} = 
 \mathbb{P}(\tb{\ti{s}}^\prime | \tb{\ti{s}}, \tb{\ti{a}}) 
=\frac{r' + (r-2r')\delta}{n \cdot 2^{r-1}} +   \frac{n-r}{n \cdot 2^r}        +    \frac{\Delta}{n}  (r-2r') \\
&\quad + \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn({{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn({{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}
\end{align} 
\end{lemma}


\pt{The following corollary provides the probability when action are as in Theorem 1. This probability only depends on $r$ and $r'$ only. i am thinking to remove this corollary and put it as the another statement in the above lemma.
} \textcolor{red}{i dont mind. can we decide upon these things after doing one round of appendix?}


\begin{corollary} \label{corollary:p_star}
From Lemma \ref{lemma:general_tp}, we observe that for any given instance $(n, \delta, \Delta, \theta)$ if the action chosen is such that the indicators vanish in the above expression, the transition probability doesn't depend on $\mathcal{I}$ and $\mathcal{T}$ and only depends on $r$ and $r'$. Hence, we define this special global action $\tb{\ti{a}}_{\theta}$ as the action whose $\{(d-1)\times (i-1)+j\}-th$ element for every $i \in [n]$ and every $j \in [d-1]$ is given by $\sgn(\theta_{i,j})$. In other words,  $\tb{\ti{a}}_{\theta} = \frac{n(d-1)}{\Delta} \times \widetilde{\theta}$. 
\end{corollary}


\subsection{Summary of Approach}


\pt{Why we created these instances like these -- why we expect good results from this instance -- etc. -- why it is hard .}


Any deterministic algorithm produces, in general, a history-dependent policy. Fixing any such policy $\pi$, we will analyze the regret of this policy on a set of hard to learn instances that differ only due to $\theta$ (i.e., have same parameters $n, \delta, \Delta$) and show that there exists an instance in the set of hard-to-learn instances that achieves lower bound on expected cumulative regret that scales similarly in terms of number of episodes as upper bound $\widetilde{O}(\sqrt{K})$ reported by \citep{trivedi2023massp}. 
Intuitively, there are two reasons why we expect at least one of the instances in this set to be very hard to be learnt for any given policy:
\begin{itemize}
    \item Firstly, all the instances are characterized by the optimum policy that at any state, the actions taken by each agent are such that they match signs with all components of respective $\theta_i$'s (Theorem \ref{thm:all_in_one}).  In other words, for a given instance $\theta = (\theta_1,1,\theta_2,1,\dots, \theta_n,1)$ we have $\widetilde{\theta} = (\theta_1,\theta_2,\dots,\theta_n)$ and the optimal policy is that: at every state, the global action to be taken must is the same as $\tb{\ti{a}}^* = \{a^*_1,a^*_2,\dots, a^*_n\}$ such that, $\tb{\ti{a}}^* = \frac{n(d-1)}{\Delta} \times \widetilde{\theta}$. 
If we consider a policy such that the action taken in one of the $2^n-1$ non-goal states differed from the optimal action in this state at just one of the $n(d-1)$ indices, then the transition probabilities would differ (from those for optimal policy) only very slightly since $\Delta$ is quite small $(<2^{-n})$. 
Hence, the value function for that policy would be only slightly higher. Observe that there would be $n(d-1).2^{n-1}$ (significant) number of such policies. The policies that differ in the above fashion at any two states are even larger in number and can't be expected to be too worse in terms of the expected cumulative cost for similar reason. Hence, separating these large number of policies efficiently is a challenge before any MASSP learning algorithm. 
\item Secondly, any learning algorithm that efficiently learns the best policy for one instance in the set of all instances, may not be able to efficiently learn some other instance in the set. Also, if a particular action is the best (optimal) for a given instance $\theta = (\theta_1,1,\theta_2,1,\dots,\theta_n,1)$, there definitely exists another instance $\theta = (-\theta_1,1,-\theta_2,1,\dots,-\theta_n,1) \in \Theta$ for whom the same action is the worst.
\end{itemize}
In the following section, we present our observations on these instances and key results that follow.


\section{Theoretical Results}
\label{sec:theory}

\pt{Need to highlight why we need these results, what are the advantages, and what is the summary etc\dots for each of these theorem.}

\pt{Also. we need to clearly highlight the novelty in the proofs, etc.}

Any 2-node LM-MASSP instance as defined in Section \ref{subsec:problem_instance} is reasonably expected to have the notion that under the optimal behavior of agents, a state with more agents at node $g$ is \textit{better}
compared to another state with fewer agents at node $g$. This can be baked mathematically in terms of value functions of states in the following lemma.
% 
\begin{lemma}
\label{prop:1}
    Consider any two states $\tb{\ti{s}}_1, \tb{\ti{s}}_2 \in \mathcal{S}$. Let $\tb{\ti{s}}_1 \in \mathcal{S}(r_1)$ and $\tb{\ti{s}}_2 \in \mathcal{S}(r_2)$. Then, if $r_1>r_2$, we have $V^*(\tb{\ti{s}}_1) > V^*(\tb{\ti{s}}_2)$ and vice-versa.
\end{lemma}
% 
The proof of this lemma is deferred to the Appendix ??. Next, recall that any  multi-agent setting leads to explosion of the number of states and actions due to which it's challenging to obtain optimal policies for the setting. In the following theorem we show that for our instances a tractable optimal policy exists. The optimal action  and the corresponding optimal value depends on the 
Further, we identify a partition of the state space based on number of agents at node $s$ and show that all the states in a particular partition set have the same optimum values. Finally we  show that our instances exhibit property given in lemma \ref{prop:1}.

 
\begin{theorem}\label{thm:all_in_one}
    Consider any instance defined as in \ref{subsec:problem_instance}.
    \begin{itemize}
        \item Then the policy of taking action $\tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$, is optimal. 
        \item Further, optimal value function for each state with the same number of agents at node $s$ takes the same value, i.e., for every $r \in [n]$, it holds that for all $\tb{\ti{s}} \in \mathcal{S}(r)$ we have $V^*(\tb{\ti{s}}) = V^*_r =$ some constant depending on only $r$. We define $V^*_0=0$.
        \item The optimal value function monotonically increases with the number of agents at node $s$ i.e., $0=V^*_0<V^*_1<V^*_2\dots<V^*_n = B^*$. 
    \end{itemize}
    
\end{theorem}


\begin{proof}(of Theorem \ref{thm:all_in_one})
    All the three claims in this theorem are proved together in a single induction argument over $r$. Note that for $r=0$, by definition costs for all actions are $0$ and $V^*=0$. The three claims hold trivially. Hence, we start from $r=1$ as base case in the induction for generalizability. 
    For $r=1$, we consider any $\tb{\ti{s}} \in \mathcal{S}(1)$. We know that the only possible next states are the same state $\tb{\ti{s}}$ or $\tb{\ti{g}}=goal$. For any action $\tb{    \ti{a}} \in \mathcal{A}$ in this state $\tb{\ti{s}}$, by standard arguments we can express the action value function as $Q^*(\tb{\ti{s}},\tb{\ti{a}}) = \frac{1}{1-p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}}}$, where $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}}$ represents the probability of transition from $\tb{\ti{s}}$ to $\tb{\ti{s}}$ itself under action $\tb{\ti{a}}$. The following corollary helps us establish that at action $ a = a_{\theta}$, $Q^*(\tb{\ti{s}}, \tb{\ti{a}})$ is minimum and thus is the optimal action at $\tb{\ti{s}}$.
\pt{instead of writing the following as the corollary, let us use this as a lemma wherever it is required as a part of big theorem}
\begin{corollary}\label{corollary:ps_s}
    From Lemma \ref{lemma:general_tp}, from any state $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$, for any action $\tb{\ti{a}} \in \mathcal{A}$, the probability that the next state is also $\tb{\ti{s}}$ is: 
    \begin{align}
        \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}}) = \frac{r(1-\delta)}{n \cdot 2^{r-1}}+\frac{n-r}{n.2^r}-r.\frac{\Delta}{n} + \frac{2\Delta}{n(d-1)}\sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p})\neq \sgn(\theta_{i,p})\}
    \end{align}
    Clearly, for any $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$, $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ is minimum at $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$ and is only dependent on $r$ for a given instance (independent of $\mathcal{I}$).
\end{corollary}
    
    Note that the above arguments follow for any $\tb{\ti{s}} \in \mathcal{S}(1)$. Also, due to the above corollary, the value is same too. Thus, the second claim holds. As, $V^*_1 > 0$, third claim holds too. 
    Having shown that the three claims hold for the base case, we assume that they hold for all $r \in [k]$ and use this to show that the three claims hold for $r=k+1$ in the same order. For this, we consider any $\tb{\ti{s}} \in \mathcal{S}(k+1)$. 
    For showing $a^* = a_{\theta}$ we again derive expression for optimal action value function $Q^*(\tb{\ti{s}}, \tb{\ti{a}})$. Note that so far we know the optimal actions at only the states in $\cup_{i \in [k]}\mathcal{S}(i)$. If along any sample path starting from this $\tb{\ti{s}}$, we could reach, with any positive probability, any state outside $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}(i)$, it would be impossible to evaluate $Q^*(\tb{\ti{s}}, \tb{\ti{a}})$. But, for our setting all the \textit{reachable} states from $\tb{\ti{s}}$ lie in $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}(i)$ i.e., $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}(i)(\tb{\ti{s}}) \subseteq \cup_{i \in [k] \cup \{0\}}\mathcal{S}(i)$. \textcolor{red}{need to make sure all these notations and definitions are defined in the \ref{subsec:prelims}} Thus $Q^*(\tb{\ti{s}}, \tb{\ti{a}})$ can be expressed appropriately as 
\begin{align}
   Q^*(\tb{\ti{s}}, \tb{\ti{a}}) = 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})Q^*(\tb{\ti{s}}, \tb{\ti{a}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +\sum_{r' \in [k]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'}V^*_{r'} 
\end{align}
    Using the partition of state space based on number of agents at node $s$, identifying that the indicator has positive coefficient if any agent in $\mathcal{I}$ moves from $s$ to $g$ or negative if it stays at $s$,    and using the above induction assumptions, \textcolor{red}{through some clever mathematical manipulations} we show that $Q^*(\tb{\ti{s}}, \tb{\ti{a}})$ is minimized for any $\tb{\ti{s}} \in \mathcal{S}(k+1)$ at $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$. This again requires using Corollary \ref{corollary:ps_s}. Corollary \ref{corollary:p_star} ensures the second claim holds. All the results discussed till now aren't enough to show that $V^*_{k+1}>V^*_k$. We observe that the follwing property holds for our instances:
\begin{property}\label{claim:probability_inequality}
    For all our instances,  for every $r \in [n-1]$, it holds that, for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$. 
\end{property}
The existence of the above property for all our instances helps us use the following lemma to show $V^*_{k+1}>V^*_k$. And thus the main induction over $r$ holds.
\begin{lemma}\label{lemma:probability_inequality}
    If for every $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.
\end{lemma}

\end{proof}

The above theorem provides a broad level of understanding of our features. In the following theorem we provide the main result of this work, namely, tight lower bound in the learning of LM-MASSPs.

\begin{theorem}
\label{thm:lower_bound}
    For any \textcolor{red}{decentralized} MASSP learning algorithm $\mathfrak{A}$ as defined in \ref{subsec:problem_formulation}, there exists a LM-MASSP instance ($\theta \in \Theta$) for every $n \geq 1$, $\delta \in (2/5,1/2)$, $\Delta < 2^{-n}.\frac{1-2\delta}{1+n+n^2}$, such that the expected cumulative regret upon running the algorithm on this instance for $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1. \big \{\frac{1-2\delta}{1+n+n^2} \big \}^2} $ episodes at least matches the reported $\widetilde{O}(\sqrt{K})$ upper bound by \citep{trivedi2023massp} in terms of number of training episodes $K$. Here $V^*_1 = \frac{2n}{n-1+2(\delta+\Delta)}$.  Specifically for this instance, we have $\mathbb{E}_{\theta,\mathfrak{A}}[R(K)] \geq \frac{d.\sqrt{\delta}\sqrt{K.V^*_1}}{2^{n+9}}$     
\end{theorem}

\begin{proof}(of Theorem \ref{thm:lower_bound})
    The proof uses similar techniques as the one for single agent SSP in \cite{min2022learning} and for a two state RL setting by  \cite{jaksch2010near}. But extension to MASSP setting poses many technical challenges such as design of novel features that satisfy the requirements \ref{reqm:1} and \ref{reqm:2}, constructing instance generalizable for any number of agents $n$ with tractable optimal policy, inability to express optimal value function in tractable closed form due to exponentially large number of states, obtaining a reasonably tight upper bound on KL divergence, etc. Some of these challenges are addressed by Theorem \ref{thm:all_in_one}. Others, we deal here. \\
    Consider any history-dependent deterministic policy $\pi$. Consider any set of instances parametrized by fixed $\Big(n \geq 1,\delta \in (2/5,1/2), \Delta < 2^{-n} \cdot \frac{1-2\delta}{1+n+n^2} \Big)$ and differing only due to $\theta \in \Theta$. 
    Suppose agents take actions according to this policy $\pi$. Let, $\tb{\ti{s}}^t$ represent the global state and $\tb{\ti{a}}^t$ the global action at time $t$. Then, the expected regret for the first episode for this instance is: \textcolor{red}{In this discussion I have let time index be superscript}
\begin{align}
R_{\theta,1} &= V^{\pi}(\tb{\ti{s}}^1) - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) \\
     &= \mathbb{E}_{\tb{\ti{a}}^1 \sim\ \pi(\tb{\ti{s}}^1), \tb{\ti{s}}^2 \sim\ \mathbb{P}(.|\tb{\ti{s}}^1,\tb{\ti{a}}^1)}[V^{\pi}(\tb{\ti{s}}^2) - V^{\pi^*_{\theta}}(\tb{\ti{s}}^2)] + \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)}[Q^{\pi^*_{\theta}}(\tb{\ti{s}}^1,\tb{\ti{a}}^1)] - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) 
\end{align} 
The first term indicates a recurrence relationship. The other terms:
\begin{align}
     \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)}[Q^{\pi^*_{\theta}}(\tb{\ti{s}}^1,\tb{\ti{a}}^1)] - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) \\
     &=\mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big \{ \sum_{\tb{\ti{s}} \in \mathcal{S}} [\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}}^1, \tb{\ti{a}}^1) - \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}}^1, \tb{\ti{a}}^1^*)] V^{\pi^*_{\theta}}(\tb{\ti{s}}) \Big \} \\
 &= \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big\{\sum_{\tb{\ti{s}}^2 \neq \tb{\ti{s}}^1} [\mathbb{P}(\tb{\ti{s}}^2|\tb{\ti{s}}^1,\tb{\ti{a}}^1)-\mathbb{P}(\tb{\ti{s}}^2|\tb{\ti{s}}^1, \tb{\ti{a}}^1^*)] V^{\pi^*_\theta}(\tb{\ti{s}}^2)  \Big \}\\
 &\quad +\mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a^1_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}^1) \Big\}
\end{align}
In the above we used the definition of $Q^{\pi^*_{\theta}}(.,.)$ and Lemma \ref{lemma:general_tp} along with $\tb{\ti{s}}^1 = (s,s,\dots,s)$. \\
Due to intractablility of optimum value function, we cannot exactly simplify the above. The following lemma helps us deal with this problem: 
\begin{lemma}\label{lemma:sum_diff_prob_v}
    For any of our instances as defined in \ref{subsec:problem_instance}, for any state $\tb{\ti{s}} \in \mathcal{S}$ and action $\tb{\ti{a}} \in \mathcal{A}$, we have, $\sum_{\tb{\ti{s}}^\prime \neq \tb{\ti{s}}} [P(\tb{\ti{s}}^\prime|\tb{\ti{s}},\tb{\ti{a}})-P(\tb{\ti{s}}^\prime|\tb{\ti{s}}, \tb{\ti{a}}^*)] V^*(\tb{\ti{s}}^\prime) \geq 0  $
\end{lemma}
Further, by recursion over all the time steps $h$ in this episode and using the monotonicity of $V^*$ established in Theorem \ref{thm:all_in_one}, 
\begin{align}
    R_{\theta,1}  \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{1} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\tb{\ti{s}}_h \neq goal \} \mathbbm{1}\{\sgn(a^h_{i,p}) \neq \sgn(\theta_{i,p})\}
\end{align}
where the expectation is with respect to trajectory induced by the policy $\pi$ and transition kernel $\mathbb{P}_{\theta}$ and $a^h_{i,p}$ denotes the $p^{th}$ component of action taken by agent $i$ at time step $h$. Similar analysis can be generalized for all $K$ episodes. \\
For this purpose, we define,  $N = \sum_{t=1}^{\infty} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} $ and for agent $i \in [n]$, $j \in [d-1]$,\\
$N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\} $  

This is to view the global action as an aggregation of multiple components to track how many times sub-optimal component is chosen similar to \citep{auer2002nonstochastic}.

Thus, the regret over all $K$ episodes can be expressed as, 
\begin{align}
    R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]} \sum_{j=1}^{d-1} N_{i,j}(\theta) \}
\end{align}
Standard Pinsker's Inequality cannot be used directly since $N_{i,j}(\theta)$ can be unbounded similar to arguments in \citep{min2022learning}, \citep{rosenberg2020near}. Hence, we define truncated sums to predefined $T$ to further lower bound $R_{\theta}(K)$ as follows: \\
$N^- = \sum_{t=1}^T\mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} $ and for any agent $i \in [n] $ and $ j \in [d-1],$\\ $N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\} $ \\ 
Thus,  $R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}$
\\
Recall that $\theta = (\theta_1,1,\theta_2,1\dots,\theta_n,1)$. We define for every $\theta \in \Theta$ and every $j \in [d-1]$, $\theta^j$ as the vector that is same as $\theta$ at all components except at $j^{th}$ index of every $\theta_i$ for $i \in [n]$ where it is exactly negative. This allows us to write:
\begin{align} \label{eqn:rthetan}
    2 \sum_{\theta \in \Theta} R_{\theta}(K) \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \{ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \} \\
    &= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}
\end{align}
To simplify the first expectation, we derive a generalisation of Lemma C2 of \citep{rosenberg2020near} as below:
\begin{lemma}\label{lemma:gen_co} If $T \geq 2KV^*_1$, then, $\mathbb{E}_{\theta}[N^-] \geq KV^*_1/4$ for any $\theta \in \Theta$
\end{lemma}
The proof of this lemma requires a tight lower bound on the probability of episode length greater than $V^*_1$. To obtain this, we derive the following general lemma and also use the succeeding corollary: 
\begin{lemma}\label{lemma:episodelength}
     Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$ as the probability that starting at state $\tb{\ti{s}} \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in R^+$. Furthermore, $\mathbb{P}^{\pi}[N_k \geq x] = \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$. \\
    Consider any $\tb{\ti{s}} \in \mathcal{S}(r)$ where $r \in [n]$. Then, for any policy $\pi$, it holds for any instance as defined in (ref) that for any $x \in R^+$
    \begin{align}
        \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}')
    \end{align}
    where $\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})$ with equality holding (for all $x \in R^+$) only at $\pi = \pi^*$  and $r'=r $ (i.e., $\tb{\ti{s}}'=\tb{\ti{s}}$) respectively. \\  Here $\pi^*$ is the policy of taking action $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$ (optimal policy from Theorem \ref{thm:all_in_one}). The equality in the middle indicates that under $\pi^*$ (for any fixed $x \in R^+$), $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ stays constant depending only on $r$ for all $\tb{\ti{s}} \in \mathcal{S}(r)$.
\end{lemma}


\begin{corollary}\label{corollary:pn_x}
    An immediate corollary of the above lemma is that $\mathbb{P}^{\pi^*}[N_k \geq x](r)$ is ordered for any $x \in R^+$ i.e., $\mathbb{P}^{\pi^*}[N_k \geq x](n) \geq \mathbb{P}^{\pi^*}[N_k \geq x](n-1) \geq \cdots \geq \mathbb{P}^{\pi^*}[N_k \geq x](2) \geq \mathbb{P}^{\pi^*}[N_k \geq x](1) \geq \mathbb{P}^{\pi^*}[N_k \geq x](0) =0 $
\end{corollary}
The above helps us deal with the first term in Equation \eqref{eqn:rthetan}. The difference in expectation is dealt with using Lemma E.3 from \citep{min2022learning} which is a standard result using Pinsker's Inequality:
\begin{lemma}\label{lemma:pinsk}
If $f:S^T\xrightarrow{}[0,D]$ then, 
$\mathbb{E}_{\mathbb{P}_1} (f(s)) - \mathbb{E}_{\mathbb{P}_2} (f(s))\leq D \sqrt{\frac{log(2)}{2}}. \sqrt{ \kl(\mathbb{P}_2 || \mathbb{P}_1)}$    
\end{lemma}
Finally, we obtain:
\begin{align}
    2 \sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{\kl(\mathbb{P}_{\theta}||\mathbb{P}_{\theta^{j}})}  \} \Big \}
\end{align}
The simplification of KL-divergence in the multi-agent setting is tricky as there are exponential terms involved due to exponential number of possible next states. The bounding techniques used by \citep{jaksch2010near} and \citep{min2022learning} are not adequate. Hence, we derive the following policy independent upper bound on the KL-divergence term by exploiting the symmetries in our problem instance. 
\begin{lemma}\label{lemma:kl_d}
 For our instances, for any policy $\pi $, any $ j \in [d-1]$, $\kl(\mathbb{P}_{\theta} || \mathbb{P}_{\theta^j}) \leq 3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]$ 
\end{lemma}
Using the above lemma, upper bounding $\mathbb{E}_{\theta}[N^-]$ by $T$ and taking $T = 2KV^*_1$, we obtain:
\begin{align}
    \frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq   V_1^*  \Big \{ \Delta  KV_1^*/4 -   (KV_1^*)^{3/2}  \frac{2^{n+2}.\Delta^2}{\sqrt{\delta} (d-1)} \Big \} 
\end{align}  
Finally, picking $\Delta^* = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}$,  ensures we have: \\
$\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{(d-1).\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+8}} \geq \frac{d.\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+9}}$. \\
Since the average of regrets over a set of instances is lower bounded by the RHS, there must exist atleast one instance for whom RHS is a lower bound. \\
But the chosen $\Delta$ must be valid i.e., $\Delta^* < 2^{-n} \cdot\frac{1-2\delta}{1+n+n^2}$. This provides a sample complexity on $K$ as $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.\{\frac{1-2\delta}{1+n+n^2}\}^2} $ where $V^*_1 = \frac{2n}{n-1+2(\delta+\Delta)}$

\end{proof}



\section{Our Approach}
\label{sec:approach}
% 
In this section, we present our approach for establishing regret lower bounds in the LM-MASSP framework.
To this end, we construct a family of LM-MASSP instances that are provably hard to learn. These instances are designed so that the optimal policy is analytically tractable, and any deviation from it incurs a quantifiable regret.

\pt{I am thinking to modify the entire section  as follows - let me know if this makes sense - define each component of the (V, S, A, P) -- While defining the transition probability -- we can give the feature design -- and then define the cost -- and the remark therein -- write the instance defintion -- because now we have all the terms defined. Then i think, we can make the sub-section where we give the lemma 2 -- etc. and while writing the lemma 2, we should define the sets Sr, I, J, etc.... This implies there will not be subsection called Features. Rather we have another subsection. }


\subsection{Construction of Hard-to-Learn LM-MASSP Instances}
\label{subsec:problem_instance}
% 
We consider a minimal yet expressive network with only two nodes: $\mathcal{V} = \{s, g \}$. This induces a global state space $\mathcal{S} = \{ s, g \}^n$ of size $|\mathcal{S}| = 2^n$, where each agent resides at either $s$ or $g$. 
We fix the initial state as $\tb{\ti{s}}_{\init} = (s, s, \dots, s)$ and the goal state as $\tb{g} = (g, g, \dots, g)$. Each agent $i \in [n]$ has the same action set $\mathcal{A}_i = \{-1, 1\}^{d-1}$, for some $d \geq 2$. 
Consequently, the global action space is $\mathcal{A} = \{-1, 1\}^{n(d-1)}$ with $|\mathcal{A}| = 2^{n(d-1)}$. To simplify the dynamics, we assume that once an agent reaches node $g$, it remains there permanently. 
That is, transitions such as $\tb{\ti{s}} = (s, s, \dots, g, g) \rightarrow \tb{\ti{s}}' = (s, s, \dots, g, s)$ are infeasible.



Further, we partition the state space $\mathcal{S}$ depending on the number of agents that are at the node $s$. 
Let $\mathcal{S}_r$ be the subset of the state space for which the number of agents at $s$ are $r$, i.e.,
\begin{align}
    \mathcal{S}_r \coloneqq \Big\{s \in \mathcal{S} : \sum_{i\in \mathbb{N}} \mathbbm{1}_{\{s_i = s\}} = r \Big\}.
\end{align}
For any $r \in \{0\} \cup [n]$, we say that a state $\tb{\ti{s}}$ is of \emph{type} $r$ if $\tb{\ti{s}} \in \mathcal{S}_r$. 
It is easy to observe that the $\cup_{r=0}^n \mathcal{S}_r = \mathcal{S}$, and $\mathcal{S}_{r_1} \cap \mathcal{S}_{r_2} = \emptyset$ for any $r_1 \neq  r_2$. Thus,  $\{ \mathcal{S}_0, \mathcal{S}_1, \dots, \mathcal{S}_n \}$ partitions $\mathcal{S}$. Moreover, for any state $\tb{\ti{s}}$, we define the set $\mathcal{S}(\tb{\ti{s}}) \coloneqq \{ \tb{\ti{s}}' \in \mathcal{S} : \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) >0, ~~ \text{for some}~ \tb{\ti{a}} \in \mathcal{A} \})$ as the set of all the states that are \emph{reachable} in the next step from $\tb{\ti{s}}$.
Further, we define the set $\mathcal{S}_r(\tb{\ti{s}})$ as the set of all the states of \emph{type} $r$ that are \emph{reachable} in the next step i.e., $\mathcal{S}_r(\tb{\ti{s}}) \coloneqq \{ \tb{\ti{s}}' \in \mathcal{S}_r : \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) >0, ~~ \text{for some} ~ \tb{\ti{a}} \in \mathcal{A} \}$.






To analyze any transition, say $\tb{\tb{s}} \rightarrow \tb{\ti{s}}'$ where $\tb{\ti{s}} \in \mathcal{S}_r$ and $\tb{\ti{s}}' \in \mathcal{S}_{r'}$,  we define context dependent sets of agents - $\mathcal{I}\coloneqq\{i_1,i_2,\dots,i_r\}$ as the set of agents at node $s$ in state $\tb{\ti{s}}$, $\mathcal{J} \coloneqq \{j_1,j_2,\dots,j_{n-r}\}$ as the set of agents already at node $g$ in state $\tb{\ti{s}}$ and $\mathcal{T} \coloneqq \{t_1,t_2,\dots, t_{r-r'}\} \subseteq\mathcal{I}$ as the set of agents that move from node $s$ to node $g$ as the global state of the system changes from $\tb{\ti{s}}$ to $\tb{\ti{s}}'$. Note that we say these are context-dependent since $\mathcal{I}, \mathcal{J}$ varies for various $\tb{\ti{s}}$ and $\mathcal{T}$ varies for various $\tb{\ti{s}}, \tb{\ti{s}}'$. Thus we are abusing the notation here a little to avoid notational overhead and the sets must more precisely be denoted as $\mathcal{I}_{\tb{\ti{s}}}, \mathcal{J_{\tb{\ti{s}}'}}$ and $\mathcal{T}_{\tb{\ti{s}}, \tb{\ti{s}}'}$.


% \pt{partitioning of the state space- -- we partition the state space based on r, the number of agents at the state s. $\mathcal{S}_r$ -- of type r... $\mathcal{S}(s)$ -- reachable from $s$. $\mathcal{S}_r(s)$ -- reachable from s of type r. }

\pt{The following instance is defined here, without telling what $\delta, \Delta$ are defined. Not a good idea to use this notation without telling anything about it.} Any of our instance is uniquely represented by a fixed tuple $(n,\delta, \Delta, \theta)$ where $n \geq 1$ is the number of agents, $ \delta \in \left( \frac{2}{5} , \frac{1}{2} \right)$ and $\Delta < 2^{-n} \cdot \frac{1-2\delta}{1+n+n^2}$ are parameters of the features described in the next section and $\theta$ is an $nd$- dimensional vector of the form $\theta = (\theta_1,1, \theta_2,1,\dots,\theta_n,1) \in \Theta$ used to define the transition probability as in Assumption \ref{assm:lfa_prob}, where for each agent $i \in [n]$, the paramter $\theta_i$ is a $(d-1)$ dimensional vector each of whose component takes one of the two values $\left\{-\frac{\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)} \right\}$. For convenience, we will also  use $\widetilde{\theta} = (\theta_1,\theta_2,\dots,\theta_n)$ wherever required.

\begin{remark}
For a general cost and transition probability function, there may in general be a trade-off between policies that moves towards the goal state quickly (i.e.,  minimizing the number of time steps to reach the goal) and the policies that take more time but may (in an overall sense) be cost efficient \citep{tarbouriech2020no}. 
\end{remark}

Such complications lead to intractability of optimal policies. To avoid this in the analysis of our instances, we let for all $\tb{\ti{s}} \in \mathcal{S}\backslash\{\tb{\ti{g}}\}$ and $\tb{\ti{a}} \in \mathcal{A}$, $c(\tb{\ti{s}},\tb{\ti{a}}) = 1$ while for any $\tb{a} \in \mathcal{A}, c(\tb{\ti{g}}, \tb{\ti{a}}) =0$. Hence, the policy that takes us \emph{closer} to goal state is better. This leads to optimal policy being directly influenced by transition probabilities alone.

To convince that we are not considering impossible instances, we have the following:
\begin{remark} \label{rem:cost_one}
    One class of such instances is the one for whom for all $i \in [n], \tb{\ti{a}} \in \mathcal{A}, K^i(\tb{\ti{s}},\tb{\ti{a}}) = \frac{1}{x_i(\tb{\ti{s}},\tb{\ti{a}})}$ for all $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$ and $ K^i(\tb{\ti{g}},\tb{\ti{a}}) = 0$ in Equation \eqref{eqn:ind_cost}. 
\end{remark}
\subsection{Feature Design} 
\label{subsec:features}


For the type of instances mentioned in the previous subsection, we now provide valid features for the transition probability model considered in Assumption \ref{assm:lfa_prob}.


Note that there can be many possible feature designs, but all of them must satisfy the following requirements to produce valid transition probabilities in any of our instances.

\begin{requirements}
    For any $(\tb{\ti{s}},\tb{\ti{a}},\tb{\ti{s}}') \in \mathcal{S}\times\mathcal{A}\times\mathcal{S}$, and 
    $\theta\in \Theta$, the parametrized transition probability satisfies $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}) = \left<  \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}), \theta \right> \geq 0$, and for any $(\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S}\times \mathcal{A}$, $\sum_{\tb{\ti{s}}' \in \mathcal{S}}\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}) = \sum_{\tb{\ti{s}}' \in \mathcal{S}} \left < \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}), \theta \right> = 1$. \label{reqm:1}
\end{requirements}
\begin{requirements}
   If there is a physically impossible transition to some $\tb{\ti{s}}' \in \mathcal{S}$ from some $\tb{\ti{s}} \in \mathcal{S}$, under action $\tb{\ti{a}} \in \mathcal{A}$, then $ \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}) = \left< \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}), \theta \right> = 0$, and if there's a certain transition to some $\tb{\ti{s}}' \in \mathcal{S}$ from some $\tb{\ti{s}} \in \mathcal{S}$ under action $\tb{\ti{a}} \in \mathcal{A}$, then $ \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}) = \left< \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}), \theta \right> = 1$. \label{reqm:2}
\end{requirements}
% 
For our instances, we consider the following feature design
% 
\begin{equation}
\label{eqn:features_global_new}
    \phi(\tb{\ti{s}}' \mid \tb{\ti{s}}, \tb{\ti{a}}) = 
    \begin{cases} 
    \left(\phi_1(s'_1|s_1,a_1),\dots, \phi_n(s'_n|s_n,a_n) \right), & \text{if } \tb{\ti{s}} \neq \tb{\ti{g}} \text{ and } s^{\prime}_i = g \text{ if } s_i = g,~ \forall~ i \in [n] \\
    \mathbf{0}_{nd}, & \text{if } \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}' \neq \tb{\ti{g}}, \text{ or } \tb{\ti{s}} \neq \tb{\ti{g}},~ \exists ~ i \in [n] \text{ s.t. } s_i = g,~ s^{\prime}_i = s \\
    (\mathbf{0}_{nd-1}, 1), & \text{if } \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}' = \tb{\ti{g}}
    \end{cases}
\end{equation}
where
\begin{equation}
\label{eqn:individual_features}
    \phi_i(s^{\prime}_i | s_i, {{a}}_i) = \begin{cases}  
    \left(-{{a}}_i, \frac{1-\delta}{n 2^{r-1}} \right)^{\top}, & \text{if} ~ {s}^i = s^{\prime}_{i} = s
    \\
    \left({{a}}_i, \frac{\delta}{n 2^{r-1}} \right)^{\top}, & \text{if} ~ {s}_i = s,~s^{\prime}_{i} = g
    \\
    \left(\mathbf{0}_{d-1}, \frac{1}{n 2^{r}} \right)^{\top}, & \text{if} ~ {s}_i = g,~ s^{\prime}_{i} = g
    \end{cases}
\end{equation}
% 
In the above, $r$ represents the number of agents at node $s$ in the current global state $\tb{\ti{s}}$.  
%
Observe that in Equation \eqref{eqn:features_global_new} the first case corresponds to the most general transitions that are allowed, the second case represents all impossible transitions and the third case takes care of the only \textit{certain} transition.

\begin{lemma}\label{lemma:valid_features}
    Features defined above in Equations \eqref{eqn:features_global_new} and \eqref{eqn:individual_features}, produce valid transition probabilities for any instance $(n,\delta,\Delta,\theta)$ as defined in \ref{subsec:problem_instance}. Specifically they satisfy both requirements \ref{reqm:1} and \ref{reqm:2}.
\end{lemma}
 The detailed proof is deferred to Appendix \ref{proof:lemma:valid_features}.

Using the above features and transition probability model in Assumption \ref{assm:lfa_prob}, we derive a general expression for the probability of any valid transition for any instance $(n, \delta, \Delta, \theta)$ as defined in Section \ref{subsec:problem_instance}. 

\textcolor{red}{the below lemma statement will simplify depending on if these definitions are incorporated in Section \ref{subsec:prelims}}
% 
\begin{lemma}
\label{lemma:general_tp} 
Consider any state $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$. In this state $\tb{\ti{s}}$, let $\mathcal{I}:=\{i_1,i_2,\dots,i_{r}\}$ denote the set of agents at node $s$ and $\mathcal{J}:=\{j_1,j_2,\dots,j_{n-r}\}$ be those at node $g$. 
Under a valid transition, either the next state is the same as $\tb{\ti{s}}$ or possibly some agents from $\mathcal{I}$ transit to node $g$. Let the set of all valid next states from $\tb{\ti{s}}$ be denoted as $\mathcal{S}(\tb{\ti{s}})$. To study a particular transition to $\tb{\ti{s}}'\in \mathcal{S}(\tb{\ti{s}})$, we define $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ as the set of all agents moving from node $s$ to node $g$. Here, $r'$ denotes the number of agents in state $\tb{\ti{s}}'$ that are at node $s$. For any action $\tb{\ti{a}} \in \mathcal{A}$, the transition probability is given as: 
\begin{align}
    &p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'} = 
 \mathbb{P}(\tb{\ti{s}}^\prime | \tb{\ti{s}}, \tb{\ti{a}}) 
=\frac{r' + (r-2r')\delta}{n \cdot 2^{r-1}} +   \frac{n-r}{n \cdot 2^r}        +    \frac{\Delta}{n}  (r-2r') \\
&\quad + \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn({{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn({{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}
\end{align} 
\end{lemma}


% \pt{The following corollary provides the probability when action are as in Theorem 1. This probability only depends on $r$ and $r'$ only. i am thinking to remove this corollary and put it as the another statement in the above lemma.
% } \textcolor{red}{i dont mind. can we decide upon these things after doing one round of appendix?}


\begin{corollary} \label{corollary:p_star}
From Lemma \ref{lemma:general_tp}, we observe that for any given instance $(n, \delta, \Delta, \theta)$ if the action chosen is such that the indicators vanish in the above expression, the transition probability doesn't depend on $\mathcal{I}$ and $\mathcal{T}$ and only depends on $r$ and $r'$. Hence, we define this special global action $\tb{\ti{a}}_{\theta}$ as the action whose $\{(d-1)\times (i-1)+j\}-th$ element for every $i \in [n]$ and every $j \in [d-1]$ is given by $\sgn(\theta_{i,j})$. In other words,  $\tb{\ti{a}}_{\theta} = \frac{n(d-1)}{\Delta} \times \widetilde{\theta}$. We will denote the associated probabilities as $p^*_{r,r'}$
\end{corollary}

The proof of this lemma is deferred to the Appendix ??. \pt{This will be a common lemma with its sub-part as corollary.}

Next, we would like to highlight why the above described instances are considered and their importance. In particular, we will provide the details on why the instances are hard, and why they one would expect a good/ sub-linear lower bound on the regret.
\textcolor{red}{again no need for this}

\subsection{Summary of Our Approach}
\label{subsec:why_hard_instance}
% 
\pt{I haven't looked at this part as of now.}

Any deterministic algorithm produces, in general, a history-dependent policy. Fixing any such policy $\pi$, we will analyze the regret of this policy on a set of hard to learn instances that differ only due to $\theta$ (i.e., have same parameters $n, \delta, \Delta$) and show that there exists an instance in the set of hard-to-learn instances that achieves lower bound on expected cumulative regret that scales similarly in terms of number of episodes as the upper bound $\widetilde{O}(\sqrt{K})$ reported by \citep{trivedi2023massp}. 
Intuitively, there are two reasons why we expect at least one of the instances in this set to be very hard to be learnt for any given policy:
\begin{itemize}
    \item Firstly, all the instances are characterized by the optimum policy that at any state, the action taken is $\tb{a}_{\theta}$. If we consider a policy such that the action taken in only one of the $2^n-1$ non-goal states differed from $a_{\theta}$ at just one of the $n(d-1)$ indices, then the transition probabilities would differ (from those for optimal policy) only very slightly since $\Delta$ is quite small $(<2^{-n})$. 
Hence, the value function for that policy would be only slightly higher. Observe that there would be $n(d-1).2^{n-1}$ (significant) number of such policies. The policies that differ in the above fashion at any two states are even larger in number and can't be expected to be too worse in terms of the expected cumulative cost for similar reason. Hence, separating these large number of policies efficiently is a challenge before any MASSP learning algorithm. 
\item Secondly, any learning algorithm that efficiently learns the best policy for one instance in the set of all instances, may not be able to efficiently learn some other instance in the set. Also, if a particular action is the best (optimal) for a given instance $\theta = (\theta_1,1,\theta_2,1,\dots,\theta_n,1)$, there definitely exists another instance $\theta = (-\theta_1,1,-\theta_2,1,\dots,-\theta_n,1) \in \Theta$ for whom the same action is the worst.
\end{itemize}
In the following section, we present our observations on these instances and key results that follow.




\pt{We would like to highlight the importance of the instance that we constructed. we would like to highlight why the above described instances are considered and their importance. In particular, we will provide the details on why the instances are hard, and why they one would expect a good/ sub-linear lower bound on the regret.}

% 
\pt{I haven't looked at this part as of now.}

Any deterministic algorithm produces, in general, a history-dependent policy. Fixing any such policy $\pi$, we will analyze the regret of this policy on a set of hard to learn instances that differ only due to $\theta$ (i.e., have same parameters $n, \delta, \Delta$) and show that there exists an instance in the set of hard-to-learn instances that achieves lower bound on expected cumulative regret that scales similarly in terms of number of episodes as the upper bound $\widetilde{O}(\sqrt{K})$ reported by \citep{trivedi2023massp}. 
Intuitively, there are two reasons why we expect at least one of the instances in this set to be very hard to be learnt for any given policy:
\begin{itemize}
    \item Firstly, all the instances are characterized by the optimum policy that at any state, the action taken is $\tb{a}_{\theta}$. If we consider a policy such that the action taken in only one of the $2^n-1$ non-goal states differed from $a_{\theta}$ at just one of the $n(d-1)$ indices, then the transition probabilities would differ (from those for optimal policy) only very slightly since $\Delta$ is quite small $(<2^{-n})$. 
Hence, the value function for that policy would be only slightly higher. Observe that there would be $n(d-1).2^{n-1}$ (significant) number of such policies. The policies that differ in the above fashion at any two states are even larger in number and can't be expected to be too worse in terms of the expected cumulative cost for similar reason. Hence, separating these large number of policies efficiently is a challenge before any MASSP learning algorithm. 
\item Secondly, any learning algorithm that efficiently learns the best policy for one instance in the set of all instances, may not be able to efficiently learn some other instance in the set. Also, if a particular action is the best (optimal) for a given instance $\theta = (\theta_1,1,\theta_2,1,\dots,\theta_n,1)$, there definitely exists another instance $\theta = (-\theta_1,1,-\theta_2,1,\dots,-\theta_n,1) \in \Theta$ for whom the same action is the worst.
\end{itemize}
In the following section, we present our observations on these instances and key results that follow.


\begin{lemma}
\label{lemma:general_tp} 
Consider any state $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$. In this state $\tb{\ti{s}}$, let $\mathcal{I}:=\{i_1,i_2,\dots,i_{r}\}$ denote the set of agents at node $s$ and $\mathcal{J}:=\{j_1,j_2,\dots,j_{n-r}\}$ be those at node $g$. 
Under a valid transition, either the next state is the same as $\tb{\ti{s}}$ or possibly some agents from $\mathcal{I}$ transit to node $g$. Let the set of all valid next states from $\tb{\ti{s}}$ be denoted as $\mathcal{S}(\tb{\ti{s}})$. To study a particular transition to $\tb{\ti{s}}'\in \mathcal{S}(\tb{\ti{s}})$, we define $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ as the set of all agents moving from node $s$ to node $g$. Here, $r'$ denotes the number of agents in state $\tb{\ti{s}}'$ that are at node $s$. For any action $\tb{\ti{a}} \in \mathcal{A}$, the transition probability is given as: 
\begin{align}
    &p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'} = 
 \mathbb{P}(\tb{\ti{s}}^\prime | \tb{\ti{s}}, \tb{\ti{a}}) 
=\frac{r' + (r-2r')\delta}{n \cdot 2^{r-1}} +   \frac{n-r}{n \cdot 2^r}        +    \frac{\Delta}{n}  (r-2r') \\
&\quad + \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn({{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn({{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}
\end{align} 
\end{lemma}



\section{Proof Outline}
\label{sec:proof_outline}

\subsection{Proof Sketch of Theorem \ref{thm:all_in_one}}

\begin{proof} 
% 
The proof uses the principle of Mathematical induction over $r$, that represents the number of agents present at node $s$ in any state $\tb{\ti{s}} \in \mathcal{S}$. In particular, all  the three claims in this theorem are proved together in a single induction argument over $r$. Note that for $r=0$, by definition costs for all actions are $0$ and $V^*=0$. All the three claims hold trivially. Hence, we take $r=1$ as base case in the induction for generalizability.  


\textbf{Base case.} For any state $\tb{\ti{s}} \in \mathcal{S}_1$, the only possible next states are either same state $\tb{\ti{s}}$ or $\tb{\ti{g}}= (g,\dots,g)$. For any action $\tb{    \ti{a}} \in \mathcal{A}$ in this state $\tb{\ti{s}}$, by  standard arguments we can express the value function for any policy $\pi_{\tb{\ti{a}}}$ of choosing action $\tb{\ti{a}}$ at $\tb{\ti{s}}$ as $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}}) = \frac{1}{1-p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}}}$, where $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}}$ represents the probability of transition from $\tb{\ti{s}}$ to $\tb{\ti{s}}$ itself under action $\tb{\ti{a}}$.
The following corollary
helps us establish that at action $ \tb{\ti{a}} = \tb{\ti{a}}_{\theta}$, $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$ is minimum and thus is the optimal action at $\tb{\ti{s}}$.

\begin{corollary}\label{corollary:ps_s}
From Lemma \ref{lemma:general_tp}, from any state $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$, for any action $\tb{\ti{a}} \in \mathcal{A}$, the probability that the next state is also $\tb{\ti{s}}$ is: 
\begin{align}
    \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}}) = \frac{r(1-\delta)}{n \cdot 2^{r-1}}+\frac{n-r}{n.2^r}-r.\frac{\Delta}{n} + \frac{2\Delta}{n(d-1)}\sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \mathbbm{1}\{\sgn({{a}}_{i,p})\neq \sgn(\theta_{i,p})\}
\end{align}
% 
Further, for any $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$, $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ is minimum at $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$ where it is only dependent on $r$ for a given instance (independent of $\mathcal{I}$).
\end{corollary}
% 
Note that the above arguments follow for any $\tb{\ti{s}} \in \mathcal{S}_1$. Also, due to the above corollary, the value is same too. Thus, the second claim holds. As, $V^*_1 > 0$, third claim holds too. This completes the proof for the base case.

\textbf{Inductive Step.} Let us assume that all the three claims of the theorem hold for every $r \in \{1,2, \dots, k\}$, and use this to show that all these claims hold for $r=k+1$ in the same order. 
To this end, consider any $\tb{\ti{s}} \in \mathcal{S}_{k+1}$. To prove the first claim, i.e., $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$ we again derive expression for value function $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$ for any policy $\pi_{\tb{\ti{a}}}$ that chooses action $\tb{\ti{a}}$ at state $\tb{\ti{s}}$ and optimal action $\tb{\ti{a}}_{\theta}$ at all the other reachable states from $\tb{\ti{s}}$.  
Note that so far we know the optimal actions at only the states in $\cup_{i \in [k]}\mathcal{S}_i$. 
If along any sample path starting from this $\tb{\ti{s}}$, we reached, with any positive probability, any state not in $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}_i$, it would be impossible to evaluate $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$. 
Fortunately, for our setting all the \textit{reachable} states from $\tb{\ti{s}}$ lie in $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}_i$ i.e., $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}_i(\tb{\ti{s}}) \subseteq \cup_{i \in [k] \cup \{0\}}\mathcal{S}_i$. 
The state value function in this case can be expressed appropriately as 
\begin{align}
    V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}}) = 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})+\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +\sum_{r' \in [k]} \sum_{\tb{\ti{s}}' \in \mathcal{S}_{r'}(\tb{\ti{s}})} p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'}V^*_{r'}. 
\end{align}
% 
Using the partition of state space based on number of agents at node $s$, identifying that the indicator has positive coefficient if any agent in $\mathcal{I}$ moves from $s$ to $g$ or negative if it stays at $s$, and using the above induction assumptions, \textcolor{red}{through some clever mathematical manipulations} we show that $ V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$ is minimized for any $\tb{\ti{s}} \in \mathcal{S}_{k+1}$ at $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$. \pt{Let us write the exact result/eqn that we use to prove this.}
% 
This again requires using Corollary \ref{corollary:ps_s}. Corollary \ref{corollary:p_star} ensures the second claim holds. Finally to prove that claim 3 holds for our case, we first show that the following lemma holds for all the instances that we consider. 
\begin{lemma}
\label{claim:probability_inequality}
    For all our instances,  for every $r \in [n-1]$, it holds that, for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$. 
\end{lemma}
The existence of the above property for all our instances helps us use the following lemma to show $V^*_{k+1}>V^*_k$. 
\begin{lemma}\label{lemma:probability_inequality}
    If for any $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.
\end{lemma}
This proves the final claim for $r=k+1$. Thus, using the Principle of Mathematical induction it holds for every $r = \{0,1,\dots, n\}$.
This completes the proof.
\end{proof}


\subsection{Proof Sketch of Theorem \ref{thm:lower_bound}}

\begin{proof}
% 
\pt{These few sentences can also be repeated in the appendix. Moreover, we can write is very precisely, not this much detailed.} The proof uses similar techniques as the one for single agent SSP in \cite{min2022learning} and for a two state RL setting by  \cite{jaksch2010near}. But extension to MASSP setting poses many technical challenges such as design of novel features that satisfy the requirements \ref{reqm:1} and \ref{reqm:2}, constructing instance generalizable for any number of agents $n$ with tractable optimal policy, inability to express optimal value function in tractable closed form due to exponentially large number of states, obtaining a reasonably tight upper bound on KL divergence, etc. Some of these challenges are addressed by Theorem \ref{thm:all_in_one}. Others, we deal here. 

Consider any history-dependent deterministic policy $\pi$ \pt{We have a notation for this, $\pi \in \Pi_{\mathrm{HD}}$ ?} and the set of instances parametrized by fixing $n \geq 1$, $\delta \in (2/5,1/2)$, and $\Delta < 2^{-n} \cdot \frac{1-2\delta}{1+n+n^2}$ \pt{the detail of $\theta$ is not clear here. It is part of instance, but how they are differing -- do you mean to say that the instances are differing in $\theta$?}  and differing only due to $\theta \in \Theta$.

Suppose agents take actions according to this policy $\pi$. Let, $\tb{\ti{s}}^t$ represent the global state and $\tb{\ti{a}}^t$ the global action at time $t$. Then, the expected regret for the first episode for this instance is
% 
\begin{align}
    R_{\theta,1} 
    &= V^{\pi}(\tb{\ti{s}}^1) - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) 
    \\
    &= \mathbb{E}_{\tb{\ti{a}}^1 \sim\ \pi(\tb{\ti{s}}^1), \tb{\ti{s}}^2 \sim\ \mathbb{P}(.|\tb{\ti{s}}^1,\tb{\ti{a}}^1)}[V^{\pi}(\tb{\ti{s}}^2) - V^{\pi^*_{\theta}}(\tb{\ti{s}}^2)] + \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)}[Q^{\pi^*_{\theta}}(\tb{\ti{s}}^1,\tb{\ti{a}}^1)] - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) 
\end{align} 
The first term indicates a recurrence relationship. The second term can further written as follows:
\begin{align}
    & \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)}[Q^{\pi^*_{\theta}}(\tb{\ti{s}}^1,\tb{\ti{a}}^1)] - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) 
    \\
    &=\mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big \{ \sum_{\tb{\ti{s}} \in \mathcal{S}} [\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}}^1, \tb{\ti{a}}^1) - \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}}^1, \tb{\ti{a}}^{1^*})] V^{\pi^*_{\theta}}(\tb{\ti{s}}) \Big \} 
    \\
    &= \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big\{\sum_{\tb{\ti{s}}^2 \neq \tb{\ti{s}}^1} [\mathbb{P}(\tb{\ti{s}}^2|\tb{\ti{s}}^1,\tb{\ti{a}}^1)-\mathbb{P}(\tb{\ti{s}}^2|\tb{\ti{s}}^1, \tb{\ti{a}}^1{^*})] V^{\pi^*_\theta}(\tb{\ti{s}}^2)  \Big \}
    \\
    &\quad +\mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a^1_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}^1) \Big\}
\end{align}
In the above we used the definition of $Q^{\pi^*_{\theta}}(\cdot, \cdot)$ and Lemma \ref{lemma:general_tp} along with $\tb{\ti{s}}^1 = (s,s,\dots,s)$.  
However, due to intractablility of optimum value function, we cannot exactly simplify the above. To handle this problem we have the following lemma
% 
\begin{lemma}
\label{lemma:sum_diff_prob_v}
    For any of our instances as defined in Section \ref{subsec:problem_instance}, for any state $\tb{\ti{s}} \in \mathcal{S}$ and action $\tb{\ti{a}} \in \mathcal{A}$, we have, $\sum_{\tb{\ti{s}}^\prime \neq \tb{\ti{s}}} [P(\tb{\ti{s}}^\prime|\tb{\ti{s}},\tb{\ti{a}})-P(\tb{\ti{s}}^\prime|\tb{\ti{s}}, \tb{\ti{a}}^*)] V^*(\tb{\ti{s}}^\prime) \geq 0  $
\end{lemma}
% 
Further, by recursion over all the time steps $h$ in this episode and using the monotonicity of $V^*$ established in Theorem \ref{thm:all_in_one} to lower bound the $V^*$ for each non-goal state in the sum, we have that
% 
\begin{align}
    R_{\theta,1}  \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{1} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\tb{\ti{s}}^h \neq goal \} \mathbbm{1}\{\sgn(a^h_{i,p}) \neq \sgn(\theta_{i,p})\}.
\end{align}
% 
where the expectation is with respect to trajectory induced by the policy $\pi$ and transition kernel $\mathbb{P}_{\theta}$ and $a^h_{i,p}$ denotes the $p^{th}$ component of action taken by agent $i$ at time step $h$.
Similar analysis can be generalized for all $K$ episodes \pt{is this generalization given below?}

For this purpose, we define
$N \coloneqq \sum_{t=1}^{\infty} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\}$, 
and for agent $i \in [n]$, $j \in [d-1]$, we define \pt{write one line description of this notation in plain english. -- This is to view the global action as an aggregation of multiple components to track how many times sub-optimal component is chosen similar to \citep{auer2002nonstochastic}.}
\begin{align}
\label{eqn:N_ij_definition}
    N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\}.
\end{align}
% 
Thus, the regret over all $K$ episodes can be expressed as, 
\begin{align}
    R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]} \sum_{j=1}^{d-1} N_{i,j}(\theta) \}
\end{align}
It is important to note that we can't use the standard Pinsker's inequality here to bound the regret, as $N_{i,j}(\theta)$ can be unbounded. This is along with the similar line to the arguments used in \citep{min2022learning,rosenberg2020near}. 
To further lower bound $R_{\theta}(K)$, we define the truncated sums upto a predefined $T$ as: $N^- = \sum_{t=1}^T\mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\}$, 
and for any agent $i \in [n] $ and $ j \in [d-1]$, we have that
% 
\begin{align}
\label{eqn:N_ij_truncated}
    N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\} 
\end{align}
% 
Thus, the regret upto $K$ episode is bounded as
% 
\begin{align}
    R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \left[ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \right]
\end{align}
% 
Now, recall that $\theta = (\theta_1,1,\theta_2,1\dots,\theta_n,1)$. We define for every $\theta \in \Theta$ and every $j \in [d-1]$, $\theta^j$ as the vector that is same as $\theta$ at all components except at $j^{th}$ index of every $\theta_i$ for any $i \in [n]$ where it is exactly negative. This allows us to write
% 
\begin{align} 
\label{eqn:rthetan}
    2 \sum_{\theta \in \Theta} R_{\theta}(K) 
    &\geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \left[ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \right] 
    \\
    &= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \left[  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \right]
\end{align}
To simplify the first expectation, we generalization the Lemma C2 of \citep{rosenberg2020near} as below
% 
\begin{lemma}
\label{lemma:gen_co} 
    If $T \geq 2KV^*_1$, then, $\mathbb{E}_{\theta}[N^-] \geq KV^*_1/4$ for any $\theta \in \Theta$
\end{lemma}
% 
the detailed proof of this lemma is  deferred to Appendix??. The proof of this lemma requires a tight lower bound on the probability of episode length greater than $V^*_1$. To this, we derive the following general lemma and also use the succeeding corollary
\begin{lemma}\label{lemma:episodelength}
     Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$ as the probability that starting at state $\tb{\ti{s}} \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in \mathbb{R}^+$. Furthermore, $\mathbb{P}^{\pi}[N_k \geq x] = \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$. \\
    Consider any $\tb{\ti{s}} \in \mathcal{S}(r)$ where $r \in [n]$. Then, for any policy $\pi$, it holds for any instance as defined in (ref) that for any $x \in R^+$
    \begin{align}
        \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}')
    \end{align}
    where $\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})$ with equality holding (for all $x \in R^+$) only at $\pi = \pi^*$  and $r'=r $ (i.e., $\tb{\ti{s}}'=\tb{\ti{s}}$) respectively. \\  Here $\pi^*$ is the policy of taking action $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$ (optimal policy from Theorem \ref{thm:all_in_one}). The equality in the middle indicates that under $\pi^*$ (for any fixed $x \in R^+$), $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ stays constant depending only on $r$ for all $\tb{\ti{s}} \in \mathcal{S}(r)$.
\end{lemma}


\begin{corollary}\label{corollary:pn_x}
    An immediate corollary of the above lemma is that $\mathbb{P}^{\pi^*}[N_k \geq x](r)$ is ordered for any $x \in R^+$ i.e., $\mathbb{P}^{\pi^*}[N_k \geq x](n) \geq \mathbb{P}^{\pi^*}[N_k \geq x](n-1) \geq \cdots \geq \mathbb{P}^{\pi^*}[N_k \geq x](2) \geq \mathbb{P}^{\pi^*}[N_k \geq x](1) \geq \mathbb{P}^{\pi^*}[N_k \geq x](0) =0 $
\end{corollary}
The above \pt{corollary or lemma} helps us deal with the first term in Equation \eqref{eqn:rthetan}. The difference in expectation is dealt with using Lemma E.3 from \citep{min2022learning} which is a standard result using the following Pinsker's inequality 
% 
\begin{lemma}
\label{lemma:pinsk}
    If $f:S^T\xrightarrow{}[0,D]$ then, 
    $\mathbb{E}_{\mathbb{P}_1} (f(s)) - \mathbb{E}_{\mathbb{P}_2} (f(s))\leq D \sqrt{\frac{log(2)}{2}}. \sqrt{ \kl(\mathbb{P}_2 || \mathbb{P}_1)}$    
\end{lemma}
% 
Using these results, we obtain
% 
\begin{align}
    2 \sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{\kl(\mathbb{P}_{\theta}||\mathbb{P}_{\theta^{j}})}  \} \Big \}
\end{align}
The simplification of KL-divergence in the multi-agent setting is tricky as there are exponential terms involved due to exponential number of possible next states.
\pt{Need to write this with more details, because this is the novelty part of the proof.} The bounding techniques used by \citep{jaksch2010near} and \citep{min2022learning} are not adequate. Hence, we derive the following policy independent upper bound on the KL-divergence term by exploiting the symmetries in our problem instance. 
% 
\begin{lemma}
\label{lemma:kl_d}
    For our instances and for any policy $\pi $, any $ j \in [d-1]$, we have
    \begin{align}
        \kl(\mathbb{P}_{\theta} || \mathbb{P}_{\theta^j}) \leq 3 \cdot 2^{2n} \cdot \frac{\Delta^2}{\delta (d-1)^2} \cdot \mathbb{E}_{\theta}[N^-].
    \end{align}
\end{lemma}
% 
Using the above lemma, and upper bounding $\mathbb{E}_{\theta}[N^-]$ by $T = 2KV^*_1$, with $\Delta = \Delta^* = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}$ and substituting it in eqn 33, we obtain
\begin{align}\label{eqn:final_avgreg}
    \frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{(d-1) \cdot \sqrt{\delta} \cdot \sqrt{KV_1^*}}{2^{n+8}} \geq \frac{d \cdot \sqrt{\delta} \cdot \sqrt{KV_1^*}}{2^{n+9}}.
\end{align}
Since the average of regrets over a set of instances is lower bounded by the RHS, there must exist atleast one instance for whom RHS is a lower bound. 

Finally to justify that the chosen $\Delta$ is valid i.e., $\Delta = \Delta^* < 2^{-n} \cdot\frac{1-2\delta}{1+n+n^2}$  provides a bound on $K$ as 
\begin{align}
    K > \frac{(d-1)^2 \cdot \delta}{2^{10} \cdot V^*_1 \cdot \{\frac{1-2\delta}{1+n+n^2}\}^2} 
\end{align}
where $V^*_1$ is given by
\begin{align}
    V^*_1= \frac{2n}{n-1+2(\delta+\Delta)}.
\end{align}
This completes the proof.
\end{proof}
\textcolor{red}{it is easy to show that $V^*_1 > V^*_n/n = B^*/n$. So the eqn \ref{eqn:final_avgreg} can be further lower bounded using this relation to $\Omega(2^{-n}d\sqrt{KB*/n})$. Take your call to include n or not for now. We will have to think about this though.}\\

\pt{Does this mean that the $K$ is almost zero? division by a large number $2^{10}$?}



% \pt{Not updated:}  \pt{mathematical manipulation lead to simplification, hence V pi is minimized for a theta. }Using the partition of state space based on number of agents at node $s$, identifying that the indicator has positive coefficient if any agent in $\mathcal{I}$ moves from $s$ to $g$ or negative if it stays at $s$, and using the above induction assumptions, \textcolor{red}{through some clever mathematical manipulations} we show that $ V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$ is minimized for any $\tb{\ti{s}} \in \mathcal{S}_{k+1}$ at $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$. \pt{Let us write the exact result/eqn that we use to prove this.}
% % 
% This again requires using Corollary \ref{corollary:ps_s}. Corollary \ref{corollary:p_star} ensures the second claim holds. Finally to prove that claim 3 holds for our case, we first show that the following lemma holds for all the instances that we consider.  \pt{Move this lemma to section 3.2}
% 

==> CR_Sections/extras2.tex <==
\section{Introduction}
\label{sec:intro}


Our major contributions are as follows:
\begin{itemize}
    \item \textbf{Analysis wrt Number of Agent}
    \item \textbf{Experiments}
\end{itemize}

% \input{CR_Sections/6_experiments}



\subsection{Proof of Lower Bound}
We construct and analyze a family of hard to learn instances. This is the same as in section 1.1. Further, we restrict $\theta$ such that $\theta_{i} \neq \theta_{j}$ $ \forall$ $ i \neq j \in [n]$ i.e., no two $\theta_i$ are the same. Let this set be denoted as $\Theta$. \pt{Why this assumption will hold. there is lot of symmetry in the problem, so $\theta$'s for two agents will be same?}. \textcolor{blue}{It's not an assumption. It's a restriction of the class of SSPs instances I'm considering. I'm free to do so. Why I do this is the rest of paragraph about. Also $\theta$ is an instance parameter, it can be anything. A way to think about this is that : even if two agents took same action, the contribution to probability of transition to any global state is not the same, this is one way how agents are not identical!} This ensures that the action to be taken by each agent to maximize the probability of transition to the all-at-goal state is different for every agent so that we don't need to consider the congestion component of the cost when the policy of maximizing the probability to reach all-goal is executed.
To further reduce complexity of the analysis, we let the private cost associated with any action in the initial state be equal to 1 and that in goal state equal to 0. This ensures that the \textit{best} policy is the one that maximizes the probability of transition to the global goal \pt{goal?} \textcolor{blue}{yes, thanks!} state.  \\
Suppose in episode \textit{k}, agents take actions according to policy $\pi$. Let, $\tb{s}_t$ represent the global state and $\tb{a}_t$ the global action at time $t$. Then, the expected regret for the \textit{k-th} episode is:
\begin{align}
    R_{\theta,k} &= V^{\pi_\theta}(\tb{s}_1) - V^*(\tb{s}_1) 
    \\
    &=  V^{\pi_\theta}(\tb{s}_1) - \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) 
    \\ 
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^\pi(\tb{s}_2)]\}  
    \\ 
    & \quad -\mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^*(\tb{s}_2)] \} + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim\ \pi(\tb{s}_1), \tb{s}_2 \sim\ \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi}(\tb{s}_2) - V^*(\tb{s}_2)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1)
\end{align}

\pt{Suggestion -- for each equation write the proper reason why it is true. This will make it easy to follow. For example, in above the second equation you added and subtracted $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] $.}
\textcolor{blue}{Ok, I'll do it after I start revisiting them. Apart from adding and subtracting Q, I've only expanded the Bellman Equation}

\textcolor{red}{I'm stuck here to find a closed form expression of $Q^*(.,.)$ and $V^*$ due to exponential number of states}

\subsection{Some proofs I have been trying since Monday}
\subsubsection{}
\begin{align} 
    & \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q^{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ c(\tb{s}_1,\tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)] \} - V^{\pi^*}(\tb{s}_1) \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim   \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - V^{\pi^*}(\tb{s}_1) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - (1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)]) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{  \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)] \}
    \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} \{ \sum_{\tb{s} \in \mathcal{S}} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*)) V^{\pi^*}(\tb{s})\}
\end{align}

\\
The above just follows from writing the definition of optimum Action value function and doing some rearrangement and remember costs throughout is 1.
\\

In the below proof, we expand the difference in probability term arising in the above equation. The initial global state, $s_1$, is with all agents at $s_{init}$ and the next state, $s$, is one where agents $i_1,i_2,..,i_r$ remain at $s_{init}$ and those at $j_1,j_2,..,j_{n-r}$ go to goal node. \\
\textcolor{red}{Following stays the same with updated features}

\begin{lalign}
\mathbb{P}(s|s_1, a_1) - \mathbb{P}(s|s_1, a_1^*)  
\\
&= \langle \phi(s|s_1,a_1), \theta \rangle - \langle \phi(s_1|s_1,a_1^*), \theta \rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1), \phi(s_2^{\prime}|s_2, a_2)..., \phi(s_n^{\prime}|s_n,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\& - \langle (\phi(s_1^{\prime}|s_1, a_1^*), \phi(s_2^{\prime}|s_2, a_2^*)..., \phi(s_n^{\prime}|s_n,a_n^*)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1),..., \phi(s_n^{\prime}|s_n,a_n)) - (\phi(s_1^{\prime}|s_1, a_1^*),..., \phi(s_n^{\prime}|s_n,a_n^*)), \\
& (\theta_1, 1,...,\theta_n,1)\rangle 
\\
&= \sum_{m = 1}^{r} \langle \phi(s_{i_m}^{\prime}|s_{i_m},a_{i_m}) - \phi(s_{i_m}^{\prime}|s_{i_m},a^*_{i_m}), (\theta_{i_m}, 1)\rangle \\ 
& + \sum_{m = 1}^{n-r} \langle \phi(s_{j_m}^{\prime}|s_{j_m},a_{j_m}) - \phi(s_{j_m}^{\prime}|s_{j_m},a^*_{j_m}), (\theta_{j_m}, 1)\rangle 
\\
&= \sum_{m=1}^{r} \langle (-a_{i_m} + a^*_{i_m}, 0), (\theta_{i_m}, 1) \rangle + \sum_{m=1}^{n-r} \langle (a_{j_m}-a^*_{j_m}, 0), (\theta_{j_m}, 1) \rangle   
\\
&= \sum_{m=1}^{r} (\langle a^*_{i_m}-a_{i_m}, \theta_{i_m} \rangle)  + \sum_{m=1}^{n-r} (\langle a_{j_m}-a^*_{j_m}, \theta_{j_m}  \rangle)  
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1} (a^*_{i_m, p} - a_{i_m, p})\theta_{i_m, p} \} + \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1} (a_{j_m, p} - a^*_{j_m, p})\theta_{j_m, p} \}
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\} \}  - \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \}
\\
&= \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\}
\end{lalign}
\\
\\
The lines 142-146 we use the linearity assumption and properties of inner product. Then, split the sum on $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Line 150 uses defination of $\phi(.,.)$. 153 uses definition of $a^*$ as the one matching all signs with $\theta$. 
\\

\\



\subsubsection{}
\textcolor{red}{I've updated below with new features} \\
\text{Probability that after taking a global action $\tb{a}$, the next global state is still the same as before i.e., $\tb{s}$}
\begin{lalign}
\mathbb{P}(\tb{s}|\tb{s}, \tb{a})
\\ Linearity Assumption\\
&= \langle \phi(\tb{s}|\tb{s},\tb{a}), \boldsymbol{\theta} \rangle
\\
$Expanded form of features$
\\
&= \langle (\phi(s|s, a_1), \phi(s|s, a_2)..., \phi(s|s,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\
$Definition of Inner Product$
\\
&= \sum_{i = 1}^{n} \langle (\phi(s|s, a_i),(\theta_i,1))
\\
$Definition of Features$
\\
&= \sum_{i = 1}^{n} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}),(\theta_i,1) \rangle
\\
&= \sum_{i = 1}^{n} \{ \langle -a_i, \theta_i \rangle + \frac{1-\delta}{n.2^{n-1}} \}
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \langle a_i, \theta_i \rangle 
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} a_{i,p}. \theta_{i,p} 
\\ $Definition of action and theta$\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Taking summation over p inside$ \\
&=  \frac{1-\delta}{2^{n-1}} - 
 \frac{\Delta}{n(d-1)} \sum_{i = 1}^{n}   \Big\{ d-1 - 2 \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Just simplify$ 
\\
&=  \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
\end{lalign}

\subsubsection{}
\textcolor{red}{i've modified the below for updated features}\\
In this subsection we derive the expression of Probability that if at state $\tb{s} = \{s_{init}, s_{init}, \dots, s_{init}\}$, if global action $\tb{a} = (a_1,a_2,\dots, a_n)$ is taken, you reach $\tb{s}^{\prime}$ where the agents at indices in $\mathcal{I}:= \{ i_1,i_2,\dots, i_r\}$ stay in the same state while agents at indices in $\mathcal{J} := \{j_1,j_2,\dots,j_{n-r} \}$ move to goal state i.e., $s'_{i_1}=s'_{i_2}=\dots=s'_{i_r}=s_{init}$ and $s'_{j_1}=s'_{j_2}=\dots=s'_{j_{n-r}}=goal$. \\
$P(\tb{s}'|\tb{s},\tb{a}) \\ 
= \langle \phi(\tb{s}'|\tb{s},\tb{a}), \theta \rangle \\
= \langle \phi((s'_1,s'_2,\dots, s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n)), (\theta_1, 1, \theta_2, 1,\dots, \theta_n,1) \rangle \\
= \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)),(\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle \phi(s'_i|s_i,a_i), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(s'_j|s_j,a_j), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle (a_j, \frac{\delta}{n.2^{n-1}}), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \Big \{  \frac{1-\delta}{n.2^{n-1}} + \langle -a_i,\theta_i \rangle \Big \} + \sum_{j \in \mathcal{J}} \Big \{ \frac{\delta}{n.2^{n-1}} + \langle a_j, \theta_j \rangle \Big \} \\
= r. \frac{1-\delta}{n.2^{n-1}} - \sum_{i \in \mathcal{I}}    \langle a_i,\theta_i \rangle  + (n-r). \frac{\delta}{n.2^{n-1}} +  \sum_{j \in \mathcal{J}}  \langle a_j, \theta_j \rangle  \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}} -  \sum_{i \in \mathcal{I}} \{ \sum_{p = 1}^{d-1} a_{i,p}.\theta_{i,p} \} + \sum_{j \in \mathcal{J}} \{ \sum_{p = 1}^{d-1} a_{j,p}.\theta_{j,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \{
\sum_{j \in \mathcal{J}}   a_{j,p}.\theta_{j,p}  -  \sum_{i \in \mathcal{I}}  a_{i,p}.\theta_{i,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \Big \{
\sum_{j \in \mathcal{J}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{j,p}) = sgn(\theta_{j,p})\} - \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{
\sum_{j \in \mathcal{J}}  \Big[ 1 - 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}}  \Big[   1 - 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{  \Big[ n-r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] - \Big[  r - \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
\sum_{p = 1}^{d-1}  \Big \{  n-2r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
  \Big \{  (d-1)(n-2r) - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\frac{\Delta . (n-2r)}{n} +\frac{2 \Delta}{n(d-1)} . 
  \Big \{  \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}     \Big \} \\
$ 
\\
Lines 186-190 follow by linearity assumption, definition of features and splitting the dot product over $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Lines 191-195 simplify the dot product and rearrange terms. Line 196 uses definition of action and theta. The remaining lines simplify the summations and rearrange the terms.
\\
From the above expression, we conclude that this probability remains same (say, $p_{a,r}$ for subsequent discussions,  for all states $s \in \mathcal{S}_{n,r}$ for every $r \in [n]$ for $a = \{a_1,a_2,\dots,a_n\}$ given global action taken at $s = \{s_{init}, s_{init},\dots, s_{init}\}$.  \\

\textcolor{blue}{state this as a lemma}
\textcolor{red}{done}

A more general result of the above relates to transition probability from some $s \in \mathcal{S}_{n,r}$ to some $s' \in \mathcal{S}_{n,r'}(s)$ where $\mathcal{S}_{n,r'}(s)$ represents the possible states of type $r'$ reachable from $s$ i.e.m   $0 \leq r' \leq r \leq n$. We discuss this below. \\ 
\textcolor{red}{I've modified this for the updated features}

\\
\textbf{Lemma}: For an instance defined by $\theta \in \Theta$, and a global action $a=\{a_1,a_2,\dots, a_n\} \in \mathcal{A}$, the transition probability for any possible transition from $\mathcal{S}_{n,r}$ to $\mathcal{S}_{n,r'}$, for $n \geq r \geq r' \geq 0$ is constant depending on only r and $r'$. \textcolor{red}{Not true!!!, true when $a^i$ are same} \\ \\ 

\textcolor{blue}{need to include the condition on relative values on $r$ and $r'$ in the statement of lemma } 
\textcolor{red}{Done}

\textcolor{blue}{and perhaps others also} 
\textcolor{red}{definition of notations will already be present in the notations part of the paper, also i've introduced them earlier}

\textcolor{blue}{we will revisit the statement of this as per the proof} \\ \textcolor{red}{I've added a small paragraph below giving an overview of what has been done, i don't think we can simplify further}

Suppose $s$ is such that agents at index in $\mathcal{I}:= \{i_1,i_2,\dots, i_r\}$ are at $s_{init}$ and those at $\mathcal{J} := \{j_1,j_2,\dots, j_{n-r}\}$ are already at goal. Let agents in $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ be the ones transiting from $s_{init}$ to $goal$ i.e., $s \in \mathcal{S}_{n,r}$ and $s' \in \mathcal{S}_{n,r'}$ where $n \geq r \geq r' \geq 0$ and $n \geq 1$. \\ \\
$P(s'|s,a)  \\= \langle \phi(s'|s,a), \theta \rangle  \\= \langle \phi((s'_1,s'_2,\dots,s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n) ), (\theta_1,1,\theta_2,1,\dots,\theta_n,1)\rangle  \\ = \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots, \theta_n,1) \rangle  \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle \phi(s|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle \phi(g|s,a_t), (\theta_t,1) \rangle \\ 
= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle (-a_i, \frac{1-\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle (a_t, \frac{\delta}{n.2^{r-1}}), (\theta_t,1) \rangle \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \{ \frac{1-\delta}{n.2^{r-1}} + \langle -a_i, \theta_i \rangle \} + \sum_{j \in \mathcal{J}}   \frac{1}{n.2^{r}}  + \sum_{t \in \mathcal{T}} \{ \langle a_t,\theta_t  \rangle + \frac{\delta}{n.2^{r-1}} \}   \\=  r'. \frac{1-\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}  + (r-r'). \frac{\delta}{n.2^{r-1}} + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}   + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} a_{i,p}. \theta_{i,p}      + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   a_{t,p} .\theta_{t,p}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} -  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{t,p}) = sgn(\theta_{t,p})\} -  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}}  \frac{\Delta}{n(d-1)} \Big \{  d-1 -  2 \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}}    \frac{\Delta}{n(d-1)} \Big \{  d-1 - 2\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} -   \frac{\Delta}{n(d-1)} \Big \{  r'(d-1) -  2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     +    \frac{\Delta}{n(d-1)} \Big \{  (r-r').(d-1) - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n(d-1)} \Big \{  (r-2r').(d-1) + 2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}
$ 

\pt{this incorporates the new features. Also, this will be the optimal probability when the sign matching property holds.}

\textcolor{blue}{we can avoid `line break' commands above } \textcolor{red}{ok, removed them but now proof may seem clumsier}  \textcolor{blue}{ok, we will see a way out, perhaps, we will introduce them}



\textcolor{blue}{we should use available  macros for lemma, proof, etc. see the style file.} 

\textcolor{blue}{these help where the proof starts and importantly ends -- Paul Halmos tomb-stone mark}
\textcolor{red}{ok, this is new for me. i'll try to learn this.}


Initial lines (not mentioning number since it is changing as we are modifying content above) use linearity assumption, definition of features and decomposing the inner product over agents who remain put at $s_{init}$, transit to goal and remain put at goal. In the next few lines, we expand the inner product terms and summations, use the definition of actions and theta and rearrange. Then, just rearrange different terms.  The indicators make sure appropriate sign is given to the dot product depending on signs of components of action and that of theta, \textcolor{blue}{we will cite some papers about these signs }. 

\textcolor{blue}{this is helpful to the reader}

\textcolor{blue}{let's write the role of indicator function above} \textcolor{red}{role as in?}


\\
\\
Notice that for a given global action, the  transition probability from any $s \in \mathcal{S}_{n,r}$ to any $s' \in \mathcal{S}_{n,r'}$ as long as the transition is possible (i.e., $s' \in \mathcal{S}_{n,r'}(s)$) remains the same as above. 

\textcolor{red}{This para is not complete yet!}Further, for any valid $r'$, one can verify that for any action the above probability decreases with $r$ when the sufficient condition holds : $n-1 < \log_2(\frac{\delta.n}{\Delta}.ln(2)).$ We need to assure that we select $\delta$ and $\Delta$ such that this assumption holds. Typically, we will take $\delta = O(2^n\Delta)=o( 1)$.
 \\
 Hence, $p_{a,r}(m) < p_{a,r}(n)$ for every $r$, $m>n$ for any global action $a$. 
 
Another important probability is that of transition to global goal state after taking a global action a in any state $s \in \mathcal{S}_{n,r}$. \\  \\
\textcolor{red}{I've changed below expressions for the updated feature}
\\
\\
 $ P(s'=(g,g,\dots,g)|s,a) \\ = \langle \phi(s' = (g,g,\dots, g)|(s,a)), \theta \rangle \\ = \langle (\phi(g|s_1,a_1), \phi(g|s_2,a_2),\dots, \phi(g|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle \phi(g|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle (a_i, \frac{\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j,1) \rangle \\ = \frac{r\delta}{n2^{r-1}} + \sum_{i \in \mathcal{I}} \langle a_i,\theta_i \rangle + \frac{n-r}{n2^{r}} \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  a_{i,p} \theta_{i,p} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}}  \frac{\Delta}{n(d-1)} \Big\{ d-1 - 2  \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
  \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  +  \frac{r \Delta}{n} - \frac{2 \Delta}{n(d-1)} \sum_{i \in \mathcal{I}}    \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
 $
\\
\\
This is very similar to above proofs and no new idea is used, only the state is explicitly mentioned.
\\

\textcolor{blue}{write this as another lemma} \textcolor{red}{i had written this before writing the above general proof which is now a lemma. this one is specific for r=n and r'=0 which game me an idea of how to express for general case. should this be a lemma or corollary } \textcolor{blue}{yes, as said over phone. }

\subsubsection{Another way to think of Q-V difference introduced in 1.4.1\textcolor{blue}{this is advantage function, isn't?}} \textcolor{red}{yes, it's like expected value of the advantage function since there is expectation over $a_1$ according to the policy \\ also i've modified below for new features}
\\
\\
In the below, $s_t$ represent global state at time t (Note it's not individual state). Similarly $a_t$ is global action at t.

\begin{lalign} }

$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1) \\
= \mathbb{E}_{a_1 \sim \pi(s_1)}[c(s_1, a_1) + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}V^*(s_2)] - V^*(s_1)  $ \\
Using Bellman Equation and cost is 1
\\ 
$=  \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{  1 + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}[V^*(s_2)] - V^*(s_1) \Big \}$
\\ Expand the Expectation $ \\
=   \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  P(s_1|s_1,a_1) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1) \Big \}
\\ $ Use expression of probability from above$
 \\= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2)  - V^*(s_1) \Bigg \}
\\$ Rearranging the terms $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*(s_1) \Big\} 
\\ $ Notice from the general expression of probability from previous proof $\\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - V^*(s_1) \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} 
\\$ Expand V*(s_1) $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 + P(s_1|s_1,a_1^*)  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - \Big\{ 1 +  P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1, a_1^*) V^*(s_2) \Big\} \Bigg \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p})\neq sgn(\theta_{i,p})\} V^*(s_1) \Big\} 
\\$ Rearrange and combine  terms$ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $
\end{lalign}

\subsubsection{Symmetry in the features lead to identical Value function of similar states}
Suppose there n agents. Let $\mathcal{S}_{n,r}$ represent the set of all states where r agents are at $s_{init}$ (Recall, $\mathcal{I}$ and $\mathcal{J}$). Note that |$\mathcal{S}_{n,r}$| = $\binom{n}{r}$. We claim that these have the same optimum value functions.  \\ \\
\textbf{Proof} \\
Use induction arguments. \\ For r = 1, \\
for any $s \in \mathcal{S}_{n,1}$, the only next possible states are $'s'$ itself and g = (goal,goal,..,goal). Suppose agent i is the one who is only at $s_{init}$. Then, \\
\begin{lalign}
    $V^*(s) = 1 + P(s|s,a^*) V^*(s) + P(g|s,a^*) V^*(g)$ \\
    But, $V^*(g) = 0$. \\
    Thus, $V^*(s) = \frac{1}{1-P(s|s,a^*)} = \frac{1}{P(g|s,a^*)}$ \\ \\
    Now, $P(g|s,a)  \\
    = \langle \phi((s^{\prime}_{1}=g,s^{\prime}_2=g,..,s^{\prime}_{i-1}=g, s^{\prime}_{i}=g,s^{\prime}_{i+1}=g..s^{\prime}_n = g)|(s_1 =g, s_2 = g,..,s_{i-1} = g, s_i = s, s_{i+1}=g,...s_n = g ), (a_1,a_2,...,a_n)), (\theta_1,1, \theta_2,1,..\theta_n,1) \rangle \\
    = \langle (\phi(g|g,a_1), \phi(g|g,a_2),...,\phi(g|g,a_{i-1}), \phi(g|s,a_{i}), \phi(g|g,a_{i+1}),...,\phi(g|g,a_n)), (\theta_1,1,\theta_2,1,...,\theta_n,1)\rangle \\
    = \langle \phi(g|g,a_1), (\theta_1,1) \rangle + \langle \phi(g|g,a_2), (\theta_2,1) \rangle + ... + \langle \phi(g|g,a_{i-1}), (\theta_{i-1},1) \rangle + \langle \phi(g|s,a_i), (\theta_i,1) \rangle, \langle \phi(g|g,a_{i+1}), (\theta_{i+1},1) \rangle + ... + \langle \phi(g|g,a_n), (\theta_n,1) \rangle \\
    = \langle (0_{d-1}, \frac{1}{n.2^1}), (\theta_1,1) \rangle + \langle (0_{d-1}, \frac{1}{n.2^1}), (\theta_2,1) \rangle + ... + \langle (0_{d-1}, \frac{1}{n.2^1}), (\theta_{i-1},1) \rangle + \langle (a_i, \frac{\delta}{n.2^0}), (\theta_i,1) \rangle, \langle (0_{d-1}, \frac{1}{n.2^1}), (\theta_{i+1},1) \rangle + ... + \langle (0_{d-1}, \frac{1}{n.2^1}), (\theta_n,1) \rangle \\
    = \frac{n-1}{2n} + \frac{\delta}{n} + \langle a_i, \theta_i \rangle$
\end{lalign}
\\
Thus, \\ $P(g|s,a^*) = \frac{n-1}{2n} + \frac{\delta}{n} + \langle a^*_i, \theta_i \rangle = \frac{n-1}{2n} + \frac{\delta}{n} + \frac{\Delta}{n}$
\\
Hence, $V^*(s) = \frac{1}{\frac{n-1}{2n} + \frac{\delta}{n} + \frac{\Delta}{n}}$ \\
\textcolor{red}{Note that at n=1, we recover Min et al solution}\\
\pt{This is with the updated features? This  optimal value is for the case when the number of agents at $s_{init}$ are 1.} 
\textcolor{red}{yes, with the ones matching Min et al}

Since we made no assumption regarding $'i'$, the above argument holds for any $i \in [N]$ due to which $V^*(s)$ will be same as above for any $s \in \mathcal{S}_{n,1}$ \\
Thus, we have shown truth for the base case. \\
Now assuming true for $1, 2,\dots,r-1$, we want to prove for $r$. \\
To rephrase, assuming that $V^*(s) = V^*_m$ $\forall$ $s \in S_{n,m}$ holds for every $m = 1, 2,...r-1$, we wish to prove the same for $r$ \\
Consider arbitrary $s \in S_{n,r}$ in which the agents indexed $i_1, i_2, ..., i_{r}$ are at $s_{init}$ while others are at $goal$. \\
The set of all possible next states is given by: $\mathcal{S^{\prime}}:= \bigcup \limits_{r'=0}^{r} \mathcal{S}_{n,r'}(s)$ where $\mathcal{S}_{n,r'}(s)$ denotes the subset of $\mathcal{S}_{n,r'}$ that is reachable from $s$. Note that not all states in $\mathcal{S}_{n,r'}$ are reachable from $s$ since some of those transitions would correspond to the impossibility condition. Precisely speaking, $|\mathcal{S}_{n,r'}(s)| = \binom{r}{r'}$ which does not depend on which $s$ is being considered from $\mathcal{S}_{n,r}$
\\
Hence, \\
$V^*(s)\\ 
= \sum_{s^{\prime} \in \mathcal{S}^{\prime}} \{P(s^{\prime}|s,a^*).[1+V^*(s^{\prime})]\}
\\
= 1 + \sum_{s^{\prime} \in \mathcal{S}^{\prime}} \{P(s^{\prime}|s,a^*).V^*(s^{\prime})\}\\  \\ $Definition of V*, expand the summation and simplify$ \\ \\
= 1 + P(s|s,a^*).V^*(s) + \sum_{s^{\prime} \in \mathcal{S}_{n,r-1}(s)} P(s^{\prime}|s,a^*).V^*(s^{\prime}) + \sum_{s^{\prime} \in \mathcal{S}_{n,r-2}(s)} P(s^{\prime}|s,a^*).V^*(s^{\prime}) + \dots +  \sum_{s^{\prime} \in \mathcal{S}_{n,1}(s)} P(s^{\prime}|s,a^*).V^*(s^{\prime})
$ \\ 
Using the result above that $P(s'|s,a)$ only depends of $r$ and $r'$, for $a^*$ lets denote that by $p^*_{r,r'}$ \\
$V^*(s) \\
= 1 + P(s|s,a^*) V^*(s) + \sum_{s^{\prime} \in \mathcal{S}_{n,r-1}(s)} p^*_{r,r-1} V^*_{r-1} + \sum_{s^{\prime} \in \mathcal{S}_{n,r-2}(s)}p^*_{r,r-2} V^*_{r-2} + \dots + \sum_{s^{\prime} \in \mathcal{S}_{n,2}(s)} p^*_{r,2} V^*_{2} + \sum_{s^{\prime} \in \mathcal{S}_{n,1}(s)} p^*_{r,1} V^*_{1} \\  \\ $Taking the induction hypothetsis to be true till $r-1$, also note that $p^*_{r,j}$ is the probability to reach a fixed state of type j starting at s (refer how s is defined again above) and taking global optimal action. Since this is the same for every state of that type the cardinality of respective set appears. \\ \\
$= 1 + P(s|s,a^*) V^*(s) + |\mathcal{S}_{n,r-1}(s)| p^*_{r,r-1} V^*_{r-1} +  |\mathcal{S}_{n,r-2}(s)|p^*_{r,r-2} V^*_{r-2} + \dots + |\mathcal{S}_{n,2}(s)| p^*_{r,2} V^*_{2} + |\mathcal{S}_{n,1}(s)| p^*_{r,1} V^*_{1}$ \\
 \\
 Hence, \\
 $V^*(s) = \{1 + |\mathcal{S}_{n,r-1}(s)| p^*_{r,r-1} V^*_{r-1} +  |\mathcal{S}_{n,r-2}(s)|p^*_{r,r-2} V^*_{r-2} + \dots + |\mathcal{S}_{n,2}(s)| p^*_{r,2} V^*_{2} + |\mathcal{S}_{n,1}(s)| p^*_{r,1} V^*_{1} \} . \{ 1 - P(s|s,a^*) \}^{-1}$
 \\
 \\
Notice that only the factor $\{1 - P(s|s,a^*)\}$ potentially depends on which s is chosen among $\mathcal{S}_{n,r}$. All other terms are constant and independent of which $s \in \mathcal{S}_{n,r}$ we are considering. To prove that $V^*(s)$ is same for every $s \in \mathcal{S}_{n,r}$, it is thus sufficient to show that this factor is same for every $s \in \mathcal{S}_{n,r}$. Below, we establish this: \pt{This can also be written as a separate lemma and we can use that lemma here directly.} \textcolor{red}{In the general transition probability lemma, putting r=r'=n gives this result. So lets state it as a corollary to that lemma. }
\\
$P(s|s,a^*) \\
= \langle \phi(s|s,a^*), \theta \rangle \\
= \langle (\phi((s'_1,s'_2,\dots,s'_n)|(s_1,s_2,\dots,s_n),(a_1^*,a_2^*,\dots,a_n^*))), (\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\
= \langle (\phi(s'_1|s_1,a_1^*), \phi(s'_2|s_2,a_2^*),\dots,\phi(s'_n|s_n,a_n^*)),(\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\
= \sum_{m = 1}^{n} \langle \phi(s'_m|s_m,a_m^*),(\theta_m,1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle \phi(s'_i|s_i,a_i^*),(\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(s'_j|s_j,a_j^*),(\theta_j,1) \rangle
\\
= \sum_{i \in \mathcal{I}} \langle \phi(s|s,a_i^*),(\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j^*),(\theta_j,1) \rangle
\\
= \sum_{i \in \mathcal{I}} \langle (-a^*_i,\frac{1-\delta}{n.2^{r-1}}),(\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^r}),(\theta_j,1) \rangle
\\
= \sum_{i \in \mathcal{I}}  \{ \frac{1-\delta}{n.2^{r-1}} + \langle -a^*_i,\theta_i \rangle \} + \sum_{j \in \mathcal{J}} \frac{1}{n.2^r} 
\\
= \sum_{i \in \mathcal{I}}  \{ \frac{1-\delta}{n.2^{r-1}} - \frac{\Delta}{n} \} + \frac{n-r}{n.2^r}  
\\
= r. \frac{1-\delta}{n.2^{r-1}} - r. \frac{\Delta}{n}  + \frac{n-r}{n.2^r}  
 \\$
The above calculation is similar in spirit to the ones in earlier section. The idea is to use linearity model of transition probability, definition of features, split the summation into two sets as earlier defined, use definition of action and theta$ \\
$
Observe that we had chosen arbitrary $s \in \mathcal{S}_{n,r}$ for whom the expression only depends on r. But this is same for every $s \in \mathcal{S}_{n,r}$. Hence, $P(s|s,a^*)$ is same for every $s \in \mathcal{S}_{n,r}$. Thus, $V^*(s)$ is same for every $s \in \mathcal{S}_{n,r}$. \\
Hence, proved. \\
\textcolor{red}{I've also modified the above proof for new features}

\\ \\

We also show below that $V_m^*$ are ordered i.e., $V_1^* < V^*_2 < V^*_3 < \dots < V^*_r <V^*_{r+1}<\dots<V^*_n$ \\
Use Induction arguments \\
For r = 1, it's easy to see using Bellman Equation that \\
$V^*_1 = 1 + (1-p^*).V^*_1 + p^*. 0 \implies V_1^* = \frac{1}{p^*}$ \\ 
In above, $p^*$ is the transition probability of the system to the global goal state under optimum  global action $a^*$ taken at some $r=1$ state. 
\\
Assuming true for every $m \in \{1, 2,\dots , r-1\}$, we try to prove for $r$. Again, using Bellman Equation, \\
$V^*_r = 1 +  p^*_{r,r} . V^*_r + \binom{r}{r-1} p^*_{r,r-1}. V^*_{r-1} + \sum_{m=1}^{r-2} \binom{r}{m} p^*_{r,m}.V^*_m \\ \implies V^*_r = \frac{1 + r.p^*_{r,r-1}. V^*_{r-1} + \sum_{m=1}^{r-2} \binom{r}{m}p^*_{r,m}.V^*_m}{1-p^*_{r,r}}$ \\ 
\\
It is thus sufficient to prove that $V^*_r > V^*_{r-1}$ \\
$V^*_r - V^*_{r-1} = \frac{1 + r.p^*_{r,r-1}. V^*_{r-1} + \sum_{m=1}^{r-2} \binom{r}{m}p^*_{r,m}.V^*_m}{1-p^*_{r,r}} - \{ 1+p^*_{r-1,r-1}V^*_{r-1} + \sum_{m=1}^{r-2} \binom{r-1}{m}p^*_{r-1,m}.V^*_m\} \\ > 1 + r.p^*_{r,r-1}. V^*_{r-1} + \sum_{m=1}^{r-2} \binom{r}{m}p^*_{r,m}.V^*_m - \{ 1+p^*_{r-1,r-1}V^*_{r-1}+\sum_{m=1}^{r-2} \binom{r-1}{m}p^*_{r-1,m}.V^*_m\} > 0 $ \\  \textcolor{red}{This is incomplete as of now but very important to show. Possibly i will have to redesign the features. EVEN THIS SEEMS VERY DIFFICULT! \\ This problem has been resolved now.  } 

\pt{Why do you need to change the features now?}\\
\textcolor{red}{to ensure monotonicity of V*}

Hence, $V^*_{r} > V^*_{r-1}$





\subsubsection{Dealing with the sum of Probability differences in 1.4.4 using 1.4.5} 

Recall from 1.4.4, \\ 
$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)   
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \\
 \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 The first term is problematic and it is not clear how to deal with it. Let's investigate the summation inside the expectation of the first term: \\ 
 $\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2) \\ = \sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} [P(s'|s_1,a_1)-P(s'|s_1, a_1^*)] V^*(s') $ (Now, use results from above sections) \\
 = $\sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\} V^*_r $ \\
= $\frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{\sum_{s' \in \mathcal{S}_{n,r}} [\{   \sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p}) \}]  \Big\}   \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n}   
 \sum_{s' \in \mathcal{S}_{n,r}} [ \mathbbm{1}\{s'_i = s_{init}\}   \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   - \mathbbm{1}\{s'_i = goal\}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \}]  \Big\} \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  
 \sum_{s' \in \mathcal{S}_{n,r}} \mathbbm{1}\{s'_i = s_{init}\}     -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \sum_{s' \in \mathcal{S}_{n,r}} 
 \mathbbm{1}\{s'_i = goal\} \Big\}  \Big\} 
 \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \binom{n-1}{r-1}    -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \binom{n-1}{r} \Big\}  \Big\} \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \{ \binom{n-1}{r-1}    -   \binom{n-1}{r} \} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} V^*_r  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} + V^*_{n-r}  \frac{2(n-r)-n}{n} \binom{n}{n-r} \} \Big\}   \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} - V^*_{n-r}  \frac{2r-n}{n} \binom{n}{r} \} \Big\}  \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  - V^*_{n-r}   \} \frac{2r-n}{n} \binom{n}{r} \Big\} \geq 0. 
 $ \\
 \\
 Observe that when $r> n/2, V^*_r > V^*_{n-r}$ and vice-versa (refer result above) \\
 Hence we have established that, \\
 $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1) \geq \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\ \\
 To generalize, we need to show that the above inequality holds for any $s_1 \in \mathcal{S}$ and not just $s_{init}$. We will use this result below.

 \subsubsection{Now going back to Lower Bound Proof with Inequality using above result}
 From 1.3, expected regret in the $k-th$ episode: \\
$R_{\theta,k} \\ = V^{\pi_\theta}(s_1) - V^*(s_1) 
\\ 
 = \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)$ \\
\\ Using 1.4.6, \\

 $R_{\theta,k} \\ \geq  \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_1 \neq goal \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 By recursion and the generalized result from the section above,
 we have: \\

 $R_{\theta,k} \\ \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{k} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_h \neq goal \} \mathbbm{1}\{sgn(a^h_{i,p}) \neq sgn(\theta^h_{i,p})\} \Big\} \\ \geq \frac{2 \Delta B^*}{n^2(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{k} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_h \neq goal \} \mathbbm{1}\{sgn(a^h_{i,p}) \neq sgn(\theta^h_{i,p})\} \Big\} $ \\
 where, the Expectation is taken with respect to trajectory induced in the $k-th$ episode by the interaction of policy $\pi$ and transition kernel $P_{\theta}$. Also, as discussed later, $B_*/n \leq V^*_1$ Now, the total expected regret over $K$ episodes is: \\
 $
 R_{\theta}(K) \\
 \geq   \frac{2 \Delta B^*}{n^2(d-1)} \sum_{t=1}^{\infty} \mathbb{E}_{\theta, \pi} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_t \neq goal \} \mathbbm{1}\{sgn(a^t_{i,p}) \neq sgn(\theta^t_{i,p})\} \Big\}
 $ \\
 Analogous to Min et al, Cohen et al, we define: \\
 $N = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} $ and for agent $i \in [n]$,\\
$N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta^t_{i,j})\} $  \\
Thus, $R_{\theta}(K) \geq \frac{2 \Delta B^*}{n^2(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]} \sum_{j=1}^{d-1} N_{i,j}(\theta) \}$ \\
To use the standard Pinsker's Inequality, we need $N_j(\theta)$ to be bounded almost surely which is known to not hold for SSPs (Min et al, Cohen et al). Hence, we use the capping trick introduced by Cohen et al and also used by Min et al. In this trick, we cap the learning process to a predetermined T. If the learning process (i.e. $K-th$ episode) ends before this, the agents continue to remain at $goal$. In this case the summation for the actual process and the capped process is the same. On the other hand when K episodes end beyond T, we have a truncated sum. Due to non-negativity of each part, the sum for the capped process lower bounds the actual sum. \\ Define \\ $N^- = \sum_{t=1}^T\mathbbm{1}\{s_t \neq goal\} $ and for any agent $i \in [n] $ and $ j \in [d-1],$\\ $N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta^t_{i,j})\} $ \\ 
It is easy to see that for any $i \in [n]$ and $j \in [d-1]$, $N^- =   N^-_{i,j}(\theta) + N^-_{i,j}(\theta^{j})  $ \\ where for every $\theta$, $\theta^j$ represents the vector that only differs at the $j-th$ index of every $\theta_i$ in $\theta = \{\theta_1,1,\theta_2,1,\dots,\theta_n,1\}$, where each $\theta_i \in \{\frac{-\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}\}^{d-1}$. \\ 
Thus,  $R_{\theta}(K) \geq \frac{2 \Delta B^*}{n^2(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}$.  Notice that $\theta \in \Theta \iff \theta^{j} \in \Theta$ (This follows from definition of $\Theta$ \textcolor{red}{without this, following equation won't hold}). Then, we have: \\
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{2 \Delta B^*}{n^2(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \{ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \} \\
= \frac{2 \Delta B^*}{n^2(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^- - N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta B^*}{n^2(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^-] - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta B^*}{n^2(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}

Need to prove generalisation of Lemma C2 in Cohen et al 2020: If $T \geq 2KB^*$, then $\mathbb{E}_{\theta}[N^-] \geq KB^*/4$  \\ \textcolor{red}{Suppose same holds, we pick $T = 2KB_*$} \\
\textbf{Pinsker's Inequality(Min et al, Lemma E.3)} \pt{$TV(p,q) \leq \sqrt{KL(p,q)}$}

If $f:S^T\xrightarrow{}[0,D]$ then, 
$\mathbb{E}_{\mathcal{P}_1} (f(s)) - \mathbb{E}_{\mathcal{P}_2} (f(s))\leq D \sqrt{\frac{log(2)}{2}}. \sqrt{ KL(\mathcal{P}_2 || \mathcal{P}_1)}$  

\pt{Note that this will hold only if $|f(s)| \leq D \sqrt{\frac{log(2)}{2}}$?}
\textcolor{red}{I dont think so. $|f(.)|$ can be D}


\pt{don't use double back slash. These are not needed. just give one line spacing.}

Then, 
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta B^*}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  \mathbb{E}_{\theta, \pi}  [N^-] +  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] - \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] \} \Big \} \\ = \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{  \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] - \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] \} \Big \} \\ 
\geq \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
$
\\
\\
\\
For appropriate $\delta, \Delta$, $KL(\mathcal{P_{\theta}||\mathcal{P_{\theta^j}}}) \leq \frac{16.\Delta^2}{(d-1)^2.\delta}.\mathbb{E_{\theta}}[N^-]$  \\
\\
\textcolor{red}{Need another intermediate similar lemma to simplify the KL-divergence term. \\ Assuming this also holds for our case, \\ }

$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
\geq \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{1/2} \sqrt{\frac{16.\Delta^2}{(d-1)^2.\delta}.\mathbb{E_{\theta}}[N^-]}  \} \Big \} \\
\geq \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{1/2} \frac{4.\Delta}{(d-1).\sqrt{\delta}}.\sqrt{T}  \} \Big \} \\
= \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -   (2KB^*)^{3/2} \sqrt{1/2} \frac{4.\Delta}{(d-1).\sqrt{\delta}} \Big \} \\ 
$\\
Notice that the term in bracket is independent of $\theta, i$ or $j$. Thus, we have: \\
$\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq  \Delta B^* |\Theta| \Big \{  KB^*/4 -   (2KB^*)^{3/2} \sqrt{1/2} \frac{4.\Delta}{(d-1).\sqrt{\delta}} \Big \} \\
\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq   B^*  \Big \{ \Delta  KB^*/4 -   (KB^*)^{3/2} \frac{8.\Delta^2}{(d-1).\sqrt{\delta}} \Big \} \\ 
$ \\
Although $\Delta$ is constrained for well-defining probabilities, the RHS will be lower bounded by the unconstrained minimization of the RHS with respect to $\Delta$. This minimizer is $\Delta^* = \frac{(d-1) \delta}{64 \sqrt{KB^*}}$. At this value of delta,\\
$\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq  \frac{(d-1).\sqrt{\delta}.\sqrt{KB^*}}{512}$ \pt{This makes it independent of number of agents, a very strong result? Is this correct or do we need to incorporate the number of agents here.} \textcolor{red}{potentially the intermediate results I used directly without verifying depend on n. the term i argued to be $+ve$ and ignored in lower bound certainly depends on n but very difficult to simplify(needs closed form V*)}


Since the average over entire set is lower bounded by the RHS, there must exist some parameter in the set for which the RHS is a lower bound. Hence proved \textcolor{blue}{ok we will discuss the proof}. \\
Although it is independent of n, it can be interpreted as a strong result in the sense that no matter how many agents are deployed to learn, this minimum regret will always hold. The independence also comes from ignoring the positive terms \textcolor{red}{(whose proof is as of now still incomplete )}.

\textcolor{blue}{we need to write the  statement that is proved, and also delineate that statement from the proof -- use macros provided in the style file} \textcolor{red}{This is not complete yet. Only if we can find the corresponding lemmas I've mentioned in the proof, it will be complete possibly with very different expression.}

%\textcolor{blue}{ think it is $\newtheorem{lemma}{command for new lemma}$}

\subsubsection{$V^*$ for multiple cases}


General formula:  \textcolor{blue}{is this a theorem?} \textcolor{red}{It follows directly from Bellman equation}\\
 $V^*(s) = \{1  + |\mathcal{S}_{n,r-1}(s)| p_{a^*,r-1} V^*_{r-1} +  |\mathcal{S}_{n,r-2}(s)|p_{a^*,r-2} V^*_{r-2} + \dots + |\mathcal{S}_{n,2}(s)| p_{a^*,2} V^*_{2} + |\mathcal{S}_{n,1}(s)| p_{a^*,1} V^*_{1} \} . \{ 1 - P(s|s,a^*) \}^{-1}$

 \\ \\
 Below $p^*_{r,r'}$ denotes transition probability for a valid transition from state of type $r$ to that of type $r'$ under optimal global action in the respective instance specicified by $\theta$ and $n$ and $V^*_0 = 0$ \\ \\
For n = 1 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$ \\ \\ 
For n = 2 \\
For r = 1 \\ 
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For n = 3 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
\\

For n=4 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\

For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
For r = 4 \\
$V^*_4 = 1 + p^*_{4,4}V^*_4 + \binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1+\binom{4}{4}p^*_{4,0}V^*_0 = \frac{1+\binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1}{1-p^*_{4,4}} = \frac{1+\binom{4}{1}p^*_{4,3}\frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} + \binom{4}{2}p^*_{4,2}\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{4}{3}p^*_{4,1}\frac{1}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+\frac{ \binom{4}{1}p^*_{4,3} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} +\frac{ \binom{4}{2}p^*_{4,2}+\frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}}  = \frac{1+ \frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+ \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}}+\frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  }{1-p^*_{4,4}}$


\pt{can you see the closed form expression here?} \textcolor{red}{i can see a pattern but can't express it nicely.}

\pt{if not, can you confirm whether this notation is correct? -- $p^*_{r,r'}$ is the probability that number agent in the state $s$ were $r$, and the number of agents in $s'$ are $r'$?} \textcolor{red}{yes, line 308-309}

\pt{also can you recall me here -- what does the  $\binom{4}{2}$ or $\binom{3}{1}$ represent in terms of $r,n,$ and $r'$? $\binom{r}{r-r'}$} \textcolor{red}{yes,in the first factor of every term in the numerator}

\pt{I will try to get the closed form expression once you mention this.}


\pt{Also can you summarize what are the intermediate results we have. summarize all of them no matter how  trivial or useful they are are. } \textcolor{red}{In the probability section there's just one important result - general formula for transition probability - the lemma. Putting different values of r and r' give other results. For V*, there's just one important result: for the same "type" of states, V* is the same. This can be expressed as a lemma too. Apart from that monotonicity proof is incomplete, hence lower bound proof is incomplete. This includes all the simplification related to V-V*.}

\pt{I can see  that you have many intermediate results.}












\textcolor{blue}{let's write here the  intermediate steps with pending proofs }
\textcolor{red}{done as of now, thought there's a pattern, to express it mathematically is a bit challenging, i'll try to think about this}

\subsubsection{Important result regrding monotonicity of V*} \\

Consider the states space, $\mathcal{S} = \{s_1,s_2,\dots,s_n\} \cup \{x,y\} $. Let under some global action, the following markov chain be induced:
\\ Cost for any transition is constant and equal to 1. Transition probability from x to $s_i$ is represented as $p_{x,i}$ and from y to $s_i$ as $p_{y,i}$ for $i \in \{1,2,\dots,n\}$ and $p_{x,x}$ and $p_{y,x}$ represent the same from x and y respectively to x. Probability from y to y is represented as $p_{y,y}$. All probabilities are considered between 0 and 1 (strictly). Further, it holds that $p_{y,s} = p_{x,s} - \delta_s$ for every $s\in \{x,1,2,\dots,n\}$ where all $\delta_s \in (0, p_{x,s})$. (We would later require that assuming $p_{x,(.)}$ is monotonic, $\delta_s$'s are such that they preserve the monotonicity of $p_{y,(.)}$. But this assumption on $\delta_s$'s is not required in this discussion.) No other transitions are possible. For the sake of discussion, we assume that the states $s_1,s_2,\dots,s_{n}$ are absorbing states (potentially there may be all kinds of transitions from there but the long term value is known hence they can be considered terminal states with these values) with value function known respectively as $V_1,V_2,\dots,V_n$ while value of state $x$ is also known as $V_x$. Assume the following condition holds for the values: $V_1<V_2<\dots<V_n < V_x$. We want to relate $V_x$ and $V_y$. \\ \\
\tb{Claim:} $V_x < V_y$ \\ \\
$p_{y,y} = 1-p_{y,x}-\sum_{i=1}^{n}p_{y,i} = 1-(p_{x,x} - \delta_x) - \sum_{i=1}^n(p_{x,i}-\delta_i) = \delta_x + \sum_{i=1}^n \delta_i$ \\ \\
$V_x = \sum_{i=1}^np_{x,i}(1+V_i)+p_{x,x}(1+V_x)$ \\ \\
Similarly, \\
$V_y = \sum_{i=1}^np_{y,i}(1+V_i) + p_{y,x}(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^n(p_{x,i}-\delta_i)(1+V_i) + (p_{x,x}-\delta_x)(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^np_{x,i}(1+V_i) + p_{x,x}(1+V_x)-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_i)\} + p_{y,y}(1+V_y) $ \\ \\
From the definition of $V_x$ above and monotonicity of V's, we have : \\
$V_y > V_x-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_x)\} + p_{y,y}V_y = V_x-p_{y,y}(1+V_x) + p_{y,y}(1+V_y) \\ \implies V_y - V_x > p_{y,y}(V_y -V_x) \\ \implies (1-p_{y,y}) (V_y - V_x) > 0 \\ \implies V_y>V_x $

 \\ 

 \subsubsection{Applying above to our case}
We want to prove that under reasonable conditions, $V^*_r^$ are strictly increasing in $r$. We will do this by induction. \\
\tb{Base Case} \\
To show: $V^*_0 < V^*_1$ \\
Recall we already proved $V$ is same for all states as long as they are of same "type" i.e., have same r. \\
Now take any state in $\mathcal{S}_{n,1}$. Let $1>p^*_{1,0}>0$ be the probability of going to global goal state under global action 
 
 \subsubsection{Monotonicity in P ensures $V^*$ ordered} \\
 Consider any initial state s. Let it be of type 'r' i.e., $s \in S_{n,r}$. Now, we will ensure that under any global action at s, the probabilities are such that they monotonically decrease with (over entire) "type set" (defined as the set of states reachable from s of the same type). This will ensure that if shown for the base case (easy to show for r=0 as and r=1 $V^*_0 = 0$ and $V^*_1 > 0$), $V^*$ are monotonically ordered due to the above result. Also, $a^*$  is the one with all signs matching with $\theta$ can be shown for r=1 (base case) easily as long as it maximizes probability to goal. For the induction argument assume this $a^*$ is best for all "type sets" till r-1. Showing $a^*$ at s is the same as the one with signs matching will prove that $a^*$ is the this same action for all states. \\ Using Bellman Equation : \\
 $Q(s,a) = \sum_{i=0}^{r-1}P(i|s,a)(1+V^*_i) + P(s|s,a)(1+V^*_s)$ \\
If we ensure that for any action, the transition probabilities satisfy reduction property as in the above case, $V^*$'s will be monotonic for all those actions. This ensures that the action that uniformly dominates in maximization of the probability to reach the lower "type sets" is the best action $a^*$. We try to construct such an instance, so that the $a^*$ remains the same as the one with all signs matched with $\theta$. \\
To summarize we need the following properties from our instance: 
\begin{itemize}
    \item For any $r \in \{0,1,\dots,n-1\}$ for any global action a, the probability to reach any type set r, r-1, r-2,..,1,0, from r must be strictly higher than from r+1. This leads to V's are ordered as long as $V_1>V_0 = 0$ which holds in general. 
    \item For any state, there must exist an action that uniformly maximises the probability to reach the lower state type sets. This will ensure that it is optimum due to monotonicity of $V^*$. We want this action to be the one matching the signs with $\theta$  \textcolor{red}{this is not possible. individual maximizers are different. hence, i'll remove this}
\end{itemize} 


\subsubsection{Proving $a^*$ is the one that matches sign with $\theta$, $V^*$ only depends on r, there exists ordering of $V^*$'s : all go hand-in-hand \textcolor{blue}{26/Feb/25 needs to be checked?}} 
\tb{Base Case}  \\ By definition, $V^*_0 = 0$. \\
Take any $s \in \mathcal{S}_{n,1}$. \\
\tb{Q.} What is $a^*$? \\
For s, only possible next global states are s itself and all-at-goal (g). This is akin to the single agent problem. But any transition probability also depends on actions of others. \\
Suppose $p^a_{s,g}$ denotes the transition probability from s to g. Then we have, \\
$V_1(s) = (1-p^a_{s,g}).(1+V_1(s)) + p^a_{s,g}.(1+V_0) \implies V_1(s) = \frac{1}{p^a_{1,0}}$ \\
Thus the optimum action at s is the one that minimizes $V_1(s)$ i.e., maximizes $p^a_{s,g}$. From the above general equation (line 177), the transition probability is maximum when $a$ is such that it matches all signs with $\theta$ for the respective components of agent who was initially at s. The signs of other components do not matter. Hence there could be multiple $a^*$ for any particular $s \in \mathcal{S}_{n,1}$. \\
Notice that this will hold true for any $s \in \mathcal{S}_{n,1}$. Note that particular $a^*$ whose sign matches with components of $\theta$ (for every agent), is common for possible $a^*$ for every $s \in \mathcal{S}_{n,1}$. We consider this $a^*$ in particular. \\
Since from the general formula, for a fixed instance ($\theta$), for a given action the probability only depends on r and r', it is the same for all states s $\in \mathcal{S}_{n,1}$ i.e., $p^{a^*}_{s,g} = p^{a^*} \forall s \in \mathcal{S}_{n,1}$. This $V^*_1(s) = V^*_1 \forall s \in \mathcal{S}_{n,1}$ \\
Since transition probability for this action is strictly between 0 and 1, $V^*_1 > V^*_0=0$ \\
\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:\\ $a^*$ is the one that matches sign with $\theta$ for any state in $\mathcal{S}_{n,k}$, hence $p^*(s \in \mathcal{S}_{n,k}  \xrightarrow{}s' \in \mathcal{S}_{n,k'}(s)) = p^*_{k,k'}$, $V^*_k(s)=V^*_k$ for any $s \in \mathcal{S}_{n,k}$ and $V^*_k>V^*_{k-1}$. Now, we need to show the same for $r+1$. \\
Consider any $s \in S_{n,r+1}$. \\
$V^a(s) = \sum_{s' \in \mathcal{S}(s)\textbackslash \{s,g\}} P(s'|s,a)\{1+V^*(s')\} + P(s|s,a).\{1+V^a(s)\} + P(g|s,a).\{1+V^*(g)\}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +\sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} p^a_{r+1,r'}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \sum_{i \in [n]} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r'}  - \binom{r}{r'-1} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Big  \}$ \\ 
Observe that the third term is always non negative since when $r'>r/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} >V^*_r$ while for $r' \leq r/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_r$. Note that the above arguments is for $r' \in [r]$. To minimize $V^a(s)$, we need to minimize $P(s|s,a)$ as well (check after rearrangement as it will appear in denominator as 1-P). Clearly, the action that matches sign with all components of $\theta$ minimizes $V^a(s)$. Hence this is $a^*$. Notice the above arguement holds for any $ s \in \mathcal{S}_{n,r+1}$. Hence $a^*$ is the same for each of them. Hence $p^*(s \in \mathcal{S}_{n,r+1} \xrightarrow{}s' \in \mathcal{S}_{n,r'}(s)) = p^*_{r+1,r'}$. Hence $V^*(s) = V^*_{r+1}$ for each of them. \\
Proving $V^*_{r+1} > V^*_r$ is tricky. The assumption of $P(.|s,a^*)$ in above theorem will make this work. 
\\ \\
\tb{Claim:} Suppose probabilities are such that for any $s \in \mathcal{S}_{n,r+1}$ and $s' \in \mathcal{S}_{n,r}(s)$ for any $r' \in \{0,1,2,\dots, r\}$, $\binom{r+1}{r'}.p^*_{r+1,r'}<\binom{r}{r'}.p^*_{r,r'}$. Then, assuming $V^*_{r}>V^*_{r-1}>\dots>V^*_2>V^*_1>V^*_0=0$, it can be shown that $V^*_{r+1}>V^*_{r}$ for any $r \in \{0,1,\dots, n-1\}$ \\
\textcolor{red}{to make this condition to hold I may have to slightly modify the features or show that this condition exists for current features. if i modify features, i need to be careful since $a^*$ may change possibly differing for every state.} \\

$V^*_r = 1 +\sum_{r'\in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'}V^*_{r'}$ \\
$V^*_{r+1} = 1+ \sum_{r' \in \{0,1,\dots,r+1\}} \binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} $ \\ 

\\
Suppose for every $r' \in \{0,1,2,\dots,r\}$, let $\binom{r+1}{r'}.p^*_{r+1,r'} = \binom{r}{r'}.p^*_{r,r'} - \delta_{r'}$ where $\delta_{r'} > 0$ for every $r'$. Note, $\sum_{r' \in \{0,1,2,\dots,r+1\}}\binom{r+1}{r'}p^*_{r+1,r'} \\= 1 \implies \binom{r+1}{r+1}p^*_{r+1,r+1} = 1-\sum_{r' \in \{0,1,2,\dots,r\}}\binom{r+1}{r'}p^*_{r+1,r'} \\= 1 - \sum_{r' \in \{0,1,\dots,r\}}(\binom{r}{r'}p^*_{r,r'} - \delta_{r'}) = 1-\sum_{r' \in \{0,1,2,\dots,r\}}p^*_{r,r'} + \sum_{r' \in  \{0,1,2,\dots,r\}} \delta_{r'} \\= \sum_{r' \in  \{0,1,2,\dots,r\}} \delta_{r'}$ \\
Now, back to $V^*_{r+1}$. \\
$V^*_{r+1} = 1 + \binom{r+1}{r+1}p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} \\= 1+\binom{r+1}{r+1}p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}} (\binom{r}{r'}p^*_{r,r'} - \delta_{r'})V^*_{r'} \\= 1+\binom{r+1}{r+1}p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - \sum_{r' \in \{0,1,\dots,r\}} \delta_{r'}V^*_{r'} \\>  1+\binom{r+1}{r+1}p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - \sum_{r' \in \{0,1,\dots,r\}} \delta_{r'}V^*_{r} $ (due to monoticity of $V^*$). \\
Thus, \\
$V^*_{r+1}  >  p^*_{r+1,r+1}V^*_{r+1} + 1+ \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - p^*_{r+1,r+1} V^*_{r} \\= p^*_{r+1,r+1}(V^*_{r+1}-V^*_r) + V^*_{r} \implies (1-p^*_{r+1,r+1}).(V^*_{r+1}-V^*_r) > 0 $ \\ Since $1>p^*_{r+1,r+1} >0$, we have $V^*_{r+1} > V^*_r$. \\
Hence by induction, $ a^* $ is same as the one that matches sign with each component of $\theta$, for every state $s \in \mathcal{S}$, $p^*(s \in \mathcal{S}_{n,r} \xrightarrow{}s' \in \mathcal{S}_{n,r'})$ only depends on $r$ and $r'$, $V^* $ is the same for all states of the same type. Hence $V^*(s)$ for any $s \in \mathcal{S}_{n,r}$ only depends on $r$. Further, under the monotonicity of $p^*$, $V^*$ are ordered monotonically increasing in r.
\\ \\
Proving $V^*_{r+1} > V^*_r$ is tricky. We will make a suitable assumption on probabilities and later show that it holds under suitable choices of $\delta$ and $\Delta$. \\
\tb{Claim} If for every $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.  \\
We will justify that the assumption on probabilities in this claim holds for our features under suitable $\delta$ and $\Delta$. For now lets assume this holds for our case and prove the implication part of claim. \\
Return to the induction argument. \\
$V^*_r = 1+\sum_{r' \in \{0,1,\dots,r\}}\binom{r}{r'}V^*_{r'}$ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'}$ \\
Suppose for every $r' \in \{0,1,2,\dots,\lfloor\frac{r+1}{2}\rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}-\delta_{r'} $ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor\ +1 , \lfloor\frac{r+1}{2}\rfloor+2,\dots,r-1,r\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}+\delta_{r'} $ where $\delta_{r'}>0$ for every $r' \in \{0,1,\dots,r\}$\\ 
Note that, $\sum_{r' \in \{ 0,1,\dots,r,r+1\}} \binom{r+1}{r'}p^*_{r+1,r'} = 1 \\ \implies \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r+1}{r'}p^*_{r+1,r'} + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r+1}{r'}p^*_{r+1,r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} (\binom{r}{r'}p^*_{r,r'}-\delta_{r'}) + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} (\binom{r}{r'}p^*_{r,r'} + \delta_{r'}) + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies  \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r}{r'}p^*_{r,r'}-\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + 1 -  \sum_{r' \in \{0,1,\dots,r-1,r} \binom{r}{r'}p^*_{r,r'} \\ \implies p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} $ \\ \\
Now, going back to $V^*_{r+1}:$ \\ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}(\binom{r}{r'}p^*_{r,r'} - \delta_{r'})V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}(\binom{r}{r'}p^*_{r,r'}+\delta_{r'})V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} V^*_{r'}+ \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, r-1,r\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\=  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ > p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{\lfloor \frac{r+1}{2} \rfloor + 1}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  (  \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} - \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}  )V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ >  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r $ \\ 
Thus,\\
$V^*_{r+1} >   p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r \implies (1-p^*_{r+1,r+1})(V^*_{r+1}-V^*_r)>0 \implies V^*_{r+1} > V^*_r$ \\
Above inequalities used monotonicity of $V^*$ due to induction assumption. \\
Below we justify that the assumption in the above claim holds for our case.
\subsubsection{Justification of assumption} \\
Recall that in the above claim, we assumed that: for every $r \in [n-1],$ for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$. \\
Below, we will derive sufficient conditions on $\delta$ and $\Delta$ such that this assumption holds. \\
Also note that from below section we have $\delta<0.5$ and $\delta>3.2^{n-1}\Delta$ so that all probabilities are well defined.
\\ \\
\tb{For $r'\leq \lfloor\frac{r+1}{2}\rfloor$}, \\
$\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \frac{r+1}{r+1-r'}p^*_{r+1,r'}<p^*_{r,r'} \Leftrightarrow \\(r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \\ \Leftrightarrow  (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \\ \impliedby (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \Leftrightarrow \frac{\Delta}{n}\frac{r^2}{8} + (r+1) \frac{\Delta}{n}<(r+1)\frac{1-2\delta}{n2^{r+1}} \Leftrightarrow \frac{\Delta}{n}(\frac{r^2}{8}+r+1)<(r+1)\frac{1-2\delta}{n2^{r+1}} \impliedby \Delta (\frac{n^2}{8}+n+1)<\frac{1-2\delta}{2^{n}} \Leftrightarrow \Delta < \frac{1-2\delta}{2^{n}(1+n+\frac{n^2}{8})}$ \\ \\
Similarly, \\ \tb{For $r' > \lfloor \frac{r+1}{2} \rfloor$}, \\ 
$\binom{r+1}{r'}p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \\ \frac{r+1}{r+1-r'}p^*_{r+1,r'}>p^*_{r,r'} \Leftrightarrow \\ (r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow \\ (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \Leftrightarrow \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow  \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0  \impliedby  (\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0 \\ \Leftrightarrow \frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2) - 0.5(r+1)(\frac{1-2\delta}{n.2^{r}}) >0 \\ \Leftrightarrow \frac{(r'-r-0.5)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2)  >0 \impliedby \frac{(-r-0.5)(1-2\delta)+0.5n }{n.2^{r}}   >   \frac{\Delta}{n}  (r^2-r-1)  \Leftrightarrow \frac{(-r-0.5)(1-2\delta)+0.5n }{1}   >   \frac{\Delta}{1}  (r^2-r-1)  (2^{r}) \\ \impliedby (-n-0.5)(1-2\delta)+0.5n    >   \Delta  (n^2-n-1)  (2^{n})$ and $ (-n-0.5)(1-2\delta)+0.5n    > 0 \\ \impliedby 0.5n-n+2n\delta-0.5+\delta>0$ and $ 0.5n-n+2n\delta-0.5+\delta >   \Delta  (n^2-n-1)  (2^{n}) \\ \impliedby (2\delta-0.5)n>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2-n-1)  (2^{n}) \\ \impliedby 2\delta-0.5>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2-n-1)  (2^{n}) \\ \Longleftrightarrow \delta>\frac{1}{3}$ and $n > \frac{0.5-\delta}{2\delta-0.5}+ \frac{\Delta  (n^2-n-1)  (2^{n})}{2\delta-0.5} \\ \impliedby \delta>1/3 $ and $\Delta  (n^2-n-1)  (2^{n})<3\delta-1 \impliedby \Delta < \frac{3\delta-1}{(n^2-n-1).2^{n}}$ \\ The last second condition is trivially satisfied for n=1. Otherwise use the condition on $\Delta$.
\\
Finally we obtain for the desired instance, fix $1/2>\delta>1/3$. Then, fix, $\Delta< 2^{-n}.min\{\frac{3\delta-1}{n^2-n-1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2/8}\}$




\subsubsection{Sufficient conditions on $\delta$ and $\Delta$ for well defined probabilities}

$p^a_{r,r'} < 1$ for every $r \in \{1,2,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$. \\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  <   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{1} <   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{\frac{n-r}{2}}{n2^{r-1}}        +    3\Delta  =  \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} +    3\Delta =  \frac{(r'-0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} +    3\Delta < \frac{0.5n(2-2\delta)}{n.2^{r-1}} + 3\Delta  < 1-\delta + 3\Delta$ \\
To ensure $p^a_{r,r'}<1$ it is sufficient to ensure $1-\delta + 3\Delta<1 \implies \delta > 3\Delta$ \\
Similarly, we must ensure, $p^a_{r,r'} > 0$ for every $r \in \{0,1,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$. \\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  > \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') -  \frac{2 \Delta}{1} > \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} - 3\Delta > \frac{(r' -0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta > \frac{( -0.5n)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta = \frac{ \delta }{2^{r-1}} - 3\Delta$ \\
To ensure, $p^a_{r,r'} > 0$ it is sufficient to ensure $ \frac{ \delta }{2^{r-1}} - 3\Delta > 0  \implies \delta > 3.2^{n-1}.\Delta$. \\ Observe that since $n \geq1$, condition from $p>0 \implies $ condition from $p<1$  Also note that in the above, we have assumed $\delta < 0.5$. Hence we can fix any $\delta, \Delta $ and $n$ that satisy the above conditions in order to fix a class of instance as above.

\section{Try product based features \textcolor{blue}{3/3/2025}} 
Assume the following (top-down) probability model: \\
At any state $s \in \mathcal{S}$, it holds that, for any agent $i \in [n]$, \\
$P(s_i^\prime=g|s_i=s,a) = \langle a, \theta \rangle + \delta$, \\
$P(s_i^\prime=s|s_i=s,a) = \langle -a, \theta \rangle + 1- \delta$ \\
$P(s_i^\prime=g|s_i=g,a) = 1$, \\
$P(s_i^\prime=s|s_i=g,a) = 0$ \\
\\
Note that for a fixed instance, for a fixed global action, transition probabilities are same for all agents at $s_{init}$. For those at $goal$ too they are trivially same (hard constraint).
\\
For these to be well defined for all instances in our analysis, we want that \\ $1 > max_{a,\theta}  \langle a, \theta \rangle + \delta = \delta+\Delta> min_{a,\theta} \langle a, \theta \rangle + \delta = \delta - \Delta >0 \implies 1> \delta+\Delta, \delta>\Delta $ \\
Similarly, we want \\
$1>  max_{a,\theta}\langle -a, \theta \rangle + 1- \delta = 1+\Delta-\delta>min_{a,\theta}  \langle -a, \theta \rangle + 1- \delta=1-\delta-\Delta >0 \implies \delta>\Delta, 1>\delta+\Delta$ (same conditions as above. note $\delta, \Delta >0$) \\These ensure that probability for general transition are well-defined. 

\\
\tb{Expression for a general transition}\\
Consider state $s \in \mathcal{S}_{n,r}$ for some $r \in \{1,2,\dots,n\}$. For any $r' \in \{0,1,\dots,r\}$, take any $s' \in \mathcal{S}_{n,r'}(s)$. Let s be such that agents in $\mathcal{I}:=\{i_1,i_2,\dots,i_r\}$ are at $s_{init}$ and those at indices in $\mathcal{J}:=\{j_1,j_2,\dots,j_{n-r}\}$ are at $goal$. Let the agents in $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ be the ones transiting to $goal$ during transition of global state from $s$ to $s'$. Then, \\ $P(s'|s,a) = \{\Pi_{t \in \mathcal{T}} p(s_t^\prime =g|s_t=s_{init},a)\} . \{\Pi_{i \in \mathcal{I}-\mathcal{T}}p(s'_i=s|s_i=s_{init},a)\}.\{\Pi_{j \in \mathcal{J}}p(s'_j=g|s_j=g,a)\} = \{ \langle a, \theta \rangle + \delta\}^{r-r'} . \{\langle -a, \theta \rangle + 1- \delta\}^{r'}.\{1\}^{n-r} $ \\
Notice  that the above expression remains the same for any $s' \in \mathcal{S}_{n,r'}(s)$. The above argument holds for any $s \in \mathcal{S}_{n,r}$ for any fixed a. \\ We will denote this as $p^a_{r,r'}$ (later we will show that the optimal action at all states is the same hence represent $p^*_{r,r'}$ for optimal action/policy). \\
\tb{The general proof} \\
Base case : r=0\\
Consider any $s \in \mathcal{S}_{n,1}$. Let the $i-th$ agent be at $s_{init}$ and all others at $goal$. Suppose global action a is taken. Then,
$V^a_1(s) = p^a_{1,0}(1+V_0) + p^a_{1,1}(1+V^a_1) = 1 + (1-p^a_{1,0})V^a_1 \implies V^a_1(s) = \frac{1}{p^a_{1,0}}$ \\
Clearly the best action at $s$ is the one that minimizes $V^a_1(s)$ i.e., maximizes $p^a_{1,0}$. From the above general expression this is the one that matches sign with all components of $\theta$. Since the above argument is true for any $s \in  \mathcal{S}_{n,1}$, $a^*$ is the same as the one that matches all signs with $\theta$ for all $s \in \mathcal{S}_{n,1}$ and we can see that since probability depends on only r and r' for given global action for a given instance, $V^*(s) = constant = V^*_1$ for all $s \in \mathcal{S}_{n,1}$. Also by definition, $V^a_0 = 0$. Thus, $V^*_0 = 0 < V^*_1$. \\ \\
Now assume that, for every $k \in [r]$, it holds that, 
\item $a^*(s) = a^*=$ same as the one matching all signs with $\theta$, for every $s \in \mathcal{S}_{n,k}$ 
\item $V^*(s) = V^*_k$ for every $s \in \mathcal{S}_{n,k}$ 
\item $V^*_k > V^*_{k-1}$ \\ \\
We need to show that the above is true for $'r+1'$ as well. Now consider any $s \in \mathcal{S}_{n,r+1}$ and $s_r \in \mathcal{S}_{n,r}(s)$\\
$V^*(s_r) = V^*_r = 1+ \sum_{r'\in \{0,1,\dots,r\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'}$ here, we know what the optimal action is \\
$V^*(s) = 1+ \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^*_{s,r'}V^*_{r'} + p^*_{s,s}V^*(s) = 1+p^*_{s,s}V^*(s) + \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^*_{s,r'}V^*_{r'} $ here we do not know what the optimal action is but whatever it is we can write the expression.\\

We will use the following result (this gives us condition on parameters): \\
We want that for every action $a$ in $s$, $\binom{r+1}{r'}p^a_{s,r'}<\binom{r}{r'}p^*_{r,r'}$ for every $r' \in \{0, [r]\}$ for every $r \in [n-1]$. \\
Thus,  $\frac{r+1}{r+1-r'}p^a_{s,r'}<p^*_{r,r'}  \impliedby \frac{r+1}{r+1-r'} (p^a)^{r+1-r'}(1-p^a)^{r'} < (p^*)^{r-r'}(1-p^*)^{r'} \impliedby \frac{r+1}{r+1-r'} (p^*)^{r+1-r'}(1-p^*)^{r'} < (p^*)^{r-r'}(1-p^*)^{r'} \impliedby \frac{r+1}{r+1-r'} p^* < 1 \impliedby p^* < \frac{1}{n}$ \\
In the above we used a claim that for any $r \in [n-1]$, for every $r' \in \{0, [r]\}$, for any global action $a$, $(p^a)^{r+1-r'}.(1-p^a)^{r'} < (p^*)^{r+1-r'}.(1-p^*)^{r'}$ where $p^*$ denotes success probability at $a^*:$one with all signs matched with $\theta$. For this to hold, it is sufficient to show that $f_{r,r'}(p):=p^a_{s,r'}=(p)^{r+1-r'}(1-p)^{r'}$ is increasing function with $p$ for every $r' \in \{0, [r]\}$ for all $r \in [n-1]$ \\
$f_{r,r'}'(p) = (r+1-r')(p)^{r-r'}(1-p)^{r'}-(p)^{r+1-r'}r'(1-p)^{r'-1} > 0 \impliedby (r+1-r')(1-p)>p.r' \impliedby (1-p)>p.r \impliedby \frac{1}{p} - 1 > n-1 \impliedby p < \frac{1}{n} \impliedby \delta + \Delta < \frac{1}{n}$
\\
We enforce that $\delta + \Delta < \frac{1}{n}$ so that the above result hold to use it as below. \\
Suppose for every $r' \in \{0,1,2,\dots,r\}$, let $\binom{r+1}{r'}.p^*_{s,r'} = \binom{r}{r'}.p^*_{r,r'} - \delta_{r'}$ where $\delta_{r'} > 0$ for every $r'$  \\

\\
Note, $\sum_{r' \in \{0,1,2,\dots,r+1\}}\binom{r+1}{r'}p^*_{s,r'} = 1 \\ \implies p^*_{s,s} = 1-\sum_{r' \in \{0,1,2,\dots,r\}}\binom{r+1}{r'}p^*_{s,r'} \\= 1 - \sum_{r' \in \{0,1,\dots,r\}}(\binom{r}{r'}p^*_{r,r'} - \delta_{r'}) = 1-\sum_{r' \in \{0,1,2,\dots,r\}} \binom{r}{r'} p^*_{r,r'} + \sum_{r' \in  \{0,1,2,\dots,r\}} \delta_{r'} \\= \sum_{r' \in  \{0,1,2,\dots,r\}} \delta_{r'}$ \\
Now, back to $V^*(s)$. \\
$V^*(s) = 1+ p^*_{s,s}V^*_{s} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^*_{s,r'}V^*_{r'} \\= 1+p^*_{s,s}V^*_{s} + \sum_{r' \in \{0,1,\dots,r\}} (\binom{r}{r'}p^*_{r,r'} - \delta_{r'})V^*_{r'} \\= 1+p^*_{s,s}V^*_{s} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - \sum_{r' \in \{0,1,\dots,r\}} \delta_{r'}V^*_{r'} \\> 1+ p^*_{s,s}V^*_{s} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - \sum_{r' \in \{0,1,\dots,r\}} \delta_{r'}V^*_{r} $ (due to monoticity of $V^*$). \\
Thus, \\
$V^*(s)  >  1+p^*_{s,s}V^*(s) + \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - p^*_{s,s} V^*_{r} \\= p^*_{s,s}(V^*(s)-V^*_r) + V^*_{r} \implies (1-p^*_{s,s}).(V^*(s)-V^*_r) > 0 $ \\ Since we will ensure $1>p^a_{s,s} >0$, we have $V^*(s) > V^*_r$. \\
Thus, clearly $V^a (s) \geq V^*(s) > V^*_r> V^*_{r-1}>\dots>V^*_1>V^*_0 = 0$
\\
\\
$V^a(s) = \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^a_{s,r'}V^*_{r'} + p^a_{s,s}V^a(s)  $ \\
Notice that if there exists an action that uniformly maximizes the probability $p^a_{s,r'}$ for all $r' \in \{0,[r]\}$, then it is optimal. This is due to monotonicity of $V's$ and positive coefficients and allotment of probabilities. We claim that this is the same as $a^*:$ the one that matches sign with all components of $\theta$. The justification is that in an above claim, we showed that, for every $r' \in  [r]$, $p^a_{s,r'}$ is an increasing function of success probability for our instances $\delta + \Delta < 1/n$. And, the success probability is maximized when action is $a^*:$ one that matches signs with components of $\theta$.  \\
Notice that the same argument can be given for any $s \in \mathcal{S}_{n,r+1}$ Thus, $a^*$ is same for all these states. Hence, $p^*_{s,r'} = p^*_{r+1,r'}$ for all $s \in \mathcal{S}_{n,r+1}$ as for the same action and $\theta$ it only depends on r+1 and $r'$. Thus $V^*(s) =V^*_{r+1}$ for all $s \in \mathcal{S}_{n,r+1}$ \\
Hence, we have showed that:
\item $a^*$ is same for all states $s \in \cup_{k=\{0,1,\dots,r+1\}} \mathcal{S}_{n,k}$ 
\item $V^*(s) = V^*_{r+1}$ for all $s \in \mathcal{S}_{n,r+1}$
\item $V^*_{r+1} > V^*_r>V^*_{r-1}>\dots>V^*_1>V^*_0=0$
Thus this holds true by induction that :
\item The optimal policy is that at every state, one takes the same action namely the one that matches sign with all components of $\theta$
\item Optimal value for states of the same type is the same
\item States with more agents at $s_{init}$ have strictly higher values(long term costs) than the one with lower number of agents at $s_{init}$

\subsubsection{Working on Lower Bound}

Suppose in episode \textit{k}, agents take actions according to policy $\pi$. Let, $\tb{s}_t$ represent the global state and $\tb{a}_t$ the global action at time $t$. Then, the expected regret for the \textit{k-th} episode is:
\begin{align}
    R_{\theta,k} &= V^{\pi_\theta}(\tb{s}_1) - V^*(\tb{s}_1) 
    \\
    &=  V^{\pi_\theta}(\tb{s}_1) - \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) 
    \\ 
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^\pi(\tb{s}_2)]\}  
    \\ 
    & \quad -\mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^*(\tb{s}_2)] \} + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim\ \pi(\tb{s}_1), \tb{s}_2 \sim\ \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi}(\tb{s}_2) - V^*(\tb{s}_2)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1)
\end{align}
\begin{align} 
    & \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q^{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ c(\tb{s}_1,\tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)] \} - V^{\pi^*}(\tb{s}_1) \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim   \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - V^{\pi^*}(\tb{s}_1) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - (1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)]) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{  \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)] \}
    \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} \{ \sum_{\tb{s} \in \mathcal{S}} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*)) V^{\pi^*}(\tb{s})\}
\end{align}

$
 \sum_{\tb{s} \in \mathcal{S}} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*))V^*(\tb{s})  = (\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*))V^*_n + \sum_{\tb{s} \in \mathcal{S} \textbackslash\tb{s}_1} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*))V^*(s) 
$\\
Remember we proved earlier that $\mathbb{P}(s|s_1,a_1) = \binom{n}{n-r'}(p^a)^{n-r'}(1-p^a)^{r'}$ is maximised at $a = a^*$ for all $r' \in \{0\} \cup [n-1]$. Hence, the second term above consists of summation of negative terms and can be lower bounded as follows:
\\$\sum_{s \in \mathcal{S}}(\mathbb{P}(s|s_1,a_1) - \mathbb{P}(s|s_1,a_1^*))V^*(s) = (\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*))V^*_n + \sum_{\tb{s} \in \mathcal{S} \textbackslash\tb{s}_1} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*))V^*(s) > (\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*))V^*_n + \sum_{\tb{s} \in \mathcal{S} \textbackslash\tb{s}_1} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*))V^*_{n-1} = (\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*))V^*_n +  (1 - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - (1-\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*)))V^*_{n-1} = (\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*))V^*_n +  ( \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) )V^*_{n-1} =  ( \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}^*_1) ) . (V^*_n - V^*_{n-1}) = ((p^a_{n,n})^n-(p^*_{n,n})^n) . (V^*_n - V^*_{n-1})  = (p^a_{n,n}-p^*_{n,n})((p^a_{n,n})^n + (p^a_{n,n})^{n-1}.p^*_{n,n}+\dots+(p^a_{n,n}).(p^*_{n,n})^{n-1} + (p^*_{n,n})^n ) . (V^*_n - V^*_{n-1}) >  (p^a_{n,n}-p^*_{n,n}) (p^*_{n,n})^n .n . (V^*_n - V^*_{n-1})  $ \\
Note that, $p^a_{n,n} = 1- \delta - \sum_{i = 1}^n \sum_{p=1}^{d-1} a_{i,p}.\theta_{i,p} = 1-\delta-\sum_{i = 1}^n \sum_{p=1}^{d-1} \frac{\Delta}{n(d-1)} (\mathbbm{1}\{sgn(a_{i,p})=sgn(\theta_{i,p}\}-\mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\})  = 1-\delta-\sum_{i = 1}^n \sum_{p=1}^{d-1} \frac{\Delta}{n(d-1)} (1-2.\mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}) = 1-\delta-\Delta + \sum_{i = 1}^n \sum_{p=1}^{d-1} \frac{2.\Delta}{n(d-1)} (\mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\})$ \\
Thus, $p^a_{n,n} - p^*_{n,n} = \sum_{i = 1}^n \sum_{p=1}^{d-1} \frac{2.\Delta}{n(d-1)} (\mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\})$
\\
Therefore, 
\\$\sum_{s \in \mathcal{S}}(\mathbb{P}(s|s_1,a_1) - \mathbb{P}(s|s_1,a_1^*))V^*(s) >  (p^a_{n,n}-p^*_{n,n}) (p^*_{n,n})^n .n . (V^*_n - V^*_{n-1}) \\= (1 - \delta -\Delta)^n .n . (V^*_n - V^*_{n-1}) \sum_{i = 1}^n \sum_{p=1}^{d-1} \frac{2.\Delta}{n(d-1)} (\mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\})   $
\\
\textcolor{red}{We abandon this model since monotonicity of V has been established for earlier model and features}
\subsection{Results to use in Lower bound proof 9-3-25}
$V^*_r = 1 +  p^*_{r,r} . V^*_r +\sum_{r'=1}^{r-1} \binom{r}{r'} p^*_{r,r'}.V^*_{r'} < 1+p^*_{r,r}V^*_r + (1-p^*_{r,r})V^*_{r-1} \Leftrightarrow V^*_r-V^*_{r-1}<\frac{1}{1-p^*_{r,r}}$ \\
Thus, \\
$V^*_n - V^*_{n-1} < \frac{1}{1-p^*_{n,n}} \\ V^*_{n-1}-V^*_{n-2}<\frac{1}{1-p^*_{n-1,n-1}}\\ &\vdots \\ V^*_{2}-V^*_1 < \frac{1}{1-p^*_{2,2}} \\ V^*_1 - V^*_0 = \frac{1}{1-p^*_{1,1}}$ \\
Adding the above, \\
$V^*_n - V^*_0 \leq \sum_{i=1}^n\frac{1}{1-p^*_{i,i}} \leq \frac{n}{1-p^*_{1,1}} = nV^*_1 \implies B^*/n \leq V^*_1$ \\
Observe that equality holds for $n=1$



\newpage
\section{\textcolor{blue}{11-3-24 } Everything Below is to be verified. I have removed some of earlier comments and sections that are no longer useful. Ive also changed the order of different sections for flow}


\section{Introduction}
\label{sec:intro}

\pt{
\begin{itemize}
    \item What are the major to-do things. \textcolor{red}{simplify kl-divergence term (see the last section), fix issues with MACCM if time permits and redo experiments} 
    \item What is the story of the entire paper. \textcolor{red}{for me, it will depend on what results are obtained, so far there's no important complete result, so can't say much}
    \item Let us start writing the paper formally. There are lot of things to do. \textcolor{red}{in my opinion, lets get at least 2 key results first, so far we have none. in fact lets concentrate completely on simplifying the kl divergence term, i'm stuck on this for a week now and it is quite non-trivial, once this is done i can move to computations part }
    \item I need some more clarity on what are the major things pending before I can start writing the paper.
    \item What are the major results? What are other results we are still aiming at, and where are we stuck? \textcolor{red}{so far there's no key complete result}
    \item What is the status of the experiments. \textcolor{red}{Cant use MACCM before resolving the issues, also haven't finished yet with lower bound proof}
    \item We need to finalize the results before we write the paper. 
    \item Let me write the story of the paper.
\end{itemize}
}


\subsection{Story of the paper.}

\pt{
\begin{itemize}
    \item Single agent SSP is a well known problem.
    \item The RL version of the SSP has become very popular recently. 
    \item The upper and lower bounds are proved.
    \item \cite{trivedi2023massp} has recently extended from the single agent to multi-agent SSP.
    \item The regret upper bounds are derived for the MA-SSP version.
    \item However, the lower bounds are majorly missing in the literature.
    \item Also, the role of number of agents in the multi-agent setup is another important missing factor in the literature.
    \item In this paper we explore two important aspects -- the regret lower bounds and the role of number of agents in the MA-SSP setup regret bounds.
    \item To the best of our knowledge, this is the first paper addressing the above missing problems in the literature. 
    \item We prove a matching lower bounds for the MA-SSP paper. \\ \textcolor{red}{for now it looks ok}
\end{itemize}
}

Our major contributions are as follows:

\begin{itemize}
    \item \textbf{Analysis wrt Number of Agent}
    \item \textbf{Experiments}
\end{itemize}

\input{CR_Sections/6_experiments}


\subsection{Proof of Lower Bound}

\pt{Need to write this thing cleanly with proper justifications. Why the following makes sense, and how would this capture the hardest instance. What is the role of congestion in this example?}

We construct and analyze a family of hard to learn instances. This is the same as in section 1.1. Further, we restrict $\theta$ such that $\theta_{i} \neq \theta_{j}$ $ \forall$ $ i \neq j \in [n]$ i.e., no two $\theta_i$ are the same. Let this set be denoted as $\Theta$. \pt{Why this assumption will hold. there is lot of symmetry in the problem, so $\theta$'s for two agents will be same?}. \textcolor{blue}{It's not an assumption. It's a restriction of the class of SSPs instances I'm considering. I'm free to do so. Why I do this is the rest of paragraph about. Also $\theta$ is an instance parameter, it can be anything. A way to think about this is that : even if two agents took same action, the contribution to probability of transition to any global state is not the same, this is one way how agents are not identical!} This ensures that the action to be taken by each agent to maximize the probability of transition to the all-at-goal state is different for every agent so that we don't need to consider the congestion component of the cost when the policy of maximizing the probability to reach all-goal is executed.
To further reduce complexity of the analysis, we let the private cost associated with any action in the initial state be equal to 1 and that in goal state equal to 0. This ensures that the \textit{best} policy is the one that maximizes the probability of transition to the global goal \pt{goal?} \textcolor{blue}{yes, thanks!} state.  \\
Suppose in episode \textit{k}, agents take actions according to policy $\pi$. Let, $\tb{s}_t$ represent the global state and $\tb{a}_t$ the global action at time $t$. Then, the expected regret for the \textit{k-th} episode is:

\pt{In the regret definition below the policy seems to have the parameters $\theta$, whereas we have originally used $\theta$ as the parameters for the transition probabilities?} \textcolor{red}{yes, we are analyzing regret of a class of instances simultaneously defined by \theta. $\pi_{\theta}$ represents the policy learned for instance defined by $\theta$. In the below everywhere $\pi ==\pi_{\theta}$. I need to update it. In fact more accurately it must be $\pi_{\theta,k}$ since the learned policy differs every episode.} 

\begin{align}
    R_{\theta,k} &= V^{\pi_\theta}(\tb{s}_1) - V^*(\tb{s}_1) \label{regret}
    \\
    &=  V^{\pi_\theta}(\tb{s}_1) - \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) 
    \\ 
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^\pi(\tb{s}_2)]\}  
    \\ 
    & \quad -\mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^*(\tb{s}_2)] \} + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim\ \pi(\tb{s}_1), \tb{s}_2 \sim\ \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi}(\tb{s}_2) - V^*(\tb{s}_2)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1)
\end{align}

\pt{Suggestion -- for each equation write the proper reason why it is true. This will make it easy to follow. For example, in above the second equation you added and subtracted $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] $.}
\textcolor{red}{Ok, I'll do it after I start revisiting them. Apart from adding and subtracting Q, I've only expanded the Bellman Equation}

\textcolor{red}{I'm stuck here to find a closed form expression of $Q^*(.,.)$ and $V^*$ due to exponential number of states}

\subsection{Some proofs I have been trying since Monday}
\subsubsection{}
\begin{align} 
    & \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q^{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ c(\tb{s}_1,\tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)] \} - V^{\pi^*}(\tb{s}_1) \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim   \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - V^{\pi^*}(\tb{s}_1) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - (1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)]) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{  \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)] \}
    \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} \{ \sum_{\tb{s} \in \mathcal{S}} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*)) V^{\pi^*}(\tb{s})\} \label{difference of probabilities}
\end{align}

\\
The above just follows from writing the definition of optimum Action value function and doing some rearrangement and remember costs throughout is 1.
\\

In the below proof, we expand the difference in probability term arising in the above equation. The initial global state, $s_1$, is with all agents at $s_{init}$ and the next state, $s$, is one where agents $i_1,i_2,..,i_r$ remain at $s_{init}$ and those at $j_1,j_2,..,j_{n-r}$ go to goal node. \\


\begin{lalign}
\mathbb{P}(s|s_1, a_1) - \mathbb{P}(s|s_1, a_1^*)  
\\
&= \langle \phi(s|s_1,a_1), \theta \rangle - \langle \phi(s_1|s_1,a_1^*), \theta \rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1), \phi(s_2^{\prime}|s_2, a_2)..., \phi(s_n^{\prime}|s_n,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\& - \langle (\phi(s_1^{\prime}|s_1, a_1^*), \phi(s_2^{\prime}|s_2, a_2^*)..., \phi(s_n^{\prime}|s_n,a_n^*)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1),..., \phi(s_n^{\prime}|s_n,a_n)) - (\phi(s_1^{\prime}|s_1, a_1^*),..., \phi(s_n^{\prime}|s_n,a_n^*)), \\
& (\theta_1, 1,...,\theta_n,1)\rangle 
\\
&= \sum_{m = 1}^{r} \langle \phi(s_{i_m}^{\prime}|s_{i_m},a_{i_m}) - \phi(s_{i_m}^{\prime}|s_{i_m},a^*_{i_m}), (\theta_{i_m}, 1)\rangle \\ 
& + \sum_{m = 1}^{n-r} \langle \phi(s_{j_m}^{\prime}|s_{j_m},a_{j_m}) - \phi(s_{j_m}^{\prime}|s_{j_m},a^*_{j_m}), (\theta_{j_m}, 1)\rangle 
\\
&= \sum_{m=1}^{r} \langle (-a_{i_m} + a^*_{i_m}, 0), (\theta_{i_m}, 1) \rangle + \sum_{m=1}^{n-r} \langle (a_{j_m}-a^*_{j_m}, 0), (\theta_{j_m}, 1) \rangle   
\\
&= \sum_{m=1}^{r} (\langle a^*_{i_m}-a_{i_m}, \theta_{i_m} \rangle)  + \sum_{m=1}^{n-r} (\langle a_{j_m}-a^*_{j_m}, \theta_{j_m}  \rangle)  
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1} (a^*_{i_m, p} - a_{i_m, p})\theta_{i_m, p} \} + \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1} (a_{j_m, p} - a^*_{j_m, p})\theta_{j_m, p} \}
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\} \}  - \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \}
\\
&= \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\}
\end{lalign}
\\
\\
The initial few lines use the linearity assumption and properties of inner product. Then, split the sum on $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Next lines use definition of $\phi(.,.)$ and $a^*$ as the one matching all signs with $\theta$. 
\\

\\



\subsubsection{}

\text{Probability that after taking a global action $\tb{a}$, the next global state is still the same as before i.e., $\tb{s}$}
\begin{lalign}
\mathbb{P}(\tb{s}|\tb{s}, \tb{a})
\\ Linearity Assumption\\
&= \langle \phi(\tb{s}|\tb{s},\tb{a}), \boldsymbol{\theta} \rangle
\\
$Expanded form of features$
\\
&= \langle (\phi(s|s, a_1), \phi(s|s, a_2)..., \phi(s|s,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\
$Definition of Inner Product$
\\
&= \sum_{i = 1}^{n} \langle (\phi(s|s, a_i),(\theta_i,1))
\\
$Definition of Features$
\\
&= \sum_{i = 1}^{n} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}),(\theta_i,1) \rangle
\\
&= \sum_{i = 1}^{n} \{ \langle -a_i, \theta_i \rangle + \frac{1-\delta}{n.2^{n-1}} \}
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \langle a_i, \theta_i \rangle 
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} a_{i,p}. \theta_{i,p} 
\\ $Definition of action and theta$\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Taking summation over p inside$ \\
&=  \frac{1-\delta}{2^{n-1}} - 
 \frac{\Delta}{n(d-1)} \sum_{i = 1}^{n}   \Big\{ d-1 - 2 \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Just simplify$ 
\\
&=  \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
\end{lalign}

\subsubsection{}
\\
In this subsection we derive the expression of Probability that if at state $\tb{s} = \{s_{init}, s_{init}, \dots, s_{init}\}$, if global action $\tb{a} = (a_1,a_2,\dots, a_n)$ is taken, you reach $\tb{s}^{\prime}$ where the agents at indices in $\mathcal{I}:= \{ i_1,i_2,\dots, i_r\}$ stay in the same state while agents at indices in $\mathcal{J} := \{j_1,j_2,\dots,j_{n-r} \}$ move to goal state i.e., $s'_{i_1}=s'_{i_2}=\dots=s'_{i_r}=s_{init}$ and $s'_{j_1}=s'_{j_2}=\dots=s'_{j_{n-r}}=goal$. \\
$P(\tb{s}'|\tb{s},\tb{a}) \\ 
= \langle \phi(\tb{s}'|\tb{s},\tb{a}), \theta \rangle \\
= \langle \phi((s'_1,s'_2,\dots, s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n)), (\theta_1, 1, \theta_2, 1,\dots, \theta_n,1) \rangle \\
= \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)),(\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle \phi(s'_i|s_i,a_i), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(s'_j|s_j,a_j), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle (a_j, \frac{\delta}{n.2^{n-1}}), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \Big \{  \frac{1-\delta}{n.2^{n-1}} + \langle -a_i,\theta_i \rangle \Big \} + \sum_{j \in \mathcal{J}} \Big \{ \frac{\delta}{n.2^{n-1}} + \langle a_j, \theta_j \rangle \Big \} \\
= r. \frac{1-\delta}{n.2^{n-1}} - \sum_{i \in \mathcal{I}}    \langle a_i,\theta_i \rangle  + (n-r). \frac{\delta}{n.2^{n-1}} +  \sum_{j \in \mathcal{J}}  \langle a_j, \theta_j \rangle  \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}} -  \sum_{i \in \mathcal{I}} \{ \sum_{p = 1}^{d-1} a_{i,p}.\theta_{i,p} \} + \sum_{j \in \mathcal{J}} \{ \sum_{p = 1}^{d-1} a_{j,p}.\theta_{j,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \{
\sum_{j \in \mathcal{J}}   a_{j,p}.\theta_{j,p}  -  \sum_{i \in \mathcal{I}}  a_{i,p}.\theta_{i,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \Big \{
\sum_{j \in \mathcal{J}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{j,p}) = sgn(\theta_{j,p})\} - \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{
\sum_{j \in \mathcal{J}}  \Big[ 1 - 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}}  \Big[   1 - 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{  \Big[ n-r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] - \Big[  r - \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
\sum_{p = 1}^{d-1}  \Big \{  n-2r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
  \Big \{  (d-1)(n-2r) - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\frac{\Delta . (n-2r)}{n} +\frac{2 \Delta}{n(d-1)} . 
  \Big \{  \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}     \Big \} \\
$ 
\\
Lines 186-190 follow by linearity assumption, definition of features and splitting the dot product over $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Lines 191-195 simplify the dot product and rearrange terms. Line 196 uses definition of action and theta. The remaining lines simplify the summations and rearrange the terms.
\\
From the above expression, we conclude that this probability remains same (say, $p_{a,r}$ for subsequent discussions,  for all states $s \in \mathcal{S}_{n,r}$ for every $r \in [n]$ for $a = \{a_1,a_2,\dots,a_n\}$ given global action taken at $s = \{s_{init}, s_{init},\dots, s_{init}\}$.  \\


A more general result of the above relates to transition probability from some $s \in \mathcal{S}_{n,r}$ to some $s' \in \mathcal{S}_{n,r'}(s)$ where $\mathcal{S}_{n,r'}(s)$ represents the possible states of type $r'$ reachable from $s$ i.e.m   $0 \leq r' \leq r \leq n$. We discuss this below. \\ 


\textcolor{blue}{below $\mathcal{I}, \mathcal{J} = \mathcal{I}^\prime$ and $\mathcal{T} \cup \mathcal{T}^\prime = [n]$}


\textcolor{blue}{these sets of agents are different from the sets of agents above and is general; general in terms of initial state $s_{init}$ }

Suppose $s$ is such that agents at index in $\mathcal{I}:= \{i_1,i_2,\dots, i_r\}$ are at $s_{init}$ and those at $\mathcal{J} := \{j_1,j_2,\dots, j_{n-r}\}$ are already at goal. Let agents in $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ be the ones transiting from $s_{init}$ to $goal$ i.e., $s \in \mathcal{S}_{n,r}$ and $s' \in \mathcal{S}_{n,r'}$ where $n \geq r \geq r' \geq 0$ and $n \geq 1$. \\ \\
$P(s'|s,a)  \\= \langle \phi(s'|s,a), \theta \rangle  \\= \langle \phi((s'_1,s'_2,\dots,s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n) ), (\theta_1,1,\theta_2,1,\dots,\theta_n,1)\rangle  \\ = \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots, \theta_n,1) \rangle  \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle \phi(s|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle \phi(g|s,a_t), (\theta_t,1) \rangle \\ 
= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle (-a_i, \frac{1-\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle (a_t, \frac{\delta}{n.2^{r-1}}), (\theta_t,1) \rangle \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \{ \frac{1-\delta}{n.2^{r-1}} + \langle -a_i, \theta_i \rangle \} + \sum_{j \in \mathcal{J}}   \frac{1}{n.2^{r}}  + \sum_{t \in \mathcal{T}} \{ \langle a_t,\theta_t  \rangle + \frac{\delta}{n.2^{r-1}} \}   \\=  r'. \frac{1-\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}  + (r-r'). \frac{\delta}{n.2^{r-1}} + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}   + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} a_{i,p}. \theta_{i,p}      + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   a_{t,p} .\theta_{t,p}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} -  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{t,p}) = sgn(\theta_{t,p})\} -  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}}  \frac{\Delta}{n(d-1)} \Big \{  d-1 -  2 \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}}    \frac{\Delta}{n(d-1)} \Big \{  d-1 - 2\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} -   \frac{\Delta}{n(d-1)} \Big \{  r'(d-1) -  2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     +    \frac{\Delta}{n(d-1)} \Big \{  (r-r').(d-1) - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n(d-1)} \Big \{  (r-2r').(d-1) + 2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\ $

So, we have 
\begin{equation}
    P(s^\prime | s, a) 
=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}            \label{general transition probability}
\end{equation}

\pt{this incorporates the new features. Also, this will be the optimal probability when the sign matching property holds.}

\textcolor{blue}{we can avoid `line break' commands above } \textcolor{red}{ok, removed them but now proof may seem clumsier}  \textcolor{blue}{ok, we will see a way out, perhaps, we will introduce them}



\textcolor{blue}{we should use available  macros for lemma, proof, etc. see the style file.} 

\textcolor{blue}{these help where the proof starts and importantly ends -- Paul Halmos tomb-stone mark}
\textcolor{red}{ok, this is new for me. i'll try to learn this.}


Initial lines (not mentioning number since it is changing as we are modifying content above) use linearity assumption, definition of features and decomposing the inner product over agents who remain put at $s_{init}$, transit to goal and remain put at goal. In the next few lines, we expand the inner product terms and summations, use the definition of actions and theta and rearrange. Then, just rearrange different terms.  The indicators make sure appropriate sign is given to the dot product depending on signs of components of action and that of theta, \textcolor{blue}{we will cite some papers about these signs }. 

\textcolor{blue}{this is helpful to the reader}

\textcolor{blue}{let's write the role of indicator function above} \textcolor{red}{role as in?}


\\
\\
Notice that for a given global action, the  transition probability from any $s \in \mathcal{S}_{n,r}$ to any $s' \in \mathcal{S}_{n,r'}$ as long as the transition is possible (i.e., $s' \in \mathcal{S}_{n,r'}(s)$) remains the same as above. 


 
Another important probability is that of transition to global goal state after taking a global action a in any state $s \in \mathcal{S}_{n,r}$. \\  \\

\\
\\
 $ P(s'=(g,g,\dots,g)|s,a) \\ = \langle \phi(s' = (g,g,\dots, g)|(s,a)), \theta \rangle \\ = \langle (\phi(g|s_1,a_1), \phi(g|s_2,a_2),\dots, \phi(g|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle \phi(g|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle (a_i, \frac{\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j,1) \rangle \\ = \frac{r\delta}{n2^{r-1}} + \sum_{i \in \mathcal{I}} \langle a_i,\theta_i \rangle + \frac{n-r}{n2^{r}} \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  a_{i,p} \theta_{i,p} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}}  \frac{\Delta}{n(d-1)} \Big\{ d-1 - 2  \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
  \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  +  \frac{r \Delta}{n} - \frac{2 \Delta}{n(d-1)} \sum_{i \in \mathcal{I}}    \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
 $
\\
\\
This is very similar to above proofs and no new idea is used, only the state is explicitly mentioned.
\\

\textcolor{blue}{write this as another lemma} \textcolor{red}{i had written this before writing the above general proof which is now a lemma. this one is specific for r=n and r'=0 which game me an idea of how to express for general case. should this be a lemma or corollary } \textcolor{blue}{yes, as said over phone. }


%\textcolor{blue}{ think it is $\newtheorem{lemma}{command for new lemma}$}

\subsubsection{$V^*$ for multiple cases}


General formula:  \textcolor{blue}{is this a theorem?} \textcolor{red}{It follows directly from Bellman equation}\\
 $V^*(s) = \{1  + |\mathcal{S}_{n,r-1}(s)| p_{a^*,r-1} V^*_{r-1} +  |\mathcal{S}_{n,r-2}(s)|p_{a^*,r-2} V^*_{r-2} + \dots + |\mathcal{S}_{n,2}(s)| p_{a^*,2} V^*_{2} + |\mathcal{S}_{n,1}(s)| p_{a^*,1} V^*_{1} \} . \{ 1 - P(s|s,a^*) \}^{-1}$

 \\ \\
 Below $p^*_{r,r'}$ denotes transition probability for a valid transition from state of type $r$ to that of type $r'$ under optimal global action in the respective instance specicified by $\theta$ and $n$ and $V^*_0 = 0$ \\ \\
For n = 1 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$ \\ \\ 
For n = 2 \\
For r = 1 \\ 
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For n = 3 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
\\

For n=4 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\

For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
For r = 4 \\
$V^*_4 = 1 + p^*_{4,4}V^*_4 + \binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1+\binom{4}{4}p^*_{4,0}V^*_0 = \frac{1+\binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1}{1-p^*_{4,4}} = \frac{1+\binom{4}{1}p^*_{4,3}\frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} + \binom{4}{2}p^*_{4,2}\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{4}{3}p^*_{4,1}\frac{1}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+\frac{ \binom{4}{1}p^*_{4,3} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} +\frac{ \binom{4}{2}p^*_{4,2}+\frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}}  = \frac{1+ \frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+ \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}}+\frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  }{1-p^*_{4,4}}$


\pt{can you see the closed form expression here?} \textcolor{red}{i can see a pattern but can't express it nicely.}

\pt{if not, can you confirm whether this notation is correct? -- $p^*_{r,r'}$ is the probability that number agent in the state $s$ were $r$, and the number of agents in $s'$ are $r'$?} \textcolor{red}{yes, line 308-309}

\pt{also can you recall me here -- what does the  $\binom{4}{2}$ or $\binom{3}{1}$ represent in terms of $r,n,$ and $r'$? $\binom{r}{r-r'}$} \textcolor{red}{yes,in the first factor of every term in the numerator}

\pt{I will try to get the closed form expression once you mention this.} \textcolor{red}{if you can get this it will be good to add}


\pt{Also can you summarize what are the intermediate results we have. summarize all of them no matter how  trivial or useful they are are. } \textcolor{red}{The general probability expression , The all in one result: $a^*$ is same for all states and is the one matching signs with each component of $\theta$, $V^*$ is same for all states of a particular type, $V^*$ are ordered and (due to) the claim on probabilities hold}

\pt{I can see  that you have many intermediate results.}












\textcolor{blue}{let's write here the  intermediate steps with pending proofs }
\textcolor{red}{done as of now, thought there's a pattern, to express it mathematically is a bit challenging, i'll try to think about this}

\subsubsection{Important result regarding monotonicity of V*, an independent result , and a result with weaker sufficient is stated and used below} \\

Consider the states space, $\mathcal{S} = \{s_1,s_2,\dots,s_n\} \cup \{x,y\} $. Let under some global action, the following markov chain be induced:
\\ Cost for any transition is constant and equal to 1. Transition probability from x to $s_i$ is represented as $p_{x,i}$ and from y to $s_i$ as $p_{y,i}$ for $i \in \{1,2,\dots,n\}$ and $p_{x,x}$ and $p_{y,x}$ represent the same from x and y respectively to x. Probability from y to y is represented as $p_{y,y}$. All probabilities are considered between 0 and 1 (strictly). Further, it holds that $p_{y,s} = p_{x,s} - \delta_s$ for every $s\in \{x,1,2,\dots,n\}$ where all $\delta_s \in (0, p_{x,s})$. (We would later require that assuming $p_{x,(.)}$ is monotonic, $\delta_s$'s are such that they preserve the monotonicity of $p_{y,(.)}$. But this assumption on $\delta_s$'s is not required in this discussion.) No other transitions are possible. For the sake of discussion, we assume that the states $s_1,s_2,\dots,s_{n}$ are absorbing states (potentially there may be all kinds of transitions from there but the long term value is known hence they can be considered terminal states with these values) with value function known respectively as $V_1,V_2,\dots,V_n$ while value of state $x$ is also known as $V_x$. Assume the following condition holds for the values: $V_1<V_2<\dots<V_n < V_x$. We want to relate $V_x$ and $V_y$. \\ \\
\tb{Claim:} $V_x < V_y$ \\ \\
$p_{y,y} = 1-p_{y,x}-\sum_{i=1}^{n}p_{y,i} = 1-(p_{x,x} - \delta_x) - \sum_{i=1}^n(p_{x,i}-\delta_i) = \delta_x + \sum_{i=1}^n \delta_i$ \\ \\
$V_x = \sum_{i=1}^np_{x,i}(1+V_i)+p_{x,x}(1+V_x)$ \\ \\
Similarly, \\
$V_y = \sum_{i=1}^np_{y,i}(1+V_i) + p_{y,x}(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^n(p_{x,i}-\delta_i)(1+V_i) + (p_{x,x}-\delta_x)(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^np_{x,i}(1+V_i) + p_{x,x}(1+V_x)-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_i)\} + p_{y,y}(1+V_y) $ \\ \\
From the definition of $V_x$ above and monotonicity of V's, we have : \\
$V_y > V_x-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_x)\} + p_{y,y}V_y = V_x-p_{y,y}(1+V_x) + p_{y,y}(1+V_y) \\ \implies V_y - V_x > p_{y,y}(V_y -V_x) \\ \implies (1-p_{y,y}) (V_y - V_x) > 0 \\ \implies V_y>V_x $

 \\ 


\subsubsection{ALL IN ONE THEOREM - Proving $a^*$ is the one that matches sign with $\theta$ for every state, $V^*$ is same for states of a particular type, there exists ordering of $V^*$'s : all go hand-in-hand \textcolor{blue}{lines after \ref{regret} are basic and hence need to be cross-checked}} 
\tb{Base Case}  \\ By definition, $V^*_0 = 0$. \\
Take any $s \in \mathcal{S}_{n,1}$. \\
\tb{Q.} What is $a^*$? \\
For s, only possible next global states are s itself and all-at-goal (g). This is akin to the single agent problem. But any transition probability also depends on actions of others. \\
Suppose $p^a_{s,g}$ denotes the transition probability from s to g. Then we have, \\
$V_1(s) = (1-p^a_{s,g}).(1+V_1(s)) + p^a_{s,g}.(1+V_0) \implies V_1(s) = \frac{1}{p^a_{1,0}}$ \\
Thus the optimum action at s is the one that minimizes $V_1(s)$ i.e., maximizes $p^a_{s,g}$. From the above general equation (line 177), the transition probability is maximum when $a$ is such that it matches all signs with $\theta$ for the respective components of agent who was initially at s. The signs of other components do not matter. Hence there could be multiple $a^*$ for any particular $s \in \mathcal{S}_{n,1}$. \\
Notice that this will hold true for any $s \in \mathcal{S}_{n,1}$. Note that particular $a^*$ whose sign matches with components of $\theta$ (for every agent), is common for possible $a^*$ for every $s \in \mathcal{S}_{n,1}$. We consider this $a^*$ in particular. \\
Since from the general formula, for a fixed instance ($\theta$), for a given action the probability only depends on r and r', it is the same for all states s $\in \mathcal{S}_{n,1}$ i.e., $p^{a^*}_{s,g} = p^{a^*} \forall s \in \mathcal{S}_{n,1}$. This $V^*_1(s) = V^*_1 \forall s \in \mathcal{S}_{n,1}$ \\
Since transition probability for this action is strictly between 0 and 1, $V^*_1 > V^*_0=0$ \\
\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:\\ $a^*$ is the one that matches sign with $\theta$ for any state in $\mathcal{S}_{n,k}$, hence $p^*(s \in \mathcal{S}_{n,k}  \xrightarrow{}s' \in \mathcal{S}_{n,k'}(s)) = p^*_{k,k'}$, $V^*_k(s)=V^*_k$ for any $s \in \mathcal{S}_{n,k}$ and $V^*_k>V^*_{k-1}$. Now, we need to show the same for $r+1$. \\
Consider any $s \in S_{n,r+1}$. \\
$V^a(s) = \sum_{s' \in \mathcal{S}(s)\textbackslash \{s,g\}} P(s'|s,a)\{1+V^*(s')\} + P(s|s,a).\{1+V^a(s)\} + P(g|s,a).\{1+V^*(g)\}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +\sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} p^a_{r+1,r'}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \sum_{i \in [n]} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r'}  - \binom{r}{r'-1} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Big  \}$ \\ 
Observe that the third term is always non negative since when $r'>r/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} >V^*_r$ while for $r' \leq r/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_r$. Note that the above arguments is for $r' \in [r]$. To minimize $V^a(s)$, we need to minimize $P(s|s,a)$ as well (check after rearrangement as it will appear in denominator as 1-P). Clearly, the action that matches sign with all components of $\theta$ minimizes $V^a(s)$. Hence this is $a^*$. Notice the above arguement holds for any $ s \in \mathcal{S}_{n,r+1}$. Hence $a^*$ is the same for each of them. Hence $p^*(s \in \mathcal{S}_{n,r+1} \xrightarrow{}s' \in \mathcal{S}_{n,r'}(s)) = p^*_{r+1,r'}$. Hence $V^*(s) = V^*_{r+1}$ for each of them. \\

\\ \\
Proving $V^*_{r+1} > V^*_r$ is tricky. We will make a suitable assumption on probabilities and later show that it holds under suitable choices of $\delta$ and $\Delta$. \\
\tb{Claim} If for every $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.  \\
We will justify that the assumption on probabilities in this claim holds for our features under suitable $\delta$ and $\Delta$. For now lets assume this holds for our case and prove the implication part of claim. \\
Return to the induction argument. \\
$V^*_r = 1+\sum_{r' \in \{0,1,\dots,r\}}\binom{r}{r'}V^*_{r'}$ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'}$ \\
Suppose for every $r' \in \{0,1,2,\dots,\lfloor\frac{r+1}{2}\rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}-\delta_{r'} $ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor\ +1 , \lfloor\frac{r+1}{2}\rfloor+2,\dots,r-1,r\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}+\delta_{r'} $ where $\delta_{r'}>0$ for every $r' \in \{0,1,\dots,r\}$\\ 
Note that, $\sum_{r' \in \{ 0,1,\dots,r,r+1\}} \binom{r+1}{r'}p^*_{r+1,r'} = 1 \\ \implies \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r+1}{r'}p^*_{r+1,r'} + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r+1}{r'}p^*_{r+1,r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} (\binom{r}{r'}p^*_{r,r'}-\delta_{r'}) + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} (\binom{r}{r'}p^*_{r,r'} + \delta_{r'}) + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies  \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r}{r'}p^*_{r,r'}-\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + 1 -  \sum_{r' \in \{0,1,\dots,r-1,r} \binom{r}{r'}p^*_{r,r'} \\ \implies p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} $ \\ \\
Now, going back to $V^*_{r+1}:$ \\ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}(\binom{r}{r'}p^*_{r,r'} - \delta_{r'})V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}(\binom{r}{r'}p^*_{r,r'}+\delta_{r'})V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} V^*_{r'}+ \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, r-1,r\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\=  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ > p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{\lfloor \frac{r+1}{2} \rfloor + 1}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  (  \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} - \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}  )V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ >  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r $ \\ 
Thus,\\
$V^*_{r+1} >   p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r \implies (1-p^*_{r+1,r+1})(V^*_{r+1}-V^*_r)>0 \implies V^*_{r+1} > V^*_r$ \\
Above inequalities used monotonicity of $V^*$ due to induction assumption. \\
Below we justify that the assumption in the above claim holds for our case.

\subsubsection{Sufficient conditions on $\delta$ and $\Delta$ for well defined probabilities; \textcolor{blue}{$\delta$ is conflicting with high probability $\delta$}}

$p^a_{r,r'} < 1$ for every $r \in \{1,2,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$. \\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  <   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{1} <   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{\frac{n-r}{2}}{n2^{r-1}}        +    3\Delta  =  \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} +    3\Delta =  \frac{(r'-0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} +    3\Delta < \frac{0.5n(2-2\delta)}{n.2^{r-1}} + 3\Delta  < 1-\delta + 3\Delta$ \\
To ensure $p^a_{r,r'}<1$ it is sufficient to ensure $1-\delta + 3\Delta<1 \implies \delta > 3\Delta$ \\
Similarly, we must ensure, $p^a_{r,r'} > 0$ for every $r \in \{0,1,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$. \\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  > \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') -  \frac{2 \Delta}{1} > \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} - 3\Delta > \frac{(r' -0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta > \frac{( -0.5n)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta = \frac{ \delta }{2^{r-1}} - 3\Delta$ \\
To ensure, $p^a_{r,r'} > 0$ it is sufficient to ensure $ \frac{ \delta }{2^{r-1}} - 3\Delta > 0  \implies \delta > 3.2^{n-1}.\Delta$. \\ Observe that since $n \geq1$, condition from $p>0 \implies $ condition from $p<1$  Also note that in the above, we have assumed $\delta < 0.5$. Hence we can fix any $\delta, \Delta $ and $n$ that satisy the above conditions in order to fix a class of instance as above.




\subsubsection{Justification of assumption in the claim} 
Recall that in the above claim, we assumed that: for every $r \in [n-1],$ for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$. \\
Below, we will derive sufficient conditions on $\delta$ and $\Delta$ such that this assumption holds. \\
Also note that from below section we have $\delta<0.5$ and $\delta>3.2^{n-1}\Delta$ so that all probabilities are well defined.
\\ \\
\tb{For $r'\leq \lfloor\frac{r+1}{2}\rfloor$}, \\
$\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \frac{r+1}{r+1-r'}p^*_{r+1,r'}<p^*_{r,r'} \Leftrightarrow \\(r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \\ \Leftrightarrow  (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \\ \impliedby (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \Leftrightarrow \frac{\Delta}{n}\frac{r^2}{8} + (r+1) \frac{\Delta}{n}<(r+1)\frac{1-2\delta}{n2^{r+1}} \Leftrightarrow \frac{\Delta}{n}(\frac{r^2}{8}+r+1)<(r+1)\frac{1-2\delta}{n2^{r+1}} \impliedby \Delta (\frac{n^2}{8}+n+1)<\frac{1-2\delta}{2^{n}} \Leftrightarrow \Delta < \frac{1-2\delta}{2^{n}(1+n+\frac{n^2}{8})}$ \\ \\
Similarly, \\ \tb{For $r' > \lfloor \frac{r+1}{2} \rfloor$}, \\ 
$\binom{r+1}{r'}p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \\ \frac{r+1}{r+1-r'}p^*_{r+1,r'}>p^*_{r,r'} \Leftrightarrow \\ (r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow \\ (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \Leftrightarrow \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow  \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0  \impliedby  (\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0 \\ \Leftrightarrow \frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2) - 0.5(r+1)(\frac{1-2\delta}{n.2^{r}}) >0 \\ \Leftrightarrow \frac{(r'-r-0.5)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2)  >0 \impliedby \frac{(-r-0.5)(1-2\delta)+0.5n }{n.2^{r}}   >   \frac{\Delta}{n}  (r^2-r-1)  \Leftrightarrow \frac{(-r-0.5)(1-2\delta)+0.5n }{1}   >   \frac{\Delta}{1}  (r^2-r-1)  (2^{r}) \\ \impliedby (-n-0.5)(1-2\delta)+0.5n    >   \Delta  (n^2-n-1)  (2^{n})$ and $ (-n-0.5)(1-2\delta)+0.5n    > 0 \\ \impliedby 0.5n-n+2n\delta-0.5+\delta>0$ and $ 0.5n-n+2n\delta-0.5+\delta >   \Delta  (n^2-n-1)  (2^{n}) \\ \impliedby (2\delta-0.5)n>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2-n-1)  (2^{n}) \\ \impliedby 2\delta-0.5>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2-n-1)  (2^{n}) \\ \Longleftrightarrow \delta>\frac{1}{3}$ and $n > \frac{0.5-\delta}{2\delta-0.5}+ \frac{\Delta  (n^2-n-1)  (2^{n})}{2\delta-0.5} \\ \impliedby \delta>1/3 $ and $\Delta  (n^2-n-1)  (2^{n})<3\delta-1 \impliedby \Delta < \frac{3\delta-1}{(n^2-n-1).2^{n}}$ \\ For n = 1, the second condition must not be used as it is trivially satisfied in the previous step.
\\
Finally we obtain for the desired instance, fix $1/2>\delta>1/3$. Then, fix, $\Delta< 2^{-n}.min\{\frac{3\delta-1}{n^2-n-1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2/8}\}$ \\



\subsubsection{Another way to think of Q-V difference introduced above \textcolor{blue}{this is advantage function, isn't?}} \textcolor{red}{yes, it's like expected value of the advantage function since there is expectation over $a_1$ according to the policy \\ also i've modified below for new features}
\\
\\
From \ref{difference of probabilities} we have the following. In the below, $s_t$ represent global state at time t (Note it's not individual state), $\textbf{s}_t$. Similarly $a_t$ is global action at t.

\begin{lalign} 

$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1) \\
= \mathbb{E}_{a_1 \sim \pi(s_1)}[c(s_1, a_1) + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}V^*(s_2)] - V^*(s_1)  $ \\
Using Bellman Equation and cost is 1
\\ 
$=  \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{  1 + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}[V^*(s_2)] - V^*(s_1) \Big \}$
\\ Expand the Expectation $ \\
=   \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  P(s_1|s_1,a_1) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1) \Big \}
\\ $ Use expression of probability from above$
 \\= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2)  - V^*(s_1) \Bigg \}
\\$ Rearranging the terms $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*(s_1) \Big\} 
\\ $ Notice from the general expression of probability from previous proof $\\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - V^*(s_1) \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} 
\\$ Expand V*(s_1) $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 + P(s_1|s_1,a_1^*)  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - \Big\{ 1 +  P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1, a_1^*) V^*(s_2) \Big\} \Bigg \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p})\neq sgn(\theta_{i,p})\} V^*(s_1) \Big\} 
\\$   

Rearrange and combine  terms to have a  lower bound 

$ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $
\end{lalign}


\\



\subsubsection{Dealing with the sum of Probability differences above} 

Recall from earlier, \\ 
$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)   
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \\
 \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 The first term is problematic and it is not clear how to deal with it. Let's investigate the summation inside the expectation of the first term: \\ 
 $\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2) \\ = \sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} [P(s'|s_1,a_1)-P(s'|s_1, a_1^*)] V^*(s') $ (Now, use results from above sections) \\
 = $\sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\} V^*_r $ \\
= $\frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{\sum_{s' \in \mathcal{S}_{n,r}} [\{   \sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p}) \}]  \Big\}   \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n}   
 \sum_{s' \in \mathcal{S}_{n,r}} [ \mathbbm{1}\{s'_i = s_{init}\}   \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   - \mathbbm{1}\{s'_i = goal\}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \}]  \Big\} \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  
 \sum_{s' \in \mathcal{S}_{n,r}} \mathbbm{1}\{s'_i = s_{init}\}     -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \sum_{s' \in \mathcal{S}_{n,r}} 
 \mathbbm{1}\{s'_i = goal\} \Big\}  \Big\} 
 \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \binom{n-1}{r-1}    -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \binom{n-1}{r} \Big\}  \Big\} \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \{ \binom{n-1}{r-1}    -   \binom{n-1}{r} \} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} V^*_r  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} + V^*_{n-r}  \frac{2(n-r)-n}{n} \binom{n}{n-r} \} \Big\}   \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} - V^*_{n-r}  \frac{2r-n}{n} \binom{n}{r} \} \Big\}  \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  - V^*_{n-r}   \} \frac{2r-n}{n} \binom{n}{r} \Big\} \geq 0. 
 $ \\
 \\
 Observe that when $r> n/2, V^*_r > V^*_{n-r}$ and vice-versa (refer result above) \\
 Hence we have established that, \\
 $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1) \geq \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\ \\
 To generalize, we need to show that the above inequality holds for any $s_1 \in \mathcal{S}$ and not just $s_{init}$. We will use this result below.

 \subsubsection{Now going back to Lower Bound Proof with Inequality using above result}
 From earlier, expected regret in the $k-th$ episode: \\
$R_{\theta,k} \\ = V^{\pi_\theta}(s_1) - V^*(s_1) 
\\ 
 = \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)$ \\
\\ Using above result, \\

 $R_{\theta,k} \\ \geq  \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_1 \neq goal \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 By recursion and the generalized result from the section above,
 we have: \\

 $R_{\theta,k} \\ \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{k} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_h \neq goal \} \mathbbm{1}\{sgn(a^h_{i,p}) \neq sgn(\theta^h_{i,p})\} \Big\}  $ \\
 where, the Expectation is taken with respect to trajectory induced in the $k-th$ episode by the interaction of policy $\pi$ and transition kernel $P_{\theta}$. Now, the total expected regret over $K$ episodes is: \\
 $
 R_{\theta}(K) \\
 \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{t=1}^{\infty} \mathbb{E}_{\theta, \pi} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_t \neq goal \} \mathbbm{1}\{sgn(a^t_{i,p}) \neq sgn(\theta^t_{i,p})\} \Big\}
 $ \\
 Analogous to Min et al, Cohen et al, we define: \\
 $N = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} $ and for agent $i \in [n]$,\\
$N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta^t_{i,j})\} $  \\
Thus, $R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]} \sum_{j=1}^{d-1} N_{i,j}(\theta) \}$ \\
To use the standard Pinsker's Inequality, we need $N_{i,j}(\theta)$ to be bounded almost surely which is known to not hold for SSPs (Min et al, Cohen et al). Hence, we use the capping trick introduced by Cohen et al and also used by Min et al. In this trick, we cap the learning process to a predetermined T. If the learning process (i.e. $K-th$ episode) ends before this, the agents continue to remain at $goal$. In this case the summation for the actual process and the capped process is the same. On the other hand when K episodes end beyond T, we have a truncated sum. Due to non-negativity of each part, the sum for the capped process lower bounds the actual sum. \\ Define \\ $N^- = \sum_{t=1}^T\mathbbm{1}\{s_t \neq goal\} $ and for any agent $i \in [n] $ and $ j \in [d-1],$\\ $N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta^t_{i,j})\} $ \\ 
It is easy to see that for any $i \in [n]$ and $j \in [d-1]$, $N^- =   N^-_{i,j}(\theta) + N^-_{i,j}(\theta^{j})  $ \\ where for every $\theta$, $\theta^j$ represents the vector that only differs at the $j-th$ index of every $\theta_i$ in $\theta = \{\theta_1,1,\theta_2,1,\dots,\theta_n,1\}$, where each $\theta_i \in \{\frac{-\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}\}^{d-1}$. \\ 
Thus,  $R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}$.  Notice that $\theta \in \Theta \iff \theta^{j} \in \Theta$ (This follows from definition of $\Theta$ \textcolor{red}{without this, following equation won't hold}). Then, we have: \\
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \{ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \} \\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^- - N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^-] - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}

Need to prove generalisation of Lemma C2 in Cohen et al 2020: If $T \geq 2KB^*$, then $\mathbb{E}_{\theta}[N^-] \geq KB^*/4$  \\ \textcolor{red}{Turns out similar lemma holds. Proof given below. We pick $T = 2KB_*$} \\
\textbf{Pinsker's Inequality(Min et al, Lemma E.3)} \pt{$TV(p,q) \leq \sqrt{KL(p,q)}$}

If $f:S^T\xrightarrow{}[0,D]$ then, 
$\mathbb{E}_{\mathcal{P}_1} (f(s)) - \mathbb{E}_{\mathcal{P}_2} (f(s))\leq D \sqrt{\frac{log(2)}{2}}. \sqrt{ KL(\mathcal{P}_2 || \mathcal{P}_1)}$  

\pt{Note that this will hold only if $|f(s)| \leq D \sqrt{\frac{log(2)}{2}}$?}
\textcolor{red}{I dont think so. $|f(.)|$ can be D}


\pt{don't use double back slash. These are not needed. just give one line spacing.}

Then, 
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  \mathbb{E}_{\theta, \pi}  [N^-] +  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] - \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] \} \Big \} \\ \geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{  \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] - \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] \} \Big \} \\ 
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
$

\textcolor{blue}{to update the above relations, equalities and inequalities } \textcolor{red}{done}
\\
\\
\\
For appropriate $\delta, \Delta$, $KL(\mathcal{P_{\theta}||\mathcal{P_{\theta^j}}}) \leq \frac{16.\Delta^2}{(d-1)^2.\delta}.\mathbb{E_{\theta}}[N^-]$  \\
\textcolor{red}{The above doesn't hold but} \\ We have the following for our case: \\
For appropriate $\delta$ and $\Delta$:
$ KL(\mathcal{P_{\theta}||\mathcal{P_{\theta^j}}}) \leq  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-] $
\\
\textcolor{red}{Need another intermediate similar lemma to simplify the KL-divergence term. \\ Assuming this also holds for our case, \\ }
\textcolor{red}{same result doesnt hold, but new one updated! (2-4-25)}

$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta V_1^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{1/2} \sqrt{3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]}  \} \Big \} \\
= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{\mathbb{E}_{\theta}[N^-]} \Big \} \\
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{T} \Big \} \\
= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \} \\ 
$\\
Notice that the term in bracket is independent of $\theta, i$ or $j$. Thus, we have: \\
$\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq  \Delta V_1^* |\Theta| \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \} \\
\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq   V_1^*  \Big \{ \Delta  KV_1^*/4 -   (KV_1^*)^{3/2}  \frac{2^{n+2}.\Delta^2}{\sqrt{\delta} (d-1)} \Big \} \\ 
$ 
Specifically, pick, $\Delta^* = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}$. \\ At this value of delta,\\
$\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq V_1^* \{  \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}. \frac{KV_1^*}{4} - \frac{(KV_1^*)^{3/2}.2^{n+2}}{\sqrt{\delta}(d-1)}.  (\frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}})^2\} \\ 
= V_1^* \{\frac{(d-1) \sqrt{\delta.K.V_1^*}}{2^{n+7}} - \frac{(d-1)\sqrt{\delta.K.V_1^*}}{2^{n+8}}\}
\\
\geq  \frac{(d-1).\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+8}} \geq \frac{d.\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+9}} $ \\ \pt{This makes it independent of number of agents, a very strong result? Is this correct or do we need to incorporate the number of agents here.} \textcolor{red}{potentially the intermediate results I used directly without verifying depend on n. the term i argued to be $+ve$ and ignored in lower bound certainly depends on n but very difficult to simplify(needs closed form V*)} \\
\textcolor{red}{update : it depends on n}

Since the average over entire set is lower bounded by the RHS, there must exist some parameter in the set for which the RHS is a lower bound. Hence proved. \textcolor{blue}{ok we will discuss the proof}. \\ \\
It remains to show that the $\Delta$ picked above is valid. \\ Hence, need to ensure that $\Delta = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}} < 2^{-n}.min\{\frac{3\delta-1}{n^2-n-1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2/8}\}$  \\ or, $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.min^2\{\frac{3\delta-1}{n^2-n-1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2/8}\}} $
\\ \\
\textcolor{blue}{updated later} \textcolor{red}{Although it is independent of $n$, it can be interpreted as a strong result in the sense that no matter how many agents are deployed to learn, this minimum regret will always hold. The independence also comes from ignoring the positive terms} \\ \textcolor{red}{(whose proof is as of now still incomplete )}. \\ \textcolor{red}{since now there is a dependence on $n$, the above para is not valid} 

\textcolor{blue}{we need to write the  statement that is proved, and also delineate that statement from the proof -- use macros provided in the style file} \textcolor{red}{This is not complete yet. Only if we can find the corresponding lemmas I've mentioned in the proof, it will be complete possibly with very different expression.} \\
\\
\textcolor{blue}{2/4/25} \textcolor{red}{The proof is now complete! Now we have one complete result!}
\\ 
\\
\textcolor{red}{3/4/25} \\
\tb{Theorem}: For any MASSP learning algorithm $\mathfrak{A}$, there exists a linear-mixture MASSP instance defined by appropriate parameters ($n, \delta, \Delta, \theta$) for whom the expected cumulated regret matches the reported upper bound $\widetilde{O}(\sqrt{K})$. \\ Specifically, the instance satisfies: \\ $\mathbb{E}_{\theta,\mathfrak{A}}[R(K)] \geq \frac{d.\sqrt{\delta}\sqrt{K.V^*_1}}{2^{n+9}}$ \\
for $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.min^2\{\frac{3\delta-1}{n^2-n-1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2/8}\}} $

\subsubsection{Generalisation of Lemma C2 of Cohen et al for our case-12/13-3-25}
\tb{Lemma:} For any deterministic learner, if $T\geq 2KV_1^*$, then, $\mathbb{E}[N_-]\geq KV^*_1/4$ \\ 

\textcolor{blue}{there is a relation between $B^\star$ and $V^\star_1$ and is given in the first half of this writeup }

\tb{Proof:} If capped process finishes before T, $N_-=N$. Else number of visits to goal state is less than $K$. \\Thus, $N_- \geq T-K$.\\ Thus, $\mathbb{E}[N_-] \geq \mathbb{E}[min\{T-K,N\}] \geq \mathbb{E}[\sum_{i=1}^Kmin\{T/K-1, N_k\}]$.\\
Since $T\geq2KV^*_1,$ and $V^*_1\geq1$ the lemma will hold for any policy (mapping of actions) if, $N_k \geq V^*_1$ with probability $\geq 1/4$ for any policy. Consider any policy. \\ We can lower bound the probability $\mathbb{P}[N_k \geq V^*_1]$ by the events that we transit to an $r=1$ state and stay there for next $\lceil V^*_r\rceil -1$ steps. \\Thus, \\
$\mathbb{P}[N_k \geq V^*_1] \\ = \mathbb{P}(s_2 \neq g|s_1=s_{init}).\mathbb{P}(s_3 \neq g|s_2).\mathbb{P}(s_4 \neq g|s_3)....\mathbb{P}(s_{\lceil V^*_1\rceil} \neq g|s_{\lceil V^*_1\rceil-1}) \\ = (1-p^{a(s_1)}_{n,0}).(1-p^{a(s_2)}_{s_2,0})...(1-p^{a(s_{\lceil V^*_1\rceil-1})}_{s_{\lceil V^*_1\rceil-1},0}) $ \\
For any state s, $1-p^{a(s)}_{n,0}$ is minimum when $p^{a(s)}_{n,0}$ is maximum. Check from line 1087 that this happens at $a^*$ which matches all signs with $\theta$. Further, $1-p^*_{s,0}$ when $s \neq g$ is minimum when $p^*_{s,0}$ is maximum at any $s \in \mathcal{S}_{n,1}$. Thus, we can lower bound the above product as: \\
$\mathbb{P}[N_k \geq V^*_1] \geq (1-p^*_{n,0}).(1-p^*_{s_2,0})...(1-p^*_{s_{\lceil V^*_1 \rceil -1},0}) \geq (1-p^*_{1,0})^{\lceil V^*_1 \rceil -1} \geq (1-p^*_{1,0})^{ V^*_1 -1} = (1-p^*_{1,0})^{ 1/{p^*_{1,0}} -1} \geq 1/e \geq 1/4$ \\
For the last second inequality, we use for $x\geq 1$, $(1-1/x)^{x-1}\geq 1/e$ \\
 Thus, $\mathbb{E}[N_-]  \geq \mathbb{E}[\sum_{i=1}^Kmin\{T/K-1, N_k\}] \geq KV^*_1/4$ \\


 
 \subsubsection{Alternate proof for dealing with $\mathbb{P}[N_k \geq V^*_1] \ge \frac{1}{4}$ 13-3-25}
 
\textcolor{blue}{the result below a general one}
 
 Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](s)$ as the probability that starting at state $s \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in R^+$. Further, $\mathbb{P}[N_k \geq x] = \mathbb{P}[N_k \geq x](s_{init})$. \\
 \tb{Claim} Consider any $s \in S_{n,r}$ where $r \in [n]$. Then, for any policy it holds for our instances that $\mathbb{P}^{\pi}[N_k \geq x](s) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](s')$ for all $x \in R$ where $s' \in \mathcal{S}_{n,r'}(s)$ for any $r' \in \{0\} \cup [r]$ with equality holding only at $\pi = \pi^*$  and $r'=r $ i.e., $s'=s$ respectively. Here $\pi^*$ is the policy of taking action $a^*$(the one matching all signs with $\theta$) at every state $s \in \mathcal{S}$. The equality in the middle says that for any $s \in \mathcal{S}_{n,r}$ under $\pi^*$, $\mathbb{P}^{\pi^*}[N_k \geq V^*_1](s)$ happens to stay a constant independent of $s$ and only depends on $r$.\\
 Proof will be similar to $V^*$ proof \\
 Will work on this later if above proof is not satisfactory.\\
 \tb{Proof} We will prove this by induction. \\
 \tb{Base Case:} For r=1: 
 Consider any $s \in \mathcal{S}_{n,1}$ \\
 For any $x \in R^+$, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x\rceil-1}$ \\
 One can check from the general formula for transition probabilities that the above is uniquely minimum when $\pi(s) = a^*$. Hence equality only holds at $\pi=\pi^*$.  \\
 Hence, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x\rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x\rceil -1}$ \\
 Recall that for the same action $a^*$ at any $s \in \mathcal{S}_{n,1}$, $P(g|s,a^*)$ remains the same. Hence, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x \rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) $ \\
 The only two possibilities for $s'$ are $s$ itself and $g$. \\
 Clearly for $s$ the equality holds and for $g$, $\mathbb{P}^{\pi^*}[N_k \geq x](s'=g) = 0$ \\ Hence, \\
  $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x \rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s')  $
  \\ Finally we showed that for any $x \in R^+$ for any policy $\pi$, for any $s \in \mathcal{S}_{n,1}$ and $s' \in \cup_{r' \in \{0,1\}} \mathcal{S}_{n,r'}(s)$,  \\
  $\mathbb{P}^{\pi}[N_k \geq x](s)  \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s')  $ \\
  where in the first inequality, equality holds only when $\pi = \pi^*$, the middle equality means that the probability is same for all $s \in \mathcal{S}_{n,1}$ and in the last inequality, equality holds only when $s' = s$. \\
  \\
  \tb{Generalization:} Assume the above holds for m = 1, 2,...,r i.e., for all $m \in [r]$ it holds that for any $x \in R^+$ for any $s \in \mathcal{S}_{n,m}$, for any policy $\pi$, for our instances, it holds that, $\mathbb{P}^{\pi}[N_k \geq x](s) \geq \mathbb{P}^{\pi^*}[N_k \geq x](s)=\mathbb{P}^{\pi^*}[N_k \geq x](m)\geq \mathbb{P}^{\pi^*}[N_k \geq x](s')$ where $\pi^*$ is the policy taking action $a^*$(the one matching signs with all components of $\theta$) at all states and $s' \in \cup_{m' \in \{\{0\} \cup [m] \}}\mathcal{S}_{n,m'}(s)$. Further, in the first inequality, equality only holds when $\pi =\pi^*$ and the middle equality implies that the probability is same for all states $s \in \mathcal{S}_{n,m}$ and in the last inequality, the equality only holds when $s' =s$.  \\
  Assuming this we need to show that the same holds for any $s \in \mathcal{S}_{n,r+1}$ \\
  Again consider any $x \in R^+$. \\
  Consider any $s \in \mathcal{S}_{n,r+1}$. \\
  We have, \\
  $\mathbb{P}^{\pi}[N_k \geq x](s) = \sum_{r' \in \{0,[r+1]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)} P(s'|s,\pi(s)) . \mathbb{P}^{\pi}[N_k \geq x-1](s') \\= P(s|s,\pi(s)). \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)). \mathbb{P}^{\pi}[N_k \geq x-1](s')$ \\ 
   If $x \leq 1$, then trivially, for all $s \neq g$, for all policies, $\mathbb{P}[N_k \geq x] =1$. Otherwise, we have the following:
  \\
$\mathbb{P}^{\pi}[N_k \geq x](s) \\ =  P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s') \\ 
  \geq P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s))  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \Bigg\} \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Bigg \} + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)}  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  
  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0, [r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \sum_{i \in [n]}      \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{t \in \mathcal{T}\} . \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{i \in [n]}        \{ \binom{r}{r'-1} -  \binom{r}{r'} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}     
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0,[r]\}} \sum_{i \in [n]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} 
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in [r]} \sum_{i \in [n]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  \Big \} \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{ \{ \binom{r}{r-r'} -  \binom{r}{r+1-r'} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big \} \Bigg \}   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{ \{ \binom{r}{r'} -  \binom{r}{r'-1} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big \} \Bigg \} \\
 = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{ \Big \{ \binom{r}{r'-1} -  \binom{r}{r'} \Big \} \Big \{ \mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq V^*_1](r+1-r') \Big \}      \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}        \Bigg \}$ \\ \\
 Notice that for $r' < (r+1)/2$, the binomial difference $\binom{r}{r'-1} - \binom{r}{r'}<0$ as well as probability difference $\mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r') < 0$ hence the product is $>0$. Similar argument holds for $r'>(r+1)/2$. For $r' = (r+1)/2$ it will be 0. Overall we can observe that the only terms dependent on action have non-negative coefficients for the sign matching indicator. Hence this term will be minimum when $a = a^*$.  Thus, we have, \\
 $\mathbb{P}^{\pi}[N_k\geq x](s) \geq   P(s|s,\pi^*(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} $\\ Also, \\
 $\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $ \\

Subtracting the above two equations, 
\\
$\mathbb{P}^{\pi}[N_k\geq x](s) - \mathbb{P}^{\pi^*}[N_k\geq x](s) \\ \geq P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) - P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) \\ \geq P(s|s,\pi^*(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) - P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) \\ 
= P(s|s,\pi^*(s)) (\mathbb{P}^{\pi}[N_k \geq x-1](s) - \mathbb{P}^{\pi^*}[N_k \geq x-1](s))$ \\
By recursion,  \\
$\mathbb{P}^{\pi}[N_k\geq x](s) - \mathbb{P}^{\pi^*}[N_k\geq x](s) \\ \geq P(s|s,\pi^*(s))^{\lfloor x \rfloor} (\mathbb{P}^{\pi}[N_k \geq x-\lfloor x \rfloor](s) - \mathbb{P}^{\pi^*}[N_k \geq x-\lfloor x \rfloor](s)) = P(s|s,\pi^*(s))^{\lfloor x \rfloor} (1- 1) = 0$  \\
Thus, $\mathbb{P}^{\pi}[N_k\geq x](s) \geq \mathbb{P}^{\pi^*}[N_k\geq x](s)$ \\
Also note that for equality, it must hold for each above inequality. Effectively this will only happen at $\pi = \pi^*$ \\ 
Recall, for any $s \in \mathcal{S}_{n,r}$, \\
$\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $
 \\
From the probability expression one can verify that the term $P(s|s,\pi^*(s))$ only depends on $r$. The only term that may differ due to $s$ is $\mathbb{P}^{\pi^*}[N_k \geq x-1](s)$. \\We claim that this is same too. This can be dealt with by induction on x itself. \\
For base case, $m = x-\lfloor x \rfloor$, for any $s \in \mathcal{S}_{n,r}$, $\mathbb{P}^{\pi^*}[N_k \geq m](s)=1$ \\ Hence showed for base case. \\ Assuming true for $m = x - \lfloor x \rfloor,  x - \lfloor x \rfloor+1,  x - \lfloor x \rfloor+2, \dots,  x - \lfloor x \rfloor+p $, we need to show that it holds for $m =  x - \lfloor x \rfloor + p+1$ \\ We can write for any $s \in \mathcal{S}_{n,r}$ that: \\
$\mathbb{P}^{\pi^*}[N_k\geq m ](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq m-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq m-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $ \\ Here the RHS doesn't depend on which $s \in \mathcal{S}_{n,r}$ is being chosen. Thus shown for m. \\
 Thus back in expression for $\mathbb{P}^{\pi^*}[N_k \geq x](s)$, $\mathbb{P}^{\pi^*}[N_k \geq x-1](s)$ is not dependent on $s \in \mathcal{S}_{n,r}$. Hence $\mathbb{P}^{\pi^*}[N_k \geq x](s)$ is same for all $s \in \mathcal{S}_{n,r}$.  \\
 Finally we need to show that, $\mathbb{P}^{\pi^*}[N_k \geq x](s) \geq \mathbb{P}^{\pi^*}[N_k \geq x](s') \forall s' \in \cup_{r' \in \{0,[r]\}}\mathcal{S}_{n,r'}$ with equality only at $s' = s$. \\
 Recall again, for any $s \in \mathcal{S}_{n,r+1}$, \\
 $\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in [r]} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} (\binom{r}{r'}  .  p^*_{r,r'} - \delta_{r'})  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\binom{r}{r'}  .  p^*_{r,r'}+ \delta_{r'}  )\mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r')) + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') )  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , r \}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') )  \\ >  P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](\lfloor \frac{r+1}{2} \rfloor + 1)) \\ =  P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  ( \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}\delta_{r'} - \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} \delta_{r'}) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1)  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  P(s|s,\pi^*(s)) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1) \\ > P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  P(s|s,\pi^*(s)) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( r) 
 $ \\
 Thus, we have, \\
 $\mathbb{P}^{\pi^*}[N_k \geq x](s) - \mathbb{P}^{\pi^*}[N_k \geq x](r) \geq P(s|s,\pi^*(s)).(\mathbb{P}^{\pi^*}[N_k \geq x-1](s) - \mathbb{P}^{\pi^*}[N_k \geq x-1](r))$ \\ By recursion and same arguments as before, \\
 $\mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r+1) >  \mathbb{P}^{\pi^*}[N_k \geq x](r)$
\\
 
 Hence the overall main induction argument for r holds. \\ \\
 Now, given this general theorem, where $s_1 \in \mathcal{S}_{n,1}$, we have, \\$\mathbb{P}^{\pi}[N_k \geq V^*_1](s) \geq \mathbb{P}^{\pi^*}[N_k \geq V^*_1](s_1) = (1-p^*(g|s,a^*))^{\lceil V^*_1 \rceil -1} \geq (1-p^*(g|s,a^*))^{ V^*_1  -1}  \geq 1/e \geq 1/4$

\subsubsection{Simplification of KL Divergence term 14-3-25} 
By chain rule of KL-Divergence, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)]$
\\
where, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $

\\
Let's simplify $\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)})$


\pt{Before doing this upper bound, why can't I break it into two terms -- first one where $s_t = (g,g,...,g)$, and the other one when $s_t \neq (g,..., g)$. I think the terms will be simplified a lot if you do this. 
 Also, you can go one step ahead and look at all the impossible transitions -- the log term will vanish for all of them. So, you are left with the cases when the transitions are valid. Now, you can utilize the same notations, $r$ to $r'$ type of transitions. For all such transitions, the ratio inside the log can be written in terms of the features and corresponding $\theta$, and $\theta^j$. note that we might need to carefully use the conditions on $\delta$ and $\Delta$ you obtained earlier. } \textcolor{red}{i won't be able to use $s_{t+1} \neq g$ inside ln(.), I need to check when the ratio inside ln maximises here:$s_{max}$ to provide upper bound. $s_{min}$ is not strictly required and any global state can be used instead as for eg. you suggested $g,g,g...$. Also yes, i'm thinking of possible transitions only although once the $s_t$ is fixed from outer  summation. But notice that when $s_t=(s_{init},s_{init},...s_{init})$, we will need to optimize over all $s \in S$.}

 \pt{i am not talking about $s_{t+1}$, I am saying you can look at the summation for two cases separately, $s_t = g$, and $s_t \neq g$. That will lead to some simplifications. } \\ \textcolor{red}{i wouldn't even think about $s_t=g$: cz then $s_{t+1}$ has to be $g$ with probability 1 : independent of $\theta$ or $\theta_j$ hence ratio inside log is 1 and this term will be 0, for other $s_{t+1}$ probability is 0 hence all those terms are 0. problem is to deal with the general case}

 \pt{exactly, that's where we can now only use the features and then explicitly write them in terms of the other parameters. Also, why you are trying to maximize the term inside the log? We can just write the expressions for $\theta$ and $\theta^j$ and then finally use some other bounds at the later stage.} 

 \textcolor{red}{explicitly substituting the probabilities using features leads to a huge sum, each of those $2^{r}$ terms will have ratio inside ln that looks like line 1765. It would be desirable to simplify those terms without bounding earlier. The reason i want to maximise is to bound before simplifying. I'm just trying an approach as of now.  }


 \pt{Some results from the Jaksch et al 2010 paper can be used at the later stage.}

 \begin{figure}[h!]
     \centering
     \includegraphics[width=0.5\linewidth]{Jaksch.png}
     \caption{The result from Jaksch et al 2010 paper. This holds for some conditions on $\delta', \epsilon'$. Need to check if these conditions hold in our work. this type of result can be used for each term inside the summation, possibly for each $r$ to $r'$ transition. }
 \end{figure}
 \textcolor{red}{i have seen this, it can't be used for our case. in fact i want to get the sum over $2^r$ next states in this form thats why looking for maximum of that ratio. thats what motivated line 1756. also if you look carefully, the above result is not exactly from Jaksch, it is from Min. Jaksch result is bit different. Also Min made has made a typo in this above equation.}
 
 


Notice this can be upper bounded as follows: \\ 
$\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ \leq \mathcal{P}_{\theta}(s_{t+1}= s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s_{min}|\textbf{s}_{t-1}, s_t = s, a_t = a)}) + (1-\mathcal{P}_{\theta}(s_{t+1  }= s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a)).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s_{max}|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s_{max}|\textbf{s}_{t-1}, s_t = s, a_t = a)})$ \\
where, \\ $s_{min} = arg min_{s' \in \mathcal{S}} \ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $ and, \\
$s_{max} = arg max_{s' \in \mathcal{S}} \ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ $ \\
Since, $s$ and $a$ are fixed in the outer summation, both $s_{min}$ and $s_{max}$ may depend on both $s$ and $a$. For any general transition, we investigate the behavior of the ratio above. Given $s_t$, we partition the set of agents at $s_{init}$, into $X$ and $Y$ based on action $a$. Suppose $a$ is such that agents in $X:$ $x_1,x_2,\dots,x_m$ have their $j-th$ components not matching signs with respective components of $\theta$. Hence, agents $x_1,x_2,\dots,x_m$ have their $j-th$ components matching signs with respective components of $\theta_j$. Similarly let agents in $Y: y_1,y_2,\dots, y_{r-m}$ be such that their $j-th$ components match with respective components in $\theta$. This means agents $y_1, y_2, \dots, y_{r-m}$ are such that their $j-th $ components do not match with $\theta_j$. Along with previous notations, the ratio can be analyzed as : \\ 
$
\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}  \\= \frac{\frac{(r'-0.5r)(1-2\delta) + 0.5n }{n.2^{r-1}}     +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)}\sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}}{  \frac{(r'-0.5r)(1-2\delta) + 0.5n }{n.2^{r-1}}          +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta^j_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta^j_{t,p})\} \Big \}} \\ 
$\\ \\
To find the optimal values of this ratio, we first check what happens at fixed $r, r'$ and then optimize for $r'$. Notice that the ratio is maximum when maximum number of agents who stayed had signs matched with $\theta_j$ and maximum number of agents who transited had signs matched with $\theta$

\textcolor{blue}{we are looking at $\mathbb{E}_P[X] - \mathbb{E}_Q[X]$ for two probability measures $P$ and $Q$. we can use change of variable and write $\mathbb{E}_Q[X] = \mathbb{E}_P[X \frac{dQ}{dP}]$? }

\textcolor{blue}{policy is $\pi_\theta$ and does $\theta$ refer to something else? }

\textcolor{blue}{based on a call on Sat 10pm, 22/3}
\textcolor{red}{hi, i thought we weren't meeting yesterday} \\
\pt{\url{http://joschu.net/blog/kl-approx.html} -- we can use some ideas from here.} \textcolor{blue}{this unbaised estimator of KL with low variance (by John Shulmann of PPO fame) would be very good to use in computations} \textcolor{red}{Im very doubtful, this blog is about constructing suitable estimate of kl-div from samples. but we need to analytically express kl-div or its suitable upper bound}

\pt{The above blog is suitable for the computations, isn't it?} \textcolor{red}{if by computation u mean implementing learning algo for massp, then no. I dont know if you are referring to any other kind of computation}

\pt{can we make use of the indicator present in line 1775 and bound the entire term.}

\pt{Other possibility is to take out the smallest of $\sum_{i\in I \cap T'}$ and $\sum_{t\in T}$?} \\ \textcolor{red}{can u try these and update above?}

\pt{Just for clarity, what I remember is:}

\pt{$\mathcal{I}$: Set of all agent are $s_{init}$.}

\pt{$\mathcal{J}$: Set of all agents at $g$}

\pt{$\mathcal{T}$: Set of all agents from $\mathcal{I}$ who move from $s$ to $g$.}

\pt{$\mathcal{T}'$: set of all agents from $\mathcal{I}$ who stayed at $s$}


\pt{If the above is correct, then $\mathcal{I}\cap \mathcal{T}'$ and $T$ are disjoint?} \textcolor{red}{yes, also above is correct}


\pt{Alternatively, upper bound the numerator, and lower bound the denominator and vice-versa and then take the min.} 
\textcolor{red}{the bounding of individual ratio doesn't help later, then there would be $2^r$ type factor}  \\ \textcolor{blue}{we can use min of two bounds and see how it effects the regret bound}

\pt{Also, note that only the orders as of now with respect to $n$ are important, not the front constants. As long as we are able to get some order of the regret bound wrt $n$, we are good.}


\pt{Any updates after Saturday?} \textcolor{red}{no break thru yet}

\textcolor{blue}{$\delta$ and $\delta_j$ are vectors with entries +1s and -1s. When entries are  +1s and 0s the Hamming distance between them is the number of entries that differ. we can \emph{temporarily} take -1s as 0s. this may  help to bound the KL$(\delta|| \delta_j)$.}
\\
\textcolor{red}{I have an update : today I performed computation of the sum in line 1758 for many instances of n,a,$s_t$ and realized that it is maximum at $s_t = (s_{init},s_{init},...,s_{init})$ : contradictory to what i was hoping (max for states of type r=1). Turns out this can be explained by property of KL-divergence. So we can upper bound this summation for any $s_t$ by the summation at this initial state. As of now i don't know if the upper bound i wish to obtain (same/similar as given in Min) still holds. Im trying to see that via computations. Will update further soon.}

\pt{Wasn't this observation intuitive and follows from the fact that KL is positive, and  when I told you that for the case when $s_t = (g,g,g...g)$, then one term was getting zero?} \textcolor{red}{Pls explain us how this is intuitive from terms becoming 0 when st is all at g, in the next meeting. Also do respond to my earlier responses on your above remarks, its further confusing when you suggest something and not elaborate anything. Also next meeting pls come prepared to explain the steps in upper bound proof that i had asked in January. The note you send is unclear to me.}

\pt{What are the next steps in theory?}

Meeting link: \url{https://ucf.zoom.us/j/99575809604?pwd=dar1hN9fReFbU4yae8Bp4YGDKfaBeP.1}
\\ \\
Property of KL-Divergence: https://math.stackexchange.com/questions/4986295/partition-form-of-the-kl-divergence


\subsection{Simplifying KL-Divergence}

By chain rule of KL-Divergence, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)]$
\\
where, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $ \\
Notice that in the above, for any fixed $(s,a)$, the inner summation is itself a KL-divergence. \\ 
Let's simplify it first: \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\  = \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) $ \\
\tb{Claim :} The above KL-divergence is maximum at $s_t = (s_{init}, s_{init},\dots, s_{init})$. (Proof can be shown by refinement property) \\
Hence we'll upper bound using the inner KL for s being global initial state. Fix this as s now.
The following holds as $KL(A|B) \leq KL(A|B) + KL(B|A)$ since $ KL(B|A) > 0$: \\ \\
$\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\ \leq   \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) + \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}) \\= \sum_{s' \in \mathcal{S}} (\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) ).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\
= \sum_{s' \in \mathcal{S}} (\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) ).\ln(1 + \frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\
\leq \sum_{s' \in \mathcal{S}} \frac{(\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) )^2}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)} \\
\leq 2^n . \frac{max_{s'}( \langle \phi(s'|s,a), \theta - \theta_j \rangle)^2}{\mathcal{P}_{\theta_j}(s_{t+1}=g|s_t = s, a_t = a)} \leq 2^n . \frac{(\frac{2 \Delta}{d-1})^2}{\frac{\delta}{2^{n-1}} - \Delta}
$ \\
From the sufficiency conditions, $\Delta < 2^{-n}. \frac{2\delta}{3} $. \\ Thus, \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)})  < 2^n. \frac{(\frac{4\Delta^2}{(d-1)^2})}{\frac{2\delta}{3.2^{n-1}}} = 3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $ \\ 
Hence, going back above: \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\  = \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) < 3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $ \\
Thus, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ < \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} \\ =  \mathcal{P}({s}_{t} \neq g) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $  \\ \\ Therefore from earlier, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] \\ <  \sum_{t=1}^{T-1} \mathcal{P}({s}_{t} \neq g) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} \leq  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} .  \sum_{t=1}^{T} \mathcal{P}({s}_{t} \neq g)  =  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]  $
\\
We use the above result in lower bound proof.

\pt{This seems good. Can you also write why the inequality in line 1847 holds} \\ \textcolor{red}{you meant the 1st line in the equations right? ive mentioned now in line 1848} \pt{yes, got it.}

\pt{Does that mean we now have a lower bound proof? I can see that the KL bound is exponential in $n$, will it lead to exponential bounds? or will it create some problems in the lower bound?}
\\
\textcolor{red}{yes we have a lower bound now. yes it looks exponential but from sufficient conditions, $\Delta$ is also of exponential order hence overall the bound is not exponentially large. from computations i've verified that this is quite tight(off by 1 order of magnitude for small n's and this difference decreases as n increases. hence we have a reasonably tight bound). ive updated and completed the lower bound proof(page 38). finally we get lower bound that scales as $1/2^n$. but we also get $\sqrt{K}$ }


\pt{Great!! So, we have the lower bound with $\sqrt{K}$, thus as tightest lower bound in terms of $K$, and can you explain what is the regret lower bound implication as $n$ increases? -- somehow not very clear to me. Particulary, i dond't understand this statement of yours  ``this difference decreases as n
increases. hence we have a reasonably tight bound''. } \textcolor{red}{yeah no problem, i will clear this in next meeting}

\pt{I think, now is the time to clean it and write the results in a nice format with all the details and explaination of each step. Can you explain the entire proof in our next meeting, and we can start writing it. }
\textcolor{red}{yes i wanted to explain everything too}
\pt{Let us connect on Friday evening 7:00 PM or Sat morning 9:00 AM India time, we can discuss this for a long time with all the details.} \textcolor{red}{sure, saturday 9am would be best}

Meeting link: \url{https://ucf.zoom.us/j/99575809604?pwd=dar1hN9fReFbU4yae8Bp4YGDKfaBeP.1}



\subsection{Related Work}
\label{subsec:related_work}



\\\\\
\newpage
\section{7-4-25}
\\
\input{CR_Sections/6_experiments}


\section{\textit{Proof of Lower Bound}}

\pt{Need to write this thing cleanly with proper justifications. Why the following makes sense, and how would this capture the hardest instance. What is the role of congestion in this example?}

We construct and analyze a family of hard to learn instances based on above discussion.  Further, we restrict $\theta$ such that $\theta_{i} \neq \theta_{j}$ $ \forall$ $ i \neq j \in [n]$ i.e., no two $\theta_i$ are the same. Let this set be denoted as $\Theta$. \pt{Why this assumption will hold. there is lot of symmetry in the problem, so $\theta$'s for two agents will be same?}. \textcolor{blue}{It's not an assumption. It's a restriction of the class of SSPs instances I'm considering. I'm free to do so. Why I do this is the rest of paragraph about. Also $\theta$ is an instance parameter, it can be anything. A way to think about this is that : even if two agents took same action, the contribution to probability of transition to any global state is not the same, this is one way how agents are not identical!} This ensures that the action to be taken by each agent to maximize the probability of transition to the all-at-goal state is different for every agent so that we don't need to consider the congestion component of the cost when the policy of maximizing the probability to reach all-goal is executed.
To further reduce complexity of the analysis, we let the private cost associated with any global action in any non-goal state be equal to 1 and that in goal state equal to 0. This will be used to ensure that the \textit{best} policy is the one that matches sign with all components of $\theta$(see all-in-one theorem \ref{all_in_one}).  \\
Consider any instance, defined by among other parameters by $\theta$. \\
Suppose in episode \textit{k}, agents take actions according to policy $\pi^k_{\theta}$. Let, $\tb{s}_t$ represent the global state and $\tb{a}_t$ the global action at time $t$. Then, the expected regret for the \textit{k-th} episode is:

\pt{In the regret definition below the policy seems to have the parameters $\theta$, whereas we have originally used $\theta$ as the parameters for the transition probabilities?} \textcolor{red}{yes, we are analyzing regret of a class of instances simultaneously defined by \theta. $\pi_{\theta}$ represents the policy learned for instance defined by $\theta$. In the below everywhere $\pi ==\pi_{\theta}$. I need to update it. In fact more accurately it must be $\pi_{\theta,k}$ since the learned policy differs every episode.} 

\begin{align}
    R_{\theta,k} &= V^{\pi^k_\theta}(\tb{s}_1) - V^*(\tb{s}_1) \label{regret}
    \\
    &=  V^{\pi^k_\theta}(\tb{s}_1) - \mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] + \mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) 
    \\ 
    &= \mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^{\pi^k_\theta}(\tb{s}_2)]\}  
    \\ 
    & \quad -\mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^*(\tb{s}_2)] \} + \mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim\ \pi^k_\theta(\tb{s}_1), \tb{s}_2 \sim\ \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^k_\theta}(\tb{s}_2) - V^*(\tb{s}_2)] + \mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \label{eq_Q_V}
\end{align} \\
In the above we see a recursive relation in the first term but it its unclear how to deal with the second term.

\pt{Suggestion -- for each equation write the proper reason why it is true. This will make it easy to follow. For example, in above the second equation you added and subtracted $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] $.}
\textcolor{red}{Ok, I'll do it after I start revisiting them. Apart from adding and subtracting Q, I've only expanded the Bellman Equation}

\textcolor{red}{I'm stuck here to find a closed form expression of $Q^*(.,.)$ and $V^*$ due to exponential number of states}

\subsection{\label{q_v}\textit{Dealing with Q-V difference in} \ref{eq_Q_V}}
\subsubsection{}
\begin{align} 
    & \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q^{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ c(\tb{s}_1,\tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)] \} - V^{\pi^*}(\tb{s}_1) \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim   \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - V^{\pi^*}(\tb{s}_1) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - (1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)]) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{  \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)] \}
    \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} \{ \sum_{\tb{s} \in \mathcal{S}} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*)) V^{\pi^*}(\tb{s})\} \label{sum of difference of probabilities into V*}
\end{align}

\\
The above just follows from writing the definition of optimum Action value function and doing some rearrangement and remember costs throughout is 1.
\\
\subsubsection{}
In the below proof, we expand the difference in probability term arising in the above equation \ref{sum of difference of probabilities into V*}. The initial global state, $\tb{s}_1$, is with all agents at $\s_{init}$ and the next state, $\tb{s}$, is one where agents in $ \mathcal{I}:=\{i_1,i_2,..,i_r\}$ remain at $s_{init}$ while those in $\mathcal{J}:=\{j_1,j_2,..,j_{n-r}\}$ go to goal node. \\


\begin{lalign}
\mathbb{P}(s|s_1, a_1) - \mathbb{P}(s|s_1, a_1^*)  \label{prob_diff_init}
\\
&= \langle \phi(s|s_1,a_1), \theta \rangle - \langle \phi(s_1|s_1,a_1^*), \theta \rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1), \phi(s_2^{\prime}|s_2, a_2)..., \phi(s_n^{\prime}|s_n,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\& - \langle (\phi(s_1^{\prime}|s_1, a_1^*), \phi(s_2^{\prime}|s_2, a_2^*)..., \phi(s_n^{\prime}|s_n,a_n^*)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1),..., \phi(s_n^{\prime}|s_n,a_n)) - (\phi(s_1^{\prime}|s_1, a_1^*),..., \phi(s_n^{\prime}|s_n,a_n^*)), \\
& (\theta_1, 1,...,\theta_n,1)\rangle 
\\
&= \sum_{m = 1}^{r} \langle \phi(s_{i_m}^{\prime}|s_{i_m},a_{i_m}) - \phi(s_{i_m}^{\prime}|s_{i_m},a^*_{i_m}), (\theta_{i_m}, 1)\rangle \\ 
& + \sum_{m = 1}^{n-r} \langle \phi(s_{j_m}^{\prime}|s_{j_m},a_{j_m}) - \phi(s_{j_m}^{\prime}|s_{j_m},a^*_{j_m}), (\theta_{j_m}, 1)\rangle 
\\
&= \sum_{m=1}^{r} \langle (-a_{i_m} + a^*_{i_m}, 0), (\theta_{i_m}, 1) \rangle + \sum_{m=1}^{n-r} \langle (a_{j_m}-a^*_{j_m}, 0), (\theta_{j_m}, 1) \rangle   
\\
&= \sum_{m=1}^{r} (\langle a^*_{i_m}-a_{i_m}, \theta_{i_m} \rangle)  + \sum_{m=1}^{n-r} (\langle a_{j_m}-a^*_{j_m}, \theta_{j_m}  \rangle)  
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1} (a^*_{i_m, p} - a_{i_m, p})\theta_{i_m, p} \} + \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1} (a_{j_m, p} - a^*_{j_m, p})\theta_{j_m, p} \}
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\} \}  - \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \}
\\
&= \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\}
\end{lalign}
\\
\\
The initial few lines use the linearity assumption and properties of inner product. Then, split the sum on $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Next lines use definition of $\phi(.,.)$ and $a^*$ as the one matching all signs with $\theta$. We prove this is $a^*$ in all in one theorem \ref{all_in_one}. 
\\

\\


\subsection{\textit{Some Expressions for Transition Probabilities}}
\subsubsection{ \label{stay_at_init} \textit{$\mathbb{P}(\tb{s}|\tb{s},\tb{a})$ where $\tb{s} = (s_{init}, s_{init},\dots,s_{init})$}}

\text{At the global initial state, probability that after taking a global action $\tb{a}$, the next global state is still the same as before i.e., $\tb{s}$}
\begin{lalign}
\mathbb{P}(\tb{s}|\tb{s}, \tb{a})
\\ Linearity Assumption\\
&= \langle \phi(\tb{s}|\tb{s},\tb{a}), \boldsymbol{\theta} \rangle
\\
$Expanded form of features$
\\
&= \langle (\phi(s|s, a_1), \phi(s|s, a_2)..., \phi(s|s,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\
$Definition of Inner Product$
\\
&= \sum_{i = 1}^{n} \langle (\phi(s|s, a_i),(\theta_i,1))
\\
$Definition of Features$
\\
&= \sum_{i = 1}^{n} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}),(\theta_i,1) \rangle
\\
&= \sum_{i = 1}^{n} \{ \langle -a_i, \theta_i \rangle + \frac{1-\delta}{n.2^{n-1}} \}
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \langle a_i, \theta_i \rangle 
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} a_{i,p}. \theta_{i,p} 
\\ $Definition of action and theta$\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Taking summation over p inside$ \\
&=  \frac{1-\delta}{2^{n-1}} - 
 \frac{\Delta}{n(d-1)} \sum_{i = 1}^{n}   \Big\{ d-1 - 2 \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Just simplify$ 
\\
&=  \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
\end{lalign}

\subsubsection{\textit{ $\mathbb{P}(s'|s,a)$ where $s = \tb{s}_{init}$ and $s':$ arbitrary state}}
\\
In this subsection we derive the expression of probability that if at state $\tb{s} = \{s_{init}, s_{init}, \dots, s_{init}\}$, if global action $\tb{a} = (a_1,a_2,\dots, a_n)$ is taken, you reach $\tb{s}^{\prime}$ where the agents at indices in $\mathcal{I}:= \{ i_1,i_2,\dots, i_r\}$ stay in the same state while agents at indices in $\mathcal{J} := \{j_1,j_2,\dots,j_{n-r} \}$ move to goal state i.e., $s'_{i_1}=s'_{i_2}=\dots=s'_{i_r}=s_{init}$ and $s'_{j_1}=s'_{j_2}=\dots=s'_{j_{n-r}}=goal$. \\
$P(\tb{s}'|\tb{s},\tb{a}) \\ 
= \langle \phi(\tb{s}'|\tb{s},\tb{a}), \theta \rangle \\
= \langle \phi((s'_1,s'_2,\dots, s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n)), (\theta_1, 1, \theta_2, 1,\dots, \theta_n,1) \rangle \\
= \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)),(\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle \phi(s'_i|s_i,a_i), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(s'_j|s_j,a_j), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle (a_j, \frac{\delta}{n.2^{n-1}}), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \Big \{  \frac{1-\delta}{n.2^{n-1}} + \langle -a_i,\theta_i \rangle \Big \} + \sum_{j \in \mathcal{J}} \Big \{ \frac{\delta}{n.2^{n-1}} + \langle a_j, \theta_j \rangle \Big \} \\
= r. \frac{1-\delta}{n.2^{n-1}} - \sum_{i \in \mathcal{I}}    \langle a_i,\theta_i \rangle  + (n-r). \frac{\delta}{n.2^{n-1}} +  \sum_{j \in \mathcal{J}}  \langle a_j, \theta_j \rangle  \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}} -  \sum_{i \in \mathcal{I}} \{ \sum_{p = 1}^{d-1} a_{i,p}.\theta_{i,p} \} + \sum_{j \in \mathcal{J}} \{ \sum_{p = 1}^{d-1} a_{j,p}.\theta_{j,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \{
\sum_{j \in \mathcal{J}}   a_{j,p}.\theta_{j,p}  -  \sum_{i \in \mathcal{I}}  a_{i,p}.\theta_{i,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \Big \{
\sum_{j \in \mathcal{J}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{j,p}) = sgn(\theta_{j,p})\} - \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{
\sum_{j \in \mathcal{J}}  \Big[ 1 - 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}}  \Big[   1 - 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{  \Big[ n-r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] - \Big[  r - \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
\sum_{p = 1}^{d-1}  \Big \{  n-2r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
  \Big \{  (d-1)(n-2r) - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\frac{\Delta . (n-2r)}{n} +\frac{2 \Delta}{n(d-1)} . 
  \Big \{  \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}     \Big \} \\
$ 
\\
Initial few lines follow by linearity assumption, definition of features and splitting the dot product over $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Next few lines simplify the dot product and rearrange terms. Then we use definition of action and theta. The remaining lines simplify the summations and rearrange the terms.
\\
From the above expression, we can observe that this probability in general can vary,  for different states $s' \in \mathcal{S}_{n,r'}$ for any $r' \in [n]$  under given global action  $a = \{a_1,a_2,\dots,a_n\}$ taken at $s = \{s_{init}, s_{init},\dots, s_{init}\}$.  Also observe that when $a=a^*$ this becomes independent of $s'$ for any given $r'$. \\


A more general result of the above relates to transition probability from some $s \in \mathcal{S}_{n,r}$ to some $s' \in \mathcal{S}_{n,r'}(s)$ where $\mathcal{S}_{n,r'}(s)$ represents the possible states of type $r'$ reachable from $s$ i.e.   $0 \leq r' \leq r \leq n$. We discuss this below. \\ 

\subsubsection{\textit{Most General transition probability}}

\textcolor{blue}{below $\mathcal{I}, \mathcal{J} = \mathcal{I}^\prime$ and $\mathcal{T} \cup \mathcal{T}^\prime = [n]$}


\textcolor{blue}{these sets of agents are different from the sets of agents above and is general; general in terms of initial state $s_{init}$ }

Suppose $s$ is such that agents at index in $\mathcal{I}:= \{i_1,i_2,\dots, i_r\}$ are at $s_{init}$ and those at $\mathcal{J} := \{j_1,j_2,\dots, j_{n-r}\}$ are already at goal. Let agents in $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ be the ones transiting from $s_{init}$ to $goal$ i.e., $s \in \mathcal{S}_{n,r}$ and $s' \in \mathcal{S}_{n,r'}$ where $n \geq r \geq r' \geq 0$ and $n \geq 1$. \\ \\
$P(s'|s,a)  \\= \langle \phi(s'|s,a), \theta \rangle  \\= \langle \phi((s'_1,s'_2,\dots,s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n) ), (\theta_1,1,\theta_2,1,\dots,\theta_n,1)\rangle  \\ = \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots, \theta_n,1) \rangle  \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle \phi(s|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle \phi(g|s,a_t), (\theta_t,1) \rangle \\ 
= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle (-a_i, \frac{1-\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle (a_t, \frac{\delta}{n.2^{r-1}}), (\theta_t,1) \rangle \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \{ \frac{1-\delta}{n.2^{r-1}} + \langle -a_i, \theta_i \rangle \} + \sum_{j \in \mathcal{J}}   \frac{1}{n.2^{r}}  + \sum_{t \in \mathcal{T}} \{ \langle a_t,\theta_t  \rangle + \frac{\delta}{n.2^{r-1}} \}   \\=  r'. \frac{1-\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}  + (r-r'). \frac{\delta}{n.2^{r-1}} + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}   + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} a_{i,p}. \theta_{i,p}      + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   a_{t,p} .\theta_{t,p}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} -  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{t,p}) = sgn(\theta_{t,p})\} -  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}}  \frac{\Delta}{n(d-1)} \Big \{  d-1 -  2 \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}}    \frac{\Delta}{n(d-1)} \Big \{  d-1 - 2\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} -   \frac{\Delta}{n(d-1)} \Big \{  r'(d-1) -  2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     +    \frac{\Delta}{n(d-1)} \Big \{  (r-r').(d-1) - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n(d-1)} \Big \{  (r-2r').(d-1) + 2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\ $

So, we have 
\begin{multline}
\mathbb{P}(s^\prime | s, a) 
=  \\ \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') + \\ \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}   \label{general_prob}
\end{multline}
    


\pt{this incorporates the new features. Also, this will be the optimal probability when the sign matching property holds.}

\textcolor{blue}{we can avoid `line break' commands above } \textcolor{red}{ok, removed them but now proof may seem clumsier}  \textcolor{blue}{ok, we will see a way out, perhaps, we will introduce them}



\textcolor{blue}{we should use available  macros for lemma, proof, etc. see the style file.} 

\textcolor{blue}{these help where the proof starts and importantly ends -- Paul Halmos tomb-stone mark}
\textcolor{red}{ok, this is new for me. i'll try to learn this.}


Initial lines use linearity assumption, definition of features and decomposing the inner product over agents who remain put at $s_{init}$, transit to goal and remain put at goal. In the next few lines, we expand the inner product terms and summations, use the definition of actions and theta and rearrange. Then, just rearrange different terms.  The indicators make sure appropriate sign is given to the dot product depending on signs of components of action and that of theta. \textcolor{blue}{we will cite some papers about these signs }. 

\textcolor{blue}{this is helpful to the reader}

\textcolor{blue}{let's write the role of indicator function above} \textcolor{red}{role as in?}


\\
\\
Notice that for a given global action, the  transition probability from a given $s \in \mathcal{S}_{n,r}$ to a $s' \in \mathcal{S}_{n,r'}$ as long as the transition is possible (i.e., $s' \in \mathcal{S}_{n,r'}(s)$)  depends on the particular $s'$ and is not independent of it even for given global action $a$ in general. Particularly one can observe that when $a=a^*$(one that matches signs with each component of $\theta$), this is independent of which $s'$ is being considered for a given $r'$. 



Another important probability is that of transition to global goal state after taking a global action a in any state $s \in \mathcal{S}_{n,r}$. This is corollory to \ref{general_prob}. \\  \\

 $ P(s'=(g,g,\dots,g)|s,a) \\ = \langle \phi(s' = (g,g,\dots, g)|(s,a)), \theta \rangle \\ = \langle (\phi(g|s_1,a_1), \phi(g|s_2,a_2),\dots, \phi(g|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle \phi(g|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle (a_i, \frac{\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j,1) \rangle \\ = \frac{r\delta}{n2^{r-1}} + \sum_{i \in \mathcal{I}} \langle a_i,\theta_i \rangle + \frac{n-r}{n2^{r}} \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  a_{i,p} \theta_{i,p} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}}  \frac{\Delta}{n(d-1)} \Big\{ d-1 - 2  \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
  \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  +  \frac{r \Delta}{n} - \frac{2 \Delta}{n(d-1)} \sum_{i \in \mathcal{I}}    \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
 $
\\
\\
This is very similar to above proofs and no new idea is used, only the state is explicitly mentioned.
\\

\textcolor{blue}{write this as another lemma} \textcolor{red}{i had written this before writing the above general proof which is now a lemma. this one is specific for r=n and r'=0 which game me an idea of how to express for general case. should this be a lemma or corollary } \textcolor{blue}{yes, as said over phone. }


%\textcolor{blue}{ think it is $\newtheorem{lemma}{command for new lemma}$}

\subsection{$V^*$ for multiple cases (This hasn't led to any key result by itself yet)}


General formula:  \textcolor{blue}{is this a theorem?} \textcolor{red}{It follows directly from Bellman equation}\\
 $V^*(s) = \{1  + |\mathcal{S}_{n,r-1}(s)| p_{a^*,r-1} V^*_{r-1} +  |\mathcal{S}_{n,r-2}(s)|p_{a^*,r-2} V^*_{r-2} + \dots + |\mathcal{S}_{n,2}(s)| p_{a^*,2} V^*_{2} + |\mathcal{S}_{n,1}(s)| p_{a^*,1} V^*_{1} \} . \{ 1 - P(s|s,a^*) \}^{-1}$

 \\ \\
 Below $p^*_{r,r'}$ denotes transition probability for a valid transition from state of type $r$ to that of type $r'$ under optimal global action in the respective instance specicified by $\theta$ and $n$ and $V^*_0 = 0$ \\ \\
For n = 1 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$ \\ \\ 
For n = 2 \\
For r = 1 \\ 
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For n = 3 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
\\

For n=4 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\

For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
For r = 4 \\
$V^*_4 = 1 + p^*_{4,4}V^*_4 + \binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1+\binom{4}{4}p^*_{4,0}V^*_0 = \frac{1+\binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1}{1-p^*_{4,4}} = \frac{1+\binom{4}{1}p^*_{4,3}\frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} + \binom{4}{2}p^*_{4,2}\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{4}{3}p^*_{4,1}\frac{1}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+\frac{ \binom{4}{1}p^*_{4,3} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} +\frac{ \binom{4}{2}p^*_{4,2}+\frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}}  = \frac{1+ \frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+ \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}}+\frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  }{1-p^*_{4,4}}$


\pt{can you see the closed form expression here?} \textcolor{red}{i can see a pattern but can't express it nicely.}

\pt{if not, can you confirm whether this notation is correct? -- $p^*_{r,r'}$ is the probability that number agent in the state $s$ were $r$, and the number of agents in $s'$ are $r'$?} \textcolor{red}{yes, line 308-309}

\pt{also can you recall me here -- what does the  $\binom{4}{2}$ or $\binom{3}{1}$ represent in terms of $r,n,$ and $r'$? $\binom{r}{r-r'}$} \textcolor{red}{yes,in the first factor of every term in the numerator}

\pt{I will try to get the closed form expression once you mention this.} \textcolor{red}{if you can get this it will be good to add}


\pt{Also can you summarize what are the intermediate results we have. summarize all of them no matter how  trivial or useful they are are. } \textcolor{red}{The general probability expression , The all in one result: $a^*$ is same for all states and is the one matching signs with each component of $\theta$, $V^*$ is same for all states of a particular type, $V^*$ are ordered and (due to) the claim on probabilities hold}

\pt{I can see  that you have many intermediate results.}












\textcolor{blue}{let's write here the  intermediate steps with pending proofs }
\textcolor{red}{done as of now, thought there's a pattern, to express it mathematically is a bit challenging, i'll try to think about this}

\subsection{NOT DIRECTLY USEFUL FOR US: Important result regarding monotonicity of V*, an independent result , and a result with weaker sufficient is stated and used below} \\

Consider the states space, $\mathcal{S} = \{s_1,s_2,\dots,s_n\} \cup \{x,y\} $. Let under some global action, the following markov chain be induced:
\\ Cost for any transition is constant and equal to 1. Transition probability from x to $s_i$ is represented as $p_{x,i}$ and from y to $s_i$ as $p_{y,i}$ for $i \in \{1,2,\dots,n\}$ and $p_{x,x}$ and $p_{y,x}$ represent the same from x and y respectively to x. Probability from y to y is represented as $p_{y,y}$. All probabilities are considered between 0 and 1 (strictly). Further, it holds that $p_{y,s} = p_{x,s} - \delta_s$ for every $s\in \{x,1,2,\dots,n\}$ where all $\delta_s \in (0, p_{x,s})$. (We would later require that assuming $p_{x,(.)}$ is monotonic, $\delta_s$'s are such that they preserve the monotonicity of $p_{y,(.)}$. But this assumption on $\delta_s$'s is not required in this discussion.) No other transitions are possible. For the sake of discussion, we assume that the states $s_1,s_2,\dots,s_{n}$ are absorbing states (potentially there may be all kinds of transitions from there but the long term value is known hence they can be considered terminal states with these values) with value function known respectively as $V_1,V_2,\dots,V_n$ while value of state $x$ is also known as $V_x$. Assume the following condition holds for the values: $V_1<V_2<\dots<V_n < V_x$. We want to relate $V_x$ and $V_y$. \\ \\
\tb{Claim:} $V_x < V_y$ \\ \\
$p_{y,y} = 1-p_{y,x}-\sum_{i=1}^{n}p_{y,i} = 1-(p_{x,x} - \delta_x) - \sum_{i=1}^n(p_{x,i}-\delta_i) = \delta_x + \sum_{i=1}^n \delta_i$ \\ \\
$V_x = \sum_{i=1}^np_{x,i}(1+V_i)+p_{x,x}(1+V_x)$ \\ \\
Similarly, \\
$V_y = \sum_{i=1}^np_{y,i}(1+V_i) + p_{y,x}(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^n(p_{x,i}-\delta_i)(1+V_i) + (p_{x,x}-\delta_x)(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^np_{x,i}(1+V_i) + p_{x,x}(1+V_x)-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_i)\} + p_{y,y}(1+V_y) $ \\ \\
From the definition of $V_x$ above and monotonicity of V's, we have : \\
$V_y > V_x-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_x)\} + p_{y,y}V_y = V_x-p_{y,y}(1+V_x) + p_{y,y}(1+V_y) \\ \implies V_y - V_x > p_{y,y}(V_y -V_x) \\ \implies (1-p_{y,y}) (V_y - V_x) > 0 \\ \implies V_y>V_x $

 \\ 


\subsection{ \label{all_in_one} \textit{ALL IN ONE THEOREM} - $a^*$ is the one that matches sign with $\theta$ for every state, $V^*$ is same for states of a particular type, there exists ordering of $V^*$'s : all go hand-in-hand \textcolor{blue}{lines after \ref{regret} are basic and hence need to be cross-checked}} 
\tb{Base Case}  \\ By definition, $V^*_0 = 0$. \\
Take any $s \in \mathcal{S}_{n,1}$. \\
\tb{Q.} What is $a^*$? \\
For s, only possible next global states are s itself and all-at-goal (g). This is akin to the single agent problem. But any transition probability also depends on actions of others. \\
Suppose $p^a_{s,g}$ denotes the transition probability from s to g. Then we have, \\
$V^a_1(s) = (1-p^a_{s,g}).(1+V^a_1(s)) + p^a_{s,g}.(1+V_0) \implies V^a_1(s) = \frac{1}{p^a_{s,g}}$ \\
Thus the optimum action at s is the one that minimizes $V^a_1(s)$ i.e., maximizes $p^a_{s,g}$. From the above general equation \ref{general_prob}, the transition probability is maximum when $a$ is such that it matches all signs with $\theta$ for the respective components of agent who was initially at s. The signs of other components do not matter. Hence there could be multiple $a^*(s)$ for any particular $s \in \mathcal{S}_{n,1}$.\\
Notice that this will hold true for any $s \in \mathcal{S}_{n,1}$. Note that particular $a^*$ whose sign matches with components of $\theta$ (for every agent), is common for possible $a^*$ for every $s \in \mathcal{S}_{n,1}$. We consider this $a^*$ in particular. \\
Since from the general formula \ref{general_prob}, for a fixed instance ($\theta$), for given action $a^*$ the probability only depends on r and r', it is the same for all states s $\in \mathcal{S}_{n,1}$ i.e., $p^{a^*}_{s,g} = p^{a^*} \forall s \in \mathcal{S}_{n,1}$. This $V^*_1(s) = V^*_1 \forall s \in \mathcal{S}_{n,1}$ \\
Since transition probability for this action is strictly between 0 and 1, $V^*_1 > V^*_0=0$ \\
\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:\\ $a^*$ is the one that matches sign with $\theta$ for any state in $\mathcal{S}_{n,k}$, hence from \ref{general_prob} and definition of $a^*$, $p^*(s \in \mathcal{S}_{n,k}  \xrightarrow{}s' \in \mathcal{S}_{n,k'}(s)) = p^*_{k,k'}$, $V^*_k(s)=V^*_k$ for any $s \in \mathcal{S}_{n,k}$ and $V^*_k>V^*_{k-1}$. Now, we need to show the same for $r+1$. \\
Consider any $s \in S_{n,r+1}$. \\
$V^a(s) = \sum_{s' \in \mathcal{S}(s)\textbackslash \{s,g\}} P(s'|s,a)\{1+V^*(s')\} + P(s|s,a).\{1+V^a(s)\} + P(g|s,a).\{1+V^*(g)\}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +\sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} p^a_{r+1,r'}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \sum_{i \in [n]} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r'}  - \binom{r}{r'-1} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Big  \}$ \\ 
Observe that the third term is always non negative since when $r'>(r+1)/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} >V^*_{r+1-r'}$ while for $r' \leq (r+1)/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_{r+1-r'}$. Note that the above arguments is for $r' \in [r]$. To minimize $V^a(s)$, we need to minimize $P(s|s,a)$ as well (check after rearrangement as it will appear in denominator as 1-P). Clearly, the action that matches sign with all components of $\theta$ minimizes $V^a(s)$ since it makes sure that the non-negative additive terms are all zero as well as P(s|s,a) is minimised. Hence this is $a^*$. Notice the above arguement holds for any $ s \in \mathcal{S}_{n,r+1}$. Hence $a^*$ is the same for each of them. Hence $p^*(s \in \mathcal{S}_{n,r+1} \xrightarrow{}s' \in \mathcal{S}_{n,r'}(s)) = p^*_{r+1,r'}$. Hence $V^*(s) = V^*_{r+1}$ for each of them. \\

\\ \\
Proving $V^*_{r+1} > V^*_r$ is tricky. We will make a suitable assumption on probabilities and later show that it holds under suitable choices of $\delta$ and $\Delta$. \\
\tb{Claim} If for every $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.  \\
We will justify that the assumption on probabilities in this claim holds for our features under suitable $\delta$ and $\Delta$. For now lets assume this holds for our case and prove the implication part of claim. \\
Return to the induction argument. \\
$V^*_r = 1+\sum_{r' \in \{0,1,\dots,r\}}\binom{r}{r'}V^*_{r'}$ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'}$ \\
Suppose for every $r' \in \{0,1,2,\dots,\lfloor\frac{r+1}{2}\rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}-\delta_{r'} $ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor\ +1 , \lfloor\frac{r+1}{2}\rfloor+2,\dots,r-1,r\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}+\delta_{r'} $ where $\delta_{r'}>0$ for every $r' \in \{0,1,\dots,r\}$\\ 
Note that, $\sum_{r' \in \{ 0,1,\dots,r,r+1\}} \binom{r+1}{r'}p^*_{r+1,r'} = 1 \\ \Leftrightarrow\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r+1}{r'}p^*_{r+1,r'} + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r+1}{r'}p^*_{r+1,r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \Leftrightarrow \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} (\binom{r}{r'}p^*_{r,r'}-\delta_{r'}) + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} (\binom{r}{r'}p^*_{r,r'} + \delta_{r'}) + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \Leftrightarrow \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r}{r'}p^*_{r,r'}-\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \Leftrightarrow p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + 1 -  \sum_{r' \in \{0,1,\dots,r-1,r\}} \binom{r}{r'}p^*_{r,r'} \\ \Leftrightarrow p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} $ \\ \\
Now, going back to $V^*_{r+1}:$ \\ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}(\binom{r}{r'}p^*_{r,r'} - \delta_{r'})V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}(\binom{r}{r'}p^*_{r,r'}+\delta_{r'})V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} V^*_{r'}+ \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, r-1,r\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\=  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ > p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{\lfloor \frac{r+1}{2} \rfloor + 1}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  (  \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} - \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}  )V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ >  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r $ \\ 
Thus,\\
$V^*_{r+1} >   p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r \Leftrightarrow (1-p^*_{r+1,r+1})(V^*_{r+1}-V^*_r)>0 \Leftrightarrow V^*_{r+1} > V^*_r$ \\
Above inequalities used monotonicity of $V^*$ due to induction assumption. \\
Below we justify that the assumption in the above claim holds for our case( \ref{sufficiency} combined with \ref{justification}).

\subsection{ \label{sufficiency}\textit{Sufficient conditions on $\delta$ and $\Delta$ for well defined probabilities}; \textcolor{blue}{$\delta$ is conflicting with high probability $\delta$}}

$p^a_{r,r'} < 1$ for every $r \in \{1,2,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$for every $a$ and instance $\theta$. \\
From general probability formula \ref{general_prob}:
\\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\ \leq    \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{1} \\ \leq   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{\frac{n-r}{2}}{n2^{r-1}}        +    3\Delta \\ =  \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} +    3\Delta \\ =  \frac{(r'-0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} +    3\Delta \\ \leq  \frac{0.5n(2-2\delta)}{n.2^{r-1}} + 3\Delta \\ \leq  1-\delta + 3\Delta$ \\
To ensure $p^a_{r,r'}<1$ it is sufficient to ensure $1-\delta + 3\Delta<1 \Leftrightarrow \delta > 3\Delta$ \\
Similarly, we must ensure, $p^a_{r,r'} > 0$ for every $r \in \{0,1,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$. \\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \\  \geq  \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') -  \frac{2 \Delta}{1}  \\ \geq  \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} - 3\Delta \\ =  \frac{(r' -0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta \\ \geq  \frac{( -0.5n)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta = \frac{ \delta }{2^{r-1}} - 3\Delta$ \\
To ensure, $p^a_{r,r'} > 0$ it is sufficient to ensure $ \frac{ \delta }{2^{r-1}} - 3\Delta > 0  \Leftrightarrow \delta > 3.2^{n-1}.\Delta$. \\ Observe that since $n \geq1$, condition from $p>0 \implies $ condition from $p<1$  Also note that in the above, we have assumed $\delta < 0.5$. Hence we can fix any $\delta, \Delta $ and $n$ that satisy the above conditions in order to fix a class of instance as above.




\subsection{ \label{justification} \textit{Justification of assumption in the claim}} 
Recall that in the above claim, we assumed that: for every $r \in [n-1],$ for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$. \\
Below, we will derive sufficient conditions on $\delta$ and $\Delta$ such that this assumption holds. \\
Also note that from above section \ref{sufficiency} we have $\delta<0.5$ and $\delta>3.2^{n-1}\Delta$ so that all probabilities are well defined.
\\ \\
\tb{For $r'\leq \lfloor\frac{r+1}{2}\rfloor$}, \\
$\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \frac{r+1}{r+1-r'}p^*_{r+1,r'}<p^*_{r,r'} \Leftrightarrow \\(r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \\ \Leftrightarrow  (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \\ \impliedby (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \impliedby \frac{\Delta}{n}\frac{r^2}{8} + (r+1) \frac{\Delta}{n}<(r+1)\frac{1-2\delta}{n2^{r+1}} \Leftrightarrow\frac{\Delta}{n}(\frac{r^2}{8}+r+1)<(r+1)\frac{1-2\delta}{n2^{r+1}} \impliedby \Delta (\frac{n^2}{8}+n+1)<\frac{1-2\delta}{2^{n}} \Leftrightarrow \Delta < \frac{1-2\delta}{2^{n}(1+n+\frac{n^2}{8})} \impliedby \Delta < \frac{1-2\delta}{2^{n}(1+n+n^2)}$  \\ \\
Similarly, \\ \tb{For $r' > \lfloor \frac{r+1}{2} \rfloor$}, \\ 
$\binom{r+1}{r'}p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \\ \frac{r+1}{r+1-r'}p^*_{r+1,r'}>p^*_{r,r'} \Leftrightarrow \\ (r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow \\ (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \Leftrightarrow \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow  \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0  \impliedby  (\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0 \\ \Leftrightarrow \frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2) - 0.5(r+1)(\frac{1-2\delta}{n.2^{r}}) >0 \\ \Leftrightarrow \frac{(r'-r-0.5)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2)  >0 \impliedby \frac{(-r-0.5)(1-2\delta)+0.5n }{n.2^{r}}   >   \frac{\Delta}{n}  (r^2-r-1)  \Leftrightarrow \frac{(-r-0.5)(1-2\delta)+0.5n }{1}   >   \frac{\Delta}{1}  (r^2-r-1)  (2^{r}) \\ \impliedby (-n-0.5)(1-2\delta)+0.5n    >   \Delta  (n^2-n-1)  (2^{n})$ and $ (-n-0.5)(1-2\delta)+0.5n    > 0 \\ \impliedby 0.5n-n+2n\delta-0.5+\delta>0$ and $ 0.5n-n+2n\delta-0.5+\delta >   \Delta  (n^2+n+1)  (2^{n}) \\ \impliedby (2\delta-0.5)n>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2+n+1)  (2^{n}) \\ \impliedby 2\delta-0.5>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2+n+1)  (2^{n}) \\ \Longleftrightarrow \delta>\frac{1}{3}$ and $n > \frac{0.5-\delta}{2\delta-0.5}+ \frac{\Delta  (n^2+n+1)  (2^{n})}{2\delta-0.5} \\ \impliedby \delta>1/3 $ and $\Delta  (n^2+n+1)  (2^{n})<3\delta-1 \impliedby \Delta < \frac{3\delta-1}{(n^2+n+1).2^{n}}$ \\ 
\\
Finally we obtain (from current subsection and \ref{sufficiency}), for the desired instance, fix $1/2>\delta>1/3$. Then, fix, $\Delta< 2^{-n}.min\{\frac{3\delta-1}{n^2+n+1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2}\}$ \\
\label{final_conds}


\subsection{\textit{Simplification of Q-V difference from above} \ref{eq_Q_V}\textcolor{blue}{this is advantage function, isn't?}} \textcolor{red}{yes, it's like expected value of the advantage function since there is expectation over $a_1$ according to the policy \\ also i've modified below for new features}
\\
\\
From \ref{q_v} we have the following. In the below, $s_t$ represent global state at time t (Note it's not individual state), $\textbf{s}_t$. Similarly $a_t$ is global action at t. In the below, we ignore writing $k$ and $\theta$ in $\pi^k_{\theta}$ and $V^*_{\theta}$ to avoid clutter as it is understood in the context:

\begin{lalign} 

$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^*(s_1,a_1)] - V^* \\
= \mathbb{E}_{a_1 \sim \pi(s_1)}[c(s_1, a_1) + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}V^*(s_2)] - V^*(s_1)  $ \\
Using Bellman Equation and cost is 1
\\ 
$=  \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{  1 + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}[V^*(s_2)] - V^*(s_1) \Big \}$
\\ Expand the Expectation $ \\
=   \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  P(s_1|s_1,a_1) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1) \Big \}
\\ $ Use expression of probability from above \ref{stay_at_init}$
 \\= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2)  - V^*(s_1) \Bigg \}
\\$ Rearranging the terms $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*(s_1) \Big\} 
\\ $ Notice from the general expression of probability from previous proof \ref{general_prob} $\\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - V^*(s_1) \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} 
\\$ Expand V*(s_1) $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 + P(s_1|s_1,a_1^*)  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - \Big\{ 1 +  P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1, a_1^*) V^*(s_2) \Big\} \Bigg \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p})\neq sgn(\theta_{i,p})\} V^*(s_1) \Big\} 
\\$   

Rearrange and combine  terms to have a  lower bound 

$ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $
\end{lalign}
\label{q_v_simp}

\\



\subsubsection{\textit{Dealing with the sum of Probability differences above}} 

Recall from earlier \ref{q_v_simp}, \\ 
$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)   
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \\
 \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 The first term is problematic and it is not clear how to deal with it. Let's investigate the summation inside the expectation of the first term: \\ 
 $\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2) \\ = \sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} [P(s'|s_1,a_1)-P(s'|s_1, a_1^*)] V^*(s') $ (Now, use results from above sections \ref{prob_diff_init}) \\
 = $\sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\} V^*_r $ \\
= $\frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{\sum_{s' \in \mathcal{S}_{n,r}} [\{   \sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p}) \}]  \Big\}   \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n}   
 \sum_{s' \in \mathcal{S}_{n,r}} [ \mathbbm{1}\{s'_i = s_{init}\}   \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   - \mathbbm{1}\{s'_i = goal\}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \}]  \Big\} \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  
 \sum_{s' \in \mathcal{S}_{n,r}} \mathbbm{1}\{s'_i = s_{init}\}     -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \sum_{s' \in \mathcal{S}_{n,r}} 
 \mathbbm{1}\{s'_i = goal\} \Big\}  \Big\} 
 \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \binom{n-1}{r-1}    -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \binom{n-1}{r} \Big\}  \Big\} \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \{ \binom{n-1}{r-1}    -   \binom{n-1}{r} \} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} V^*_r  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} + V^*_{n-r}  \frac{2(n-r)-n}{n} \binom{n}{n-r} \} \Big\}   \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} - V^*_{n-r}  \frac{2r-n}{n} \binom{n}{r} \} \Big\}  \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  - V^*_{n-r}   \} \frac{2r-n}{n} \binom{n}{r} \Big\} \geq 0. 
 $ \\
 \\
 Observe that when $r> n/2, V^*_r > V^*_{n-r}$ and vice-versa (refer result above) \\
 Hence we have established that, \\
 $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1) \geq \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \label{q_v_further_simp} \\ \\
 In the above we showed the inequality for $s_1=(s_{init},s_{init},\dots, s_{init})$. Using similar arguments same inequality can be shown to hold for any $s_1 \in \mathcal{S}$. We will use this general result below.

 \subsection{\textit{Back to Lower Bound Proof}}
 From earlier \ref{eq_Q_V}, expected regret in the $k-th$ episode: \\
$R_{\theta,k} \\ = V^{\pi_\theta}(s_1) - V^*(s_1) 
\\ 
 = \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)$ \\
\\ Using above result \ref{q_v_further_simp}, \\
 $R_{\theta,k} \\ \geq  \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_1 \neq goal \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 By recursion and the generalized result from the section above,
 we have: \\

 $R_{\theta,k} \\ \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{k} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_h \neq goal \} \mathbbm{1}\{sgn(a^h_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}  $ \\
 where, the Expectation is taken with respect to trajectory induced in the $k-th$ episode by the interaction of policy $\pi$ and transition kernel $P_{\theta}$. Now, the total expected regret over $K$ episodes is: \\
 $
 R_{\theta}(K) \\
 \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{t=1}^{\infty} \mathbb{E}_{\theta, \pi} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_t \neq goal \} \mathbbm{1}\{sgn(a^t_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
 $ \\
 Analogous to Min et al, Cohen et al, we define: \\
 $N = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} $ and for agent $i \in [n]$, $j \in [d-1]$,\\
$N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta_{i,j})\} $  \\
Thus, $R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]} \sum_{j=1}^{d-1} N_{i,j}(\theta) \}$ \\
To use the standard Pinsker's Inequality, we need $N_{i,j}(\theta)$ to be bounded almost surely which is known to not hold for SSPs (Min et al, Cohen et al). Hence, we use the capping trick introduced by Cohen et al and also used by Min et al. In this trick, we cap the learning process to a predetermined T. If the learning process (i.e. $K-th$ episode) ends before this, the agents continue to remain at $goal$. In this case the summation for the actual process and the capped process is the same. On the other hand when K episodes end beyond T, we have a truncated sum. Due to non-negativity of each part, the sum for the capped process lower bounds the actual sum. \\ Define \\ $N^- = \sum_{t=1}^T\mathbbm{1}\{s_t \neq goal\} $ and for any agent $i \in [n] $ and $ j \in [d-1],$\\ $N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta_{i,j})\} $ \\ 
It is easy to see that for any $i \in [n]$ and $j \in [d-1]$, $N^- =   N^-_{i,j}(\theta) + N^-_{i,j}(\theta^{j})  $ \\ where for every $\theta$, $\theta^j$ represents the vector that only differs at the $j-th$ index of every $\theta_i$ in $\theta = \{\theta_1,1,\theta_2,1,\dots,\theta_n,1\}$, where each $\theta_i \in \{\frac{-\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}\}^{d-1}$. \\  
Thus,  $R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}$n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}$.  Notice that $\theta \in \Theta \iff \theta^{j} \in \Theta$ (This follows from definition of $\Theta$ \textcolor{red}{without this, following equation won't hold}). Then, we have: \\
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \{ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \} \\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^- - N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^-] - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}

Generalisation of Lemma C2 in Cohen et al 2020: If $T \geq 2KB^*$, then $\mathbb{E}_{\theta}[N^-] \geq KB^*/4$  \\ Proof given below \ref{generalise_cohen}. We pick $T = 2KB_*$ \\
\textbf{Pinsker's Inequality(Min et al, Lemma E.3)} \pt{$TV(p,q) \leq \sqrt{KL(p,q)}$}

If $f:S^T\xrightarrow{}[0,D]$ then, 
$\mathbb{E}_{\mathcal{P}_1} (f(s)) - \mathbb{E}_{\mathcal{P}_2} (f(s))\leq D \sqrt{\frac{log(2)}{2}}. \sqrt{ KL(\mathcal{P}_2 || \mathcal{P}_1)}$  

\pt{Note that this will hold only if $|f(s)| \leq D \sqrt{\frac{log(2)}{2}}$?}
\textcolor{red}{I dont think so. $|f(.)|$ can be D}


\pt{don't use double back slash. These are not needed. just give one line spacing.}

Then, 
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  \mathbb{E}_{\theta, \pi}  [N^-] +  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] - \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] \} \Big \} \\ \geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{  \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] - \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] \} \Big \} \\ 
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
$

\textcolor{blue}{to update the above relations, equalities and inequalities } \textcolor{red}{done}
\\
\\
\\
 We have the following for our case (proof:\ref{simplify_kld}): \\
For appropriate $\delta$ and $\Delta$:
$ KL(\mathcal{P_{\theta}||\mathcal{P_{\theta^j}}}) \leq  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-] $
\\


$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta V_1^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{1/2} \sqrt{3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]}  \} \Big \} \\
= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{\mathbb{E}_{\theta}[N^-]} \Big \} \\
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{T} \Big \} \\
= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \} \\ 
$\\
Notice that the term in bracket is independent of $\theta, i$ or $j$. Thus, we have: \\
$\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq  \Delta V_1^* |\Theta| \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \} \\
\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq   V_1^*  \Big \{ \Delta  KV_1^*/4 -   (KV_1^*)^{3/2}  \frac{2^{n+2}.\Delta^2}{\sqrt{\delta} (d-1)} \Big \} \\ 
$ 
Specifically, pick, $\Delta^* = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}$. \\ At this value of delta,\\
$\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq V_1^* \{  \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}. \frac{KV_1^*}{4} - \frac{(KV_1^*)^{3/2}.2^{n+2}}{\sqrt{\delta}(d-1)}.  (\frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}})^2\} \\ 
= V_1^* \{\frac{(d-1) \sqrt{\delta.K.V_1^*}}{2^{n+7}} - \frac{(d-1)\sqrt{\delta.K.V_1^*}}{2^{n+8}}\}
\\
\geq  \frac{(d-1).\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+8}} \geq \frac{d.\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+9}} $ \\ \pt{This makes it independent of number of agents, a very strong result? Is this correct or do we need to incorporate the number of agents here.} \textcolor{red}{potentially the intermediate results I used directly without verifying depend on n. the term i argued to be $+ve$ and ignored in lower bound certainly depends on n but very difficult to simplify(needs closed form V*)} \\
\textcolor{red}{update : it depends on n}

Since the average over entire set is lower bounded by the RHS, there must exist some parameter in the set for which the RHS is a lower bound. Hence proved. \textcolor{blue}{ok we will discuss the proof}. \\ \\
It remains to show that the $\Delta$ picked above is valid. \\ Hence, need to ensure that $\Delta = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}} < 2^{-n}.min\{\frac{3\delta-1}{n^2+n+1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2}\}$  \\ or, $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.min^2\{\frac{3\delta-1}{n^2+n+1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2}\}} $
\\ \\
\textcolor{blue}{updated later} \textcolor{red}{Although it is independent of $n$, it can be interpreted as a strong result in the sense that no matter how many agents are deployed to learn, this minimum regret will always hold. The independence also comes from ignoring the positive terms} \\ \textcolor{red}{(whose proof is as of now still incomplete )}. \\ \textcolor{red}{since now there is a dependence on $n$, the above para is not valid} 

\textcolor{blue}{we need to write the  statement that is proved, and also delineate that statement from the proof -- use macros provided in the style file} \textcolor{red}{This is not complete yet. Only if we can find the corresponding lemmas I've mentioned in the proof, it will be complete possibly with very different expression.} \\
\\
\textcolor{blue}{2/4/25} \textcolor{red}{The proof is now complete! Now we have one complete result!}
\\ 
\\
\textcolor{red}{3/4/25} \\
\tb{Theorem}: For any MASSP learning algorithm $\mathfrak{A}$, there exists a linear-mixture MASSP instance defined by appropriate parameters ($n, \delta, \Delta, \theta$) for whom the expected cumulated regret matches the reported upper bound $\widetilde{O}(\sqrt{K})$. \\ Specifically, the instance satisfies: \\ $\mathbb{E}_{\theta,\mathfrak{A}}[R(K)] \geq \frac{d.\sqrt{\delta}\sqrt{K.V^*_1}}{2^{n+9}}$ \\
for $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.min^2\{\frac{3\delta-1}{n^2+n+1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2}\}} $

\subsection{ \label{generalise_cohen} \textit{Generalisation of Lemma C2 of Cohen et al for our case}-12/13-3-25}
\tb{Lemma:} For any deterministic learner, if $T\geq 2KV_1^*$, then, $\mathbb{E}[N_-]\geq KV^*_1/4$ \\ 

\textcolor{blue}{there is a relation between $B^\star$ and $V^\star_1$ and is given in the first half of this writeup }

\tb{Proof:} If capped process finishes before T, $N_-=N$. Else number of visits to goal state is less than $K$. \\Thus, $N_- \geq T-K$.\\ Thus, $\mathbb{E}[N_-] \geq \mathbb{E}[min\{T-K,N\}] \geq \mathbb{E}[\sum_{i=1}^Kmin\{T/K-1, N_k\}]$.\\
Since $T\geq2KV^*_1,$ and $V^*_1\geq1$ the lemma will hold for any policy (mapping of actions) if, $N_k \geq V^*_1$ with probability $\geq 1/4$ for any policy. Consider any policy. \\ We can lower bound the probability $\mathbb{P}[N_k \geq V^*_1]$ by the events that we transit to an $r=1$ state and stay there for next $\lceil V^*_r\rceil -1$ steps. \\Thus, \\
$\mathbb{P}[N_k \geq V^*_1] \\ = \mathbb{P}(s_2 \neq g|s_1=s_{init}).\mathbb{P}(s_3 \neq g|s_2).\mathbb{P}(s_4 \neq g|s_3)....\mathbb{P}(s_{\lceil V^*_1\rceil} \neq g|s_{\lceil V^*_1\rceil-1}) \\ = (1-p^{a(s_1)}_{n,0}).(1-p^{a(s_2)}_{s_2,0})...(1-p^{a(s_{\lceil V^*_1\rceil-1})}_{s_{\lceil V^*_1\rceil-1},0}) $ \\
For any state s, $1-p^{a(s)}_{n,0}$ is minimum when $p^{a(s)}_{n,0}$ is maximum. Check from line 1087 that this happens at $a^*$ which matches all signs with $\theta$. Further, $1-p^*_{s,0}$ when $s \neq g$ is minimum when $p^*_{s,0}$ is maximum at any $s \in \mathcal{S}_{n,1}$. Thus, we can lower bound the above product as: \\
$\mathbb{P}[N_k \geq V^*_1] \geq (1-p^*_{n,0}).(1-p^*_{s_2,0})...(1-p^*_{s_{\lceil V^*_1 \rceil -1},0}) \geq (1-p^*_{1,0})^{\lceil V^*_1 \rceil -1} \geq (1-p^*_{1,0})^{ V^*_1 -1} = (1-p^*_{1,0})^{ 1/{p^*_{1,0}} -1} \geq 1/e \geq 1/4$ \\
For the last second inequality, we use for $x\geq 1$, $(1-1/x)^{x-1}\geq 1/e$ \\
 Thus, $\mathbb{E}[N_-]  \geq \mathbb{E}[\sum_{i=1}^Kmin\{T/K-1, N_k\}] \geq KV^*_1/4$ \\


 
 \subsubsection{\textit{Alternate proof for dealing with $\mathbb{P}[N_k \geq V^*_1] \ge \frac{1}{4}}$ 13-3-25}
 
\textcolor{blue}{the result below a general one}
 
 Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](s)$ as the probability that starting at state $s \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in R^+$. Further, $\mathbb{P}[N_k \geq x] = \mathbb{P}[N_k \geq x](s_{init})$. \\
 \tb{Claim} Consider any $s \in S_{n,r}$ where $r \in [n]$. Then, for any policy it holds for our instances that $\mathbb{P}^{\pi}[N_k \geq x](s) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](s')$ for all $x \in R$ where $s' \in \mathcal{S}_{n,r'}(s)$ for any $r' \in \{0\} \cup [r]$ with equality holding only at $\pi = \pi^*$  and $r'=r $ i.e., $s'=s$ respectively. Here $\pi^*$ is the policy of taking action $a^*$(the one matching all signs with $\theta$) at every state $s \in \mathcal{S}$. The equality in the middle says that for any $s \in \mathcal{S}_{n,r}$ under $\pi^*$, $\mathbb{P}^{\pi^*}[N_k \geq V^*_1](s)$ happens to stay a constant independent of $s$ and only depends on $r$.\\
 Proof will be similar to $V^*$ proof \\
 Will work on this later if above proof is not satisfactory.\\
 \tb{Proof} We will prove this by induction. \\
 \tb{Base Case:} For r=1: 
 Consider any $s \in \mathcal{S}_{n,1}$ \\
 For any $x \in R^+$, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x\rceil-1}$ \\
 One can check from the general formula for transition probabilities that the above is uniquely minimum when $\pi(s) = a^*$. Hence equality only holds at $\pi=\pi^*$.  \\
 Hence, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x\rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x\rceil -1}$ \\
 Recall that for the same action $a^*$ at any $s \in \mathcal{S}_{n,1}$, $P(g|s,a^*)$ remains the same. Hence, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x \rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) $ \\
 The only two possibilities for $s'$ are $s$ itself and $g$. \\
 Clearly for $s$ the equality holds and for $g$, $\mathbb{P}^{\pi^*}[N_k \geq x](s'=g) = 0$ \\ Hence, \\
  $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x \rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s')  $
  \\ Finally we showed that for any $x \in R^+$ for any policy $\pi$, for any $s \in \mathcal{S}_{n,1}$ and $s' \in \cup_{r' \in \{0,1\}} \mathcal{S}_{n,r'}(s)$,  \\
  $\mathbb{P}^{\pi}[N_k \geq x](s)  \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s')  $ \\
  where in the first inequality, equality holds only when $\pi = \pi^*$, the middle equality means that the probability is same for all $s \in \mathcal{S}_{n,1}$ and in the last inequality, equality holds only when $s' = s$. \\
  \\
  \tb{Generalization:} Assume the above holds for m = 1, 2,...,r i.e., for all $m \in [r]$ it holds that for any $x \in R^+$ for any $s \in \mathcal{S}_{n,m}$, for any policy $\pi$, for our instances, it holds that, $\mathbb{P}^{\pi}[N_k \geq x](s) \geq \mathbb{P}^{\pi^*}[N_k \geq x](s)=\mathbb{P}^{\pi^*}[N_k \geq x](m)\geq \mathbb{P}^{\pi^*}[N_k \geq x](s')$ where $\pi^*$ is the policy taking action $a^*$(the one matching signs with all components of $\theta$) at all states and $s' \in \cup_{m' \in \{\{0\} \cup [m] \}}\mathcal{S}_{n,m'}(s)$. Further, in the first inequality, equality only holds when $\pi =\pi^*$ and the middle equality implies that the probability is same for all states $s \in \mathcal{S}_{n,m}$ and in the last inequality, the equality only holds when $s' =s$.  \\
  Assuming this we need to show that the same holds for any $s \in \mathcal{S}_{n,r+1}$ \\
  Again consider any $x \in R^+$. \\
  Consider any $s \in \mathcal{S}_{n,r+1}$. \\
  We have, \\
  $\mathbb{P}^{\pi}[N_k \geq x](s) = \sum_{r' \in \{0,[r+1]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)} P(s'|s,\pi(s)) . \mathbb{P}^{\pi}[N_k \geq x-1](s') \\= P(s|s,\pi(s)). \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)). \mathbb{P}^{\pi}[N_k \geq x-1](s')$ \\ 
   If $x \leq 1$, then trivially, for all $s \neq g$, for all policies, $\mathbb{P}[N_k \geq x] =1$. Otherwise, we have the following:
  \\
$\mathbb{P}^{\pi}[N_k \geq x](s) \\ =  P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s') \\ 
  \geq P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s))  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \Bigg\} \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Bigg \} + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)}  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  
  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0, [r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \sum_{i \in [n]}      \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{t \in \mathcal{T}\} . \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{i \in [n]}        \{ \binom{r}{r'-1} -  \binom{r}{r'} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}     
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0,[r]\}} \sum_{i \in [n]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} 
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in [r]} \sum_{i \in [n]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  \Big \} \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{ \{ \binom{r}{r-r'} -  \binom{r}{r+1-r'} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big \} \Bigg \}   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{ \{ \binom{r}{r'} -  \binom{r}{r'-1} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big \} \Bigg \} \\
 = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{ \Big \{ \binom{r}{r'-1} -  \binom{r}{r'} \Big \} \Big \{ \mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq V^*_1](r+1-r') \Big \}      \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}        \Bigg \}$ \\ \\
 Notice that for $r' < (r+1)/2$, the binomial difference $\binom{r}{r'-1} - \binom{r}{r'}<0$ as well as probability difference $\mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r') < 0$ hence the product is $>0$. Similar argument holds for $r'>(r+1)/2$. For $r' = (r+1)/2$ it will be 0. Overall we can observe that the only terms dependent on action have non-negative coefficients for the sign matching indicator. Hence this term will be minimum when $a = a^*$.  Thus, we have, \\
 $\mathbb{P}^{\pi}[N_k\geq x](s) \geq   P(s|s,\pi^*(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} $\\ Also, \\
 $\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $ \\

Subtracting the above two equations, 
\\
$\mathbb{P}^{\pi}[N_k\geq x](s) - \mathbb{P}^{\pi^*}[N_k\geq x](s) \\ \geq P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) - P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) \\ \geq P(s|s,\pi^*(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) - P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) \\ 
= P(s|s,\pi^*(s)) (\mathbb{P}^{\pi}[N_k \geq x-1](s) - \mathbb{P}^{\pi^*}[N_k \geq x-1](s))$ \\
By recursion,  \\
$\mathbb{P}^{\pi}[N_k\geq x](s) - \mathbb{P}^{\pi^*}[N_k\geq x](s) \\ \geq P(s|s,\pi^*(s))^{\lfloor x \rfloor} (\mathbb{P}^{\pi}[N_k \geq x-\lfloor x \rfloor](s) - \mathbb{P}^{\pi^*}[N_k \geq x-\lfloor x \rfloor](s)) = P(s|s,\pi^*(s))^{\lfloor x \rfloor} (1- 1) = 0$  \\
Thus, $\mathbb{P}^{\pi}[N_k\geq x](s) \geq \mathbb{P}^{\pi^*}[N_k\geq x](s)$ \\
Also note that for equality, it must hold for each above inequality. Effectively this will only happen at $\pi = \pi^*$ \\ 
Recall, for any $s \in \mathcal{S}_{n,r}$, \\
$\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $
 \\
From the probability expression one can verify that the term $P(s|s,\pi^*(s))$ only depends on $r$. The only term that may differ due to $s$ is $\mathbb{P}^{\pi^*}[N_k \geq x-1](s)$. \\We claim that this is same too. This can be dealt with by induction on x itself. \\
For base case, $m = x-\lfloor x \rfloor$, for any $s \in \mathcal{S}_{n,r}$, $\mathbb{P}^{\pi^*}[N_k \geq m](s)=1$ \\ Hence showed for base case. \\ Assuming true for $m = x - \lfloor x \rfloor,  x - \lfloor x \rfloor+1,  x - \lfloor x \rfloor+2, \dots,  x - \lfloor x \rfloor+p $, we need to show that it holds for $m =  x - \lfloor x \rfloor + p+1$ \\ We can write for any $s \in \mathcal{S}_{n,r}$ that: \\
$\mathbb{P}^{\pi^*}[N_k\geq m ](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq m-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq m-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $ \\ Here the RHS doesn't depend on which $s \in \mathcal{S}_{n,r}$ is being chosen. Thus shown for m. \\
 Thus back in expression for $\mathbb{P}^{\pi^*}[N_k \geq x](s)$, $\mathbb{P}^{\pi^*}[N_k \geq x-1](s)$ is not dependent on $s \in \mathcal{S}_{n,r}$. Hence $\mathbb{P}^{\pi^*}[N_k \geq x](s)$ is same for all $s \in \mathcal{S}_{n,r}$.  \\
 Finally we need to show that, $\mathbb{P}^{\pi^*}[N_k \geq x](s) \geq \mathbb{P}^{\pi^*}[N_k \geq x](s') \forall s' \in \cup_{r' \in \{0,[r]\}}\mathcal{S}_{n,r'}$ with equality only at $s' = s$. \\
 Recall again, for any $s \in \mathcal{S}_{n,r+1}$, \\
 $\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in [r]} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} (\binom{r}{r'}  .  p^*_{r,r'} - \delta_{r'})  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\binom{r}{r'}  .  p^*_{r,r'}+ \delta_{r'}  )\mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r')) + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') )  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , r \}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') )  \\ >  P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](\lfloor \frac{r+1}{2} \rfloor + 1)) \\ =  P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  ( \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}\delta_{r'} - \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} \delta_{r'}) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1)  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  P(s|s,\pi^*(s)) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1) \\ > P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  P(s|s,\pi^*(s)) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( r) 
 $ \\
 Thus, we have, \\
 $\mathbb{P}^{\pi^*}[N_k \geq x](s) - \mathbb{P}^{\pi^*}[N_k \geq x](r) \geq P(s|s,\pi^*(s)).(\mathbb{P}^{\pi^*}[N_k \geq x-1](s) - \mathbb{P}^{\pi^*}[N_k \geq x-1](r))$ \\ By recursion and same arguments as before, \\
 $\mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r+1) >  \mathbb{P}^{\pi^*}[N_k \geq x](r)$
\\
 
 Hence the overall main induction argument for r holds. \\ \\
 Now, given this general theorem, where $s_1 \in \mathcal{S}_{n,1}$, we have, \\$\mathbb{P}^{\pi}[N_k \geq V^*_1](s) \geq \mathbb{P}^{\pi^*}[N_k \geq V^*_1](s_1) = (1-p^*(g|s,a^*))^{\lceil V^*_1 \rceil -1} \geq (1-p^*(g|s,a^*))^{ V^*_1  -1}  \geq 1/e \geq 1/4$

\subsubsection{Ignore this and check next section: Simplification of KL Divergence term 14-3-25} 
By chain rule of KL-Divergence, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)]$
\\
where, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $

\\
Let's simplify $\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)})$


\pt{Before doing this upper bound, why can't I break it into two terms -- first one where $s_t = (g,g,...,g)$, and the other one when $s_t \neq (g,..., g)$. I think the terms will be simplified a lot if you do this. 
 Also, you can go one step ahead and look at all the impossible transitions -- the log term will vanish for all of them. So, you are left with the cases when the transitions are valid. Now, you can utilize the same notations, $r$ to $r'$ type of transitions. For all such transitions, the ratio inside the log can be written in terms of the features and corresponding $\theta$, and $\theta^j$. note that we might need to carefully use the conditions on $\delta$ and $\Delta$ you obtained earlier. } \textcolor{red}{i won't be able to use $s_{t+1} \neq g$ inside ln(.), I need to check when the ratio inside ln maximises here:$s_{max}$ to provide upper bound. $s_{min}$ is not strictly required and any global state can be used instead as for eg. you suggested $g,g,g...$. Also yes, i'm thinking of possible transitions only although once the $s_t$ is fixed from outer  summation. But notice that when $s_t=(s_{init},s_{init},...s_{init})$, we will need to optimize over all $s \in S$.}

 \pt{i am not talking about $s_{t+1}$, I am saying you can look at the summation for two cases separately, $s_t = g$, and $s_t \neq g$. That will lead to some simplifications. } \\ \textcolor{red}{i wouldn't even think about $s_t=g$: cz then $s_{t+1}$ has to be $g$ with probability 1 : independent of $\theta$ or $\theta_j$ hence ratio inside log is 1 and this term will be 0, for other $s_{t+1}$ probability is 0 hence all those terms are 0. problem is to deal with the general case}

 \pt{exactly, that's where we can now only use the features and then explicitly write them in terms of the other parameters. Also, why you are trying to maximize the term inside the log? We can just write the expressions for $\theta$ and $\theta^j$ and then finally use some other bounds at the later stage.} 

 \textcolor{red}{explicitly substituting the probabilities using features leads to a huge sum, each of those $2^{r}$ terms will have ratio inside ln that looks like line 1765. It would be desirable to simplify those terms without bounding earlier. The reason i want to maximise is to bound before simplifying. I'm just trying an approach as of now.  }


 \pt{Some results from the Jaksch et al 2010 paper can be used at the later stage.}

 \begin{figure}[h!]
     \centering
     \includegraphics[width=0.5\linewidth]{Jaksch.png}
     \caption{The result from Jaksch et al 2010 paper. This holds for some conditions on $\delta', \epsilon'$. Need to check if these conditions hold in our work. this type of result can be used for each term inside the summation, possibly for each $r$ to $r'$ transition. }
 \end{figure}
 \textcolor{red}{i have seen this, it can't be used for our case. in fact i want to get the sum over $2^r$ next states in this form thats why looking for maximum of that ratio. thats what motivated line 1756. also if you look carefully, the above result is not exactly from Jaksch, it is from Min. Jaksch result is bit different. Also Min made has made a typo in this above equation.}
 
 


Notice this can be upper bounded as follows: \\ 
$\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ \leq \mathcal{P}_{\theta}(s_{t+1}= s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s_{min}|\textbf{s}_{t-1}, s_t = s, a_t = a)}) + (1-\mathcal{P}_{\theta}(s_{t+1  }= s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a)).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s_{max}|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s_{max}|\textbf{s}_{t-1}, s_t = s, a_t = a)})$ \\
where, \\ $s_{min} = arg min_{s' \in \mathcal{S}} \ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $ and, \\
$s_{max} = arg max_{s' \in \mathcal{S}} \ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ $ \\
Since, $s$ and $a$ are fixed in the outer summation, both $s_{min}$ and $s_{max}$ may depend on both $s$ and $a$. For any general transition, we investigate the behavior of the ratio above. Given $s_t$, we partition the set of agents at $s_{init}$, into $X$ and $Y$ based on action $a$. Suppose $a$ is such that agents in $X:$ $x_1,x_2,\dots,x_m$ have their $j-th$ components not matching signs with respective components of $\theta$. Hence, agents $x_1,x_2,\dots,x_m$ have their $j-th$ components matching signs with respective components of $\theta_j$. Similarly let agents in $Y: y_1,y_2,\dots, y_{r-m}$ be such that their $j-th$ components match with respective components in $\theta$. This means agents $y_1, y_2, \dots, y_{r-m}$ are such that their $j-th $ components do not match with $\theta_j$. Along with previous notations, the ratio can be analyzed as : \\ 
$
\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}  \\= \frac{\frac{(r'-0.5r)(1-2\delta) + 0.5n }{n.2^{r-1}}     +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)}\sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}}{  \frac{(r'-0.5r)(1-2\delta) + 0.5n }{n.2^{r-1}}          +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta^j_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta^j_{t,p})\} \Big \}} \\ 
$\\ \\
To find the optimal values of this ratio, we first check what happens at fixed $r, r'$ and then optimize for $r'$. Notice that the ratio is maximum when maximum number of agents who stayed had signs matched with $\theta_j$ and maximum number of agents who transited had signs matched with $\theta$

\textcolor{blue}{we are looking at $\mathbb{E}_P[X] - \mathbb{E}_Q[X]$ for two probability measures $P$ and $Q$. we can use change of variable and write $\mathbb{E}_Q[X] = \mathbb{E}_P[X \frac{dQ}{dP}]$? }

\textcolor{blue}{policy is $\pi_\theta$ and does $\theta$ refer to something else? }

\textcolor{blue}{based on a call on Sat 10pm, 22/3}
\textcolor{red}{hi, i thought we weren't meeting yesterday} \\
\pt{\url{http://joschu.net/blog/kl-approx.html} -- we can use some ideas from here.} \textcolor{blue}{this unbaised estimator of KL with low variance (by John Shulmann of PPO fame) would be very good to use in computations} \textcolor{red}{Im very doubtful, this blog is about constructing suitable estimate of kl-div from samples. but we need to analytically express kl-div or its suitable upper bound}

\pt{The above blog is suitable for the computations, isn't it?} \textcolor{red}{if by computation u mean implementing learning algo for massp, then no. I dont know if you are referring to any other kind of computation}

\pt{can we make use of the indicator present in line 1775 and bound the entire term.}

\pt{Other possibility is to take out the smallest of $\sum_{i\in I \cap T'}$ and $\sum_{t\in T}$?} \\ \textcolor{red}{can u try these and update above?}

\pt{Just for clarity, what I remember is:}

\pt{$\mathcal{I}$: Set of all agent are $s_{init}$.}

\pt{$\mathcal{J}$: Set of all agents at $g$}

\pt{$\mathcal{T}$: Set of all agents from $\mathcal{I}$ who move from $s$ to $g$.}

\pt{$\mathcal{T}'$: set of all agents from $\mathcal{I}$ who stayed at $s$}


\pt{If the above is correct, then $\mathcal{I}\cap \mathcal{T}'$ and $T$ are disjoint?} \textcolor{red}{yes, also above is correct}


\pt{Alternatively, upper bound the numerator, and lower bound the denominator and vice-versa and then take the min.} 
\textcolor{red}{the bounding of individual ratio doesn't help later, then there would be $2^r$ type factor}  \\ \textcolor{blue}{we can use min of two bounds and see how it effects the regret bound}

\pt{Also, note that only the orders as of now with respect to $n$ are important, not the front constants. As long as we are able to get some order of the regret bound wrt $n$, we are good.}


\pt{Any updates after Saturday?} \textcolor{red}{no break thru yet}

\textcolor{blue}{$\delta$ and $\delta_j$ are vectors with entries +1s and -1s. When entries are  +1s and 0s the Hamming distance between them is the number of entries that differ. we can \emph{temporarily} take -1s as 0s. this may  help to bound the KL$(\delta|| \delta_j)$.}
\\
\textcolor{red}{I have an update : today I performed computation of the sum in line 1758 for many instances of n,a,$s_t$ and realized that it is maximum at $s_t = (s_{init},s_{init},...,s_{init})$ : contradictory to what i was hoping (max for states of type r=1). Turns out this can be explained by property of KL-divergence. So we can upper bound this summation for any $s_t$ by the summation at this initial state. As of now i don't know if the upper bound i wish to obtain (same/similar as given in Min) still holds. Im trying to see that via computations. Will update further soon.}

\pt{Wasn't this observation intuitive and follows from the fact that KL is positive, and  when I told you that for the case when $s_t = (g,g,g...g)$, then one term was getting zero?} \textcolor{red}{Pls explain us how this is intuitive from terms becoming 0 when st is all at g, in the next meeting. Also do respond to my earlier responses on your above remarks, its further confusing when you suggest something and not elaborate anything. Also next meeting pls come prepared to explain the steps in upper bound proof that i had asked in January. The note you send is unclear to me.}

\pt{What are the next steps in theory?}

Meeting link: \url{https://ucf.zoom.us/j/99575809604?pwd=dar1hN9fReFbU4yae8Bp4YGDKfaBeP.1}
\\ \\
Property of KL-Divergence: https://math.stackexchange.com/questions/4986295/partition-form-of-the-kl-divergence


\subsection{\textit{Simplifying KL-Divergence} \label{simplify_kld}}

By chain rule of KL-Divergence, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)]$
\\
where, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $ \\
Notice that in the above, for any fixed $(s,a)$, the inner summation is itself a KL-divergence. \\ 
Let's simplify it first: \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\  = \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) $ \\
Hence we'll upper bound using the inner KL for any $\tb{s} \in \mathcal{S}$. \\
As $ KL(B|A) > 0$, $KL(A|B) \leq KL(A|B) + KL(B|A)$ for any distributions $A, B$. Thus: \\ \\
$\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\ \leq   \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) + \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}) \\= \sum_{s' \in \mathcal{S}} (\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) ).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\
= \sum_{s' \in \mathcal{S}} (\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) ).\ln(1 + \frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\
\leq \sum_{s' \in \mathcal{S}} \frac{(\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) )^2}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)} \\
\leq 2^n . \frac{max_{s'}( \langle \phi(s'|s,a), \theta - \theta_j \rangle)^2}{ min_{s}\mathcal{P}_{\theta_j}(s_{t+1}=g|s_t = s, a_t = a)} \leq 2^n . \frac{(\frac{2 \Delta}{d-1})^2}{\frac{\delta}{2^{n-1}} - \Delta}
$ \\
Since $2/5<\delta<1/2$ and $\Delta<2^{-n}\frac{1-2\delta}{1+n+n^2}$, $\Delta < 2^{-n}. \frac{2\delta}{3} $. \\ Thus, \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)})  < 2^n. \frac{(\frac{4\Delta^2}{(d-1)^2})}{\frac{2\delta}{3.2^{n-1}}} = 3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $ \\ 
Hence, going back above: \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\  = \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) < 3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $ \\
Thus, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ < \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} \\ =  \mathcal{P}({s}_{t} \neq g) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $  \\ \\ Therefore from earlier, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] \\ <  \sum_{t=1}^{T-1} \mathcal{P}({s}_{t} \neq g) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} \leq  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} .  \sum_{t=1}^{T} \mathcal{P}({s}_{t} \neq g)  =  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]  $
\\
We use the above result in lower bound proof.

\pt{This seems good. Can you also write why the inequality in line 1847 holds} \\ \textcolor{red}{you meant the 1st line in the equations right? ive mentioned now in line 1848} \pt{yes, got it.}

\pt{Does that mean we now have a lower bound proof? I can see that the KL bound is exponential in $n$, will it lead to exponential bounds? or will it create some problems in the lower bound?}
\\
\textcolor{red}{yes we have a lower bound now. yes it looks exponential but from sufficient conditions, $\Delta$ is also of exponential order hence overall the bound is not exponentially large. from computations i've verified that this is quite tight(off by 1 order of magnitude for small n's and this difference decreases as n increases. hence we have a reasonably tight bound). ive updated and completed the lower bound proof(page 38). finally we get lower bound that scales as $1/2^n$. but we also get $\sqrt{K}$ }


\pt{Great!! So, we have the lower bound with $\sqrt{K}$, thus as tightest lower bound in terms of $K$, and can you explain what is the regret lower bound implication as $n$ increases? -- somehow not very clear to me. Particulary, i dond't understand this statement of yours  ``this difference decreases as n
increases. hence we have a reasonably tight bound''. } \textcolor{red}{yeah no problem, i will clear this in next meeting}

\pt{I think, now is the time to clean it and write the results in a nice format with all the details and explaination of each step. Can you explain the entire proof in our next meeting, and we can start writing it. }
\textcolor{red}{yes i wanted to explain everything too}
\pt{Let us connect on Friday evening 7:00 PM or Sat morning 9:00 AM India time, we can discuss this for a long time with all the details.} \textcolor{red}{sure, saturday 9am would be best}

Meeting link: \url{https://ucf.zoom.us/j/99575809604?pwd=dar1hN9fReFbU4yae8Bp4YGDKfaBeP.1}

\subsection{\textit{Upper Bound proof and Implementation}}
\begin{itemize}
    \item Simplification of T
    \item Min-max : convergence to best policy
    \item Appendix C3 line 3: $a_{m,h}$ is not the same as argmin_a $Q^i_{j_i}(s_{m,h},a)$ for this algo.
    \item Algorithm: V update-what about $a^{-i}$
\end{itemize}

\subsection{Related Work}
\label{subsec:related_work}

\input{CR_Sections/extras}


\begin{corollary}\label{corollary:ps_s}
For any non-goal state $\tb{\ti{s}} \in \mathcal{S}_r$ of type $r$, the self-transition probability under action $\tb{\ti{a}}$ is
\begin{align}
    \mathbb{P}(\tb{\ti{s}} | \tb{\ti{s}}, \tb{\ti{a}}) = \frac{r(1-\delta)}{n \cdot 2^{r-1}} + \frac{n - r}{n \cdot 2^r} -  \frac{r \cdot \Delta}{n} + \frac{2\Delta}{n(d - 1)} \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d - 1} \mathbbm{1}\{\sgn({a}_{i,p}) \neq \sgn(\theta_{i,p})\}.
\end{align}
This is minimized when $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$ and the resulting probability only depends on $r$.
\end{corollary}
% 





\begin{lemma} \label{lemma:episodelength} 
Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$ as the probability that starting at state $\tb{\ti{s}} \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in R^+$. Furthermore, $\mathbb{P}^{\pi}[N_k \geq x] = \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$. 
Consider any $\tb{\ti{s}} \in \mathcal{S}(r)$ where $r \in [n]$. Then, for any policy $\pi$, it holds for any instance as defined in (ref) that for any $x \in R^+$: \\ $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}')$ \\ where $\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})$ with equality holding (for all $x \in R^+$) only at $\pi = \pi^*$  and $r'=r $ (i.e., $\tb{\ti{s}}'=\tb{\ti{s}}$) respectively. \\  Here $\pi^*$ is the policy of taking action $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$ (optimal policy from Theorem \ref{thm:all_in_one}). The equality in the middle indicates that under $\pi^*$ (for any fixed $x \in R^+$), $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ stays constant depending only on $r$ for all $\tb{\ti{s}} \in \mathcal{S}(r)$.
\end{lemma}

\begin{corollary}
\label{corollary:pn_x}
An immediate corollary of the above lemma is that $\mathbb{P}^{\pi^*}[N_k \geq x](r)$ is ordered for any $x \in R^+$ i.e., $\mathbb{P}^{\pi^*}[N_k \geq x](n) \geq \mathbb{P}^{\pi^*}[N_k \geq x](n-1) \geq \cdots \geq \mathbb{P}^{\pi^*}[N_k \geq x](2) \geq \mathbb{P}^{\pi^*}[N_k \geq x](1) \geq \mathbb{P}^{\pi^*}[N_k \geq x](0) =0 $

\end{corollary}



\subsection{Proof of Lemma \ref{lemma:episodelength}}
Used in proof of Lemma 5.

\textbf{Recall the Lemma \ref{lemma:episodelength}. } 
% 
\textit{Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$ as the probability that starting at state $\tb{\ti{s}} \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in R^+$. Furthermore, $\mathbb{P}^{\pi}[N_k \geq x] = \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$.} 

\textit{Consider any $\tb{\ti{s}} \in \mathcal{S}(r)$ where $r \in [n]$. Then, for any policy $\pi$, it holds for any instance as defined in (ref) that for any $x \in R^+$: \\ $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}')$ \\ where $\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})$ with equality holding (for all $x \in R^+$) only at $\pi = \pi^*$  and $r'=r $ (i.e., $\tb{\ti{s}}'=\tb{\ti{s}}$) respectively. \\  Here $\pi^*$ is the policy of taking action $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$ (optimal policy from Theorem \ref{thm:all_in_one}). The equality in the middle indicates that under $\pi^*$ (for any fixed $x \in R^+$), $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ stays constant depending only on $r$ for all $\tb{\ti{s}} \in \mathcal{S}(r)$.}


\begin{proof}
 
We will prove this by induction.
\\
 \tb{Base Case:} \\ For r=1: 
 Consider any $\tb{\ti{s}} \in \mathcal{S}(1)$ \\
 For any $x \in R^+$, 
 \begin{align}
     \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) = (1-\mathbb{P}(\tb{g}|\tb{\ti{s}},\pi(\tb{\ti{s}})))^{\lceil x\rceil-1}
 \end{align}
 One can check from Lemma \ref{lemma:general_tp} that the above is uniquely minimum when $\pi(\tb{\ti{s}}) = \tb{\ti{a}}^*$. Hence equality only holds at $\pi=\pi^*$.  \\
 Hence,
 \begin{align}\label{eqn:prob_n}
     \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) = (1-\mathbb{P}(\tb{g}|\tb{\ti{s}},\pi(\tb{\ti{s}})))^{\lceil x\rceil-1} \geq (1-\mathbb{P}(\tb{g}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})))^{\lceil x\rceil -1}
 \end{align}
 Recall that for the same action $\tb{\ti{a}}^*$ at any $\tb{\ti{s}} \in \mathcal{S}(1)$, $\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}}^*)$ remains the same (Corollary \ref{corollary:p_star}).\\
 Hence, we further have, 
 \begin{align}
     \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) = (1-\mathbb{P}(\tb{g}|\tb{\ti{s}},\pi(\tb{\ti{s}})))^{\lceil x \rceil-1} \geq (1-\mathbb{P}(\tb{g}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) 
 \end{align}
 The only two possibilities for next state $\tb{\ti{s}}'$ are $\tb{\ti{s}}$ itself and $\tb{g}$. \\
 Clearly for $\tb{\ti{s}}$ the equality holds and for $\tb{g}$, $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}'=\tb{\ti{g}}) = 0$ \\ Hence, 
 \begin{align}
     \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) = (1-\mathbb{P}(\tb{\ti{g}}|\tb{\ti{s}},\pi(\tb{\ti{s}})))^{\lceil x \rceil-1} \geq (1-\mathbb{P}(\tb{\ti{g}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}') 
 \end{align}
  \\ To recap, we have shown above that for any $x \in R^+$ for any policy $\pi$, for any $\tb{\ti{s}} \in \mathcal{S}(1)$ and $\tb{\ti{s}}' \in \cup_{r' \in \{0,1\}} \mathcal{S}(r')(\tb{\ti{s}})$,  \\
  \begin{align}
      \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})  \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}') 
  \end{align}
  where in the first inequality, equality holds for all $x \in R^+$ only when $\pi = \pi^*$, the middle equality means that the probability is same for all $\tb{\ti{s}} \in \mathcal{S}(1)$ and in the last inequality, equality holds only when $\tb{\ti{s}}' = \tb{\ti{s}}$. \\
  \\
  \tb{Generalization:} \\ Assume the above holds for m = 1, 2,\dots,r i.e., for all $m \in [r]$ it holds that for any $x \in R^+$ for any $\tb{\ti{s}} \in \mathcal{S}(m)$, for any policy $\pi$, for our instances, 
  \begin{align}
   \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})=\mathbb{P}^{\pi^*}[N_k \geq x](m)\geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}')   
  \end{align}
   where $\pi^*$ is the policy taking action $\tb{\ti{a}}^*=\tb{\ti{a}}_{\theta}$ at all states and $\tb{\ti{s}}' \in \cup_{m' \in \{\{0\} \cup [m] \}}\mathcal{S}(m')(\tb{\ti{s}}) = \mathcal{S}(\tb{\ti{s}})$. Further, in the first inequality, equality only holds for all $x \in R^+$ when $\pi =\pi^*$ and the middle equality implies that the probability is same for all states of same \emph{type} $\tb{\ti{s}} \in \mathcal{S}(m)$ and in the last inequality, the equality only holds when $\tb{\ti{s}}' = \tb{\ti{s}}$.  \\
  Assuming this, we need to show that the same holds for any $\tb{\ti{s}} \in \mathcal{S}(r+1)$ \\ 
  Now, consider any $x \in R^+$. \\
  Consider any $\tb{\ti{s}} \in \mathcal{S}(r+1)$. \\
  We have, 
  \begin{align}
      &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \\
      &= \sum_{r' \in \{0,[r+1]\}} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\pi(\tb{\ti{s}})) . \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}') \\
      &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})). \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' \in \{0,[r]\}} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})}  \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\pi(\tb{\ti{s}})). \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}')
  \end{align}
   If $x \leq 1$, then trivially, for all $\tb{\ti{s}} \neq \tb{g}$, for all policies, $\mathbb{P}[N_k \geq x] = 1$. However,in general, we have the following:
   \begin{align}
      &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})  \\
      &=  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' \in \{0,[r]\}} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})}  \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}') \\
      &\geq \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' \in \{0,[r]\}} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})}  \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](r') 
      \end{align}
      The above follows from induction assumption. \\
      Thus,
      \begin{align}
      &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})  \\   
      &\geq  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})}  \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\pi(\tb{\ti{s}})) \\
      &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) +  \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \times \\ 
      &\quad  \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r') +  \\
    &\quad \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}   -\sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}  \Bigg\} \\
    &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
    &\quad \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Bigg \} + \\ 
    &\quad \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \times \\
    &\quad   \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})}  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}   -\sum_{t \in \mathcal{T}} \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}  
  \end{align}
  In the first term, we observe that the term inside the inner summation over $s' \in \mathcal{S}(r')(\tb{\ti{s}}')$, the terms inside that summation do not depend on which $\tb{\ti{s}}'$ is being considered for a fixed $r'$ and $\tb{\ti{s}}$ and are the same. Hence, the whole summation simplifies to the product of this term and the cardinality of that set which is $\binom{r+1}{r'}$. Also, we realize that for the second term for any agent the coefficient of the indicator is $+1$ if he stays at node $s$ itself while it is $-1$ when he transits to node $g$. Hence we can simplify the above as following including some rearrangement of summation and using the fact that the probability terms vanish for state of \emph{type} 0, namely $\tb{\ti{g}}$ :
  \begin{align}
   &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})  \\   
  &\geq \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
  &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ 
  &\quad \frac{2 \Delta}{n(d-1)} \times \\
  &\sum_{p \in [d-1]} \sum_{r' \in  [r]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \sum_{i \in \mathcal{I}}      \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\}.   - \mathbbm{1}\{i \in \mathcal{T}\}\Big \} . \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} 
   \\
   &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
   &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ 
   &\quad \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in [r]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{i \in \mathcal{I}}      \Big  \{ \binom{r}{r'-1} -  \binom{r}{r'} \Big \}. \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}
   \end{align}
   The last step follows by taking the summation over $s'$ inside and observing that from any fixed $\tb{\ti{s}}$ of \emph{type} $r$, the number of states of \emph{type} $r'$ reachable from $\tb{\ti{s}}$ in which any agent at node $s$ stays at node $s$ is $\binom{r}{r'-1}$ and those in which he transits to node $g$ is $\binom{r}{r'}$. Thus, we have:
   \begin{align}
   &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})  \\  
   &\geq \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
   &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ 
   &\quad \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in [r]} \sum_{i \in \mathcal{I}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{  \binom{r}{r'-1} -  \binom{r}{r'}  \Big \} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}
   \\
   &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
   &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ 
   &\quad \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \binom{r}{r'-1} -  \binom{r}{r'}  \Big \}\mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}  \\
   &\quad + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{  \binom{r}{r-r'} -  \binom{r}{r+1-r'} \Big \}. \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Bigg \}   
   \end{align}
    In the last step, we use $\sum_{a\in[m]}f(a) = \sum_{a\in[m]} f(m+1-a)$ for any $f(\cdot)$ \\
    We simplify above as:
   \begin{align}
   &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \\    
   &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
   &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ 
   &\quad \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]}  \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{  \binom{r}{r'-1} -  \binom{r}{r'} \Big \} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}  \\
   &\quad + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{  \binom{r}{r'} -  \binom{r}{r'-1}\Big \}. \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Bigg \} \\
   &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\
   &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\
   &\quad \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]}  \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \Bigg \{ \Big \{ \binom{r}{r'-1} -  \binom{r}{r'} \Big \} \Big \{ \mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq V^*_1](r+1-r') \Big \}   . \\
   &\quad \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}        \Bigg \}
   \end{align}
 Notice that for $r' \leq  (r+1)/2$, the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as probability difference $\mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r') \leq  0$ due to induction assumption, hence the product is $ \geq 0$. Similar argument holds for $r'\geq (r+1)/2$.  \\
 Overall we can observe that the only terms dependent on action have non-negative coefficients for the sign matching indicator. Hence the overall summation will be minimum when this term will be minimum which happens at $a = a^*=a_{\theta}$.  \\
 Thus, we have, 
 \begin{align}
     &\mathbb{P}^{\pi}[N_k\geq x](\tb{\ti{s}}) \\
     &\geq   \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
     &\sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} 
 \end{align}
 Also, 
 \begin{align}
     & \mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}}) \\
     & =   \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) \\
     &\quad+  \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} + \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 \end{align}
Subtracting the above two equations, 
\begin{align}
    &\mathbb{P}^{\pi}[N_k\geq x](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}}) \\ 
    &\geq \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) - \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) \\ 
    &\geq \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) - \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) \\ 
    &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) (\mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}))
\end{align}
The last second step follows from Corollary \ref{corollary:ps_s}.\\
By recursion we have,  
\begin{align}\label{eqn:pnxnx}
    &\mathbb{P}^{\pi}[N_k\geq x](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}}) \\ 
    &\geq \mathbb{P}\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}}))^{\lfloor x \rfloor} \{\mathbb{P}^{\pi}[N_k \geq x-\lfloor x \rfloor](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k \geq x-\lfloor x \rfloor](\tb{\ti{s}})\} \\
    &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}}))^{\lfloor x \rfloor} (1- 1) \\
    &= 0
\end{align}
In the last second step, we use the fact that $x-[x]$ is a fractional value or equal to $0$ for any $x \in R^+$ hence for any $\tb{\ti{s}} \neq \tb{\ti{g}},$ certainly (w.p. 1), at least one time step is required to reach reach $\tb{\ti{g}}$. \\
Thus, 
\begin{align}
   \mathbb{P}^{\pi}[N_k\geq x](s) \geq \mathbb{P}^{\pi^*}[N_k\geq x](s) 
\end{align}
Also note that for equality for all $x \in R^+$, the equality must hold at every one of the above inequalities. Effectively this will only happen if $\pi = \pi^*$ \\ 


Recall, for any $\tb{\ti{s}} \in \mathcal{S}(r)$, 
\begin{align}\label{eqn:prob_nxs}
    &\mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}}) \\
    &=   \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
    &\sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
\end{align}
From the probability expression one can verify that the term $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}}))$ only depends on $r$. The second term is independent of $\tb{\ti{s}} \in \mathcal{S}(\tb{\ti{r}})$ due to induction hypothesis and $r+1$ is same. \\Thus, the only term in the above expression that may differ due to $\tb{\ti{s}}$ is $\mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}})$. \\We claim that this is same too for all $\tb{\ti{s}} \in \mathcal{S}(r)$.\\ 
This can be dealt with by induction on $x$ itself.  \\
For base case, $m = x-\lfloor x \rfloor$, for any $\tb{\ti{s}} \in \mathcal{S}(r)$, $\mathbb{P}^{\pi^*}[N_k \geq m](\tb{\ti{s}})=1$ \\ 
Hence showed for base case. \\ 
Assuming true for $ x - \lfloor x \rfloor,  x - \lfloor x \rfloor+1,  x - \lfloor x \rfloor+2, \dots,  x - \lfloor x \rfloor+q $, we need to show that it holds for $m =  x - \lfloor x \rfloor + q+1$ \\ We can write for any $\tb{\ti{s}} \in \mathcal{S}(r)$ that: 
\begin{align}
   &\mathbb{P}^{\pi^*}[N_k\geq m ](\tb{\ti{s}}) \\
   &=\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq m-1](\tb{\ti{s}}) \\
   &+  \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq m-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} 
\end{align}
 Here the RHS doesn't depend on which $\tb{\ti{s}} \in \mathcal{S}(r)$ is being chosen again due to induction assumption and Corollary \ref{corollary:p_star}. Thus shown for m. \textcolor{blue}{$m = x - \lfloor x \rfloor + q + 1$} ? \\
 Thus, back in expression for $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ in Equation \eqref{eqn:prob_nxs}, $\mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}})$ is also not dependent on $\tb{\ti{s}} \in \mathcal{S}(r)$. Therefore, $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ is same for all $\tb{\ti{s}} \in \mathcal{S}(r)$.  \\

 
 Finally we need to show that, 
    \begin{align}
        \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}') \forall \tb{\ti{s}}' \in \cup_{r' \in \{0,[r]\}}\mathcal{S}(r')
    \end{align}
 with equality only at $\tb{\ti{s}}' = \tb{\ti{s}}$. \\
 Recall again, for any $\tb{\ti{s}} \in \mathcal{S}(r+1)$, 
 \begin{align}
     &\mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}})\\
     &=   \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' \in [r]} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\ 
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' = 1}^{ \lfloor \frac{r+1}{2} \rfloor } \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\
     &\quad + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{ r} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') 
     \end{align}
     In the above, we just split the summation and below, we use the fact that Claim \ref{claim:probability_inequality} is true for our instances.\\
     In the below all $\delta_{r'}$ are all positive. Note that for different $r$, these will be different and technically we must write $\delta_{r,r'}$ but we let it be to avoid notational overhead. \textcolor{red}{we can use $\delta_{r,r'}$. for now im leaving it as it is}
     
     \begin{align}
     &\mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}})\\
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r'= 1}^{ \lfloor \frac{r+1}{2} \rfloor } \Big\{\binom{r}{r'}  .  p^*_{r,r'} - \delta_{r'} \Big\}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\
     &\quad + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{ r} \Big \{\binom{r}{r'}  .  p^*_{r,r'}+ \delta_{r'}  \Big\}\mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \\ 
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' = 1}^{ \lfloor \frac{r+1}{2} \rfloor } \Big\{\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\} \\
     &\quad -  \sum_{r' = 1}^{\lfloor \frac{r+1}{2} \rfloor }\Big\{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r')\Big\}   + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{ r} \Big\{\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r')\Big\} \\
     &\quad + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \Big\{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\}  \\ 
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' = 1}^{ r} \Big\{ \binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\} \\
     &\quad -  \sum_{r' =1}^{ \lfloor \frac{r+1}{2} \rfloor}\Big\{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\}   + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{ r} \Big\{ \delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\} \\ 
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  \\
     &\quad -  \sum_{r' = 1}^{ \lfloor \frac{r+1}{2} \rfloor }\Big\{ \delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\}  + \sum_{r'= \lfloor \frac{r+1}{2} \rfloor +1}^{r} \Big\{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\}  
     \end{align}
    The last step is using the definition of $\mathbb{P}^{\pi^*}[N_k \geq x](r)$. \\
    Below we use Corollary \ref{corollary:pn_x}:
     \begin{align}
     &\mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}})\\
     &\geq  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \sum_{r'=1}^{ \lfloor \frac{r+1}{2} \rfloor } \Big \{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1)\Big\} \\
     &\quad+ \sum_{r' =\lfloor \frac{r+1}{2} \rfloor +1}^{r} \Big\{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](\lfloor \frac{r+1}{2} \rfloor + 1)\Big\} \\ 
     &=  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \Big\{ \sum_{r'= 1}^{ \lfloor \frac{r+1}{2} \rfloor }\delta_{r'} - \sum_{r'= \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'} \Big\} . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1)  \\ 
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1) \\ 
     &> \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( r) 
 \end{align}
 In the last second step, we used the result and the discussion that leads to Equation \eqref{eqn:prr}.\\
 For the last step, we further use Corollary \ref{corollary:pn_x}.\\
 Thus, we have, 
 \begin{align}
     \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k \geq x](r) \geq P(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})).(\mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k \geq x-1](r))
 \end{align}
 By recursion and same arguments as before that follows Equation \eqref{eqn:pnxnx}, \\
 \begin{align}
     \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r+1) >  \mathbb{P}^{\pi^*}[N_k \geq x](r)
 \end{align}
 Hence the overall main induction argument for $r$ holds.     
\end{proof}

==> CR_Sections/intro_old.tex <==
\pt{what is our problem, and what are challenges, what is novelty, why it is significant, and how is the flow of the entire thing. If not, can you try to think of how to take care of these important points. }.

...

\pt{Something along these lines has to be written in the intro.}

At the heart of this paper lies the following central question, which we state clearly:

\begin{center} \emph{``What is the fundamental difficulty of decentralized learning in multi-agent stochastic shortest path problems under linear function approximation?''} \end{center}

Multi-agent stochastic systems are ubiquitous -- appearing in domains like swarm robotics, traffic networks, and distributed control systems. In many such settings, agents must act collaboratively while having access to only partial, local information, and without centralized coordination. Understanding the inherent hardness of learning in these decentralized environments is therefore crucial: it informs the limits of achievable performance and guides the design of more efficient algorithms.

In particular, linear function approximation is an essential modeling tool to overcome the curse of dimensionality, but it also complicates the learning task by introducing generalization errors. Thus, quantifying the true difficulty in decentralized linear MDPs and SSPs is not only of theoretical importance but also necessary for building scalable, robust multi-agent systems.


Furthermore, the problem of establishing a \emph{regret lower bound} is crucial in evaluating the performance of decentralized learning algorithms. Specifically, we wish to understand how the performance of decentralized agents compares to that of an oracle following the optimal policy $\pi^*$ over $K$ episodes. The regret lower bound provides a benchmark against which the efficiency of the learning algorithms can be measured. A lower bound on regret helps establish the limits of what is achievable by decentralized agents when trying to minimize the total cost in the MA-SSP problem. 



A popular class of problems studied under the literature on Markov Decision Problems is the Stochastic Shortest Path (SSP) Problem \citep{eaton},\citep{berttsit}\citep{yu2013boundedness}\citep{yu2013q}\citep{bert_prop_pol}\citep{guillot2017stochasticshortestpathproblem}. It is also known as total reward undiscounted MDP \citep{puterman2014markov}, \citep{bertsekas2012dynamic}. It generalizes from the well-known Shortest Path (SP) Problem where one has to chose the best links at every node to traverse from one node to another on a \textit{known} network. To model various uncertainties, under SSP, costs are treated as stochastic, actions are represented as more abstract quantities, and there exists conditional probability distributions associated over \textit{next states} for any \textit{state-action} pair. Depending on how many agents are to traverse, the problem may be single or multi-agent. When cost and transition structures are known to the agent(s), the problem is that of searching the right strategy of chosing actions. When either of these are not available, the agent(s) must \textit{explore} and learn the environment over time and pick the \textit{best} actions. A line of works has recently emerged studying the learning version of SSP problem with single agent with finite state and action spaces \citep{tarbouriech2020no} \citep{rosenberg2020near} \citep{tarbouriech2021stochastic}\citep{cohen2021minimax}. 
To extend above works for large number of state and action spaces, \citep{min2022learning}
 and \citep{vial2022regret} use linear function approximations. While \citep{min2022learning} approximates only the transition dynamics and assumes the knowledge of costs, \citep{vial2022regret}'s model assumes approximation of costs as well. In summary, these works propose algorithms motivated by existing works in other classes of MDP and Bandit Literature. Additionally, the optimality of these algorithms has also been well established through tight lower bounds. 
 Many real world goal oriented settings however, involve interaction of multiple independent decision makers. To incorporate such settings, \citep{trivedi2023massp} introduce the problem of Decentralised Learning of Stochastic Shortest Path. The paper provides an algorithm for this setting and report an upper bound on regret of $\widetilde{O}({B^*}^{1.5}d \sqrt{nK/c_{min}})$ where $B^*$ is the maximum expected cost to reach goal from any state, $n$ is the number of agents, $d$ is related to the feature dimensions and $K$ is the number of episodes. The paper, however, does not comment on its optimality. Are better learning algorithms possible in this setting? If yes, what are the optimality gaps that new algorithms can fill? Can we comment on tightness of regret bounds with respect to number of agents? To answer such questions, it is important to obtain good lower bounds for this setting. Typical lower bound proofs in the literature of single-agent SSP \citep{rosenberg2020near}, \citep{min2022learning} or that of multi-armed bandits \citep{auer2002nonstochastic} or in general RL \citep{jaksch2010near} are generally based on hard to learn instances. 

The transition from single agent SSP to Multi-Agent SSP, leads to the following complications: 
\begin{itemize}
    \item The state and action space explodes (exponentially in number of agents $n$). Due to exponentially large number of states and actions, it is challenging to create and analyze such an instance for regret lower bound. Further, it is desirable to create generalizable instance in the number of agents in order to have analyses for all $n \geq 1$.  
    \item Next state transition probabilities and costs of individual agents (and thus of the system as a whole) depends not only on individual current state and action but also on that of others.
    \item Cost information is available only locally and needs to be shared with other agents to meet global objective. However, there may be privacy, security and scaling issues \citep{zhang2018fully}. 
    \item Existing lower bound proofs for previously studied settings typically consider only two node networks. For single agent cases, it corresponds to only two states. Both the optimal policies as well as values are easily characterizable. But, in a multi-agent (n agents) set up, even a two node network corresponds to $2^n$ states. It is unclear whether tractable optimal policies exist. Further, tractable closed form expression of optimal value function is no longer easy to obtain to use it in lower-bound regret analysis. We circumvent this issue by ignoring a non-exactly simplifiable summation of not neccesarily all positive terms, by showing that the entire summation is itself positive (\ref{lemma:sum_diff_prob_v}).
    \item In our analysis, we observe another similar challenge when simplifying a KL-divergence term that arises due to information theoretic bound on difference between expectations over different measures of the same random variable (\ref{eqn:exp_diff}) that captures the number of times sub-optimal component of action is taken similar in spirit to proofs in \citep{auer2002nonstochastic}. Instead of exact simplification, a suitably tight upper bounding technique that exploits symmetry of probability distrubution arising due to symmetry in state-space to simplify KL-divergence works for us.
 \end{itemize}

 
 
Major contribution of our work are 

\begin{itemize}

\item \textbf{Novel Feature Design.}  Design of new features generalizable to any number of agents to use in creating hard to learn LM-MASSP instance
\item Provide and study classes of valid LM-MASSP instances that are hard to learn to prove matching $\sqrt{K}$ lower bound. Such a lower bound analysis is first-of-its kind for exponential number of states and actions arising here due to muli-agent setting and can be generalizable to other multi state, multi action settings.

\item We characterize optimal policies for any 2-node instance as proposed in \ref{subsec:problem_instance} and show that its very tractable. Further, these instances have an interesting partition of state space based on number of agents at a given node - all states lying the same partition set have same optimum value function implying that under optimal policy, states with same number distribution of agents across the two nodes are equivalent as value function is independent of who is present and only dependent on how many are present

\end{itemize}

% \pt{I feel this is not needed in the conference papers.}

% In \ref{subsec:relatedwork} we provide a brief background on this line of literature. \\
% In \ref{subsec:prelims} we introduce the problem setting and necessary definitions. \\
% In \ref{subsec:problem_formulation} we formulate our problem. \\
% In \ref{subsec:problem_instance} we provide details of our instances. \\
% In \ref{subsec:features} we provide the features to use in the function approximation of transition probabilities. \\
% \ref{sec:theory} discusses major results with proof overviews.\\
% In \ref{sec:discussion} we summarize our contribution and suggest some interesting open problems arising from our work.\\
% All the detailed analyses and proofs leading to the key results are deferred to the appendix \ref{sec:appendix}

\subsection{Related Works}\label{subsec:relatedwork}


% \pt{If these are incorporated, we can remove this itemize list.} \textcolor{red}{d/one}


\paragraph{Shortest Path Problems.} The shortest path problems are one of the classical problems studied in the fields of computer science and operations research. The first evidence of stochastic shortest path problem may be traced back to 
\cite{eaton}. They studied the problem in pursuit evasion games. \cite{berttsit} proved the natural generalization of results for deterministic shortest path to the stochastic setting. Recently there has been a growing interest in studying the learning version of the problem \cite{tarbouriech2020no}, \cite{tarbouriech2021stochastic}, \cite{cohen2021minimax},\cite{rosenberg2020near}, \cite{vial2022regret}, \cite{min2022learning}. \\
\citep{tarbouriech2020no} provides first no-regret SSP learning algorithm UC-SSP whose regret bound scales as $\widetilde{O}(DS\sqrt{ADK/c_{min}})$ after K episodes for any tabular SSP with $S$ states, $A$ actions, positive costs bounded above $c_{min}>0$ and $D$ diameter of SSP defined as the smallest expected hitting time from any state to goal. In a follow-up work, \cite{rosenberg2020near} provide an algorithm whose regret upper bound gets rid of the $c_{min}$ dependence and scales as $\widetilde{O}(B^*S\sqrt{AK})$ where $B^*$ is analogous to $D$ above but in terms of cost rather than time. Importantly, they provide a lower bound scaling as $\Omega(B^*\sqrt{SAK})$ showing that their algorithm is optimal to a factor of $\sqrt{S}$. 

\paragraph{Learning in SSP.} \citep{tarbouriech2021stochastic} provide EP-SSP, a model based SSP learning algorithm whose regret upper bound scales as $\widetilde{O}(B^*\sqrt{SAK})$ achieving the previously reported lower bound. EP-SSP does not require prior knowledge of $B^*$. The paper also dicusses various cases that lead to first-nearly horizon-free regret bound beyond the finite horizon MDP setting. \citep{cohen2021minimax} assumed costs to be i.i.d and unknown while previous works assumed it to be known and deterministic and provided an algorithm based on reducing the SSP to finite horizon MDPs whose regret upper bound also achieves the reported lower bound. \\
The above works were for tabular SSPs. To deal with higher number of states and actions, \citep{min2022learning} and \citep{vial2022regret} assumed slightly different linear function approximation models for transition probabilities. \citep{vial2022regret} provides an algorithm that, under minimal assumption, obtains sublinear regret, is computationally efficient, and uses stationary policies. \citep{min2022learning} first proposes an algorithm with Hoeffding-type confidence sets that attains $\widetilde{O}(d{B^*}^{1.5}\sqrt{K/c_{min}})$
 regret for positive costs. A further improvement of the regret bound to  $\widetilde{O}(d{B^*}\sqrt{K/c_{min}})$ is achieved for another proposed algorithm using refined Bernstien-type confidence sets. Additionally provided lower bound of $\Omega(dB^*\sqrt{K})$ suggests that their algorithm is optimal to a $\sqrt{c_{min}}$ factor. \\
 All the above works consider that there is just a single traversing agent. \citep{trivedi2023massp} extend the problem to a decentralized multi-agent setup and provide a MACCM algorithm with a MAEVI subroutine whose regret scales as $\widetilde{O}({B^*}^{1.5}d\sqrt{nK/c_{min}})$. The paper does not comment on how tight the bound is. Hence the optimality of proposed algorithm is not well-established. \\
 \citep{zhang2021decentralized} propose two fully decentralized actor-critic algorithms for large scale MARL problems with convergence guarantees when value functions can be approximated by linear functions.

 
% \pt{let us keep the flow of the paper as it is now, this is very standard flow in the ML community.} \textcolor{red}{ok}

==> CR_Sections/outline.tex <==
\section{Outline of the Paper}

Here is the first attempt to the outline of the paper. We need to change or modify it as we write the paper. 

\begin{abstract}
We investigate the theoretical foundations of the multi-agent stochastic shortest path (MA-SSP) problem from a regret minimization perspective. While single-agent SSP has been well-studied with established regret upper and lower bounds, the multi-agent version remains under-explored. Recent work has extended regret upper bounds to the MA-SSP setting, but fundamental questions remain unresolved. In this paper, we derive the first regret lower bounds for MA-SSP and analyze how the number of agents impacts the complexity of learning. Our results bridge a critical gap in the literature and provide new insights into the design of efficient multi-agent learning algorithms.
\end{abstract}

\section{Introduction}

Briefly describe SSP, transition to RL version
Gaps in literature: lower bounds, agent scaling. And finally our major  contributions.
\begin{itemize}
    \item Start with the importance of the Stochastic Shortest Path (SSP) problem in planning and decision-making.
    \item Mention that Single-Agent SSP is well studied; cite foundational RL results with known upper and lower bounds.
    \item Emphasize that the multi-agent extension (MA-SSP) is less explored; mention \cite{trivedi2023massp} as a recent attempt.
    \item Point out the gaps in literature: No lower bounds for regret in MA-SSP.
    \item The effect of the number of agents on regret is poorly understood.
\end{itemize}

\textbf{Major Contributions:}

First regret lower bounds for MA-SSP.

Analysis of agent scaling in regret.

Matching (or near-matching) lower and upper bounds.

Novel intermediate theoretical insights (e.g., feature design).

Some additional results that can be of interest to the  ML community in other domains.

\subsection{Related Work}

SSP in RL: single-agent case. 
MARL literature, MA-SSP work. 
Prior bounds.  Highlight novelty Mention that to the best of our knowledge, these results are novel. Divide the entire section into 3-4 sub parts and dostinguish our work with the existing and also highlight the challenges and novelty. 

\begin{itemize}
    \item Classical SSP in RL: key algorithms, upper/lower bounds.
    \item Regret analysis in online RL (e.g., UCRL2, UBEV).
    \item Multi-agent RL and planning: MARL challenges, coordination, scalability.  
    \item \cite{trivedi2023massp} as the most relevant prior work on MA-SSP (upper bounds only).
    \item Lower bounds in MARL (mention scarcity).
    \item Highlight the novelty of your contributions in contrast.
\end{itemize}


\section{Problem Formulation}

Notations and Prelims -- Define MA-SSP setup: states, joint actions, dynamics, cost. Define regret. 
Key assumptions -- policy class, etc.



\begin{itemize}
    \item Formal definition of the MA-SSP setting: State space, action space, transitions, cost structure.
    \item Agents act in a shared environment to reach a terminal state.
    \item \textbf{Objective}: minimize cumulative cost  over episodes.
    \item Define regret formally over $K$ episodes.
    \item In detail explain assumptions: decentralized learning, linear MDP, feature design (complex process) etc. The linear MDP transitions can't be decomposed as a separate agents. 
    \item Highlight complexity due to joint actions and decentralized learning constraints (if any).
    \item Policy class restriction etc. 
\end{itemize}

\section{Our Approach}

High-level strategy to prove lower bounds. Intuition: why MA-SSP is harder. How to design the hard instances? Why they are hard. Major challanges, and how we address them. 

\begin{itemize}
    \item High-level outline of how you study the regret lower bounds in MA-SSP.
    \item Intuition: Construct ``hard'' MA-SSP instances.
    \item Show how agent interactions increase complexity
    \item Describe what makes SSP harder in the multi-agent case vs. single-agent.
    \item Brief overview of feature design techniques used in analysis.
    \item Clearly highlight the challenges and then how they are addressed. 
\end{itemize}

\section{Theoretical Results}

Theorem: regret lower bound. Sketch of proof. Dependence on number of agents. Matching to known upper bounds. Feature-related insights. Other key results in the form of lemma, corollary and propositions, remarks etc. 



\section{Experiments (If available)}

Toy MA-SSP setup. Regret vs. agents graph if possible. Empirical support for theory

\begin{itemize}
    \item Simple MA-SSP instances with n=3, 4, etc?
    \item Plot regret vs. number of agents.
    \item Show alignment between theory and practice (at least qualitatively).
    \item Highlight how coordination and joint action space increase learning complexity.
\end{itemize}

\section{Conclusion/Discussion}

Recap contributions. Importance of theoretical results. Future work directions.

==> CR_Sections/updated_features.tex <==
\section*{Updated Features}





==> Sections/0_abstract.tex <==
\begin{abstract}
    Multi-agent systems (MAS) are central to applications such as swarm robotics and traffic routing, where agents must coordinate in a decentralized manner to achieve a common objective. Stochastic Shortest Path (SSP) problems provide a natural framework for modeling decentralized control in such settings.
    While the problem of learning in SSP has been extensively studied in single-agent settings, the decentralized multi-agent variant remains largely unexplored. In this work, we take a step towards addressing that gap. 
    We study decentralized multi-agent SSPs (Dec-MASSPs) under linear function approximation, where the transition dynamics and costs are represented using linear models. Applying novel symmetry-based arguments, we identify the structure of optimal policies. Our main contribution is the first regret lower bound for this setting based on the construction of hard-to-learn instances  for any number of agents, $n$. Our regret lower bound of $\Omega(\sqrt{K})$, over $K$ episodes, highlights the inherent learning difficulty in Dec-MASSPs. These insights clarify the learning complexity of decentralized control and can further guide the design of efficient learning algorithms in multi-agent systems.
\end{abstract}





% \begin{abstract}
%     \textcolor{red}{Goal Oriented}
%     Multi-agent systems are central to applications like swarm robotics and traffic routing, where agents must coordinate in a  decentralized fashion. While the stochastic shortest path (SSP) framework has been extensively studied in single-agent settings, the decentralized multi-agent variant remains largely unexplored. 
%     In this work, we establish the first regret lower bound for 
%     \textcolor{red}{the current lower bound holds for general MASSP} \textcolor{blue}{this change is not clear}decentralized multi-agent SSPs (\textcolor{red}{Dec-}MA-SSPs) 
%     with linear function approximation, showing that learning in these environments is inherently hard \textcolor{red}{what does this mean?}. \textcolor{blue}{based on my printout: we establish the first lower bound for model with linear apprx for both transition probabilities and policies. Our regret lower bound of $\Omega(\sqrt{K})$ matches the available upper bound and thus shows  that learning in multi-agent SSPs is inherently hard}. Our result 
%     \textcolor{red}{this work} 
%     provides an $\Omega(\sqrt{K})$ lower bound, matching existing 
%     \textcolor{red}{should we mention it ?} 
%     upper bounds, and introduces novel symmetry-based techniques to analyze the structure of optimal policies. This work lays the foundation for understanding the learning complexity of decentralized planning and guides future algorithmic developments in multi-agent systems. \textcolor{blue}{can further guide ... }
% \end{abstract}

==> Sections/1_intro.tex <==
\section{Introduction}
\label{sec:intro}




The Stochastic Shortest Path (SSP) problem is a foundational model for goal-oriented decision-making under uncertainty, extending classical shortest path formulations by incorporating stochastic transitions and random costs \cite{berttsit, bertsekas2012dynamic}. It serves as a core abstraction in many areas, including robotics, automated planning and reinforcement learning.  While planning in fully known SSPs is well understood \cite{bertsekas_nlp}, the focus has increasingly shifted to the learning setting, where the agent must learn the optimal policy through interaction with the environment. The quality of learning algorithms is typically measured using the notion of regret, which quantifies the difference between the cost incurred by following a learning algorithm and the unknown optimal policy \cite{jaksch2010near,auer2006logarithmic,auer2002nonstochastic}.


Given its broad applicability, the problem of learning optimal policies in tabular SSP environments has garnered significant attention, leading to algorithms with optimal or near-optimal regret guarantees \cite{tarbouriech2020no, rosenberg2020near, tarbouriech2021stochastic, cohen2021minimax}.
However, in many real-world applications, the state and action spaces are exponentially large, making tabular approaches computationally infeasible. To overcome this, recent works has assumed linear structure in the cost function or transition dynamics \cite{yang2019sample,min2022learning,vial2022regret}. These approaches have led to algorithms that achieve sublinear regret in SSPs with both known or unknown cost settings, along with tight upper and lower bounds on regret \cite{tarbouriech2020no, rosenberg2020near, cohen2021minimax, min2022learning, vial2022regret}, making the single-agent SSP well understood.

Despite significant progress in SSP, many real-world applications such as robotics, traffic routing, and distributed control naturally involve multiple agents interacting in a shared environment \cite{giel, ota, anton, linkai}.
These multi-agent systems are often decentralized, meaning agents cannot or choose not to share private information (e.g., their actions or incurred costs). However, they can exchange certain parameters (e.g., cost or transition estimates) over a predefined communication graph. 
% 
Motivated by this,  \cite{trivedi2023massp}  introduced the decentralized multi-agent stochastic shortest path (Dec-MASSP) problem with linear function approximations, where both transition dynamics and costs are modeled using linear function approximations. They propose a learning algorithm and report a sub-linear regret upper bound 
of $\widetilde{O}(B^{*1.5}d\sqrt{nK / c_{\min}})$, where $n$ is the number of agents, $K$ is the number of episodes, $d$ is the feature dimension, $B^*$ is the maximum expected cost-to-go, and $c_{\min} > 0$ is a lower bound on per-period cost. 
While this result provides the first regret guarantee for Dec-MASSPs, the optimality of their algorithm remains an open question.
This leads us to a central question:

\emph{What are the fundamental limits of learning in Dec-MASSPs with linear function approximations?}

To address this question, we establish tight regret lower bounds for the decentralized MASSP setting by constructing hard-to-learn instances. Extending single-agent SSP lower bound techniques \cite{min2022learning, rosenberg2020near} to decentralized MASSPs presents several key challenges, which we overcome using novel methods.

(i) \textbf{Exponential state-action space.} Even with just two nodes in the network, the global state space grows as $2^n$ with the number of agents $n$, which complicates both instance construction and lower bound analysis. 
To address this in the linear setting, we introduce a novel feature design for the transition probabilities specific to our MASSP instances. 
These features lead to a valid transition probability distribution and can serve as a foundational approach for feature design in other decentralized multi-agent reinforcement learning (MARL) applications.


(ii) \textbf{Coupled costs and dynamics.} In the MASSP setting, both transition probabilities and cost functions are inherently coupled across agents, depending on the global state-action space. To construct hard-to-learn instances and establish a meaningful regret lower bound, we first demonstrate that it suffices to restrict to uniform cost. We derive closed-form expressions for the transition probabilities using our novel feature design. This explicit formulation allows us to identify the structure of optimal actions, making our approach both tractable and novel.

(iii) \textbf{Intractable value functions.}  Unlike the single-agent setting with two nodes \cite{min2022learning}, where a closed-form expression for the optimal value function can be derived, obtaining a similar expression in  multi-agent system is significantly challenging due to the exponential state space.
To address this, we observe that the state space can be partitioned   based on the number of agents present at each node. This key insight allows us to establish a monotonicity property of the value function, which in turn is sufficient to derive regret lower bounds without requiring its explicit closed-form.

(iv) \textbf{Bounding KL divergence.}  A standard approach for deriving regret lower bounds relies on information-theoretic techniques, particularly bounding the Kullback–Leibler (KL) divergence between two  distributions. 
In the SSP setting \cite{min2022learning}, the KL divergence reduces to just two analytically tractable terms. 
However, in the MASSP setting, the KL divergence involves an exponential number of terms,  making exact analysis intractable. To overcome this, we exploit the non-negativity of the KL divergence and leverage the symmetry in our problem instances, which allows us to bound the KL divergence 
efficiently depending on the number of agents present at each node. 

% However, in our MASSP setting, there are an exponential number of such terms, each of which is hard to simplify. To overcome this, we use the non-negativity property of KL divergence, along with the symmetry in our instances, which allows us to bound the KL divergence 
% efficiently depending on the number of agents present at each node. 

% despite the complexity and large number of terms.

Building on the challenges outlined above and the novel methods we use to address them, we now summarize the major contributions of our work.
\begin{itemize}[left=5pt]
    \item \textbf{Regret lower bounds:} We establish the first $\Omega(\sqrt{K})$ regret lower bound for decentralized MASSPs under linear function approximation, which matches the previously reported upper bounds up to constant and poly-logarithmic factors \cite{trivedi2023massp}, thereby providing a precise characterization of the fundamental limits of learning in these settings. Notably, our result also recovers the lower bound of \cite{min2022learning} as a special case of $n=1$, which matches the corresponding upper bound.
    
    \item \textbf{Design of hard-to-learn MASSP instances:} The above regret bound is based on a proposed family of decentralized MASSP instances with linearly parameterized costs and transitions that are provably hard-to-learn.
    As scalability with $n$ is a key factor in evaluating the efficiency 
    of MARL algorithms,  our increasingly hard-to-learn instances (with respect to $n$) offer a valuable insights for assessing the performance of such algorithms. 

    % \textcolor{blue}{we can flip these 2, after rewording}
% 
    
 
    \item \textbf{First  analysis of instances with exponential state-action space}: Our lower bound analysis is the first to  handle the  exponential state and action space in MASSP settings. These lower bounds are based on the identification of the optimal policies and value functions in two-node MASSPs. These optimal policies have the  same optimal value for all the states with  identical number of agents at each node. 
\end{itemize}



\subsection{Related work}
\label{subsec:relatedwork}

\textbf{Stochastic shortest path (SSP) problems and learning in tabular setting.}
The stochastic shortest path (SSP) problem is a classical framework introduced in early work by \cite{eaton}. \cite{berttsit} later extended deterministic shortest path theory to stochastic environments, formalizing the SSP setting within dynamic programming. More recently, the focus has shifted toward learning in SSPs under unknown dynamics, in the tabular settings. 
\cite{tarbouriech2020no} introduced UC-SSP, the first no-regret algorithm for tabular SSPs, with regret $\widetilde{O}(DS\sqrt{ADK/c_{\min}})$, where $D$ is the expected hitting time and $c_{\min}$ the minimum cost, $S$ and $A$ denote the cardinality of state and action space and $K$ is the number of episodes. Follow-up work by \cite{rosenberg2020near} improved this bound by removing the $c_{\min}$ dependence and give a lower bound of $\Omega(B^*\sqrt{SAK})$, where $B^*$ captures the maximum cost-to-go, showing near-optimality.
\cite{tarbouriech2021stochastic} further refined SSP learning through EP-SSP, a model-based algorithm with regret $\widetilde{O}(B^*\sqrt{SAK})$, that doesn't require prior knowledge of $B^*$.  \cite{cohen2021minimax} introduced a minimax-optimal algorithm under stochastic  costs with matching bounds by reducing the SSP to a finite-horizon MDP. 

\textbf{Function approximation in SSPs.}
To address scalability beyond the tabular regime, recent efforts have explored SSPs under linear function approximation. \cite{vial2022regret} designed a model-free algorithm with sub-linear regret and is computationally efficient under minimal assumptions, using stationary policies. 
Parallelly, \cite{min2022learning}  proposed two algorithms, each based on Hoeffding-type and Bernstien-type sets. The Bernstien-type confidence set based algorithm has a better regret upper bound  $\widetilde{O}(dB^*\sqrt{K/c_{\min}})$. Additionally, the paper provides a lower bound $\Omega(dB^*\sqrt{K})$ in this setting.


\textbf{Decentralized multi-agent SSP.}
The extension of SSP learning to decentralized multi-agent systems is still in its early stages. Trivedi et al. \cite{trivedi2023massp} introduced the MASSP framework with linearly parameterized costs and transitions, and proposed MACCM, a decentralized algorithm with a reported regret upper bound of $\widetilde{O}(B^{*1.5}d\sqrt{nK / c_{\min}})$, where $n$ is the number of agents. However, their work does not establish any lower bounds, leaving open the fundamental question of the inherent difficulty and optimal regret rates for decentralized MASSP learning. We close this gap by establishing the first regret lower bounds for decentralized MASSPs (with any number of agents) with linear structure.
% 
\begin{table}[h]
\centering
\setlength{\tabcolsep}{15pt}
% \renewcommand{\arraystretch}{1.15}
\small
\begin{tabular}{lcccccc}
\toprule
\textbf{Reference}  & \textbf{Setting} & \textbf{LFA} & \textbf{Upper Bound} & \textbf{Lower Bound}  
\\
\midrule
\cite{tarbouriech2020no} 
% Tarbouriech et al. (2020) 
& $\bullet$   & \xmark & $\widetilde{O}(DS\sqrt{ADK})$ & -- 
\\
\cite{rosenberg2020near} 
% Rosenberg et al. (2020)  
& $\bullet$ & \xmark & $\widetilde{O}(B^*S\sqrt{AK})$ & $\Omega(B^*\sqrt{SAK})$ \\
\cite{cohen2021minimax} 
% Cohen et al. (2021) 
for $B^*>1 $& $\bullet$  & \xmark & $\widetilde{O}(B^*\sqrt{SAK})$ & -- 
\\
\cite{cohen2021minimax} 
% Cohen et al. (2021)
for $B^*<1$& $\bullet$  & \xmark & $\widetilde{O}(\sqrt{B^*SAK})$ & $\Omega(\sqrt{B^*SAK})$
\\
\cite{min2022learning}
% Min et al. (2022)  
& $\star$ & \cmark & $\widetilde{O}(dB^*\sqrt{K})$ & $\Omega(dB^*\sqrt{K})$
\\
\cite{vial2022regret} 
% Vial et al. (2022)
& $\star$ & \cmark & $\widetilde{O}(dB^*\sqrt{d{B^*}K})$ & --
\\
\midrule \midrule
% \cite{zhang2021decentralized} & \cmark & \cmark & \cmark & Convergence only & \xmark & MARL (ergodic MDPs) 
% \\
\cite{trivedi2023massp}
% Trivedi and Hemachandra (2023)  
& $\ddagger$ & \cmark & $\widetilde{O}(B^{*1.5}d\sqrt{nK})$ &  -- 
\\
\textbf{This work} & $\ddagger$ & \cmark & --  & $\Omega(\sqrt{K})$ 
\\
\toprule
\end{tabular}
\caption{Comparison of related work in SSP learning and decentralized multi-agent SSPs. LFA refers to linear function approximation. Here 
$S$ and $A$ denote the number of states and actions, respectively; 
$K$ is the number of episodes; $B^*$ is the SSP diameter; and 
$D$ is the expected hitting time. Symbols: $\bullet$ = tabular SSP, $\star$ = linear mixture SSP, $\ddagger$ = decentralized MA-SSP. }
\label{tab:comparison}
\end{table}
% 
% \textbf{Related Work in Decentralized MARL.}
% More broadly, decentralized multi-agent reinforcement learning (MARL) under function approximation has been studied in contexts beyond SSPs. For instance, \cite{zhang2021decentralized} proposed fully decentralized actor-critic algorithms with convergence guarantees when value functions are linearly approximated. However, these results pertain to ergodic or discounted MDPs and do not address the unique structural challenges of goal-directed, episodic SSPs. \pt{This can be combined in previous sections.} \textcolor{red}{i think its ok but we need to stress  somewhere that SSP === total reward undiscounted MDP \cite{puterman2014markov, bertsekas2012dynamic}}
% ....
% 
% \begin{table}[h]
% \centering
% \setlength{\tabcolsep}{2pt}
% % \renewcommand{\arraystretch}{1.5}
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Work} & \textbf{Multi-agent} & \textbf{Decentralized} & \textbf{Linear Approx.} & \textbf{Regret Upper Bound} & \textbf{Regret Lower Bound} & \textbf{Setting} \\
% \midrule
% \cite{tarbouriech2020no} & No & No & No & $\widetilde{O}(DS\sqrt{ADK/c_{\min}})$ & No & Tabular SSP \\
% \cite{rosenberg2020near} & No & No & No & $\widetilde{O}(B^*S\sqrt{AK})$ & $\Omega(B^*\sqrt{SAK})$ & Tabular SSP \\
% \cite{cohen2021minimax} & No & No & No & $\widetilde{O}(B^*\sqrt{SAK})$ & Yes & Tabular SSP with stochastic costs \\
% \cite{min2022learning} & No & No & Yes & $\widetilde{O}(dB^*\sqrt{K/c_{\min}})$ & $\Omega(dB^*\sqrt{K})$ & Linear SSP \\
% \cite{vial2022regret} & No & No & Yes & Sublinear (stationary) & No & Linear SSP \\
% \cite{trivedi2023massp} & Yes & Yes & Yes & $\widetilde{O}(B^{*1.5}d\sqrt{nK/c_{\min}})$ & No & Decentralized MASSP \\
% \cite{zhang2021decentralized} & Yes & Yes & Yes & Convergence only & No & MARL (ergodic MDPs) \\
% \textbf{This work} & Yes & Yes & Yes & --- & $\Omega(\sqrt{K})$ & Decentralized MASSP \\
% \bottomrule
% \end{tabular}
% \caption{Comparison of related works in SSP learning and decentralized RL. Our work uniquely establishes regret lower bounds for decentralized multi-agent SSPs under linear approximation.}
% \label{tab:comparison}
% \end{table}
% \begin{table}[h]
% \centering
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Work} & \textbf{Multi-} & \textbf{Decen-} & \textbf{Linear} & \textbf{Regret Upper} & \textbf{Regret Lower} & \textbf{Setting} \\
% & \textbf{agent} & \textbf{tralized} & \textbf{Approx.} & \textbf{Bound} & \textbf{Bound} & \\
% \midrule
% \cite{tarbouriech2020no}       & \xmark & \xmark & \xmark & $\widetilde{O}(DS\sqrt{ADK/c_{\min}})$ & \xmark & Tabular SSP \\
% \cite{rosenberg2020near}       & \xmark & \xmark & \xmark & $\widetilde{O}(B^*S\sqrt{AK})$ & $\Omega(B^*\sqrt{SAK})$ & Tabular SSP \\
% \cite{cohen2021minimax}        & \xmark & \xmark & \xmark & $\widetilde{O}(B^*\sqrt{SAK})$ & \cmark & Tabular SSP w/ stochastic costs \\
% \cite{min2022learning}         & \xmark & \xmark & \cmark & $\widetilde{O}(dB^*\sqrt{K/c_{\min}})$ & $\Omega(dB^*\sqrt{K})$ & Linear SSP \\
% \cite{vial2022regret}          & \xmark & \xmark & \cmark & Sublinear (stationary) & \xmark & Linear SSP \\
% \cite{trivedi2023massp}        & \cmark & \cmark & \cmark & $\widetilde{O}(B^{*1.5}d\sqrt{nK/c_{\min}})$ & \xmark & Decentralized MASSP \\
% \cite{zhang2021decentralized}  & \cmark & \cmark & \cmark & Convergence only & \xmark & MARL (ergodic MDPs) \\
% \textbf{This work}              & \cmark & \cmark & \cmark & --- & $\Omega(\sqrt{K})$ & Decentralized MASSP \\
% \bottomrule
% \end{tabular}
% \caption{Comparison of related works in SSP learning and decentralized RL. Our work uniquely establishes regret lower bounds for decentralized multi-agent SSPs under linear approximation.}
% \label{tab:comparison}
% \end{table}




==> Sections/2_prelims.tex <==
\section{Preliminaries and problem formulation} 
\label{sec:problem}
% 
In this section, we introduce the Multi-Agent Stochastic Shortest Path (MASSP) problem, and also present the formal setup and notations that underpin the decentralized learning framework. 
% 
\subsection{Notations and preliminaries}
\label{subsec:prelims}
% 
A MASSP problem is defined by the tuple $(\mathcal{V}, \mathcal{N}, \mathbb{P}, \mathcal{A})$, where $\mathcal{V} = \{v_1, v_2, \dots, v_q \}$ is the set of nodes and $\mathcal{N} = \{ 1, 2, \dots, n \}$
is the set of agents.
Each agent occupies exactly one node at any given time, leading to a global system state $\tb{\ti{s}} = (s_1, s_2, \dots, s_n)$ in the global state space $\mathcal{S} = \mathcal{V}^n$, so $| \mathcal{S} | = q^n$.  
 We assume that all agents start at the same node $s$ and aim to reach the common goal node $g$, resulting in initial and goal states $\tb{\ti{s}}_{\init} = (s, \dots, s)$ and $\tb{\ti{g}} = (g, \dots, g)$, respectively.
% Our analysis can be easily extended to scenarios where agents begin and end at different nodes. 
Each agent $i \in \mathcal{N}$ has a finite action space $\mathcal{A}_i$ at every node, leading to a joint action $\tb{\ti{a}} = (a_1, \dots, a_n) \in \mathcal{A} = \mathcal{A}_1 \times \cdots \times \mathcal{A}_n$. 
Once an action $\tb{\ti{a}}$  is taken in the state 
$\tb{\ti{s}}$, the system evolves to next state $\tb{\ti{s}}'$ according to a Markovian transition kernel $\mathbb{P}(\cdot \mid \tb{\ti{s}}, \tb{\ti{a}})$ and each agent $i\in \mathcal{N}$ incurs an instantaneous cost $c_i(\tb{\ti{s}}, \tb{\ti{a}}) \in [c_{\min}, 1]$, where $c_{\min} > 0$. 

The cost function $c_i(\tb{\ti{s}}, \tb{\ti{a}})$ captures complex dependencies of individual costs on both the positions and actions of all agents. For example, the cost can be modeled by taking  $c_i(\tb{\ti{s}}, \tb{\ti{a}}) = x_i(\tb{\ti{s}}, \tb{\ti{a}}) \cdot K_i(\tb{\ti{s}}, \tb{\ti{a}})$ where $x_i(\tb{\ti{s}}, \tb{\ti{a}}) \coloneqq \sum_{j=1}^n \mathbbm{1}_{\{a_j = a_i\}}$ is the 
congestion (number of agents choosing the same action) and $K_i(\tb{\ti{s}}, \tb{\ti{a}})$ encodes the cost due to private efficiency and all other complex dependencies (except congestion). 
The global cost is defined as the average of individual costs: 
$c(\tb{\ti{s}}, \tb{\ti{a}}) = \frac{1}{n} \sum_{i=1}^n c_i(\tb{\ti{s}}, \tb{\ti{a}})$.

A stationary Markov deterministic policy is a mapping $\pi: \mathcal{S} \to \mathcal{A}$.
Given the stationary Markovian dynamics $\mathbb{P}$ and cost $c$, an optimal policy lies in the class $\Pi_{\mathrm{MD}}$ of Markov deterministic policies \cite{puterman2014markov}.
We further focus on the class of proper policies $\Pi_p \subseteq \Pi_{\mathrm{MD}}$, i.e., each agent reach the goal state $\tb{\ti{g}}$ from any initial state with probability one \cite{tarbouriech2020no, tarbouriech2021stochastic, cohen2021minimax, min2022learning}. 
Given any proper policy $\pi \in \Pi_p$, the value function (or cost-to-go function) is defined as   $V^\pi(\tb{\ti{s}}) = \mathbb{E} \left[ \sum_{t=1}^{\tau^\pi(\tb{\ti{s}})} c(\tb{\ti{s}}^t, \pi(\tb{\ti{s}}^t)) ~ \Big | ~ \tb{\ti{s}}^1 = \tb{\ti{s}} \right]$,
where the expectation is over all sample paths due to interaction of policy $\pi$ and transition kernel $\mathbb{P}$.
$\tau^\pi(\tb{\ti{s}})$ is the random time to reach the goal state $\tb{\ti{g}}$ under policy $\pi$ starting at $\tb{\ti{s}}$. 
The objective is to find a policy that minimizes the expected cumulative global cost from the initial state  $\tb{\ti{s}}_{\init}$  to the goal state $\tb{\ti{g}}$. The optimal value function with the corresponding optimal policy $\pi^*$ 
is thus 
\begin{align} 
\label{eqn:v_star}
    V^*(\tb{\ti{s}}) = \min_{\pi \in \Pi_p} V^\pi(\tb{\ti{s}}).
\end{align} 
We further define the diameter of MASSP as $B^* = \max_{\tb{\ti{s}}\in \mathcal{S}} V^*(\tb{\ti{s}})$.

% 
\subsection{Problem formulation}
\label{subsec:problem_formulation}
% 
When transition kernel $\mathbb{P}$ and cost $c(\cdot, \cdot)$ are known, the objective of MASSP problem is to find an optimal policy in the space of proper policies, as in Equation~\eqref{eqn:v_star}.
However, in the learning setting with unknown transition kernel $\mathbb{P}$ or cost $c(\cdot, \cdot)$, agents must actively \emph{explore} to learn an optimal policy. Though the goal is to minimize the cumulative global cost to reach $\tb{\ti{g}}$, agents in our setup act independently and lack knowledge of others' actions or costs.
% 
A natural solution is to employ a central controller that aggregates signals from all agents to coordinate learning \cite{zhang2019multi}. 
However, such centralization poses several challenges: (i) poor scalability with the number of agents due to increased communication overhead \cite{cour} (ii) vulnerability to single-point failures and adversarial attacks \cite{zhang2018fully}, and (iii) privacy concerns, as agents may be unwilling to reveal their individual costs. 
These limitations motivate decentralized learning, where the agents do not explicitly share the actions or private costs among themselves via a central controller. This setting falls within the purview of Decentralized Multi-Agent Reinforcement Learning (Dec-MARL).

To make decentralized learning tractable, prior works (e.g., \cite{zhang2018fully, trivedi2022multi}) adopt linear cost approximations as $c(\tb{\ti{s}}, \tb{\ti{a}}) = \langle \psi(\tb{\ti{s}}, \tb{\ti{a}}), \tb{\ti{w}} \rangle$, where $\psi(\tb{\ti{s}}, \tb{\ti{a}}) \in \mathbb{R}^{nd}$ is a known feature map, and $\tb{\ti{w}} \in \mathbb{R}^{nd}$ is an unknown parameter, with $nd << |\mathcal{S}| |\mathcal{A}|$. 
This allows agents to coordinate via shared parameter estimates rather than raw cost values. Given the large state-action space, we also assume a linear model of transitions, commonly used in recent literature \cite{min2022learning, trivedi2023massp}.
% 
\begin{assumption} \label{assm:lfa_prob}
    For every pair $(\tb{\ti{s}},\tb{\ti{a}},\tb{\ti{s}}') \in \mathcal{S}\times\mathcal{A}\times\mathcal{S}$,  there exists known features $\phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \in \mathbb{R}^{nd}$ and unknown parameter $\theta \in \mathbb{R}^{nd}$ with $d\geq2$  such that $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) = \langle \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}),\theta \rangle$. 
\end{assumption}
%  
We design the features $\phi(\tb{\ti{s}}' | \tb{\ti{s}}, \tb{\ti{a}})$ specific to our setting in the next section. We refer to this setting as the Linear Mixture Multi-Agent Stochastic Shortest Path (LM-MASSP), which lays the foundation of our problem. 
% In LM-MASSP, agents interact with the environment over $K$ episodes, each beginning at $\tb{\ti{s}}_{\init}$ and ending upon reaching the goal state $\tb{\ti{g}}$.
Analogous to  \cite{osb,osband2016lower}, we define a general (possibly randomized) Dec-MARL algorithm as a sequence of deterministic functions
$\pi = \{\pi^t\}_{t=1}^\infty$, where at each time step $t$, the algorithm specifies a policy $\pi^t = (\pi^t_1, \dots, \pi^t_n)$. Here $\pi^t_i: \mathcal{H}^t_i \rightarrow \Delta(\mathcal{A}_i)$ maps the history observed by agent $i$ to a distribution over its action space $\mathcal{A}_i$, from which the agent samples its action.
% For deterministic decentralized algorithms, we have $\forall~(i, t)~,\pi^t_i \in ext(\Delta(\mathcal{A}_i))$, where $ext(.)$ is the extreme points of 
% As such an algorithm outputs an action for every history, its value can be analogously defined as in Equation \ref{eqn:v_star}.
% 
% If we \textcolor{blue}{to shorten much this sentence (well known fact) }restrict the , i.e., only assigning probability 1 to a single action per history  
% \textcolor{red}{Since we are commenting about an "dec-marl-algorithm", its important to define what we mean. So following existing literature, we define it (general randomized dec-marl-algo) as a sequence of functions $\{{\pi^t}\}_{t=1}^{\infty}$ for each time step from initial to infinity. At each time step we refer to corresponding function : at $t$ refer to $\pi^t$. Each of this $\pi^t$ is itself an $n-$ tuple of functions to be referred by each agent $n$. So, $\pi^t = (\pi^t_1,\pi^t_2,\dots, \pi^t_n)$. For every agent $i \in [n]$, $\pi^t_i$ looks at the history observed by this agent $i$ and suggests a probability distribution over this agent's action space. 
% Hence $\pi^t_i$ is a map from all agent $i$'s observable histories ($\mathcal{H}^i_t$) to the probability simplex $d^t_i(h^t_i)$over $i$'s action space (If we restrict to extreme points of this simplex, then for each history there's a particular action mapped. This would lead to deterministic algo definition). Now, given this distribution $d^t_i(h^t_i)$ agent $i$ samples an action to chose in the current $t^{th}$ time step. Effectively if you look at it, algorithm is just a history dependent policy (for our case suitably modified for decentralisation).}
\paragraph{Performance criteria.} Let $(\tb{\ti{s}}^{k,h}, \tb{\ti{a}}^{k,h})$ denote the state-action pair encountered at step $h$ of episode $k$ under a given algorithm $\pi$ and model parameter $\theta$.  Let $h_k$ represent the (random) length of episode $k$. The expected cumulative regret after 
$K$ episodes is defined as
\begin{align} \label{eqn:regret_def}
    \mathbb{E}_{\theta,\pi}[R(K)] = \mathbb{E}_{\theta,\pi} \Bigg[ \sum_{k=1}^K \sum_{h=1}^{h_k} c(\tb{\ti{s}}^{k,h}, \tb{\ti{a}}^{k,h}) \Bigg] - K \cdot V^*(\tb{\ti{s}}_{\init}).
\end{align}
The above regret measures the difference between the total expected cost by following the algorithm $\pi$ instead of (unknown) optimal policy. A desirable algorithm achieves sublinear regret in $K$, indicating that it \emph{eventually} learns the optimal policy. 
In the setting described above, \cite{trivedi2023massp} propose an algorithm with expected cumulative regret $\widetilde{\mathcal{O}}(\sqrt{K})$.  
However, the optimality of this algorithm has not yet been established 
% \textcolor{red}{line repeating exactly from intro so can be compressed with the sentence before as "regret root K without establishing optimality.."}
raising questions such as: Are better learning algorithms possible in this setting? If so, in what aspects can they improve compared to the existing  ones? 
To answer these questions, it is essential to derive tight regret lower bounds. 
Hence, we construct hard-to-learn instances with tractable optimal policies and analyze the regret of any algorithm. 
Following \cite{auer2002nonstochastic}, we consider deterministic algorithms, though similar analysis can be extended to randomized algorithms.
% Thus, in this work, we restrict to deterministic policies. \textcolor{red}{last line is not needed}
% 
% 
% 
% The construction of hard instances and detailed proof strategy is developed in the subsequent sections.
% 
% ...
% When the costs and transition probabilities are known, the MASSP problem is to search the optimal policy as in \eqref{eqn:v_star}. When either of them is unknown, the agents must explore the actions and eventually learn the best policy. This is the MASSP learning problem we study. Particularly, in our setting, we assume that the costs and the transition probabilities are both not known to any agent. 
% Recall that the best policy minimizes the expected cumulative global cost to reach $\tb{\ti{g}}$ and not just the cost of any single agent. However, any agent independently makes decision but is unaware of the actions and costs of other agents. A global objective cannot be met unless information is shared. 
% Thus, the objective as given in Equation \eqref{eqn:v_star} could be achieved by having a central controller who may coordinate with the agents by receiving the actions and the cost signals from each agent. 
% However, there are certain problems with this approach: (i) It significantly increases computation and transmission costs for higher number of agents and is thus unscalable. (ii) Centralization of all information makes the system prone to malicious attacks \cite{zhang2018fully}. (iii) Further, the agents may be unwilling to share their individual costs due to privacy concerns. 
% Hence a mechanism that ensures agents learn the best policy independently (without explicit sharing of costs and actions) is desirable which takes us into the purview of Decentralized Multi-Agent Reinforcement Learning. 
% 
% Many existing works in Decentralized MARL (\cite{zhang2018fully,trivedi2023massp}) assume linear parametrization of costs i.e., for all $(\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S} \times \mathcal{A}$,
% there exist known features $\psi(\tb{\ti{s}},\tb{\ti{a}}) \in \mathbb{R}^{nd}$ and an unknown parameter $\tb{\ti{w}} \in \mathbb{R}^{nd}$ for the instance such that 
% % 
% \begin{align} \label{eqn:cost_param}
%     \mathbb{E}[c(\tb{\ti{s}},\tb{\ti{a}})]=\langle \psi(\tb{\ti{s}},\tb{\ti{a}}),\tb{\ti{w}} \rangle, \quad \forall ~~ (\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S} \times \mathcal{A}.
% \end{align}
% % 
% Hence, instead of sharing actual costs, agents can now share their estimates of the unknown parameter.
% 
% Further, since the state and action space is explosively large, we assume the following linear function approximation of transition probabilities common in this line of literature (\cite{min2022learning}; \cite{trivedi2023massp}) to hold:
% \begin{assumption} \label{assm:lfa_prob}
%     For every pair $(\tb{\ti{s}},\tb{\ti{a}},\tb{\ti{s}}') \in \mathcal{S}\times\mathcal{A}\times\mathcal{S}$,  there exists known features $\phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \in \mathbb{R}^{nd}$ and unknown $\theta \in \mathbb{R}^{nd}$ such that, for any $\tb{\ti{s}}' \in \mathcal{S}$, $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) = \langle \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}),\theta \rangle$. 
% \end{assumption}
% 
% Due to the above linear function approximations of costs and the transition probabilities, we refer to these settings as Linear Mixture - Multi-Agent Stochastic Shortest Path (LM -MASSPs). 
% We will now describe the problem we are solving in the LM-MASSP domain.



==> Sections/3_approach.tex <==
\section{Our approach}
\label{sec:approach}
% 
In this section, we construct a family of provably hard instances for LM-MASSP. These are designed so that the optimal policy is analytically tractable, where any deviation leads to measurable regret.
% 
% \pt{I am thinking to modify the entire section  as follows - let me know if this makes sense - define each component of the (V, S, A, P) -- While defining the transition probability -- we can give the feature design -- and then define the cost -- and the remark therein -- write the instance defintion -- because now we have all the terms defined. Then i think, we can make the sub-section where we give the lemma 2 -- etc. and while writing the lemma 2, we should define the sets Sr, I, J, etc.... This implies there will not be subsection called Features. Rather we have another subsection. }

\subsection{Construction of hard-to-learn LM-MASSP instances}
\label{subsec:problem_instance}
% 
We consider a minimal yet expressive network with only two nodes: $\mathcal{V} = \{s, g \}$ with $n$ agents. This induces a global state space $\mathcal{S} = \{ s, g \}^n$ of size $|\mathcal{S}| = 2^n$, where any agent can either be at $s$ or $g$. 
We fix the initial state as $\tb{\ti{s}}_{\init} = (s, s, \dots, s)$ and the goal state as $\tb{\ti{g}} = (g, g, \dots, g)$. We assume that once an agent reaches node $g$, it is impossible to go back to node $s$.  Each agent $i \in [n]$ has the same action set $\mathcal{A}_i = \{-1, 1\}^{d-1}$, for some $d \geq 2$. 
Consequently, the global action space is $\mathcal{A} = \{-1, 1\}^{n(d-1)}$ with $|\mathcal{A}| = 2^{n(d-1)}$. 
We parameterize transition probabilities according to Assumption \ref{assm:lfa_prob}. 
Next, we define the valid features $\phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}})$, which may be of independent interest to the MARL community, as it offers practical guidance for designing valid feature representations\footnote{While there are many possible ways to design the features, any valid feature construction must satisfy the conditions specified in Lemma~\ref{lemma:valid_features} below.}.  
% Note that there can be many possible feature designs, but all of them must satisfy the following requirements to produce valid transition probabilities in any of our instances.
% 
\begin{equation}
\label{eqn:features_global_new}
    \phi(\tb{\ti{s}}' \mid \tb{\ti{s}}, \tb{\ti{a}}) = 
    \begin{cases} 
    \left(\phi_1(s'_1|s_1,a_1),\dots, \phi_n(s'_n|s_n,a_n) \right), & \text{if } \tb{\ti{s}} \neq \tb{\ti{g}} \text{ and } s^{\prime}_i = g \text{ if } s_i = g ~ \forall~ i \in [n] 
    \\
    \mathbf{0}_{nd}, & \text{if } ~ s_i = g,~ s^{\prime}_i = s ~ \text{for any} ~ i \in [n]
    \\
    (\mathbf{0}_{nd-1}, 1), & \text{if } \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}' = \tb{\ti{g}}
    \end{cases}
\end{equation}
% 
where for every  agent $i\in \mathcal{N}$ the feature map $\phi_i(s'_i \mid s_i, a_i)$ is defined as follows
% 
\begin{equation}
\label{eqn:individual_features}
    \phi_i(s^{\prime}_i | s_i, {{a}}_i) = \begin{cases}  
    \left(-{{a}}_i, \frac{1-\delta}{n \cdot 2^{r-1}} \right)^{\top}, & \text{if} ~ {s}_i = s^{\prime}_{i} = s
    \\
    \left({{a}}_i, \frac{\delta}{n \cdot 2^{r-1}} \right)^{\top}, & \text{if} ~ {s}_i = s,~s^{\prime}_{i} = g
    \\
    \left(\mathbf{0}_{d-1}, \frac{1}{n \cdot 2^{r}} \right)^{\top}, & \text{if} ~ {s}_i = g,~ s^{\prime}_{i} = g.
    \end{cases}
\end{equation}
% 
In the above, $r$ denotes the number of agents at node $s$ in the current global state $\tb{\ti{s}} \in \mathcal{S}$. The parameters $\delta$ and $\Delta$ are chosen such that $\delta \in \left( \frac{2}{5}, \frac{1}{2} \right) ~ \text{and} ~ \Delta < 2^{-n} ( \frac{1 - 2\delta}{1 + n + n^2})$ (details are available in the next section).
Furthermore, the transition model is parameterized by a vector $\theta \in \mathbb{R}^{nd}$ of the form $ \theta = (\theta_1, 1, \theta_2, 1, \dots, \theta_n, 1)^{\top}$,
where each $\theta_i \in \left\{ -\frac{\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)} \right\}^{d-1}$. Let the set of all such $\theta$ be $\Theta$. Thus, $|\Theta| = 2^{n(d-1)}$. For any $i \in [n]$ and $p \in [d-1],$ we denote the $p^{th}$ component of $a_i \text{ and }\theta_i$ as $a_{i,p} \text{ and } \theta_{i,p}$, respectively.  
These parameters along with the features $\phi(.|.,.)$ define the transition probabilities as in assumption~\ref{assm:lfa_prob}. 
% W
% e denote the transition kernel of instance with parameter $\theta$ as $\mathbb{P}_{\theta}$.
Observe that the first case in Eqn \eqref{eqn:features_global_new} captures general transitions, the second captures disallowed transitions and the third corresponds to the only \emph{certain} transition.

% ....

% In the above, $r$ represents the number of agents at node $s$ in the current global state $\tb{\ti{s}}$, and $\delta$ and $\Delta$ are the parameters satisfying: $ \delta \in \left( \frac{2}{5} , \frac{1}{2} \right)$ and $\Delta < 2^{-n} \cdot \frac{1-2\delta}{1+n+n^2}$.
% Further $\theta$ is an $nd$- dimensional vector of the form $\theta = (\theta_1,1, \theta_2,1,\dots,\theta_n,1) \in \Theta$ \textcolor{red}{need to define $\Theta$ properly} used to define the transition probability as in Assumption \ref{assm:lfa_prob}, where for each agent $i \in [n]$, each component of the parameter $\theta_i \in \mathbb{R}^{d-1}$ takes one of the two values $\left\{-\frac{\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)} \right\}$. 
% Observe that Eqn \eqref{eqn:features_global_new} the first case corresponds to the most general transitions that are allowed, the second case represents all impossible transitions and the third case takes care of the only \textit{certain} transition.

\textbf{Instances.} With the above construction, we define hard-to-learn LM-MASSP instances by varying key problem parameters while maintaining analytical tractability of the optimal policy. In particular, we define each instance by a fixed tuple $(n,\delta, \Delta, \theta)$ as defined above. 
% 
\begin{restatable*}{lem}{featuresvalid}
% \begin{lemma}
\label{lemma:valid_features}
For any instance $(n,\delta,\Delta,\theta)$, features defined in Equation \eqref{eqn:features_global_new} , \eqref{eqn:individual_features} yield a valid transition probabilities, i.e., 
\begin{enumerate}[left=5pt]
    \item 
    % \textcolor{red}{need to change due to $s'$} 
    For any $\theta$, we have,  $\langle \phi(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}), \theta \rangle \geq 0 ~ \forall ~ (\tb{\ti{s}}, \tb{\ti{a}}, \tb{\ti{s}}')$ and $\sum_{\tb{\ti{s}}' \in \mathcal{S}} \langle \phi(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}), \theta \rangle = 1 ~ \forall ~ (\tb{\ti{s}}, \tb{\ti{a}}) $.
    \item For any $(\tb{\ti{s}}, \tb{\ti{a}}) $, if transition to $\tb{\ti{s}}'$ is impossible, we have $\langle \phi(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}), \theta \rangle = 0$; on the other hand, if the transition is certain, then $\langle \phi(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}), \theta \rangle = 1$.
\end{enumerate}
% 
\end{restatable*}
% 
The detailed proof of this lemma is given in Appendix~\ref{proof:lemma_valid_features}. Analysis of a general SSP instance is complicated due to trade-offs between policies that quickly reach the goal state (minimizing time) and those that take longer but are cost-efficient \cite{tarbouriech2020no}. These make optimal policies, in general, intractable.
To avoid this, we adopt a uniform cost structure i.e., $\forall ~\tb{\ti{a}}, c(\tb{\ti{s}}, \tb{\ti{a}}) = 1 ~\forall~\tb{\ti{s}} \ne \tb{\ti{g}}$ and $c(\tb{\ti{g}}, \tb{\ti{a}}) = 0$. Thus, the optimal policy is the one that minimizes the expected time to reach goal and depends only on transition dynamics. 
Note that the above cost structure is not merely hypothetical; in our instance design, for all $i \in [n]$, $\tb{\ti{a}} \in \mathcal{A}$, and $\tb{\ti{s}} \ne \tb{\ti{g}}$, we  define $K^i(\tb{\ti{s}}, \tb{\ti{a}}) = \frac{1}{x_i(\tb{\ti{s}}, \tb{\ti{a}})}$ and set $K^i(\tb{\ti{g}}, \tb{\ti{a}}) = 0$. 
% ...

% The detailed proof is deferred to Appendix \ref{proof:lemma:valid_features}. Now, there is one more complication in the instance defined above \textcolor{red}{true for any instance in general}.  We present this issue in the following remark.  
% % 
% \begin{remark}
% For a general cost and transition probability function, there may in general be a trade-off between policies that moves towards the goal state quickly (i.e.,  minimizing the number of time steps to reach the goal) and the policies that take more time but may (in an overall sense) be cost efficient \cite{tarbouriech2020no}. 
% \end{remark}
% % 
% Such complications lead to intractability of optimal policies. To avoid this in the analysis of our instances, we let for all $\tb{\ti{s}} \in \mathcal{S}\backslash\{\tb{\ti{g}}\}$ and $\tb{\ti{a}} \in \mathcal{A}$, $c(\tb{\ti{s}},\tb{\ti{a}}) = 1$ while for any $\tb{a} \in \mathcal{A}, c(\tb{\ti{g}}, \tb{\ti{a}}) =0$. Hence, \textcolor{red}{between two policies,} the policy \textcolor{red}{one} that takes us \emph{closer} to goal state is better \textcolor{red}{than the other}. This leads to optimal policy being directly influenced by transition probabilities alone. To convince that we are not considering impossible instances, we have the following:
% \begin{remark} \label{rem:cost_one}
%     One class of such instances is the one for whom for all $i \in [n], \tb{\ti{a}} \in \mathcal{A}, K^i(\tb{\ti{s}},\tb{\ti{a}}) = \frac{1}{x_i(\tb{\ti{s}},\tb{\ti{a}})}$ for all $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$ and $ K^i(\tb{\ti{g}},\tb{\ti{a}}) = 0$ in Eqn \eqref{eqn:ind_cost}. 
% \end{remark}







% For our instances, we consider the following feature design
% 




% To simplify the dynamics, we assume that once an agent reaches node $g$, it remains there permanently. 
% That is, transitions such as $\tb{\ti{s}} = (s, s, \dots, g, g) \rightarrow \tb{\ti{s}}' = (s, s, \dots, g, s)$ are infeasible.










% \pt{partitioning of the state space- -- we partition the state space based on r, the number of agents at the state s. $\mathcal{S}_r$ -- of type r... $\mathcal{S}(s)$ -- reachable from $s$. $\mathcal{S}_r(s)$ -- reachable from s of type r. }


\subsection{Transition probabilities } 
\label{subsec:general_tp}
% 
Using above features and transition model in Assumption \ref{assm:lfa_prob}, we now derive a general expression for transition probabilities for any instance $(n, \delta, \Delta, \theta)$ in the  lemma below. We partition the state space $\mathcal{S}$ based on the number of agents at node $s$. 
Let $\mathcal{S}_r$ be the subset of state space with $r$ agents at node $s$, i.e., 
$
\mathcal{S}_r \coloneqq \big\{ (s_1,s_2,\dots,s_n) \in \mathcal{S} : \sum_{i\in \mathcal{N}} \mathbbm{1}_{\{s_i = s\}} = r \big\}.
$
For any $r \in \{0\} \cup [n]$, we say that a state $\tb{\ti{s}}$ is of \emph{type} $r$ if $\tb{\ti{s}} \in \mathcal{S}_r$. 
Clearly, $\cup_{r=0}^n \mathcal{S}_r = \mathcal{S}$ and $\mathcal{S}_{r_1} \cap \mathcal{S}_{r_2} = \emptyset$ for any $r_1 \neq  r_2$. Thus,  $\{ \mathcal{S}_0, \mathcal{S}_1, \dots, \mathcal{S}_n \}$ partitions $\mathcal{S}$. Further, for any $\tb{\ti{s}}$, we define $\mathcal{S}(\tb{\ti{s}}) \coloneqq \{ \tb{\ti{s}}' \in \mathcal{S} : \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) >0, ~~ \text{for some}~ \tb{\ti{a}} \in \mathcal{A} \}$ as the set of all states that are \emph{reachable} from $\tb{\ti{s}}$ in the next step.
Also let  $\mathcal{S}_r(\tb{\ti{s}})$ be the set of all states of \emph{type} $r$ that are \emph{reachable} in the next step from $\tb{\ti{s}}$, i.e., $\mathcal{S}_r(\tb{\ti{s}}) \coloneqq \mathcal{S}_r \cap \mathcal{S} (\tb{\ti{s}})$. 

% To analyze any transition, say $\tb{\tb{s}} \rightarrow \tb{\ti{s}}'$ where $\tb{\ti{s}} \in \mathcal{S}_r$ and $\tb{\ti{s}}' \in \mathcal{S}_{r'}$,  we define context dependent sets of agents - $\mathcal{I}\coloneqq\{i_1,i_2,\dots,i_r\}$ as the set of agents at node $s$ in state $\tb{\ti{s}}$, $\mathcal{J} \coloneqq \{j_1,j_2,\dots,j_{n-r}\}$ as the set of agents already at node $g$ in state $\tb{\ti{s}}$ and $\mathcal{T} \coloneqq \{t_1,t_2,\dots, t_{r-r'}\} \subseteq\mathcal{I}$ as the set of agents that move from node $s$ to node $g$ as the global state of the system changes from $\tb{\ti{s}}$ to $\tb{\ti{s}}'$. Note that we say these are context-dependent since $\mathcal{I}, \mathcal{J}$ varies for various $\tb{\ti{s}}$ and $\mathcal{T}$ varies for various $\tb{\ti{s}}, \tb{\ti{s}}'$. Thus we are abusing the notation here a little to avoid notational overhead and the sets must more precisely be denoted as $\mathcal{I}_{\tb{\ti{s}}}, \mathcal{J_{\tb{\ti{s}}'}}$ and $\mathcal{T}_{\tb{\ti{s}}, \tb{\ti{s}}'}$.
% \pt{Thinking to remove this entire thing upto corollary 1 from main paper. while just adding the details about the $a_\theta$}
% 
\begin{restatable*}{lem}{genprob}
\label{lemma:general_tp} 
% 
For a given state $\tb{\ti{s}} \in \mathcal{S} \setminus {\tb{\ti{g}}}$, let $\mathcal{I}$ denote the set of agents at node $s$. Consider a transition to $\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})$ under joint action $\tb{\ti{a}} \in \mathcal{A}$. Let $\mathcal{T} \subseteq \mathcal{I}$ be the set of agents moving from $s$ to $g$. Define $r = |\mathcal{I}|$, $r' = |\mathcal{I} \setminus \mathcal{T}|$ and $\mathcal{T}' = \mathcal{N} \setminus \mathcal{T}$. Then,
% 
\begin{align}
    \mathbb{P}(\tb{\ti{s}}^\prime | \tb{\ti{s}}, \tb{\ti{a}}) \nonumber 
    &= \frac{r' + (r - 2r')\delta}{n \cdot 2^{r-1}} 
    + \frac{n - r}{n \cdot 2^r} 
    + \frac{\Delta}{n}(r - 2r') \nonumber 
    \\
    &\quad + \frac{2\Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big[
    \sum_{i \in \mathcal{I} \cap \mathcal{T}'} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} 
    - \sum_{t \in \mathcal{T}} \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\}
    \Big]. \nonumber
\end{align}
\end{restatable*}
% 
\begin{restatable*}{cor}{corpstar}
\label{corollary:p_star}
Following Lemma~\ref{lemma:general_tp}, if agent $i\in \mathcal{I}$ selects its action according to $a_{i,j} = \sgn(\theta_{i,j})~\forall~j \in [d-1]$, the resulting transition probability is independent of $\mathcal{I}$ and $\mathcal{T}$, and it only depends on $r$ and $r'$. We denote the corresponding global action by $\tb{\ti{a}}_\theta$ and resulting transition probabilities by $p^*_{r,r'}$.
\end{restatable*}
% 
We observe the following property regarding behavior of $p^*_{r,r'}$ with $r$ and $r'$. This helps us identify optimal policies (Theorem \ref{thm:all_in_one}) as well as derive regret lower bounds (Theorem \ref{thm:lower_bound}).
% 
\begin{restatable*}{lem}{monotonic}
\label{claim:probability_inequality}
For every $r \in [n-1]$, the following holds: (a) for $r' \in \{0, \dots, \lfloor \frac{r+1}{2} \rfloor\}$, we have $\binom{r+1}{r'} p^*_{r+1,r'} < \binom{r}{r'} p^*_{r,r'}$ and (b) for $r' \in \{\lfloor \frac{r+1}{2} \rfloor + 1, \dots, r\}$, we have $\binom{r+1}{r'} p^*_{r+1,r'} > \binom{r}{r'} p^*_{r,r'}$.
\end{restatable*}
% 
\paragraph{Why do we expect tight lower bounds for these instances?} In Theorem \ref{thm:all_in_one} we establishes that, for any instance $(n, \delta, \Delta, \theta)$ the optimal policy selects action $\tb{\ti{a}}_{\theta}$ is taken in every state.
Now consider a policy that differs from $\tb{\ti{a}}_{\theta}$ in only one non-goal state and exactly at one component of global action. Due to the small $\Delta (< 2^{-n})$, the transition probability (Lemma \ref{lemma:general_tp}) for any $(\tb{\ti{s}}, \tb{\ti{a}}, \tb{\ti{s}}')$ is nearly identical to the one under optimal policy, implying the value of such a policy is only slightly worse. 
There are $(2^{n} - 1) \times n(d - 1)$ such policies. 
Moreover, there are exponentially many policies that differ in just two components of the global action in a single state, or in one component across two states, whose values are expected to be only marginally worse. The existence of so many near-optimal policies makes learning the optimal policy particularly challenging for any algorithm.



% \textcolor{red}{Fix any instance $(n, \delta, \Delta, \theta)$. The optimal action is the one which takes $\tb{\ti{a}}_{\theta}$ at all states. Consider another policy that differs from $\tb{\ti{a}}_{\theta}$ only in any one state and only in any one component of only any one agent. Due to small $\Delta (< 2^{-n})$ the transition probabilities for any ($\tb{\ti{s}},\tb{\ti{a}},\tb{\ti{s}}'$) in markov chain induced due to this policy are very close to the corresponding transition probabilities in the optimal policy case. Thus we expect the value of this policy to be only slightly higher than that of the optimal one. There are a total of $(2^{n}-1) \times n(d-1)$ such policies. Similar arguments can be made for policies that differ at any two components of global action in any one state and policies that differ in any one component of global action at any two states. Such policies are much larger in number that the policies of earlier kind are only slightly worse than them. These exponentially many near-optimal policies make it difficult to  learn the optimal policy for any algorithm.} 
    % \item \textbf{Worst-case reversals.} \textcolor{red}{what does the title mean?}  An algorithm that efficiently learns the optimal policy for one instance may struggle to do the same for other instances in the set. For example, if an action is optimal for an instance defined by $\theta = (\theta_1, 1,  \theta_2, 1,  \dots, \theta_n, 1)$, there exists a mirrored instance $\theta' = (-\theta_1, 1,  -\theta_2, 1,  \dots, -\theta_n, 1)$ where the same action becomes the worst.
% \end{itemize}

% In the following section, we formalize these intuitions and present key results that establish our regret lower bound.


% ....


% \pt{We would like to highlight the importance of the instance that we constructed. we would like to highlight why the above described instances are considered and their importance. In particular, we will provide the details on why the instances are hard, and why they one would expect a good/ sub-linear lower bound on the regret.}

% % 
% \pt{I haven't looked at this part as of now.}

% Any deterministic algorithm produces, in general, a history-dependent policy. Fixing any such policy $\pi$, we will analyze the regret of this policy on a set of hard to learn instances that differ only due to $\theta$ (i.e., have same parameters $n, \delta, \Delta$) and show that there exists an instance in the set of hard-to-learn instances that achieves lower bound on expected cumulative regret that scales similarly in terms of number of episodes as the upper bound $\widetilde{O}(\sqrt{K})$ reported by \cite{trivedi2023massp}. 
% Intuitively, there are two reasons why we expect at least one of the instances in this set to be very hard to be learnt for any given policy:
% \begin{itemize}
%     \item Firstly, all the instances are characterized by the optimum policy that at any state, the action taken is $\tb{a}_{\theta}$. If we consider a policy such that the action taken in only one of the $2^n-1$ non-goal states differed from $a_{\theta}$ at just one of the $n(d-1)$ indices, then the transition probabilities would differ (from those for optimal policy) only very slightly since $\Delta$ is quite small $(<2^{-n})$. 
% Hence, the value function for that policy would be only slightly higher. Observe that there would be $n(d-1).2^{n-1}$ (significant) number of such policies. The policies that differ in the above fashion at any two states are even larger in number and can't be expected to be too worse in terms of the expected cumulative cost for similar reason. Hence, separating these large number of policies efficiently is a challenge before any MASSP learning algorithm. 
% \item Secondly, any learning algorithm that efficiently learns the best policy for one instance in the set of all instances, may not be able to efficiently learn some other instance in the set. Also, if a particular action is the best (optimal) for a given instance $\theta = (\theta_1,1,\theta_2,1,\dots,\theta_n,1)$, there definitely exists another instance $\theta = (-\theta_1,1,-\theta_2,1,\dots,-\theta_n,1) \in \Theta$ for whom the same action is the worst.
% \end{itemize}
% In the following section, we present our observations on these instances and key results that follow.




% \textbf{Near-indistinguishable policies.} Each optimal policy selects the fixed action $\tb{\ti{a}}_\theta$ in all states (see  Theorem~\ref{thm:all_in_one}). A policy that deviates from $\tb{\ti{a}}_\theta$ in even a single out of $n(d-1)$ components yields only a marginal difference in value due to the small parameter $\Delta (< 2^{-n})$. Since there are exponentially many near-optimal policies, making it difficult to  distinguish solely on the performance. \textcolor{red}{can elaborate this a lot \pt{can you write whatever you have in mind.}}

==> Sections/4_results.tex <==
\section{Theoretical results}
\label{sec:theory}

We now present our main theoretical findings. Our goals are twofold: (i) to characterize the structure of the optimal policy and value function in our LM-MASSP instances and (ii) to establish a tight regret lower bound for any decentralized learning algorithm in this setting.
Intuitively, any state with less agents at the initial node $s$ is expected to be \emph{closer} to the $goal$ state than any other state with more agents at $s$. Thus, its desirable to have the state with less agents at $s$ to get a relatively lower cumulative cost-to-go. 
Such monotonicity allows us to reason about the value function at a coarser level depending on the number of agents at node $s$. 
Leveraging this structure, we characterize the optimal policy and value function in the following theorem.
% 
\begin{restatable*}[Structure of the optimal value and policy]{thm}{optimalvalue}
\label{thm:all_in_one}
For any instance $(n, \delta, \Delta, \theta)$,

(a) the policy that selects action $\tb{\ti{a}}_{\theta}$ as given in Corollary \ref{corollary:p_star} in every state $\tb{\ti{s}} \in \mathcal{S}$ is optimal.  

(b) the optimal value  is  same for all states of same type, i.e.,  for every $r \in [n]$, we have,  
    $V^*(\tb{\ti{s}}) = V^*_r$ for every $\tb{\ti{s}} \in \mathcal{S}_r$, where $V^*_r$ depends only on $r$. We define $V^*_0 = 0$.

(c) the optimal value function is strictly increasing with $r$, i.e., 
    $0 = V^*_0 < V^*_1 < \cdots < V^*_n = B^*$.
\end{restatable*}
% 
The detailed proof is deferred to Appendix \ref{proof:thm_all}. The theorem reveals that our instances admit a simple optimal policy depending only on a parameter $\theta$. 
Despite exponential state space, the value function is fully characterized by its \emph{type}.  We emphasize that this result is critical, enabling our regret analysis and may be of independent interest in broader classes of symmetric decentralized multi-agent settings. 

We now present our main result: regret lower bound for decentralized learning in LM-MASSPs. It matches the upper bound of \cite{min2022learning} (for $n=1$) and reported upper bound in \cite{trivedi2023massp} for a general $n$.

\begin{restatable*}[Lower bound on regret]{thm}{regret}
\label{thm:lower_bound}
Let $\pi$ be any decentralized learning algorithm. For every $n \geq 1$, $\delta \in (2/5, 1/2)$, and $\Delta < 2^{-n} ( \frac{1 - 2\delta}{1 + n + n^2})$, there exists an LM-MASSP instance $(\theta \in \Theta)$ such that, after $K > \frac{n(d-1)^2 \cdot \delta}{2^{10} B^* \left( \frac{1 - 2\delta}{1 + n + n^2} \right)^2}$ episodes, the expected cumulative regret incurred by $\pi$ satisfies
\begin{align}
    \mathbb{E}_{\theta,\pi}[R(K)] \geq \frac{d \cdot \sqrt{\delta} \cdot \sqrt{K \cdot B^*/n}}{2^{n+9}}.
\end{align}
\end{restatable*}
% 
The proof is provided in Appendix \ref{proof:thm_lb}.
This theorem highlights that even with strong structure and symmetry in the instances, any decentralized learning algorithm suffers from fundamental information bottlenecks, and no learning algorithm can escape the fundamental $\Omega(\sqrt{K})$ regret. Moreover, our lower bound recovers the previously established single-agent result as a special case.
% 
\begin{remark}
The exponential decay of regret lower bound with $n$ may not be misinterpreted as weakening of the bound with increasing $n$. To analyze regret scaling with $n$, one must fix parameters $(\delta, \Delta, \theta)$. Since $\Delta < 2^{-n} ( \frac{1 - 2\delta}{1 + n + n^2})$, it inherently fixes the range on $n$. So for any valid instance, there exist exponentially many near-optimal policies (see discussion after Lemma~\ref{claim:probability_inequality}).
In these instances, as $n$ increases within this range, more suboptimal policies get closer to optimal, making learning significantly harder. The corresponding decay of the lower bound reflects the increased difficulty.
% \pt{The exponential decay of regret lower bound with $n$ must not be misunderstood as weakening of the lower bound with increasing $n$. Recall that to analyze regret scaling with $n$, we need to let all other parameters $(\delta,\Delta,\theta)$ stay constant. Most crucial of which is to choose $\Delta$ that is compatible for the desired range of $n$. Note that we can't analyze this scaling for arbitrary high $n$ since $\Delta<2^{-n}$ needs to be fixed. The most restrictive condition on $\Delta$ for valid instance comes from $n$ under analysis. Fixing such a $\Delta$, for any of our instance, there are exponentially many policies in close neighborhood of the optimal policy in terms of value (see discussion after Lemma \ref{claim:probability_inequality}).
% With increasing $n$, increasing number of sub-optimal policies get closer to the optimal. Hence, our instances are \emph{harder} to learn with increasing $n$. Consequently, the lower bound shall be expected to decrease with increasing $n$.}
\end{remark}




% \pt{The instances that we created, with increasing n, the instances are harder-- we could have designed the easier instance, but in out case they are hard- - there are lot of policy that are close to optimal . and the number of policy that are close to optimal increases with n, that's why the expected regret is decreasing. Why thera are more polciy close to optimal policy - -- consider an instance, a theta at every stae is optimal, imagine policy a policy that takes optimal action at all sates expect one state -- in this state it is not taking the optimal -- for all but one agent -- it again taking optimal action -- for this action -- at all component it is optimal action except only one comp out of d-1 componetnts for this agents -- now look at the dynamics - they are not too different -- nbcz prob has Delta / n(d-1) -- Delta itself is 2 -n. THERE Are too many policis of such nature -- all of these are very close they are clos in terms of prob and hence the value. -- similar 2 components etc -- too many sub-optimal policy that are in nbd of optimal policy. This difference of optimal - sub -- depend on Delta, and, n. Delta is exp decaying in n. So, with higher n, this closeness is increases. That's why exponential --- thus, regret is tight in n. in our case, it is tight -- for our instances -- in space of all instance it is tight in K --- but tighness in n is not known in general, -- for iur instances it is tight -- designing instance with increasing regret with linear increase in n would be  be intersting -- furture work}






% ....

% \section{Theoretical Results}
% \label{sec:theory}

% We now present our main theoretical findings. The goal is twofold: (i) to characterize the structure of the optimal policy and value function in our linearly-parameterized multi-agent SSP (LM-MASSP) instances, and (ii) to establish a tight $\Omega(\sqrt{K})$ regret lower bound for any decentralized learning algorithm in this setting.

% A key challenge in decentralized multi-agent SSPs is the exponential growth of the state and action spaces, which makes reasoning about optimality non-trivial. However, in our structured 2-node LM-MASSP instances, we can exploit symmetries and cost structures to derive several tractable properties of the optimal policy.
% To build intuition, consider the following observation: in a goal-directed task with stochastic costs, a state with more agents at the goal node $g$ should intuitively be ``closer'' to the terminal condition. 
% Therefore, we expect the optimal value of such a state to be lower (i.e., better in terms of cumulative cost-to-go) compared to states with fewer agents at $g$. This intuition is formalized in the next property, which plays a central role in enabling our analysis.
% % 
% \begin{property}[Monotonicity of Value Functions]
% \label{prop:1}
% Let $\tb{\ti{s}}_1, \tb{\ti{s}}_2 \in \mathcal{S}$ be two states with $r_1$ and $r_2$ agents at the start node $s$, i.e., $\tb{\ti{s}}_1 \in \mathcal{S}_{r_1}$ and $\tb{\ti{s}}_2 \in \mathcal{S}_{r_2}$. Then, if $r_1 > r_2$, we have $V^*(\tb{\ti{s}}_1) > V^*(\tb{\ti{s}}_2)$ and vice versa.
% \end{property}
% % 
% This monotonicity allows us to reason about the value function at a coarser granularity using state partitions based on type of state $r$. Using this, we characterize the structure of the optimal policy and value function in the following theorem.
% % 
% \begin{theorem}[Structure of Optimal Policy and Value Function]
% \label{thm:all_in_one}
% Consider any instance $(n, \delta, \Delta, \theta)$ defined in Section \ref{subsec:problem_instance}. Then
% \begin{enumerate}[label=(\alph*), left=5pt]
%     \item The policy that selects action $\tb{\ti{a}}_{\theta}$ in every state $\tb{\ti{s}} \in \mathcal{S}$ is optimal.
    
%     \item The optimal value function is constant within each state partition. That is, for every $r \in [n]$ and all $\tb{\ti{s}} \in \mathcal{S}_r$, we have $V^*(\tb{\ti{s}}) = V^*_r$, where $V^*_r$ depends only on $r$ (with $V^*_0 = 0$).
%     \item The optimal value function is strictly increasing with $r$, i.e.,  $0 = V^*_0 < V^*_1 < \cdots < V^*_n = B^*$.
% \end{enumerate}
% \end{theorem}
% % 
% The proof of this Theorem is given in Appendix ??. This theorem reveals that our instance class admits a simple yet optimal policy that depends only on a global parameter $\theta$. 
% Despite the exponential size of the state space, the value function is fully characterized by the index $r$. This structure enables tractable analysis of policy performance and is critical in proving our regret lower bound.
% We believe this result may be of independent interest for analyzing symmetric decentralized MDPs or multi-agent control problems with exchangeable structures.

% \begin{remark}
% The symmetry and partition-based optimality revealed by Theorem~\ref{thm:all_in_one} could provide useful insights beyond our current setting. For example, decentralized load-balancing, crowd dynamics, and anonymous MARL problems often exhibit similar state exchangeability. Our proof techniques could potentially be adapted to those domains.
% \end{remark}

% We are now ready to state our main theoretical result: a regret lower bound for decentralized learning in LM-MASSPs. This bound matches the $\widetilde{O}(\sqrt{K})$ upper bound shown by \cite{trivedi2023massp}, thus establishing its optimality (up to constants).

% \begin{theorem}[Lower Bound on Decentralized Regret]
% \label{thm:lower_bound}
% Let $\mathfrak{A}$ be any decentralized learning algorithm as defined in Section \ref{subsec:problem_formulation}. Then, for every $n \geq 1$, $\delta \in (2/5, 1/2)$, and $\Delta < 2^{-n} \cdot \frac{1 - 2\delta}{1 + n + n^2}$, there exists a LM-MASSP instance $(\theta \in \Theta)$ such that when $\mathfrak{A}$ is run on this instance for $K > \frac{(d-1)^2 \cdot \delta}{2^{10} V^*_1 \left( \frac{1 - 2\delta}{1 + n + n^2} \right)^2}$ episodes, the expected regret satisfies
% \[
% \mathbb{E}_{\theta,\mathfrak{A}}[R(K)] \geq \frac{d \cdot \sqrt{\delta} \cdot \sqrt{K \cdot V^*_1}}{2^{n+9}},
% \]
% where $V^*_1 = \frac{2n}{n - 1 + 2(\delta + \Delta)}$.
% \end{theorem}

% The detailed proof is given in Appendix ??. The above Theorem~\ref{thm:lower_bound} establishes a fundamental performance limit for decentralized learning in linearly-parameterized multi-agent SSPs. 
% It shows that even under strong structure and symmetry, no algorithm can achieve $\Omega(\sqrt{K})$ regret. 
% This matches the known upper bounds and confirms the statistical hardness of decentralized goal-directed planning under linear function approximation.




% ....

% \section{Theoretical Results}
% \label{sec:theory}

% Any 2-node LM-MASSP instance as defined in Section \ref{subsec:problem_instance} is reasonably expected to have the notion that under the optimal behavior of agents, a state with more agents at node $g$ is \textit{better}
% compared to another state with fewer agents at node $g$. This can be baked mathematically in terms of value functions of states in the following property. \pt{we can write this better, why we need this property? -- intuitively, if there are more number of agents at s, then then cost (hence the value function) will be more.}
% % 
% \begin{property}
% \label{prop:1}
%     Consider any two states $\tb{\ti{s}}_1, \tb{\ti{s}}_2 \in \mathcal{S}$. Let $\tb{\ti{s}}_1 \in \mathcal{S}_{r_1}$ and $\tb{\ti{s}}_2 \in \mathcal{S}_{r_2}$. Then, if $r_1>r_2$, we have $V^*(\tb{\ti{s}}_1) > V^*(\tb{\ti{s}}_2)$ and vice-versa.
% \end{property}
% % 
% Recall that to obtain regret lower bound, we wish to compare any policy with the optimal in terms of their values. Also, recall that any multi-agent setting leads to explosion of the number of states and actions due to which it's challenging to obtain optimal policies for the setting. 
% In the following theorem we show that for our instances, a tractable optimal policy exists. Though optimum value is still intractable, our partitions based on type of state exhibit interesting behavior. 
% Particularly, states of same type are equivalent in terms of their values under optimal policy. Finally, we show that our instances exhibit the property \ref{prop:1} too. This is key in proving both Theorems \ref{thm:all_in_one} and \ref{thm:lower_bound}.

% \begin{theorem}\label{thm:all_in_one}
% Consider any instance $(n, \delta, \Delta, \theta)$ defined in section \ref{subsec:problem_instance}. 

% a) Then the policy of taking action $\tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$, is optimal. 

% b) Further, optimal value for each state of same type is the same, i.e., for every $r \in [n]$, it holds that for all $\tb{\ti{s}} \in \mathcal{S}_r$ we have $V^*(\tb{\ti{s}}) = V^*_r =$ some constant depending on only $r$. We define $V^*_0=0$.

% c) The optimal value function monotonically increases with the number of agents at node $s$ i.e., $0=V^*_0<V^*_1<V^*_2\dots<V^*_n = B^*$. 
% \end{theorem}


% The above theorem provides a broad level of understanding of our features. \pt{To highlight here itself that this result can be of independent interest to other communities and give the proper justification of why we are saying this. If this is correct, we can write it as a remark, and emphasis it throughout in the intro, abstract, conclusion and major contributions.}


% In the following theorem we provide the main result of this work, namely, tight lower bound in the learning of LM-MASSPs. \pt{We are now ready to prove the main result of our work that gives the lower  bound on the regret defined in eqn???} 


% \begin{theorem}
% \label{thm:lower_bound}
% % 
% For any decentralized MASSP learning algorithm $\mathfrak{A}$ as defined in \ref{subsec:problem_formulation}, there exists a LM-MASSP instance ($\theta \in \Theta$) for every $n \geq 1$, $\delta \in (2/5,1/2)$, $\Delta < 2^{-n}.\frac{1-2\delta}{1+n+n^2}$, such that the expected cumulative regret upon running the algorithm on this instance for $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1. \big \{\frac{1-2\delta}{1+n+n^2} \big \}^2} $ episodes at least matches the reported $\widetilde{O}(\sqrt{K})$ upper bound by \cite{trivedi2023massp} in terms of number of training episodes $K$. Here $V^*_1 = \frac{2n}{n-1+2(\delta+\Delta)}$.  Specifically for this instance, we have $\mathbb{E}_{\theta,\mathfrak{A}}[R(K)] \geq \frac{d.\sqrt{\delta}\sqrt{K.V^*_1}}{2^{n+9}}$     
% \end{theorem}
% % 

% \pt{To close this section by summary what we have achieved using this thm -- by writing the interpretation and summary of this theorem.}




==> Sections/5_proof.tex <==
\section{Outline of proofs}
\label{sec:proof_outline}

\subsection{Proof sketch of Theorem \ref{thm:all_in_one}}
% 
\begin{proof} 
% 
We use the Mathematical induction on $r$, the number of agents at node $s$ in any  $\tb{\ti{s}} \in \mathcal{S} $. All the claims trivially holds for  $r=0$. So, we consider $r=1$ as the base case.
% All  
% For $r = 0 $, $V^* $ are zero by definition, so the claims hold trivially.
% We use $r = 1 $ as the base case for generality.


\textbf{Base case $(r=1)$.} For any state $\tb{\ti{s}} \in \mathcal{S}_1$, the only \emph{reachable} next state is either $\tb{\ti{s}}$ or $\tb{\ti{g}}$. For any action $\tb{\ti{a}} \in \mathcal{A}$, value of the policy $\pi_{\tb{\ti{a}}}$ that always selects action $\tb{\ti{a}}$ at $\tb{\ti{s}}$  is given by $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}}) = \frac{1}{1 - \mathbb{P}(\tb{\ti{s}}| \tb{\ti{s}}, \tb{\ti{a}})}$. 
Using Lemma \ref{lemma:general_tp}, one observes that the self-transition probability $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}}, \tb{\ti{a}})$ is minimized at $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$. 
This establishes the first claim. 
The above arguments hold for every $\tb{\ti{s}} \in \mathcal{S}_1$ and  using corollary~\ref{corollary:p_star}, the self-transition probability with the value is identical for all states, establishing the second claim. The third claim holds as  $V^*_1 > 0$.

% Note that the above arguments hold for any $\tb{\ti{s}} \in \mathcal{S}_1$, and by Corollary~\ref{corollary:ps_s}, the value function is identical across all such states. Hence, the second claim is satisfied. Since $V^*_1 > 0$, the third claim also holds. This concludes the proof of the base case.

\textbf{Inductive Step.} Assume the three claims of the theorem hold for all $r \in \{1, 2, \dots, k\}$. We now show they also hold for $r = k+1$, in the same order.
% 
Consider any state $\tb{\ti{s}} \in \mathcal{S}_{k+1}$. To prove the first claim, we evaluate the value $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$ under a policy $\pi_{\tb{\ti{a}}}$ that always takes action $\tb{\ti{a}}$ at $\tb{\ti{s}}$ and optimal action $\tb{\ti{a}}_{\theta}$ in other \emph{reachable} states. By the inductive hypothesis, values and optimal actions are known for all states in $\cup_{i=0}^k \mathcal{S}_i$. Since all states reachable from $\tb{\ti{s}}$ lie in this set, i.e., $\cup_{i \in [k] \cup \{0\}}\mathcal{S}_i(\tb{\ti{s}}) \subseteq \cup_{i \in [k] \cup \{0\}}\mathcal{S}_i$, the value  $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$ is given by
% 
\begin{align}
\label{eqn:v_pia}
    V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}}) = 1 + \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}}) V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}}) + \mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}}) V^*(\tb{g}) + \sum_{r' \in [k]} \sum_{\tb{\ti{s}}' \in \mathcal{S}_{r'}(\tb{\ti{s}})} \mathbb{P}(\tb{\ti{s}}' | \tb{\ti{s}},\tb{\ti{a}}) V^*_{r'}.
\end{align}
% 
Using the inductive hypothesis and Lemma \ref{lemma:general_tp}, we show that $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$ is minimized when $\tb{\ti{a}} = \tb{\ti{a}}_{\theta} ~\forall ~\tb{\ti{s}} \in \mathcal{S}_{k+1}$, proving the first claim. The second claim follows directly from Corollary~\ref{corollary:p_star} and Eqn \eqref{eqn:v_pia}. For the third claim, we use Lemma \ref{claim:probability_inequality} along with the following result (see appendix \ref{proof:lemma_prob_ineq}).


\begin{restatable*}{lem}{valuemonotonic}
\label{lemma:probability_inequality}
    Let $r \in [n-1]$. Suppose that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, we have
    $\binom{r+1}{r'} p^*_{r+1,r'} < \binom{r}{r'} p^*_{r,r'}$, and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \dots, r\}$, we have
    $\binom{r+1}{r'} p^*_{r+1,r'} > \binom{r}{r'} p^*_{r,r'}$. Further, if  
    $V^*_r > V^*_{r-1} > \dots > V^*_1 > V^*_0 = 0$, then $V^*_{r+1} > V^*_r$.
\end{restatable*}
This proves the final claim for $r=k+1$. By induction, the claim holds for all $r = \{0,1,\dots, n\}$.
\end{proof}

\subsection{Proof sketch of Theorem \ref{thm:lower_bound}}

\begin{proof}
% 
%
Consider instances $(n, \delta, \Delta, \theta)$ where $n \geq 1$, $\delta \in (2/5, 1/2)$ and $\Delta < 2^{-n} ( \frac{1 - 2\delta}{1 + n + n^2})$ are fixed, while $\theta$ varies across instances with corresponding optimal policy $\pi_{\theta}^*$ as described in Theorem \ref{thm:all_in_one}. Let $\tb{\ti{s}}^t$ and $\tb{\ti{a}}^t$ be the global state and action at time $t$, respectively. 
The expected regret of an algorithm $\pi$ in the first episode is
% 
\begin{align}
   \mathbb{E}_{\theta,\pi}[R_{1}] 
    &= V^{\pi}(\tb{\ti{s}}^1) - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1)  \nonumber
    \\
    &= \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1),\ \tb{\ti{s}}^2 \sim \mathbb{P}(\cdot|\tb{\ti{s}}^1,\tb{\ti{a}}^1)}\left[ V^{\pi}(\tb{\ti{s}}^2) - V^{\pi^*_{\theta}}(\tb{\ti{s}}^2) \right] 
    + \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)}\left[ Q^{\pi^*_{\theta}}(\tb{\ti{s}}^1,\tb{\ti{a}}^1) \right] 
    - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) \label{eqn:simp_reg_vv}
\end{align}
where in the second step we add and subtract the expectation of optimal $Q$-function \cite{sutton2018reinforcement} and use its definition. We emphasize that unlike the value of any Markov stationary policy, the value of any learning algorithm for any intermediate state $\tb{\ti{s}}^t$ depends, in general, on the past history till $t$. 
This implies that the $V^{\pi}(\tb{\ti{s}}^2)$ above is not independent of the history 
% $(\tb{\ti{s}}^1, \tb{\ti{a}}^1, \{c^1_i(s_i^1,a_i^1)\}_{i=1}^n)$ 
for any fixed $\tb{\ti{s}}^2$. 
% \textcolor{red}{should we add a section in appendix to discuss this and add reference here? or this is clear by itself?}. 
The first expectation in Eqn~\eqref{eqn:simp_reg_vv} suggests a recurrence.
Using definition of $Q^{\pi^*_{\theta}}(.,.)$ and Lemma~\ref{lemma:general_tp}, 
\begin{align} 
\mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)}\left[ Q^{\pi^*_{\theta}}(\tb{\ti{s}}^1,\tb{\ti{a}}^1) \right] - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) 
&= \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Bigg\{ \sum_{\tb{\ti{s}}^2 \neq \tb{\ti{s}}^1} \left[ \mathbb{P}(\tb{\ti{s}}^2|\tb{\ti{s}}^1,\tb{\ti{a}}^1) - \mathbb{P}(\tb{\ti{s}}^2|\tb{\ti{s}}^1, \tb{\ti{a}}^{1^*}) \right] V^{\pi^*_\theta}(\tb{\ti{s}}^2) \nonumber
\\
& \quad +  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a^1_{i,p}) \neq \sgn(\theta_{i,p})\} \cdot V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) \Bigg\}. \nonumber
\end{align}
We further lower bound the above using the following lemma (see appendix \ref{proof:lemma_sum_diff}). 
% 
\begin{restatable*}{lem}{probdiff}
\label{lemma:sum_diff_prob_v}
     For any of our instances, $\forall ~(\tb{\ti{s}}, \tb{\ti{a}}) \in \mathcal{S} \times \mathcal{A}$,  $\sum_{\tb{\ti{s}}^\prime \neq \tb{\ti{s}}} \big\{\mathbb{P}(\tb{\ti{s}}^\prime|\tb{\ti{s}},\tb{\ti{a}})-\mathbb{P}(\tb{\ti{s}}^\prime|\tb{\ti{s}}, \tb{\ti{a}}^*)\big \} V^*(\tb{\ti{s}}^\prime) \geq 0  $. 
\end{restatable*}
Further, unrolling the relationship in Eqn \eqref{eqn:simp_reg_vv} recursively over all time steps $h$ in the first episode and applying the third claim in Theorem~\ref{thm:all_in_one} to lower bound $V^{\pi^*_{\theta}}(\tb{\ti{s}}')$ for each non-goal state $\tb{\ti{s}}'$, we get
\begin{align}
    \mathbb{E}_{\theta,\pi}[R_{1}] \geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{\theta,\pi} \Bigg[ \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\tb{\ti{s}}^h \neq \text{goal}\} \cdot \mathbbm{1}\{\sgn(a^h_{i,p}) \neq \sgn(\theta_{i,p})\} \Bigg].
\end{align}
% where 
% the expectation is taken over trajectories in the first episode generated by the policy $\pi$ under the transition kernel $\mathbb{P}_{\theta}$ and 
% $a^h_{i,p}$ is the $p^{\text{th}}$ component of the action taken by agent $i$ at time step $h$.
Extending this over all the $K$ episodes, the lower bound can be expressed as 
\begin{align}
    \mathbb{E}_{\theta,\pi}[R(K)] \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \Big\{ \sum_{i =1}^{n} \sum_{j=1}^{d-1} N_{i,j}(\theta) \Big\},
\end{align}
where $N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} \cdot \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\}$ for each $i \in [n], j \in [d-1]$. It is important to note that we can't use the standard Pinsker's inequality here to bound the regret, as $N_{i,j}(\theta)$ can be unbounded. 
To handle this, we define the truncated sums upto a predefined $T$ as $N^- = \sum_{t=1}^T\mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\}$ 
and $N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\} $ for any agent $i \in [n] $ and $ j \in [d-1]$.
% 
Thus, the regret upto $K$ episode can be further lower bounded as
% 
\begin{align}
   \mathbb{E}_{\theta,\pi}[R(K)] \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \Bigg[ \sum_{i=1}^{ n}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \Bigg].
\end{align}
% 
For every $\theta = (\theta_1,1,\theta_2,1\dots,\theta_n,1) \in \Theta$ and $j \in [d-1]$, let $\theta^j = (\theta_1', 1, \theta_2', 1, \dots, \theta_n', 1)$, where for every $i \in [n],~\theta_i'$ is identical to $\theta_i$ except at the $j^{\text{th}}$ coordinate, where $\theta'_{i,j} = -\theta_{i,j}$. Thus, we have
% 
\begin{align} 
    2 \sum_{\theta \in \Theta} \mathbb{E}_{\theta,\pi}[R(K)] 
    &\geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i=1}^{n} \sum_{j=1}^{d-1} \left[ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \right] 
    \\
    &= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i=1}^{n} \sum_{j=1}^{d-1}  \left[  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \right].
\label{eqn:rthetan}
\end{align}
The last step follows since $N^- = N^-_{i,j}(\theta) + N^-_{i,j}(\theta^j)$ for any $i \in [n], ~j\in[d-1]$. To simplify first expectation, we generalize Lemma C.2 in \cite{rosenberg2020near} as follows
% 
\begin{restatable*}{lem}{nlowerbound}
\label{lemma:gen_co}  
    For any instance $(n,\delta, \Delta, \theta)$, algorithm $\pi$, and $T \geq 2KV^*_1$, we have $\mathbb{E}_{\theta, \pi}[N^-] \geq \frac{KV^*_1}{4}$. 
\end{restatable*}

This bounds the first term in Eqn~\eqref{eqn:rthetan}.
The remaining terms capture the difference in expectations under different model parameters. Applying the Pinsker's inequality (Lemma E.3 in \cite{min2022learning}), we get
% % 
% \begin{lemma}
% \label{lemma:pinsk}
%     If $f:S^T\xrightarrow{}[0,D]$ then, 
%     $\mathbb{E}_{\mathbb{P}_1} (f(s)) - \mathbb{E}_{\mathbb{P}_2} (f(s))\leq D \sqrt{\frac{log(2)}{2}}. \sqrt{ \kl(\mathbb{P}_2 || \mathbb{P}_1)}$    
% \end{lemma}
% % 
% Thus, we obtain the following:
\begin{align}
\label{eqn:regret_expression_last}
    2 \sum_{\theta \in \Theta} \mathbb{E}_{\theta,\pi}[R(K)] 
    \geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i=1}^{n} \sum_{j=1}^{d-1} \left\{ \frac{K V^*_1}{4} - T \sqrt{\frac{\log 2}{2}} \cdot \sqrt{\mathrm{KL}(\mathbb{P}^{\pi}_{\theta} \Vert \mathbb{P}^{\pi}_{\theta^{j}})} \right\}
\end{align}
% 
In the above $\mathbb{P}^\pi_\theta$ represents the distribution over the $T$- length state sample paths due to interaction of algorithm $\pi$ and the transition dynamics described by parameter $\theta$. Bounding the KL divergence in the multi-agent setting is challenging due to the exponential number of next states and actions. Since existing techniques ( \cite{jaksch2010near}, \cite{min2022learning}) do not directly apply, we leverage symmetries in our instance to derive a algorithm-independent upper bound on the KL divergence.
% 
\begin{restatable*}{lem}{klbound}
\label{lemma:kl_d}
    For any instance $(n, \delta, \Delta, \theta)$ and algorithm $\pi$, for any $j \in [d-1]$, we have
    \begin{align}
        \kl(\mathbb{P}{^\pi_\theta} || \mathbb{P}^{\pi}_{\theta^j}) \leq 3 \cdot 2^{2n} \cdot \frac{\Delta^2}{\delta (d-1)^2} \cdot \mathbb{E}_{\theta, \pi}[N^-].
    \end{align}
\end{restatable*}
% 
The proof of this lemma is deferred to Appendix \ref{proof:lemma_kl_d}. Using Lemma \ref{lemma:kl_d},  $\mathbb{E}_{\theta,\pi}[N^-] \leq T = 2K V^*_1$ and picking $\Delta = \Delta^* = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}$ in Eqn \eqref{eqn:regret_expression_last} we get 
\begin{align}
\label{eqn:final_avgreg}
    \frac{1}{|\Theta|} \sum_{\theta \in \Theta} \mathbb{E}_{\theta,\pi}[R(K)]
    \geq \frac{(d-1) \cdot \sqrt{\delta} \cdot \sqrt{K V^*_1}}{2^{n+8}} 
    \geq \frac{d \cdot \sqrt{\delta} \cdot \sqrt{K V^*_1}}{2^{n+9}}  \geq \frac{d \cdot \sqrt{\delta} \cdot \sqrt{K B^*/n}}{2^{n+9}},
\end{align}
% 
where the last inequality holds due to the result $V^*_1 \geq B^*/n$ for any of our instances. 
Since this is a lower bound on the average of expected regret over $\Theta$, there must exist at least one instance $\theta \in \Theta$ for which the lower bound in Eqn~\eqref{eqn:final_avgreg} holds. 
Finally, to ensure that the chosen $\Delta = \Delta^*$ is valid, i.e., $\Delta < 2^{-n} ( \frac{1 - 2\delta}{1 + n + n^2})$, we obtain the following sufficient condition  $K > \frac{n (d-1)^2 \cdot \delta}{2^{10} \cdot B^* \cdot \left( \frac{1 - 2\delta}{1 + n + n^2} \right)^2 }$.
This completes the proof.
\end{proof}



% \pt{Does this mean that the $K$ is almost zero? division by a large number $2^{10}$?} 
% \textcolor{blue}{we should remark why this is not so}

==> Sections/6_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
% 
This work takes a first step toward closing the gap in our understanding of Dec-MASSPs under linear function approximations. We establish the first regret lower bound for this setting, obtained by carefully constructed hard-to-learn instances whose complexity scales with the number of agents. By leveraging symmetry-based arguments, we identify the structure of optimal policies.
Our lower bound of $\Omega(\sqrt{K})$ over $K$ episodes underscores the fundamental difficulty of decentralized learning in stochastic environments. These findings deepen the theoretical understanding of decentralized control and provide a foundation for designing more efficient and scalable algorithms in MARL.


Our MASSP instances design is based on the linear function approximations; thus, a key limitation of this work is to get a suitable regret lower bounds with  non-linear function approximations. 

An important open direction is to formally understand the increased complexity of decentralized MA-SSPs compared to single-agent SSPs. In particular, demonstrating a separation where the regret lower bound for a Dec-MASSP instance exceeds the upper bound for a single-agent case would justify the fundamental challenges in  decentralized learning.

% We conjecture that decentralized MA-SSPs are fundamentally harder to solve than single-agent SSPs. Establishing this would require proving that the regret lower bound for Dec-MASSPs exceeds the best known upper bound for the single-agent case—a key open problem.

% Our lower bounds hold for fixed 
% $n$, but extending them to arbitrary or growing $n$ remains a major challenge \textcolor{red}{this is misleading, need to elaborate that to study variation with $n$ discussion}. We conjecture that Dec-MASSPs are strictly harder than single-agent SSPs due to the combinatorial complexity of agent interactions. \textcolor{red}{hint to prove - a lower bound for massp need to be shown to be ckhigher than any upper bound for single agent ssp, it was written nicely in one of the earlier versions maybe there now in extra} Proving this likely requires new instance constructions that capture this increased difficulty, which is crucial for understanding the scalability of decentralized multi-agent learning.

==> Sections/all_updated_7_4_25.tex <==
\section{Experiments}
\label{sec:experiment}
In this section, we provide the details of the MDP network that we use to prove that lower bound. Consider a network with two nodes $\{s_{init}, g\}$. Thus, the number of states is $2^n$, where $n$ is the number of agents.
In each state the actions available to each agent are $\mathcal{A}^i = \{-1, 1\}^{d-1}$, for some given $d\geq 2$. So, the total number of actions is $2^{nd}$. 
Since the number of states and actions is exponentially large, we parameterize the transition probability. For each $(\tb{\ti{s}}^{\prime}, \tb{\ti{a}}, \tb{\ti{s}}) \in \mathcal{S} \times \mathcal{A} \times \mathcal{S}$, the global transition probability is parameterized as $\mathbb{P}_{\boldsymbol{\theta}}(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}) = \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},\tb{\ti{a}}), {\boldsymbol{\theta}} \rangle$.  The global features  are described below.


\textcolor{red}{Below are the updated features that match Min et al at n=1. The proof for this is in the appendix below proof for previous features.}

\pt{These are the final updated features, right? If this is the case. The first result we need to write is -- the features are valid and hence satisfy all the properties. These features will reduce to the Min paper when $n=1$.}
\textcolor{red}{yes these are the final ones from my side as of now, i would remove the 4th case in $\phi^i(.)$ definition}

\begin{equation}
\label{eqn:features_global_new}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  \tb{\ti{a}}) = 
\begin{cases} (\phi(s^{\prime^1} | s^1, \tb{\ti{a}}^1), \dots, \phi(s^{\prime^n} | s^n, \tb{\ti{a}}^n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}} ~\text{and}~  s^{i'} = g ~\text{if} ~ s^i = g,~ \forall~ i\in N
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}}, \text{or },  \exists~ i \in N,~ s.t. ~ s^i \neq s_{init}, s^{i'} = s_{init}
\\
(\mb{0}_{nd-1}, 1), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}}, 
\end{cases}
\end{equation}

Here $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i)$ are defined as 
\begin{equation*}
\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) = \begin{cases}  
\left(-\tb{\ti{a}}^i, \frac{1-\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}^i = s^{\prime^{i}} = s_{init}
\\
\left(\tb{\ti{a}}^i, \frac{\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}^i = s_{init},~s^{\prime^{i}} = g
\\
\left(\mathbf{0}_{d-1}, \frac{1}{n 2^{r}} \right)^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = g
\\
\mathbf{0}_d^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = s_{init}.
\end{cases}
\end{equation*}

==> Sections/checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: 
    % \answerTODO{} % Replace by 
    \answerYes{}
    % , \answerNo{}, or \answerNA{}.
    \item[] Justification: The claims are demonstrated in the key results in Lemmas and Theorems, with explanations next to them. 
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  The assumptions given in the paper give the limitations of this work. Further, future work direction in the conclusions describe another limitation of this work. %See Introduction, Discussion, and other sections.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have provided the assumptions used in this work, that are used in main the results.  %See assumptions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experimental results are not provided, since we are providing the regret lower bounds, that require a construction of hard-to-learn instance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not include experiments requiring code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work is theoretical, and hence there are no computational  experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper is theoretical, thus it does not include any experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not include experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the points mentioned in the NeurIPS Code of Ethics are taken into consideration.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Applications of decentralized MASSP are mentioned in introduction with positive societal impacts because of better resource utilization.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no release of data or models. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no  code, data, models, etc. involved. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no  code, data, models, etc. involved in the paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does neither involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does involve research with human subjects, thus no approvals are required.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}
\end{enumerate}

==> Sections/experiments.tex <==
\section{\textit{Transition Probability Model} Experiments}
\label{sec:experiment}
In this section, we provide the details of the MDP network that we use to prove that lower bound. Consider a network with two nodes $\{s_{init}, g\}$. Thus, the number of states is $2^n$, where $n$ is the number of agents.
In each state the actions available to each agent are $\mathcal{A}^i = \{-1, 1\}^{d-1}$, for some given $d\geq 2$. So, the total number of actions is $2^{nd}$. 
Since the number of states and actions is exponentially large, we parameterize the transition probability. For each $(\tb{\ti{s}}^{\prime}, \tb{\ti{a}}, \tb{\ti{s}}) \in \mathcal{S} \times \mathcal{A} \times \mathcal{S}$, the global transition probability is parameterized as $\mathbb{P}_{\boldsymbol{\theta}}(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}) = \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},\tb{\ti{a}}), {\boldsymbol{\theta}} \rangle$.  The global features  are described below. \\
\textcolor{red}{in the above, total # actions need to be $2^{n(d-1)}$}


\textcolor{red}{Below are the updated features that match Min et al at n=1. The proof for this is in the appendix below proof for previous features.}

\pt{These are the final updated features, right? If this is the case. The first result we need to write is -- the features are valid and hence satisfy all the properties. These features will reduce to the Min paper when $n=1$.}
\textcolor{red}{yes these are the final ones from my side as of now, i would remove the 4th case in $\phi^i(.)$ definition}

\begin{equation}
\label{eqn:features_global_new}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  \tb{\ti{a}}) = 
\begin{cases} (\phi(s^{\prime^1} | s^1, \tb{\ti{a}}^1), \dots, \phi(s^{\prime^n} | s^n, \tb{\ti{a}}^n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}} ~\text{and}~  s^{i'} = g ~\text{if} ~ s^i = g,~ \forall~ i\in N
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}}, \text{or },  \exists~ i \in N,~ s.t. ~ s^i \neq s_{init}, s^{i'} = s_{init}
\\
(\mb{0}_{nd-1}, 1), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}}, 
\end{cases}
\end{equation}

Here $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i)$ are defined as 
\begin{equation*}
\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) = \begin{cases}  
\left(-\tb{\ti{a}}^i, \frac{1-\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}^i = s^{\prime^{i}} = s_{init}
\\
\left(\tb{\ti{a}}^i, \frac{\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}^i = s_{init},~s^{\prime^{i}} = g
\\
\left(\mathbf{0}_{d-1}, \frac{1}{n 2^{r}} \right)^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = g
\\
\mathbf{0}_d^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = s_{init}.
\end{cases}
\end{equation*}
\\

In the above, $r$ represents the number of agents at $s_{init}$ and $\theta$ is an $nd$- dimensional vector of the form $\theta = (\theta_1,1, \theta_2,1,\dots,\theta_n,1)$ where for every $i \in [n]$, $\theta_i$ is a d-1 dimensional vector each of whose component is $(+/-) \frac{\Delta}{n(d-1)}$. To prove lower bound, we will further impose that for our instances, none of the two $\theta_i's$ are equal.


==> Sections/extra-appedix.tex <==
\section*{Appendix}

\section{Proofs}
\label{app:proofs}

In this section, we provide the details and proofs of the main results we stated in the paper.

\subsection{Proof of Lemma \ref{lemma: feature_properties}}
\label{app-proof:features_properties}

Recall, the global features  are given by
\begin{equation}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  \tb{\ti{a}}) = 
\begin{cases} (\phi(s^{\prime^1} | s^1, \tb{\ti{a}}^1), \dots, \phi(s^{\prime^n} | s^n, \tb{\ti{a}}^n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}}, ~\tb{\ti{s}}' \neq \tb{\ti{g}}, ~\text{and}~  s^{i'} = g ~\text{if} ~ s^i = g,~ \forall~ i\in N
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}}, \text{or },  \exists~ i \in N,~ s.t. ~ s^i \neq s_{init}, s^{i'} = g
\\
(\mb{0}_{nd-1}, 1), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}}, 
\end{cases}
\end{equation}
the first condition ensures that if an agent is at $g$, it should remain at $g$. The second condition make sure that the probability of the infeasible transitions is zero.

Here $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i)$ are defined as 
\begin{equation*}
\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) = \begin{cases}  
\left(-\tb{\ti{a}}^i, \frac{1-\delta}{r 2^r} \right)^{\top}, & if ~ {s}^i = s^{\prime^{i}} = s_{init}
\\
\left(\tb{\ti{a}}^i, \frac{\delta}{r 2^r} \right)^{\top}, & if ~ {s}^i = s_{init},~s^{\prime^{i}} = g
\\
\left(\mathbf{0}_{d-1}, \frac{1}{(n-r) 2^{r+1}} \right)^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = g
\\
\mathbf{0}_d^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = s_{init}.
\end{cases}
\end{equation*}
Here $r$ denotes the number of agent in $s_{init}$ in the global state $\tb{\ti{s}}$. The vector $\mathbf{0}_d^{\top} = (0,0, \dots, 0)^{\top}$ is a vector of $d$ dimension with all zeros. 
Thus, the features $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) \in \mathbb{R}^{nd}$. Moreover, the transition probability parameters are taken as $\boldsymbol{\theta} = \left( \boldsymbol{\theta}^1, 1,  \boldsymbol{\theta}^2, 1 \dots, \boldsymbol{\theta}^n, 1 \right)$ where $\boldsymbol{\theta}^i \in \left\lbrace -\frac{\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}  \right\rbrace^{d-1} $, and $\Delta < \delta$. 

\textbf{Recall the Lemma.}
    \textit{The features $\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},\tb{\ti{a}})$ satisfy the following: (a) $\sum_{\tb{\ti{s}}^{\prime}} \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = 1, ~ \forall ~\tb{\ti{s}}, \tb{\ti{a}}$; (b) $\langle \phi(\tb{\ti{s}}^{\prime} = \tb{\ti{g}} | \tb{\ti{s}} = \tb{\ti{g}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = 1, ~\forall~\tb{\ti{a}}$; (c) $\langle \phi(\tb{\ti{s}}^{\prime} \neq \tb{\ti{g}} | \tb{\ti{s}} = \tb{\ti{g}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = 0,~ \forall ~\tb{\ti{a}}$.}


\begin{proof}
   
    We will prove part (a), proof of the other parts follow directly from the feature design. 

\textbf{Case 1.} $\tb{\ti{s}}\neq \ti{\ti{g}}$

    Without loss of generality let us assume that $\tb{\ti{s}}$ is such that $r$ agents are at $s_{init}$, and remaining $n-r$ agents are at $g$. 

    The inner product in the summation can be rewritten as
    \begin{equation}
    \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle.
    \end{equation}
    Thus, proving the original equation reduces to proving
    \begin{equation}
        \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}} \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle = 1.
    \end{equation}
    We first note that out of $2^n$ total number of states, there are $2^r$ feasible states. For the remaining states, the features are zero by design,  and hence the above summation reduces to 
    \begin{equation}
        \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}_F} \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle = 1,
    \end{equation}
    where $\mathcal{S}_F$ is the set of all feasible state space. 
    
    Consider an agent $i$, who is at $s_{init}$. Out of total $2^r$ next possible states, there are exactly $\frac{2^r}{2}$ states in which agent $i$ will remain at $s_{init}$, and in remaining $\frac{2^r}{2}$ states in which the agents move to goal node. 
    The probability that the next node of agent $i$ is $s_{init}$ given that the current node of agent $i$ is $s_{init}$ is given by $- \langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{1-\delta}{r 2^r}$. And the probability that the next node of agent $i$ is $g$ given that the current node of agent $i$ is $s_{init}$ is  $ \langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{\delta}{r 2^r}$.
    Since, this is true for all the $r$ agents which are at $s_{init}$ so the contribution to the probability term from these $r$ agents who are at $s_{init}$ is
    \begin{eqnarray*}
        \sum_{i=1}^r \left\lbrace \left( -\langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{1-\delta}{r 2^r} \right) \times \frac{2^r}{2} \right\rbrace + \sum_{i=1}^r  \left\lbrace \left(\langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{\delta}{r 2^r} \right) \times \frac{2^r}{2} \right\rbrace = \frac{1}{2}.
    \end{eqnarray*}
    Next, consider an agent whose state is $g$; for this agent, there is only only possibility, the agent should stay at $g$. This is because it any agent tries to move to $s_{init}$, that state space is no more belong to the set of feasible state spaces. Therefore, the total number of such cases are  transitions are $2^r$. The probability that agent will stay at $g$ is  $\frac{1}{(n-r)} \times \frac{1}{2^{r+1}}$.  So the total probability in this case is  
    \begin{equation*}
        \sum_{i = r+1}^n  \frac{1}{(n-r) 2^{r+1}} \times 2^r = \frac{1}{2}.
    \end{equation*}
    So, the sum of these linearly approximated probabilities is
	\begin{eqnarray*}
		\sum_{\tb{\ti{s}}^{\prime}\in \mathcal{S}} \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \sum_{\tb{\ti{s}}^{\prime}\in \mathcal{S}_F} \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \frac{1}{2} + \frac{1}{2} = 1.
	\end{eqnarray*}

\textbf{Case 2.} $\tb{\ti{s}} =  \ti{\ti{g}}$

\begin{align}
    \sum_{\tb{\ti{s}}'\in \mathcal{S}} \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle &=  \langle \phi(\tb{\ti{s}}^{\prime} = \tb{\ti{g}}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle + \sum_{\tb{\ti{s}}' \neq \tb{\ti{g}}} \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle 
    \\
    & = 0 +  \langle (\tb{0}_{nd-1}, 1), (\theta^1, 1, \theta^2, 1,\dots, \theta^n, 1) \rangle \\ 
    &= 1.
\end{align}
This completes the proof. 
\end{proof}


\begin{proof} 
% 
\textcolor{red}{THIS IS FOR UPDATED FEATURES WHICH MATCH MIN ET AL FOR n=1. I HAVEN'T VERIFIED THE EXPLANATIONS IN ENGLISH BUT ONLY MODIFIED THE RESPECTIVE MATHEMATICAL EXPRESSIONS} 

We will prove part (a), proof of the other parts follow directly from the feature design. 

\textbf{Case 1.} $\tb{\ti{s}}\neq \ti{\ti{g}}$

    Without loss of generality let us assume that $\tb{\ti{s}}$ is such that $r$ agents are at $s_{init}$, and remaining $n-r$ agents are at $g$. 

    The inner product in the summation can be rewritten as
    \begin{equation}
    \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle.
    \end{equation}
    Thus, proving the original equation reduces to proving
    \begin{equation}
        \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}} \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle = 1.
    \end{equation}
    We first note that out of $2^n$ total number of states, there are $2^r$ feasible states. For the remaining states, the features are zero by design,  and hence the above summation reduces to 
    \begin{equation}
        \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}_F} \sum_{i=1}^{n} \langle \phi(s^{\prime^i} | s^i, \tb{\ti{a}}^i), (\boldsymbol{\theta}^i, 1)  \rangle = 1,
    \end{equation}
    where $\mathcal{S}_F$ is the set of all feasible state space. 
    
    Consider an agent $i$, who is at $s_{init}$. Out of total $2^r$ next possible states, there are exactly $\frac{2^r}{2}$ states in which agent $i$ will remain at $s_{init}$, and in remaining $\frac{2^r}{2}$ states in which the agents move to goal node. 
    The probability that the next node of agent $i$ is $s_{init}$ given that the current node of agent $i$ is $s_{init}$ is given by $- \langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{1-\delta}{n 2^{r-1}}$. And the probability that the next node of agent $i$ is $g$ given that the current node of agent $i$ is $s_{init}$ is  $ \langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{\delta}{n 2^{r-1}}$.
    Since, this is true for all the $r$ agents which are at $s_{init}$ so the contribution to the probability term from these $r$ agents who are at $s_{init}$ is
    \begin{eqnarray*}
        \sum_{i=1}^r \left\lbrace \left( -\langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{1-\delta}{n 2^{r-1}} \right) \times \frac{2^r}{2} \right\rbrace + \sum_{i=1}^r  \left\lbrace \left(\langle \tb{\ti{a}}^i, \boldsymbol{\theta}^i \rangle + \frac{\delta}{n 2^{r-1}} \right) \times \frac{2^r}{2} \right\rbrace = \frac{r}{n}.
    \end{eqnarray*}
    Next, consider an agent whose state is $g$; for this agent, there is only only possibility, the agent should stay at $g$. This is because it any agent tries to move to $s_{init}$, that state space is no more belong to the set of feasible state spaces. Therefore, the total number of such cases are  transitions are $2^r$. The probability that agent will stay at $g$ is  $\frac{1}{n} \times \frac{1}{2^{r}}$.  So the total probability in this case is  
    \begin{equation*}
        \sum_{i = r+1}^n  \frac{1}{n 2^{r}} \times 2^r = \frac{n-r}{n}.
    \end{equation*}
    So, the sum of these linearly approximated probabilities is
	\begin{eqnarray*}
		\sum_{\tb{\ti{s}}^{\prime}\in \mathcal{S}} \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \sum_{\tb{\ti{s}}^{\prime}\in \mathcal{S}_F} \langle \phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}), \boldsymbol{\theta}  \rangle = \frac{r}{n} + \frac{n-r}{n} = 1.
	\end{eqnarray*}

\textbf{Case 2.} $\tb{\ti{s}} =  \ti{\ti{g}}$

\begin{align}
    \sum_{\tb{\ti{s}}'\in \mathcal{S}} \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle &=  \langle \phi(\tb{\ti{s}}^{\prime} = \tb{\ti{g}}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle + \sum_{\tb{\ti{s}}' \neq \tb{\ti{g}}} \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle 
    \\
    & = 0 +  \langle (\tb{0}_{nd-1}, 1), (\theta^1, 1, \theta^2, 1,\dots, \theta^n, 1) \rangle \\ 
    &= 1.
\end{align}
This completes the proof. 
\end{proof}







==> Sections/extras1.tex <==
\begin{subsection}{Proposed Model}
    


Hey, I had come up with the following feature design
\begin{equation*}
\label{eqn: features_global}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  \tb{\ti{a}}) = 
\begin{cases} (\phi(s^{\prime^1} | s^1, \tb{\ti{a}}^1), \dots, \phi(s^{\prime^n} | s^n, \tb{\ti{a}}^n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}} and s^{i}=g \implies s^{\prime^i} = g  \forall i \in [N]
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}},   or if ~\tb{\ti{s}} \neq \tb{\ti{g}} but \exists i \in [N] s.t. s^{i}=g but s^{\prime^i} \neq g
\\
(\mb{0}_{nd-1}, 1), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}},
\end{cases}
\end{equation*}

where $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i)$ is defined as 
\begin{equation*}
\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) = \begin{cases}  
\left(-\tb{\ti{a}}^i, \frac{1-\delta}{k.2^k} \right)^{\top}, & if ~ {s}^i = s^{\prime^{i}} = s_{init}
\\
\left(\tb{\ti{a}}^i, \frac{\delta}{k.2^k} \right)^{\top}, & if ~ {s}^i = s_{init},~s^{\prime^{i}} = g
\\
\left(\mathbf{0}_{d-1}, \frac{1}{(n-k).2^{k+1}} \right)^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = g.
\end{cases}
\end{equation*}
Here $\mathbf{0}_d^{\top} = (0,0, \dots, 0)^{\top}$ is a vector of $d$ dimension with all zeros.
Thus, the features $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) \in \mathbb{R}^{nd}$. Moreover, the transition probability parameters are taken as $\boldsymbol{\theta} = \left( \boldsymbol{\theta}^1, 1,  \boldsymbol{\theta}^2, 1 \dots, \boldsymbol{\theta}^n, 1 \right)$ where $\boldsymbol{\theta}^i \in \left\lbrace -\frac{\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}  \right\rbrace^{d-1} $, and $\Delta < \delta$. Also, k represents the number of agents at $s_{init}$ in s. \\
\end{subsection}
\begin{subsection}{Why the above Model works}
Let's partition the set of all global transitions $( \tb{s}, \tb{\ti{a}}, \tb{s}^{\prime}) \in \mathcal{S}\times\mathcal{A}\times\mathcal{S}$ into the following: \pt{Note that the entire thing is true irrespective of the agent's action.}
\\
\begin{enumerate}
    \item When $\tb{s} = \tb{g}$ 
    \begin{enumerate}
        \item $\tb{s}^{\prime} = \tb{g}$ \\
        Corresponds to the third case in the definition of global $\phi(.|.,.)$
        \\
    Then, 
    \begin{align}
    \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
    \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
    & =\langle \phi((g,g,g,...,g)|(s,g,g,...,g),(a_1, a_2,...a_n)),\theta \rangle \\
    &= \langle (\tb{0}_{nd-1}, 1), (\theta_1, 1, \theta_2, 1, ..., \theta_n, 1) \rangle \\ 
    &= 1.
\end{align}   
        \item When $\tb{s}^{\prime} \neq \tb{g}$ \\ (This implies that there is at least one agent that moves back to $s_{init}$. Corresponds to first part of the second condition in the definition of global $\phi(.|.,.)$. This takes care of the $2^{n}-1$ impossible transitions for any global action)
        \begin{align}
    \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
    \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
    & =\langle \tb{0}_{nd},\theta \rangle \\
    &= 0.
    \end{align}
    \end{enumerate}
    \item When $\tb{s} \neq \tb{g}$
    \begin{enumerate}
        
        \item When there exists some agent who transits from g to $s_{init}$. \pt{This case was not considered in the previous feature design. And hence this probability was non-zero.} \\
        This corresponds to the "or" part of the second case in the definition of global $\phi(.|.,.)$

        \begin{align}
    \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
    \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
    & =\langle \tb{0}_{nd},\theta \rangle \\
    &= 0.
    \end{align}

        \item When there exists no agent who transits from g to $s_{init}$. \\ That means all agents either remain put in their original state or only transit from $s_{init}$ to $g$. This is the most general case and the most interesting one too. Takes care of all but the corner cases mentioned above.\\
        Consider a general initial state: $\tb{s} = (s_1,s_2,\dots,s_n)$ where agents $i_1, i_2, \dots, i_r$ are at $s_{init}$ while agents $j_1, j_2, \dots, j_{n-r}$ are already at g. We consider $r \geq 1$ as $r = 0$ is taken care of above. Let $\mathcal{I} := \{i_1, i_2, \dots, i_r\}$ and $\mathcal{J} := \{j_1, j_2, \dots, j_{n-r}\}$. Agents in $\mathcal{I}$ can transit to $s_{init}$ or g while those in $\mathcal{J}$ remain at g. Then, (where $\tb{s}^{\prime}$ denotes only a possible state i.e., not one of those discussed above with 0 probability of transition)
\begin{lalign}    \sum_{\tb{s}^{\prime}}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
 \\ &&\text{Just expand the notation} \\
&= \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})}\mathbb{P}((\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})| (\ti{s}^1, \ti{s}^2,...,\ti{s}^n), (\ti{a}^1, \ti{a}^2,...,\ti{a}^n))

\\ &&\text{Using Model} 

    \\ &=\sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2}, \dots ,\ti{s}^{\prime^n})}
    \langle \phi((\ti{s}^{\prime^1}, \ti{s}^{\prime^2}, \dots ,\ti{s}^{\prime^n})|(\ti{s}^1, \ti{s}^2,...,\ti{s}^n), (\ti{a}^1, \ti{a}^2,...,\ti{a}^n)),(\theta_1, 1, \theta_2, 1, ..., \theta_n, 1) \rangle \\
   \\&& \text{Using Features} \\ &=\sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})}
    \langle (\phi(\ti{s}^{\prime^1}|\ti{s}^1,\ti{a}^1), \phi(\ti{s}^{\prime^2}|\ti{s}^2,\ti{a}^2),...,\phi(\ti{s}^{\prime^n}|\ti{s}^n,\ti{a}^n)),(\theta_1, 1, \theta_2, 1, ..., \theta_n, 1) \rangle \\
    \\ &&\text{Individual Dot Products} \\
    &= \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})} \sum_{m = 1, 2,\dots,n}
    \langle \phi(\ti{s}^{\prime^m}|\ti{s}^m,\ti{a}^m),(\theta_m, 1) \rangle 
    \\ 
     &&\text{Sum over all agents broken into sum over two partition sets} \\
    &= \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})} \{(\sum_{i \in \mathcal{I}}
    \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle) + (\sum_{j \in \mathcal{J}}
    \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle)\}  \\ &&\text{Distributing the outer sum }\\
    &= \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},\dots ,\ti{s}^{\prime^n})} \sum_{i \in \mathcal{I}}
    \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle +  \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2}, \dots ,\ti{s}^{\prime^n})} \sum_{j \in \mathcal{J}}
    \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle
    \\ &&\text{Switching summations }\\
    &= \sum_{i \in \mathcal{I}} \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})}
    \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle +  \sum_{j \in \mathcal{J}} \sum_{(\ti{s}^{\prime^1}, \ti{s}^{\prime^2},...,\ti{s}^{\prime^n})} 
    \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle
    \\&&\text{Property of Summations }\\
&= \sum_{i \in \mathcal{I}} \Big\{  \sum_{\ti{s}^{\prime^1}} \sum_{\ti{s}^{\prime^2}} \dots \sum_{\ti{s}^{\prime^n}} \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle \Big \} + \sum_{j \in \mathcal{J}}  \Big \{  \sum_{\ti{s}^{\prime^1}} \sum_{\ti{s}^{\prime^2}} \dots \sum_{\ti{s}^{\prime^n}} \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle \Big \}
\\&&\text{'j' summations have only one choice (again according to property of summations)}\\
&= \sum_{i \in \mathcal{I}}
 \Big \{     \sum_{\ti{s}^{\prime^{i_1}}} \sum_{\ti{s}^{\prime^{i_2}}} \dots \sum_{\ti{s}^{\prime^{i_r}}} \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle \Big \} +  \sum_{j \in \mathcal{J}}  \Big \{  \sum_{\ti{s}^{\prime^{i_1}}}     \sum_{\ti{s}^{\prime^{i_2}}} \dots
\sum_{\ti{s}^{\prime^{i_r}}} 
    \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle \}
    \\
\\&& \text{Fixing an outer 'i', every other i has two choices hence $2^{r-1}$ but fixing outer 'j' every other 'i' still has 2 choices hence $2^r$.}
    \\
    &=  \sum_{i \in \mathcal{I}} \{2^{r-1}. \sum_{\ti{s}^{\prime^i}}
    \langle \phi(\ti{s}^{\prime^i}|\ti{s}^i,\ti{a}^i),(\theta_i, 1) \rangle \} +  \sum_{j \in \mathcal{J}} \{  2^r. 
    \langle \phi(\ti{s}^{\prime^j}|\ti{s}^j,\ti{a}^j),(\theta_j, 1) \rangle \}
    \\
    & \text{\pt{This is not clear, why we get $2^{r-1}$ and $2^r$? }}
    \\ 
     &= 
     \sum_{i \in \mathcal{I}} \{2^{r-1}. 
    \langle (0_{d-1}, \frac{1}{r.2^r})),(\theta_i, 1) \rangle \} +  \sum_{j \in \mathcal{J}} \{  2^r.  
    \langle (0_{d-1}, \frac{1}{(n-r).2^{r+1}}),(\theta_j, 1) \rangle \} 
     \\
     &= 
     \sum_{i \in \mathcal{I}} \frac{1}{2.r} +  \sum_{j \in \mathcal{J}} \frac{1}{2.(n-r)} 
     \\
     &= \frac{1}{2} + \frac{1}{2}
    \\
    & = 1.
\end{lalign}
\\

    \textcolor{brown}{Also need to show that all probabilities lie between 0 and 1. This leads to $\delta = O(2^n.\Delta) = o(1)$. But I haven't shown so far. } \\

\pt{Surprisingly, there are no terms involving $\delta$ in your entire proof. What happen to such terms?}\\
\textcolor{blue}{DOUBT ON POWERS OF 2 - I think maybe now it's clearer, I added a couple of intermediate steps. It's just mathematical simplification. 
}\\
\textcolor{blue}{ The sum over all global s' can be written as nested summations (standard technique in such summations). These summations can be permuted freely. If you permute such that the i fixed from the outer sum is the innermost summation, you will observe that this summation remains constant for all outside summations over each possibility of state. As there are 2 possibilities for $s^{\prime^l}$ for every l and as there are r-1 such states outside, factor of 2 from each of those results in $2^{r-1}$. In the sum over j, there are r states (outer summations) with the constant inner term hence $2^r$. A standard doubt may be why it is multiplying and not adding. Try to expand any nested summation and you will see why!}
\textcolor{blue}{WHY NO $\delta$ - When you add, over possible $s^{\prime^i}$ (i.e. s and g) in the first summation, you can observe that the $\delta$ terms in the corresponding features add in such a way that they cancel each other. I just haven't written explicitly that step, but it's too trivial.}
\pt{we should write the proof in more details and clean it with more readability?}
\textcolor{blue}{Absolutely, there are plenty many things I've to add. Once I add them all, we can make it more detailed.}

\pt{Still it is not clear to me. Is there a way to simplify this proof. These notations, etc are very complicated. }

\textcolor{blue}{I don't think it can be simplified. The notations were meant to simplify the transitions between steps.}
        
    \end{enumerate}
\end{enumerate}
    
\end{subsection}


Recall, the global features defined in the MACCM paper are given by
\begin{equation*}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  \tb{\ti{a}}) = 
\begin{cases} (\phi(s^{\prime^1} | s^1, \tb{\ti{a}}^1), \dots, \phi(s^{\prime^n} | s^n, \tb{\ti{a}}^n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}},
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}},
\\
(\mb{0}_{nd-1}, 2^{n-1}), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}},
\end{cases}
\end{equation*}
where $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i)$ is defined as 
\begin{equation*}
\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) = \begin{cases}  
\left(-\tb{\ti{a}}^i, \frac{1-\delta}{n} \right)^{\top}, & if ~ {s}^i = s^{\prime^{i}} = s_{init}
\\
\left(\tb{\ti{a}}^i, \frac{\delta}{n} \right)^{\top}, & if ~ {s}^i = s_{init},~s^{\prime^{i}} = g
\\
\mathbf{0}_{d}^{\top}, & if ~ {s}^i = g,~s^{\prime^{i}} = s_{init}
\\
\left(\mathbf{0}_{d-1}, \frac{1}{n} \right)^{\top}, & if ~ {s}^i = g,~ s^{\prime^{i}} = g.
\end{cases}
\end{equation*}
Here $\mathbf{0}_d^{\top} = (0,0, \dots, 0)^{\top}$ is a vector of $d$ dimension with all zeros.
Thus, the features $\phi(s^{\prime^{i}} | s^i, \tb{\ti{a}}^i) \in \mathbb{R}^{nd}$. Moreover, the transition probability parameters are taken as $\boldsymbol{\theta} = \left( \boldsymbol{\theta}^1, \frac{1}{2^{n-1}},  \boldsymbol{\theta}^2, \frac{1}{2^{n-1}} \dots, \boldsymbol{\theta}^n, \frac{1}{2^{n-1}} \right)$ where $\boldsymbol{\theta}^i \in \left\lbrace -\frac{\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}  \right\rbrace^{d-1} $, and $\Delta < \delta$. 

However, these features doesn't capture the following case.

Let $\tb{\ti{s}} = (s, g, g,..., g)$ and  $\tb{\ti{s}}^{\prime} =(s, g, g, ..., s)$. Let's check the probability of transition under an arbitrary global action $\tb{\ti{a}} = (a_1, a_2,...,a_n)$ using the given model: 
\begin{align}
    \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
    \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
    & =\langle \phi((s,g,g,...,s)|(s,g,g,...,g),(a_1, a_2,...a_n)),\theta \rangle \\
    &= \langle (\phi(s|s,a_1), \phi(g|g,a_2),...\phi(s|g,a_n)), (\theta_1, \frac{1}{2^{n-1}}, \theta_2, \frac{1}{2^{n-1}}, ..., \theta_n, \frac{1}{2^{n-1}}) \rangle \\ 
    &= \langle ((-a_1, \frac{1-\delta}{n}), (0_{d-1}, \frac{1}{n}), ..., (0_d)), ( \theta_1, \frac{1}{2^{n-1}}, \theta_2, \frac{1}{2^{n-1}}, ..., \theta_n ,  \frac{1}{2^{n-1}})  \rangle \\
    &= \langle -a_1, \theta_1 \rangle + \frac{1-\delta}{n} . \frac{1}{2^{n-1}} + \frac{1}{n} . \frac{1}{2^{n-1}} . (n-2) + 0 
    \\
    & \neq 0.
\end{align}

Therefore, the above feature design is not capturing the transition probabilities correctly. 

Note that if we use the above feature design along with the condition that $\mathbb{P}(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}) = 0$, if any agent $i$ is transitioning from $s^i = g$ to  $s^{\prime^i} = s_{\text{init}}$. Then, we get the following

\begin{align}
    \sum_{\tb{\ti{s}}^{\prime}} \mathbb{P}(\tb{\ti{s}}^{\prime} | \tb{\ti{s}}, \tb{\ti{a}}) = \frac{r  2^{r-1} 
    + (n-r) 2^r}{n \cdot 2^{n-1}} \neq 1,
\end{align}
where $r$ is total number of agent at $s_{\text{init}}$ in the current state $\tb{\ti{s}}$.

\pt{Utkarsh -- try to see if you can proof the above result, and using this you can adjust your features or the $\boldsymbol{\theta}$ vector.}



..... 

\pt{Here I am copying what you have written Utkarsh in the proofs.}



\dots

\begin{enumerate}
    \item When $\tb{\ti{s}} = \tb{g}$ 
    \begin{enumerate}
        \item $\tb{\ti{s}}^{\prime} = \tb{g}$ \\
        Corresponds to the third case in the definition of global $\phi(.|.,.)$(\ref{eqn:features_global_new})
        \\
        Then, using Assumption \ref{assm:lfa_prob} and features (\ref{eqn:features_global_new}, \ref{eqn:features_global_new_gen}), for any $\tb{\ti{a}} \in \mathcal{A}$
        \begin{align}
        \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
        \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
         & =\langle \phi((g,g,g,\dots,g)|(g,g,g,\dots,g),(a_1, a_2,\dotsa_n)),\boldsymbol{\theta} \rangle \\
         &= \langle (\tb{0}_{nd-1}, 1), (\theta_1, 1, \theta_2, 1, \dots, \theta_n, 1) \rangle \\ 
         &= 1.
        \end{align}   
        \item When $\tb{\ti{s}}^{\prime} \neq \tb{g}$ \\ This implies that there is at least one agent that moves back to node $s$. Corresponds to first part of the second condition in the definition of global $\phi(.|.,.)$ (\ref{eqn:features_global_new}). This takes care of the $2^{n}-1$ impossible transitions for any global action. Using Assumption \ref{assm:lfa_prob} and features (\ref{eqn:features_global_new}, \ref{eqn:features_global_new_gen}) for any global action $\tb{\ti{a}} \in \mathcal{A}$
        \begin{align}
        \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
        \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
        & =\langle \tb{0}_{nd},\theta \rangle \\
        &= 0.
        \end{align}
    \end{enumerate}
    \item When $\tb{\ti{s}} \neq \tb{g}$
        \begin{enumerate}
        \item When there exists some agent who transits from node $g$ to node $s$. This captures all the remaining impossible transitions for any action.
        This corresponds to the "or" part of the second case in the definition of global $\phi(.|.,.)$ (\ref{eqn:features_global_new}). Using Assumption \ref{assm:lfa_prob} and features (\ref{eqn:features_global_new}, \ref{eqn:features_global_new_gen}), for any global action $\tb{\ti{a}} \in \mathcal{A}$
        \begin{align}
        \mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) &=
        \langle \phi(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) ,\boldsymbol{\theta} \rangle \\
        & =\langle \tb{0}_{nd},\theta \rangle \\
        &= 0.
        \end{align}
        \item When there exists no agent who transits from node $g$ to node $s$. \\ That means any agent either remains put in its original node (either $s$ or $g$) or only transit from node $s$ to node $g$. This is the most general and the most interesting case. Corner cases are taken care of above.\\
        Consider a general initial state: $\tb{\ti{s}} = (s_1,s_2,\dots,s_n)$ where agents in $\mathcal{I}:=\{i_1, i_2, \dots, i_r \}$ are at node $s$ while agents in $\mathcal{J}:= \{j_1, j_2, \dots, j_{n-r} \}$ are already at node g. Here, we only consider $r \geq 1$ since $r = 0$ is taken care of above. Agents in $\mathcal{I}$ can either stay at node $s$ itself or transit to $g$ while those in $\mathcal{J}$ remain at $g$. Let $\mathcal{S}(\tb{\ti{s}})$ represent the set of all possible next states from $\tb{\ti{s}}$. \\
        Then, using Assumption \ref{assm:lfa_prob} and features (\ref{eqn:features_global_new}), for any $\tb{\ti{a}} = \{a_1,a_2,\dots,a_n\} \in \mathcal{A}$: 
    \begin{align}    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
    &= \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)}\mathbb{P}(({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)| ({s}_1, {s}_2,\dots,{s}_n), ({a}_1, {a}_2,\dots,{a}_n))
    \\ &=\sum_{({s}^{\prime}_1, {s}^{\prime}_2, \dots ,{s}^{\prime}_n)}
    \langle \phi((\ti{s}^{\prime}_1, {s}^{\prime}_2, \dots ,{s}^{\prime}_n)|({s}_1, {s}_2,\dots,{s}_n), ({a}_1, {a}_2,\dots,{a}_n)),(\theta_1, 1, \theta_2, 1, \dots, \theta_n, 1) \rangle \\
    &=\sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)}
    \langle (\phi({s}^{\prime}_1|{s}_1,{a}_1), \phi({s}^{\prime}_2|{s}_2,{a}_2),\dots,\phi({s}^{\prime}_n|{s}_n,{a}_n)),(\theta_1, 1, \theta_2, 1, \dots, \theta_n, 1) \rangle \\
    &= \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)} \sum_{m \in [n]}
    \langle \phi({s}^{\prime}_m|{s}_m,{a}_m),(\theta_m, 1) \rangle 
    \end{align}
    In the below step, we split the summation into two set of agents based on which node they are present at. This helps us later to exploit the similarity in the number of times the local inner product $\langle \phi(s'_i|s_i,a_i),(\theta_i,1)\rangle$ appears in the entire sum. 
    \begin{align}
    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
    &= \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)} \Bigg\{\sum_{i \in \mathcal{I}}
    \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}}
    \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \Bigg \}  \\ 
    &= \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots ,{s}^{\prime}_n)} \sum_{i \in \mathcal{I}}
    \langle \phi(\ti{s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle +  \sum_{({s}^{\prime}_1, {s}^{\prime}_2, \dots ,{s}^{\prime}_n)} \sum_{j \in \mathcal{J}}
    \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle
    \\ 
    &= \sum_{i \in \mathcal{I}} \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)}
    \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle +  \sum_{j \in \mathcal{J}} \sum_{({s}^{\prime}_1, {s}^{\prime}_2,\dots,{s}^{\prime}_n)} 
    \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle
    \\
    &= \sum_{i \in \mathcal{I}} \Big\{  \sum_{{s}^{\prime}_1} \sum_{{s}^{\prime}_2} \dots \sum_{{s}^{\prime}_n} \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle \Big \} + \sum_{j \in \mathcal{J}}  \Big \{  \sum_{{s}^{\prime}_1} \sum_{{s}^{\prime}_2} \dots \sum_{{s}^{\prime}_n} \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \Big \}
    \end{align}
    Since for any $j \in \mathcal{J}, s'_j \equiv g$, 
    \begin{align}
    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
&= \sum_{i \in \mathcal{I}}
 \Big \{     \sum_{{s}^{\prime}_{i_1}} \sum_{{s}^{\prime}_{i_2}} \dots \sum_{{s}^{\prime}_{i_r}} \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle \Big \} +  \sum_{j \in \mathcal{J}}  \Big \{  \sum_{{s}^{\prime}_{i_1}}     \sum_{{s}^{\prime}_{i_2}} \dots
\sum_{{s}^{\prime}_{i_r}} 
    \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \Big \}
    \end{align}
    For any fixed $i \in \mathcal{I},$ the $\sum_{{s}^{\prime}_i}
    \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle $ doesn't depend on next state of other agents in $\mathcal{I}$. Similarly for any $j \in \mathcal{J}, \langle \phi(\ti{s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle $ doesn't depend on next state of any agent in $\mathcal{I}$. Hence,
    \begin{align}
    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
    &=  \sum_{i \in \mathcal{I}} \{2^{r-1}. \sum_{{s}^{\prime}_i}
    \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle \} +  \sum_{j \in \mathcal{J}} \{  2^r. 
    \langle \phi(\ti{s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \}
    \end{align}
    Using features (\ref{eqn:features_global_new_gen})
    \begin{align}
    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
     &= 
     \sum_{i \in \mathcal{I}} \{2^{r-1}. 
    \langle (0_{d-1}, \frac{1}{n.2^{r-1}})),(\theta_i, 1) \rangle \} +  \sum_{j \in \mathcal{J}} \{  2^r.  
    \langle (0_{d-1}, \frac{1}{n.2^{r}}),(\theta_j, 1) \rangle \} 
     \\
     &= 
     \sum_{i \in \mathcal{I}} \frac{1}{n} +  \sum_{j \in \mathcal{J}} \frac{1}{n} 
     \\
     &= \frac{r}{n} + \frac{n-r}{n}
    \\
    & = 1.
    \end{align}
\end{enumerate}


    Since for any $j \in \mathcal{J}, s'_j \equiv g$, 
    \begin{align}
    &\sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \\
    &= \sum_{i \in \mathcal{I}}
     \Big \{     \sum_{{s}^{\prime}_{i_1}} \sum_{{s}^{\prime}_{i_2}} \dots \sum_{{s}^{\prime}_{i_r}} \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle \Big \} +  \sum_{j \in \mathcal{J}}  \Big \{  \sum_{{s}^{\prime}_{i_1}}     \sum_{{s}^{\prime}_{i_2}} \dots
    \sum_{{s}^{\prime}_{i_r}} 
    \langle \phi({s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \Big \}
\end{align}

For any fixed $i \in \mathcal{I},$ the $\sum_{{s}^{\prime}_i}
\langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle $ doesn't depend on next state of other agents in $\mathcal{I}$. Similarly for any $j \in \mathcal{J}, \langle \phi(\ti{s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle $ doesn't depend on next state of any agent in $\mathcal{I}$. Hence,
\begin{align}
    \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) 
    & =  \sum_{i \in \mathcal{I}} \bigg\{2^{r-1} \sum_{{s}^{\prime}_i}
    \langle \phi({s}^{\prime}_i|{s}_i,{a}_i),(\theta_i, 1) \rangle \bigg\} +  \sum_{j \in \mathcal{J}} \bigg\{  2^r  
    \langle \phi(\ti{s}^{\prime}_j|{s}_j,{a}_j),(\theta_j, 1) \rangle \bigg\}
\end{align}
Using features in Equation (\ref{eqn:features_global_new_gen})
\begin{align}
    \sum_{\tb{\ti{s}}^{\prime} \in \mathcal{S}(\tb{\ti{s}})}\mathbb{P}(\tb{\ti{s}}^{\prime}| \tb{\ti{s}}, \tb{\ti{a}}) \nonumber
     &= 
     \sum_{i \in \mathcal{I}} \bigg\{2^{r-1}. 
    \langle (0_{d-1}, \frac{1}{n.2^{r-1}})),(\theta_i, 1) \rangle \bigg\} +  \sum_{j \in \mathcal{J}} \bigg\{  2^r.  
    \langle (0_{d-1}, \frac{1}{n.2^{r}}),(\theta_j, 1) \rangle \bigg\} 
     \\
     &= 
     \sum_{i \in \mathcal{I}} \frac{1}{n} +  \sum_{j \in \mathcal{J}} \frac{1}{n} 
     \\
     &= \frac{r}{n} + \frac{n-r}{n}
    \\
    & = 1.
\end{align}

It remains to check that individual transition probabilities also lie in $[0,1]$. \\
For the transitions from $\tb{\ti{s}}=\tb{g}$ and other impossible transitions, we saw above that this holds. \\
For general transitions, we check below. \\
Consider any instance $n\geq1,\theta \in \Theta, \delta \in (2/5,1/2), \Delta < 2^{-n}\frac{1-2\delta}{1+n+n^2}$. \\
For any $r \in [n], r' \in [r] \cup \{0\}$, consider any $\tb{\ti{s}} \in \mathcal{S}(r)$, $\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})$ and any action $\tb{\ti{a}} \in \mathcal{A}$.  

\begin{align}
    \Delta & <  \frac{2^{-n} (1-2\delta)}{1+n+n^2} <  \frac{2^{-n} \cdot 2  \delta}{3}
\end{align}

    The above follows since for $\delta \in (2/5,1/2)$, $1-2\delta<2\delta$ and for $n\geq 1, 1+n+n^2 \geq 3$. \\ Further as $r \leq n$, \\
    \begin{align}
    &\delta > 3.2^{n-1}.\Delta \\
    &\implies \delta > 3.2^{r-1}.\Delta \\
    &\Longleftrightarrow \frac{\delta}{2^{r-1}} - 3\Delta>0 \\
    &\Longleftrightarrow \frac{( -0.5n)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta > 0 
    \end{align} 

    Since for any $r \in [n], 0\leq r' \leq r, \delta \in (2/5,1/2)$ we have $r'-0.5r \geq -0.5n$, the above implies: 
    \begin{align}
     &\frac{( r'-0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta > 0 \\
    &\Longleftrightarrow \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} - 3\Delta > 0 
    \end{align}
    Since $r' \leq r \leq n$ we have $\frac{\Delta}{n}(r-2r') \geq -\Delta$. Hence,
    \begin{align}
    &\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') -  \frac{2 \Delta}{1} > 0 \end{align}


    As indicator function can take only $0$ and $1$ values, \\ $\sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \geq -(r-r') \geq -r \geq -n $. \\ Thus, we have, along with the general transition probability expression from \ref{lemma:general_tp},
    \begin{align}
    &\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') \\
    &\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{   \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} > 0 \\
    &\quad \Longleftrightarrow p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'} > 0
\end{align}



Similarly, 
\begin{align}
    &2/5 < \delta < 1/2, \Delta < 2^{-n}.\frac{1-2\delta}{1+n+n^2}, n\geq 1 \\
    &\implies \Delta < 2^{-n} . \frac{2\delta}{3} \\
    &\Longleftrightarrow \delta > 3.2^{n-1}.\Delta \\
    &\implies \delta > 3\Delta \\
    &\Longleftrightarrow 1>1-\delta+3\Delta \\
    &\implies 1> \frac{0.5n(2-2\delta)}{n.2^{r-1}} + 3\Delta \\
    &\implies 1> \frac{(r'-0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} +    3\Delta \\
    &\Longleftrightarrow 1>  \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} +    3\Delta  \\
    &\implies 1> \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{1} \\ 
    &\implies 1>  \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') + \\
    &\quad \frac{2 \Delta}{n(d-1)}\sum_{p \in [d-1]}  \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \\
    &\Longleftrightarrow 1>p^{\tb{\ti{a}}}_{\tb{\ti{s}},{s^\prime}}
\end{align}

Hence, the features described in Equation \eqref{eqn:features_global_new},\ref{eqn:features_global_new_gen} along with the transition probability  (Assumption \ref{assm:lfa_prob}) define valid instances.

\subsection{Proof of Lemma \ref{lemma:general_tp}}

Suppose $\tb{\ti{s}} \in \mathcal{S}\setminus\{\goal\}$ is such that agents at index in $\mathcal{I}:= \{i_1,i_2,\dots, i_r\}$ are at node $s$ and those at $\mathcal{J} := \{j_1,j_2,\dots, j_{n-r}\}$ are already at node $g$. Let agents in $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ be the ones transiting from node $s$ to node $g$ i.e., $\tb{\ti{s}} \in \mathcal{S}(r)$ and $s' \in \mathcal{S}(r')$ where $n \geq r \geq r' \geq 0$ and $n \geq 1$. 

Then using \ref{assm:lfa_prob}: 
\begin{align} 
\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) &= \langle \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}), \theta \rangle \\
&= \langle \phi((s'_1,s'_2,\dots,s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n) ), (\theta_1,1,\theta_2,1,\dots,\theta_n,1)\rangle
\end{align} 
Using Equation \eqref{eqn:features_global_new}, 
\begin{align}
&\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \\
&= \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots, \theta_n,1) \rangle  \\
&= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle \phi(s|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle \phi(g|s,a_t), (\theta_t,1) \rangle \\
\end{align}

Using Equation \eqref{eqn:features_global_new_gen}
\begin{align}
&\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \\
&= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle (-a_i, \frac{1-\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j, 1) \rangle  + \sum_{t \in \mathcal{T}} \langle (a_t, \frac{\delta}{n.2^{r-1}}), (\theta_t,1) \rangle \\
&= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \Big \{ \frac{1-\delta}{n.2^{r-1}} + \langle -a_i, \theta_i \rangle \Big \} + \sum_{j \in \mathcal{J}}   \frac{1}{n.2^{r}}  + \sum_{t \in \mathcal{T}} \Big \{ \langle a_t,\theta_t  \rangle + \frac{\delta}{n.2^{r-1}} \Big \}   \\
&=  r'. \frac{1-\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}  + (r-r'). \frac{\delta}{n.2^{r-1}} + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\
&= \frac{r' + (r-2r')\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}   + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle 
\end{align} 



Since for any $i \in [n], a_i \in \{-1,1\}^{d-1}, \theta_i \in \Big \{ \frac{-\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)} \Big \}^{d-1}$, we have:
\begin{align}
&\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \\
&= \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} a_{i,p}. \theta_{i,p}      + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   a_{t,p} .\theta_{t,p}  \\
&= \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} \\
&\quad - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{\sgn(a_{i,p}) = \sgn(\theta_{i,p})\} -  \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Big \}     \\
&\quad + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{\sgn(a_{t,p}) = \sgn(\theta_{t,p})\} -  \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}  \\
&= \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} \\
&\quad - \sum_{i \in \mathcal{I} \cap \mathcal{T'}}  \frac{\Delta}{n(d-1)} \Big \{  d-1 -  2 \sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Big \}   \\
&\quad + \sum_{t \in \mathcal{T}}    \frac{\Delta}{n(d-1)} \Big \{  d-1 - 2\sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}  \\
&= \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}   \\
&\quad - \frac{\Delta}{n(d-1)} \Big \{  r'(d-1) -  2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Big \}  \\
&\quad +    \frac{\Delta}{n(d-1)} \Big \{  (r-r').(d-1) - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \\
&=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}      \\
&\quad +    \frac{\Delta}{n(d-1)} \Big \{  (r-2r').(d-1) \Big \} + \frac{2\Delta}{n(d-1)}. \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \\
&\quad - \frac{2\Delta}{n(d-1)} . \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \\
&=  \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')  + \\
&\quad \frac{2 \Delta}{n(d-1)}\sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}  -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} 
\end{align}

  


Proof of Claim \ref{claim:probability_inequality}


For any of our instances ($n \geq 1, 2/5< \delta <1/2, \Delta<2^{-n}\frac{1-2\delta}{1+n+n^2}$ ), consider any $r \in [n]$. 

\tb{For $0 \leq r'\leq \lfloor\frac{r+1}{2}\rfloor$}, \\

For any of our instances, 
\begin{align}
& \Delta < \frac{1-2\delta}{2^{n}(1+n+n^2)} 
\\
&\implies \Delta < \frac{1-2\delta}{2^{n} (1+n+\frac{n^2}{8})} \\
&\Longleftrightarrow \Delta (\frac{n^2}{8}+n+1)<\frac{1-2\delta}{2^{n}} 
\end{align}
Since $0 \leq r \leq n,$ we have $\frac{n^2}{8}+n+1 \geq \frac{r^2}{8}+r+1$. \\
Also, $\frac{(r+1)}{2^{r+1}} \geq \frac{1}{2^n}$. \\
As $2/5 < \delta < 1/2$, we have:
\begin{align}
& \frac{\Delta}{n}(\frac{r^2}{8}+r+1)<(r+1)\frac{1-2\delta}{n2^{r+1}} \\
&\Longleftrightarrow \frac{\Delta}{n}\frac{r^2}{8} + (r+1) \frac{\Delta}{n}<(r+1)\frac{1-2\delta}{n2^{r+1}} 
\end{align}
As $0\leq r' \leq r, r'(r-2r') \leq r^2/8$. Thus, \\
\begin{align}
&(r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0 
\end{align}
Since we are considering $0 \leq r' \leq \lfloor\frac{r+1}{2}\rfloor$, we have $\frac{2r'-(r+1)}{2} \leq 0$. \\
Also, since $0 \leq r' \leq r \leq n, \delta \in (2/5,1/2)$, we have $0.5n + (1-2\delta)(r'-0.5r) \geq 0.5n + (1-2\delta)(-0.5r) \geq 0.5n + (1-2\delta)(-0.5n) = n(1-\delta) > 0.$\\
Using above,
\begin{align}
&\Big \{\frac{2r'-(r+1)}{2} \Big \}. \Big \{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}} \Big \} +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0 \\
& \Longleftrightarrow (r+1).\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}\Big\}  + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')< \\
& \quad (r+1-r').\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}} \Big \}    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\
& \Longleftrightarrow  (r+1).\Big \{\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r') \Big \} \\
&  
\quad < (r+1-r').\Big \{ \frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')\Big \}
\\
& \Longleftrightarrow (r+1).\Big\{\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r')\Big\}
\\ 
& \quad < (r+1-r').\Big \{\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n \cdot 2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')\Big \} \\
& \Longleftrightarrow (r+1).\Big \{\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r') \Big \}
\\
& \quad < (r+1-r').\Big \{\frac{r' + (r-2r')\delta}{n \cdot 2^{r-1}} +   \frac{n-r}{n \cdot 2^r}        +    \frac{\Delta}{n}  (r-2r') \Big \} 
\\
& \Longleftrightarrow  \frac{r+1}{r+1-r'}p^*_{r+1,r'}<p^*_{r,r'} \\
& \Longleftrightarrow  \binom{r+1}{r'} p^*_{r+1,r'}
 < \binom{r}{r'}p^*_{r,r'} 
\end{align}
In the last second step, we use the expression for $p^*_{r+1,r'}$ and $p^*_{r,r'}$ from the general transition probability expression in Lemma \ref{lemma:general_tp}. 

Similarly, \\ \tb{For $r' > \lfloor \frac{r+1}{2} \rfloor$}, \\
Again, for any of our instances, we have:
\begin{align}
     \Delta  < \frac{1-2\delta}{(n^2+n+1).2^{n}},  1/2>\delta>2/5 
\end{align}
Since for this range of $\delta$ we have, $1-2\delta < 3\delta-1,$ we obtain:
\begin{align}
      \Delta & < \frac{3\delta-1}{(n^2+n+1).2^{n}} 
      \\
      \Longleftrightarrow & \Delta  (n^2+n+1)  (2^{n})
      < 3\delta-1 
      \end{align}
As $n \geq 1$, using above and $\delta \in (2/5,1/2)$, we have:
\begin{align}
      &n > \frac{0.5-\delta}{2\delta-0.5}+ \frac{\Delta  (n^2+n+1)  (2^{n})}{2\delta-0.5} 
      \\
      \Longleftrightarrow  & (2\delta-0.5)n > 0.5-\delta +  \Delta  (n^2+n+1)  (2^{n}) 
      \\
      \Longleftrightarrow  & 0.5n-n+2n\delta-0.5+\delta >   \Delta  (n^2+n+1)  (2^{n}) 
      \end{align}
      Since for $n \geq 1$ we have $n^2+n+1 \geq n^2-n-1$. Thus:
      \begin{align}
      & (-n-0.5)(1-2\delta)+0.5n    >   \Delta  (n^2-n-1)  (2^{n}) 
      \end{align}
      As $n \geq r, \delta \in (2/5,1/2),$ we have:
      \begin{align}
      & \frac{(-r-0.5)(1-2\delta)+0.5n }{1}   >   \frac{\Delta}{1}  (r^2-r-1)  (2^{r}) \\
      \Longleftrightarrow & \frac{(-r-0.5)(1-2\delta)+0.5n }{n.2^{r}}   >   \frac{\Delta}{n}  (r^2-r-1) 
      \end{align}


     Further since $r \geq r'\geq \lfloor \frac{r+1}{2}\rfloor$, we have $r \cdot r'-2r'^2 \geq -r^2$. \\
      Also, using $\delta \in (2/5,1/2)$,
      \begin{align}
      & \frac{(r'-r-0.5)(1-2\delta)+0.5n }{n \cdot 2^r} +  \frac{\Delta}{n}  (1+r+r \cdot r'-2r'^2)  >0 \\
      \Longleftrightarrow & \frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^r} \\
      & \quad +  \frac{\Delta}{n}  (1+r+r \cdot r'-2r'^2) - 0.5(r+1)(\frac{1-2\delta}{n \cdot 2^r}) >0 \\
      \Longleftrightarrow  & (\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^r}) \\
      & \quad +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n \cdot 2^r} + \frac{\Delta}{n}) >0  \label{}
      \end{align}

      As $r' \geq \lfloor \frac{r+1}{2} \rfloor$, we have $\frac{2r'-(r+1)}{2} \geq 1/2$. Hence, \textcolor{blue}{we can simplify the above,}

      \begin{align}
        & \Big\{\frac{2r'-(r+1)}{2}\Big\}.\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}}\Big\}  \\
      & \quad + (r')\frac{\Delta}{n}  (r-2r') + (r+1)\Big \{\frac{\delta-0.5}{n \cdot 2^r} + \frac{\Delta}{n} \Big\}>0 \\
      \Longleftrightarrow  &  (r+1).\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^r}\Big\} \\
      & \quad + (r+1)\Big\{\frac{\delta-0.5}{n \cdot 2^r} + \frac{\Delta}{n}\Big\}     +    (r+1)\frac{\Delta}{n}  (r-2r')
      \\
      & \quad > (r+1-r').\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}}\Big\}    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\
      \Longleftrightarrow &   (r+1).\Big\{\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n \cdot 2^r}    +    \frac{\Delta}{n}  (r+1-2r')\Big\}
      \\
      & \quad >(r+1-r').\Big\{\frac{(r'-0.5r)(1-2\delta)+0.5n }{n \cdot 2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')\Big\}   \\
      \Longleftrightarrow & (r+1).\Big\{\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n \cdot 2^r}    +    \frac{\Delta}{n}  (r+1-2r')\Big\}
      \\
      & \quad >(r+1-r').\Big\{\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n \cdot 2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')\Big\}  \\
      \Longleftrightarrow &  (r+1).\Big \{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r')\Big\}
      \\
      & \quad >(r+1-r').\Big\{\frac{r' + (r-2r')\delta}{n \cdot 2^{r-1}} +   \frac{n-r}{n \cdot 2^r}        +    \frac{\Delta}{n}  (r-2r')\Big\}
      \\
      \Longleftrightarrow & \frac{r+1}{r+1-r'}p^*_{r+1,r'}>p^*_{r,r'} \\
      \Longleftrightarrow &  \binom{r+1}{r'}p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'} 
\end{align}


\subsection{Proof of Lemma \ref{lemma:probability_inequality}}

\textbf{Recall Lemma \ref{lemma:probability_inequality}:}
\textit{ If for every $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.}

\begin{proof} 
By definition of $V^*,$
\begin{align}
    V^*_r & = 1+\sum_{r'=0}^{r} \binom{r}{r'} p^*_{r,r'} V^*_{r'}, \quad \text{and}
    \\
    V^*_{r+1} &= 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r'=0}^{r}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'}
\end{align}
From the lemma hypothesis, we have
\begin{align}
    \binom{r+1}{r'} p^*_{r+1,r'} 
    &= \binom{r}{r'}p^*_{r,r'}-\delta_{r'}, \quad \forall
    ~~r' \in \{0,1,2,\dots,\lfloor\frac{r+1}{2}\rfloor\},
    \\
    \binom{r+1}{r'} p^*_{r+1,r'}
    & =
    \binom{r}{r'}p^*_{r,r'}+\delta_{r'}, \quad \forall ~~ r' \in \{\lfloor \frac{r+1}{2} \rfloor\ +1 , \lfloor\frac{r+1}{2}\rfloor+2,\dots,r-1,r\}
\end{align}
As Claim \ref{claim:probability_inequality} holds for our instances, \\
suppose for every $r' \in \{0,1,2,\dots,\lfloor\frac{r+1}{2}\rfloor\}$, 
\begin{align}
    \binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}-\delta_{r'} 
\end{align}
and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor\ +1 , \lfloor\frac{r+1}{2}\rfloor+2,\dots,r-1,r\}$, 
\begin{align}
\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}+\delta_{r'}
\end{align}
where $\delta_{r'}>0$ for every $r' \in \{0,1,\dots,r\}$\\ 

Note that, 
\begin{align}
&\sum_{r'=0}^{r+1} \binom{r+1}{r'}p^*_{r+1,r'} = 1 \\
    &\Longleftrightarrow\sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \binom{r+1}{r'}p^*_{r+1,r'} + \sum_{r'=\lfloor \frac{r+1}{2} \rfloor +1}^{r} \binom{r+1}{r'}p^*_{r+1,r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1\\
    &\Longleftrightarrow \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \Big\{\binom{r}{r'}p^*_{r,r'}-\delta_{r'} \Big\} + \sum_{ r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \Big \{ \binom{r}{r'}p^*_{r,r'} + \delta_{r'} \Big\} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\
    &\Longleftrightarrow \sum_{r'=0}^{ \lfloor \frac{r+1}{2} \rfloor} \binom{r}{r'}p^*_{r,r'}-\sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'} + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \binom{r}{r'}p^*_{r,r'} + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\
    &\Longleftrightarrow p^*_{r+1,r+1} = \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'}  -  \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1 }^{ r } \delta_{r'} + 1 -  \sum_{0 \leq r' \leq r} \binom{r}{r'}p^*_{r,r'} \\
    &\Longleftrightarrow p^*_{r+1,r+1} = \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'}  -  \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'} \label{eqn:p_r_r}
\end{align}
Now, going back: 
\begin{align}
&V^*_{r+1}  \\
&=1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' = 0}^r \binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'}  \\
&= 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' = 0}^ {\lfloor \frac{r+1}{2} \rfloor} \binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'}  +  \sum_{r'= \lfloor \frac{r+1}{2} \rfloor +1}^{r}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} \\
&= 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \Big\{\binom{r}{r'}p^*_{r,r'} - \delta_{r'}\Big\}V^*_{r'}  +  \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{ r}\Big\{\binom{r}{r'}p^*_{r,r'}+\delta_{r'} \Big\}V^*_{r'} \\
&= 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' =0}^{ \lfloor \frac{r+1}{2} \rfloor}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' =0}^{ \lfloor \frac{r+1}{2} \rfloor} \delta_{r'} V^*_{r'}  + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \binom{r}{r'}p^*_{r,r'} V^*_{r'}+ \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'}V^*_{r'} \\
&= 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' = 0}^{r} \binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'} V^*_{r'}  +  \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'}V^*_{r'} \\
&=   p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' = 0}^{ \lfloor \frac{r+1}{2} \rfloor} \delta_{r'} V^*_{r'}  +   \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'}V^*_{r'} \\
&> p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'} V^*_{\lfloor \frac{r+1}{2} \rfloor + 1}  +   \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r } \delta_{r'}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} 
\end{align}
The above inequality holds due to induction assumption on monotonicity of $V^*$'s. Thus,
\begin{align}
&V^*_{r+1} \\
&> p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  \Big\{  \sum_{r'=0}^{\lfloor \frac{r+1}{2} \rfloor} \delta_{r'} - \sum_{r' =  \lfloor \frac{r+1}{2} \rfloor +1}^r \delta_{r'}  \Big\}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\
&= p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ &>  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r 
\end{align}
In the last second step we use the expression for $p^*_{r+1,r+1}$ obtained above \ref{eqn:p_r_r}. The inequality in the last step is due to assumption on monotonicity of $V^*$'s.\\
Thus, combining above with the fact that for our instances for any $r \in [n] \cup \{0\}, p^*_{r+1,r+1} < 1$:
\begin{align}
V^*_{r+1} >   p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r \Longleftrightarrow (1-p^*_{r+1,r+1})(V^*_{r+1}-V^*_r)>0 \Longleftrightarrow V^*_{r+1} > V^*_r
\end{align}

\end{proof}


 \subsection{Proof of Theorem \ref{thm:all_in_one}}

\textbf{Recall the Theorem \ref{thm:all_in_one}:} \pt{To improve the statement. The current statement doesn't look good.} \textit{Consider any instance defined as in (ref). Define global action $\tb{\ti{a}}_{\theta}$ as the action whose $\{(d-1)\times (i-1)+j\}^{th}$ element for every $i \in [n]$ and every $j \in [d-1]$ is given by $\sgn(\theta_{i,j})$. \pt{The following holds simultaneously.}
\begin{itemize}
    \item Then the policy of taking action $\tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$, is optimal. 
    \item Further, optimal value function for each state with the same number of agents at node $s$ takes the same value, i.e., suppose for every $r \in [n]$, $\mathcal{S}(r)$ denotes the set of all states with any $r$ agents at node $s$ and remaining $n-r$ agents at $g$. Then, $V^*(s) = V^*_r(constant)$ for all $s \in \mathcal{S}(r)$. We define $V^*_0=0$.
    \item There exists increasing monotonicity of optimal value function with the number of agents at node $s$ i.e., $0=V^*_0<V^*_1<V^*_2\dots<V^*_n = B^*$. 
\end{itemize}}
    

\begin{proof}
\tb{Base Case}  \\ By definition, $V^*_0 = 0$. \\
Take any $\tb{\ti{s}} \in \mathcal{S}(1)$. \\
We wish to find the optimal action in this state.\\
From $\tb{\ti{s}}$, only possible next global states are $\tb{\ti{s}}$ itself and the global goal state ($goal =\tb{g} = (g,g,g,\dots,g)$). This is akin to the single agent problem. But now, any transition probability also depends on actions of others. \\
Suppose $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$ denotes the transition probability from \tb{\ti{s}} to \tb{g} for any $\tb{\ti{a}} \in \mathcal{A}$. Then the value of this action at $\tb{\ti{s}}$ can be expressed as:  \\
$V^{\tb{\ti{a}}}(\tb{\ti{s}}) = (1-p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}).(1+V^{\tb{\ti{a}}}(\tb{\ti{s}})) + p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}.(1+V_0) \implies V^{\tb{a}}(\tb{\ti{s}}) = \frac{1}{p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}}$ \\
Thus, the optimal action at \tb{\ti{s}} is the one that minimizes $V^{\tb{a}}_1(\tb{\ti{s}})$ i.e., maximizes $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$. From the expression of general transition probability in Lemma \ref{lemma:general_tp}, the transition probability is maximum when $\tb{\ti{a}}$ is such that it matches all signs with $\theta$ at the respective components of agent who was initially at node $s$ in $\tb{\ti{s}}$. The signs of other components do not matter. Hence, there could be multiple optimal actions $\tb{\ti{a}}^*$ for any particular $\tb{\ti{s}} \in \mathcal{S}(1)$. \\
Notice that the above analysis holds for any $\tb{\ti{s}} \in \mathcal{S}(1)$. Note that the particular action $\tb{\ti{a}}_{\theta}$ each of whose components' sign matches with respective components of $\theta$ (as defined in theorem \ref{thm:all_in_one}), is common for possible optimal actions for every $\tb{\ti{s}} \in \mathcal{S}(1)$. We consider this $\tb{\ti{a}}^*=\tb{\ti{a}}_{\theta}$ in particular. \\
From Corollary \ref{corollary:p_star}, $p^{\tb{\ti{a}}^*}_{\tb{\ti{s}},\tb{g}} = p^{\tb{\ti{a}}^*} \forall \tb{\ti{s}} \in \mathcal{S}(1)$. Thus $V^*(\tb{\ti{s}}) = V^*_1 \forall \tb{\ti{s}} \in \mathcal{S}(1)$ \\
Clearly, $V^*_1 = \frac{1}{p^*_{\tb{\ti{s}},\tb{g}}}>0= V^*_0$ \\
Hence, all the three claims of Theorem \ref{thm:all_in_one} hold for the base case.\\
\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:
\begin{itemize}
    \item The optimal action $\tb{\ti{a}}^*$ is the one that matches sign at all components with $\theta$ (i.e., $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$) for any state in $\mathcal{S}(k)$. This implies from Corollary \ref{corollary:p_star} that, $p^*(\tb{\ti{s}} \in \mathcal{S}(k)  \xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})) = p^*_{k,k'}$, where $\tb{\ti{s}}' \in \mathcal{S}(k')$ for any $k' \in \{0,1,2,\dots,k\}$.
    \item $V^*_k(\tb{\ti{s}})=V^*_k$ for all $\tb{\ti{s}} \in \mathcal{S}(k)$
    \item $V^*_k>V^*_{k-1}>\dots>V^*_0 = 0$
\end{itemize}
Now, we need to show the same three claims hold for $r+1$. \\
Consider any $\tb{\ti{s}} \in S(r+1)$. \\
We again want to know what's the optimal action in this state. We know the optimal action in all the other states that can be reached from $\tb{\ti{s}}$. Hence, we consider the value of any action $\tb{a} \in \mathcal{A}$ in $\tb{\ti{s}}$ as follows (This is the same as $Q^*(\tb{\ti{s}},\tb{a})$ in most literature):
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}}) \\
&= \sum_{\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}}) \setminus \{\tb{\ti{s}},\tb{g}\}} \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}})\{1+V^*(\tb{\ti{s}}')\} + \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^{\tb{\ti{a}}}(\tb{\ti{s}})\} + \mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^*(\tb{g})\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +\sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'}V^*_{r'} 
\end{align}
Using general expression for transition probability from Lemma \ref{lemma:general_tp}:
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}})\\
&= 1+ \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) \\
&\quad +  \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Bigg\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^\tb{\ti{a}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}  \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} + \\
&\quad   \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \sum_{i \in [n]} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)} \times \\
&\quad  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{ \Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'} \Bigg \}  +  \\ 
&\quad \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  + \frac{\Delta}{n(d-1)} 
 \times \\
&\quad \Bigg\{  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Big \} + \\
&\quad \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \} \Bigg\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^a({\tb{\ti{s}}} +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
 &\quad \sum_{r' \in [r]}  \Bigg\{\Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}.V^*_{r'} \Bigg \}  \\
&\quad +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Big \} \\
&\quad + \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{  \{ \binom{r}{r'}  - \binom{r}{r'-1} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        + \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  +   \\
&\quad \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Big  \}
\end{align}

Observe that the term inside the summation is always non negative since when $r' \geq r/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} \geq V^*_{r+1-r'}$ while for $r' \leq r/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_{r+1-r'}$ due to property of Binomial coefficients and the Induction assumption of monotonicity of $V^*$ . Note that the above argument is for $r' \in [r]$. \\
To minimize $V^{\tb{\ti{a}}}(\tb{\ti{s}})$, we need to minimize $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well (check after rearrangement as it will appear in denominator as $1-\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$). \\
Clearly, the action that matches sign with all components of $\theta$ (i.e., $\tb{\ti{a}}_{\theta}$) minimizes $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well as makes the sum of non-negative terms the minimum i.e., $0$. Hence, it minimizes $V^\tb{\ti{a}}(\tb{\ti{s}})$. Hence this action $\tb{\ti{a}}_{\theta}$ is the optimal action $\tb{\ti{a}}^*$. \\
Notice the above argument holds for any $ \tb{\ti{s}} \in \mathcal{S}(r+1)$. Hence $\tb{\ti{a}}^*$ is the same for each of them. \\
Again, by Corollary \ref{corollary:p_star}, $p^*(\tb{\ti{s}} \in \mathcal{S}(\tb{\ti{s}})\xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})) = p^*_{r+1,r'}$ for any $r' \in [r] \cup \{0\}$. \\
Thus, $V^*(\tb{\ti{s}}) = V^*_{r+1}$ for any $\tb{\ti{s}} \in \mathcal{S}(r+1)$. \\
Using the induction assumption combined with this result, Claim \ref{claim:probability_inequality} and Lemma \ref{lemma:probability_inequality}, we have $V^*_{r+1}>V^*_r$. \\
Hence by induction, all three claims of the theorem hold.
\end{proof}


\begin{proof}
\tb{Base Case}  

By definition, $V^*_0 = 0$.

Take any $\tb{\ti{s}} \in \mathcal{S}(1)$. \\
We wish to find the optimal action in this state.\\
From $\tb{\ti{s}}$, only possible next global states are $\tb{\ti{s}}$ itself and the global goal state ($goal =\tb{g} = (g,g,g,\dots,g)$). This is akin to the single agent problem. But now, any transition probability also depends on actions of others. \\
Suppose $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$ denotes the transition probability from \tb{\ti{s}} to \tb{g} for any $\tb{\ti{a}} \in \mathcal{A}$. Then the value of this action at $\tb{\ti{s}}$ can be expressed as:  \\
$V^{\tb{\ti{a}}}(\tb{\ti{s}}) = (1-p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}).(1+V^{\tb{\ti{a}}}(\tb{\ti{s}})) + p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}.(1+V_0) \implies V^{\tb{a}}(\tb{\ti{s}}) = \frac{1}{p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}}$ \\
Thus, the optimal action at \tb{\ti{s}} is the one that minimizes $V^{\tb{a}}_1(\tb{\ti{s}})$ i.e., maximizes $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$. From the expression of general transition probability in Lemma \ref{lemma:general_tp}, the transition probability is maximum when $\tb{\ti{a}}$ is such that it matches all signs with $\theta$ at the respective components of agent who was initially at node $s$ in $\tb{\ti{s}}$. The signs of other components do not matter. Hence, there could be multiple optimal actions $\tb{\ti{a}}^*$ for any particular $\tb{\ti{s}} \in \mathcal{S}(1)$. \\
Notice that the above analysis holds for any $\tb{\ti{s}} \in \mathcal{S}(1)$. Note that the particular action $\tb{\ti{a}}_{\theta}$ each of whose components' sign matches with respective components of $\theta$ (as defined in theorem \ref{thm:all_in_one}), is common for possible optimal actions for every $\tb{\ti{s}} \in \mathcal{S}(1)$. We consider this $\tb{\ti{a}}^*=\tb{\ti{a}}_{\theta}$ in particular. \\
From Corollary \ref{corollary:p_star}, $p^{\tb{\ti{a}}^*}_{\tb{\ti{s}},\tb{g}} = p^{\tb{\ti{a}}^*} \forall \tb{\ti{s}} \in \mathcal{S}(1)$. Thus $V^*(\tb{\ti{s}}) = V^*_1 \forall \tb{\ti{s}} \in \mathcal{S}(1)$ \\
Clearly, $V^*_1 = \frac{1}{p^*_{\tb{\ti{s}},\tb{g}}}>0= V^*_0$ \\
Hence, all the three claims of Theorem \ref{thm:all_in_one} hold for the base case.\\
\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:
\begin{itemize}
    \item The optimal action $\tb{\ti{a}}^*$ is the one that matches sign at all components with $\theta$ (i.e., $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$) for any state in $\mathcal{S}(k)$. This implies from Corollary \ref{corollary:p_star} that, $p^*(\tb{\ti{s}} \in \mathcal{S}(k)  \xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})) = p^*_{k,k'}$, where $\tb{\ti{s}}' \in \mathcal{S}(k')$ for any $k' \in \{0,1,2,\dots,k\}$.
    \item $V^*_k(\tb{\ti{s}})=V^*_k$ for all $\tb{\ti{s}} \in \mathcal{S}(k)$
    \item $V^*_k>V^*_{k-1}>\dots>V^*_0 = 0$
\end{itemize}
Now, we need to show the same three claims hold for $r+1$. \\
Consider any $\tb{\ti{s}} \in S(r+1)$. \\
We again want to know what's the optimal action in this state. We know the optimal action in all the other states that can be reached from $\tb{\ti{s}}$. Hence, we consider the value of any action $\tb{a} \in \mathcal{A}$ in $\tb{\ti{s}}$ as follows (This is the same as $Q^*(\tb{\ti{s}},\tb{a})$ in most literature):
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}}) \\
&= \sum_{\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}}) \setminus \{\tb{\ti{s}},\tb{g}\}} \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}})\{1+V^*(\tb{\ti{s}}')\} + \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^{\tb{\ti{a}}}(\tb{\ti{s}})\} + \mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^*(\tb{g})\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +\sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'}V^*_{r'} 
\end{align}
Using general expression for transition probability from Lemma \ref{lemma:general_tp}:
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}})\\
&= 1+ \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) \\
&\quad +  \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Bigg\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^\tb{\ti{a}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}  \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} + \\
&\quad   \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \sum_{i \in [n]} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)} \times \\
&\quad  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{ \Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'} \Bigg \}  +  \\ 
&\quad \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  + \frac{\Delta}{n(d-1)} 
 \times \\
&\quad \Bigg\{  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Big \} + \\
&\quad \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \} \Bigg\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^a({\tb{\ti{s}}} +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
 &\quad \sum_{r' \in [r]}  \Bigg\{\Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}.V^*_{r'} \Bigg \}  \\
&\quad +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Big \} \\
&\quad + \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{  \{ \binom{r}{r'}  - \binom{r}{r'-1} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        + \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  +   \\
&\quad \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Big  \}
\end{align}

Observe that the term inside the summation is always non negative since when $r' \geq r/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} \geq V^*_{r+1-r'}$ while for $r' \leq r/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_{r+1-r'}$ due to property of Binomial coefficients and the Induction assumption of monotonicity of $V^*$ . Note that the above argument is for $r' \in [r]$. \\
To minimize $V^{\tb{\ti{a}}}(\tb{\ti{s}})$, we need to minimize $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well (check after rearrangement as it will appear in denominator as $1-\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$). \\
Clearly, the action that matches sign with all components of $\theta$ (i.e., $\tb{\ti{a}}_{\theta}$) minimizes $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well as makes the sum of non-negative terms the minimum i.e., $0$. Hence, it minimizes $V^\tb{\ti{a}}(\tb{\ti{s}})$. Hence this action $\tb{\ti{a}}_{\theta}$ is the optimal action $\tb{\ti{a}}^*$. \\
Notice the above argument holds for any $ \tb{\ti{s}} \in \mathcal{S}(r+1)$. Hence $\tb{\ti{a}}^*$ is the same for each of them. \\
Again, by Corollary \ref{corollary:p_star}, $p^*(\tb{\ti{s}} \in \mathcal{S}(\tb{\ti{s}})\xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})) = p^*_{r+1,r'}$ for any $r' \in [r] \cup \{0\}$. \\
Thus, $V^*(\tb{\ti{s}}) = V^*_{r+1}$ for any $\tb{\ti{s}} \in \mathcal{S}(r+1)$. \\
Using the induction assumption combined with this result, Claim \ref{claim:probability_inequality} and Lemma \ref{lemma:probability_inequality}, we have $V^*_{r+1}>V^*_r$. \\
Hence by induction, all three claims of the theorem hold.
\end{proof}


\section{Notations and Prelims}

..... \pt{Your writeup starts here.}

A general Multi-Agent Stochastic Shortest Path (MA-SSP) problem is defined as $(\mathcal{V}, N, \mathbb{P}, \mathcal{A})$. Here $\mathcal{V} \coloneqq
\{v_1,v_2,v_3,\dots,v_q\}$ is the set of nodes. $N=\{1,2,\dots,n\} = [n]$ is the set of agents.  
At any instant, each agent can be at exactly one node in $\mathcal{V}$. We represent the global state of the system by $\tb{\ti{s}} = \{s_1,s_2,\dots,s_{n}\}$ where for every agent $i \in N$, $s_i \in \mathcal{V}$ represents the node where the agent $i$ is present. 
Hence, the set of all possible states $\mathcal{S}$ is $\Pi_{i=1}^{n}\mathcal{V}= \mathcal{V}^n$. At time step, each agent can take an action. We assume that the set of actions available for any agent $i \in [n]$, namely $\mathcal{A}^i$ is independent of the node at which it is present.
We represent the global action $\tb{\ti{a}} = \{a_1,a_2,\dots,a_n\}$ where for every $i \in N,a^i \in \mathcal{A}^i$ represents the action taken by the agent $i$. 
Hence, the set of all actions possible at any state $\tb{\ti{s}} \in \mathcal{S}$ is $\mathcal{A}=\Pi_{i=1}^n \mathcal{A}^i$. At any state $\tb{\ti{s}} \in \mathcal{S}$, if action $\tb{\ti{a}}$ is taken, then each agent $i \in N$ incurs a cost $c^i(\tb{\ti{s}},\tb{\ti{a}})$ which in general is a random variable, in that instant where,  $0<c_{\min} \leq c^i(\tb{\ti{s}},\tb{\ti{a}})\leq 1$. Note that individual cost depends on global state and global action. This model encapsulates complexities arising due to multi-agent setup. 

We show below how congestion can be modeled and incorporated in this framework. Suppose for any agent $i \in N, \tb{\ti{s}} = (s_1,s_2,\dots,s_n) \in \mathcal{S}, \tb{\ti{a}} = (a_1,a_2,\dots,a_n) \in \mathcal{A}$, $K^i(\tb{\ti{s}},\tb{\ti{a}})$ denotes the cost to the agent $i$ due to private efficiency and all other complex multi-agent interdependencies except congestion. Congestion can be modeled by considering the total number of agents who take the same actions. We define Congestion Factor:
\begin{align}
    c_f^i(\tb{\ti{s}},\tb{\ti{a}}) = \sum_{j=1}^n \mathbbm{1}\{a_j = a_i\}
\end{align}
Thus, we model the cost to agent $i \in N$  as 
\begin{align} \label{eqn:ind_cost}
    c^i(\tb{\ti{s}},\tb{\ti{a}}) = c_f^i(\tb{\ti{s}},\tb{\ti{a}}) \times K^i(\tb{\ti{s}},\tb{\ti{a}})=\sum_{j=1}^n \mathbbm{1}\{a_j = a_i\}.K^i(\tb{\ti{s}},\tb{\ti{a}})
\end{align}
We define the global cost (to the system) as the average of individual costs i.e., 
\begin{align} \label{eqn:glb_cost}
c(\tb{\ti{s}},\tb{\ti{a}}) = \frac{1}{n}\sum_{i=1}^n c^i(\tb{\ti{s}},\tb{\ti{a}}) = \frac{1}{n}\sum_{i=1}^n c^i_f(\tb{\ti{s}}, \tb{\ti{a}}) \times K^i(\tb{\ti{s}},\tb{\ti{a}})  = \frac{1}{n}\sum_{i=1}^n \Bigg \{\sum_{j=1}^n \mathbbm{1}\{a_j = a_i\} \Bigg \}\times K^i(\tb{\ti{s}},\tb{\ti{a}}) 
\end{align}
\pt{congestion} \textcolor{red}{i've added some discussion on congestion above}
The environment also responds with a next state $\tb{\ti{s}}^\prime$ sampled according to a probability distribution depending on $\tb{\ti{s}}$ and $\tb{\ti{a}}$ i.e., $\tb{\ti{s}}^\prime \sim \mathbb{P}(.|\tb{\ti{s}},\tb{\ti{a}})$. 
This captures that in the multi-agent set up, the next state of any agent is also influenced by state and action of other players. 
In planning setting, the cost function and the transition probability function is known. While in learning setting, atleast one of the two is unknown. \\
Finally, we define a policy($\pi$) as a \ti{scheme} of taking actions in various states. 

\pt{In our setup} -- Given an ordered pair of states $(\tb{\ti{s}}_\init, \tb{g}) \in \mathcal{S} \times \mathcal{S}\setminus\tb{g}$, the problem is to find the best policy ($\pi^*$) to reach state $\tb{g}$ starting from  $\tb{\ti{s}}_\init$ in a cumulative global cost minimization sense. Due to stochastic costs and transition dynamics, one can only evaluate policies in terms of their expected behavior. The most general way is to consider the set of all history-dependent randomized policies $\Pi = \{\pi:\mathcal{H}\xrightarrow{}\Delta(\mathcal{A})\}$, where each policy $\pi$ is a mapping from the set of all histories $\mathcal{H}$ to the set of all probability distributions over global actions $\Delta(\mathcal{A})$. 

Due to Markovian and stationary transition and cost structure,
it is sufficient to consider policies in the Markov and Deterministic space to find the optimal policy(\textcolor{red}{can this statement be made better?}cite). Even then, there may be "bad" policies which do not lead to \tb{g} almost surely. We call these as improper policies. On the other hand, those policies that lead to \tb{g} almost surely are said to be proper. We further assume that the set of proper policies ($\Pi_p$) is non-empty (\textcolor{red}{should this be written under begin assumption? or this is ok?}). 
For any policy $\pi \in \Pi$, we define for any state $\tb{\ti{s}} \in \mathcal{S}$, the expected long-term cost as:
\begin{align}
    V^{\pi}(\tb{\ti{s}}) = \mathbb{E}[c(\tb{\ti{s}}_1,\pi(\tb{\ti{s}}_1))+c(\tb{\ti{s}}_2,\pi(\tb{\ti{s}}_2))+\dots|\tb{\ti{s}}_1=\tb{\ti{s}}]
\end{align}
where $\tb{\ti{s}}_{t+1} \sim \mathbb{P}(.|s_t,\pi(s_t))$  for time steps $t=1,2, \cdots$. In general, the expectation is due to randomized action due to policy, stochastic cost and transition dynamics. For an improper policy \pt{what is improper policy?}, the above becomes unbounded for at least one state. However, for any proper policy the summation inside the expectation almost surely has random but finite bounded terms and thus the expectation becomes overall bounded.  
Restricting to proper policies ($\Pi_{p}$), planning version of the MASSP problem can be expressed as the following: 
\begin{align}
    \pi^* = \arg \min_{\pi \in \Pi_p} V^\pi(\tb{\ti{s}}_{init})
\end{align}
We define diameter $B^*$ of any MA-SSP problem as: 
\begin{align}
    B^* = \max_{\tb{\ti{s}}\in \mathcal{S}}V^*(\tb{\ti{s}})
\end{align}
In learning setting, due to the lack of knowledge of cost and transition probability functions, one needs to \textit{sufficiently} explore all state-action pairs while ensuring that the best policy is learned over time and actions are taken according to it. 
As we wish to learn the best policy to navigate from one state to the another, any MASSP learning algorithm is run over multiple episodes all starting at $\tb{\ti{s}}_{init}$ and ending at $goal$. 

The learnability of an MASSP learning algorithm $\mathfrak{A}$ is thus characterized by the notion of cumulative regret over $K$ episodes in hindsight. It is a measure of the difference between the expected long term cost of chosing actions as prescribed by the algorithm and that by choosing actions according to the optimal policy.  Suppose, $h_1,h_2,\dots,h_k$ represent the random variables representing the length of episodes $1,2,\dots,K$ respectively. Then, expected cumulative regret of the algorithm is defined as: \pt{regret of policy}
\begin{align}\label{eqn:regret}
    \mathbb{E}_{\mathfrak{A}}[R(K)] = \mathbb{E} \Bigg \{ \sum_{k=1}
^{K}\sum_{h=1}^{h_k} c(\tb{\ti{s}}_{k,h},\tb{\ti{a}}_{k,h}) \Bigg \} - K.V^*(s_{init}) \end{align}
where $\tb{\ti{s}}_{k,h}$ and $\tb{\ti{a}}_{k,h}$ respectively denote the random variables associated with state and action at the $h^{th}$ step in the $k^{th}$ episode. 

... \pt{Your writeup ends here}



\subsection{Related Works}\label{subsec:relatedwork}

\begin{itemize}
    \item Planning SSP: Bertsekas, Tsitsiklis, Guillot,..
    \item Learning SSP 1 agent - \\Tabular: Tarbouriech, Cohen, Rosenberg, \\Linear Mixture SSP: Min et al (Closest to our work), Vial .
    \item Learning SSP Multi-Agent : Trivedi and Hemachandra.
    \item Dec-MARL : Zhang
\end{itemize}


\section{Proof of Thm 1}

\pt{the above thing is not for the induction -- want to show for the types of r=1 to n -- need to mention though about r=0. the episode ends at g. eqn 120 is for r=1, not from r=0. thus, we have that eqn for r=1. by defn we have V=0. base case to be taken as r=1,}
    



This completes the base case.
        

=== 

\pt{Now assume that it is true for all r upto k. , and then prove it for r = k+1. }


for r=1 , claim 1,2,3, holds,  ==>  r=2, claim 1,2,3 holds, ==-=> r=k, claim 1, 2, 3 holds.. Then first we need to prove that claim 1 holds for r= k+1, then using this claim, --- prove claim 2, and then prove claim 3...



===

   

\end{proof}



\begin{proof}
    We will prove this result using the principle of Mathematical induction on $r$.  First we consider the base case $r = 0$.

\paragraph{Base case: $r=0, \mathcal{S}(0)$. -- better to start from $\mathcal{S}(1)$.} 


\pt{All the agents are at goal  node. Hence, any policy is optimal. so claim 1 holds be default. since their is only one state of type $r=0$, the second claim holds. The third claim holds by definition. }




By definition, we have $V^*_0 = 0$. For any state $\tb{\ti{s}} \in \mathcal{S}(1)$, we would like to find the optimal action in this state.  From $\tb{\ti{s}}$ the only possible next global states are $\tb{\ti{s}}$ itself and the global goal state $\tb{\ti{g}} = (g, \dots ,g)$. This is akin to the single agent problem, however, the transition probability  depends on actions of others. Suppose $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$ denotes the transition probability from \tb{\ti{s}} to \tb{g} for any $\tb{\ti{a}} \in \mathcal{A}$. Then the value of this action at $\tb{\ti{s}}$ can be expressed as
% 
\begin{align}
    V^{\tb{\ti{a}}}(\tb{\ti{s}}) = (1-p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}) \cdot (1+V^{\tb{\ti{a}}}(\tb{\ti{s}})) + p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}} \cdot (1+V_0)
    \quad \implies V^{\tb{a}}(\tb{\ti{s}}) = \frac{1}{p^\tb{\ti{a}}_{\tb{\ti{s}},\tb{g}}}.
\end{align}
\pt{this is $Q(s,a)$. }

Thus, the optimal action at $\tb{\ti{s}}$ is the one that minimizes $V^{\tb{a}}_1(\tb{\ti{s}})$ i.e., maximizes $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{g}}$.

From the expression of general transition probability in Lemma \ref{lemma:general_tp}, the transition probability is maximum when $\tb{\ti{a}}$ is such that it matches all signs with $\theta$ at the respective components of agent who was initially at node $s$ in $\tb{\ti{s}}$. The sign of other components do not matter. Hence, there could be multiple optimal actions $\tb{\ti{a}}^*$ for any particular $\tb{\ti{s}} \in \mathcal{S}(1)$.

\pt{we can write the exact expression of the probability again here. This will make it more clear. Explain this part abut indicators.}



Notice that the above analysis holds for any $\tb{\ti{s}} \in \mathcal{S}(1)$. Note that the particular action $\tb{\ti{a}}_{\theta}$ each of whose components' sign matches with respective components of $\theta$ (as defined in theorem \ref{thm:all_in_one}), is common for possible optimal actions for every $\tb{\ti{s}} \in \mathcal{S}(1)$.

We consider this as $\tb{\ti{a}}^*=\tb{\ti{a}}_{\theta}$ in particular. 



\pt{all the states of same type has the same optimal action. This is equivalent to the threshold type policies -- to think and write more in this direction. We  partition the state space, and in each partition we have clarity about what is optimal action -- sign mathcing property.}

From Corollary \ref{corollary:p_star}, $p^{\tb{\ti{a}}^*}_{\tb{\ti{s}},\tb{g}} = p^{\tb{\ti{a}}^*} \forall \tb{\ti{s}} \in \mathcal{S}(1)$. Thus 
\begin{align}
    V^*(\tb{\ti{s}}) = V^*_1, \quad ~ \forall ~ \tb{\ti{s}} \in \mathcal{S}(1)
\end{align}
Clearly, $V^*_1 = \frac{1}{p^*_{\tb{\ti{s}},\tb{g}}}>0= V^*_0$. \pt{So, the vlues are same for all states in $\mathcal{S}(1)$. }

\pt{I do not understand the above proof. Can you explain it in more details. }

\pt{Why we suddenly mentioned that all the claims are true? It's not clear to me.}

This proves that all the three claims of Theorem \ref{thm:all_in_one} hold for the base case. 



\end{proof}

...

\begin{proof}
\tb{Base Case}  

\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:
\begin{itemize}
    \item The optimal action $\tb{\ti{a}}^*$ is the one that matches sign at all components with $\theta$ (i.e., $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$) for any state in $\mathcal{S}(k)$. This implies from Corollary \ref{corollary:p_star} that, $p^*(\tb{\ti{s}} \in \mathcal{S}(k)  \xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})) = p^*_{k,k'}$, where $\tb{\ti{s}}' \in \mathcal{S}(k')$ for any $k' \in \{0,1,2,\dots,k\}$.
    \item $V^*_k(\tb{\ti{s}})=V^*_k$ for all $\tb{\ti{s}} \in \mathcal{S}(k)$
    \item $V^*_k>V^*_{k-1}>\dots>V^*_0 = 0$
\end{itemize}
Now, we need to show the same three claims hold for $r+1$. \\
Consider any $\tb{\ti{s}} \in S(r+1)$. \\
We again want to know what's the optimal action in this state. We know the optimal action in all the other states that can be reached from $\tb{\ti{s}}$.

\pt{upto $r$, reachable ... }

Hence, we consider the value of any action $\tb{a} \in \mathcal{A}$ in $\tb{\ti{s}}$ as follows (This is the same as $Q^*(\tb{\ti{s}},\tb{a})$ in most literature):
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}}) \\
&= \sum_{\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}}) \setminus \{\tb{\ti{s}},\tb{g}\}} \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}})\{1+V^*(\tb{\ti{s}}')\} + \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^{\tb{\ti{a}}}(\tb{\ti{s}})\} + \mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}}).\{1+V^*(\tb{g})\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +\sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'}V^*_{r'} 
\end{align}

\pt{let us write the english explanation of the last term.. Now focus on third term.}


Using general expression for transition probability from Lemma \ref{lemma:general_tp}:
\begin{align}
&V^{\tb{\ti{a}}}(\tb{\ti{s}})\\
&= 1+ \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) \\
&\quad +  \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Bigg\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^\tb{\ti{a}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}  \\
&\quad +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} 
\end{align}
The last line follows from observing that for fixed $r'$, the inner summation over $s'$ in line 127 is just the sum of $|\mathcal{S}(
r')(\tb{\ti{s}})| = \binom{r+1}{r'}$ terms and the outer summations are taken in side for the term in eqn128.\\
In the below, we alternatively represent the summation over sets $\mathcal{I} \cap \mathcal{T}$ and $\mathcal{T}$ as an appropriate summation over $\mathcal{I}$ and in the next step, we take the $V^*(.)$ factor inside and take the summation over two terms:
\begin{align}
&V^a(\tb{\ti{s}})  \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} + \\
&\quad   \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \sum_{i \in \mathcal{I}} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)} \times \\
&\quad  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{ \Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} V^*_{r'} \Bigg \}  +  \\ 
&\quad \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} \Big  \}V^*_{r'} 
\end{align}
In the last step, we identified that for every agent $i \in \mathcal{I}$ for a fixed $r'$ the number of states in $\mathcal{S}(r')(\tb{\ti{s}})$ in which it stays at node $s$ itself is $\binom{r}{r'-1}$ and those in which it transits to node $g$ is $\binom{r}{r'}$. \\
In the immediate below step, we use $\sum_{a \in [m]} f(a) = \sum_{a \in [m]} f(1+m-a)$ for any function $f(.)$ and natural number $m$. (Here, the part of eqn 141 inside the summations over $p$ and $i$ is our $f$, $ a$ is $r'$ and $m$ is $r$.) In the next few steps, we simplify the expression using properties of binomial coefficients and simplify: 
\begin{align} 
&V^a(\tb{\ti{s}}) \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +  \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  + \frac{\Delta}{n(d-1)} 
 \times \\
&\quad \Bigg\{  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Big \} + \\
&\quad \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \} \Bigg\} \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^a({\tb{\ti{s}}} +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
 &\quad \sum_{r' \in [r]}  \Bigg\{\Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'}.V^*_{r'} \Bigg \}  \\
&\quad +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Bigg \{ \Big \{ \binom{r}{r'-1}  - \binom{r}{r'} \Big \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r'} \Bigg \} \\
&\quad + \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Bigg \{ \Big \{ \binom{r}{r'}  - \binom{r}{r'-1} \Big \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Bigg  \}  \\
&= 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\tb{\ti{a}}}(\tb{\ti{s}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) + \\
&\quad \sum_{r' \in [r]}  \Bigg\{\Big\{\frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        + \frac{\Delta}{n}  (r+1-2r')\Big\}.\binom{r+1}{r'} . V^*_{r'}\Bigg \}  +   \\
&\quad \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Bigg \{ \Big\{ \binom{r}{r'-1}  - \binom{r}{r'} \Big \} . \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Bigg \}
\end{align}
\pt{We identified the partitions based on the type, the action is common. }

\pt{Sum over r' is written in terms of binomials -- in how many states of type r', reach from s, agent i is not transiting or transiting, respectively.}

\pt{sum backward.. rather than forward.}

Observe that the term inside the summation is always non negative since when $r' \geq r/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} \geq V^*_{r+1-r'}$ while for $r' \leq r/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_{r+1-r'}$ due to property of Binomial coefficients and the Induction assumption of monotonicity of $V^*$ . Note that the above argument is for $r' \in [r]$. \\
To minimize $V^{\tb{\ti{a}}}(\tb{\ti{s}})$, we need to minimize $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well (check after rearrangement as it will appear in denominator as $1-\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$). \\
Clearly, the action that matches sign with all components of $\theta$ (i.e., $\tb{\ti{a}}_{\theta}$) minimizes $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ as well as makes the sum of non-negative terms the minimum i.e., $0$. Hence, it minimizes $V^\tb{\ti{a}}(\tb{\ti{s}})$. Hence this action $\tb{\ti{a}}_{\theta}$ is the optimal action $\tb{\ti{a}}^*$. \\
Notice the above argument holds for any $ \tb{\ti{s}} \in \mathcal{S}(r+1)$. Hence $\tb{\ti{a}}^*$ is the same for each of them. \\
Again, by Corollary \ref{corollary:p_star}, $p^*(\tb{\ti{s}} \in \mathcal{S}(\tb{\ti{s}})\xrightarrow{}\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})) = p^*_{r+1,r'}$ for any $r' \in [r] \cup \{0\}$. \\
Thus, $V^*(\tb{\ti{s}}) = V^*_{r+1}$ for any $\tb{\ti{s}} \in \mathcal{S}(r+1)$. \\
Using the induction assumption combined with this result, Claim \ref{claim:probability_inequality} and Lemma \ref{lemma:probability_inequality}, we have $V^*_{r+1}>V^*_r$. \\
Hence by induction, all three claims of the theorem hold.





\pt{Why this part is written here, need to be written in prelims or the introduction.} \textcolor{red}{removed from here and placed into introduction}
\textcolor{red}{The transition from single agent SSP to Multi-Agent SSP, leads to the following complications: 
\begin{itemize}
    \item The state and action space explodes 
    \item Next state transition probabilities and costs of individual agents depends not only on individual current state and action but also on that of others.
    \item Information needs to be shared to meet global objective however there may be privacy and scaling issues. 
    \item Tractable closed form expression of optimal value function is no longer easy to obtain to use it in lower-bound regret analysis. This is because at $n=1$, the number of states for single agent instances are only 2 and these are the same as nodes themselves $(s,g)$. But with $n>1$, this is exponential in $n$ and it's quite challenging to obtain closed form expressions for $V^*$ for these states and use them in regret lower bound analysis. We circumvent this issue by ignoring a non-exactly simplifiable summation of not neccesarily all positive terms, by showing that the entire summation is itself positive (\ref{lemma:sum_diff_prob_v}).
    \item In our analysis, we observe another similar challenge when simplifying a KL-divergence term that arises due to information theoretic bound on difference between expectations over different measures of the same random variable (\ref{eqn:exp_diff}). Instead of direct simplification, a suitable upper bounding technique that exploits symmetry of state-space for KL-divergence works for us.
 \end{itemize}
 }

\textcolor{red}{We conjecture that the decentralised MASSP problem is harder to solve compared to the single agent SSP learning problem. (Open problem, would require to prove that a lower bound for D-MASSP is higher compared to an upper bound on SASSP).} \textcolor{red}{have moved this to conclusion} \pt{conclusion}


\subsection{Proof of Theorem \ref{thm:lower_bound}}

\textbf{Recall Theorem \ref{thm:lower_bound}. }
    \textit{For any MASSP learning algorithm $\mathfrak{A}$ as defined in \ref{subsec:problem_formulation}, there exists a LM-MASSP instance ($\theta \in \Theta$) for every $n \geq 1$, $\delta \in (2/5,1/2)$, $\Delta < 2^{-n}.\frac{1-2\delta}{1+n+n^2}$, such that the expected cumulative regret upon running the algorithm on this instance for $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.\{\frac{1-2\delta}{1+n+n^2}\}^2} $ episodes at least matches the reported $\widetilde{O}(\sqrt{K})$ upper bound by \citep{trivedi2023massp} in terms of number of training episodes $K$. Here $V^*_1 = \frac{2n}{n-1+2(\delta+\Delta)}$. 
    Specifically for this instance, we have $\mathbb{E}_{\theta,\mathfrak{A}}[R(K)] \geq \frac{d.\sqrt{\delta}\sqrt{K.V^*_1}}{2^{n+9}}$  }   



\begin{proof}
We construct and analyze a family of hard to learn instances based on the discussion in \ref{sec:approach}.  Recall that for our instances, we  restricted $\theta$ (global theta) such that (no two local theta are same) $\theta_{i} \neq \theta_{j}$ $ \forall$ $ i \neq j \in [n]$ i.e., no two $\theta_i$ are the same. We denoted the set of all $\theta$ as $\Theta$. 
\\
In Theorem $\ref{thm:all_in_one}$, we characterized the optimal policy. The restriction on $\theta$ ensures that for the optimal global action, the individual actions for each agent are all different.
To further reduce complexity of the analysis, we let our instances be such that the cost of any global action in any non-goal state is equal to 1 (see Remark \ref{rem:cost_one}) and that in goal state equal to 0.  \\
Consider any instance parameters $(n\geq 1, \delta \in (2/5,1/2), \Delta < 2^{-n} . \frac{1-2\delta}{1+n+n^2})$. We want to analyze regrets for any policy for instances that are defined by above fixed parameters $(n,\delta, \Delta)$ and any  $\theta \in \Theta$. \\
Suppose in episode \textit{k}, agents take actions according to policy $\pi^k_{\theta}$. Let, $\tb{\ti{s}}_t$ represent the global state and $\tb{\ti{a}}_t$ the global action at time $t$. Then, the expected regret for the \textit{k-th} episode is:

\begin{align}
    & R_{\theta,k}  \\
    &= V^{\pi^k_\theta}(\tb{\ti{s}}_1) - V^*(\tb{\ti{s}}_1)  \label{regret}
    \\
    &=  V^{\pi^k_\theta}(\tb{\ti{s}}_1) - \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}[Q^{\pi^*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] + \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}[Q^{\pi^*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^{\pi^*}(\tb{\ti{s}}_1) 
    \end{align}
    In the above, we add and subtract $\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}[Q^{\pi^*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)]$. \\
    Below, we expand using the definitions of $V^{\pi^k_{\theta}}(.)$ and $Q^{\pi^*}(.,.)$ and rearrange:
    \begin{align}
    R_{\theta,k}
    &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}\{c(\tb{\ti{s}}_1, \tb{\ti{a}}_1) + \mathbb{E}_{\tb{\ti{s}}_2 \sim \mathbb{P}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)}[V^{\pi^k_\theta}(\tb{\ti{s}}_2)]\}  
    \\ 
    & \quad -\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}\{c(\tb{\ti{s}}_1, \tb{\ti{a}}_1) + \mathbb{E}_{\tb{\ti{s}}_2 \sim \mathbb{P}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)}[V^*(\tb{\ti{s}}_2)] \} + \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}[Q^{\pi^*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^{\pi^*}(\tb{\ti{s}}_1) \\
    &= \mathbb{E}_{\tb{\ti{a}}_1 \sim\ \pi^k_\theta(\tb{\ti{s}}_1), \tb{\ti{s}}_2 \sim\ \mathbb{P}(.|\tb{\ti{s}}_1,\tb{\ti{a}}_1)}[V^{\pi^k_\theta}(\tb{\ti{s}}_2) - V^*(\tb{\ti{s}}_2)] + \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_\theta(\tb{\ti{s}}_1)}[Q^{\pi^*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^{\pi^*}(\tb{\ti{s}}_1) \label{eq_Q_V}
\end{align}
In the above expression, there appears to be a recursive relation from the first term but it its unclear how to deal with the second term. \\ 
We expand upon it below where $Q^* (.,.)= Q^{\pi^*}, V^*(.)=V^{\pi^*}$:
\begin{align}
  &\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[Q^{*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^*(\tb{\ti{s}}_1) \\
    &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[c(\tb{\ti{s}}_1, \tb{\ti{a}}_1) + \mathbb{E}_{\tb{\ti{s}}_2 \sim \mathbb{P}(.|\tb{\ti{s}}_1,\tb{\ti{a}}_1)}\{V^*(\tb{\ti{s}}_2)\}] - V^*(\tb{\ti{s}}_1) 
    \end{align}
    Above, we use the definition of $Q^*(.,.)$. \\
    Below, we use that the cost $c(\tb{\ti{s}}, \tb{\ti{a}}) \equiv 1 \forall (\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S}\backslash\{\tb{\ti{g}}\} \times \mathcal{A}$ and then expand the expectation:
    \begin{align}
    &\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[Q^{*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^*(\tb{\ti{s}}_1) \\
    &=  \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{  1 + \mathbb{E}_{\tb{\ti{s}}_2 \sim \mathbb{P}(.,\tb{\ti{s}}_1,\tb{\ti{a}}_1)}[V^*(\tb{\ti{s}}_2)] - V^*(\tb{\ti{s}}_1) \Big \} \\
    &=   \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k(\tb{\ti{s}}_1)} \Big\{ 1 +  \mathbb{P}(\tb{\ti{s}}_1|\tb{\ti{s}}_1,\tb{\ti{a}}_1) V^*(\tb{\ti{s}}_1) + \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)V^*(\tb{\ti{s}}_2) - V^*(\tb{\ti{s}}_1) \Big \} \end{align}
   To simplify above, we use the general transition probability expression from Lemma \ref{lemma:general_tp} and then rearrange:
    \begin{align}
   &\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[Q^{*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^*(\tb{\ti{s}}_1) \\
    &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi_{\theta}^k(\tb{\ti{s}}_1)} \Bigg\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Big \}  V^*(\tb{\ti{s}}_1) \\
  &+ \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)V^*(\tb{\ti{s}}_2)  - V^*(\tb{\ti{s}}_1) \Bigg \} \\
  &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta \Big \}  V^*(\tb{\ti{s}}_1) + \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)V^*(\tb{\ti{s}}_2) - V^*(\tb{\ti{s}}_1)  \Big \} \\
  &+ \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi_{\theta}^k(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} . V^*(\tb{\ti{s}}_1) \Big\} \\
  &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ 1 +\mathbb{P}(\tb{\ti{s}}_1|\tb{\ti{s}}_1,a_1^*) V^*(\tb{\ti{s}}_1) + \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)V^*(\tb{\ti{s}}_2) - V^*(\tb{\ti{s}}_1) \Big \} \\
  &+ \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}_1) \Big\}  
  \end{align}
The last step follows from transition probability expression in Lemma \ref{lemma:general_tp} since $\tb{\ti{s}} = (s,s,\dots,s)$.\\  
Below, we expand $V^*(\tb{\ti{s}}_1)$ and simplify:
  \begin{align}
  &\mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[Q^{*}(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^*(\tb{\ti{s}}_1) \\    
  &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Bigg\{ 1 + \mathbb{P}(\tb{\ti{s}}_1|\tb{\ti{s}}_1,\tb{\ti{a}}_1^*)  V^*(\tb{\ti{s}}_1) + \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)V^*(\tb{\ti{s}}_2) - \Big\{ 1 +  \mathbb{P}(\tb{\ti{s}}_1|\tb{\ti{s}}_1,\tb{\ti{a}}_1^*) V^*(\tb{\ti{s}}_1) \\
  &+ \sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} \mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1, \tb{\ti{a}}_1^*) V^*(\tb{\ti{s}}_2) \Big\} \Bigg \} + \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p})\neq \sgn(\theta_{i,p})\} V^*(\tb{\ti{s}}_1) \Big\} \\
  &= \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{\sum_{\tb{\ti{s}}_2 \neq \tb{\ti{s}}_1} [\mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1,\tb{\ti{a}}_1)-\mathbb{P}(\tb{\ti{s}}_2|\tb{\ti{s}}_1, \tb{\ti{a}}_1^*)] V^*(\tb{\ti{s}}_2)  \Big \} \\
  &+ \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}_1) \Big\}
\end{align}

Using Lemma \ref{lemma:sum_diff_prob_v}, 
\begin{align}
    \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)}[Q^*(\tb{\ti{s}}_1,\tb{\ti{a}}_1)] - V^*(\tb{\ti{s}}_1) \geq \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}_1) \Big\} \label{eqn:final_qv}
\end{align}
Using Equation \eqref{eqn:final_qv} in Equation \eqref{eq_Q_V}, 
\begin{align}
    &R_{\theta,k} \geq  \mathbb{E}_{\tb{\ti{a}}_1 \sim\ \pi^k_{\theta}(\tb{\ti{s}}_1), \tb{\ti{s}}_2 \sim\ \mathbb{P}(.|\tb{\ti{s}}_1,\tb{\ti{a}}_1)}[V^{\pi^k_{\theta}}(\tb{\ti{s}}_2) - V^*(\tb{\ti{s}}_2)] \\
 &+ \mathbb{E}_{\tb{\ti{a}}_1 \sim \pi^k_{\theta}(\tb{\ti{s}}_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\tb{\ti{s}}_1 \neq goal \} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}_1) \Big\}
\end{align}

By recursion, Lemma \ref{lemma:sum_diff_prob_v} and since $V^*(\tb{\ti{s}}) \geq V^*_1$ for any $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$: \\
\begin{align}
    R_{\theta,k}  \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{k} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\tb{\ti{s}}_h \neq goal \} \mathbbm{1}\{\sgn(a^h_{i,p}) \neq \sgn(\theta_{i,p})\} \Big\}
\end{align}
 where, the expectation is taken with respect to trajectory induced in the $k^{th}$ episode by the interaction of policy $\pi^k_{\theta}$ and transition kernel $\mathbb{P}_{\theta}(.|.,.)$. Now, the total expected regret over $K$ episodes is: 
 \begin{align}
     R_{\theta}(K) \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{t=1}^{\infty} \mathbb{E}_{\theta, \pi_{\theta}} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\tb{\ti{s}}_t \neq goal \} \mathbbm{1}\{\sgn(a^t_{i,p}) \neq \sgn(\theta_{i,p})\} \Big\}
 \end{align}
 Analogous to \cite{min2022learning}, \cite{cohen2021minimax}, we define: 
 \begin{align}
     N = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq \goal\}
 \end{align}
\textcolor{red}{Remark:we need to deal with same notation as $[n]$} representing the random variable for total number of time steps over K episodes and for agent $i \in [n]$, $j \in [d-1]$,
 \begin{align}
     N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\}
 \end{align}
that represents the number of times in the entire duration of $K$ episodes that the agent $i$ chose $j^{th}$ component of its action as same as that of the optimal. Thus, 
\begin{align}
    R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi_{\theta}}  [ \sum_{i=1}^{n} \sum_{j=1}^{d-1} N_{i,j}(\theta) ]
\end{align}
To use the standard Pinsker's Inequality, we need $N_{i,j}(\theta)$ to be bounded almost surely which is known to not hold for SSPs (\cite{min2022learning},\cite{cohen2021minimax}). Hence, we use the capping trick introduced by \cite{cohen2021minimax} and also used by \cite{min2022learning}. In this trick, we cap the learning process to a predetermined $T$. 
If the learning process (i.e. $K^{th}$ episode) ends before this, the agents continue to remain at $goal$. In this case the summation for the actual process and the capped process is the same. On the other hand when $K$ episodes end beyond $T$, we have a truncated sum. Due to non-negativity of each part (Indicator function), the sum for the capped process lower bounds the actual sum. \\ Define 
\begin{align}
    N^- = \sum_{t=1}^T\mathbbm{1}\{\tb{\ti{s}}_t \neq \goal\}
\end{align} 
and for any agent $i \in [n] $ and $ j \in [d-1],$
\begin{align}
    N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{\tb{\ti{s}}_t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\}
\end{align} 
It is easy to see that (since any component of action has to match corresponding of $\theta$ or $\theta^j$) for any $i \in [n]$ and $j \in [d-1]$, 
\begin{align}\label{eqn:ntotal}
    N^- =   N^-_{i,j}(\theta) + N^-_{i,j}(\theta^{j}) 
\end{align}
 where for every $\theta \in \Theta$, $\theta^j$ represents the vector that only differs from $\theta$ at the $j^{th}$ index of every $\theta_i$ in $\theta = \{\theta_1,1,\theta_2,1,\dots,\theta_n,1\}$, where each $\theta_i \in \{\frac{-\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}\}^{d-1}$. \\  
Thus,  
\begin{align}
    R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi_{\theta}}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}
\end{align}
  Notice that $\theta \in \Theta \iff \theta^{j} \in \Theta$. This follows from definition of $\Theta$. Fixing $\pi_{\theta} = \pi$, this helps us write as follows: 
  \begin{align}
      2 \sum_{\theta \in \Theta} &R_{\theta}(K)\\
      &\geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \{ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \} \\
      &= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^- - N^-_{i,j}(\theta)] \}
      \end{align}
    Above, we use \eqref{eqn:ntotal}
      \begin{align}
       &2 \sum_{\theta \in \Theta} R_{\theta}(K)\\
          &= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^-] - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}\\
      &= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}
  \end{align}
  The above step is due to for any $j \in [d-1]$, for any $f(.)$, we have $\sum_{\theta \in \Theta} f(\theta^j) = \sum_{\theta \in \Theta} f(\theta) $
Using Lemma \ref{lemma:pinsk} and Lemma \ref{lemma:gen_co}, \\
\begin{align}
    &2 \sum_{\theta \in \Theta} R_{\theta}(K) \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  \mathbb{E}_{\theta, \pi}  [N^-] +  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] - \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] \} \Big \} \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV^*_1/4 -  \{  \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] - \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] \} \Big \} \label{eqn:exp_diff} \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV^*_1/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \}
\end{align}
Using Lemma \ref{lemma:kl_d}, 
\begin{align}
    &2 \sum_{\theta \in \Theta} R_{\theta}(K) \\
    &\geq \frac{2 \Delta V_1^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{1/2} \sqrt{3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]}  \} \Big \}  \\
    &= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{\mathbb{E}_{\theta}[N^-]} \Big \} \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{T} \Big \} \\
    &= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \}
\end{align}
In the last second step we used the fact that $N^- \leq T$ \\
Further, notice that the term inside the bracket is independent of $\theta, i$ or $j$. Thus, we have: 
\begin{align}
    \sum_{\theta \in \Theta} R_{\theta}(K) \geq  \Delta V_1^* |\Theta| \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \}
\end{align}
Thus by rearranging and using $\sqrt{3}<2$,
\begin{align}
    \frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq   V_1^*  \Big \{ \Delta  KV_1^*/4 -   (KV_1^*)^{3/2}  \frac{2^{n+2}.\Delta^2}{\sqrt{\delta} (d-1)} \Big \}
\end{align}
Pick, 
\begin{align}
    \Delta^* = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}
\end{align}
At this value of $\Delta$,
\begin{align}
    &\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \\
    &\geq V_1^* \Bigg \{  \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}. \frac{KV_1^*}{4} - \frac{(KV_1^*)^{3/2}.2^{n+2}}{\sqrt{\delta}(d-1)}. \Big \{\frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}\Big\}^2 \Bigg \} \\
    &= V_1^* \Bigg\{\frac{(d-1) \sqrt{\delta.K.V_1^*}}{2^{n+7}} - \frac{(d-1)\sqrt{\delta.K.V_1^*}}{2^{n+8}}\Bigg\} \\
    &\geq  \frac{(d-1).\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+8}} \\
    &\geq \frac{d.\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+9}}
\end{align}
In the last second line, we use that $V^*_1>1$ and in the last line, we use $d-1 \geq d/2$ for any natural number $d\geq 2$ which holds for our instances. Since the average over entire set is lower bounded by the RHS, there must exist some parameter in the set for which the RHS is a lower bound. Hence proved. \\
It remains to show that the $\Delta$ picked above is valid. \\ Hence, need to ensure that: 
\begin{align}
    \Delta = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}} < 2^{-n}.\Bigg \{\frac{1-2\delta}{1+n+n^2} \Bigg \} 
\end{align}
which gives: 
\begin{align}
    K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.\{\frac{1-2\delta}{1+n+n^2}\}^2} 
\end{align}
\end{proof}


\subsection{Proof of Lemma \ref{lemma:gen_co}}

\textbf{Recall the Lemma  \ref{lemma:gen_co}.}  \textit{If $T \geq 2KV^*_1$, then, $\mathbb{E}_{\theta}[N^-] \geq KV^*_1/4$,  for any $\theta \in \Theta$.} 

\begin{proof}
If capped process finishes before $T$, then $N^-=N$. Else, number of visits to $goal$ state is less than $K$ due to which $N^- \geq T-K$. Therefore, we have
% 
\begin{align}
    \mathbb{E}[N^-] \geq \mathbb{E}[\min\{T-K,N\}] \geq \mathbb{E}[\sum_{i=1}^K\min\{T/K-1, N_k\}]
\end{align}
% 
In the above, $N_k$ is the random variable representing the length of episode $k$. Since $T\geq2KV^*_1,$ and $V^*_1\geq1$ the lemma will hold for any policy if $N_k \geq V^*_1$ with probability $\geq 1/4$ for any policy. Consider any policy.  
\begin{align}
    \mathbb{P}[N_k \geq V^*_1] &= \mathbb{P}(\tb{\ti{s}}_2 \neq \tb{\ti{g}}|\tb{\ti{s}}_1=\tb{\ti{s}}).\mathbb{P}(\tb{\ti{s}}_3 \neq \tb{\ti{g}}|\tb{\ti{s}}_2).\mathbb{P}(\tb{\ti{s}}_4 \neq \tb{\ti{g}}|\tb{\ti{s}}_3) \dots \mathbb{P}(\tb{\ti{s}}_{\lceil V^*_1\rceil} \neq \tb{\ti{g}}|\tb{\ti{s}}_{\lfloor V^*_1\rfloor-1}) 
    \\ 
    &= (1-p^{a(\tb{\ti{s}}_1)}_{\tb{\ti{s}}_1,goal}).(1-p^{a(\tb{\ti{s}}_2)}_{\tb{\ti{s}}_2,goal})\dots(1-p^{a(\tb{\ti{s}}_{\lfloor V^*_1\rfloor-1})}_{\tb{\ti{s}}_{\lfloor V^*_1\rfloor-1},goal}) 
\end{align}
For any state $\tb{\ti{s}}$, $1-p^{a(\tb{\ti{s}})}_{\tb{\ti{s}},goal}$ is minimum when $p^{a(\tb{\ti{s}})}_{\tb{\ti{s}},goal}$ is maximum. Check from Lemma \ref{lemma:general_tp} that this happens at $a^*$ which matches all signs with $\theta$, i.e., $a^* = a_{\theta}$ and at any $\tb{\ti{s}} \in \mathcal{S}_{n,1}$(i.e., $p^*_{1,0}$). Thus, we can lower bound the above product as: 
\begin{align}
    \mathbb{P}[N_k \geq V^*_1]  & \geq 
    (1-p^*_{\tb{\ti{s}}_1,goal}).(1-p^*_{\tb{\ti{s}}_2,goal})\dots(1-p^*_{s_{\lfloor V^*_1 \rfloor -1},goal}) 
    \\
    & \geq (1-p^*_{1,0})^{\lfloor V^*_1 \rfloor -1} 
    \\
    & \geq (1-p^*_{1,0})^{ V^*_1 } 
    \\
    &= (1-p^*_{1,0})^{ 1/{p^*_{1,0}} }
    \\
    & \geq 1/4
\end{align}
For the last second inequality, we use for $x\geq 2$, $(1-1/x)^{x}\geq 1/4$ 
Why here $x = 1/p^*_{1,0}\geq 2$ is shown at the end of the alternate proof below. \\
\textcolor{red}{can someone comment if there's any issue with above proof?}
Thus, 
 \begin{align}
     \mathbb{E}[N^-]  \geq \mathbb{E}[\sum_{i=1}^K min  \{T/K-1, N_k\}] \geq KV^*_1/4
 \end{align}

\subsubsection{Alternate proof for showing $\mathbb{P}[N_k \geq V^*_1] \ge \frac{1}{4}$}
 
Using Lemma \ref{lemma:episodelength}, for some $\tb{\ti{s}}_1 \in \mathcal{S}(1)$, we have, 
\begin{align}
    \mathbb{P}^{\pi}[N_k \geq V^*_1](\tb{\ti{s}}) 
    &\geq 
    \mathbb{P}^{\pi^*}[N_k \geq V^*_1](\tb{\ti{s}})  
    \\
    &\geq \mathbb{P}^{\pi^*}[N_k \geq V^*_1](\tb{\ti{s}}_1) 
    \\
    &= (1-p^*(goal|\tb{\ti{s}}_1,\tb{\ti{a}}^*))^{\lfloor V^*_1 \rfloor  } 
    \\
    &\geq (1-p^*(goal|\tb{\ti{s}}_1,\tb{\ti{a}}^*))^{ V^*_1 }  
    \\
    &\geq 1/4
\end{align}
% 
Here, the last inequality comes from the fact $V^*_1 = 1/p^*(goal|\tb{\ti{s}}_1, \tb{\ti{a}}^*)$ (see proof of Theorem \ref{thm:all_in_one}) that for $x>2$, $(1-1/x)^x \geq 1/4$. \\Note that $V^*_1 = \frac{2n}{n-1+2(\delta+\Delta)} > 2$ since 
\begin{align}
    \frac{1}{V^*_1} & = \frac{n-1}{2n} + \frac{2(\delta+\Delta)}{2n} 
    \\
    & < \frac{n-1}{2n} + \frac{2(\delta+2^{-n}.\frac{1-2\delta}{1+n+n^2})}{2n} 
    \\
    & < \frac{n-1}{2n} + \frac{2(\delta+\frac{1-2\delta}{6})}{2n} 
    \\
    &= \frac{n-1}{2n} + \frac{(\frac{1+4\delta}{3})}{2n} 
    \\
    & < 1/2
\end{align}
Above, the first inequality arises due to $\Delta < \frac{1-2\delta}{1+n+n^2}$ for our instances, the second inequality arises due to $n \geq 1$ and the final step is due to $\delta < 1/2$.
\end{proof}


\section{Preliminaries and Problem Formulation} 
\label{sec:problem}




\subsection{Notations and Preliminaries}
\label{subsec:prelims}


\begin{itemize}
    \item Directly start with our setup --- multi-agent ssp -- what it is -- 
\end{itemize}



\paragraph{General MA-SSP.} We consider a general \emph{Multi-Agent Stochastic Shortest Path (MA-SSP)} problem, defined by the tuple $(\mathcal{V}, N, \mathbb{P}, \mathcal{A})$. Here $\mathcal{V} = \{v_1, v_2, \dots, v_q\}$ denotes the set of nodes, and $N = \{1,2,\dots,n\}$ is the set of $n$ agents. At any given time, each agent occupies exactly one node. The global state of the system is represented as $\tb{\ti{s}} = (s_1, s_2, \dots, s_n) \in \mathcal{S}$, where $s_i \in \mathcal{V}$ denotes the node occupied by agent $i$. Thus, the overall state space is $\mathcal{S} = \mathcal{V}^n$.
\\
\textcolor{red}{Need to mention definition of $r$ and the partition}

Each agent $i \in N$ has an action space $\mathcal{A}^i$, assumed to be independent of its current location. \textcolor{red}{reframing the prev sentence as: "The set of actions $\mathcal{A}^i$ available to any agent $i \in N$ is the same at every node." Also we missed to emphasize that each agent takes action independently. So we can add this line: "Agents take these actions independently."} A global action is denoted as $\tb{\ti{a}} = (a_1, a_2, \dots, a_n) \in \mathcal{A}$, where $\mathcal{A} = \mathcal{A}^1 \times \cdots \times \mathcal{A}^n$. The transition dynamics of the system are governed by a probability distribution $\mathbb{P}$ such that, given a state-action pair $(\tb{\ti{s}}, \tb{\ti{a}})$, the next state $\tb{\ti{s}}'$ is drawn from $\mathbb{P}(\cdot \mid \tb{\ti{s}}, \tb{a})$. This formulation naturally captures the coupling among agents: the future state of each agent may depend on the joint configuration and action of all agents.

Each agent $i$ incurs a \textcolor{red}{an instantaneous} random cost $c^i(\tb{\ti{s}}, \tb{a}) \in [c_{\min}, 1]$ upon taking action $\tb{a}$ in state $\tb{\ti{s}}$, where $c_{\min} > 0$. \textcolor{red}{prev statement sounds like agent i is taking the action $\tb{\ti{a}}$. We can reframe it as: "When global action $\tb{\ti{a}} \in \mathcal{A}$ is taken in global state $\tb{\ti{s}} \in \mathcal{S}$, agent $i \in N$ recieves cost $c^i(\tb{\ti{s}},\tb{\ti{a}})$". I'm also thinking do we need to write the range of cost because it is nowhere used in lower bound analysis. I have used cost as 1 but that doesn't require specific condition on costs. In upper bound, I think there are some steps that need this. But we don't need it for lower bound.}
This individual cost can depend on the full joint state and joint action, encapsulating complex multi-agent interdependencies. \textcolor{red}{Reframing previous sentence: Notice that, in general, the individual costs depends on the location and action of other agents as well as of itself encapsulating complex multi-agent interdependencies. } \\
\\
\textcolor{red}{I personally think there is no need to even talk anything in detail about congestion: basically we can get rid of the next two equations to reduce this section. The last line of the previous paragraph suggests a broad generalisation. Or we can push the discussion on how congestion can be modelled into into appendix and reference here in one line. }

We consider the notion of \emph{congestion-aware costs} to model multi-agent interference. Let $K^i(\tb{\ti{s}}, \tb{a})$ denote a private cost component for agent $i$, capturing all factors other than congestion. The congestion factor for agent $i$ is modeled as:
\begin{align}
    c_f^i(\tb{\ti{s}}, \tb{a}) = \sum_{j=1}^n \mathbbm{1}\{a_j = a_i\},
\end{align}
which counts how many agents (including $i$ itself) are taking the same action. The total cost to agent $i$ is then given by:
\begin{align}\label{eqn:ind_cost}
    c^i(\tb{\ti{s}}, \tb{a}) = c_f^i(\tb{\ti{s}}, \tb{a}) \cdot K^i(\tb{\ti{s}}, \tb{a}).
\end{align}
The global cost is defined as the average of individual costs:
\begin{align}\label{eqn:glb_cost}
    c(\tb{\ti{s}}, \tb{a}) = \frac{1}{n} \sum_{i=1}^n c^i(\tb{\ti{s}}, \tb{a}) = \frac{1}{n} \sum_{i=1}^n \left( \sum_{j=1}^n \mathbbm{1}\{a_j = a_i\} \cdot K^i(\tb{\ti{s}}, \tb{a}) \right).
\end{align}

The goal is to design policies that \textcolor{red}{instead reframe as : The goal is to identify a policy i.e., a \emph{scheme} of taking actions to} minimize the expected cumulative global cost incurred in reaching a target state $\tb{g}$ from a fixed initial state $\tb{\ti{s}}_{\init}$. 
Let $\Pi_{\textcolor{red}{HR}}$ denote the set of all history-dependent randomized policies mapping past trajectories to \textcolor{red}{probability} distributions over actions. Due to the Markovian and stationary nature of the system's $\textcolor{red}{transition}$ dynamics and cost structure, it suffices to consider deterministic Markovian  policies ($\textcolor{red}{\Pi_{MD}}$) without loss of optimality (see, e.g., \cite{puterman2014markov}).

\textcolor{red}{Further,} Not all \textcolor{red}{such} policies ensure successful completion of the task. \textcolor{red}{we didn't define what the task is so better to say "termination of the navigation process to \tb{\ti{g}}"} 
A policy is termed \emph{proper} if it leads to the goal state $\tb{g}$ almost surely, from any initial state. Otherwise, it is termed \emph{improper}, and its expected cumulative cost may be \textcolor{red}{why may be? replace with : is for at least one state?} unbounded. We assume the existence of at least one proper policy and denote the set of all proper policies as $\Pi_p$ \citep{tarbouriech2020no, tarbouriech2021stochastic, cohen2021minimax,min2022learning}.

For any policy $\pi \in \Pi_p$, we define the value function at state $\tb{\ti{s}}$ \textcolor{red}{for any state} as the expected cumulative cost until reaching $\tb{g}$:
\begin{align}
    V^\pi(\tb{\ti{s}}) = \mathbb{E} \left[ \sum_{t=1}^{\tau^\pi} c(\tb{\ti{s}}_t, \pi(\tb{\ti{s}}_t)) \,\middle|\, \tb{\ti{s}}_1 = \tb{\ti{s}} \right],
\end{align}
where $\tau^\pi$ denotes the (random) hitting time of the goal under policy $\pi$. The optimal value function is defined as $V^*(\tb{\ti{s}}) = \min_{\pi \in \Pi_p} V^\pi(\tb{\ti{s}})$, and the optimal policy $\pi^*$ achieves this minimum. We define the \emph{diameter} $B^*$ of the MA-SSP problem as the worst-case \textcolor{red}{worst-case sounds informal, replace with maximum expected} cost-to-go from any state under the optimal policy:
\begin{align}
    B^* = \max_{\tb{\ti{s}} \in \mathcal{S}} V^*(\tb{\ti{s}}).
\end{align}

In the \emph{learning} setting, the transition function $\mathbb{P}$ and/or the cost function $c(.,.)$ are initially unknown. The agent must interact with the environment over $K$ episodes, each beginning at $\tb{\ti{s}}$ and terminating upon reaching $\tb{\ti{g}}$. The agent must balance exploration and exploitation to learn the optimal policy efficiently.

Let $h_k$ be the random episode length for episode $k$ 
 \textcolor{red}{replace as: be the random length of episode $k$}, and let $(\tb{\ti{s}}_{k,h}, \tb{a}_{k,h})$ denote the state and action at step $h$ of episode $k$. Then, the expected cumulative regret of a learning algorithm $\mathfrak{A}$ over $K$ episodes is defined as:
\begin{align}\label{eqn:regret}
    \mathbb{E}_{\mathfrak{A}}[R(K)] = \mathbb{E} \left[ \sum_{k=1}^K \sum_{h=1}^{h_k} c(\tb{\ti{s}}_{k,h}, \tb{a}_{k,h}) \right] - K \cdot V^*(\tb{\ti{s}}_{\init}).
\end{align}
This regret quantifies the performance gap between the learning agent \textcolor{red}{we have multiple learning agents} and an oracle that follows the optimal policy from the start. The goal in MA-SSP learning is to design algorithms that minimize regret, ideally achieving sublinear growth in $K$. 


Recall that the best policy must minimize the cumulative global cost to go from $s_{init}$ to $goal$ and not just the cumulative cost to a particular agent. However, the actions are taken by individual agents. But these agents directly receive only their individual costs and do not have a direct access to others' costs or to the global cost. 
This problem could be solved by the use of a central controller who may coordinate actions and receive signals (individual costs from each agent). However, this significantly increases computation and transmission costs for higher number of agents and would degrade robustness to malicious attacks \citep{zhang2018fully}. Further, agents may be unwilling to share their individual costs to preserve privacy. \pt{As opposed to the central controller approach we consider a decentralized setting where the agents action and thus the reward are preserved.} 
Hence mechanism that ensure agents learn the best policy independently is desirable which takes us into the purview of Decentralized Multi-Agent Reinforcement Learning. But a common goal cannot be achieved without sharing of any information (\textcolor{red}{why? cite?}). For this, (\textcolor{red}{cost parametrisation was motivated from which papers? or was completely new in maccm paper?})(cite) proposes parametrizing the expected costs, namely for all $(\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S} \times \mathcal{A}$, there exist known features $\psi(\tb{\ti{s}},\tb{\ti{a}}) \in R^{nd}$ and an unknown parameter $\tb{w} \in R^{nd}$ for the instance such that $\mathbb{E}[c(\tb{\ti{s}},\tb{\ti{a}})]=\langle \psi(\tb{\ti{s}},\tb{\ti{a}}),\tb{w} \rangle$.
Hence, instead of sharing actual costs, agents can now share their estimate of the unknown parameter. 
Further, since the state and action space is explosively large, we assume the following linear function approximation of transition probabilities to hold:
\begin{assumption} \label{assm:lfa_prob}
    For every pair $(\tb{\ti{s}},\tb{\ti{a}},\tb{\ti{s}}') \in \mathcal{S}\times\mathcal{A}\times\mathcal{S}$,  there exists known features $\phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \in \mathbb{R}^{nd}$ and unknown $\theta \in \mathbb{R}^{nd}$ such that, for any $\tb{\ti{s}}' \in \mathcal{S}$, $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) = \langle \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}),\theta \rangle$. 
\end{assumption}


\pt{We can directly write this thing after defining the features, no need to write it here.}

Due to the above two linear function approximations we will refer to these MASSPs as Linear Mixture MASSPs, LM-MASSPs. They are in general able to capture complex transition interdependencies. We describe a possible feature design for transition probabilities in \ref{subsec:features}. 


\subsection{Problem Formulation}
\label{subsec:problem_formulation}
% 
In the above-described setting, \citep{trivedi2023massp} provided an algorithm whose expected cumulative regret scales as $\widetilde{O}(\sqrt{K})$. To obtain a lower bound in this setting, we need to construct difficult-to-learn instances with tractable optimal policy and analyze its difference from any policy in terms of value function. Similar to arguments in the lower bound proof in \citep{auer2002nonstochastic}, it is sufficient to consider deterministic policies just for notational convenience and the proposed proof can be extended for randomized policies as well. 



Similar to \cite{osband2016lowerboundsregretreinforcement}, we define a Decentralized Multi-Agent Reinforcement Learning algorithm as a deterministic sequence of $\{\pi_t|t=1,2\dots\}$ functions. Here each function $\pi_t$ maps history $\mathcal{H}_t$ till time $t$ to a map in the set of all maps from the set of agents to the set of all possible probability distributions over actions i.e., $\pi_t \in \{(\pi^1,\pi^2,\dots,\pi^n) : \pi^i \in \Delta(\mathcal{A}^i) \forall i \in [n] \}$ where $\Delta(\mathcal{A}^i)$ denotes the probability simplex over individual actions, $\pi^i$ for $i \in [n]$ denotes the independent strategy of choosing actions by agent $i$. \\
In the below section, we demonstrate how to construct these hard to learn instances.

\pt{This section is vey loose as of now. we need to handle the cases.}



\subsection{Construction of the Problem Instances}
\label{subsec:problem_instance}

All instances in our consideration have only two nodes i.e., $\mathcal{V} = \{s,g\}$. Hence, $\mathcal{S} = \Pi_{i \in [n]} \{s,g\} = \{s,g\}^{n}$. Thus, the total number of states, $|\mathcal{S}| = 2^n$. Also, we fix $\tb{\ti{s}}_{\init} = (s,s,\dots,s)$ and $goal = \tb{g} = (g,g,\dots, g)$. At every node, we let the actions available to any agent $i \in [n]$ be the same as $\mathcal{A}^i = \{-1,1\}^{d-1}$ for some $d \geq 2$. Thus the global action space $\mathcal{A}=\{-1,1\}^{n(d-1)}$. Hence, $|\mathcal{A}| = 2^{n(d-1)}$. Further, we assume that once an agent reaches node $g$, it cannot go back to node $s$. Hence, transitions like $\tb{\ti{s}} = (s,s,\dots,g,g) \rightarrow \tb{\ti{s}}'=(s,s,\dots ,g,s)$ are impossible.

\pt{partitioning of the state space- -- we partition the state space based on r, the number of agents at the state s. $\mathcal{S}_r$ -- of type r... $\mathcal{S}(s)$ -- reachable from $s$. $\mathcal{S}_r(s)$ -- reachable from s of type r. }

Any of our instance is parametrized by a tuple $(n,\delta, \Delta, \theta)$ where $n \geq 1$ is the number of agents, $2/5 < \delta < 1/2$ and $\Delta < 2^{-n} \cdot \frac{1-2\delta}{1+n+n^2}$ are parameters of our proposed features \pt{ref this section .. that the detailed feature design in given in the next subsection. The features are defiend for a given instance. }

, and $\theta$ is an $nd$- dimensional vector of the form $\theta = (\theta_1,1, \theta_2,1,\dots,\theta_n,1)$ where for every $i \in [n]$, $\theta_i$ is a $(d-1)$ dimensional vector each of whose component is $\pm \frac{\Delta}{n(d-1)}$. Let the set of all such $\theta$'s be $\Theta$. $\theta$ is a parameter related to the transition probability model mentioned in Assumption \ref{assm:lfa_prob}. For convenience, we will sometimes use $\widetilde{\theta} = (\theta_1,\theta_2,\dots,\theta_n)$ wherever required.

\pt{This is an additional challenge -- and this is very common in MARL Setting. so, to avoid that the instance is suitably chosen -- via cost -- then comes remark 2 -- why such  is possible -- here we need to the cost eqn from previous section. }

\begin{remark}
    For a general cost and transition probability function, there may in general be a trade-off between policy that takes the system ``closer'' to the goal (hence minimizing the number of time steps to reach the goal) and another that takes more time but may be (in an overall sense) cost efficient \citep{tarbouriech2020no}. 
\end{remark}




To avoid this complication in the analysis of our instances, we let for all $\tb{\ti{s}} \in \mathcal{S}\backslash\{\tb{\ti{g}}\}$ and $\tb{\ti{a}} \in \mathcal{A}$, $c(\tb{\ti{s}},\tb{\ti{a}}) = 1$ while for any $\tb{a} \in \mathcal{A}, c(\tb{\ti{g}}, \tb{\ti{a}}) =0$. Hence, the policy that takes us "nearer" to $goal$ is better. This leads to optimum policy being directly influenced by transition probabilities. 

The following justifies how such instances are possible.
\begin{remark} \label{rem:cost_one}
    One class of such instances is the one for whom for all $i \in [n], \tb{\ti{a}} \in \mathcal{A}, K^i(\tb{\ti{s}},\tb{\ti{a}}) = \frac{1}{\sum_{j=1}^n \mathbbm{1}\{a_j=a_i\}}$ for all $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$ and $ K^i(\tb{\ti{g}},\tb{\ti{a}}) = 0$ . From Equation \ref{eqn:ind_cost} and Equation \ref{eqn:glb_cost} one observes that for such instances for all $(\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S}\backslash\tb{\ti{g}} \times \mathcal{A}$, $c(\tb{\ti{s}},\tb{\ti{a}}) = 1$ and $c(\tb{\ti{g}}, \tb{\ti{a}}) = 0$. 
\end{remark}

 


\subsection{Features} 
\label{subsec:features}


For the type of instances mentioned in the previous subsection, we now provide the valid features for the transition probability model mentioned in Assumption \ref{assm:lfa_prob}.


Note that there can be many possible feature designs but all of them must satisfy the following requirements to produce valid transition probabilities in any instance defined above in \ref{subsec:problem_formulation}:
\begin{requirements}
    For any $(\tb{\ti{s}},\tb{\ti{a}},\tb{\ti{s}}') \in \mathcal{S}\times\mathcal{A}\times\mathcal{S}$, the transition probability $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) \geq 0$ and for any $(\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S}\times \mathcal{A}$, $\sum_{\tb{\ti{s}}' \in \mathcal{S}}\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) = 1$ \label{reqm:1}
\end{requirements}
\begin{requirements}
   If there is a physically impossible transition to some $\tb{\ti{s}}' \in \mathcal{S}$ from some $\tb{\ti{s}} \in \mathcal{S}$, under action $\tb{\ti{a}} \in \mathcal{A}$, then $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) = 0$ and if there's a certain transition to some $\tb{\ti{s}}' \in \mathcal{S}$ from some $\tb{\ti{s}} \in \mathcal{S}$ under action $\tb{\ti{a}} \in \mathcal{A}$, then $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) = 1$. \label{reqm:2}
\end{requirements}
For our instances, we consider the following feature design :
\begin{equation}
\label{eqn:features_global_new}
\phi(\tb{\ti{s}}^{\prime} | \tb{\ti{s}},  {\ti{a}}) = 
\begin{cases} (\phi(s^{\prime}_1 | s_1, {\ti{a}}_1), \dots, \phi(s^{\prime}_n | s_n, {\ti{a}}_n)), & if ~\tb{\ti{s}} \neq \tb{\ti{g}} ~\text{and}~  s^\prime_{i} = g ~\text{if} ~ s_i = g,~ \forall~ i\in [n]
\\
\mb{0}_{nd}, & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime} \neq \tb{\ti{g}}, \text{or } \tb{\ti{s}} \neq \tb{\ti{g}} ,  \exists~ i \in [n],~ s.t. ~ s_i = g, s^\prime_i = s
\\
(\mb{0}_{nd-1}, 1), & if ~ \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}^{\prime}  = \tb{\ti{g}} 
\end{cases}
\end{equation}

Recall that, in the above, $a_i$, $s_i$ and $s^{\prime}_i$ represent the individual action, current node and next node, respectively, of agent $i \in [n]$. Also, observe that the first case corresponds to the most general transitions that are allowed, the second case represents all impossible transitions and the third case takes care of the only \textit{certain} transition.\\
Further, $\phi(s^{\prime}_i | s_i, {\ti{a}}_i)$ are defined as 
\begin{equation} \label{eqn:features_global_new_gen}
\phi(s^{\prime}_i | s_i, {\ti{a}}_i) = \begin{cases}  
\left(-{\ti{a}}_i, \frac{1-\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}_i = s^{\prime}_i = s
\\
\left({\ti{a}}_i, \frac{\delta}{n 2^{r-1}} \right)^{\top}, & if ~ {s}_i = s,~s^{\prime}_i = g
\\
\left(\mathbf{0}_{d-1}, \frac{1}{n 2^{r}} \right)^{\top}, & if ~ {s}_i = g,~ s^{\prime}_i = g
\end{cases}
\end{equation}

In the above, $r$ represents the number of agents at node $s$ in the current global state $\tb{\ti{s}}$. 

\begin{lemma}\label{lemma:valid_features}
    Features defined above in equations \ref{eqn:features_global_new} and \ref{eqn:features_global_new_gen}, produce valid transition probabilities for any instance $(n,\delta,\Delta,\theta)$ as defined in \ref{subsec:problem_instance}. Specifically they satisfy both requirements \ref{reqm:1} and \ref{reqm:2}.
\end{lemma}
We refer the reader to Appendix \ref{proof:lemma:valid_features} for the proof.

In the following lemma, we derive a general expression for the probability of any valid transition for any instance $(n, \delta, \Delta, \theta)$ as defined in \ref{subsec:problem_instance}. 
\textcolor{red}{the below lemma statement will simplify depending on if these definitions are incorporated in \ref{subsec:prelims}}
\begin{lemma}
\label{lemma:general_tp} 
Consider any state $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$. In this state $\tb{\ti{s}}$, let $\mathcal{I}:=\{i_1,i_2,\dots,i_{r}\}$ denote the set of agents at node $s$ and $\mathcal{J}:=\{j_1,j_2,\dots,j_{n-r}\}$ be those at node $g$. 
Under a valid transition, either the next state is the same as $\tb{\ti{s}}$ or possibly some agents from $\mathcal{I}$ transit to node $g$. Let the set of all valid next states from $\tb{\ti{s}}$ be denoted as $\mathcal{S}(\tb{\ti{s}})$. To study a particular transition to $\tb{\ti{s}}'\in \mathcal{S}(\tb{\ti{s}})$, we define $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ as the set of all agents moving from node $s$ to node $g$. Here, $r'$ denotes the number of agents in state $\tb{\ti{s}}'$ that are at node $s$. For any action $\tb{\ti{a}} \in \mathcal{A}$, the transition probability is given as: 
\begin{align}
    &p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'} = 
 \mathbb{P}(\tb{\ti{s}}^\prime | \tb{\ti{s}}, \tb{\ti{a}}) 
=\frac{r' + (r-2r')\delta}{n \cdot 2^{r-1}} +   \frac{n-r}{n \cdot 2^r}        +    \frac{\Delta}{n}  (r-2r') \\
&\quad + \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn({{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn({{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}
\end{align} 
\end{lemma}


\pt{The following corollary provides the probability when action are as in Theorem 1. This probability only depends on $r$ and $r'$ only. i am thinking to remove this corollary and put it as the another statement in the above lemma.
} \textcolor{red}{i dont mind. can we decide upon these things after doing one round of appendix?}


\begin{corollary} \label{corollary:p_star}
From Lemma \ref{lemma:general_tp}, we observe that for any given instance $(n, \delta, \Delta, \theta)$ if the action chosen is such that the indicators vanish in the above expression, the transition probability doesn't depend on $\mathcal{I}$ and $\mathcal{T}$ and only depends on $r$ and $r'$. Hence, we define this special global action $\tb{\ti{a}}_{\theta}$ as the action whose $\{(d-1)\times (i-1)+j\}-th$ element for every $i \in [n]$ and every $j \in [d-1]$ is given by $\sgn(\theta_{i,j})$. In other words,  $\tb{\ti{a}}_{\theta} = \frac{n(d-1)}{\Delta} \times \widetilde{\theta}$. 
\end{corollary}


\subsection{Summary of Approach}


\pt{Why we created these instances like these -- why we expect good results from this instance -- etc. -- why it is hard .}


Any deterministic algorithm produces, in general, a history-dependent policy. Fixing any such policy $\pi$, we will analyze the regret of this policy on a set of hard to learn instances that differ only due to $\theta$ (i.e., have same parameters $n, \delta, \Delta$) and show that there exists an instance in the set of hard-to-learn instances that achieves lower bound on expected cumulative regret that scales similarly in terms of number of episodes as upper bound $\widetilde{O}(\sqrt{K})$ reported by \citep{trivedi2023massp}. 
Intuitively, there are two reasons why we expect at least one of the instances in this set to be very hard to be learnt for any given policy:
\begin{itemize}
    \item Firstly, all the instances are characterized by the optimum policy that at any state, the actions taken by each agent are such that they match signs with all components of respective $\theta_i$'s (Theorem \ref{thm:all_in_one}).  In other words, for a given instance $\theta = (\theta_1,1,\theta_2,1,\dots, \theta_n,1)$ we have $\widetilde{\theta} = (\theta_1,\theta_2,\dots,\theta_n)$ and the optimal policy is that: at every state, the global action to be taken must is the same as $\tb{\ti{a}}^* = \{a^*_1,a^*_2,\dots, a^*_n\}$ such that, $\tb{\ti{a}}^* = \frac{n(d-1)}{\Delta} \times \widetilde{\theta}$. 
If we consider a policy such that the action taken in one of the $2^n-1$ non-goal states differed from the optimal action in this state at just one of the $n(d-1)$ indices, then the transition probabilities would differ (from those for optimal policy) only very slightly since $\Delta$ is quite small $(<2^{-n})$. 
Hence, the value function for that policy would be only slightly higher. Observe that there would be $n(d-1).2^{n-1}$ (significant) number of such policies. The policies that differ in the above fashion at any two states are even larger in number and can't be expected to be too worse in terms of the expected cumulative cost for similar reason. Hence, separating these large number of policies efficiently is a challenge before any MASSP learning algorithm. 
\item Secondly, any learning algorithm that efficiently learns the best policy for one instance in the set of all instances, may not be able to efficiently learn some other instance in the set. Also, if a particular action is the best (optimal) for a given instance $\theta = (\theta_1,1,\theta_2,1,\dots,\theta_n,1)$, there definitely exists another instance $\theta = (-\theta_1,1,-\theta_2,1,\dots,-\theta_n,1) \in \Theta$ for whom the same action is the worst.
\end{itemize}
In the following section, we present our observations on these instances and key results that follow.


\section{Theoretical Results}
\label{sec:theory}

\pt{Need to highlight why we need these results, what are the advantages, and what is the summary etc\dots for each of these theorem.}

\pt{Also. we need to clearly highlight the novelty in the proofs, etc.}

Any 2-node LM-MASSP instance as defined in Section \ref{subsec:problem_instance} is reasonably expected to have the notion that under the optimal behavior of agents, a state with more agents at node $g$ is \textit{better}
compared to another state with fewer agents at node $g$. This can be baked mathematically in terms of value functions of states in the following lemma.
% 
\begin{lemma}
\label{prop:1}
    Consider any two states $\tb{\ti{s}}_1, \tb{\ti{s}}_2 \in \mathcal{S}$. Let $\tb{\ti{s}}_1 \in \mathcal{S}(r_1)$ and $\tb{\ti{s}}_2 \in \mathcal{S}(r_2)$. Then, if $r_1>r_2$, we have $V^*(\tb{\ti{s}}_1) > V^*(\tb{\ti{s}}_2)$ and vice-versa.
\end{lemma}
% 
The proof of this lemma is deferred to the Appendix ??. Next, recall that any  multi-agent setting leads to explosion of the number of states and actions due to which it's challenging to obtain optimal policies for the setting. In the following theorem we show that for our instances a tractable optimal policy exists. The optimal action  and the corresponding optimal value depends on the 
Further, we identify a partition of the state space based on number of agents at node $s$ and show that all the states in a particular partition set have the same optimum values. Finally we  show that our instances exhibit property given in lemma \ref{prop:1}.

 
\begin{theorem}\label{thm:all_in_one}
    Consider any instance defined as in \ref{subsec:problem_instance}.
    \begin{itemize}
        \item Then the policy of taking action $\tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$, is optimal. 
        \item Further, optimal value function for each state with the same number of agents at node $s$ takes the same value, i.e., for every $r \in [n]$, it holds that for all $\tb{\ti{s}} \in \mathcal{S}(r)$ we have $V^*(\tb{\ti{s}}) = V^*_r =$ some constant depending on only $r$. We define $V^*_0=0$.
        \item The optimal value function monotonically increases with the number of agents at node $s$ i.e., $0=V^*_0<V^*_1<V^*_2\dots<V^*_n = B^*$. 
    \end{itemize}
    
\end{theorem}


\begin{proof}(of Theorem \ref{thm:all_in_one})
    All the three claims in this theorem are proved together in a single induction argument over $r$. Note that for $r=0$, by definition costs for all actions are $0$ and $V^*=0$. The three claims hold trivially. Hence, we start from $r=1$ as base case in the induction for generalizability. 
    For $r=1$, we consider any $\tb{\ti{s}} \in \mathcal{S}(1)$. We know that the only possible next states are the same state $\tb{\ti{s}}$ or $\tb{\ti{g}}=goal$. For any action $\tb{    \ti{a}} \in \mathcal{A}$ in this state $\tb{\ti{s}}$, by standard arguments we can express the action value function as $Q^*(\tb{\ti{s}},\tb{\ti{a}}) = \frac{1}{1-p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}}}$, where $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}}$ represents the probability of transition from $\tb{\ti{s}}$ to $\tb{\ti{s}}$ itself under action $\tb{\ti{a}}$. The following corollary helps us establish that at action $ a = a_{\theta}$, $Q^*(\tb{\ti{s}}, \tb{\ti{a}})$ is minimum and thus is the optimal action at $\tb{\ti{s}}$.
\pt{instead of writing the following as the corollary, let us use this as a lemma wherever it is required as a part of big theorem}
\begin{corollary}\label{corollary:ps_s}
    From Lemma \ref{lemma:general_tp}, from any state $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$, for any action $\tb{\ti{a}} \in \mathcal{A}$, the probability that the next state is also $\tb{\ti{s}}$ is: 
    \begin{align}
        \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}}) = \frac{r(1-\delta)}{n \cdot 2^{r-1}}+\frac{n-r}{n.2^r}-r.\frac{\Delta}{n} + \frac{2\Delta}{n(d-1)}\sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \mathbbm{1}\{\sgn(\tb{\ti{a}}_{i,p})\neq \sgn(\theta_{i,p})\}
    \end{align}
    Clearly, for any $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$, $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ is minimum at $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$ and is only dependent on $r$ for a given instance (independent of $\mathcal{I}$).
\end{corollary}
    
    Note that the above arguments follow for any $\tb{\ti{s}} \in \mathcal{S}(1)$. Also, due to the above corollary, the value is same too. Thus, the second claim holds. As, $V^*_1 > 0$, third claim holds too. 
    Having shown that the three claims hold for the base case, we assume that they hold for all $r \in [k]$ and use this to show that the three claims hold for $r=k+1$ in the same order. For this, we consider any $\tb{\ti{s}} \in \mathcal{S}(k+1)$. 
    For showing $a^* = a_{\theta}$ we again derive expression for optimal action value function $Q^*(\tb{\ti{s}}, \tb{\ti{a}})$. Note that so far we know the optimal actions at only the states in $\cup_{i \in [k]}\mathcal{S}(i)$. If along any sample path starting from this $\tb{\ti{s}}$, we could reach, with any positive probability, any state outside $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}(i)$, it would be impossible to evaluate $Q^*(\tb{\ti{s}}, \tb{\ti{a}})$. But, for our setting all the \textit{reachable} states from $\tb{\ti{s}}$ lie in $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}(i)$ i.e., $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}(i)(\tb{\ti{s}}) \subseteq \cup_{i \in [k] \cup \{0\}}\mathcal{S}(i)$. \textcolor{red}{need to make sure all these notations and definitions are defined in the \ref{subsec:prelims}} Thus $Q^*(\tb{\ti{s}}, \tb{\ti{a}})$ can be expressed appropriately as 
\begin{align}
   Q^*(\tb{\ti{s}}, \tb{\ti{a}}) = 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})Q^*(\tb{\ti{s}}, \tb{\ti{a}}) +\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +\sum_{r' \in [k]} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'}V^*_{r'} 
\end{align}
    Using the partition of state space based on number of agents at node $s$, identifying that the indicator has positive coefficient if any agent in $\mathcal{I}$ moves from $s$ to $g$ or negative if it stays at $s$,    and using the above induction assumptions, \textcolor{red}{through some clever mathematical manipulations} we show that $Q^*(\tb{\ti{s}}, \tb{\ti{a}})$ is minimized for any $\tb{\ti{s}} \in \mathcal{S}(k+1)$ at $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$. This again requires using Corollary \ref{corollary:ps_s}. Corollary \ref{corollary:p_star} ensures the second claim holds. All the results discussed till now aren't enough to show that $V^*_{k+1}>V^*_k$. We observe that the follwing property holds for our instances:
\begin{property}\label{claim:probability_inequality}
    For all our instances,  for every $r \in [n-1]$, it holds that, for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$. 
\end{property}
The existence of the above property for all our instances helps us use the following lemma to show $V^*_{k+1}>V^*_k$. And thus the main induction over $r$ holds.
\begin{lemma}\label{lemma:probability_inequality}
    If for every $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.
\end{lemma}

\end{proof}

The above theorem provides a broad level of understanding of our features. In the following theorem we provide the main result of this work, namely, tight lower bound in the learning of LM-MASSPs.

\begin{theorem}
\label{thm:lower_bound}
    For any \textcolor{red}{decentralized} MASSP learning algorithm $\mathfrak{A}$ as defined in \ref{subsec:problem_formulation}, there exists a LM-MASSP instance ($\theta \in \Theta$) for every $n \geq 1$, $\delta \in (2/5,1/2)$, $\Delta < 2^{-n}.\frac{1-2\delta}{1+n+n^2}$, such that the expected cumulative regret upon running the algorithm on this instance for $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1. \big \{\frac{1-2\delta}{1+n+n^2} \big \}^2} $ episodes at least matches the reported $\widetilde{O}(\sqrt{K})$ upper bound by \citep{trivedi2023massp} in terms of number of training episodes $K$. Here $V^*_1 = \frac{2n}{n-1+2(\delta+\Delta)}$.  Specifically for this instance, we have $\mathbb{E}_{\theta,\mathfrak{A}}[R(K)] \geq \frac{d.\sqrt{\delta}\sqrt{K.V^*_1}}{2^{n+9}}$     
\end{theorem}

\begin{proof}(of Theorem \ref{thm:lower_bound})
    The proof uses similar techniques as the one for single agent SSP in \cite{min2022learning} and for a two state RL setting by  \cite{jaksch2010near}. But extension to MASSP setting poses many technical challenges such as design of novel features that satisfy the requirements \ref{reqm:1} and \ref{reqm:2}, constructing instance generalizable for any number of agents $n$ with tractable optimal policy, inability to express optimal value function in tractable closed form due to exponentially large number of states, obtaining a reasonably tight upper bound on KL divergence, etc. Some of these challenges are addressed by Theorem \ref{thm:all_in_one}. Others, we deal here. \\
    Consider any history-dependent deterministic policy $\pi$. Consider any set of instances parametrized by fixed $\Big(n \geq 1,\delta \in (2/5,1/2), \Delta < 2^{-n} \cdot \frac{1-2\delta}{1+n+n^2} \Big)$ and differing only due to $\theta \in \Theta$. 
    Suppose agents take actions according to this policy $\pi$. Let, $\tb{\ti{s}}^t$ represent the global state and $\tb{\ti{a}}^t$ the global action at time $t$. Then, the expected regret for the first episode for this instance is: \textcolor{red}{In this discussion I have let time index be superscript}
\begin{align}
R_{\theta,1} &= V^{\pi}(\tb{\ti{s}}^1) - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) \\
     &= \mathbb{E}_{\tb{\ti{a}}^1 \sim\ \pi(\tb{\ti{s}}^1), \tb{\ti{s}}^2 \sim\ \mathbb{P}(.|\tb{\ti{s}}^1,\tb{\ti{a}}^1)}[V^{\pi}(\tb{\ti{s}}^2) - V^{\pi^*_{\theta}}(\tb{\ti{s}}^2)] + \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)}[Q^{\pi^*_{\theta}}(\tb{\ti{s}}^1,\tb{\ti{a}}^1)] - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) 
\end{align} 
The first term indicates a recurrence relationship. The other terms:
\begin{align}
     \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)}[Q^{\pi^*_{\theta}}(\tb{\ti{s}}^1,\tb{\ti{a}}^1)] - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) \\
     &=\mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big \{ \sum_{\tb{\ti{s}} \in \mathcal{S}} [\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}}^1, \tb{\ti{a}}^1) - \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}}^1, \tb{\ti{a}}^1^*)] V^{\pi^*_{\theta}}(\tb{\ti{s}}) \Big \} \\
 &= \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big\{\sum_{\tb{\ti{s}}^2 \neq \tb{\ti{s}}^1} [\mathbb{P}(\tb{\ti{s}}^2|\tb{\ti{s}}^1,\tb{\ti{a}}^1)-\mathbb{P}(\tb{\ti{s}}^2|\tb{\ti{s}}^1, \tb{\ti{a}}^1^*)] V^{\pi^*_\theta}(\tb{\ti{s}}^2)  \Big \}\\
 &\quad +\mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a^1_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}^1) \Big\}
\end{align}
In the above we used the definition of $Q^{\pi^*_{\theta}}(.,.)$ and Lemma \ref{lemma:general_tp} along with $\tb{\ti{s}}^1 = (s,s,\dots,s)$. \\
Due to intractablility of optimum value function, we cannot exactly simplify the above. The following lemma helps us deal with this problem: 
\begin{lemma}\label{lemma:sum_diff_prob_v}
    For any of our instances as defined in \ref{subsec:problem_instance}, for any state $\tb{\ti{s}} \in \mathcal{S}$ and action $\tb{\ti{a}} \in \mathcal{A}$, we have, $\sum_{\tb{\ti{s}}^\prime \neq \tb{\ti{s}}} [P(\tb{\ti{s}}^\prime|\tb{\ti{s}},\tb{\ti{a}})-P(\tb{\ti{s}}^\prime|\tb{\ti{s}}, \tb{\ti{a}}^*)] V^*(\tb{\ti{s}}^\prime) \geq 0  $
\end{lemma}
Further, by recursion over all the time steps $h$ in this episode and using the monotonicity of $V^*$ established in Theorem \ref{thm:all_in_one}, 
\begin{align}
    R_{\theta,1}  \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{1} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\tb{\ti{s}}_h \neq goal \} \mathbbm{1}\{\sgn(a^h_{i,p}) \neq \sgn(\theta_{i,p})\}
\end{align}
where the expectation is with respect to trajectory induced by the policy $\pi$ and transition kernel $\mathbb{P}_{\theta}$ and $a^h_{i,p}$ denotes the $p^{th}$ component of action taken by agent $i$ at time step $h$. Similar analysis can be generalized for all $K$ episodes. \\
For this purpose, we define,  $N = \sum_{t=1}^{\infty} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} $ and for agent $i \in [n]$, $j \in [d-1]$,\\
$N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\} $  

This is to view the global action as an aggregation of multiple components to track how many times sub-optimal component is chosen similar to \citep{auer2002nonstochastic}.

Thus, the regret over all $K$ episodes can be expressed as, 
\begin{align}
    R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]} \sum_{j=1}^{d-1} N_{i,j}(\theta) \}
\end{align}
Standard Pinsker's Inequality cannot be used directly since $N_{i,j}(\theta)$ can be unbounded similar to arguments in \citep{min2022learning}, \citep{rosenberg2020near}. Hence, we define truncated sums to predefined $T$ to further lower bound $R_{\theta}(K)$ as follows: \\
$N^- = \sum_{t=1}^T\mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} $ and for any agent $i \in [n] $ and $ j \in [d-1],$\\ $N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\} $ \\ 
Thus,  $R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}$
\\
Recall that $\theta = (\theta_1,1,\theta_2,1\dots,\theta_n,1)$. We define for every $\theta \in \Theta$ and every $j \in [d-1]$, $\theta^j$ as the vector that is same as $\theta$ at all components except at $j^{th}$ index of every $\theta_i$ for $i \in [n]$ where it is exactly negative. This allows us to write:
\begin{align} \label{eqn:rthetan}
    2 \sum_{\theta \in \Theta} R_{\theta}(K) \\
    &\geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \{ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \} \\
    &= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}
\end{align}
To simplify the first expectation, we derive a generalisation of Lemma C2 of \citep{rosenberg2020near} as below:
\begin{lemma}\label{lemma:gen_co} If $T \geq 2KV^*_1$, then, $\mathbb{E}_{\theta}[N^-] \geq KV^*_1/4$ for any $\theta \in \Theta$
\end{lemma}
The proof of this lemma requires a tight lower bound on the probability of episode length greater than $V^*_1$. To obtain this, we derive the following general lemma and also use the succeeding corollary: 
\begin{lemma}\label{lemma:episodelength}
     Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$ as the probability that starting at state $\tb{\ti{s}} \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in R^+$. Furthermore, $\mathbb{P}^{\pi}[N_k \geq x] = \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$. \\
    Consider any $\tb{\ti{s}} \in \mathcal{S}(r)$ where $r \in [n]$. Then, for any policy $\pi$, it holds for any instance as defined in (ref) that for any $x \in R^+$
    \begin{align}
        \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}')
    \end{align}
    where $\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})$ with equality holding (for all $x \in R^+$) only at $\pi = \pi^*$  and $r'=r $ (i.e., $\tb{\ti{s}}'=\tb{\ti{s}}$) respectively. \\  Here $\pi^*$ is the policy of taking action $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$ (optimal policy from Theorem \ref{thm:all_in_one}). The equality in the middle indicates that under $\pi^*$ (for any fixed $x \in R^+$), $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ stays constant depending only on $r$ for all $\tb{\ti{s}} \in \mathcal{S}(r)$.
\end{lemma}


\begin{corollary}\label{corollary:pn_x}
    An immediate corollary of the above lemma is that $\mathbb{P}^{\pi^*}[N_k \geq x](r)$ is ordered for any $x \in R^+$ i.e., $\mathbb{P}^{\pi^*}[N_k \geq x](n) \geq \mathbb{P}^{\pi^*}[N_k \geq x](n-1) \geq \cdots \geq \mathbb{P}^{\pi^*}[N_k \geq x](2) \geq \mathbb{P}^{\pi^*}[N_k \geq x](1) \geq \mathbb{P}^{\pi^*}[N_k \geq x](0) =0 $
\end{corollary}
The above helps us deal with the first term in Equation \eqref{eqn:rthetan}. The difference in expectation is dealt with using Lemma E.3 from \citep{min2022learning} which is a standard result using Pinsker's Inequality:
\begin{lemma}\label{lemma:pinsk}
If $f:S^T\xrightarrow{}[0,D]$ then, 
$\mathbb{E}_{\mathbb{P}_1} (f(s)) - \mathbb{E}_{\mathbb{P}_2} (f(s))\leq D \sqrt{\frac{log(2)}{2}}. \sqrt{ \kl(\mathbb{P}_2 || \mathbb{P}_1)}$    
\end{lemma}
Finally, we obtain:
\begin{align}
    2 \sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{\kl(\mathbb{P}_{\theta}||\mathbb{P}_{\theta^{j}})}  \} \Big \}
\end{align}
The simplification of KL-divergence in the multi-agent setting is tricky as there are exponential terms involved due to exponential number of possible next states. The bounding techniques used by \citep{jaksch2010near} and \citep{min2022learning} are not adequate. Hence, we derive the following policy independent upper bound on the KL-divergence term by exploiting the symmetries in our problem instance. 
\begin{lemma}\label{lemma:kl_d}
 For our instances, for any policy $\pi $, any $ j \in [d-1]$, $\kl(\mathbb{P}_{\theta} || \mathbb{P}_{\theta^j}) \leq 3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]$ 
\end{lemma}
Using the above lemma, upper bounding $\mathbb{E}_{\theta}[N^-]$ by $T$ and taking $T = 2KV^*_1$, we obtain:
\begin{align}
    \frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq   V_1^*  \Big \{ \Delta  KV_1^*/4 -   (KV_1^*)^{3/2}  \frac{2^{n+2}.\Delta^2}{\sqrt{\delta} (d-1)} \Big \} 
\end{align}  
Finally, picking $\Delta^* = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}$,  ensures we have: \\
$\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{(d-1).\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+8}} \geq \frac{d.\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+9}}$. \\
Since the average of regrets over a set of instances is lower bounded by the RHS, there must exist atleast one instance for whom RHS is a lower bound. \\
But the chosen $\Delta$ must be valid i.e., $\Delta^* < 2^{-n} \cdot\frac{1-2\delta}{1+n+n^2}$. This provides a sample complexity on $K$ as $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.\{\frac{1-2\delta}{1+n+n^2}\}^2} $ where $V^*_1 = \frac{2n}{n-1+2(\delta+\Delta)}$

\end{proof}



\section{Our Approach}
\label{sec:approach}
% 
In this section, we present our approach for establishing regret lower bounds in the LM-MASSP framework.
To this end, we construct a family of LM-MASSP instances that are provably hard to learn. These instances are designed so that the optimal policy is analytically tractable, and any deviation from it incurs a quantifiable regret.

\pt{I am thinking to modify the entire section  as follows - let me know if this makes sense - define each component of the (V, S, A, P) -- While defining the transition probability -- we can give the feature design -- and then define the cost -- and the remark therein -- write the instance defintion -- because now we have all the terms defined. Then i think, we can make the sub-section where we give the lemma 2 -- etc. and while writing the lemma 2, we should define the sets Sr, I, J, etc.... This implies there will not be subsection called Features. Rather we have another subsection. }


\subsection{Construction of Hard-to-Learn LM-MASSP Instances}
\label{subsec:problem_instance}
% 
We consider a minimal yet expressive network with only two nodes: $\mathcal{V} = \{s, g \}$. This induces a global state space $\mathcal{S} = \{ s, g \}^n$ of size $|\mathcal{S}| = 2^n$, where each agent resides at either $s$ or $g$. 
We fix the initial state as $\tb{\ti{s}}_{\init} = (s, s, \dots, s)$ and the goal state as $\tb{g} = (g, g, \dots, g)$. Each agent $i \in [n]$ has the same action set $\mathcal{A}_i = \{-1, 1\}^{d-1}$, for some $d \geq 2$. 
Consequently, the global action space is $\mathcal{A} = \{-1, 1\}^{n(d-1)}$ with $|\mathcal{A}| = 2^{n(d-1)}$. To simplify the dynamics, we assume that once an agent reaches node $g$, it remains there permanently. 
That is, transitions such as $\tb{\ti{s}} = (s, s, \dots, g, g) \rightarrow \tb{\ti{s}}' = (s, s, \dots, g, s)$ are infeasible.



Further, we partition the state space $\mathcal{S}$ depending on the number of agents that are at the node $s$. 
Let $\mathcal{S}_r$ be the subset of the state space for which the number of agents at $s$ are $r$, i.e.,
\begin{align}
    \mathcal{S}_r \coloneqq \Big\{s \in \mathcal{S} : \sum_{i\in \mathbb{N}} \mathbbm{1}_{\{s_i = s\}} = r \Big\}.
\end{align}
For any $r \in \{0\} \cup [n]$, we say that a state $\tb{\ti{s}}$ is of \emph{type} $r$ if $\tb{\ti{s}} \in \mathcal{S}_r$. 
It is easy to observe that the $\cup_{r=0}^n \mathcal{S}_r = \mathcal{S}$, and $\mathcal{S}_{r_1} \cap \mathcal{S}_{r_2} = \emptyset$ for any $r_1 \neq  r_2$. Thus,  $\{ \mathcal{S}_0, \mathcal{S}_1, \dots, \mathcal{S}_n \}$ partitions $\mathcal{S}$. Moreover, for any state $\tb{\ti{s}}$, we define the set $\mathcal{S}(\tb{\ti{s}}) \coloneqq \{ \tb{\ti{s}}' \in \mathcal{S} : \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) >0, ~~ \text{for some}~ \tb{\ti{a}} \in \mathcal{A} \})$ as the set of all the states that are \emph{reachable} in the next step from $\tb{\ti{s}}$.
Further, we define the set $\mathcal{S}_r(\tb{\ti{s}})$ as the set of all the states of \emph{type} $r$ that are \emph{reachable} in the next step i.e., $\mathcal{S}_r(\tb{\ti{s}}) \coloneqq \{ \tb{\ti{s}}' \in \mathcal{S}_r : \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}) >0, ~~ \text{for some} ~ \tb{\ti{a}} \in \mathcal{A} \}$.






To analyze any transition, say $\tb{\tb{s}} \rightarrow \tb{\ti{s}}'$ where $\tb{\ti{s}} \in \mathcal{S}_r$ and $\tb{\ti{s}}' \in \mathcal{S}_{r'}$,  we define context dependent sets of agents - $\mathcal{I}\coloneqq\{i_1,i_2,\dots,i_r\}$ as the set of agents at node $s$ in state $\tb{\ti{s}}$, $\mathcal{J} \coloneqq \{j_1,j_2,\dots,j_{n-r}\}$ as the set of agents already at node $g$ in state $\tb{\ti{s}}$ and $\mathcal{T} \coloneqq \{t_1,t_2,\dots, t_{r-r'}\} \subseteq\mathcal{I}$ as the set of agents that move from node $s$ to node $g$ as the global state of the system changes from $\tb{\ti{s}}$ to $\tb{\ti{s}}'$. Note that we say these are context-dependent since $\mathcal{I}, \mathcal{J}$ varies for various $\tb{\ti{s}}$ and $\mathcal{T}$ varies for various $\tb{\ti{s}}, \tb{\ti{s}}'$. Thus we are abusing the notation here a little to avoid notational overhead and the sets must more precisely be denoted as $\mathcal{I}_{\tb{\ti{s}}}, \mathcal{J_{\tb{\ti{s}}'}}$ and $\mathcal{T}_{\tb{\ti{s}}, \tb{\ti{s}}'}$.


% \pt{partitioning of the state space- -- we partition the state space based on r, the number of agents at the state s. $\mathcal{S}_r$ -- of type r... $\mathcal{S}(s)$ -- reachable from $s$. $\mathcal{S}_r(s)$ -- reachable from s of type r. }

\pt{The following instance is defined here, without telling what $\delta, \Delta$ are defined. Not a good idea to use this notation without telling anything about it.} Any of our instance is uniquely represented by a fixed tuple $(n,\delta, \Delta, \theta)$ where $n \geq 1$ is the number of agents, $ \delta \in \left( \frac{2}{5} , \frac{1}{2} \right)$ and $\Delta < 2^{-n} \cdot \frac{1-2\delta}{1+n+n^2}$ are parameters of the features described in the next section and $\theta$ is an $nd$- dimensional vector of the form $\theta = (\theta_1,1, \theta_2,1,\dots,\theta_n,1) \in \Theta$ used to define the transition probability as in Assumption \ref{assm:lfa_prob}, where for each agent $i \in [n]$, the paramter $\theta_i$ is a $(d-1)$ dimensional vector each of whose component takes one of the two values $\left\{-\frac{\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)} \right\}$. For convenience, we will also  use $\widetilde{\theta} = (\theta_1,\theta_2,\dots,\theta_n)$ wherever required.

\begin{remark}
For a general cost and transition probability function, there may in general be a trade-off between policies that moves towards the goal state quickly (i.e.,  minimizing the number of time steps to reach the goal) and the policies that take more time but may (in an overall sense) be cost efficient \citep{tarbouriech2020no}. 
\end{remark}

Such complications lead to intractability of optimal policies. To avoid this in the analysis of our instances, we let for all $\tb{\ti{s}} \in \mathcal{S}\backslash\{\tb{\ti{g}}\}$ and $\tb{\ti{a}} \in \mathcal{A}$, $c(\tb{\ti{s}},\tb{\ti{a}}) = 1$ while for any $\tb{a} \in \mathcal{A}, c(\tb{\ti{g}}, \tb{\ti{a}}) =0$. Hence, the policy that takes us \emph{closer} to goal state is better. This leads to optimal policy being directly influenced by transition probabilities alone.

To convince that we are not considering impossible instances, we have the following:
\begin{remark} \label{rem:cost_one}
    One class of such instances is the one for whom for all $i \in [n], \tb{\ti{a}} \in \mathcal{A}, K^i(\tb{\ti{s}},\tb{\ti{a}}) = \frac{1}{x_i(\tb{\ti{s}},\tb{\ti{a}})}$ for all $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$ and $ K^i(\tb{\ti{g}},\tb{\ti{a}}) = 0$ in Equation \eqref{eqn:ind_cost}. 
\end{remark}
\subsection{Feature Design} 
\label{subsec:features}


For the type of instances mentioned in the previous subsection, we now provide valid features for the transition probability model considered in Assumption \ref{assm:lfa_prob}.


Note that there can be many possible feature designs, but all of them must satisfy the following requirements to produce valid transition probabilities in any of our instances.

\begin{requirements}
    For any $(\tb{\ti{s}},\tb{\ti{a}},\tb{\ti{s}}') \in \mathcal{S}\times\mathcal{A}\times\mathcal{S}$, and 
    $\theta\in \Theta$, the parametrized transition probability satisfies $\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}) = \left<  \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}), \theta \right> \geq 0$, and for any $(\tb{\ti{s}},\tb{\ti{a}}) \in \mathcal{S}\times \mathcal{A}$, $\sum_{\tb{\ti{s}}' \in \mathcal{S}}\mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}) = \sum_{\tb{\ti{s}}' \in \mathcal{S}} \left < \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}), \theta \right> = 1$. \label{reqm:1}
\end{requirements}
\begin{requirements}
   If there is a physically impossible transition to some $\tb{\ti{s}}' \in \mathcal{S}$ from some $\tb{\ti{s}} \in \mathcal{S}$, under action $\tb{\ti{a}} \in \mathcal{A}$, then $ \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}) = \left< \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}), \theta \right> = 0$, and if there's a certain transition to some $\tb{\ti{s}}' \in \mathcal{S}$ from some $\tb{\ti{s}} \in \mathcal{S}$ under action $\tb{\ti{a}} \in \mathcal{A}$, then $ \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}}, \tb{\ti{a}}) = \left< \phi(\tb{\ti{s}}'|\tb{\ti{s}},\tb{\ti{a}}), \theta \right> = 1$. \label{reqm:2}
\end{requirements}
% 
For our instances, we consider the following feature design
% 
\begin{equation}
\label{eqn:features_global_new}
    \phi(\tb{\ti{s}}' \mid \tb{\ti{s}}, \tb{\ti{a}}) = 
    \begin{cases} 
    \left(\phi_1(s'_1|s_1,a_1),\dots, \phi_n(s'_n|s_n,a_n) \right), & \text{if } \tb{\ti{s}} \neq \tb{\ti{g}} \text{ and } s^{\prime}_i = g \text{ if } s_i = g,~ \forall~ i \in [n] \\
    \mathbf{0}_{nd}, & \text{if } \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}' \neq \tb{\ti{g}}, \text{ or } \tb{\ti{s}} \neq \tb{\ti{g}},~ \exists ~ i \in [n] \text{ s.t. } s_i = g,~ s^{\prime}_i = s \\
    (\mathbf{0}_{nd-1}, 1), & \text{if } \tb{\ti{s}} = \tb{\ti{g}},~ \tb{\ti{s}}' = \tb{\ti{g}}
    \end{cases}
\end{equation}
where
\begin{equation}
\label{eqn:individual_features}
    \phi_i(s^{\prime}_i | s_i, {{a}}_i) = \begin{cases}  
    \left(-{{a}}_i, \frac{1-\delta}{n 2^{r-1}} \right)^{\top}, & \text{if} ~ {s}^i = s^{\prime}_{i} = s
    \\
    \left({{a}}_i, \frac{\delta}{n 2^{r-1}} \right)^{\top}, & \text{if} ~ {s}_i = s,~s^{\prime}_{i} = g
    \\
    \left(\mathbf{0}_{d-1}, \frac{1}{n 2^{r}} \right)^{\top}, & \text{if} ~ {s}_i = g,~ s^{\prime}_{i} = g
    \end{cases}
\end{equation}
% 
In the above, $r$ represents the number of agents at node $s$ in the current global state $\tb{\ti{s}}$.  
%
Observe that in Equation \eqref{eqn:features_global_new} the first case corresponds to the most general transitions that are allowed, the second case represents all impossible transitions and the third case takes care of the only \textit{certain} transition.

\begin{lemma}\label{lemma:valid_features}
    Features defined above in Equations \eqref{eqn:features_global_new} and \eqref{eqn:individual_features}, produce valid transition probabilities for any instance $(n,\delta,\Delta,\theta)$ as defined in \ref{subsec:problem_instance}. Specifically they satisfy both requirements \ref{reqm:1} and \ref{reqm:2}.
\end{lemma}
 The detailed proof is deferred to Appendix \ref{proof:lemma:valid_features}.

Using the above features and transition probability model in Assumption \ref{assm:lfa_prob}, we derive a general expression for the probability of any valid transition for any instance $(n, \delta, \Delta, \theta)$ as defined in Section \ref{subsec:problem_instance}. 

\textcolor{red}{the below lemma statement will simplify depending on if these definitions are incorporated in Section \ref{subsec:prelims}}
% 
\begin{lemma}
\label{lemma:general_tp} 
Consider any state $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$. In this state $\tb{\ti{s}}$, let $\mathcal{I}:=\{i_1,i_2,\dots,i_{r}\}$ denote the set of agents at node $s$ and $\mathcal{J}:=\{j_1,j_2,\dots,j_{n-r}\}$ be those at node $g$. 
Under a valid transition, either the next state is the same as $\tb{\ti{s}}$ or possibly some agents from $\mathcal{I}$ transit to node $g$. Let the set of all valid next states from $\tb{\ti{s}}$ be denoted as $\mathcal{S}(\tb{\ti{s}})$. To study a particular transition to $\tb{\ti{s}}'\in \mathcal{S}(\tb{\ti{s}})$, we define $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ as the set of all agents moving from node $s$ to node $g$. Here, $r'$ denotes the number of agents in state $\tb{\ti{s}}'$ that are at node $s$. For any action $\tb{\ti{a}} \in \mathcal{A}$, the transition probability is given as: 
\begin{align}
    &p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'} = 
 \mathbb{P}(\tb{\ti{s}}^\prime | \tb{\ti{s}}, \tb{\ti{a}}) 
=\frac{r' + (r-2r')\delta}{n \cdot 2^{r-1}} +   \frac{n-r}{n \cdot 2^r}        +    \frac{\Delta}{n}  (r-2r') \\
&\quad + \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn({{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn({{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}
\end{align} 
\end{lemma}


% \pt{The following corollary provides the probability when action are as in Theorem 1. This probability only depends on $r$ and $r'$ only. i am thinking to remove this corollary and put it as the another statement in the above lemma.
% } \textcolor{red}{i dont mind. can we decide upon these things after doing one round of appendix?}


\begin{corollary} \label{corollary:p_star}
From Lemma \ref{lemma:general_tp}, we observe that for any given instance $(n, \delta, \Delta, \theta)$ if the action chosen is such that the indicators vanish in the above expression, the transition probability doesn't depend on $\mathcal{I}$ and $\mathcal{T}$ and only depends on $r$ and $r'$. Hence, we define this special global action $\tb{\ti{a}}_{\theta}$ as the action whose $\{(d-1)\times (i-1)+j\}-th$ element for every $i \in [n]$ and every $j \in [d-1]$ is given by $\sgn(\theta_{i,j})$. In other words,  $\tb{\ti{a}}_{\theta} = \frac{n(d-1)}{\Delta} \times \widetilde{\theta}$. We will denote the associated probabilities as $p^*_{r,r'}$
\end{corollary}

The proof of this lemma is deferred to the Appendix ??. \pt{This will be a common lemma with its sub-part as corollary.}

Next, we would like to highlight why the above described instances are considered and their importance. In particular, we will provide the details on why the instances are hard, and why they one would expect a good/ sub-linear lower bound on the regret.
\textcolor{red}{again no need for this}

\subsection{Summary of Our Approach}
\label{subsec:why_hard_instance}
% 
\pt{I haven't looked at this part as of now.}

Any deterministic algorithm produces, in general, a history-dependent policy. Fixing any such policy $\pi$, we will analyze the regret of this policy on a set of hard to learn instances that differ only due to $\theta$ (i.e., have same parameters $n, \delta, \Delta$) and show that there exists an instance in the set of hard-to-learn instances that achieves lower bound on expected cumulative regret that scales similarly in terms of number of episodes as the upper bound $\widetilde{O}(\sqrt{K})$ reported by \citep{trivedi2023massp}. 
Intuitively, there are two reasons why we expect at least one of the instances in this set to be very hard to be learnt for any given policy:
\begin{itemize}
    \item Firstly, all the instances are characterized by the optimum policy that at any state, the action taken is $\tb{a}_{\theta}$. If we consider a policy such that the action taken in only one of the $2^n-1$ non-goal states differed from $a_{\theta}$ at just one of the $n(d-1)$ indices, then the transition probabilities would differ (from those for optimal policy) only very slightly since $\Delta$ is quite small $(<2^{-n})$. 
Hence, the value function for that policy would be only slightly higher. Observe that there would be $n(d-1).2^{n-1}$ (significant) number of such policies. The policies that differ in the above fashion at any two states are even larger in number and can't be expected to be too worse in terms of the expected cumulative cost for similar reason. Hence, separating these large number of policies efficiently is a challenge before any MASSP learning algorithm. 
\item Secondly, any learning algorithm that efficiently learns the best policy for one instance in the set of all instances, may not be able to efficiently learn some other instance in the set. Also, if a particular action is the best (optimal) for a given instance $\theta = (\theta_1,1,\theta_2,1,\dots,\theta_n,1)$, there definitely exists another instance $\theta = (-\theta_1,1,-\theta_2,1,\dots,-\theta_n,1) \in \Theta$ for whom the same action is the worst.
\end{itemize}
In the following section, we present our observations on these instances and key results that follow.




\pt{We would like to highlight the importance of the instance that we constructed. we would like to highlight why the above described instances are considered and their importance. In particular, we will provide the details on why the instances are hard, and why they one would expect a good/ sub-linear lower bound on the regret.}

% 
\pt{I haven't looked at this part as of now.}

Any deterministic algorithm produces, in general, a history-dependent policy. Fixing any such policy $\pi$, we will analyze the regret of this policy on a set of hard to learn instances that differ only due to $\theta$ (i.e., have same parameters $n, \delta, \Delta$) and show that there exists an instance in the set of hard-to-learn instances that achieves lower bound on expected cumulative regret that scales similarly in terms of number of episodes as the upper bound $\widetilde{O}(\sqrt{K})$ reported by \citep{trivedi2023massp}. 
Intuitively, there are two reasons why we expect at least one of the instances in this set to be very hard to be learnt for any given policy:
\begin{itemize}
    \item Firstly, all the instances are characterized by the optimum policy that at any state, the action taken is $\tb{a}_{\theta}$. If we consider a policy such that the action taken in only one of the $2^n-1$ non-goal states differed from $a_{\theta}$ at just one of the $n(d-1)$ indices, then the transition probabilities would differ (from those for optimal policy) only very slightly since $\Delta$ is quite small $(<2^{-n})$. 
Hence, the value function for that policy would be only slightly higher. Observe that there would be $n(d-1).2^{n-1}$ (significant) number of such policies. The policies that differ in the above fashion at any two states are even larger in number and can't be expected to be too worse in terms of the expected cumulative cost for similar reason. Hence, separating these large number of policies efficiently is a challenge before any MASSP learning algorithm. 
\item Secondly, any learning algorithm that efficiently learns the best policy for one instance in the set of all instances, may not be able to efficiently learn some other instance in the set. Also, if a particular action is the best (optimal) for a given instance $\theta = (\theta_1,1,\theta_2,1,\dots,\theta_n,1)$, there definitely exists another instance $\theta = (-\theta_1,1,-\theta_2,1,\dots,-\theta_n,1) \in \Theta$ for whom the same action is the worst.
\end{itemize}
In the following section, we present our observations on these instances and key results that follow.


\begin{lemma}
\label{lemma:general_tp} 
Consider any state $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$. In this state $\tb{\ti{s}}$, let $\mathcal{I}:=\{i_1,i_2,\dots,i_{r}\}$ denote the set of agents at node $s$ and $\mathcal{J}:=\{j_1,j_2,\dots,j_{n-r}\}$ be those at node $g$. 
Under a valid transition, either the next state is the same as $\tb{\ti{s}}$ or possibly some agents from $\mathcal{I}$ transit to node $g$. Let the set of all valid next states from $\tb{\ti{s}}$ be denoted as $\mathcal{S}(\tb{\ti{s}})$. To study a particular transition to $\tb{\ti{s}}'\in \mathcal{S}(\tb{\ti{s}})$, we define $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ as the set of all agents moving from node $s$ to node $g$. Here, $r'$ denotes the number of agents in state $\tb{\ti{s}}'$ that are at node $s$. For any action $\tb{\ti{a}} \in \mathcal{A}$, the transition probability is given as: 
\begin{align}
    &p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'} = 
 \mathbb{P}(\tb{\ti{s}}^\prime | \tb{\ti{s}}, \tb{\ti{a}}) 
=\frac{r' + (r-2r')\delta}{n \cdot 2^{r-1}} +   \frac{n-r}{n \cdot 2^r}        +    \frac{\Delta}{n}  (r-2r') \\
&\quad + \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn({{a}}_{i,p}) \neq \sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn({{a}}_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}
\end{align} 
\end{lemma}



\section{Proof Outline}
\label{sec:proof_outline}

\subsection{Proof Sketch of Theorem \ref{thm:all_in_one}}

\begin{proof} 
% 
The proof uses the principle of Mathematical induction over $r$, that represents the number of agents present at node $s$ in any state $\tb{\ti{s}} \in \mathcal{S}$. In particular, all  the three claims in this theorem are proved together in a single induction argument over $r$. Note that for $r=0$, by definition costs for all actions are $0$ and $V^*=0$. All the three claims hold trivially. Hence, we take $r=1$ as base case in the induction for generalizability.  


\textbf{Base case.} For any state $\tb{\ti{s}} \in \mathcal{S}_1$, the only possible next states are either same state $\tb{\ti{s}}$ or $\tb{\ti{g}}= (g,\dots,g)$. For any action $\tb{    \ti{a}} \in \mathcal{A}$ in this state $\tb{\ti{s}}$, by  standard arguments we can express the value function for any policy $\pi_{\tb{\ti{a}}}$ of choosing action $\tb{\ti{a}}$ at $\tb{\ti{s}}$ as $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}}) = \frac{1}{1-p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}}}$, where $p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}}$ represents the probability of transition from $\tb{\ti{s}}$ to $\tb{\ti{s}}$ itself under action $\tb{\ti{a}}$.
The following corollary
helps us establish that at action $ \tb{\ti{a}} = \tb{\ti{a}}_{\theta}$, $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$ is minimum and thus is the optimal action at $\tb{\ti{s}}$.

\begin{corollary}\label{corollary:ps_s}
From Lemma \ref{lemma:general_tp}, from any state $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$, for any action $\tb{\ti{a}} \in \mathcal{A}$, the probability that the next state is also $\tb{\ti{s}}$ is: 
\begin{align}
    \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}}) = \frac{r(1-\delta)}{n \cdot 2^{r-1}}+\frac{n-r}{n.2^r}-r.\frac{\Delta}{n} + \frac{2\Delta}{n(d-1)}\sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \mathbbm{1}\{\sgn({{a}}_{i,p})\neq \sgn(\theta_{i,p})\}
\end{align}
% 
Further, for any $\tb{\ti{s}} \in \mathcal{S}\backslash\tb{\ti{g}}$, $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})$ is minimum at $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$ where it is only dependent on $r$ for a given instance (independent of $\mathcal{I}$).
\end{corollary}
% 
Note that the above arguments follow for any $\tb{\ti{s}} \in \mathcal{S}_1$. Also, due to the above corollary, the value is same too. Thus, the second claim holds. As, $V^*_1 > 0$, third claim holds too. This completes the proof for the base case.

\textbf{Inductive Step.} Let us assume that all the three claims of the theorem hold for every $r \in \{1,2, \dots, k\}$, and use this to show that all these claims hold for $r=k+1$ in the same order. 
To this end, consider any $\tb{\ti{s}} \in \mathcal{S}_{k+1}$. To prove the first claim, i.e., $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$ we again derive expression for value function $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$ for any policy $\pi_{\tb{\ti{a}}}$ that chooses action $\tb{\ti{a}}$ at state $\tb{\ti{s}}$ and optimal action $\tb{\ti{a}}_{\theta}$ at all the other reachable states from $\tb{\ti{s}}$.  
Note that so far we know the optimal actions at only the states in $\cup_{i \in [k]}\mathcal{S}_i$. 
If along any sample path starting from this $\tb{\ti{s}}$, we reached, with any positive probability, any state not in $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}_i$, it would be impossible to evaluate $V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$. 
Fortunately, for our setting all the \textit{reachable} states from $\tb{\ti{s}}$ lie in $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}_i$ i.e., $ \cup_{i \in [k] \cup \{0\}}\mathcal{S}_i(\tb{\ti{s}}) \subseteq \cup_{i \in [k] \cup \{0\}}\mathcal{S}_i$. 
The state value function in this case can be expressed appropriately as 
\begin{align}
    V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}}) = 1+\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\tb{\ti{a}})V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})+\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}})V^*(\tb{g}) +\sum_{r' \in [k]} \sum_{\tb{\ti{s}}' \in \mathcal{S}_{r'}(\tb{\ti{s}})} p^{\tb{\ti{a}}}_{\tb{\ti{s}},\tb{\ti{s}}'}V^*_{r'}. 
\end{align}
% 
Using the partition of state space based on number of agents at node $s$, identifying that the indicator has positive coefficient if any agent in $\mathcal{I}$ moves from $s$ to $g$ or negative if it stays at $s$, and using the above induction assumptions, \textcolor{red}{through some clever mathematical manipulations} we show that $ V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$ is minimized for any $\tb{\ti{s}} \in \mathcal{S}_{k+1}$ at $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$. \pt{Let us write the exact result/eqn that we use to prove this.}
% 
This again requires using Corollary \ref{corollary:ps_s}. Corollary \ref{corollary:p_star} ensures the second claim holds. Finally to prove that claim 3 holds for our case, we first show that the following lemma holds for all the instances that we consider. 
\begin{lemma}
\label{claim:probability_inequality}
    For all our instances,  for every $r \in [n-1]$, it holds that, for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$. 
\end{lemma}
The existence of the above property for all our instances helps us use the following lemma to show $V^*_{k+1}>V^*_k$. 
\begin{lemma}\label{lemma:probability_inequality}
    If for any $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.
\end{lemma}
This proves the final claim for $r=k+1$. Thus, using the Principle of Mathematical induction it holds for every $r = \{0,1,\dots, n\}$.
This completes the proof.
\end{proof}


\subsection{Proof Sketch of Theorem \ref{thm:lower_bound}}

\begin{proof}
% 
\pt{These few sentences can also be repeated in the appendix. Moreover, we can write is very precisely, not this much detailed.} The proof uses similar techniques as the one for single agent SSP in \cite{min2022learning} and for a two state RL setting by  \cite{jaksch2010near}. But extension to MASSP setting poses many technical challenges such as design of novel features that satisfy the requirements \ref{reqm:1} and \ref{reqm:2}, constructing instance generalizable for any number of agents $n$ with tractable optimal policy, inability to express optimal value function in tractable closed form due to exponentially large number of states, obtaining a reasonably tight upper bound on KL divergence, etc. Some of these challenges are addressed by Theorem \ref{thm:all_in_one}. Others, we deal here. 

Consider any history-dependent deterministic policy $\pi$ \pt{We have a notation for this, $\pi \in \Pi_{\mathrm{HD}}$ ?} and the set of instances parametrized by fixing $n \geq 1$, $\delta \in (2/5,1/2)$, and $\Delta < 2^{-n} \cdot \frac{1-2\delta}{1+n+n^2}$ \pt{the detail of $\theta$ is not clear here. It is part of instance, but how they are differing -- do you mean to say that the instances are differing in $\theta$?}  and differing only due to $\theta \in \Theta$.

Suppose agents take actions according to this policy $\pi$. Let, $\tb{\ti{s}}^t$ represent the global state and $\tb{\ti{a}}^t$ the global action at time $t$. Then, the expected regret for the first episode for this instance is
% 
\begin{align}
    R_{\theta,1} 
    &= V^{\pi}(\tb{\ti{s}}^1) - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) 
    \\
    &= \mathbb{E}_{\tb{\ti{a}}^1 \sim\ \pi(\tb{\ti{s}}^1), \tb{\ti{s}}^2 \sim\ \mathbb{P}(.|\tb{\ti{s}}^1,\tb{\ti{a}}^1)}[V^{\pi}(\tb{\ti{s}}^2) - V^{\pi^*_{\theta}}(\tb{\ti{s}}^2)] + \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)}[Q^{\pi^*_{\theta}}(\tb{\ti{s}}^1,\tb{\ti{a}}^1)] - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) 
\end{align} 
The first term indicates a recurrence relationship. The second term can further written as follows:
\begin{align}
    & \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)}[Q^{\pi^*_{\theta}}(\tb{\ti{s}}^1,\tb{\ti{a}}^1)] - V^{\pi^*_{\theta}}(\tb{\ti{s}}^1) 
    \\
    &=\mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big \{ \sum_{\tb{\ti{s}} \in \mathcal{S}} [\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}}^1, \tb{\ti{a}}^1) - \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}}^1, \tb{\ti{a}}^{1^*})] V^{\pi^*_{\theta}}(\tb{\ti{s}}) \Big \} 
    \\
    &= \mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big\{\sum_{\tb{\ti{s}}^2 \neq \tb{\ti{s}}^1} [\mathbb{P}(\tb{\ti{s}}^2|\tb{\ti{s}}^1,\tb{\ti{a}}^1)-\mathbb{P}(\tb{\ti{s}}^2|\tb{\ti{s}}^1, \tb{\ti{a}}^1{^*})] V^{\pi^*_\theta}(\tb{\ti{s}}^2)  \Big \}
    \\
    &\quad +\mathbb{E}_{\tb{\ti{a}}^1 \sim \pi(\tb{\ti{s}}^1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\sgn(a^1_{i,p}) \neq \sgn(\theta_{i,p})\}V^*(\tb{\ti{s}}^1) \Big\}
\end{align}
In the above we used the definition of $Q^{\pi^*_{\theta}}(\cdot, \cdot)$ and Lemma \ref{lemma:general_tp} along with $\tb{\ti{s}}^1 = (s,s,\dots,s)$.  
However, due to intractablility of optimum value function, we cannot exactly simplify the above. To handle this problem we have the following lemma
% 
\begin{lemma}
\label{lemma:sum_diff_prob_v}
    For any of our instances as defined in Section \ref{subsec:problem_instance}, for any state $\tb{\ti{s}} \in \mathcal{S}$ and action $\tb{\ti{a}} \in \mathcal{A}$, we have, $\sum_{\tb{\ti{s}}^\prime \neq \tb{\ti{s}}} [P(\tb{\ti{s}}^\prime|\tb{\ti{s}},\tb{\ti{a}})-P(\tb{\ti{s}}^\prime|\tb{\ti{s}}, \tb{\ti{a}}^*)] V^*(\tb{\ti{s}}^\prime) \geq 0  $
\end{lemma}
% 
Further, by recursion over all the time steps $h$ in this episode and using the monotonicity of $V^*$ established in Theorem \ref{thm:all_in_one} to lower bound the $V^*$ for each non-goal state in the sum, we have that
% 
\begin{align}
    R_{\theta,1}  \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{1} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{\tb{\ti{s}}^h \neq goal \} \mathbbm{1}\{\sgn(a^h_{i,p}) \neq \sgn(\theta_{i,p})\}.
\end{align}
% 
where the expectation is with respect to trajectory induced by the policy $\pi$ and transition kernel $\mathbb{P}_{\theta}$ and $a^h_{i,p}$ denotes the $p^{th}$ component of action taken by agent $i$ at time step $h$.
Similar analysis can be generalized for all $K$ episodes \pt{is this generalization given below?}

For this purpose, we define
$N \coloneqq \sum_{t=1}^{\infty} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\}$, 
and for agent $i \in [n]$, $j \in [d-1]$, we define \pt{write one line description of this notation in plain english. -- This is to view the global action as an aggregation of multiple components to track how many times sub-optimal component is chosen similar to \citep{auer2002nonstochastic}.}
\begin{align}
\label{eqn:N_ij_definition}
    N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\}.
\end{align}
% 
Thus, the regret over all $K$ episodes can be expressed as, 
\begin{align}
    R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]} \sum_{j=1}^{d-1} N_{i,j}(\theta) \}
\end{align}
It is important to note that we can't use the standard Pinsker's inequality here to bound the regret, as $N_{i,j}(\theta)$ can be unbounded. This is along with the similar line to the arguments used in \citep{min2022learning,rosenberg2020near}. 
To further lower bound $R_{\theta}(K)$, we define the truncated sums upto a predefined $T$ as: $N^- = \sum_{t=1}^T\mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\}$, 
and for any agent $i \in [n] $ and $ j \in [d-1]$, we have that
% 
\begin{align}
\label{eqn:N_ij_truncated}
    N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{\tb{\ti{s}}^t \neq \goal\} \mathbbm{1}\{\sgn(a^t_{i,j}) \neq \sgn(\theta_{i,j})\} 
\end{align}
% 
Thus, the regret upto $K$ episode is bounded as
% 
\begin{align}
    R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \left[ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \right]
\end{align}
% 
Now, recall that $\theta = (\theta_1,1,\theta_2,1\dots,\theta_n,1)$. We define for every $\theta \in \Theta$ and every $j \in [d-1]$, $\theta^j$ as the vector that is same as $\theta$ at all components except at $j^{th}$ index of every $\theta_i$ for any $i \in [n]$ where it is exactly negative. This allows us to write
% 
\begin{align} 
\label{eqn:rthetan}
    2 \sum_{\theta \in \Theta} R_{\theta}(K) 
    &\geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \left[ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \right] 
    \\
    &= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \left[  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \right]
\end{align}
To simplify the first expectation, we generalization the Lemma C2 of \citep{rosenberg2020near} as below
% 
\begin{lemma}
\label{lemma:gen_co} 
    If $T \geq 2KV^*_1$, then, $\mathbb{E}_{\theta}[N^-] \geq KV^*_1/4$ for any $\theta \in \Theta$
\end{lemma}
% 
the detailed proof of this lemma is  deferred to Appendix??. The proof of this lemma requires a tight lower bound on the probability of episode length greater than $V^*_1$. To this, we derive the following general lemma and also use the succeeding corollary
\begin{lemma}\label{lemma:episodelength}
     Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$ as the probability that starting at state $\tb{\ti{s}} \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in \mathbb{R}^+$. Furthermore, $\mathbb{P}^{\pi}[N_k \geq x] = \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$. \\
    Consider any $\tb{\ti{s}} \in \mathcal{S}(r)$ where $r \in [n]$. Then, for any policy $\pi$, it holds for any instance as defined in (ref) that for any $x \in R^+$
    \begin{align}
        \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}')
    \end{align}
    where $\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})$ with equality holding (for all $x \in R^+$) only at $\pi = \pi^*$  and $r'=r $ (i.e., $\tb{\ti{s}}'=\tb{\ti{s}}$) respectively. \\  Here $\pi^*$ is the policy of taking action $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$ (optimal policy from Theorem \ref{thm:all_in_one}). The equality in the middle indicates that under $\pi^*$ (for any fixed $x \in R^+$), $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ stays constant depending only on $r$ for all $\tb{\ti{s}} \in \mathcal{S}(r)$.
\end{lemma}


\begin{corollary}\label{corollary:pn_x}
    An immediate corollary of the above lemma is that $\mathbb{P}^{\pi^*}[N_k \geq x](r)$ is ordered for any $x \in R^+$ i.e., $\mathbb{P}^{\pi^*}[N_k \geq x](n) \geq \mathbb{P}^{\pi^*}[N_k \geq x](n-1) \geq \cdots \geq \mathbb{P}^{\pi^*}[N_k \geq x](2) \geq \mathbb{P}^{\pi^*}[N_k \geq x](1) \geq \mathbb{P}^{\pi^*}[N_k \geq x](0) =0 $
\end{corollary}
The above \pt{corollary or lemma} helps us deal with the first term in Equation \eqref{eqn:rthetan}. The difference in expectation is dealt with using Lemma E.3 from \citep{min2022learning} which is a standard result using the following Pinsker's inequality 
% 
\begin{lemma}
\label{lemma:pinsk}
    If $f:S^T\xrightarrow{}[0,D]$ then, 
    $\mathbb{E}_{\mathbb{P}_1} (f(s)) - \mathbb{E}_{\mathbb{P}_2} (f(s))\leq D \sqrt{\frac{log(2)}{2}}. \sqrt{ \kl(\mathbb{P}_2 || \mathbb{P}_1)}$    
\end{lemma}
% 
Using these results, we obtain
% 
\begin{align}
    2 \sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{\kl(\mathbb{P}_{\theta}||\mathbb{P}_{\theta^{j}})}  \} \Big \}
\end{align}
The simplification of KL-divergence in the multi-agent setting is tricky as there are exponential terms involved due to exponential number of possible next states.
\pt{Need to write this with more details, because this is the novelty part of the proof.} The bounding techniques used by \citep{jaksch2010near} and \citep{min2022learning} are not adequate. Hence, we derive the following policy independent upper bound on the KL-divergence term by exploiting the symmetries in our problem instance. 
% 
\begin{lemma}
\label{lemma:kl_d}
    For our instances and for any policy $\pi $, any $ j \in [d-1]$, we have
    \begin{align}
        \kl(\mathbb{P}_{\theta} || \mathbb{P}_{\theta^j}) \leq 3 \cdot 2^{2n} \cdot \frac{\Delta^2}{\delta (d-1)^2} \cdot \mathbb{E}_{\theta}[N^-].
    \end{align}
\end{lemma}
% 
Using the above lemma, and upper bounding $\mathbb{E}_{\theta}[N^-]$ by $T = 2KV^*_1$, with $\Delta = \Delta^* = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}$ and substituting it in eqn 33, we obtain
\begin{align}\label{eqn:final_avgreg}
    \frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{(d-1) \cdot \sqrt{\delta} \cdot \sqrt{KV_1^*}}{2^{n+8}} \geq \frac{d \cdot \sqrt{\delta} \cdot \sqrt{KV_1^*}}{2^{n+9}}.
\end{align}
Since the average of regrets over a set of instances is lower bounded by the RHS, there must exist atleast one instance for whom RHS is a lower bound. 

Finally to justify that the chosen $\Delta$ is valid i.e., $\Delta = \Delta^* < 2^{-n} \cdot\frac{1-2\delta}{1+n+n^2}$  provides a bound on $K$ as 
\begin{align}
    K > \frac{(d-1)^2 \cdot \delta}{2^{10} \cdot V^*_1 \cdot \{\frac{1-2\delta}{1+n+n^2}\}^2} 
\end{align}
where $V^*_1$ is given by
\begin{align}
    V^*_1= \frac{2n}{n-1+2(\delta+\Delta)}.
\end{align}
This completes the proof.
\end{proof}
\textcolor{red}{it is easy to show that $V^*_1 > V^*_n/n = B^*/n$. So the eqn \ref{eqn:final_avgreg} can be further lower bounded using this relation to $\Omega(2^{-n}d\sqrt{KB*/n})$. Take your call to include n or not for now. We will have to think about this though.}\\

\pt{Does this mean that the $K$ is almost zero? division by a large number $2^{10}$?}



% \pt{Not updated:}  \pt{mathematical manipulation lead to simplification, hence V pi is minimized for a theta. }Using the partition of state space based on number of agents at node $s$, identifying that the indicator has positive coefficient if any agent in $\mathcal{I}$ moves from $s$ to $g$ or negative if it stays at $s$, and using the above induction assumptions, \textcolor{red}{through some clever mathematical manipulations} we show that $ V^{\pi_{\tb{\ti{a}}}}(\tb{\ti{s}})$ is minimized for any $\tb{\ti{s}} \in \mathcal{S}_{k+1}$ at $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$. \pt{Let us write the exact result/eqn that we use to prove this.}
% % 
% This again requires using Corollary \ref{corollary:ps_s}. Corollary \ref{corollary:p_star} ensures the second claim holds. Finally to prove that claim 3 holds for our case, we first show that the following lemma holds for all the instances that we consider.  \pt{Move this lemma to section 3.2}
% 

==> Sections/extras2.tex <==
\section{Introduction}
\label{sec:intro}


Our major contributions are as follows:
\begin{itemize}
    \item \textbf{Analysis wrt Number of Agent}
    \item \textbf{Experiments}
\end{itemize}

% \input{Sections/6_experiments}



\subsection{Proof of Lower Bound}
We construct and analyze a family of hard to learn instances. This is the same as in section 1.1. Further, we restrict $\theta$ such that $\theta_{i} \neq \theta_{j}$ $ \forall$ $ i \neq j \in [n]$ i.e., no two $\theta_i$ are the same. Let this set be denoted as $\Theta$. \pt{Why this assumption will hold. there is lot of symmetry in the problem, so $\theta$'s for two agents will be same?}. \textcolor{blue}{It's not an assumption. It's a restriction of the class of SSPs instances I'm considering. I'm free to do so. Why I do this is the rest of paragraph about. Also $\theta$ is an instance parameter, it can be anything. A way to think about this is that : even if two agents took same action, the contribution to probability of transition to any global state is not the same, this is one way how agents are not identical!} This ensures that the action to be taken by each agent to maximize the probability of transition to the all-at-goal state is different for every agent so that we don't need to consider the congestion component of the cost when the policy of maximizing the probability to reach all-goal is executed.
To further reduce complexity of the analysis, we let the private cost associated with any action in the initial state be equal to 1 and that in goal state equal to 0. This ensures that the \textit{best} policy is the one that maximizes the probability of transition to the global goal \pt{goal?} \textcolor{blue}{yes, thanks!} state.  \\
Suppose in episode \textit{k}, agents take actions according to policy $\pi$. Let, $\tb{s}_t$ represent the global state and $\tb{a}_t$ the global action at time $t$. Then, the expected regret for the \textit{k-th} episode is:
\begin{align}
    R_{\theta,k} &= V^{\pi_\theta}(\tb{s}_1) - V^*(\tb{s}_1) 
    \\
    &=  V^{\pi_\theta}(\tb{s}_1) - \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) 
    \\ 
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^\pi(\tb{s}_2)]\}  
    \\ 
    & \quad -\mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^*(\tb{s}_2)] \} + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim\ \pi(\tb{s}_1), \tb{s}_2 \sim\ \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi}(\tb{s}_2) - V^*(\tb{s}_2)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1)
\end{align}

\pt{Suggestion -- for each equation write the proper reason why it is true. This will make it easy to follow. For example, in above the second equation you added and subtracted $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] $.}
\textcolor{blue}{Ok, I'll do it after I start revisiting them. Apart from adding and subtracting Q, I've only expanded the Bellman Equation}

\textcolor{red}{I'm stuck here to find a closed form expression of $Q^*(.,.)$ and $V^*$ due to exponential number of states}

\subsection{Some proofs I have been trying since Monday}
\subsubsection{}
\begin{align} 
    & \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q^{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ c(\tb{s}_1,\tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)] \} - V^{\pi^*}(\tb{s}_1) \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim   \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - V^{\pi^*}(\tb{s}_1) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - (1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)]) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{  \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)] \}
    \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} \{ \sum_{\tb{s} \in \mathcal{S}} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*)) V^{\pi^*}(\tb{s})\}
\end{align}

\\
The above just follows from writing the definition of optimum Action value function and doing some rearrangement and remember costs throughout is 1.
\\

In the below proof, we expand the difference in probability term arising in the above equation. The initial global state, $s_1$, is with all agents at $s_{init}$ and the next state, $s$, is one where agents $i_1,i_2,..,i_r$ remain at $s_{init}$ and those at $j_1,j_2,..,j_{n-r}$ go to goal node. \\
\textcolor{red}{Following stays the same with updated features}

\begin{lalign}
\mathbb{P}(s|s_1, a_1) - \mathbb{P}(s|s_1, a_1^*)  
\\
&= \langle \phi(s|s_1,a_1), \theta \rangle - \langle \phi(s_1|s_1,a_1^*), \theta \rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1), \phi(s_2^{\prime}|s_2, a_2)..., \phi(s_n^{\prime}|s_n,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\& - \langle (\phi(s_1^{\prime}|s_1, a_1^*), \phi(s_2^{\prime}|s_2, a_2^*)..., \phi(s_n^{\prime}|s_n,a_n^*)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1),..., \phi(s_n^{\prime}|s_n,a_n)) - (\phi(s_1^{\prime}|s_1, a_1^*),..., \phi(s_n^{\prime}|s_n,a_n^*)), \\
& (\theta_1, 1,...,\theta_n,1)\rangle 
\\
&= \sum_{m = 1}^{r} \langle \phi(s_{i_m}^{\prime}|s_{i_m},a_{i_m}) - \phi(s_{i_m}^{\prime}|s_{i_m},a^*_{i_m}), (\theta_{i_m}, 1)\rangle \\ 
& + \sum_{m = 1}^{n-r} \langle \phi(s_{j_m}^{\prime}|s_{j_m},a_{j_m}) - \phi(s_{j_m}^{\prime}|s_{j_m},a^*_{j_m}), (\theta_{j_m}, 1)\rangle 
\\
&= \sum_{m=1}^{r} \langle (-a_{i_m} + a^*_{i_m}, 0), (\theta_{i_m}, 1) \rangle + \sum_{m=1}^{n-r} \langle (a_{j_m}-a^*_{j_m}, 0), (\theta_{j_m}, 1) \rangle   
\\
&= \sum_{m=1}^{r} (\langle a^*_{i_m}-a_{i_m}, \theta_{i_m} \rangle)  + \sum_{m=1}^{n-r} (\langle a_{j_m}-a^*_{j_m}, \theta_{j_m}  \rangle)  
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1} (a^*_{i_m, p} - a_{i_m, p})\theta_{i_m, p} \} + \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1} (a_{j_m, p} - a^*_{j_m, p})\theta_{j_m, p} \}
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\} \}  - \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \}
\\
&= \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\}
\end{lalign}
\\
\\
The lines 142-146 we use the linearity assumption and properties of inner product. Then, split the sum on $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Line 150 uses defination of $\phi(.,.)$. 153 uses definition of $a^*$ as the one matching all signs with $\theta$. 
\\

\\



\subsubsection{}
\textcolor{red}{I've updated below with new features} \\
\text{Probability that after taking a global action $\tb{a}$, the next global state is still the same as before i.e., $\tb{s}$}
\begin{lalign}
\mathbb{P}(\tb{s}|\tb{s}, \tb{a})
\\ Linearity Assumption\\
&= \langle \phi(\tb{s}|\tb{s},\tb{a}), \boldsymbol{\theta} \rangle
\\
$Expanded form of features$
\\
&= \langle (\phi(s|s, a_1), \phi(s|s, a_2)..., \phi(s|s,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\
$Definition of Inner Product$
\\
&= \sum_{i = 1}^{n} \langle (\phi(s|s, a_i),(\theta_i,1))
\\
$Definition of Features$
\\
&= \sum_{i = 1}^{n} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}),(\theta_i,1) \rangle
\\
&= \sum_{i = 1}^{n} \{ \langle -a_i, \theta_i \rangle + \frac{1-\delta}{n.2^{n-1}} \}
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \langle a_i, \theta_i \rangle 
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} a_{i,p}. \theta_{i,p} 
\\ $Definition of action and theta$\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Taking summation over p inside$ \\
&=  \frac{1-\delta}{2^{n-1}} - 
 \frac{\Delta}{n(d-1)} \sum_{i = 1}^{n}   \Big\{ d-1 - 2 \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Just simplify$ 
\\
&=  \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
\end{lalign}

\subsubsection{}
\textcolor{red}{i've modified the below for updated features}\\
In this subsection we derive the expression of Probability that if at state $\tb{s} = \{s_{init}, s_{init}, \dots, s_{init}\}$, if global action $\tb{a} = (a_1,a_2,\dots, a_n)$ is taken, you reach $\tb{s}^{\prime}$ where the agents at indices in $\mathcal{I}:= \{ i_1,i_2,\dots, i_r\}$ stay in the same state while agents at indices in $\mathcal{J} := \{j_1,j_2,\dots,j_{n-r} \}$ move to goal state i.e., $s'_{i_1}=s'_{i_2}=\dots=s'_{i_r}=s_{init}$ and $s'_{j_1}=s'_{j_2}=\dots=s'_{j_{n-r}}=goal$. \\
$P(\tb{s}'|\tb{s},\tb{a}) \\ 
= \langle \phi(\tb{s}'|\tb{s},\tb{a}), \theta \rangle \\
= \langle \phi((s'_1,s'_2,\dots, s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n)), (\theta_1, 1, \theta_2, 1,\dots, \theta_n,1) \rangle \\
= \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)),(\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle \phi(s'_i|s_i,a_i), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(s'_j|s_j,a_j), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle (a_j, \frac{\delta}{n.2^{n-1}}), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \Big \{  \frac{1-\delta}{n.2^{n-1}} + \langle -a_i,\theta_i \rangle \Big \} + \sum_{j \in \mathcal{J}} \Big \{ \frac{\delta}{n.2^{n-1}} + \langle a_j, \theta_j \rangle \Big \} \\
= r. \frac{1-\delta}{n.2^{n-1}} - \sum_{i \in \mathcal{I}}    \langle a_i,\theta_i \rangle  + (n-r). \frac{\delta}{n.2^{n-1}} +  \sum_{j \in \mathcal{J}}  \langle a_j, \theta_j \rangle  \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}} -  \sum_{i \in \mathcal{I}} \{ \sum_{p = 1}^{d-1} a_{i,p}.\theta_{i,p} \} + \sum_{j \in \mathcal{J}} \{ \sum_{p = 1}^{d-1} a_{j,p}.\theta_{j,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \{
\sum_{j \in \mathcal{J}}   a_{j,p}.\theta_{j,p}  -  \sum_{i \in \mathcal{I}}  a_{i,p}.\theta_{i,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \Big \{
\sum_{j \in \mathcal{J}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{j,p}) = sgn(\theta_{j,p})\} - \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{
\sum_{j \in \mathcal{J}}  \Big[ 1 - 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}}  \Big[   1 - 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{  \Big[ n-r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] - \Big[  r - \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
\sum_{p = 1}^{d-1}  \Big \{  n-2r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
  \Big \{  (d-1)(n-2r) - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\frac{\Delta . (n-2r)}{n} +\frac{2 \Delta}{n(d-1)} . 
  \Big \{  \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}     \Big \} \\
$ 
\\
Lines 186-190 follow by linearity assumption, definition of features and splitting the dot product over $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Lines 191-195 simplify the dot product and rearrange terms. Line 196 uses definition of action and theta. The remaining lines simplify the summations and rearrange the terms.
\\
From the above expression, we conclude that this probability remains same (say, $p_{a,r}$ for subsequent discussions,  for all states $s \in \mathcal{S}_{n,r}$ for every $r \in [n]$ for $a = \{a_1,a_2,\dots,a_n\}$ given global action taken at $s = \{s_{init}, s_{init},\dots, s_{init}\}$.  \\

\textcolor{blue}{state this as a lemma}
\textcolor{red}{done}

A more general result of the above relates to transition probability from some $s \in \mathcal{S}_{n,r}$ to some $s' \in \mathcal{S}_{n,r'}(s)$ where $\mathcal{S}_{n,r'}(s)$ represents the possible states of type $r'$ reachable from $s$ i.e.m   $0 \leq r' \leq r \leq n$. We discuss this below. \\ 
\textcolor{red}{I've modified this for the updated features}

\\
\textbf{Lemma}: For an instance defined by $\theta \in \Theta$, and a global action $a=\{a_1,a_2,\dots, a_n\} \in \mathcal{A}$, the transition probability for any possible transition from $\mathcal{S}_{n,r}$ to $\mathcal{S}_{n,r'}$, for $n \geq r \geq r' \geq 0$ is constant depending on only r and $r'$. \textcolor{red}{Not true!!!, true when $a^i$ are same} \\ \\ 

\textcolor{blue}{need to include the condition on relative values on $r$ and $r'$ in the statement of lemma } 
\textcolor{red}{Done}

\textcolor{blue}{and perhaps others also} 
\textcolor{red}{definition of notations will already be present in the notations part of the paper, also i've introduced them earlier}

\textcolor{blue}{we will revisit the statement of this as per the proof} \\ \textcolor{red}{I've added a small paragraph below giving an overview of what has been done, i don't think we can simplify further}

Suppose $s$ is such that agents at index in $\mathcal{I}:= \{i_1,i_2,\dots, i_r\}$ are at $s_{init}$ and those at $\mathcal{J} := \{j_1,j_2,\dots, j_{n-r}\}$ are already at goal. Let agents in $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ be the ones transiting from $s_{init}$ to $goal$ i.e., $s \in \mathcal{S}_{n,r}$ and $s' \in \mathcal{S}_{n,r'}$ where $n \geq r \geq r' \geq 0$ and $n \geq 1$. \\ \\
$P(s'|s,a)  \\= \langle \phi(s'|s,a), \theta \rangle  \\= \langle \phi((s'_1,s'_2,\dots,s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n) ), (\theta_1,1,\theta_2,1,\dots,\theta_n,1)\rangle  \\ = \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots, \theta_n,1) \rangle  \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle \phi(s|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle \phi(g|s,a_t), (\theta_t,1) \rangle \\ 
= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle (-a_i, \frac{1-\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle (a_t, \frac{\delta}{n.2^{r-1}}), (\theta_t,1) \rangle \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \{ \frac{1-\delta}{n.2^{r-1}} + \langle -a_i, \theta_i \rangle \} + \sum_{j \in \mathcal{J}}   \frac{1}{n.2^{r}}  + \sum_{t \in \mathcal{T}} \{ \langle a_t,\theta_t  \rangle + \frac{\delta}{n.2^{r-1}} \}   \\=  r'. \frac{1-\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}  + (r-r'). \frac{\delta}{n.2^{r-1}} + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}   + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} a_{i,p}. \theta_{i,p}      + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   a_{t,p} .\theta_{t,p}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} -  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{t,p}) = sgn(\theta_{t,p})\} -  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}}  \frac{\Delta}{n(d-1)} \Big \{  d-1 -  2 \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}}    \frac{\Delta}{n(d-1)} \Big \{  d-1 - 2\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} -   \frac{\Delta}{n(d-1)} \Big \{  r'(d-1) -  2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     +    \frac{\Delta}{n(d-1)} \Big \{  (r-r').(d-1) - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n(d-1)} \Big \{  (r-2r').(d-1) + 2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}
$ 

\pt{this incorporates the new features. Also, this will be the optimal probability when the sign matching property holds.}

\textcolor{blue}{we can avoid `line break' commands above } \textcolor{red}{ok, removed them but now proof may seem clumsier}  \textcolor{blue}{ok, we will see a way out, perhaps, we will introduce them}



\textcolor{blue}{we should use available  macros for lemma, proof, etc. see the style file.} 

\textcolor{blue}{these help where the proof starts and importantly ends -- Paul Halmos tomb-stone mark}
\textcolor{red}{ok, this is new for me. i'll try to learn this.}


Initial lines (not mentioning number since it is changing as we are modifying content above) use linearity assumption, definition of features and decomposing the inner product over agents who remain put at $s_{init}$, transit to goal and remain put at goal. In the next few lines, we expand the inner product terms and summations, use the definition of actions and theta and rearrange. Then, just rearrange different terms.  The indicators make sure appropriate sign is given to the dot product depending on signs of components of action and that of theta, \textcolor{blue}{we will cite some papers about these signs }. 

\textcolor{blue}{this is helpful to the reader}

\textcolor{blue}{let's write the role of indicator function above} \textcolor{red}{role as in?}


\\
\\
Notice that for a given global action, the  transition probability from any $s \in \mathcal{S}_{n,r}$ to any $s' \in \mathcal{S}_{n,r'}$ as long as the transition is possible (i.e., $s' \in \mathcal{S}_{n,r'}(s)$) remains the same as above. 

\textcolor{red}{This para is not complete yet!}Further, for any valid $r'$, one can verify that for any action the above probability decreases with $r$ when the sufficient condition holds : $n-1 < \log_2(\frac{\delta.n}{\Delta}.ln(2)).$ We need to assure that we select $\delta$ and $\Delta$ such that this assumption holds. Typically, we will take $\delta = O(2^n\Delta)=o( 1)$.
 \\
 Hence, $p_{a,r}(m) < p_{a,r}(n)$ for every $r$, $m>n$ for any global action $a$. 
 
Another important probability is that of transition to global goal state after taking a global action a in any state $s \in \mathcal{S}_{n,r}$. \\  \\
\textcolor{red}{I've changed below expressions for the updated feature}
\\
\\
 $ P(s'=(g,g,\dots,g)|s,a) \\ = \langle \phi(s' = (g,g,\dots, g)|(s,a)), \theta \rangle \\ = \langle (\phi(g|s_1,a_1), \phi(g|s_2,a_2),\dots, \phi(g|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle \phi(g|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle (a_i, \frac{\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j,1) \rangle \\ = \frac{r\delta}{n2^{r-1}} + \sum_{i \in \mathcal{I}} \langle a_i,\theta_i \rangle + \frac{n-r}{n2^{r}} \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  a_{i,p} \theta_{i,p} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}}  \frac{\Delta}{n(d-1)} \Big\{ d-1 - 2  \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
  \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  +  \frac{r \Delta}{n} - \frac{2 \Delta}{n(d-1)} \sum_{i \in \mathcal{I}}    \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
 $
\\
\\
This is very similar to above proofs and no new idea is used, only the state is explicitly mentioned.
\\

\textcolor{blue}{write this as another lemma} \textcolor{red}{i had written this before writing the above general proof which is now a lemma. this one is specific for r=n and r'=0 which game me an idea of how to express for general case. should this be a lemma or corollary } \textcolor{blue}{yes, as said over phone. }

\subsubsection{Another way to think of Q-V difference introduced in 1.4.1\textcolor{blue}{this is advantage function, isn't?}} \textcolor{red}{yes, it's like expected value of the advantage function since there is expectation over $a_1$ according to the policy \\ also i've modified below for new features}
\\
\\
In the below, $s_t$ represent global state at time t (Note it's not individual state). Similarly $a_t$ is global action at t.

\begin{lalign} }

$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1) \\
= \mathbb{E}_{a_1 \sim \pi(s_1)}[c(s_1, a_1) + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}V^*(s_2)] - V^*(s_1)  $ \\
Using Bellman Equation and cost is 1
\\ 
$=  \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{  1 + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}[V^*(s_2)] - V^*(s_1) \Big \}$
\\ Expand the Expectation $ \\
=   \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  P(s_1|s_1,a_1) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1) \Big \}
\\ $ Use expression of probability from above$
 \\= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2)  - V^*(s_1) \Bigg \}
\\$ Rearranging the terms $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*(s_1) \Big\} 
\\ $ Notice from the general expression of probability from previous proof $\\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - V^*(s_1) \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} 
\\$ Expand V*(s_1) $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 + P(s_1|s_1,a_1^*)  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - \Big\{ 1 +  P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1, a_1^*) V^*(s_2) \Big\} \Bigg \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p})\neq sgn(\theta_{i,p})\} V^*(s_1) \Big\} 
\\$ Rearrange and combine  terms$ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $
\end{lalign}

\subsubsection{Symmetry in the features lead to identical Value function of similar states}
Suppose there n agents. Let $\mathcal{S}_{n,r}$ represent the set of all states where r agents are at $s_{init}$ (Recall, $\mathcal{I}$ and $\mathcal{J}$). Note that |$\mathcal{S}_{n,r}$| = $\binom{n}{r}$. We claim that these have the same optimum value functions.  \\ \\
\textbf{Proof} \\
Use induction arguments. \\ For r = 1, \\
for any $s \in \mathcal{S}_{n,1}$, the only next possible states are $'s'$ itself and g = (goal,goal,..,goal). Suppose agent i is the one who is only at $s_{init}$. Then, \\
\begin{lalign}
    $V^*(s) = 1 + P(s|s,a^*) V^*(s) + P(g|s,a^*) V^*(g)$ \\
    But, $V^*(g) = 0$. \\
    Thus, $V^*(s) = \frac{1}{1-P(s|s,a^*)} = \frac{1}{P(g|s,a^*)}$ \\ \\
    Now, $P(g|s,a)  \\
    = \langle \phi((s^{\prime}_{1}=g,s^{\prime}_2=g,..,s^{\prime}_{i-1}=g, s^{\prime}_{i}=g,s^{\prime}_{i+1}=g..s^{\prime}_n = g)|(s_1 =g, s_2 = g,..,s_{i-1} = g, s_i = s, s_{i+1}=g,...s_n = g ), (a_1,a_2,...,a_n)), (\theta_1,1, \theta_2,1,..\theta_n,1) \rangle \\
    = \langle (\phi(g|g,a_1), \phi(g|g,a_2),...,\phi(g|g,a_{i-1}), \phi(g|s,a_{i}), \phi(g|g,a_{i+1}),...,\phi(g|g,a_n)), (\theta_1,1,\theta_2,1,...,\theta_n,1)\rangle \\
    = \langle \phi(g|g,a_1), (\theta_1,1) \rangle + \langle \phi(g|g,a_2), (\theta_2,1) \rangle + ... + \langle \phi(g|g,a_{i-1}), (\theta_{i-1},1) \rangle + \langle \phi(g|s,a_i), (\theta_i,1) \rangle, \langle \phi(g|g,a_{i+1}), (\theta_{i+1},1) \rangle + ... + \langle \phi(g|g,a_n), (\theta_n,1) \rangle \\
    = \langle (0_{d-1}, \frac{1}{n.2^1}), (\theta_1,1) \rangle + \langle (0_{d-1}, \frac{1}{n.2^1}), (\theta_2,1) \rangle + ... + \langle (0_{d-1}, \frac{1}{n.2^1}), (\theta_{i-1},1) \rangle + \langle (a_i, \frac{\delta}{n.2^0}), (\theta_i,1) \rangle, \langle (0_{d-1}, \frac{1}{n.2^1}), (\theta_{i+1},1) \rangle + ... + \langle (0_{d-1}, \frac{1}{n.2^1}), (\theta_n,1) \rangle \\
    = \frac{n-1}{2n} + \frac{\delta}{n} + \langle a_i, \theta_i \rangle$
\end{lalign}
\\
Thus, \\ $P(g|s,a^*) = \frac{n-1}{2n} + \frac{\delta}{n} + \langle a^*_i, \theta_i \rangle = \frac{n-1}{2n} + \frac{\delta}{n} + \frac{\Delta}{n}$
\\
Hence, $V^*(s) = \frac{1}{\frac{n-1}{2n} + \frac{\delta}{n} + \frac{\Delta}{n}}$ \\
\textcolor{red}{Note that at n=1, we recover Min et al solution}\\
\pt{This is with the updated features? This  optimal value is for the case when the number of agents at $s_{init}$ are 1.} 
\textcolor{red}{yes, with the ones matching Min et al}

Since we made no assumption regarding $'i'$, the above argument holds for any $i \in [N]$ due to which $V^*(s)$ will be same as above for any $s \in \mathcal{S}_{n,1}$ \\
Thus, we have shown truth for the base case. \\
Now assuming true for $1, 2,\dots,r-1$, we want to prove for $r$. \\
To rephrase, assuming that $V^*(s) = V^*_m$ $\forall$ $s \in S_{n,m}$ holds for every $m = 1, 2,...r-1$, we wish to prove the same for $r$ \\
Consider arbitrary $s \in S_{n,r}$ in which the agents indexed $i_1, i_2, ..., i_{r}$ are at $s_{init}$ while others are at $goal$. \\
The set of all possible next states is given by: $\mathcal{S^{\prime}}:= \bigcup \limits_{r'=0}^{r} \mathcal{S}_{n,r'}(s)$ where $\mathcal{S}_{n,r'}(s)$ denotes the subset of $\mathcal{S}_{n,r'}$ that is reachable from $s$. Note that not all states in $\mathcal{S}_{n,r'}$ are reachable from $s$ since some of those transitions would correspond to the impossibility condition. Precisely speaking, $|\mathcal{S}_{n,r'}(s)| = \binom{r}{r'}$ which does not depend on which $s$ is being considered from $\mathcal{S}_{n,r}$
\\
Hence, \\
$V^*(s)\\ 
= \sum_{s^{\prime} \in \mathcal{S}^{\prime}} \{P(s^{\prime}|s,a^*).[1+V^*(s^{\prime})]\}
\\
= 1 + \sum_{s^{\prime} \in \mathcal{S}^{\prime}} \{P(s^{\prime}|s,a^*).V^*(s^{\prime})\}\\  \\ $Definition of V*, expand the summation and simplify$ \\ \\
= 1 + P(s|s,a^*).V^*(s) + \sum_{s^{\prime} \in \mathcal{S}_{n,r-1}(s)} P(s^{\prime}|s,a^*).V^*(s^{\prime}) + \sum_{s^{\prime} \in \mathcal{S}_{n,r-2}(s)} P(s^{\prime}|s,a^*).V^*(s^{\prime}) + \dots +  \sum_{s^{\prime} \in \mathcal{S}_{n,1}(s)} P(s^{\prime}|s,a^*).V^*(s^{\prime})
$ \\ 
Using the result above that $P(s'|s,a)$ only depends of $r$ and $r'$, for $a^*$ lets denote that by $p^*_{r,r'}$ \\
$V^*(s) \\
= 1 + P(s|s,a^*) V^*(s) + \sum_{s^{\prime} \in \mathcal{S}_{n,r-1}(s)} p^*_{r,r-1} V^*_{r-1} + \sum_{s^{\prime} \in \mathcal{S}_{n,r-2}(s)}p^*_{r,r-2} V^*_{r-2} + \dots + \sum_{s^{\prime} \in \mathcal{S}_{n,2}(s)} p^*_{r,2} V^*_{2} + \sum_{s^{\prime} \in \mathcal{S}_{n,1}(s)} p^*_{r,1} V^*_{1} \\  \\ $Taking the induction hypothetsis to be true till $r-1$, also note that $p^*_{r,j}$ is the probability to reach a fixed state of type j starting at s (refer how s is defined again above) and taking global optimal action. Since this is the same for every state of that type the cardinality of respective set appears. \\ \\
$= 1 + P(s|s,a^*) V^*(s) + |\mathcal{S}_{n,r-1}(s)| p^*_{r,r-1} V^*_{r-1} +  |\mathcal{S}_{n,r-2}(s)|p^*_{r,r-2} V^*_{r-2} + \dots + |\mathcal{S}_{n,2}(s)| p^*_{r,2} V^*_{2} + |\mathcal{S}_{n,1}(s)| p^*_{r,1} V^*_{1}$ \\
 \\
 Hence, \\
 $V^*(s) = \{1 + |\mathcal{S}_{n,r-1}(s)| p^*_{r,r-1} V^*_{r-1} +  |\mathcal{S}_{n,r-2}(s)|p^*_{r,r-2} V^*_{r-2} + \dots + |\mathcal{S}_{n,2}(s)| p^*_{r,2} V^*_{2} + |\mathcal{S}_{n,1}(s)| p^*_{r,1} V^*_{1} \} . \{ 1 - P(s|s,a^*) \}^{-1}$
 \\
 \\
Notice that only the factor $\{1 - P(s|s,a^*)\}$ potentially depends on which s is chosen among $\mathcal{S}_{n,r}$. All other terms are constant and independent of which $s \in \mathcal{S}_{n,r}$ we are considering. To prove that $V^*(s)$ is same for every $s \in \mathcal{S}_{n,r}$, it is thus sufficient to show that this factor is same for every $s \in \mathcal{S}_{n,r}$. Below, we establish this: \pt{This can also be written as a separate lemma and we can use that lemma here directly.} \textcolor{red}{In the general transition probability lemma, putting r=r'=n gives this result. So lets state it as a corollary to that lemma. }
\\
$P(s|s,a^*) \\
= \langle \phi(s|s,a^*), \theta \rangle \\
= \langle (\phi((s'_1,s'_2,\dots,s'_n)|(s_1,s_2,\dots,s_n),(a_1^*,a_2^*,\dots,a_n^*))), (\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\
= \langle (\phi(s'_1|s_1,a_1^*), \phi(s'_2|s_2,a_2^*),\dots,\phi(s'_n|s_n,a_n^*)),(\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\
= \sum_{m = 1}^{n} \langle \phi(s'_m|s_m,a_m^*),(\theta_m,1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle \phi(s'_i|s_i,a_i^*),(\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(s'_j|s_j,a_j^*),(\theta_j,1) \rangle
\\
= \sum_{i \in \mathcal{I}} \langle \phi(s|s,a_i^*),(\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j^*),(\theta_j,1) \rangle
\\
= \sum_{i \in \mathcal{I}} \langle (-a^*_i,\frac{1-\delta}{n.2^{r-1}}),(\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^r}),(\theta_j,1) \rangle
\\
= \sum_{i \in \mathcal{I}}  \{ \frac{1-\delta}{n.2^{r-1}} + \langle -a^*_i,\theta_i \rangle \} + \sum_{j \in \mathcal{J}} \frac{1}{n.2^r} 
\\
= \sum_{i \in \mathcal{I}}  \{ \frac{1-\delta}{n.2^{r-1}} - \frac{\Delta}{n} \} + \frac{n-r}{n.2^r}  
\\
= r. \frac{1-\delta}{n.2^{r-1}} - r. \frac{\Delta}{n}  + \frac{n-r}{n.2^r}  
 \\$
The above calculation is similar in spirit to the ones in earlier section. The idea is to use linearity model of transition probability, definition of features, split the summation into two sets as earlier defined, use definition of action and theta$ \\
$
Observe that we had chosen arbitrary $s \in \mathcal{S}_{n,r}$ for whom the expression only depends on r. But this is same for every $s \in \mathcal{S}_{n,r}$. Hence, $P(s|s,a^*)$ is same for every $s \in \mathcal{S}_{n,r}$. Thus, $V^*(s)$ is same for every $s \in \mathcal{S}_{n,r}$. \\
Hence, proved. \\
\textcolor{red}{I've also modified the above proof for new features}

\\ \\

We also show below that $V_m^*$ are ordered i.e., $V_1^* < V^*_2 < V^*_3 < \dots < V^*_r <V^*_{r+1}<\dots<V^*_n$ \\
Use Induction arguments \\
For r = 1, it's easy to see using Bellman Equation that \\
$V^*_1 = 1 + (1-p^*).V^*_1 + p^*. 0 \implies V_1^* = \frac{1}{p^*}$ \\ 
In above, $p^*$ is the transition probability of the system to the global goal state under optimum  global action $a^*$ taken at some $r=1$ state. 
\\
Assuming true for every $m \in \{1, 2,\dots , r-1\}$, we try to prove for $r$. Again, using Bellman Equation, \\
$V^*_r = 1 +  p^*_{r,r} . V^*_r + \binom{r}{r-1} p^*_{r,r-1}. V^*_{r-1} + \sum_{m=1}^{r-2} \binom{r}{m} p^*_{r,m}.V^*_m \\ \implies V^*_r = \frac{1 + r.p^*_{r,r-1}. V^*_{r-1} + \sum_{m=1}^{r-2} \binom{r}{m}p^*_{r,m}.V^*_m}{1-p^*_{r,r}}$ \\ 
\\
It is thus sufficient to prove that $V^*_r > V^*_{r-1}$ \\
$V^*_r - V^*_{r-1} = \frac{1 + r.p^*_{r,r-1}. V^*_{r-1} + \sum_{m=1}^{r-2} \binom{r}{m}p^*_{r,m}.V^*_m}{1-p^*_{r,r}} - \{ 1+p^*_{r-1,r-1}V^*_{r-1} + \sum_{m=1}^{r-2} \binom{r-1}{m}p^*_{r-1,m}.V^*_m\} \\ > 1 + r.p^*_{r,r-1}. V^*_{r-1} + \sum_{m=1}^{r-2} \binom{r}{m}p^*_{r,m}.V^*_m - \{ 1+p^*_{r-1,r-1}V^*_{r-1}+\sum_{m=1}^{r-2} \binom{r-1}{m}p^*_{r-1,m}.V^*_m\} > 0 $ \\  \textcolor{red}{This is incomplete as of now but very important to show. Possibly i will have to redesign the features. EVEN THIS SEEMS VERY DIFFICULT! \\ This problem has been resolved now.  } 

\pt{Why do you need to change the features now?}\\
\textcolor{red}{to ensure monotonicity of V*}

Hence, $V^*_{r} > V^*_{r-1}$





\subsubsection{Dealing with the sum of Probability differences in 1.4.4 using 1.4.5} 

Recall from 1.4.4, \\ 
$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)   
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \\
 \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 The first term is problematic and it is not clear how to deal with it. Let's investigate the summation inside the expectation of the first term: \\ 
 $\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2) \\ = \sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} [P(s'|s_1,a_1)-P(s'|s_1, a_1^*)] V^*(s') $ (Now, use results from above sections) \\
 = $\sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\} V^*_r $ \\
= $\frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{\sum_{s' \in \mathcal{S}_{n,r}} [\{   \sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p}) \}]  \Big\}   \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n}   
 \sum_{s' \in \mathcal{S}_{n,r}} [ \mathbbm{1}\{s'_i = s_{init}\}   \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   - \mathbbm{1}\{s'_i = goal\}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \}]  \Big\} \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  
 \sum_{s' \in \mathcal{S}_{n,r}} \mathbbm{1}\{s'_i = s_{init}\}     -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \sum_{s' \in \mathcal{S}_{n,r}} 
 \mathbbm{1}\{s'_i = goal\} \Big\}  \Big\} 
 \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \binom{n-1}{r-1}    -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \binom{n-1}{r} \Big\}  \Big\} \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \{ \binom{n-1}{r-1}    -   \binom{n-1}{r} \} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} V^*_r  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} + V^*_{n-r}  \frac{2(n-r)-n}{n} \binom{n}{n-r} \} \Big\}   \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} - V^*_{n-r}  \frac{2r-n}{n} \binom{n}{r} \} \Big\}  \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  - V^*_{n-r}   \} \frac{2r-n}{n} \binom{n}{r} \Big\} \geq 0. 
 $ \\
 \\
 Observe that when $r> n/2, V^*_r > V^*_{n-r}$ and vice-versa (refer result above) \\
 Hence we have established that, \\
 $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1) \geq \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\ \\
 To generalize, we need to show that the above inequality holds for any $s_1 \in \mathcal{S}$ and not just $s_{init}$. We will use this result below.

 \subsubsection{Now going back to Lower Bound Proof with Inequality using above result}
 From 1.3, expected regret in the $k-th$ episode: \\
$R_{\theta,k} \\ = V^{\pi_\theta}(s_1) - V^*(s_1) 
\\ 
 = \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)$ \\
\\ Using 1.4.6, \\

 $R_{\theta,k} \\ \geq  \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_1 \neq goal \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 By recursion and the generalized result from the section above,
 we have: \\

 $R_{\theta,k} \\ \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{k} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_h \neq goal \} \mathbbm{1}\{sgn(a^h_{i,p}) \neq sgn(\theta^h_{i,p})\} \Big\} \\ \geq \frac{2 \Delta B^*}{n^2(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{k} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_h \neq goal \} \mathbbm{1}\{sgn(a^h_{i,p}) \neq sgn(\theta^h_{i,p})\} \Big\} $ \\
 where, the Expectation is taken with respect to trajectory induced in the $k-th$ episode by the interaction of policy $\pi$ and transition kernel $P_{\theta}$. Also, as discussed later, $B_*/n \leq V^*_1$ Now, the total expected regret over $K$ episodes is: \\
 $
 R_{\theta}(K) \\
 \geq   \frac{2 \Delta B^*}{n^2(d-1)} \sum_{t=1}^{\infty} \mathbb{E}_{\theta, \pi} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_t \neq goal \} \mathbbm{1}\{sgn(a^t_{i,p}) \neq sgn(\theta^t_{i,p})\} \Big\}
 $ \\
 Analogous to Min et al, Cohen et al, we define: \\
 $N = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} $ and for agent $i \in [n]$,\\
$N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta^t_{i,j})\} $  \\
Thus, $R_{\theta}(K) \geq \frac{2 \Delta B^*}{n^2(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]} \sum_{j=1}^{d-1} N_{i,j}(\theta) \}$ \\
To use the standard Pinsker's Inequality, we need $N_j(\theta)$ to be bounded almost surely which is known to not hold for SSPs (Min et al, Cohen et al). Hence, we use the capping trick introduced by Cohen et al and also used by Min et al. In this trick, we cap the learning process to a predetermined T. If the learning process (i.e. $K-th$ episode) ends before this, the agents continue to remain at $goal$. In this case the summation for the actual process and the capped process is the same. On the other hand when K episodes end beyond T, we have a truncated sum. Due to non-negativity of each part, the sum for the capped process lower bounds the actual sum. \\ Define \\ $N^- = \sum_{t=1}^T\mathbbm{1}\{s_t \neq goal\} $ and for any agent $i \in [n] $ and $ j \in [d-1],$\\ $N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta^t_{i,j})\} $ \\ 
It is easy to see that for any $i \in [n]$ and $j \in [d-1]$, $N^- =   N^-_{i,j}(\theta) + N^-_{i,j}(\theta^{j})  $ \\ where for every $\theta$, $\theta^j$ represents the vector that only differs at the $j-th$ index of every $\theta_i$ in $\theta = \{\theta_1,1,\theta_2,1,\dots,\theta_n,1\}$, where each $\theta_i \in \{\frac{-\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}\}^{d-1}$. \\ 
Thus,  $R_{\theta}(K) \geq \frac{2 \Delta B^*}{n^2(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}$.  Notice that $\theta \in \Theta \iff \theta^{j} \in \Theta$ (This follows from definition of $\Theta$ \textcolor{red}{without this, following equation won't hold}). Then, we have: \\
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{2 \Delta B^*}{n^2(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \{ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \} \\
= \frac{2 \Delta B^*}{n^2(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^- - N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta B^*}{n^2(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^-] - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta B^*}{n^2(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}

Need to prove generalisation of Lemma C2 in Cohen et al 2020: If $T \geq 2KB^*$, then $\mathbb{E}_{\theta}[N^-] \geq KB^*/4$  \\ \textcolor{red}{Suppose same holds, we pick $T = 2KB_*$} \\
\textbf{Pinsker's Inequality(Min et al, Lemma E.3)} \pt{$TV(p,q) \leq \sqrt{KL(p,q)}$}

If $f:S^T\xrightarrow{}[0,D]$ then, 
$\mathbb{E}_{\mathcal{P}_1} (f(s)) - \mathbb{E}_{\mathcal{P}_2} (f(s))\leq D \sqrt{\frac{log(2)}{2}}. \sqrt{ KL(\mathcal{P}_2 || \mathcal{P}_1)}$  

\pt{Note that this will hold only if $|f(s)| \leq D \sqrt{\frac{log(2)}{2}}$?}
\textcolor{red}{I dont think so. $|f(.)|$ can be D}


\pt{don't use double back slash. These are not needed. just give one line spacing.}

Then, 
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta B^*}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  \mathbb{E}_{\theta, \pi}  [N^-] +  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] - \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] \} \Big \} \\ = \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{  \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] - \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] \} \Big \} \\ 
\geq \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
$
\\
\\
\\
For appropriate $\delta, \Delta$, $KL(\mathcal{P_{\theta}||\mathcal{P_{\theta^j}}}) \leq \frac{16.\Delta^2}{(d-1)^2.\delta}.\mathbb{E_{\theta}}[N^-]$  \\
\\
\textcolor{red}{Need another intermediate similar lemma to simplify the KL-divergence term. \\ Assuming this also holds for our case, \\ }

$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
\geq \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{1/2} \sqrt{\frac{16.\Delta^2}{(d-1)^2.\delta}.\mathbb{E_{\theta}}[N^-]}  \} \Big \} \\
\geq \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{1/2} \frac{4.\Delta}{(d-1).\sqrt{\delta}}.\sqrt{T}  \} \Big \} \\
= \frac{2 \Delta B^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -   (2KB^*)^{3/2} \sqrt{1/2} \frac{4.\Delta}{(d-1).\sqrt{\delta}} \Big \} \\ 
$\\
Notice that the term in bracket is independent of $\theta, i$ or $j$. Thus, we have: \\
$\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq  \Delta B^* |\Theta| \Big \{  KB^*/4 -   (2KB^*)^{3/2} \sqrt{1/2} \frac{4.\Delta}{(d-1).\sqrt{\delta}} \Big \} \\
\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq   B^*  \Big \{ \Delta  KB^*/4 -   (KB^*)^{3/2} \frac{8.\Delta^2}{(d-1).\sqrt{\delta}} \Big \} \\ 
$ \\
Although $\Delta$ is constrained for well-defining probabilities, the RHS will be lower bounded by the unconstrained minimization of the RHS with respect to $\Delta$. This minimizer is $\Delta^* = \frac{(d-1) \delta}{64 \sqrt{KB^*}}$. At this value of delta,\\
$\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq  \frac{(d-1).\sqrt{\delta}.\sqrt{KB^*}}{512}$ \pt{This makes it independent of number of agents, a very strong result? Is this correct or do we need to incorporate the number of agents here.} \textcolor{red}{potentially the intermediate results I used directly without verifying depend on n. the term i argued to be $+ve$ and ignored in lower bound certainly depends on n but very difficult to simplify(needs closed form V*)}


Since the average over entire set is lower bounded by the RHS, there must exist some parameter in the set for which the RHS is a lower bound. Hence proved \textcolor{blue}{ok we will discuss the proof}. \\
Although it is independent of n, it can be interpreted as a strong result in the sense that no matter how many agents are deployed to learn, this minimum regret will always hold. The independence also comes from ignoring the positive terms \textcolor{red}{(whose proof is as of now still incomplete )}.

\textcolor{blue}{we need to write the  statement that is proved, and also delineate that statement from the proof -- use macros provided in the style file} \textcolor{red}{This is not complete yet. Only if we can find the corresponding lemmas I've mentioned in the proof, it will be complete possibly with very different expression.}

%\textcolor{blue}{ think it is $\newtheorem{lemma}{command for new lemma}$}

\subsubsection{$V^*$ for multiple cases}


General formula:  \textcolor{blue}{is this a theorem?} \textcolor{red}{It follows directly from Bellman equation}\\
 $V^*(s) = \{1  + |\mathcal{S}_{n,r-1}(s)| p_{a^*,r-1} V^*_{r-1} +  |\mathcal{S}_{n,r-2}(s)|p_{a^*,r-2} V^*_{r-2} + \dots + |\mathcal{S}_{n,2}(s)| p_{a^*,2} V^*_{2} + |\mathcal{S}_{n,1}(s)| p_{a^*,1} V^*_{1} \} . \{ 1 - P(s|s,a^*) \}^{-1}$

 \\ \\
 Below $p^*_{r,r'}$ denotes transition probability for a valid transition from state of type $r$ to that of type $r'$ under optimal global action in the respective instance specicified by $\theta$ and $n$ and $V^*_0 = 0$ \\ \\
For n = 1 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$ \\ \\ 
For n = 2 \\
For r = 1 \\ 
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For n = 3 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
\\

For n=4 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\

For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
For r = 4 \\
$V^*_4 = 1 + p^*_{4,4}V^*_4 + \binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1+\binom{4}{4}p^*_{4,0}V^*_0 = \frac{1+\binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1}{1-p^*_{4,4}} = \frac{1+\binom{4}{1}p^*_{4,3}\frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} + \binom{4}{2}p^*_{4,2}\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{4}{3}p^*_{4,1}\frac{1}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+\frac{ \binom{4}{1}p^*_{4,3} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} +\frac{ \binom{4}{2}p^*_{4,2}+\frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}}  = \frac{1+ \frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+ \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}}+\frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  }{1-p^*_{4,4}}$


\pt{can you see the closed form expression here?} \textcolor{red}{i can see a pattern but can't express it nicely.}

\pt{if not, can you confirm whether this notation is correct? -- $p^*_{r,r'}$ is the probability that number agent in the state $s$ were $r$, and the number of agents in $s'$ are $r'$?} \textcolor{red}{yes, line 308-309}

\pt{also can you recall me here -- what does the  $\binom{4}{2}$ or $\binom{3}{1}$ represent in terms of $r,n,$ and $r'$? $\binom{r}{r-r'}$} \textcolor{red}{yes,in the first factor of every term in the numerator}

\pt{I will try to get the closed form expression once you mention this.}


\pt{Also can you summarize what are the intermediate results we have. summarize all of them no matter how  trivial or useful they are are. } \textcolor{red}{In the probability section there's just one important result - general formula for transition probability - the lemma. Putting different values of r and r' give other results. For V*, there's just one important result: for the same "type" of states, V* is the same. This can be expressed as a lemma too. Apart from that monotonicity proof is incomplete, hence lower bound proof is incomplete. This includes all the simplification related to V-V*.}

\pt{I can see  that you have many intermediate results.}












\textcolor{blue}{let's write here the  intermediate steps with pending proofs }
\textcolor{red}{done as of now, thought there's a pattern, to express it mathematically is a bit challenging, i'll try to think about this}

\subsubsection{Important result regrding monotonicity of V*} \\

Consider the states space, $\mathcal{S} = \{s_1,s_2,\dots,s_n\} \cup \{x,y\} $. Let under some global action, the following markov chain be induced:
\\ Cost for any transition is constant and equal to 1. Transition probability from x to $s_i$ is represented as $p_{x,i}$ and from y to $s_i$ as $p_{y,i}$ for $i \in \{1,2,\dots,n\}$ and $p_{x,x}$ and $p_{y,x}$ represent the same from x and y respectively to x. Probability from y to y is represented as $p_{y,y}$. All probabilities are considered between 0 and 1 (strictly). Further, it holds that $p_{y,s} = p_{x,s} - \delta_s$ for every $s\in \{x,1,2,\dots,n\}$ where all $\delta_s \in (0, p_{x,s})$. (We would later require that assuming $p_{x,(.)}$ is monotonic, $\delta_s$'s are such that they preserve the monotonicity of $p_{y,(.)}$. But this assumption on $\delta_s$'s is not required in this discussion.) No other transitions are possible. For the sake of discussion, we assume that the states $s_1,s_2,\dots,s_{n}$ are absorbing states (potentially there may be all kinds of transitions from there but the long term value is known hence they can be considered terminal states with these values) with value function known respectively as $V_1,V_2,\dots,V_n$ while value of state $x$ is also known as $V_x$. Assume the following condition holds for the values: $V_1<V_2<\dots<V_n < V_x$. We want to relate $V_x$ and $V_y$. \\ \\
\tb{Claim:} $V_x < V_y$ \\ \\
$p_{y,y} = 1-p_{y,x}-\sum_{i=1}^{n}p_{y,i} = 1-(p_{x,x} - \delta_x) - \sum_{i=1}^n(p_{x,i}-\delta_i) = \delta_x + \sum_{i=1}^n \delta_i$ \\ \\
$V_x = \sum_{i=1}^np_{x,i}(1+V_i)+p_{x,x}(1+V_x)$ \\ \\
Similarly, \\
$V_y = \sum_{i=1}^np_{y,i}(1+V_i) + p_{y,x}(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^n(p_{x,i}-\delta_i)(1+V_i) + (p_{x,x}-\delta_x)(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^np_{x,i}(1+V_i) + p_{x,x}(1+V_x)-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_i)\} + p_{y,y}(1+V_y) $ \\ \\
From the definition of $V_x$ above and monotonicity of V's, we have : \\
$V_y > V_x-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_x)\} + p_{y,y}V_y = V_x-p_{y,y}(1+V_x) + p_{y,y}(1+V_y) \\ \implies V_y - V_x > p_{y,y}(V_y -V_x) \\ \implies (1-p_{y,y}) (V_y - V_x) > 0 \\ \implies V_y>V_x $

 \\ 

 \subsubsection{Applying above to our case}
We want to prove that under reasonable conditions, $V^*_r^$ are strictly increasing in $r$. We will do this by induction. \\
\tb{Base Case} \\
To show: $V^*_0 < V^*_1$ \\
Recall we already proved $V$ is same for all states as long as they are of same "type" i.e., have same r. \\
Now take any state in $\mathcal{S}_{n,1}$. Let $1>p^*_{1,0}>0$ be the probability of going to global goal state under global action 
 
 \subsubsection{Monotonicity in P ensures $V^*$ ordered} \\
 Consider any initial state s. Let it be of type 'r' i.e., $s \in S_{n,r}$. Now, we will ensure that under any global action at s, the probabilities are such that they monotonically decrease with (over entire) "type set" (defined as the set of states reachable from s of the same type). This will ensure that if shown for the base case (easy to show for r=0 as and r=1 $V^*_0 = 0$ and $V^*_1 > 0$), $V^*$ are monotonically ordered due to the above result. Also, $a^*$  is the one with all signs matching with $\theta$ can be shown for r=1 (base case) easily as long as it maximizes probability to goal. For the induction argument assume this $a^*$ is best for all "type sets" till r-1. Showing $a^*$ at s is the same as the one with signs matching will prove that $a^*$ is the this same action for all states. \\ Using Bellman Equation : \\
 $Q(s,a) = \sum_{i=0}^{r-1}P(i|s,a)(1+V^*_i) + P(s|s,a)(1+V^*_s)$ \\
If we ensure that for any action, the transition probabilities satisfy reduction property as in the above case, $V^*$'s will be monotonic for all those actions. This ensures that the action that uniformly dominates in maximization of the probability to reach the lower "type sets" is the best action $a^*$. We try to construct such an instance, so that the $a^*$ remains the same as the one with all signs matched with $\theta$. \\
To summarize we need the following properties from our instance: 
\begin{itemize}
    \item For any $r \in \{0,1,\dots,n-1\}$ for any global action a, the probability to reach any type set r, r-1, r-2,..,1,0, from r must be strictly higher than from r+1. This leads to V's are ordered as long as $V_1>V_0 = 0$ which holds in general. 
    \item For any state, there must exist an action that uniformly maximises the probability to reach the lower state type sets. This will ensure that it is optimum due to monotonicity of $V^*$. We want this action to be the one matching the signs with $\theta$  \textcolor{red}{this is not possible. individual maximizers are different. hence, i'll remove this}
\end{itemize} 


\subsubsection{Proving $a^*$ is the one that matches sign with $\theta$, $V^*$ only depends on r, there exists ordering of $V^*$'s : all go hand-in-hand \textcolor{blue}{26/Feb/25 needs to be checked?}} 
\tb{Base Case}  \\ By definition, $V^*_0 = 0$. \\
Take any $s \in \mathcal{S}_{n,1}$. \\
\tb{Q.} What is $a^*$? \\
For s, only possible next global states are s itself and all-at-goal (g). This is akin to the single agent problem. But any transition probability also depends on actions of others. \\
Suppose $p^a_{s,g}$ denotes the transition probability from s to g. Then we have, \\
$V_1(s) = (1-p^a_{s,g}).(1+V_1(s)) + p^a_{s,g}.(1+V_0) \implies V_1(s) = \frac{1}{p^a_{1,0}}$ \\
Thus the optimum action at s is the one that minimizes $V_1(s)$ i.e., maximizes $p^a_{s,g}$. From the above general equation (line 177), the transition probability is maximum when $a$ is such that it matches all signs with $\theta$ for the respective components of agent who was initially at s. The signs of other components do not matter. Hence there could be multiple $a^*$ for any particular $s \in \mathcal{S}_{n,1}$. \\
Notice that this will hold true for any $s \in \mathcal{S}_{n,1}$. Note that particular $a^*$ whose sign matches with components of $\theta$ (for every agent), is common for possible $a^*$ for every $s \in \mathcal{S}_{n,1}$. We consider this $a^*$ in particular. \\
Since from the general formula, for a fixed instance ($\theta$), for a given action the probability only depends on r and r', it is the same for all states s $\in \mathcal{S}_{n,1}$ i.e., $p^{a^*}_{s,g} = p^{a^*} \forall s \in \mathcal{S}_{n,1}$. This $V^*_1(s) = V^*_1 \forall s \in \mathcal{S}_{n,1}$ \\
Since transition probability for this action is strictly between 0 and 1, $V^*_1 > V^*_0=0$ \\
\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:\\ $a^*$ is the one that matches sign with $\theta$ for any state in $\mathcal{S}_{n,k}$, hence $p^*(s \in \mathcal{S}_{n,k}  \xrightarrow{}s' \in \mathcal{S}_{n,k'}(s)) = p^*_{k,k'}$, $V^*_k(s)=V^*_k$ for any $s \in \mathcal{S}_{n,k}$ and $V^*_k>V^*_{k-1}$. Now, we need to show the same for $r+1$. \\
Consider any $s \in S_{n,r+1}$. \\
$V^a(s) = \sum_{s' \in \mathcal{S}(s)\textbackslash \{s,g\}} P(s'|s,a)\{1+V^*(s')\} + P(s|s,a).\{1+V^a(s)\} + P(g|s,a).\{1+V^*(g)\}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +\sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} p^a_{r+1,r'}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \sum_{i \in [n]} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r'}  - \binom{r}{r'-1} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Big  \}$ \\ 
Observe that the third term is always non negative since when $r'>r/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} >V^*_r$ while for $r' \leq r/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_r$. Note that the above arguments is for $r' \in [r]$. To minimize $V^a(s)$, we need to minimize $P(s|s,a)$ as well (check after rearrangement as it will appear in denominator as 1-P). Clearly, the action that matches sign with all components of $\theta$ minimizes $V^a(s)$. Hence this is $a^*$. Notice the above arguement holds for any $ s \in \mathcal{S}_{n,r+1}$. Hence $a^*$ is the same for each of them. Hence $p^*(s \in \mathcal{S}_{n,r+1} \xrightarrow{}s' \in \mathcal{S}_{n,r'}(s)) = p^*_{r+1,r'}$. Hence $V^*(s) = V^*_{r+1}$ for each of them. \\
Proving $V^*_{r+1} > V^*_r$ is tricky. The assumption of $P(.|s,a^*)$ in above theorem will make this work. 
\\ \\
\tb{Claim:} Suppose probabilities are such that for any $s \in \mathcal{S}_{n,r+1}$ and $s' \in \mathcal{S}_{n,r}(s)$ for any $r' \in \{0,1,2,\dots, r\}$, $\binom{r+1}{r'}.p^*_{r+1,r'}<\binom{r}{r'}.p^*_{r,r'}$. Then, assuming $V^*_{r}>V^*_{r-1}>\dots>V^*_2>V^*_1>V^*_0=0$, it can be shown that $V^*_{r+1}>V^*_{r}$ for any $r \in \{0,1,\dots, n-1\}$ \\
\textcolor{red}{to make this condition to hold I may have to slightly modify the features or show that this condition exists for current features. if i modify features, i need to be careful since $a^*$ may change possibly differing for every state.} \\

$V^*_r = 1 +\sum_{r'\in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'}V^*_{r'}$ \\
$V^*_{r+1} = 1+ \sum_{r' \in \{0,1,\dots,r+1\}} \binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} $ \\ 

\\
Suppose for every $r' \in \{0,1,2,\dots,r\}$, let $\binom{r+1}{r'}.p^*_{r+1,r'} = \binom{r}{r'}.p^*_{r,r'} - \delta_{r'}$ where $\delta_{r'} > 0$ for every $r'$. Note, $\sum_{r' \in \{0,1,2,\dots,r+1\}}\binom{r+1}{r'}p^*_{r+1,r'} \\= 1 \implies \binom{r+1}{r+1}p^*_{r+1,r+1} = 1-\sum_{r' \in \{0,1,2,\dots,r\}}\binom{r+1}{r'}p^*_{r+1,r'} \\= 1 - \sum_{r' \in \{0,1,\dots,r\}}(\binom{r}{r'}p^*_{r,r'} - \delta_{r'}) = 1-\sum_{r' \in \{0,1,2,\dots,r\}}p^*_{r,r'} + \sum_{r' \in  \{0,1,2,\dots,r\}} \delta_{r'} \\= \sum_{r' \in  \{0,1,2,\dots,r\}} \delta_{r'}$ \\
Now, back to $V^*_{r+1}$. \\
$V^*_{r+1} = 1 + \binom{r+1}{r+1}p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} \\= 1+\binom{r+1}{r+1}p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}} (\binom{r}{r'}p^*_{r,r'} - \delta_{r'})V^*_{r'} \\= 1+\binom{r+1}{r+1}p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - \sum_{r' \in \{0,1,\dots,r\}} \delta_{r'}V^*_{r'} \\>  1+\binom{r+1}{r+1}p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - \sum_{r' \in \{0,1,\dots,r\}} \delta_{r'}V^*_{r} $ (due to monoticity of $V^*$). \\
Thus, \\
$V^*_{r+1}  >  p^*_{r+1,r+1}V^*_{r+1} + 1+ \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - p^*_{r+1,r+1} V^*_{r} \\= p^*_{r+1,r+1}(V^*_{r+1}-V^*_r) + V^*_{r} \implies (1-p^*_{r+1,r+1}).(V^*_{r+1}-V^*_r) > 0 $ \\ Since $1>p^*_{r+1,r+1} >0$, we have $V^*_{r+1} > V^*_r$. \\
Hence by induction, $ a^* $ is same as the one that matches sign with each component of $\theta$, for every state $s \in \mathcal{S}$, $p^*(s \in \mathcal{S}_{n,r} \xrightarrow{}s' \in \mathcal{S}_{n,r'})$ only depends on $r$ and $r'$, $V^* $ is the same for all states of the same type. Hence $V^*(s)$ for any $s \in \mathcal{S}_{n,r}$ only depends on $r$. Further, under the monotonicity of $p^*$, $V^*$ are ordered monotonically increasing in r.
\\ \\
Proving $V^*_{r+1} > V^*_r$ is tricky. We will make a suitable assumption on probabilities and later show that it holds under suitable choices of $\delta$ and $\Delta$. \\
\tb{Claim} If for every $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.  \\
We will justify that the assumption on probabilities in this claim holds for our features under suitable $\delta$ and $\Delta$. For now lets assume this holds for our case and prove the implication part of claim. \\
Return to the induction argument. \\
$V^*_r = 1+\sum_{r' \in \{0,1,\dots,r\}}\binom{r}{r'}V^*_{r'}$ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'}$ \\
Suppose for every $r' \in \{0,1,2,\dots,\lfloor\frac{r+1}{2}\rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}-\delta_{r'} $ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor\ +1 , \lfloor\frac{r+1}{2}\rfloor+2,\dots,r-1,r\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}+\delta_{r'} $ where $\delta_{r'}>0$ for every $r' \in \{0,1,\dots,r\}$\\ 
Note that, $\sum_{r' \in \{ 0,1,\dots,r,r+1\}} \binom{r+1}{r'}p^*_{r+1,r'} = 1 \\ \implies \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r+1}{r'}p^*_{r+1,r'} + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r+1}{r'}p^*_{r+1,r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} (\binom{r}{r'}p^*_{r,r'}-\delta_{r'}) + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} (\binom{r}{r'}p^*_{r,r'} + \delta_{r'}) + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies  \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r}{r'}p^*_{r,r'}-\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + 1 -  \sum_{r' \in \{0,1,\dots,r-1,r} \binom{r}{r'}p^*_{r,r'} \\ \implies p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} $ \\ \\
Now, going back to $V^*_{r+1}:$ \\ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}(\binom{r}{r'}p^*_{r,r'} - \delta_{r'})V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}(\binom{r}{r'}p^*_{r,r'}+\delta_{r'})V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} V^*_{r'}+ \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, r-1,r\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\=  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ > p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{\lfloor \frac{r+1}{2} \rfloor + 1}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  (  \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} - \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}  )V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ >  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r $ \\ 
Thus,\\
$V^*_{r+1} >   p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r \implies (1-p^*_{r+1,r+1})(V^*_{r+1}-V^*_r)>0 \implies V^*_{r+1} > V^*_r$ \\
Above inequalities used monotonicity of $V^*$ due to induction assumption. \\
Below we justify that the assumption in the above claim holds for our case.
\subsubsection{Justification of assumption} \\
Recall that in the above claim, we assumed that: for every $r \in [n-1],$ for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$. \\
Below, we will derive sufficient conditions on $\delta$ and $\Delta$ such that this assumption holds. \\
Also note that from below section we have $\delta<0.5$ and $\delta>3.2^{n-1}\Delta$ so that all probabilities are well defined.
\\ \\
\tb{For $r'\leq \lfloor\frac{r+1}{2}\rfloor$}, \\
$\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \frac{r+1}{r+1-r'}p^*_{r+1,r'}<p^*_{r,r'} \Leftrightarrow \\(r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \\ \Leftrightarrow  (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \\ \impliedby (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \Leftrightarrow \frac{\Delta}{n}\frac{r^2}{8} + (r+1) \frac{\Delta}{n}<(r+1)\frac{1-2\delta}{n2^{r+1}} \Leftrightarrow \frac{\Delta}{n}(\frac{r^2}{8}+r+1)<(r+1)\frac{1-2\delta}{n2^{r+1}} \impliedby \Delta (\frac{n^2}{8}+n+1)<\frac{1-2\delta}{2^{n}} \Leftrightarrow \Delta < \frac{1-2\delta}{2^{n}(1+n+\frac{n^2}{8})}$ \\ \\
Similarly, \\ \tb{For $r' > \lfloor \frac{r+1}{2} \rfloor$}, \\ 
$\binom{r+1}{r'}p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \\ \frac{r+1}{r+1-r'}p^*_{r+1,r'}>p^*_{r,r'} \Leftrightarrow \\ (r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow \\ (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \Leftrightarrow \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow  \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0  \impliedby  (\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0 \\ \Leftrightarrow \frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2) - 0.5(r+1)(\frac{1-2\delta}{n.2^{r}}) >0 \\ \Leftrightarrow \frac{(r'-r-0.5)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2)  >0 \impliedby \frac{(-r-0.5)(1-2\delta)+0.5n }{n.2^{r}}   >   \frac{\Delta}{n}  (r^2-r-1)  \Leftrightarrow \frac{(-r-0.5)(1-2\delta)+0.5n }{1}   >   \frac{\Delta}{1}  (r^2-r-1)  (2^{r}) \\ \impliedby (-n-0.5)(1-2\delta)+0.5n    >   \Delta  (n^2-n-1)  (2^{n})$ and $ (-n-0.5)(1-2\delta)+0.5n    > 0 \\ \impliedby 0.5n-n+2n\delta-0.5+\delta>0$ and $ 0.5n-n+2n\delta-0.5+\delta >   \Delta  (n^2-n-1)  (2^{n}) \\ \impliedby (2\delta-0.5)n>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2-n-1)  (2^{n}) \\ \impliedby 2\delta-0.5>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2-n-1)  (2^{n}) \\ \Longleftrightarrow \delta>\frac{1}{3}$ and $n > \frac{0.5-\delta}{2\delta-0.5}+ \frac{\Delta  (n^2-n-1)  (2^{n})}{2\delta-0.5} \\ \impliedby \delta>1/3 $ and $\Delta  (n^2-n-1)  (2^{n})<3\delta-1 \impliedby \Delta < \frac{3\delta-1}{(n^2-n-1).2^{n}}$ \\ The last second condition is trivially satisfied for n=1. Otherwise use the condition on $\Delta$.
\\
Finally we obtain for the desired instance, fix $1/2>\delta>1/3$. Then, fix, $\Delta< 2^{-n}.min\{\frac{3\delta-1}{n^2-n-1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2/8}\}$




\subsubsection{Sufficient conditions on $\delta$ and $\Delta$ for well defined probabilities}

$p^a_{r,r'} < 1$ for every $r \in \{1,2,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$. \\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  <   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{1} <   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{\frac{n-r}{2}}{n2^{r-1}}        +    3\Delta  =  \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} +    3\Delta =  \frac{(r'-0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} +    3\Delta < \frac{0.5n(2-2\delta)}{n.2^{r-1}} + 3\Delta  < 1-\delta + 3\Delta$ \\
To ensure $p^a_{r,r'}<1$ it is sufficient to ensure $1-\delta + 3\Delta<1 \implies \delta > 3\Delta$ \\
Similarly, we must ensure, $p^a_{r,r'} > 0$ for every $r \in \{0,1,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$. \\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  > \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') -  \frac{2 \Delta}{1} > \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} - 3\Delta > \frac{(r' -0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta > \frac{( -0.5n)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta = \frac{ \delta }{2^{r-1}} - 3\Delta$ \\
To ensure, $p^a_{r,r'} > 0$ it is sufficient to ensure $ \frac{ \delta }{2^{r-1}} - 3\Delta > 0  \implies \delta > 3.2^{n-1}.\Delta$. \\ Observe that since $n \geq1$, condition from $p>0 \implies $ condition from $p<1$  Also note that in the above, we have assumed $\delta < 0.5$. Hence we can fix any $\delta, \Delta $ and $n$ that satisy the above conditions in order to fix a class of instance as above.

\section{Try product based features \textcolor{blue}{3/3/2025}} 
Assume the following (top-down) probability model: \\
At any state $s \in \mathcal{S}$, it holds that, for any agent $i \in [n]$, \\
$P(s_i^\prime=g|s_i=s,a) = \langle a, \theta \rangle + \delta$, \\
$P(s_i^\prime=s|s_i=s,a) = \langle -a, \theta \rangle + 1- \delta$ \\
$P(s_i^\prime=g|s_i=g,a) = 1$, \\
$P(s_i^\prime=s|s_i=g,a) = 0$ \\
\\
Note that for a fixed instance, for a fixed global action, transition probabilities are same for all agents at $s_{init}$. For those at $goal$ too they are trivially same (hard constraint).
\\
For these to be well defined for all instances in our analysis, we want that \\ $1 > max_{a,\theta}  \langle a, \theta \rangle + \delta = \delta+\Delta> min_{a,\theta} \langle a, \theta \rangle + \delta = \delta - \Delta >0 \implies 1> \delta+\Delta, \delta>\Delta $ \\
Similarly, we want \\
$1>  max_{a,\theta}\langle -a, \theta \rangle + 1- \delta = 1+\Delta-\delta>min_{a,\theta}  \langle -a, \theta \rangle + 1- \delta=1-\delta-\Delta >0 \implies \delta>\Delta, 1>\delta+\Delta$ (same conditions as above. note $\delta, \Delta >0$) \\These ensure that probability for general transition are well-defined. 

\\
\tb{Expression for a general transition}\\
Consider state $s \in \mathcal{S}_{n,r}$ for some $r \in \{1,2,\dots,n\}$. For any $r' \in \{0,1,\dots,r\}$, take any $s' \in \mathcal{S}_{n,r'}(s)$. Let s be such that agents in $\mathcal{I}:=\{i_1,i_2,\dots,i_r\}$ are at $s_{init}$ and those at indices in $\mathcal{J}:=\{j_1,j_2,\dots,j_{n-r}\}$ are at $goal$. Let the agents in $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ be the ones transiting to $goal$ during transition of global state from $s$ to $s'$. Then, \\ $P(s'|s,a) = \{\Pi_{t \in \mathcal{T}} p(s_t^\prime =g|s_t=s_{init},a)\} . \{\Pi_{i \in \mathcal{I}-\mathcal{T}}p(s'_i=s|s_i=s_{init},a)\}.\{\Pi_{j \in \mathcal{J}}p(s'_j=g|s_j=g,a)\} = \{ \langle a, \theta \rangle + \delta\}^{r-r'} . \{\langle -a, \theta \rangle + 1- \delta\}^{r'}.\{1\}^{n-r} $ \\
Notice  that the above expression remains the same for any $s' \in \mathcal{S}_{n,r'}(s)$. The above argument holds for any $s \in \mathcal{S}_{n,r}$ for any fixed a. \\ We will denote this as $p^a_{r,r'}$ (later we will show that the optimal action at all states is the same hence represent $p^*_{r,r'}$ for optimal action/policy). \\
\tb{The general proof} \\
Base case : r=0\\
Consider any $s \in \mathcal{S}_{n,1}$. Let the $i-th$ agent be at $s_{init}$ and all others at $goal$. Suppose global action a is taken. Then,
$V^a_1(s) = p^a_{1,0}(1+V_0) + p^a_{1,1}(1+V^a_1) = 1 + (1-p^a_{1,0})V^a_1 \implies V^a_1(s) = \frac{1}{p^a_{1,0}}$ \\
Clearly the best action at $s$ is the one that minimizes $V^a_1(s)$ i.e., maximizes $p^a_{1,0}$. From the above general expression this is the one that matches sign with all components of $\theta$. Since the above argument is true for any $s \in  \mathcal{S}_{n,1}$, $a^*$ is the same as the one that matches all signs with $\theta$ for all $s \in \mathcal{S}_{n,1}$ and we can see that since probability depends on only r and r' for given global action for a given instance, $V^*(s) = constant = V^*_1$ for all $s \in \mathcal{S}_{n,1}$. Also by definition, $V^a_0 = 0$. Thus, $V^*_0 = 0 < V^*_1$. \\ \\
Now assume that, for every $k \in [r]$, it holds that, 
\item $a^*(s) = a^*=$ same as the one matching all signs with $\theta$, for every $s \in \mathcal{S}_{n,k}$ 
\item $V^*(s) = V^*_k$ for every $s \in \mathcal{S}_{n,k}$ 
\item $V^*_k > V^*_{k-1}$ \\ \\
We need to show that the above is true for $'r+1'$ as well. Now consider any $s \in \mathcal{S}_{n,r+1}$ and $s_r \in \mathcal{S}_{n,r}(s)$\\
$V^*(s_r) = V^*_r = 1+ \sum_{r'\in \{0,1,\dots,r\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'}$ here, we know what the optimal action is \\
$V^*(s) = 1+ \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^*_{s,r'}V^*_{r'} + p^*_{s,s}V^*(s) = 1+p^*_{s,s}V^*(s) + \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^*_{s,r'}V^*_{r'} $ here we do not know what the optimal action is but whatever it is we can write the expression.\\

We will use the following result (this gives us condition on parameters): \\
We want that for every action $a$ in $s$, $\binom{r+1}{r'}p^a_{s,r'}<\binom{r}{r'}p^*_{r,r'}$ for every $r' \in \{0, [r]\}$ for every $r \in [n-1]$. \\
Thus,  $\frac{r+1}{r+1-r'}p^a_{s,r'}<p^*_{r,r'}  \impliedby \frac{r+1}{r+1-r'} (p^a)^{r+1-r'}(1-p^a)^{r'} < (p^*)^{r-r'}(1-p^*)^{r'} \impliedby \frac{r+1}{r+1-r'} (p^*)^{r+1-r'}(1-p^*)^{r'} < (p^*)^{r-r'}(1-p^*)^{r'} \impliedby \frac{r+1}{r+1-r'} p^* < 1 \impliedby p^* < \frac{1}{n}$ \\
In the above we used a claim that for any $r \in [n-1]$, for every $r' \in \{0, [r]\}$, for any global action $a$, $(p^a)^{r+1-r'}.(1-p^a)^{r'} < (p^*)^{r+1-r'}.(1-p^*)^{r'}$ where $p^*$ denotes success probability at $a^*:$one with all signs matched with $\theta$. For this to hold, it is sufficient to show that $f_{r,r'}(p):=p^a_{s,r'}=(p)^{r+1-r'}(1-p)^{r'}$ is increasing function with $p$ for every $r' \in \{0, [r]\}$ for all $r \in [n-1]$ \\
$f_{r,r'}'(p) = (r+1-r')(p)^{r-r'}(1-p)^{r'}-(p)^{r+1-r'}r'(1-p)^{r'-1} > 0 \impliedby (r+1-r')(1-p)>p.r' \impliedby (1-p)>p.r \impliedby \frac{1}{p} - 1 > n-1 \impliedby p < \frac{1}{n} \impliedby \delta + \Delta < \frac{1}{n}$
\\
We enforce that $\delta + \Delta < \frac{1}{n}$ so that the above result hold to use it as below. \\
Suppose for every $r' \in \{0,1,2,\dots,r\}$, let $\binom{r+1}{r'}.p^*_{s,r'} = \binom{r}{r'}.p^*_{r,r'} - \delta_{r'}$ where $\delta_{r'} > 0$ for every $r'$  \\

\\
Note, $\sum_{r' \in \{0,1,2,\dots,r+1\}}\binom{r+1}{r'}p^*_{s,r'} = 1 \\ \implies p^*_{s,s} = 1-\sum_{r' \in \{0,1,2,\dots,r\}}\binom{r+1}{r'}p^*_{s,r'} \\= 1 - \sum_{r' \in \{0,1,\dots,r\}}(\binom{r}{r'}p^*_{r,r'} - \delta_{r'}) = 1-\sum_{r' \in \{0,1,2,\dots,r\}} \binom{r}{r'} p^*_{r,r'} + \sum_{r' \in  \{0,1,2,\dots,r\}} \delta_{r'} \\= \sum_{r' \in  \{0,1,2,\dots,r\}} \delta_{r'}$ \\
Now, back to $V^*(s)$. \\
$V^*(s) = 1+ p^*_{s,s}V^*_{s} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^*_{s,r'}V^*_{r'} \\= 1+p^*_{s,s}V^*_{s} + \sum_{r' \in \{0,1,\dots,r\}} (\binom{r}{r'}p^*_{r,r'} - \delta_{r'})V^*_{r'} \\= 1+p^*_{s,s}V^*_{s} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - \sum_{r' \in \{0,1,\dots,r\}} \delta_{r'}V^*_{r'} \\> 1+ p^*_{s,s}V^*_{s} + \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - \sum_{r' \in \{0,1,\dots,r\}} \delta_{r'}V^*_{r} $ (due to monoticity of $V^*$). \\
Thus, \\
$V^*(s)  >  1+p^*_{s,s}V^*(s) + \sum_{r' \in \{0,1,\dots,r\}} \binom{r}{r'}p^*_{r,r'} V^*_{r'} - p^*_{s,s} V^*_{r} \\= p^*_{s,s}(V^*(s)-V^*_r) + V^*_{r} \implies (1-p^*_{s,s}).(V^*(s)-V^*_r) > 0 $ \\ Since we will ensure $1>p^a_{s,s} >0$, we have $V^*(s) > V^*_r$. \\
Thus, clearly $V^a (s) \geq V^*(s) > V^*_r> V^*_{r-1}>\dots>V^*_1>V^*_0 = 0$
\\
\\
$V^a(s) = \sum_{r' \in \{0,1,\dots,r\}} \binom{r+1}{r'}p^a_{s,r'}V^*_{r'} + p^a_{s,s}V^a(s)  $ \\
Notice that if there exists an action that uniformly maximizes the probability $p^a_{s,r'}$ for all $r' \in \{0,[r]\}$, then it is optimal. This is due to monotonicity of $V's$ and positive coefficients and allotment of probabilities. We claim that this is the same as $a^*:$ the one that matches sign with all components of $\theta$. The justification is that in an above claim, we showed that, for every $r' \in  [r]$, $p^a_{s,r'}$ is an increasing function of success probability for our instances $\delta + \Delta < 1/n$. And, the success probability is maximized when action is $a^*:$ one that matches signs with components of $\theta$.  \\
Notice that the same argument can be given for any $s \in \mathcal{S}_{n,r+1}$ Thus, $a^*$ is same for all these states. Hence, $p^*_{s,r'} = p^*_{r+1,r'}$ for all $s \in \mathcal{S}_{n,r+1}$ as for the same action and $\theta$ it only depends on r+1 and $r'$. Thus $V^*(s) =V^*_{r+1}$ for all $s \in \mathcal{S}_{n,r+1}$ \\
Hence, we have showed that:
\item $a^*$ is same for all states $s \in \cup_{k=\{0,1,\dots,r+1\}} \mathcal{S}_{n,k}$ 
\item $V^*(s) = V^*_{r+1}$ for all $s \in \mathcal{S}_{n,r+1}$
\item $V^*_{r+1} > V^*_r>V^*_{r-1}>\dots>V^*_1>V^*_0=0$
Thus this holds true by induction that :
\item The optimal policy is that at every state, one takes the same action namely the one that matches sign with all components of $\theta$
\item Optimal value for states of the same type is the same
\item States with more agents at $s_{init}$ have strictly higher values(long term costs) than the one with lower number of agents at $s_{init}$

\subsubsection{Working on Lower Bound}

Suppose in episode \textit{k}, agents take actions according to policy $\pi$. Let, $\tb{s}_t$ represent the global state and $\tb{a}_t$ the global action at time $t$. Then, the expected regret for the \textit{k-th} episode is:
\begin{align}
    R_{\theta,k} &= V^{\pi_\theta}(\tb{s}_1) - V^*(\tb{s}_1) 
    \\
    &=  V^{\pi_\theta}(\tb{s}_1) - \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) 
    \\ 
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^\pi(\tb{s}_2)]\}  
    \\ 
    & \quad -\mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^*(\tb{s}_2)] \} + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim\ \pi(\tb{s}_1), \tb{s}_2 \sim\ \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi}(\tb{s}_2) - V^*(\tb{s}_2)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1)
\end{align}
\begin{align} 
    & \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q^{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ c(\tb{s}_1,\tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)] \} - V^{\pi^*}(\tb{s}_1) \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim   \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - V^{\pi^*}(\tb{s}_1) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - (1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)]) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{  \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)] \}
    \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} \{ \sum_{\tb{s} \in \mathcal{S}} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*)) V^{\pi^*}(\tb{s})\}
\end{align}

$
 \sum_{\tb{s} \in \mathcal{S}} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*))V^*(\tb{s})  = (\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*))V^*_n + \sum_{\tb{s} \in \mathcal{S} \textbackslash\tb{s}_1} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*))V^*(s) 
$\\
Remember we proved earlier that $\mathbb{P}(s|s_1,a_1) = \binom{n}{n-r'}(p^a)^{n-r'}(1-p^a)^{r'}$ is maximised at $a = a^*$ for all $r' \in \{0\} \cup [n-1]$. Hence, the second term above consists of summation of negative terms and can be lower bounded as follows:
\\$\sum_{s \in \mathcal{S}}(\mathbb{P}(s|s_1,a_1) - \mathbb{P}(s|s_1,a_1^*))V^*(s) = (\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*))V^*_n + \sum_{\tb{s} \in \mathcal{S} \textbackslash\tb{s}_1} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*))V^*(s) > (\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*))V^*_n + \sum_{\tb{s} \in \mathcal{S} \textbackslash\tb{s}_1} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*))V^*_{n-1} = (\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*))V^*_n +  (1 - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - (1-\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*)))V^*_{n-1} = (\mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*))V^*_n +  ( \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1^*) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) )V^*_{n-1} =  ( \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}_1|\tb{s}_1, \tb{a}^*_1) ) . (V^*_n - V^*_{n-1}) = ((p^a_{n,n})^n-(p^*_{n,n})^n) . (V^*_n - V^*_{n-1})  = (p^a_{n,n}-p^*_{n,n})((p^a_{n,n})^n + (p^a_{n,n})^{n-1}.p^*_{n,n}+\dots+(p^a_{n,n}).(p^*_{n,n})^{n-1} + (p^*_{n,n})^n ) . (V^*_n - V^*_{n-1}) >  (p^a_{n,n}-p^*_{n,n}) (p^*_{n,n})^n .n . (V^*_n - V^*_{n-1})  $ \\
Note that, $p^a_{n,n} = 1- \delta - \sum_{i = 1}^n \sum_{p=1}^{d-1} a_{i,p}.\theta_{i,p} = 1-\delta-\sum_{i = 1}^n \sum_{p=1}^{d-1} \frac{\Delta}{n(d-1)} (\mathbbm{1}\{sgn(a_{i,p})=sgn(\theta_{i,p}\}-\mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\})  = 1-\delta-\sum_{i = 1}^n \sum_{p=1}^{d-1} \frac{\Delta}{n(d-1)} (1-2.\mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}) = 1-\delta-\Delta + \sum_{i = 1}^n \sum_{p=1}^{d-1} \frac{2.\Delta}{n(d-1)} (\mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\})$ \\
Thus, $p^a_{n,n} - p^*_{n,n} = \sum_{i = 1}^n \sum_{p=1}^{d-1} \frac{2.\Delta}{n(d-1)} (\mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\})$
\\
Therefore, 
\\$\sum_{s \in \mathcal{S}}(\mathbb{P}(s|s_1,a_1) - \mathbb{P}(s|s_1,a_1^*))V^*(s) >  (p^a_{n,n}-p^*_{n,n}) (p^*_{n,n})^n .n . (V^*_n - V^*_{n-1}) \\= (1 - \delta -\Delta)^n .n . (V^*_n - V^*_{n-1}) \sum_{i = 1}^n \sum_{p=1}^{d-1} \frac{2.\Delta}{n(d-1)} (\mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\})   $
\\
\textcolor{red}{We abandon this model since monotonicity of V has been established for earlier model and features}
\subsection{Results to use in Lower bound proof 9-3-25}
$V^*_r = 1 +  p^*_{r,r} . V^*_r +\sum_{r'=1}^{r-1} \binom{r}{r'} p^*_{r,r'}.V^*_{r'} < 1+p^*_{r,r}V^*_r + (1-p^*_{r,r})V^*_{r-1} \Leftrightarrow V^*_r-V^*_{r-1}<\frac{1}{1-p^*_{r,r}}$ \\
Thus, \\
$V^*_n - V^*_{n-1} < \frac{1}{1-p^*_{n,n}} \\ V^*_{n-1}-V^*_{n-2}<\frac{1}{1-p^*_{n-1,n-1}}\\ &\vdots \\ V^*_{2}-V^*_1 < \frac{1}{1-p^*_{2,2}} \\ V^*_1 - V^*_0 = \frac{1}{1-p^*_{1,1}}$ \\
Adding the above, \\
$V^*_n - V^*_0 \leq \sum_{i=1}^n\frac{1}{1-p^*_{i,i}} \leq \frac{n}{1-p^*_{1,1}} = nV^*_1 \implies B^*/n \leq V^*_1$ \\
Observe that equality holds for $n=1$



\newpage
\section{\textcolor{blue}{11-3-24 } Everything Below is to be verified. I have removed some of earlier comments and sections that are no longer useful. Ive also changed the order of different sections for flow}


\section{Introduction}
\label{sec:intro}

\pt{
\begin{itemize}
    \item What are the major to-do things. \textcolor{red}{simplify kl-divergence term (see the last section), fix issues with MACCM if time permits and redo experiments} 
    \item What is the story of the entire paper. \textcolor{red}{for me, it will depend on what results are obtained, so far there's no important complete result, so can't say much}
    \item Let us start writing the paper formally. There are lot of things to do. \textcolor{red}{in my opinion, lets get at least 2 key results first, so far we have none. in fact lets concentrate completely on simplifying the kl divergence term, i'm stuck on this for a week now and it is quite non-trivial, once this is done i can move to computations part }
    \item I need some more clarity on what are the major things pending before I can start writing the paper.
    \item What are the major results? What are other results we are still aiming at, and where are we stuck? \textcolor{red}{so far there's no key complete result}
    \item What is the status of the experiments. \textcolor{red}{Cant use MACCM before resolving the issues, also haven't finished yet with lower bound proof}
    \item We need to finalize the results before we write the paper. 
    \item Let me write the story of the paper.
\end{itemize}
}


\subsection{Story of the paper.}

\pt{
\begin{itemize}
    \item Single agent SSP is a well known problem.
    \item The RL version of the SSP has become very popular recently. 
    \item The upper and lower bounds are proved.
    \item \cite{trivedi2023massp} has recently extended from the single agent to multi-agent SSP.
    \item The regret upper bounds are derived for the MA-SSP version.
    \item However, the lower bounds are majorly missing in the literature.
    \item Also, the role of number of agents in the multi-agent setup is another important missing factor in the literature.
    \item In this paper we explore two important aspects -- the regret lower bounds and the role of number of agents in the MA-SSP setup regret bounds.
    \item To the best of our knowledge, this is the first paper addressing the above missing problems in the literature. 
    \item We prove a matching lower bounds for the MA-SSP paper. \\ \textcolor{red}{for now it looks ok}
\end{itemize}
}

Our major contributions are as follows:

\begin{itemize}
    \item \textbf{Analysis wrt Number of Agent}
    \item \textbf{Experiments}
\end{itemize}

\input{Sections/6_experiments}


\subsection{Proof of Lower Bound}

\pt{Need to write this thing cleanly with proper justifications. Why the following makes sense, and how would this capture the hardest instance. What is the role of congestion in this example?}

We construct and analyze a family of hard to learn instances. This is the same as in section 1.1. Further, we restrict $\theta$ such that $\theta_{i} \neq \theta_{j}$ $ \forall$ $ i \neq j \in [n]$ i.e., no two $\theta_i$ are the same. Let this set be denoted as $\Theta$. \pt{Why this assumption will hold. there is lot of symmetry in the problem, so $\theta$'s for two agents will be same?}. \textcolor{blue}{It's not an assumption. It's a restriction of the class of SSPs instances I'm considering. I'm free to do so. Why I do this is the rest of paragraph about. Also $\theta$ is an instance parameter, it can be anything. A way to think about this is that : even if two agents took same action, the contribution to probability of transition to any global state is not the same, this is one way how agents are not identical!} This ensures that the action to be taken by each agent to maximize the probability of transition to the all-at-goal state is different for every agent so that we don't need to consider the congestion component of the cost when the policy of maximizing the probability to reach all-goal is executed.
To further reduce complexity of the analysis, we let the private cost associated with any action in the initial state be equal to 1 and that in goal state equal to 0. This ensures that the \textit{best} policy is the one that maximizes the probability of transition to the global goal \pt{goal?} \textcolor{blue}{yes, thanks!} state.  \\
Suppose in episode \textit{k}, agents take actions according to policy $\pi$. Let, $\tb{s}_t$ represent the global state and $\tb{a}_t$ the global action at time $t$. Then, the expected regret for the \textit{k-th} episode is:

\pt{In the regret definition below the policy seems to have the parameters $\theta$, whereas we have originally used $\theta$ as the parameters for the transition probabilities?} \textcolor{red}{yes, we are analyzing regret of a class of instances simultaneously defined by \theta. $\pi_{\theta}$ represents the policy learned for instance defined by $\theta$. In the below everywhere $\pi ==\pi_{\theta}$. I need to update it. In fact more accurately it must be $\pi_{\theta,k}$ since the learned policy differs every episode.} 

\begin{align}
    R_{\theta,k} &= V^{\pi_\theta}(\tb{s}_1) - V^*(\tb{s}_1) \label{regret}
    \\
    &=  V^{\pi_\theta}(\tb{s}_1) - \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) 
    \\ 
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^\pi(\tb{s}_2)]\}  
    \\ 
    & \quad -\mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^*(\tb{s}_2)] \} + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim\ \pi(\tb{s}_1), \tb{s}_2 \sim\ \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi}(\tb{s}_2) - V^*(\tb{s}_2)] + \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1)
\end{align}

\pt{Suggestion -- for each equation write the proper reason why it is true. This will make it easy to follow. For example, in above the second equation you added and subtracted $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] $.}
\textcolor{red}{Ok, I'll do it after I start revisiting them. Apart from adding and subtracting Q, I've only expanded the Bellman Equation}

\textcolor{red}{I'm stuck here to find a closed form expression of $Q^*(.,.)$ and $V^*$ due to exponential number of states}

\subsection{Some proofs I have been trying since Monday}
\subsubsection{}
\begin{align} 
    & \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q^{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ c(\tb{s}_1,\tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)] \} - V^{\pi^*}(\tb{s}_1) \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim   \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - V^{\pi^*}(\tb{s}_1) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - (1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)]) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{  \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)] \}
    \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} \{ \sum_{\tb{s} \in \mathcal{S}} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*)) V^{\pi^*}(\tb{s})\} \label{difference of probabilities}
\end{align}

\\
The above just follows from writing the definition of optimum Action value function and doing some rearrangement and remember costs throughout is 1.
\\

In the below proof, we expand the difference in probability term arising in the above equation. The initial global state, $s_1$, is with all agents at $s_{init}$ and the next state, $s$, is one where agents $i_1,i_2,..,i_r$ remain at $s_{init}$ and those at $j_1,j_2,..,j_{n-r}$ go to goal node. \\


\begin{lalign}
\mathbb{P}(s|s_1, a_1) - \mathbb{P}(s|s_1, a_1^*)  
\\
&= \langle \phi(s|s_1,a_1), \theta \rangle - \langle \phi(s_1|s_1,a_1^*), \theta \rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1), \phi(s_2^{\prime}|s_2, a_2)..., \phi(s_n^{\prime}|s_n,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\& - \langle (\phi(s_1^{\prime}|s_1, a_1^*), \phi(s_2^{\prime}|s_2, a_2^*)..., \phi(s_n^{\prime}|s_n,a_n^*)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1),..., \phi(s_n^{\prime}|s_n,a_n)) - (\phi(s_1^{\prime}|s_1, a_1^*),..., \phi(s_n^{\prime}|s_n,a_n^*)), \\
& (\theta_1, 1,...,\theta_n,1)\rangle 
\\
&= \sum_{m = 1}^{r} \langle \phi(s_{i_m}^{\prime}|s_{i_m},a_{i_m}) - \phi(s_{i_m}^{\prime}|s_{i_m},a^*_{i_m}), (\theta_{i_m}, 1)\rangle \\ 
& + \sum_{m = 1}^{n-r} \langle \phi(s_{j_m}^{\prime}|s_{j_m},a_{j_m}) - \phi(s_{j_m}^{\prime}|s_{j_m},a^*_{j_m}), (\theta_{j_m}, 1)\rangle 
\\
&= \sum_{m=1}^{r} \langle (-a_{i_m} + a^*_{i_m}, 0), (\theta_{i_m}, 1) \rangle + \sum_{m=1}^{n-r} \langle (a_{j_m}-a^*_{j_m}, 0), (\theta_{j_m}, 1) \rangle   
\\
&= \sum_{m=1}^{r} (\langle a^*_{i_m}-a_{i_m}, \theta_{i_m} \rangle)  + \sum_{m=1}^{n-r} (\langle a_{j_m}-a^*_{j_m}, \theta_{j_m}  \rangle)  
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1} (a^*_{i_m, p} - a_{i_m, p})\theta_{i_m, p} \} + \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1} (a_{j_m, p} - a^*_{j_m, p})\theta_{j_m, p} \}
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\} \}  - \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \}
\\
&= \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\}
\end{lalign}
\\
\\
The initial few lines use the linearity assumption and properties of inner product. Then, split the sum on $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Next lines use definition of $\phi(.,.)$ and $a^*$ as the one matching all signs with $\theta$. 
\\

\\



\subsubsection{}

\text{Probability that after taking a global action $\tb{a}$, the next global state is still the same as before i.e., $\tb{s}$}
\begin{lalign}
\mathbb{P}(\tb{s}|\tb{s}, \tb{a})
\\ Linearity Assumption\\
&= \langle \phi(\tb{s}|\tb{s},\tb{a}), \boldsymbol{\theta} \rangle
\\
$Expanded form of features$
\\
&= \langle (\phi(s|s, a_1), \phi(s|s, a_2)..., \phi(s|s,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\
$Definition of Inner Product$
\\
&= \sum_{i = 1}^{n} \langle (\phi(s|s, a_i),(\theta_i,1))
\\
$Definition of Features$
\\
&= \sum_{i = 1}^{n} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}),(\theta_i,1) \rangle
\\
&= \sum_{i = 1}^{n} \{ \langle -a_i, \theta_i \rangle + \frac{1-\delta}{n.2^{n-1}} \}
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \langle a_i, \theta_i \rangle 
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} a_{i,p}. \theta_{i,p} 
\\ $Definition of action and theta$\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Taking summation over p inside$ \\
&=  \frac{1-\delta}{2^{n-1}} - 
 \frac{\Delta}{n(d-1)} \sum_{i = 1}^{n}   \Big\{ d-1 - 2 \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Just simplify$ 
\\
&=  \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
\end{lalign}

\subsubsection{}
\\
In this subsection we derive the expression of Probability that if at state $\tb{s} = \{s_{init}, s_{init}, \dots, s_{init}\}$, if global action $\tb{a} = (a_1,a_2,\dots, a_n)$ is taken, you reach $\tb{s}^{\prime}$ where the agents at indices in $\mathcal{I}:= \{ i_1,i_2,\dots, i_r\}$ stay in the same state while agents at indices in $\mathcal{J} := \{j_1,j_2,\dots,j_{n-r} \}$ move to goal state i.e., $s'_{i_1}=s'_{i_2}=\dots=s'_{i_r}=s_{init}$ and $s'_{j_1}=s'_{j_2}=\dots=s'_{j_{n-r}}=goal$. \\
$P(\tb{s}'|\tb{s},\tb{a}) \\ 
= \langle \phi(\tb{s}'|\tb{s},\tb{a}), \theta \rangle \\
= \langle \phi((s'_1,s'_2,\dots, s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n)), (\theta_1, 1, \theta_2, 1,\dots, \theta_n,1) \rangle \\
= \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)),(\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle \phi(s'_i|s_i,a_i), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(s'_j|s_j,a_j), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle (a_j, \frac{\delta}{n.2^{n-1}}), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \Big \{  \frac{1-\delta}{n.2^{n-1}} + \langle -a_i,\theta_i \rangle \Big \} + \sum_{j \in \mathcal{J}} \Big \{ \frac{\delta}{n.2^{n-1}} + \langle a_j, \theta_j \rangle \Big \} \\
= r. \frac{1-\delta}{n.2^{n-1}} - \sum_{i \in \mathcal{I}}    \langle a_i,\theta_i \rangle  + (n-r). \frac{\delta}{n.2^{n-1}} +  \sum_{j \in \mathcal{J}}  \langle a_j, \theta_j \rangle  \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}} -  \sum_{i \in \mathcal{I}} \{ \sum_{p = 1}^{d-1} a_{i,p}.\theta_{i,p} \} + \sum_{j \in \mathcal{J}} \{ \sum_{p = 1}^{d-1} a_{j,p}.\theta_{j,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \{
\sum_{j \in \mathcal{J}}   a_{j,p}.\theta_{j,p}  -  \sum_{i \in \mathcal{I}}  a_{i,p}.\theta_{i,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \Big \{
\sum_{j \in \mathcal{J}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{j,p}) = sgn(\theta_{j,p})\} - \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{
\sum_{j \in \mathcal{J}}  \Big[ 1 - 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}}  \Big[   1 - 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{  \Big[ n-r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] - \Big[  r - \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
\sum_{p = 1}^{d-1}  \Big \{  n-2r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
  \Big \{  (d-1)(n-2r) - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\frac{\Delta . (n-2r)}{n} +\frac{2 \Delta}{n(d-1)} . 
  \Big \{  \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}     \Big \} \\
$ 
\\
Lines 186-190 follow by linearity assumption, definition of features and splitting the dot product over $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Lines 191-195 simplify the dot product and rearrange terms. Line 196 uses definition of action and theta. The remaining lines simplify the summations and rearrange the terms.
\\
From the above expression, we conclude that this probability remains same (say, $p_{a,r}$ for subsequent discussions,  for all states $s \in \mathcal{S}_{n,r}$ for every $r \in [n]$ for $a = \{a_1,a_2,\dots,a_n\}$ given global action taken at $s = \{s_{init}, s_{init},\dots, s_{init}\}$.  \\


A more general result of the above relates to transition probability from some $s \in \mathcal{S}_{n,r}$ to some $s' \in \mathcal{S}_{n,r'}(s)$ where $\mathcal{S}_{n,r'}(s)$ represents the possible states of type $r'$ reachable from $s$ i.e.m   $0 \leq r' \leq r \leq n$. We discuss this below. \\ 


\textcolor{blue}{below $\mathcal{I}, \mathcal{J} = \mathcal{I}^\prime$ and $\mathcal{T} \cup \mathcal{T}^\prime = [n]$}


\textcolor{blue}{these sets of agents are different from the sets of agents above and is general; general in terms of initial state $s_{init}$ }

Suppose $s$ is such that agents at index in $\mathcal{I}:= \{i_1,i_2,\dots, i_r\}$ are at $s_{init}$ and those at $\mathcal{J} := \{j_1,j_2,\dots, j_{n-r}\}$ are already at goal. Let agents in $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ be the ones transiting from $s_{init}$ to $goal$ i.e., $s \in \mathcal{S}_{n,r}$ and $s' \in \mathcal{S}_{n,r'}$ where $n \geq r \geq r' \geq 0$ and $n \geq 1$. \\ \\
$P(s'|s,a)  \\= \langle \phi(s'|s,a), \theta \rangle  \\= \langle \phi((s'_1,s'_2,\dots,s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n) ), (\theta_1,1,\theta_2,1,\dots,\theta_n,1)\rangle  \\ = \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots, \theta_n,1) \rangle  \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle \phi(s|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle \phi(g|s,a_t), (\theta_t,1) \rangle \\ 
= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle (-a_i, \frac{1-\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle (a_t, \frac{\delta}{n.2^{r-1}}), (\theta_t,1) \rangle \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \{ \frac{1-\delta}{n.2^{r-1}} + \langle -a_i, \theta_i \rangle \} + \sum_{j \in \mathcal{J}}   \frac{1}{n.2^{r}}  + \sum_{t \in \mathcal{T}} \{ \langle a_t,\theta_t  \rangle + \frac{\delta}{n.2^{r-1}} \}   \\=  r'. \frac{1-\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}  + (r-r'). \frac{\delta}{n.2^{r-1}} + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}   + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} a_{i,p}. \theta_{i,p}      + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   a_{t,p} .\theta_{t,p}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} -  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{t,p}) = sgn(\theta_{t,p})\} -  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}}  \frac{\Delta}{n(d-1)} \Big \{  d-1 -  2 \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}}    \frac{\Delta}{n(d-1)} \Big \{  d-1 - 2\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} -   \frac{\Delta}{n(d-1)} \Big \{  r'(d-1) -  2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     +    \frac{\Delta}{n(d-1)} \Big \{  (r-r').(d-1) - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n(d-1)} \Big \{  (r-2r').(d-1) + 2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\ $

So, we have 
\begin{equation}
    P(s^\prime | s, a) 
=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}            \label{general transition probability}
\end{equation}

\pt{this incorporates the new features. Also, this will be the optimal probability when the sign matching property holds.}

\textcolor{blue}{we can avoid `line break' commands above } \textcolor{red}{ok, removed them but now proof may seem clumsier}  \textcolor{blue}{ok, we will see a way out, perhaps, we will introduce them}



\textcolor{blue}{we should use available  macros for lemma, proof, etc. see the style file.} 

\textcolor{blue}{these help where the proof starts and importantly ends -- Paul Halmos tomb-stone mark}
\textcolor{red}{ok, this is new for me. i'll try to learn this.}


Initial lines (not mentioning number since it is changing as we are modifying content above) use linearity assumption, definition of features and decomposing the inner product over agents who remain put at $s_{init}$, transit to goal and remain put at goal. In the next few lines, we expand the inner product terms and summations, use the definition of actions and theta and rearrange. Then, just rearrange different terms.  The indicators make sure appropriate sign is given to the dot product depending on signs of components of action and that of theta, \textcolor{blue}{we will cite some papers about these signs }. 

\textcolor{blue}{this is helpful to the reader}

\textcolor{blue}{let's write the role of indicator function above} \textcolor{red}{role as in?}


\\
\\
Notice that for a given global action, the  transition probability from any $s \in \mathcal{S}_{n,r}$ to any $s' \in \mathcal{S}_{n,r'}$ as long as the transition is possible (i.e., $s' \in \mathcal{S}_{n,r'}(s)$) remains the same as above. 


 
Another important probability is that of transition to global goal state after taking a global action a in any state $s \in \mathcal{S}_{n,r}$. \\  \\

\\
\\
 $ P(s'=(g,g,\dots,g)|s,a) \\ = \langle \phi(s' = (g,g,\dots, g)|(s,a)), \theta \rangle \\ = \langle (\phi(g|s_1,a_1), \phi(g|s_2,a_2),\dots, \phi(g|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle \phi(g|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle (a_i, \frac{\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j,1) \rangle \\ = \frac{r\delta}{n2^{r-1}} + \sum_{i \in \mathcal{I}} \langle a_i,\theta_i \rangle + \frac{n-r}{n2^{r}} \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  a_{i,p} \theta_{i,p} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}}  \frac{\Delta}{n(d-1)} \Big\{ d-1 - 2  \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
  \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  +  \frac{r \Delta}{n} - \frac{2 \Delta}{n(d-1)} \sum_{i \in \mathcal{I}}    \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
 $
\\
\\
This is very similar to above proofs and no new idea is used, only the state is explicitly mentioned.
\\

\textcolor{blue}{write this as another lemma} \textcolor{red}{i had written this before writing the above general proof which is now a lemma. this one is specific for r=n and r'=0 which game me an idea of how to express for general case. should this be a lemma or corollary } \textcolor{blue}{yes, as said over phone. }


%\textcolor{blue}{ think it is $\newtheorem{lemma}{command for new lemma}$}

\subsubsection{$V^*$ for multiple cases}


General formula:  \textcolor{blue}{is this a theorem?} \textcolor{red}{It follows directly from Bellman equation}\\
 $V^*(s) = \{1  + |\mathcal{S}_{n,r-1}(s)| p_{a^*,r-1} V^*_{r-1} +  |\mathcal{S}_{n,r-2}(s)|p_{a^*,r-2} V^*_{r-2} + \dots + |\mathcal{S}_{n,2}(s)| p_{a^*,2} V^*_{2} + |\mathcal{S}_{n,1}(s)| p_{a^*,1} V^*_{1} \} . \{ 1 - P(s|s,a^*) \}^{-1}$

 \\ \\
 Below $p^*_{r,r'}$ denotes transition probability for a valid transition from state of type $r$ to that of type $r'$ under optimal global action in the respective instance specicified by $\theta$ and $n$ and $V^*_0 = 0$ \\ \\
For n = 1 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$ \\ \\ 
For n = 2 \\
For r = 1 \\ 
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For n = 3 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
\\

For n=4 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\

For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
For r = 4 \\
$V^*_4 = 1 + p^*_{4,4}V^*_4 + \binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1+\binom{4}{4}p^*_{4,0}V^*_0 = \frac{1+\binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1}{1-p^*_{4,4}} = \frac{1+\binom{4}{1}p^*_{4,3}\frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} + \binom{4}{2}p^*_{4,2}\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{4}{3}p^*_{4,1}\frac{1}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+\frac{ \binom{4}{1}p^*_{4,3} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} +\frac{ \binom{4}{2}p^*_{4,2}+\frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}}  = \frac{1+ \frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+ \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}}+\frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  }{1-p^*_{4,4}}$


\pt{can you see the closed form expression here?} \textcolor{red}{i can see a pattern but can't express it nicely.}

\pt{if not, can you confirm whether this notation is correct? -- $p^*_{r,r'}$ is the probability that number agent in the state $s$ were $r$, and the number of agents in $s'$ are $r'$?} \textcolor{red}{yes, line 308-309}

\pt{also can you recall me here -- what does the  $\binom{4}{2}$ or $\binom{3}{1}$ represent in terms of $r,n,$ and $r'$? $\binom{r}{r-r'}$} \textcolor{red}{yes,in the first factor of every term in the numerator}

\pt{I will try to get the closed form expression once you mention this.} \textcolor{red}{if you can get this it will be good to add}


\pt{Also can you summarize what are the intermediate results we have. summarize all of them no matter how  trivial or useful they are are. } \textcolor{red}{The general probability expression , The all in one result: $a^*$ is same for all states and is the one matching signs with each component of $\theta$, $V^*$ is same for all states of a particular type, $V^*$ are ordered and (due to) the claim on probabilities hold}

\pt{I can see  that you have many intermediate results.}












\textcolor{blue}{let's write here the  intermediate steps with pending proofs }
\textcolor{red}{done as of now, thought there's a pattern, to express it mathematically is a bit challenging, i'll try to think about this}

\subsubsection{Important result regarding monotonicity of V*, an independent result , and a result with weaker sufficient is stated and used below} \\

Consider the states space, $\mathcal{S} = \{s_1,s_2,\dots,s_n\} \cup \{x,y\} $. Let under some global action, the following markov chain be induced:
\\ Cost for any transition is constant and equal to 1. Transition probability from x to $s_i$ is represented as $p_{x,i}$ and from y to $s_i$ as $p_{y,i}$ for $i \in \{1,2,\dots,n\}$ and $p_{x,x}$ and $p_{y,x}$ represent the same from x and y respectively to x. Probability from y to y is represented as $p_{y,y}$. All probabilities are considered between 0 and 1 (strictly). Further, it holds that $p_{y,s} = p_{x,s} - \delta_s$ for every $s\in \{x,1,2,\dots,n\}$ where all $\delta_s \in (0, p_{x,s})$. (We would later require that assuming $p_{x,(.)}$ is monotonic, $\delta_s$'s are such that they preserve the monotonicity of $p_{y,(.)}$. But this assumption on $\delta_s$'s is not required in this discussion.) No other transitions are possible. For the sake of discussion, we assume that the states $s_1,s_2,\dots,s_{n}$ are absorbing states (potentially there may be all kinds of transitions from there but the long term value is known hence they can be considered terminal states with these values) with value function known respectively as $V_1,V_2,\dots,V_n$ while value of state $x$ is also known as $V_x$. Assume the following condition holds for the values: $V_1<V_2<\dots<V_n < V_x$. We want to relate $V_x$ and $V_y$. \\ \\
\tb{Claim:} $V_x < V_y$ \\ \\
$p_{y,y} = 1-p_{y,x}-\sum_{i=1}^{n}p_{y,i} = 1-(p_{x,x} - \delta_x) - \sum_{i=1}^n(p_{x,i}-\delta_i) = \delta_x + \sum_{i=1}^n \delta_i$ \\ \\
$V_x = \sum_{i=1}^np_{x,i}(1+V_i)+p_{x,x}(1+V_x)$ \\ \\
Similarly, \\
$V_y = \sum_{i=1}^np_{y,i}(1+V_i) + p_{y,x}(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^n(p_{x,i}-\delta_i)(1+V_i) + (p_{x,x}-\delta_x)(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^np_{x,i}(1+V_i) + p_{x,x}(1+V_x)-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_i)\} + p_{y,y}(1+V_y) $ \\ \\
From the definition of $V_x$ above and monotonicity of V's, we have : \\
$V_y > V_x-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_x)\} + p_{y,y}V_y = V_x-p_{y,y}(1+V_x) + p_{y,y}(1+V_y) \\ \implies V_y - V_x > p_{y,y}(V_y -V_x) \\ \implies (1-p_{y,y}) (V_y - V_x) > 0 \\ \implies V_y>V_x $

 \\ 


\subsubsection{ALL IN ONE THEOREM - Proving $a^*$ is the one that matches sign with $\theta$ for every state, $V^*$ is same for states of a particular type, there exists ordering of $V^*$'s : all go hand-in-hand \textcolor{blue}{lines after \ref{regret} are basic and hence need to be cross-checked}} 
\tb{Base Case}  \\ By definition, $V^*_0 = 0$. \\
Take any $s \in \mathcal{S}_{n,1}$. \\
\tb{Q.} What is $a^*$? \\
For s, only possible next global states are s itself and all-at-goal (g). This is akin to the single agent problem. But any transition probability also depends on actions of others. \\
Suppose $p^a_{s,g}$ denotes the transition probability from s to g. Then we have, \\
$V_1(s) = (1-p^a_{s,g}).(1+V_1(s)) + p^a_{s,g}.(1+V_0) \implies V_1(s) = \frac{1}{p^a_{1,0}}$ \\
Thus the optimum action at s is the one that minimizes $V_1(s)$ i.e., maximizes $p^a_{s,g}$. From the above general equation (line 177), the transition probability is maximum when $a$ is such that it matches all signs with $\theta$ for the respective components of agent who was initially at s. The signs of other components do not matter. Hence there could be multiple $a^*$ for any particular $s \in \mathcal{S}_{n,1}$. \\
Notice that this will hold true for any $s \in \mathcal{S}_{n,1}$. Note that particular $a^*$ whose sign matches with components of $\theta$ (for every agent), is common for possible $a^*$ for every $s \in \mathcal{S}_{n,1}$. We consider this $a^*$ in particular. \\
Since from the general formula, for a fixed instance ($\theta$), for a given action the probability only depends on r and r', it is the same for all states s $\in \mathcal{S}_{n,1}$ i.e., $p^{a^*}_{s,g} = p^{a^*} \forall s \in \mathcal{S}_{n,1}$. This $V^*_1(s) = V^*_1 \forall s \in \mathcal{S}_{n,1}$ \\
Since transition probability for this action is strictly between 0 and 1, $V^*_1 > V^*_0=0$ \\
\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:\\ $a^*$ is the one that matches sign with $\theta$ for any state in $\mathcal{S}_{n,k}$, hence $p^*(s \in \mathcal{S}_{n,k}  \xrightarrow{}s' \in \mathcal{S}_{n,k'}(s)) = p^*_{k,k'}$, $V^*_k(s)=V^*_k$ for any $s \in \mathcal{S}_{n,k}$ and $V^*_k>V^*_{k-1}$. Now, we need to show the same for $r+1$. \\
Consider any $s \in S_{n,r+1}$. \\
$V^a(s) = \sum_{s' \in \mathcal{S}(s)\textbackslash \{s,g\}} P(s'|s,a)\{1+V^*(s')\} + P(s|s,a).\{1+V^a(s)\} + P(g|s,a).\{1+V^*(g)\}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +\sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} p^a_{r+1,r'}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \sum_{i \in [n]} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r'}  - \binom{r}{r'-1} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Big  \}$ \\ 
Observe that the third term is always non negative since when $r'>r/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} >V^*_r$ while for $r' \leq r/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_r$. Note that the above arguments is for $r' \in [r]$. To minimize $V^a(s)$, we need to minimize $P(s|s,a)$ as well (check after rearrangement as it will appear in denominator as 1-P). Clearly, the action that matches sign with all components of $\theta$ minimizes $V^a(s)$. Hence this is $a^*$. Notice the above arguement holds for any $ s \in \mathcal{S}_{n,r+1}$. Hence $a^*$ is the same for each of them. Hence $p^*(s \in \mathcal{S}_{n,r+1} \xrightarrow{}s' \in \mathcal{S}_{n,r'}(s)) = p^*_{r+1,r'}$. Hence $V^*(s) = V^*_{r+1}$ for each of them. \\

\\ \\
Proving $V^*_{r+1} > V^*_r$ is tricky. We will make a suitable assumption on probabilities and later show that it holds under suitable choices of $\delta$ and $\Delta$. \\
\tb{Claim} If for every $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.  \\
We will justify that the assumption on probabilities in this claim holds for our features under suitable $\delta$ and $\Delta$. For now lets assume this holds for our case and prove the implication part of claim. \\
Return to the induction argument. \\
$V^*_r = 1+\sum_{r' \in \{0,1,\dots,r\}}\binom{r}{r'}V^*_{r'}$ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'}$ \\
Suppose for every $r' \in \{0,1,2,\dots,\lfloor\frac{r+1}{2}\rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}-\delta_{r'} $ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor\ +1 , \lfloor\frac{r+1}{2}\rfloor+2,\dots,r-1,r\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}+\delta_{r'} $ where $\delta_{r'}>0$ for every $r' \in \{0,1,\dots,r\}$\\ 
Note that, $\sum_{r' \in \{ 0,1,\dots,r,r+1\}} \binom{r+1}{r'}p^*_{r+1,r'} = 1 \\ \implies \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r+1}{r'}p^*_{r+1,r'} + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r+1}{r'}p^*_{r+1,r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} (\binom{r}{r'}p^*_{r,r'}-\delta_{r'}) + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} (\binom{r}{r'}p^*_{r,r'} + \delta_{r'}) + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies  \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r}{r'}p^*_{r,r'}-\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \implies p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + 1 -  \sum_{r' \in \{0,1,\dots,r-1,r} \binom{r}{r'}p^*_{r,r'} \\ \implies p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} $ \\ \\
Now, going back to $V^*_{r+1}:$ \\ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}(\binom{r}{r'}p^*_{r,r'} - \delta_{r'})V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}(\binom{r}{r'}p^*_{r,r'}+\delta_{r'})V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} V^*_{r'}+ \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, r-1,r\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\=  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ > p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{\lfloor \frac{r+1}{2} \rfloor + 1}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  (  \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} - \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}  )V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ >  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r $ \\ 
Thus,\\
$V^*_{r+1} >   p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r \implies (1-p^*_{r+1,r+1})(V^*_{r+1}-V^*_r)>0 \implies V^*_{r+1} > V^*_r$ \\
Above inequalities used monotonicity of $V^*$ due to induction assumption. \\
Below we justify that the assumption in the above claim holds for our case.

\subsubsection{Sufficient conditions on $\delta$ and $\Delta$ for well defined probabilities; \textcolor{blue}{$\delta$ is conflicting with high probability $\delta$}}

$p^a_{r,r'} < 1$ for every $r \in \{1,2,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$. \\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  <   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{1} <   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{\frac{n-r}{2}}{n2^{r-1}}        +    3\Delta  =  \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} +    3\Delta =  \frac{(r'-0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} +    3\Delta < \frac{0.5n(2-2\delta)}{n.2^{r-1}} + 3\Delta  < 1-\delta + 3\Delta$ \\
To ensure $p^a_{r,r'}<1$ it is sufficient to ensure $1-\delta + 3\Delta<1 \implies \delta > 3\Delta$ \\
Similarly, we must ensure, $p^a_{r,r'} > 0$ for every $r \in \{0,1,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$. \\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  > \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') -  \frac{2 \Delta}{1} > \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} - 3\Delta > \frac{(r' -0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta > \frac{( -0.5n)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta = \frac{ \delta }{2^{r-1}} - 3\Delta$ \\
To ensure, $p^a_{r,r'} > 0$ it is sufficient to ensure $ \frac{ \delta }{2^{r-1}} - 3\Delta > 0  \implies \delta > 3.2^{n-1}.\Delta$. \\ Observe that since $n \geq1$, condition from $p>0 \implies $ condition from $p<1$  Also note that in the above, we have assumed $\delta < 0.5$. Hence we can fix any $\delta, \Delta $ and $n$ that satisy the above conditions in order to fix a class of instance as above.




\subsubsection{Justification of assumption in the claim} 
Recall that in the above claim, we assumed that: for every $r \in [n-1],$ for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$. \\
Below, we will derive sufficient conditions on $\delta$ and $\Delta$ such that this assumption holds. \\
Also note that from below section we have $\delta<0.5$ and $\delta>3.2^{n-1}\Delta$ so that all probabilities are well defined.
\\ \\
\tb{For $r'\leq \lfloor\frac{r+1}{2}\rfloor$}, \\
$\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \frac{r+1}{r+1-r'}p^*_{r+1,r'}<p^*_{r,r'} \Leftrightarrow \\(r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \\ \Leftrightarrow  (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \\ \impliedby (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \Leftrightarrow \frac{\Delta}{n}\frac{r^2}{8} + (r+1) \frac{\Delta}{n}<(r+1)\frac{1-2\delta}{n2^{r+1}} \Leftrightarrow \frac{\Delta}{n}(\frac{r^2}{8}+r+1)<(r+1)\frac{1-2\delta}{n2^{r+1}} \impliedby \Delta (\frac{n^2}{8}+n+1)<\frac{1-2\delta}{2^{n}} \Leftrightarrow \Delta < \frac{1-2\delta}{2^{n}(1+n+\frac{n^2}{8})}$ \\ \\
Similarly, \\ \tb{For $r' > \lfloor \frac{r+1}{2} \rfloor$}, \\ 
$\binom{r+1}{r'}p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \\ \frac{r+1}{r+1-r'}p^*_{r+1,r'}>p^*_{r,r'} \Leftrightarrow \\ (r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow \\ (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \Leftrightarrow \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow  \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0  \impliedby  (\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0 \\ \Leftrightarrow \frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2) - 0.5(r+1)(\frac{1-2\delta}{n.2^{r}}) >0 \\ \Leftrightarrow \frac{(r'-r-0.5)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2)  >0 \impliedby \frac{(-r-0.5)(1-2\delta)+0.5n }{n.2^{r}}   >   \frac{\Delta}{n}  (r^2-r-1)  \Leftrightarrow \frac{(-r-0.5)(1-2\delta)+0.5n }{1}   >   \frac{\Delta}{1}  (r^2-r-1)  (2^{r}) \\ \impliedby (-n-0.5)(1-2\delta)+0.5n    >   \Delta  (n^2-n-1)  (2^{n})$ and $ (-n-0.5)(1-2\delta)+0.5n    > 0 \\ \impliedby 0.5n-n+2n\delta-0.5+\delta>0$ and $ 0.5n-n+2n\delta-0.5+\delta >   \Delta  (n^2-n-1)  (2^{n}) \\ \impliedby (2\delta-0.5)n>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2-n-1)  (2^{n}) \\ \impliedby 2\delta-0.5>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2-n-1)  (2^{n}) \\ \Longleftrightarrow \delta>\frac{1}{3}$ and $n > \frac{0.5-\delta}{2\delta-0.5}+ \frac{\Delta  (n^2-n-1)  (2^{n})}{2\delta-0.5} \\ \impliedby \delta>1/3 $ and $\Delta  (n^2-n-1)  (2^{n})<3\delta-1 \impliedby \Delta < \frac{3\delta-1}{(n^2-n-1).2^{n}}$ \\ For n = 1, the second condition must not be used as it is trivially satisfied in the previous step.
\\
Finally we obtain for the desired instance, fix $1/2>\delta>1/3$. Then, fix, $\Delta< 2^{-n}.min\{\frac{3\delta-1}{n^2-n-1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2/8}\}$ \\



\subsubsection{Another way to think of Q-V difference introduced above \textcolor{blue}{this is advantage function, isn't?}} \textcolor{red}{yes, it's like expected value of the advantage function since there is expectation over $a_1$ according to the policy \\ also i've modified below for new features}
\\
\\
From \ref{difference of probabilities} we have the following. In the below, $s_t$ represent global state at time t (Note it's not individual state), $\textbf{s}_t$. Similarly $a_t$ is global action at t.

\begin{lalign} 

$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1) \\
= \mathbb{E}_{a_1 \sim \pi(s_1)}[c(s_1, a_1) + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}V^*(s_2)] - V^*(s_1)  $ \\
Using Bellman Equation and cost is 1
\\ 
$=  \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{  1 + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}[V^*(s_2)] - V^*(s_1) \Big \}$
\\ Expand the Expectation $ \\
=   \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  P(s_1|s_1,a_1) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1) \Big \}
\\ $ Use expression of probability from above$
 \\= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2)  - V^*(s_1) \Bigg \}
\\$ Rearranging the terms $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*(s_1) \Big\} 
\\ $ Notice from the general expression of probability from previous proof $\\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - V^*(s_1) \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} 
\\$ Expand V*(s_1) $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 + P(s_1|s_1,a_1^*)  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - \Big\{ 1 +  P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1, a_1^*) V^*(s_2) \Big\} \Bigg \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p})\neq sgn(\theta_{i,p})\} V^*(s_1) \Big\} 
\\$   

Rearrange and combine  terms to have a  lower bound 

$ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $
\end{lalign}


\\



\subsubsection{Dealing with the sum of Probability differences above} 

Recall from earlier, \\ 
$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)   
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \\
 \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 The first term is problematic and it is not clear how to deal with it. Let's investigate the summation inside the expectation of the first term: \\ 
 $\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2) \\ = \sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} [P(s'|s_1,a_1)-P(s'|s_1, a_1^*)] V^*(s') $ (Now, use results from above sections) \\
 = $\sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\} V^*_r $ \\
= $\frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{\sum_{s' \in \mathcal{S}_{n,r}} [\{   \sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p}) \}]  \Big\}   \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n}   
 \sum_{s' \in \mathcal{S}_{n,r}} [ \mathbbm{1}\{s'_i = s_{init}\}   \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   - \mathbbm{1}\{s'_i = goal\}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \}]  \Big\} \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  
 \sum_{s' \in \mathcal{S}_{n,r}} \mathbbm{1}\{s'_i = s_{init}\}     -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \sum_{s' \in \mathcal{S}_{n,r}} 
 \mathbbm{1}\{s'_i = goal\} \Big\}  \Big\} 
 \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \binom{n-1}{r-1}    -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \binom{n-1}{r} \Big\}  \Big\} \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \{ \binom{n-1}{r-1}    -   \binom{n-1}{r} \} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} V^*_r  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} + V^*_{n-r}  \frac{2(n-r)-n}{n} \binom{n}{n-r} \} \Big\}   \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} - V^*_{n-r}  \frac{2r-n}{n} \binom{n}{r} \} \Big\}  \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  - V^*_{n-r}   \} \frac{2r-n}{n} \binom{n}{r} \Big\} \geq 0. 
 $ \\
 \\
 Observe that when $r> n/2, V^*_r > V^*_{n-r}$ and vice-versa (refer result above) \\
 Hence we have established that, \\
 $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1) \geq \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\ \\
 To generalize, we need to show that the above inequality holds for any $s_1 \in \mathcal{S}$ and not just $s_{init}$. We will use this result below.

 \subsubsection{Now going back to Lower Bound Proof with Inequality using above result}
 From earlier, expected regret in the $k-th$ episode: \\
$R_{\theta,k} \\ = V^{\pi_\theta}(s_1) - V^*(s_1) 
\\ 
 = \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)$ \\
\\ Using above result, \\

 $R_{\theta,k} \\ \geq  \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_1 \neq goal \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 By recursion and the generalized result from the section above,
 we have: \\

 $R_{\theta,k} \\ \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{k} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_h \neq goal \} \mathbbm{1}\{sgn(a^h_{i,p}) \neq sgn(\theta^h_{i,p})\} \Big\}  $ \\
 where, the Expectation is taken with respect to trajectory induced in the $k-th$ episode by the interaction of policy $\pi$ and transition kernel $P_{\theta}$. Now, the total expected regret over $K$ episodes is: \\
 $
 R_{\theta}(K) \\
 \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{t=1}^{\infty} \mathbb{E}_{\theta, \pi} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_t \neq goal \} \mathbbm{1}\{sgn(a^t_{i,p}) \neq sgn(\theta^t_{i,p})\} \Big\}
 $ \\
 Analogous to Min et al, Cohen et al, we define: \\
 $N = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} $ and for agent $i \in [n]$,\\
$N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta^t_{i,j})\} $  \\
Thus, $R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]} \sum_{j=1}^{d-1} N_{i,j}(\theta) \}$ \\
To use the standard Pinsker's Inequality, we need $N_{i,j}(\theta)$ to be bounded almost surely which is known to not hold for SSPs (Min et al, Cohen et al). Hence, we use the capping trick introduced by Cohen et al and also used by Min et al. In this trick, we cap the learning process to a predetermined T. If the learning process (i.e. $K-th$ episode) ends before this, the agents continue to remain at $goal$. In this case the summation for the actual process and the capped process is the same. On the other hand when K episodes end beyond T, we have a truncated sum. Due to non-negativity of each part, the sum for the capped process lower bounds the actual sum. \\ Define \\ $N^- = \sum_{t=1}^T\mathbbm{1}\{s_t \neq goal\} $ and for any agent $i \in [n] $ and $ j \in [d-1],$\\ $N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta^t_{i,j})\} $ \\ 
It is easy to see that for any $i \in [n]$ and $j \in [d-1]$, $N^- =   N^-_{i,j}(\theta) + N^-_{i,j}(\theta^{j})  $ \\ where for every $\theta$, $\theta^j$ represents the vector that only differs at the $j-th$ index of every $\theta_i$ in $\theta = \{\theta_1,1,\theta_2,1,\dots,\theta_n,1\}$, where each $\theta_i \in \{\frac{-\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}\}^{d-1}$. \\ 
Thus,  $R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}$.  Notice that $\theta \in \Theta \iff \theta^{j} \in \Theta$ (This follows from definition of $\Theta$ \textcolor{red}{without this, following equation won't hold}). Then, we have: \\
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \{ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \} \\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^- - N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^-] - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}

Need to prove generalisation of Lemma C2 in Cohen et al 2020: If $T \geq 2KB^*$, then $\mathbb{E}_{\theta}[N^-] \geq KB^*/4$  \\ \textcolor{red}{Turns out similar lemma holds. Proof given below. We pick $T = 2KB_*$} \\
\textbf{Pinsker's Inequality(Min et al, Lemma E.3)} \pt{$TV(p,q) \leq \sqrt{KL(p,q)}$}

If $f:S^T\xrightarrow{}[0,D]$ then, 
$\mathbb{E}_{\mathcal{P}_1} (f(s)) - \mathbb{E}_{\mathcal{P}_2} (f(s))\leq D \sqrt{\frac{log(2)}{2}}. \sqrt{ KL(\mathcal{P}_2 || \mathcal{P}_1)}$  

\pt{Note that this will hold only if $|f(s)| \leq D \sqrt{\frac{log(2)}{2}}$?}
\textcolor{red}{I dont think so. $|f(.)|$ can be D}


\pt{don't use double back slash. These are not needed. just give one line spacing.}

Then, 
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  \mathbb{E}_{\theta, \pi}  [N^-] +  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] - \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] \} \Big \} \\ \geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{  \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] - \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] \} \Big \} \\ 
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
$

\textcolor{blue}{to update the above relations, equalities and inequalities } \textcolor{red}{done}
\\
\\
\\
For appropriate $\delta, \Delta$, $KL(\mathcal{P_{\theta}||\mathcal{P_{\theta^j}}}) \leq \frac{16.\Delta^2}{(d-1)^2.\delta}.\mathbb{E_{\theta}}[N^-]$  \\
\textcolor{red}{The above doesn't hold but} \\ We have the following for our case: \\
For appropriate $\delta$ and $\Delta$:
$ KL(\mathcal{P_{\theta}||\mathcal{P_{\theta^j}}}) \leq  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-] $
\\
\textcolor{red}{Need another intermediate similar lemma to simplify the KL-divergence term. \\ Assuming this also holds for our case, \\ }
\textcolor{red}{same result doesnt hold, but new one updated! (2-4-25)}

$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta V_1^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{1/2} \sqrt{3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]}  \} \Big \} \\
= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{\mathbb{E}_{\theta}[N^-]} \Big \} \\
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{T} \Big \} \\
= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \} \\ 
$\\
Notice that the term in bracket is independent of $\theta, i$ or $j$. Thus, we have: \\
$\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq  \Delta V_1^* |\Theta| \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \} \\
\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq   V_1^*  \Big \{ \Delta  KV_1^*/4 -   (KV_1^*)^{3/2}  \frac{2^{n+2}.\Delta^2}{\sqrt{\delta} (d-1)} \Big \} \\ 
$ 
Specifically, pick, $\Delta^* = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}$. \\ At this value of delta,\\
$\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq V_1^* \{  \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}. \frac{KV_1^*}{4} - \frac{(KV_1^*)^{3/2}.2^{n+2}}{\sqrt{\delta}(d-1)}.  (\frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}})^2\} \\ 
= V_1^* \{\frac{(d-1) \sqrt{\delta.K.V_1^*}}{2^{n+7}} - \frac{(d-1)\sqrt{\delta.K.V_1^*}}{2^{n+8}}\}
\\
\geq  \frac{(d-1).\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+8}} \geq \frac{d.\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+9}} $ \\ \pt{This makes it independent of number of agents, a very strong result? Is this correct or do we need to incorporate the number of agents here.} \textcolor{red}{potentially the intermediate results I used directly without verifying depend on n. the term i argued to be $+ve$ and ignored in lower bound certainly depends on n but very difficult to simplify(needs closed form V*)} \\
\textcolor{red}{update : it depends on n}

Since the average over entire set is lower bounded by the RHS, there must exist some parameter in the set for which the RHS is a lower bound. Hence proved. \textcolor{blue}{ok we will discuss the proof}. \\ \\
It remains to show that the $\Delta$ picked above is valid. \\ Hence, need to ensure that $\Delta = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}} < 2^{-n}.min\{\frac{3\delta-1}{n^2-n-1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2/8}\}$  \\ or, $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.min^2\{\frac{3\delta-1}{n^2-n-1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2/8}\}} $
\\ \\
\textcolor{blue}{updated later} \textcolor{red}{Although it is independent of $n$, it can be interpreted as a strong result in the sense that no matter how many agents are deployed to learn, this minimum regret will always hold. The independence also comes from ignoring the positive terms} \\ \textcolor{red}{(whose proof is as of now still incomplete )}. \\ \textcolor{red}{since now there is a dependence on $n$, the above para is not valid} 

\textcolor{blue}{we need to write the  statement that is proved, and also delineate that statement from the proof -- use macros provided in the style file} \textcolor{red}{This is not complete yet. Only if we can find the corresponding lemmas I've mentioned in the proof, it will be complete possibly with very different expression.} \\
\\
\textcolor{blue}{2/4/25} \textcolor{red}{The proof is now complete! Now we have one complete result!}
\\ 
\\
\textcolor{red}{3/4/25} \\
\tb{Theorem}: For any MASSP learning algorithm $\mathfrak{A}$, there exists a linear-mixture MASSP instance defined by appropriate parameters ($n, \delta, \Delta, \theta$) for whom the expected cumulated regret matches the reported upper bound $\widetilde{O}(\sqrt{K})$. \\ Specifically, the instance satisfies: \\ $\mathbb{E}_{\theta,\mathfrak{A}}[R(K)] \geq \frac{d.\sqrt{\delta}\sqrt{K.V^*_1}}{2^{n+9}}$ \\
for $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.min^2\{\frac{3\delta-1}{n^2-n-1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2/8}\}} $

\subsubsection{Generalisation of Lemma C2 of Cohen et al for our case-12/13-3-25}
\tb{Lemma:} For any deterministic learner, if $T\geq 2KV_1^*$, then, $\mathbb{E}[N_-]\geq KV^*_1/4$ \\ 

\textcolor{blue}{there is a relation between $B^\star$ and $V^\star_1$ and is given in the first half of this writeup }

\tb{Proof:} If capped process finishes before T, $N_-=N$. Else number of visits to goal state is less than $K$. \\Thus, $N_- \geq T-K$.\\ Thus, $\mathbb{E}[N_-] \geq \mathbb{E}[min\{T-K,N\}] \geq \mathbb{E}[\sum_{i=1}^Kmin\{T/K-1, N_k\}]$.\\
Since $T\geq2KV^*_1,$ and $V^*_1\geq1$ the lemma will hold for any policy (mapping of actions) if, $N_k \geq V^*_1$ with probability $\geq 1/4$ for any policy. Consider any policy. \\ We can lower bound the probability $\mathbb{P}[N_k \geq V^*_1]$ by the events that we transit to an $r=1$ state and stay there for next $\lceil V^*_r\rceil -1$ steps. \\Thus, \\
$\mathbb{P}[N_k \geq V^*_1] \\ = \mathbb{P}(s_2 \neq g|s_1=s_{init}).\mathbb{P}(s_3 \neq g|s_2).\mathbb{P}(s_4 \neq g|s_3)....\mathbb{P}(s_{\lceil V^*_1\rceil} \neq g|s_{\lceil V^*_1\rceil-1}) \\ = (1-p^{a(s_1)}_{n,0}).(1-p^{a(s_2)}_{s_2,0})...(1-p^{a(s_{\lceil V^*_1\rceil-1})}_{s_{\lceil V^*_1\rceil-1},0}) $ \\
For any state s, $1-p^{a(s)}_{n,0}$ is minimum when $p^{a(s)}_{n,0}$ is maximum. Check from line 1087 that this happens at $a^*$ which matches all signs with $\theta$. Further, $1-p^*_{s,0}$ when $s \neq g$ is minimum when $p^*_{s,0}$ is maximum at any $s \in \mathcal{S}_{n,1}$. Thus, we can lower bound the above product as: \\
$\mathbb{P}[N_k \geq V^*_1] \geq (1-p^*_{n,0}).(1-p^*_{s_2,0})...(1-p^*_{s_{\lceil V^*_1 \rceil -1},0}) \geq (1-p^*_{1,0})^{\lceil V^*_1 \rceil -1} \geq (1-p^*_{1,0})^{ V^*_1 -1} = (1-p^*_{1,0})^{ 1/{p^*_{1,0}} -1} \geq 1/e \geq 1/4$ \\
For the last second inequality, we use for $x\geq 1$, $(1-1/x)^{x-1}\geq 1/e$ \\
 Thus, $\mathbb{E}[N_-]  \geq \mathbb{E}[\sum_{i=1}^Kmin\{T/K-1, N_k\}] \geq KV^*_1/4$ \\


 
 \subsubsection{Alternate proof for dealing with $\mathbb{P}[N_k \geq V^*_1] \ge \frac{1}{4}$ 13-3-25}
 
\textcolor{blue}{the result below a general one}
 
 Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](s)$ as the probability that starting at state $s \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in R^+$. Further, $\mathbb{P}[N_k \geq x] = \mathbb{P}[N_k \geq x](s_{init})$. \\
 \tb{Claim} Consider any $s \in S_{n,r}$ where $r \in [n]$. Then, for any policy it holds for our instances that $\mathbb{P}^{\pi}[N_k \geq x](s) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](s')$ for all $x \in R$ where $s' \in \mathcal{S}_{n,r'}(s)$ for any $r' \in \{0\} \cup [r]$ with equality holding only at $\pi = \pi^*$  and $r'=r $ i.e., $s'=s$ respectively. Here $\pi^*$ is the policy of taking action $a^*$(the one matching all signs with $\theta$) at every state $s \in \mathcal{S}$. The equality in the middle says that for any $s \in \mathcal{S}_{n,r}$ under $\pi^*$, $\mathbb{P}^{\pi^*}[N_k \geq V^*_1](s)$ happens to stay a constant independent of $s$ and only depends on $r$.\\
 Proof will be similar to $V^*$ proof \\
 Will work on this later if above proof is not satisfactory.\\
 \tb{Proof} We will prove this by induction. \\
 \tb{Base Case:} For r=1: 
 Consider any $s \in \mathcal{S}_{n,1}$ \\
 For any $x \in R^+$, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x\rceil-1}$ \\
 One can check from the general formula for transition probabilities that the above is uniquely minimum when $\pi(s) = a^*$. Hence equality only holds at $\pi=\pi^*$.  \\
 Hence, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x\rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x\rceil -1}$ \\
 Recall that for the same action $a^*$ at any $s \in \mathcal{S}_{n,1}$, $P(g|s,a^*)$ remains the same. Hence, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x \rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) $ \\
 The only two possibilities for $s'$ are $s$ itself and $g$. \\
 Clearly for $s$ the equality holds and for $g$, $\mathbb{P}^{\pi^*}[N_k \geq x](s'=g) = 0$ \\ Hence, \\
  $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x \rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s')  $
  \\ Finally we showed that for any $x \in R^+$ for any policy $\pi$, for any $s \in \mathcal{S}_{n,1}$ and $s' \in \cup_{r' \in \{0,1\}} \mathcal{S}_{n,r'}(s)$,  \\
  $\mathbb{P}^{\pi}[N_k \geq x](s)  \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s')  $ \\
  where in the first inequality, equality holds only when $\pi = \pi^*$, the middle equality means that the probability is same for all $s \in \mathcal{S}_{n,1}$ and in the last inequality, equality holds only when $s' = s$. \\
  \\
  \tb{Generalization:} Assume the above holds for m = 1, 2,...,r i.e., for all $m \in [r]$ it holds that for any $x \in R^+$ for any $s \in \mathcal{S}_{n,m}$, for any policy $\pi$, for our instances, it holds that, $\mathbb{P}^{\pi}[N_k \geq x](s) \geq \mathbb{P}^{\pi^*}[N_k \geq x](s)=\mathbb{P}^{\pi^*}[N_k \geq x](m)\geq \mathbb{P}^{\pi^*}[N_k \geq x](s')$ where $\pi^*$ is the policy taking action $a^*$(the one matching signs with all components of $\theta$) at all states and $s' \in \cup_{m' \in \{\{0\} \cup [m] \}}\mathcal{S}_{n,m'}(s)$. Further, in the first inequality, equality only holds when $\pi =\pi^*$ and the middle equality implies that the probability is same for all states $s \in \mathcal{S}_{n,m}$ and in the last inequality, the equality only holds when $s' =s$.  \\
  Assuming this we need to show that the same holds for any $s \in \mathcal{S}_{n,r+1}$ \\
  Again consider any $x \in R^+$. \\
  Consider any $s \in \mathcal{S}_{n,r+1}$. \\
  We have, \\
  $\mathbb{P}^{\pi}[N_k \geq x](s) = \sum_{r' \in \{0,[r+1]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)} P(s'|s,\pi(s)) . \mathbb{P}^{\pi}[N_k \geq x-1](s') \\= P(s|s,\pi(s)). \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)). \mathbb{P}^{\pi}[N_k \geq x-1](s')$ \\ 
   If $x \leq 1$, then trivially, for all $s \neq g$, for all policies, $\mathbb{P}[N_k \geq x] =1$. Otherwise, we have the following:
  \\
$\mathbb{P}^{\pi}[N_k \geq x](s) \\ =  P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s') \\ 
  \geq P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s))  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \Bigg\} \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Bigg \} + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)}  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  
  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0, [r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \sum_{i \in [n]}      \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{t \in \mathcal{T}\} . \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{i \in [n]}        \{ \binom{r}{r'-1} -  \binom{r}{r'} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}     
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0,[r]\}} \sum_{i \in [n]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} 
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in [r]} \sum_{i \in [n]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  \Big \} \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{ \{ \binom{r}{r-r'} -  \binom{r}{r+1-r'} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big \} \Bigg \}   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{ \{ \binom{r}{r'} -  \binom{r}{r'-1} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big \} \Bigg \} \\
 = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{ \Big \{ \binom{r}{r'-1} -  \binom{r}{r'} \Big \} \Big \{ \mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq V^*_1](r+1-r') \Big \}      \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}        \Bigg \}$ \\ \\
 Notice that for $r' < (r+1)/2$, the binomial difference $\binom{r}{r'-1} - \binom{r}{r'}<0$ as well as probability difference $\mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r') < 0$ hence the product is $>0$. Similar argument holds for $r'>(r+1)/2$. For $r' = (r+1)/2$ it will be 0. Overall we can observe that the only terms dependent on action have non-negative coefficients for the sign matching indicator. Hence this term will be minimum when $a = a^*$.  Thus, we have, \\
 $\mathbb{P}^{\pi}[N_k\geq x](s) \geq   P(s|s,\pi^*(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} $\\ Also, \\
 $\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $ \\

Subtracting the above two equations, 
\\
$\mathbb{P}^{\pi}[N_k\geq x](s) - \mathbb{P}^{\pi^*}[N_k\geq x](s) \\ \geq P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) - P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) \\ \geq P(s|s,\pi^*(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) - P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) \\ 
= P(s|s,\pi^*(s)) (\mathbb{P}^{\pi}[N_k \geq x-1](s) - \mathbb{P}^{\pi^*}[N_k \geq x-1](s))$ \\
By recursion,  \\
$\mathbb{P}^{\pi}[N_k\geq x](s) - \mathbb{P}^{\pi^*}[N_k\geq x](s) \\ \geq P(s|s,\pi^*(s))^{\lfloor x \rfloor} (\mathbb{P}^{\pi}[N_k \geq x-\lfloor x \rfloor](s) - \mathbb{P}^{\pi^*}[N_k \geq x-\lfloor x \rfloor](s)) = P(s|s,\pi^*(s))^{\lfloor x \rfloor} (1- 1) = 0$  \\
Thus, $\mathbb{P}^{\pi}[N_k\geq x](s) \geq \mathbb{P}^{\pi^*}[N_k\geq x](s)$ \\
Also note that for equality, it must hold for each above inequality. Effectively this will only happen at $\pi = \pi^*$ \\ 
Recall, for any $s \in \mathcal{S}_{n,r}$, \\
$\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $
 \\
From the probability expression one can verify that the term $P(s|s,\pi^*(s))$ only depends on $r$. The only term that may differ due to $s$ is $\mathbb{P}^{\pi^*}[N_k \geq x-1](s)$. \\We claim that this is same too. This can be dealt with by induction on x itself. \\
For base case, $m = x-\lfloor x \rfloor$, for any $s \in \mathcal{S}_{n,r}$, $\mathbb{P}^{\pi^*}[N_k \geq m](s)=1$ \\ Hence showed for base case. \\ Assuming true for $m = x - \lfloor x \rfloor,  x - \lfloor x \rfloor+1,  x - \lfloor x \rfloor+2, \dots,  x - \lfloor x \rfloor+p $, we need to show that it holds for $m =  x - \lfloor x \rfloor + p+1$ \\ We can write for any $s \in \mathcal{S}_{n,r}$ that: \\
$\mathbb{P}^{\pi^*}[N_k\geq m ](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq m-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq m-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $ \\ Here the RHS doesn't depend on which $s \in \mathcal{S}_{n,r}$ is being chosen. Thus shown for m. \\
 Thus back in expression for $\mathbb{P}^{\pi^*}[N_k \geq x](s)$, $\mathbb{P}^{\pi^*}[N_k \geq x-1](s)$ is not dependent on $s \in \mathcal{S}_{n,r}$. Hence $\mathbb{P}^{\pi^*}[N_k \geq x](s)$ is same for all $s \in \mathcal{S}_{n,r}$.  \\
 Finally we need to show that, $\mathbb{P}^{\pi^*}[N_k \geq x](s) \geq \mathbb{P}^{\pi^*}[N_k \geq x](s') \forall s' \in \cup_{r' \in \{0,[r]\}}\mathcal{S}_{n,r'}$ with equality only at $s' = s$. \\
 Recall again, for any $s \in \mathcal{S}_{n,r+1}$, \\
 $\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in [r]} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} (\binom{r}{r'}  .  p^*_{r,r'} - \delta_{r'})  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\binom{r}{r'}  .  p^*_{r,r'}+ \delta_{r'}  )\mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r')) + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') )  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , r \}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') )  \\ >  P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](\lfloor \frac{r+1}{2} \rfloor + 1)) \\ =  P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  ( \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}\delta_{r'} - \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} \delta_{r'}) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1)  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  P(s|s,\pi^*(s)) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1) \\ > P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  P(s|s,\pi^*(s)) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( r) 
 $ \\
 Thus, we have, \\
 $\mathbb{P}^{\pi^*}[N_k \geq x](s) - \mathbb{P}^{\pi^*}[N_k \geq x](r) \geq P(s|s,\pi^*(s)).(\mathbb{P}^{\pi^*}[N_k \geq x-1](s) - \mathbb{P}^{\pi^*}[N_k \geq x-1](r))$ \\ By recursion and same arguments as before, \\
 $\mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r+1) >  \mathbb{P}^{\pi^*}[N_k \geq x](r)$
\\
 
 Hence the overall main induction argument for r holds. \\ \\
 Now, given this general theorem, where $s_1 \in \mathcal{S}_{n,1}$, we have, \\$\mathbb{P}^{\pi}[N_k \geq V^*_1](s) \geq \mathbb{P}^{\pi^*}[N_k \geq V^*_1](s_1) = (1-p^*(g|s,a^*))^{\lceil V^*_1 \rceil -1} \geq (1-p^*(g|s,a^*))^{ V^*_1  -1}  \geq 1/e \geq 1/4$

\subsubsection{Simplification of KL Divergence term 14-3-25} 
By chain rule of KL-Divergence, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)]$
\\
where, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $

\\
Let's simplify $\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)})$


\pt{Before doing this upper bound, why can't I break it into two terms -- first one where $s_t = (g,g,...,g)$, and the other one when $s_t \neq (g,..., g)$. I think the terms will be simplified a lot if you do this. 
 Also, you can go one step ahead and look at all the impossible transitions -- the log term will vanish for all of them. So, you are left with the cases when the transitions are valid. Now, you can utilize the same notations, $r$ to $r'$ type of transitions. For all such transitions, the ratio inside the log can be written in terms of the features and corresponding $\theta$, and $\theta^j$. note that we might need to carefully use the conditions on $\delta$ and $\Delta$ you obtained earlier. } \textcolor{red}{i won't be able to use $s_{t+1} \neq g$ inside ln(.), I need to check when the ratio inside ln maximises here:$s_{max}$ to provide upper bound. $s_{min}$ is not strictly required and any global state can be used instead as for eg. you suggested $g,g,g...$. Also yes, i'm thinking of possible transitions only although once the $s_t$ is fixed from outer  summation. But notice that when $s_t=(s_{init},s_{init},...s_{init})$, we will need to optimize over all $s \in S$.}

 \pt{i am not talking about $s_{t+1}$, I am saying you can look at the summation for two cases separately, $s_t = g$, and $s_t \neq g$. That will lead to some simplifications. } \\ \textcolor{red}{i wouldn't even think about $s_t=g$: cz then $s_{t+1}$ has to be $g$ with probability 1 : independent of $\theta$ or $\theta_j$ hence ratio inside log is 1 and this term will be 0, for other $s_{t+1}$ probability is 0 hence all those terms are 0. problem is to deal with the general case}

 \pt{exactly, that's where we can now only use the features and then explicitly write them in terms of the other parameters. Also, why you are trying to maximize the term inside the log? We can just write the expressions for $\theta$ and $\theta^j$ and then finally use some other bounds at the later stage.} 

 \textcolor{red}{explicitly substituting the probabilities using features leads to a huge sum, each of those $2^{r}$ terms will have ratio inside ln that looks like line 1765. It would be desirable to simplify those terms without bounding earlier. The reason i want to maximise is to bound before simplifying. I'm just trying an approach as of now.  }


 \pt{Some results from the Jaksch et al 2010 paper can be used at the later stage.}

 \begin{figure}[h!]
     \centering
     \includegraphics[width=0.5\linewidth]{Jaksch.png}
     \caption{The result from Jaksch et al 2010 paper. This holds for some conditions on $\delta', \epsilon'$. Need to check if these conditions hold in our work. this type of result can be used for each term inside the summation, possibly for each $r$ to $r'$ transition. }
 \end{figure}
 \textcolor{red}{i have seen this, it can't be used for our case. in fact i want to get the sum over $2^r$ next states in this form thats why looking for maximum of that ratio. thats what motivated line 1756. also if you look carefully, the above result is not exactly from Jaksch, it is from Min. Jaksch result is bit different. Also Min made has made a typo in this above equation.}
 
 


Notice this can be upper bounded as follows: \\ 
$\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ \leq \mathcal{P}_{\theta}(s_{t+1}= s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s_{min}|\textbf{s}_{t-1}, s_t = s, a_t = a)}) + (1-\mathcal{P}_{\theta}(s_{t+1  }= s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a)).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s_{max}|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s_{max}|\textbf{s}_{t-1}, s_t = s, a_t = a)})$ \\
where, \\ $s_{min} = arg min_{s' \in \mathcal{S}} \ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $ and, \\
$s_{max} = arg max_{s' \in \mathcal{S}} \ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ $ \\
Since, $s$ and $a$ are fixed in the outer summation, both $s_{min}$ and $s_{max}$ may depend on both $s$ and $a$. For any general transition, we investigate the behavior of the ratio above. Given $s_t$, we partition the set of agents at $s_{init}$, into $X$ and $Y$ based on action $a$. Suppose $a$ is such that agents in $X:$ $x_1,x_2,\dots,x_m$ have their $j-th$ components not matching signs with respective components of $\theta$. Hence, agents $x_1,x_2,\dots,x_m$ have their $j-th$ components matching signs with respective components of $\theta_j$. Similarly let agents in $Y: y_1,y_2,\dots, y_{r-m}$ be such that their $j-th$ components match with respective components in $\theta$. This means agents $y_1, y_2, \dots, y_{r-m}$ are such that their $j-th $ components do not match with $\theta_j$. Along with previous notations, the ratio can be analyzed as : \\ 
$
\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}  \\= \frac{\frac{(r'-0.5r)(1-2\delta) + 0.5n }{n.2^{r-1}}     +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)}\sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}}{  \frac{(r'-0.5r)(1-2\delta) + 0.5n }{n.2^{r-1}}          +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta^j_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta^j_{t,p})\} \Big \}} \\ 
$\\ \\
To find the optimal values of this ratio, we first check what happens at fixed $r, r'$ and then optimize for $r'$. Notice that the ratio is maximum when maximum number of agents who stayed had signs matched with $\theta_j$ and maximum number of agents who transited had signs matched with $\theta$

\textcolor{blue}{we are looking at $\mathbb{E}_P[X] - \mathbb{E}_Q[X]$ for two probability measures $P$ and $Q$. we can use change of variable and write $\mathbb{E}_Q[X] = \mathbb{E}_P[X \frac{dQ}{dP}]$? }

\textcolor{blue}{policy is $\pi_\theta$ and does $\theta$ refer to something else? }

\textcolor{blue}{based on a call on Sat 10pm, 22/3}
\textcolor{red}{hi, i thought we weren't meeting yesterday} \\
\pt{\url{http://joschu.net/blog/kl-approx.html} -- we can use some ideas from here.} \textcolor{blue}{this unbaised estimator of KL with low variance (by John Shulmann of PPO fame) would be very good to use in computations} \textcolor{red}{Im very doubtful, this blog is about constructing suitable estimate of kl-div from samples. but we need to analytically express kl-div or its suitable upper bound}

\pt{The above blog is suitable for the computations, isn't it?} \textcolor{red}{if by computation u mean implementing learning algo for massp, then no. I dont know if you are referring to any other kind of computation}

\pt{can we make use of the indicator present in line 1775 and bound the entire term.}

\pt{Other possibility is to take out the smallest of $\sum_{i\in I \cap T'}$ and $\sum_{t\in T}$?} \\ \textcolor{red}{can u try these and update above?}

\pt{Just for clarity, what I remember is:}

\pt{$\mathcal{I}$: Set of all agent are $s_{init}$.}

\pt{$\mathcal{J}$: Set of all agents at $g$}

\pt{$\mathcal{T}$: Set of all agents from $\mathcal{I}$ who move from $s$ to $g$.}

\pt{$\mathcal{T}'$: set of all agents from $\mathcal{I}$ who stayed at $s$}


\pt{If the above is correct, then $\mathcal{I}\cap \mathcal{T}'$ and $T$ are disjoint?} \textcolor{red}{yes, also above is correct}


\pt{Alternatively, upper bound the numerator, and lower bound the denominator and vice-versa and then take the min.} 
\textcolor{red}{the bounding of individual ratio doesn't help later, then there would be $2^r$ type factor}  \\ \textcolor{blue}{we can use min of two bounds and see how it effects the regret bound}

\pt{Also, note that only the orders as of now with respect to $n$ are important, not the front constants. As long as we are able to get some order of the regret bound wrt $n$, we are good.}


\pt{Any updates after Saturday?} \textcolor{red}{no break thru yet}

\textcolor{blue}{$\delta$ and $\delta_j$ are vectors with entries +1s and -1s. When entries are  +1s and 0s the Hamming distance between them is the number of entries that differ. we can \emph{temporarily} take -1s as 0s. this may  help to bound the KL$(\delta|| \delta_j)$.}
\\
\textcolor{red}{I have an update : today I performed computation of the sum in line 1758 for many instances of n,a,$s_t$ and realized that it is maximum at $s_t = (s_{init},s_{init},...,s_{init})$ : contradictory to what i was hoping (max for states of type r=1). Turns out this can be explained by property of KL-divergence. So we can upper bound this summation for any $s_t$ by the summation at this initial state. As of now i don't know if the upper bound i wish to obtain (same/similar as given in Min) still holds. Im trying to see that via computations. Will update further soon.}

\pt{Wasn't this observation intuitive and follows from the fact that KL is positive, and  when I told you that for the case when $s_t = (g,g,g...g)$, then one term was getting zero?} \textcolor{red}{Pls explain us how this is intuitive from terms becoming 0 when st is all at g, in the next meeting. Also do respond to my earlier responses on your above remarks, its further confusing when you suggest something and not elaborate anything. Also next meeting pls come prepared to explain the steps in upper bound proof that i had asked in January. The note you send is unclear to me.}

\pt{What are the next steps in theory?}

Meeting link: \url{https://ucf.zoom.us/j/99575809604?pwd=dar1hN9fReFbU4yae8Bp4YGDKfaBeP.1}
\\ \\
Property of KL-Divergence: https://math.stackexchange.com/questions/4986295/partition-form-of-the-kl-divergence


\subsection{Simplifying KL-Divergence}

By chain rule of KL-Divergence, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)]$
\\
where, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $ \\
Notice that in the above, for any fixed $(s,a)$, the inner summation is itself a KL-divergence. \\ 
Let's simplify it first: \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\  = \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) $ \\
\tb{Claim :} The above KL-divergence is maximum at $s_t = (s_{init}, s_{init},\dots, s_{init})$. (Proof can be shown by refinement property) \\
Hence we'll upper bound using the inner KL for s being global initial state. Fix this as s now.
The following holds as $KL(A|B) \leq KL(A|B) + KL(B|A)$ since $ KL(B|A) > 0$: \\ \\
$\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\ \leq   \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) + \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}) \\= \sum_{s' \in \mathcal{S}} (\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) ).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\
= \sum_{s' \in \mathcal{S}} (\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) ).\ln(1 + \frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\
\leq \sum_{s' \in \mathcal{S}} \frac{(\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) )^2}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)} \\
\leq 2^n . \frac{max_{s'}( \langle \phi(s'|s,a), \theta - \theta_j \rangle)^2}{\mathcal{P}_{\theta_j}(s_{t+1}=g|s_t = s, a_t = a)} \leq 2^n . \frac{(\frac{2 \Delta}{d-1})^2}{\frac{\delta}{2^{n-1}} - \Delta}
$ \\
From the sufficiency conditions, $\Delta < 2^{-n}. \frac{2\delta}{3} $. \\ Thus, \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)})  < 2^n. \frac{(\frac{4\Delta^2}{(d-1)^2})}{\frac{2\delta}{3.2^{n-1}}} = 3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $ \\ 
Hence, going back above: \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\  = \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) < 3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $ \\
Thus, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ < \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} \\ =  \mathcal{P}({s}_{t} \neq g) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $  \\ \\ Therefore from earlier, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] \\ <  \sum_{t=1}^{T-1} \mathcal{P}({s}_{t} \neq g) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} \leq  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} .  \sum_{t=1}^{T} \mathcal{P}({s}_{t} \neq g)  =  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]  $
\\
We use the above result in lower bound proof.

\pt{This seems good. Can you also write why the inequality in line 1847 holds} \\ \textcolor{red}{you meant the 1st line in the equations right? ive mentioned now in line 1848} \pt{yes, got it.}

\pt{Does that mean we now have a lower bound proof? I can see that the KL bound is exponential in $n$, will it lead to exponential bounds? or will it create some problems in the lower bound?}
\\
\textcolor{red}{yes we have a lower bound now. yes it looks exponential but from sufficient conditions, $\Delta$ is also of exponential order hence overall the bound is not exponentially large. from computations i've verified that this is quite tight(off by 1 order of magnitude for small n's and this difference decreases as n increases. hence we have a reasonably tight bound). ive updated and completed the lower bound proof(page 38). finally we get lower bound that scales as $1/2^n$. but we also get $\sqrt{K}$ }


\pt{Great!! So, we have the lower bound with $\sqrt{K}$, thus as tightest lower bound in terms of $K$, and can you explain what is the regret lower bound implication as $n$ increases? -- somehow not very clear to me. Particulary, i dond't understand this statement of yours  ``this difference decreases as n
increases. hence we have a reasonably tight bound''. } \textcolor{red}{yeah no problem, i will clear this in next meeting}

\pt{I think, now is the time to clean it and write the results in a nice format with all the details and explaination of each step. Can you explain the entire proof in our next meeting, and we can start writing it. }
\textcolor{red}{yes i wanted to explain everything too}
\pt{Let us connect on Friday evening 7:00 PM or Sat morning 9:00 AM India time, we can discuss this for a long time with all the details.} \textcolor{red}{sure, saturday 9am would be best}

Meeting link: \url{https://ucf.zoom.us/j/99575809604?pwd=dar1hN9fReFbU4yae8Bp4YGDKfaBeP.1}



\subsection{Related Work}
\label{subsec:related_work}



\\\\\
\newpage
\section{7-4-25}
\\
\input{Sections/6_experiments}


\section{\textit{Proof of Lower Bound}}

\pt{Need to write this thing cleanly with proper justifications. Why the following makes sense, and how would this capture the hardest instance. What is the role of congestion in this example?}

We construct and analyze a family of hard to learn instances based on above discussion.  Further, we restrict $\theta$ such that $\theta_{i} \neq \theta_{j}$ $ \forall$ $ i \neq j \in [n]$ i.e., no two $\theta_i$ are the same. Let this set be denoted as $\Theta$. \pt{Why this assumption will hold. there is lot of symmetry in the problem, so $\theta$'s for two agents will be same?}. \textcolor{blue}{It's not an assumption. It's a restriction of the class of SSPs instances I'm considering. I'm free to do so. Why I do this is the rest of paragraph about. Also $\theta$ is an instance parameter, it can be anything. A way to think about this is that : even if two agents took same action, the contribution to probability of transition to any global state is not the same, this is one way how agents are not identical!} This ensures that the action to be taken by each agent to maximize the probability of transition to the all-at-goal state is different for every agent so that we don't need to consider the congestion component of the cost when the policy of maximizing the probability to reach all-goal is executed.
To further reduce complexity of the analysis, we let the private cost associated with any global action in any non-goal state be equal to 1 and that in goal state equal to 0. This will be used to ensure that the \textit{best} policy is the one that matches sign with all components of $\theta$(see all-in-one theorem \ref{all_in_one}).  \\
Consider any instance, defined by among other parameters by $\theta$. \\
Suppose in episode \textit{k}, agents take actions according to policy $\pi^k_{\theta}$. Let, $\tb{s}_t$ represent the global state and $\tb{a}_t$ the global action at time $t$. Then, the expected regret for the \textit{k-th} episode is:

\pt{In the regret definition below the policy seems to have the parameters $\theta$, whereas we have originally used $\theta$ as the parameters for the transition probabilities?} \textcolor{red}{yes, we are analyzing regret of a class of instances simultaneously defined by \theta. $\pi_{\theta}$ represents the policy learned for instance defined by $\theta$. In the below everywhere $\pi ==\pi_{\theta}$. I need to update it. In fact more accurately it must be $\pi_{\theta,k}$ since the learned policy differs every episode.} 

\begin{align}
    R_{\theta,k} &= V^{\pi^k_\theta}(\tb{s}_1) - V^*(\tb{s}_1) \label{regret}
    \\
    &=  V^{\pi^k_\theta}(\tb{s}_1) - \mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] + \mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) 
    \\ 
    &= \mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^{\pi^k_\theta}(\tb{s}_2)]\}  
    \\ 
    & \quad -\mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}\{c(\tb{s}_1, \tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(\tb{s}_1,\tb{a}_1)}[V^*(\tb{s}_2)] \} + \mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim\ \pi^k_\theta(\tb{s}_1), \tb{s}_2 \sim\ \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^k_\theta}(\tb{s}_2) - V^*(\tb{s}_2)] + \mathbb{E}_{\tb{a}_1 \sim \pi^k_\theta(\tb{s}_1)}[Q_{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \label{eq_Q_V}
\end{align} \\
In the above we see a recursive relation in the first term but it its unclear how to deal with the second term.

\pt{Suggestion -- for each equation write the proper reason why it is true. This will make it easy to follow. For example, in above the second equation you added and subtracted $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] $.}
\textcolor{red}{Ok, I'll do it after I start revisiting them. Apart from adding and subtracting Q, I've only expanded the Bellman Equation}

\textcolor{red}{I'm stuck here to find a closed form expression of $Q^*(.,.)$ and $V^*$ due to exponential number of states}

\subsection{\label{q_v}\textit{Dealing with Q-V difference in} \ref{eq_Q_V}}
\subsubsection{}
\begin{align} 
    & \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)}[Q^{\pi^*}(\tb{s}_1,\tb{a}_1)] - V^{\pi^*}(\tb{s}_1) \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ c(\tb{s}_1,\tb{a}_1) + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)] \} - V^{\pi^*}(\tb{s}_1) \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim   \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - V^{\pi^*}(\tb{s}_1) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{ 1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - (1 + \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)]) \}
    \\
    &=  \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} 
    \{  \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1)}[V^{\pi^*}(\tb{s}_2)]  - \mathbb{E}_{\tb{s}_2 \sim \mathbb{P}(.|\tb{s}_1,\tb{a}_1^*)}[V^{\pi^*}(\tb{s}_2)] \}
    \\
    &= \mathbb{E}_{\tb{a}_1 \sim \pi(\tb{s}_1)} \{ \sum_{\tb{s} \in \mathcal{S}} (\mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1) - \mathbb{P}(\tb{s}|\tb{s}_1, \tb{a}_1^*)) V^{\pi^*}(\tb{s})\} \label{sum of difference of probabilities into V*}
\end{align}

\\
The above just follows from writing the definition of optimum Action value function and doing some rearrangement and remember costs throughout is 1.
\\
\subsubsection{}
In the below proof, we expand the difference in probability term arising in the above equation \ref{sum of difference of probabilities into V*}. The initial global state, $\tb{s}_1$, is with all agents at $\s_{init}$ and the next state, $\tb{s}$, is one where agents in $ \mathcal{I}:=\{i_1,i_2,..,i_r\}$ remain at $s_{init}$ while those in $\mathcal{J}:=\{j_1,j_2,..,j_{n-r}\}$ go to goal node. \\


\begin{lalign}
\mathbb{P}(s|s_1, a_1) - \mathbb{P}(s|s_1, a_1^*)  \label{prob_diff_init}
\\
&= \langle \phi(s|s_1,a_1), \theta \rangle - \langle \phi(s_1|s_1,a_1^*), \theta \rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1), \phi(s_2^{\prime}|s_2, a_2)..., \phi(s_n^{\prime}|s_n,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\& - \langle (\phi(s_1^{\prime}|s_1, a_1^*), \phi(s_2^{\prime}|s_2, a_2^*)..., \phi(s_n^{\prime}|s_n,a_n^*)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle
\\
&= \langle (\phi(s_1^{\prime}|s_1, a_1),..., \phi(s_n^{\prime}|s_n,a_n)) - (\phi(s_1^{\prime}|s_1, a_1^*),..., \phi(s_n^{\prime}|s_n,a_n^*)), \\
& (\theta_1, 1,...,\theta_n,1)\rangle 
\\
&= \sum_{m = 1}^{r} \langle \phi(s_{i_m}^{\prime}|s_{i_m},a_{i_m}) - \phi(s_{i_m}^{\prime}|s_{i_m},a^*_{i_m}), (\theta_{i_m}, 1)\rangle \\ 
& + \sum_{m = 1}^{n-r} \langle \phi(s_{j_m}^{\prime}|s_{j_m},a_{j_m}) - \phi(s_{j_m}^{\prime}|s_{j_m},a^*_{j_m}), (\theta_{j_m}, 1)\rangle 
\\
&= \sum_{m=1}^{r} \langle (-a_{i_m} + a^*_{i_m}, 0), (\theta_{i_m}, 1) \rangle + \sum_{m=1}^{n-r} \langle (a_{j_m}-a^*_{j_m}, 0), (\theta_{j_m}, 1) \rangle   
\\
&= \sum_{m=1}^{r} (\langle a^*_{i_m}-a_{i_m}, \theta_{i_m} \rangle)  + \sum_{m=1}^{n-r} (\langle a_{j_m}-a^*_{j_m}, \theta_{j_m}  \rangle)  
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1} (a^*_{i_m, p} - a_{i_m, p})\theta_{i_m, p} \} + \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1} (a_{j_m, p} - a^*_{j_m, p})\theta_{j_m, p} \}
\\
&= \sum_{m=1}^{r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\} \}  - \sum_{m=1}^{n-r} \{ \sum_{p=1}^{d-1}\frac{2 \Delta}{n(d-1)} \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \}
\\
&= \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\}
\end{lalign}
\\
\\
The initial few lines use the linearity assumption and properties of inner product. Then, split the sum on $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Next lines use definition of $\phi(.,.)$ and $a^*$ as the one matching all signs with $\theta$. We prove this is $a^*$ in all in one theorem \ref{all_in_one}. 
\\

\\


\subsection{\textit{Some Expressions for Transition Probabilities}}
\subsubsection{ \label{stay_at_init} \textit{$\mathbb{P}(\tb{s}|\tb{s},\tb{a})$ where $\tb{s} = (s_{init}, s_{init},\dots,s_{init})$}}

\text{At the global initial state, probability that after taking a global action $\tb{a}$, the next global state is still the same as before i.e., $\tb{s}$}
\begin{lalign}
\mathbb{P}(\tb{s}|\tb{s}, \tb{a})
\\ Linearity Assumption\\
&= \langle \phi(\tb{s}|\tb{s},\tb{a}), \boldsymbol{\theta} \rangle
\\
$Expanded form of features$
\\
&= \langle (\phi(s|s, a_1), \phi(s|s, a_2)..., \phi(s|s,a_n)), (\theta_1, 1, \theta_2, 1,...,\theta_n,1)\rangle \\
$Definition of Inner Product$
\\
&= \sum_{i = 1}^{n} \langle (\phi(s|s, a_i),(\theta_i,1))
\\
$Definition of Features$
\\
&= \sum_{i = 1}^{n} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}),(\theta_i,1) \rangle
\\
&= \sum_{i = 1}^{n} \{ \langle -a_i, \theta_i \rangle + \frac{1-\delta}{n.2^{n-1}} \}
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \langle a_i, \theta_i \rangle 
\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} a_{i,p}. \theta_{i,p} 
\\ $Definition of action and theta$\\
&=  \frac{1-\delta}{2^{n-1}} - \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Taking summation over p inside$ \\
&=  \frac{1-\delta}{2^{n-1}} - 
 \frac{\Delta}{n(d-1)} \sum_{i = 1}^{n}   \Big\{ d-1 - 2 \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
\\ $Just simplify$ 
\\
&=  \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
\end{lalign}

\subsubsection{\textit{ $\mathbb{P}(s'|s,a)$ where $s = \tb{s}_{init}$ and $s':$ arbitrary state}}
\\
In this subsection we derive the expression of probability that if at state $\tb{s} = \{s_{init}, s_{init}, \dots, s_{init}\}$, if global action $\tb{a} = (a_1,a_2,\dots, a_n)$ is taken, you reach $\tb{s}^{\prime}$ where the agents at indices in $\mathcal{I}:= \{ i_1,i_2,\dots, i_r\}$ stay in the same state while agents at indices in $\mathcal{J} := \{j_1,j_2,\dots,j_{n-r} \}$ move to goal state i.e., $s'_{i_1}=s'_{i_2}=\dots=s'_{i_r}=s_{init}$ and $s'_{j_1}=s'_{j_2}=\dots=s'_{j_{n-r}}=goal$. \\
$P(\tb{s}'|\tb{s},\tb{a}) \\ 
= \langle \phi(\tb{s}'|\tb{s},\tb{a}), \theta \rangle \\
= \langle \phi((s'_1,s'_2,\dots, s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n)), (\theta_1, 1, \theta_2, 1,\dots, \theta_n,1) \rangle \\
= \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)),(\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle \phi(s'_i|s_i,a_i), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(s'_j|s_j,a_j), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \langle (-a_i, \frac{1-\delta}{n.2^{n-1}}), (\theta_i, 1) \rangle + \sum_{j \in \mathcal{J}} \langle (a_j, \frac{\delta}{n.2^{n-1}}), (\theta_j, 1) \rangle \\
= \sum_{i \in \mathcal{I}} \Big \{  \frac{1-\delta}{n.2^{n-1}} + \langle -a_i,\theta_i \rangle \Big \} + \sum_{j \in \mathcal{J}} \Big \{ \frac{\delta}{n.2^{n-1}} + \langle a_j, \theta_j \rangle \Big \} \\
= r. \frac{1-\delta}{n.2^{n-1}} - \sum_{i \in \mathcal{I}}    \langle a_i,\theta_i \rangle  + (n-r). \frac{\delta}{n.2^{n-1}} +  \sum_{j \in \mathcal{J}}  \langle a_j, \theta_j \rangle  \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}} -  \sum_{i \in \mathcal{I}} \{ \sum_{p = 1}^{d-1} a_{i,p}.\theta_{i,p} \} + \sum_{j \in \mathcal{J}} \{ \sum_{p = 1}^{d-1} a_{j,p}.\theta_{j,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \{
\sum_{j \in \mathcal{J}}   a_{j,p}.\theta_{j,p}  -  \sum_{i \in \mathcal{I}}  a_{i,p}.\theta_{i,p} \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \Big \{
\sum_{j \in \mathcal{J}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{j,p}) = sgn(\theta_{j,p})\} - \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}} \frac{\Delta}{n(d-1)} \Big[ \mathbbm{1} \{ sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{
\sum_{j \in \mathcal{J}}  \Big[ 1 - 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] -  \sum_{i \in \mathcal{I}}  \Big[   1 - 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\sum_{p = 1}^{d-1} \frac{\Delta}{n(d-1)} \Big \{  \Big[ n-r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\} \Big] - \Big[  r - \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big]   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
\sum_{p = 1}^{d-1}  \Big \{  n-2r - 
\sum_{j \in \mathcal{J}} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} 2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + \frac{\Delta}{n(d-1)} . 
  \Big \{  (d-1)(n-2r) - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} 2.\mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}   + \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  2.\mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   \Big \} \\
= \frac{r + (n-2r). \delta}{n.2^{n-1}}  + 
\frac{\Delta . (n-2r)}{n} +\frac{2 \Delta}{n(d-1)} . 
  \Big \{  \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d-1}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  - 
\sum_{j \in \mathcal{J}} \sum_{p = 1}^{d-1} \mathbbm{1} \{sgn(a_{j,p}) \neq sgn(\theta_{j,p})\}     \Big \} \\
$ 
\\
Initial few lines follow by linearity assumption, definition of features and splitting the dot product over $\mathcal{I}$ and $\mathcal{J}$ as defined earlier. Next few lines simplify the dot product and rearrange terms. Then we use definition of action and theta. The remaining lines simplify the summations and rearrange the terms.
\\
From the above expression, we can observe that this probability in general can vary,  for different states $s' \in \mathcal{S}_{n,r'}$ for any $r' \in [n]$  under given global action  $a = \{a_1,a_2,\dots,a_n\}$ taken at $s = \{s_{init}, s_{init},\dots, s_{init}\}$.  Also observe that when $a=a^*$ this becomes independent of $s'$ for any given $r'$. \\


A more general result of the above relates to transition probability from some $s \in \mathcal{S}_{n,r}$ to some $s' \in \mathcal{S}_{n,r'}(s)$ where $\mathcal{S}_{n,r'}(s)$ represents the possible states of type $r'$ reachable from $s$ i.e.   $0 \leq r' \leq r \leq n$. We discuss this below. \\ 

\subsubsection{\textit{Most General transition probability}}

\textcolor{blue}{below $\mathcal{I}, \mathcal{J} = \mathcal{I}^\prime$ and $\mathcal{T} \cup \mathcal{T}^\prime = [n]$}


\textcolor{blue}{these sets of agents are different from the sets of agents above and is general; general in terms of initial state $s_{init}$ }

Suppose $s$ is such that agents at index in $\mathcal{I}:= \{i_1,i_2,\dots, i_r\}$ are at $s_{init}$ and those at $\mathcal{J} := \{j_1,j_2,\dots, j_{n-r}\}$ are already at goal. Let agents in $\mathcal{T}:=\{t_1,t_2,\dots,t_{r-r'}\} \subseteq \mathcal{I}$ be the ones transiting from $s_{init}$ to $goal$ i.e., $s \in \mathcal{S}_{n,r}$ and $s' \in \mathcal{S}_{n,r'}$ where $n \geq r \geq r' \geq 0$ and $n \geq 1$. \\ \\
$P(s'|s,a)  \\= \langle \phi(s'|s,a), \theta \rangle  \\= \langle \phi((s'_1,s'_2,\dots,s'_n)|(s_1,s_2,\dots,s_n),(a_1,a_2,\dots,a_n) ), (\theta_1,1,\theta_2,1,\dots,\theta_n,1)\rangle  \\ = \langle (\phi(s'_1|s_1,a_1), \phi(s'_2|s_2,a_2),\dots,\phi(s'_n|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots, \theta_n,1) \rangle  \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle \phi(s|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle \phi(g|s,a_t), (\theta_t,1) \rangle \\ 
= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \langle (-a_i, \frac{1-\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j, 1) \rangle + \sum_{t \in \mathcal{T}} \langle (a_t, \frac{\delta}{n.2^{r-1}}), (\theta_t,1) \rangle \\= \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \{ \frac{1-\delta}{n.2^{r-1}} + \langle -a_i, \theta_i \rangle \} + \sum_{j \in \mathcal{J}}   \frac{1}{n.2^{r}}  + \sum_{t \in \mathcal{T}} \{ \langle a_t,\theta_t  \rangle + \frac{\delta}{n.2^{r-1}} \}   \\=  r'. \frac{1-\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}  + (r-r'). \frac{\delta}{n.2^{r-1}} + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} + \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\langle -a_i, \theta_i \rangle  +   \frac{n-r}{n2^{r}}   + \sum_{t \in \mathcal{T}} \langle a_t,\theta_t  \rangle \\ =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} a_{i,p}. \theta_{i,p}      + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   a_{t,p} .\theta_{t,p}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \sum_{p \in [d-1]} \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} -  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]}   \frac{\Delta}{n(d-1)} \Big \{  \mathbbm{1}\{sgn(a_{t,p}) = sgn(\theta_{t,p})\} -  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} - \sum_{i \in \mathcal{I} \cap \mathcal{T'}}  \frac{\Delta}{n(d-1)} \Big \{  d-1 -  2 \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     + \sum_{t \in \mathcal{T}}    \frac{\Delta}{n(d-1)} \Big \{  d-1 - 2\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}} -   \frac{\Delta}{n(d-1)} \Big \{  r'(d-1) -  2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}     +    \frac{\Delta}{n(d-1)} \Big \{  (r-r').(d-1) - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \\=   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n(d-1)} \Big \{  (r-2r').(d-1) + 2 \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - 2 \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\ $

So, we have 
\begin{multline}
\mathbb{P}(s^\prime | s, a) 
=  \\ \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') + \\ \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}   \label{general_prob}
\end{multline}
    


\pt{this incorporates the new features. Also, this will be the optimal probability when the sign matching property holds.}

\textcolor{blue}{we can avoid `line break' commands above } \textcolor{red}{ok, removed them but now proof may seem clumsier}  \textcolor{blue}{ok, we will see a way out, perhaps, we will introduce them}



\textcolor{blue}{we should use available  macros for lemma, proof, etc. see the style file.} 

\textcolor{blue}{these help where the proof starts and importantly ends -- Paul Halmos tomb-stone mark}
\textcolor{red}{ok, this is new for me. i'll try to learn this.}


Initial lines use linearity assumption, definition of features and decomposing the inner product over agents who remain put at $s_{init}$, transit to goal and remain put at goal. In the next few lines, we expand the inner product terms and summations, use the definition of actions and theta and rearrange. Then, just rearrange different terms.  The indicators make sure appropriate sign is given to the dot product depending on signs of components of action and that of theta. \textcolor{blue}{we will cite some papers about these signs }. 

\textcolor{blue}{this is helpful to the reader}

\textcolor{blue}{let's write the role of indicator function above} \textcolor{red}{role as in?}


\\
\\
Notice that for a given global action, the  transition probability from a given $s \in \mathcal{S}_{n,r}$ to a $s' \in \mathcal{S}_{n,r'}$ as long as the transition is possible (i.e., $s' \in \mathcal{S}_{n,r'}(s)$)  depends on the particular $s'$ and is not independent of it even for given global action $a$ in general. Particularly one can observe that when $a=a^*$(one that matches signs with each component of $\theta$), this is independent of which $s'$ is being considered for a given $r'$. 



Another important probability is that of transition to global goal state after taking a global action a in any state $s \in \mathcal{S}_{n,r}$. This is corollory to \ref{general_prob}. \\  \\

 $ P(s'=(g,g,\dots,g)|s,a) \\ = \langle \phi(s' = (g,g,\dots, g)|(s,a)), \theta \rangle \\ = \langle (\phi(g|s_1,a_1), \phi(g|s_2,a_2),\dots, \phi(g|s_n,a_n)), (\theta_1,1,\theta_2,1,\dots,\theta_n,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle \phi(g|s,a_i), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle \phi(g|g,a_j), (\theta_j,1) \rangle \\ = \sum_{i \in \mathcal{I}} \langle (a_i, \frac{\delta}{n.2^{r-1}}), (\theta_i,1) \rangle + \sum_{j \in \mathcal{J}} \langle (0_{d-1}, \frac{1}{n.2^{r}}), (\theta_j,1) \rangle \\ = \frac{r\delta}{n2^{r-1}} + \sum_{i \in \mathcal{I}} \langle a_i,\theta_i \rangle + \frac{n-r}{n2^{r}} \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  a_{i,p} \theta_{i,p} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}} \sum_{p=1}^{d-1}  \frac{\Delta}{n(d-1)} \Big\{ \mathbbm{1}\{sgn(a_{i,p}) = sgn(\theta_{i,p})\} - \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
 \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  + \sum_{i \in \mathcal{I}}  \frac{\Delta}{n(d-1)} \Big\{ d-1 - 2  \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big\} 
  \\ = \frac{r\delta}{n2^{r-1}} + \frac{n-r}{n2^{r}}  +  \frac{r \Delta}{n} - \frac{2 \Delta}{n(d-1)} \sum_{i \in \mathcal{I}}    \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}
 $
\\
\\
This is very similar to above proofs and no new idea is used, only the state is explicitly mentioned.
\\

\textcolor{blue}{write this as another lemma} \textcolor{red}{i had written this before writing the above general proof which is now a lemma. this one is specific for r=n and r'=0 which game me an idea of how to express for general case. should this be a lemma or corollary } \textcolor{blue}{yes, as said over phone. }


%\textcolor{blue}{ think it is $\newtheorem{lemma}{command for new lemma}$}

\subsection{$V^*$ for multiple cases (This hasn't led to any key result by itself yet)}


General formula:  \textcolor{blue}{is this a theorem?} \textcolor{red}{It follows directly from Bellman equation}\\
 $V^*(s) = \{1  + |\mathcal{S}_{n,r-1}(s)| p_{a^*,r-1} V^*_{r-1} +  |\mathcal{S}_{n,r-2}(s)|p_{a^*,r-2} V^*_{r-2} + \dots + |\mathcal{S}_{n,2}(s)| p_{a^*,2} V^*_{2} + |\mathcal{S}_{n,1}(s)| p_{a^*,1} V^*_{1} \} . \{ 1 - P(s|s,a^*) \}^{-1}$

 \\ \\
 Below $p^*_{r,r'}$ denotes transition probability for a valid transition from state of type $r$ to that of type $r'$ under optimal global action in the respective instance specicified by $\theta$ and $n$ and $V^*_0 = 0$ \\ \\
For n = 1 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$ \\ \\ 
For n = 2 \\
For r = 1 \\ 
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For n = 3 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\
For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
\\

For n=4 \\
For r = 1 \\
$V^*_1 = 1 + p^*_{1,1}V^*_1+p^*_{1,0}V^*_0 \implies V^*_1 = \frac{1}{1-p^*_{1,1}}$  \\
For r = 2 \\
$V^*_2 = 1 + p^*_{2,2}V^*_2+\binom{2}{1}p^*_{2,1}V^*_1+\binom{2}{2}p^*_{2,0}V^*_0 \implies V^*_2 = \frac{1+\binom{2}{1}p^*_{2,1}V^*_1}{1-p^*_{2,2}} = \frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} $ \\
\\

For r = 3 \\ 
$V^*_3 = 1 + p^*_{3,3}V^*_3+\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1+\binom{3}{3}p^*_{3,0}V^*_0 \implies V^*_3 = \frac{1 +\binom{3}{1}p^*_{3,2}V^*_2+\binom{3}{2}p^*_{3,1}V^*_1 }{1-p^*_{3,3}} = \frac{1+\binom{3}{1}p^*_{3,2}.\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{3}{2}p^*_{3,1}.\frac{1}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1+\frac{\binom{3}{1}p^*_{3,2}+\frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} }{1-p^*_{3,3}} = \frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}}$ \\
For r = 4 \\
$V^*_4 = 1 + p^*_{4,4}V^*_4 + \binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1+\binom{4}{4}p^*_{4,0}V^*_0 = \frac{1+\binom{4}{1}p^*_{4,3}V^*_3 + \binom{4}{2}p^*_{4,2}V^*_2 + \binom{4}{3}p^*_{4,1}V^*_1}{1-p^*_{4,4}} = \frac{1+\binom{4}{1}p^*_{4,3}\frac{1 + \frac{\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} + \binom{4}{2}p^*_{4,2}\frac{1+\frac{\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \binom{4}{3}p^*_{4,1}\frac{1}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+\frac{ \binom{4}{1}p^*_{4,3} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{1-p^*_{1,1}} 
+\frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{1-p^*_{2,2}} +  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})} }{1-p^*_{3,3}} +\frac{ \binom{4}{2}p^*_{4,2}+\frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{1-p^*_{1,1}}}{1-p^*_{2,2}} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}}  = \frac{1+ \frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}}{1-p^*_{4,4}} = \frac{1+ \frac{\binom{4}{3}p^*_{4,1}}{1-p^*_{1,1}}  + \frac{\binom{4}{2}p^*_{4,2}}{1-p^*_{2,2}}+\frac{\binom{4}{1}p^*_{4,3} }{1-p^*_{3,3}} + \frac{ \binom{4}{1}p^*_{4,3}\binom{3}{2}p^*_{3,1}}{(1-p^*_{1,1})(1-p^*_{3,3})} + \frac{ \binom{4}{2}p^*_{4,2}\binom{2}{1}p^*_{2,1}}{(1-p^*_{1,1})(1-p^*_{2,2})} + \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2}}{(1-p^*_{2,2})(1-p^*_{3,3})} +   
  \frac{\binom{4}{1}p^*_{4,3}\binom{3}{1}p^*_{3,2} \binom{2}{1}p^*_{2,1}}{(1-p^*_{2,2}) (1-p^*_{1,1})(1-p^*_{3,3})}  }{1-p^*_{4,4}}$


\pt{can you see the closed form expression here?} \textcolor{red}{i can see a pattern but can't express it nicely.}

\pt{if not, can you confirm whether this notation is correct? -- $p^*_{r,r'}$ is the probability that number agent in the state $s$ were $r$, and the number of agents in $s'$ are $r'$?} \textcolor{red}{yes, line 308-309}

\pt{also can you recall me here -- what does the  $\binom{4}{2}$ or $\binom{3}{1}$ represent in terms of $r,n,$ and $r'$? $\binom{r}{r-r'}$} \textcolor{red}{yes,in the first factor of every term in the numerator}

\pt{I will try to get the closed form expression once you mention this.} \textcolor{red}{if you can get this it will be good to add}


\pt{Also can you summarize what are the intermediate results we have. summarize all of them no matter how  trivial or useful they are are. } \textcolor{red}{The general probability expression , The all in one result: $a^*$ is same for all states and is the one matching signs with each component of $\theta$, $V^*$ is same for all states of a particular type, $V^*$ are ordered and (due to) the claim on probabilities hold}

\pt{I can see  that you have many intermediate results.}












\textcolor{blue}{let's write here the  intermediate steps with pending proofs }
\textcolor{red}{done as of now, thought there's a pattern, to express it mathematically is a bit challenging, i'll try to think about this}

\subsection{NOT DIRECTLY USEFUL FOR US: Important result regarding monotonicity of V*, an independent result , and a result with weaker sufficient is stated and used below} \\

Consider the states space, $\mathcal{S} = \{s_1,s_2,\dots,s_n\} \cup \{x,y\} $. Let under some global action, the following markov chain be induced:
\\ Cost for any transition is constant and equal to 1. Transition probability from x to $s_i$ is represented as $p_{x,i}$ and from y to $s_i$ as $p_{y,i}$ for $i \in \{1,2,\dots,n\}$ and $p_{x,x}$ and $p_{y,x}$ represent the same from x and y respectively to x. Probability from y to y is represented as $p_{y,y}$. All probabilities are considered between 0 and 1 (strictly). Further, it holds that $p_{y,s} = p_{x,s} - \delta_s$ for every $s\in \{x,1,2,\dots,n\}$ where all $\delta_s \in (0, p_{x,s})$. (We would later require that assuming $p_{x,(.)}$ is monotonic, $\delta_s$'s are such that they preserve the monotonicity of $p_{y,(.)}$. But this assumption on $\delta_s$'s is not required in this discussion.) No other transitions are possible. For the sake of discussion, we assume that the states $s_1,s_2,\dots,s_{n}$ are absorbing states (potentially there may be all kinds of transitions from there but the long term value is known hence they can be considered terminal states with these values) with value function known respectively as $V_1,V_2,\dots,V_n$ while value of state $x$ is also known as $V_x$. Assume the following condition holds for the values: $V_1<V_2<\dots<V_n < V_x$. We want to relate $V_x$ and $V_y$. \\ \\
\tb{Claim:} $V_x < V_y$ \\ \\
$p_{y,y} = 1-p_{y,x}-\sum_{i=1}^{n}p_{y,i} = 1-(p_{x,x} - \delta_x) - \sum_{i=1}^n(p_{x,i}-\delta_i) = \delta_x + \sum_{i=1}^n \delta_i$ \\ \\
$V_x = \sum_{i=1}^np_{x,i}(1+V_i)+p_{x,x}(1+V_x)$ \\ \\
Similarly, \\
$V_y = \sum_{i=1}^np_{y,i}(1+V_i) + p_{y,x}(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^n(p_{x,i}-\delta_i)(1+V_i) + (p_{x,x}-\delta_x)(1+V_x)+p_{y,y}(1+V_y) = \sum_{i=1}^np_{x,i}(1+V_i) + p_{x,x}(1+V_x)-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_i)\} + p_{y,y}(1+V_y) $ \\ \\
From the definition of $V_x$ above and monotonicity of V's, we have : \\
$V_y > V_x-\{\delta_x(1+V_x)+\sum_{i=1}^n\delta_i(1+V_x)\} + p_{y,y}V_y = V_x-p_{y,y}(1+V_x) + p_{y,y}(1+V_y) \\ \implies V_y - V_x > p_{y,y}(V_y -V_x) \\ \implies (1-p_{y,y}) (V_y - V_x) > 0 \\ \implies V_y>V_x $

 \\ 


\subsection{ \label{all_in_one} \textit{ALL IN ONE THEOREM} - $a^*$ is the one that matches sign with $\theta$ for every state, $V^*$ is same for states of a particular type, there exists ordering of $V^*$'s : all go hand-in-hand \textcolor{blue}{lines after \ref{regret} are basic and hence need to be cross-checked}} 
\tb{Base Case}  \\ By definition, $V^*_0 = 0$. \\
Take any $s \in \mathcal{S}_{n,1}$. \\
\tb{Q.} What is $a^*$? \\
For s, only possible next global states are s itself and all-at-goal (g). This is akin to the single agent problem. But any transition probability also depends on actions of others. \\
Suppose $p^a_{s,g}$ denotes the transition probability from s to g. Then we have, \\
$V^a_1(s) = (1-p^a_{s,g}).(1+V^a_1(s)) + p^a_{s,g}.(1+V_0) \implies V^a_1(s) = \frac{1}{p^a_{s,g}}$ \\
Thus the optimum action at s is the one that minimizes $V^a_1(s)$ i.e., maximizes $p^a_{s,g}$. From the above general equation \ref{general_prob}, the transition probability is maximum when $a$ is such that it matches all signs with $\theta$ for the respective components of agent who was initially at s. The signs of other components do not matter. Hence there could be multiple $a^*(s)$ for any particular $s \in \mathcal{S}_{n,1}$.\\
Notice that this will hold true for any $s \in \mathcal{S}_{n,1}$. Note that particular $a^*$ whose sign matches with components of $\theta$ (for every agent), is common for possible $a^*$ for every $s \in \mathcal{S}_{n,1}$. We consider this $a^*$ in particular. \\
Since from the general formula \ref{general_prob}, for a fixed instance ($\theta$), for given action $a^*$ the probability only depends on r and r', it is the same for all states s $\in \mathcal{S}_{n,1}$ i.e., $p^{a^*}_{s,g} = p^{a^*} \forall s \in \mathcal{S}_{n,1}$. This $V^*_1(s) = V^*_1 \forall s \in \mathcal{S}_{n,1}$ \\
Since transition probability for this action is strictly between 0 and 1, $V^*_1 > V^*_0=0$ \\
\tb{Generalization/Induction} \\
Now, let us assume that for all $k \in \{0,1,2,\dots,r\}$, it holds that:\\ $a^*$ is the one that matches sign with $\theta$ for any state in $\mathcal{S}_{n,k}$, hence from \ref{general_prob} and definition of $a^*$, $p^*(s \in \mathcal{S}_{n,k}  \xrightarrow{}s' \in \mathcal{S}_{n,k'}(s)) = p^*_{k,k'}$, $V^*_k(s)=V^*_k$ for any $s \in \mathcal{S}_{n,k}$ and $V^*_k>V^*_{k-1}$. Now, we need to show the same for $r+1$. \\
Consider any $s \in S_{n,r+1}$. \\
$V^a(s) = \sum_{s' \in \mathcal{S}(s)\textbackslash \{s,g\}} P(s'|s,a)\{1+V^*(s')\} + P(s|s,a).\{1+V^a(s)\} + P(g|s,a).\{1+V^*(g)\}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +\sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} p^a_{r+1,r'}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'}  +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \sum_{i \in [n]} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \Bigg \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} V^*_{r'}\Bigg \} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{i \in \mathcal{T}\}  \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]}  \Big \{ \binom{r}{r'-1} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} - \binom{r}{r'} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big  \}V^*_{r'} \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{2 \Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r+1-r'-1}  - \binom{r}{r+1-r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r'}  +  \{ \binom{r}{r'}  - \binom{r}{r'-1} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*_{r+1-r'} \Big  \}  \\= 1+P(s|s,a)V^a(s) +P(g|s,a)V^*(g) +  \sum_{r' \in [r]}  \Bigg\{(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r')).\binom{r+1}{r'} \Bigg \} V^*_{r'} +  \frac{\Delta}{n(d-1)}  \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]}  \Big \{ \{ \binom{r}{r'-1}  - \binom{r}{r'} \} . \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . (V^*_{r'}  - V^*_{r+1-r'}) \Big  \}$ \\ 
Observe that the third term is always non negative since when $r'>(r+1)/2$ the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \geq 0$ as well as $V^*_{r'} >V^*_{r+1-r'}$ while for $r' \leq (r+1)/2$, $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as $V^*_{r'} \leq V^*_{r+1-r'}$. Note that the above arguments is for $r' \in [r]$. To minimize $V^a(s)$, we need to minimize $P(s|s,a)$ as well (check after rearrangement as it will appear in denominator as 1-P). Clearly, the action that matches sign with all components of $\theta$ minimizes $V^a(s)$ since it makes sure that the non-negative additive terms are all zero as well as P(s|s,a) is minimised. Hence this is $a^*$. Notice the above arguement holds for any $ s \in \mathcal{S}_{n,r+1}$. Hence $a^*$ is the same for each of them. Hence $p^*(s \in \mathcal{S}_{n,r+1} \xrightarrow{}s' \in \mathcal{S}_{n,r'}(s)) = p^*_{r+1,r'}$. Hence $V^*(s) = V^*_{r+1}$ for each of them. \\

\\ \\
Proving $V^*_{r+1} > V^*_r$ is tricky. We will make a suitable assumption on probabilities and later show that it holds under suitable choices of $\delta$ and $\Delta$. \\
\tb{Claim} If for every $r \in [n-1]$, it holds that for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,\lfloor \frac{r+1}{2} \rfloor +2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$, then,  $V^*_r>V^*_{r-1}>\dots>V^*_{1}>V^*_{0}=0 \implies V^*_{r+1}>V^*_r$.  \\
We will justify that the assumption on probabilities in this claim holds for our features under suitable $\delta$ and $\Delta$. For now lets assume this holds for our case and prove the implication part of claim. \\
Return to the induction argument. \\
$V^*_r = 1+\sum_{r' \in \{0,1,\dots,r\}}\binom{r}{r'}V^*_{r'}$ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'}$ \\
Suppose for every $r' \in \{0,1,2,\dots,\lfloor\frac{r+1}{2}\rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}-\delta_{r'} $ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor\ +1 , \lfloor\frac{r+1}{2}\rfloor+2,\dots,r-1,r\}$, $\binom{r+1}{r'} p^*_{r+1,r'}=\binom{r}{r'}p^*_{r,r'}+\delta_{r'} $ where $\delta_{r'}>0$ for every $r' \in \{0,1,\dots,r\}$\\ 
Note that, $\sum_{r' \in \{ 0,1,\dots,r,r+1\}} \binom{r+1}{r'}p^*_{r+1,r'} = 1 \\ \Leftrightarrow\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r+1}{r'}p^*_{r+1,r'} + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r+1}{r'}p^*_{r+1,r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \Leftrightarrow \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} (\binom{r}{r'}p^*_{r,r'}-\delta_{r'}) + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} (\binom{r}{r'}p^*_{r,r'} + \delta_{r'}) + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \Leftrightarrow \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \binom{r}{r'}p^*_{r,r'}-\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} + \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + \binom{r+1}{r+1} p^*_{r+1,r+1} = 1 \\ \Leftrightarrow p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} + 1 -  \sum_{r' \in \{0,1,\dots,r-1,r\}} \binom{r}{r'}p^*_{r,r'} \\ \Leftrightarrow p^*_{r+1,r+1} = \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'}  -  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'} $ \\ \\
Now, going back to $V^*_{r+1}:$ \\ \\
$V^*_{r+1} = 1 + p^*_{r+1,r+1}V^*_{r+1} + \sum_{r' \in \{0,1,\dots,r\}}\binom{r+1}{r'} p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}\binom{r+1}{r'}p^*_{r+1,r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}(\binom{r}{r'}p^*_{r,r'} - \delta_{r'})V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}}(\binom{r}{r'}p^*_{r,r'}+\delta_{r'})V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +  \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \binom{r}{r'}p^*_{r,r'} V^*_{r'}+ \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ = 1 + p^*_{r+1,r+1}V^*_{r+1} +\sum_{r' \in \{0,1,\dots, r-1,r\}}\binom{r}{r'}p^*_{r,r'}V^*_{r'} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\=  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{r'}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{r'} \\ > p^*_{r+1,r+1}V^*_{r+1} + V^*_{r} - \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} V^*_{\lfloor \frac{r+1}{2} \rfloor + 1}  +   \sum_{r' \in \{ \lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  (  \sum_{r' \in \{0,1,\dots, \lfloor \frac{r+1}{2} \rfloor\}} \delta_{r'} - \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2, \dots, r-1,r \}} \delta_{r'}  )V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ = p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_{\lfloor \frac{r+1}{2} \rfloor +1} \\ >  p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r $ \\ 
Thus,\\
$V^*_{r+1} >   p^*_{r+1,r+1}V^*_{r+1} + V^*_{r}   -  p^*_{r+1,r+1}V^*_r \Leftrightarrow (1-p^*_{r+1,r+1})(V^*_{r+1}-V^*_r)>0 \Leftrightarrow V^*_{r+1} > V^*_r$ \\
Above inequalities used monotonicity of $V^*$ due to induction assumption. \\
Below we justify that the assumption in the above claim holds for our case( \ref{sufficiency} combined with \ref{justification}).

\subsection{ \label{sufficiency}\textit{Sufficient conditions on $\delta$ and $\Delta$ for well defined probabilities}; \textcolor{blue}{$\delta$ is conflicting with high probability $\delta$}}

$p^a_{r,r'} < 1$ for every $r \in \{1,2,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$for every $a$ and instance $\theta$. \\
From general probability formula \ref{general_prob}:
\\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \\ \leq    \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{1} \\ \leq   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{\frac{n-r}{2}}{n2^{r-1}}        +    3\Delta \\ =  \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} +    3\Delta \\ =  \frac{(r'-0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} +    3\Delta \\ \leq  \frac{0.5n(2-2\delta)}{n.2^{r-1}} + 3\Delta \\ \leq  1-\delta + 3\Delta$ \\
To ensure $p^a_{r,r'}<1$ it is sufficient to ensure $1-\delta + 3\Delta<1 \Leftrightarrow \delta > 3\Delta$ \\
Similarly, we must ensure, $p^a_{r,r'} > 0$ for every $r \in \{0,1,\dots,n\}$ for every $r' \in \{0,1,\dots,r\}$. \\
$p^a_{r,r'}  =   \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \} \\  \geq  \frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r') -  \frac{2 \Delta}{1}  \\ \geq  \frac{r'(1-2\delta) + r(\delta-0.5) + 0.5n}{n.2^{r-1}} - 3\Delta \\ =  \frac{(r' -0.5r)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta \\ \geq  \frac{( -0.5n)(1-2\delta) + 0.5n}{n.2^{r-1}} - 3\Delta = \frac{ \delta }{2^{r-1}} - 3\Delta$ \\
To ensure, $p^a_{r,r'} > 0$ it is sufficient to ensure $ \frac{ \delta }{2^{r-1}} - 3\Delta > 0  \Leftrightarrow \delta > 3.2^{n-1}.\Delta$. \\ Observe that since $n \geq1$, condition from $p>0 \implies $ condition from $p<1$  Also note that in the above, we have assumed $\delta < 0.5$. Hence we can fix any $\delta, \Delta $ and $n$ that satisy the above conditions in order to fix a class of instance as above.




\subsection{ \label{justification} \textit{Justification of assumption in the claim}} 
Recall that in the above claim, we assumed that: for every $r \in [n-1],$ for every $r' \in \{0,1,\dots,\lfloor \frac{r+1}{2} \rfloor\}$, $\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'}$ and for every $r' \in \{\lfloor \frac{r+1}{2} \rfloor +1,  \lfloor \frac{r+1}{2} \rfloor+2,\dots,r-1,r \}$, $\binom{r+1}{r'} p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'}$. \\
Below, we will derive sufficient conditions on $\delta$ and $\Delta$ such that this assumption holds. \\
Also note that from above section \ref{sufficiency} we have $\delta<0.5$ and $\delta>3.2^{n-1}\Delta$ so that all probabilities are well defined.
\\ \\
\tb{For $r'\leq \lfloor\frac{r+1}{2}\rfloor$}, \\
$\binom{r+1}{r'} p^*_{r+1,r'}<\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \frac{r+1}{r+1-r'}p^*_{r+1,r'}<p^*_{r,r'} \Leftrightarrow \\(r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \\ \Leftrightarrow  (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \\ \Leftrightarrow (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')<(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \\ \impliedby (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) <0  \impliedby \frac{\Delta}{n}\frac{r^2}{8} + (r+1) \frac{\Delta}{n}<(r+1)\frac{1-2\delta}{n2^{r+1}} \Leftrightarrow\frac{\Delta}{n}(\frac{r^2}{8}+r+1)<(r+1)\frac{1-2\delta}{n2^{r+1}} \impliedby \Delta (\frac{n^2}{8}+n+1)<\frac{1-2\delta}{2^{n}} \Leftrightarrow \Delta < \frac{1-2\delta}{2^{n}(1+n+\frac{n^2}{8})} \impliedby \Delta < \frac{1-2\delta}{2^{n}(1+n+n^2)}$  \\ \\
Similarly, \\ \tb{For $r' > \lfloor \frac{r+1}{2} \rfloor$}, \\ 
$\binom{r+1}{r'}p^*_{r+1,r'}>\binom{r}{r'}p^*_{r,r'} \Leftrightarrow \\ \frac{r+1}{r+1-r'}p^*_{r+1,r'}>p^*_{r,r'} \Leftrightarrow \\ (r+1).(\frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r' + (r-2r')\delta}{n.2^{r-1}} +   \frac{n-r}{n2^{r}}        +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow \\ (r+1).(\frac{r'(1-2\delta)+r(\delta-0.5)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{r'(1-2\delta)+r(\delta-0.5)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r'))  \Leftrightarrow \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+\delta-0.5+0.5n }{n.2^{r}}    +    \frac{\Delta}{n}  (r+1-2r'))>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}    +    \frac{\Delta}{n}  (r-2r')) \Leftrightarrow  \\ (r+1).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n})     +    (r+1)\frac{\Delta}{n}  (r-2r')>(r+1-r').(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}})    +  (r+1-r')  \frac{\Delta}{n}  (r-2r') \\ \Leftrightarrow (\frac{2r'-(r+1)}{2}).(\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r-1}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0  \impliedby  (\frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}}) +  (r')\frac{\Delta}{n}  (r-2r') + (r+1)(\frac{\delta-0.5}{n.2^{r}} + \frac{\Delta}{n}) >0 \\ \Leftrightarrow \frac{(r'-0.5r)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2) - 0.5(r+1)(\frac{1-2\delta}{n.2^{r}}) >0 \\ \Leftrightarrow \frac{(r'-r-0.5)(1-2\delta)+0.5n }{n.2^{r}} +  \frac{\Delta}{n}  (1+r+r.r'-2r'^2)  >0 \impliedby \frac{(-r-0.5)(1-2\delta)+0.5n }{n.2^{r}}   >   \frac{\Delta}{n}  (r^2-r-1)  \Leftrightarrow \frac{(-r-0.5)(1-2\delta)+0.5n }{1}   >   \frac{\Delta}{1}  (r^2-r-1)  (2^{r}) \\ \impliedby (-n-0.5)(1-2\delta)+0.5n    >   \Delta  (n^2-n-1)  (2^{n})$ and $ (-n-0.5)(1-2\delta)+0.5n    > 0 \\ \impliedby 0.5n-n+2n\delta-0.5+\delta>0$ and $ 0.5n-n+2n\delta-0.5+\delta >   \Delta  (n^2+n+1)  (2^{n}) \\ \impliedby (2\delta-0.5)n>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2+n+1)  (2^{n}) \\ \impliedby 2\delta-0.5>0.5-\delta$ and $ (2\delta-0.5)n > 0.5-\delta+  \Delta  (n^2+n+1)  (2^{n}) \\ \Longleftrightarrow \delta>\frac{1}{3}$ and $n > \frac{0.5-\delta}{2\delta-0.5}+ \frac{\Delta  (n^2+n+1)  (2^{n})}{2\delta-0.5} \\ \impliedby \delta>1/3 $ and $\Delta  (n^2+n+1)  (2^{n})<3\delta-1 \impliedby \Delta < \frac{3\delta-1}{(n^2+n+1).2^{n}}$ \\ 
\\
Finally we obtain (from current subsection and \ref{sufficiency}), for the desired instance, fix $1/2>\delta>1/3$. Then, fix, $\Delta< 2^{-n}.min\{\frac{3\delta-1}{n^2+n+1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2}\}$ \\
\label{final_conds}


\subsection{\textit{Simplification of Q-V difference from above} \ref{eq_Q_V}\textcolor{blue}{this is advantage function, isn't?}} \textcolor{red}{yes, it's like expected value of the advantage function since there is expectation over $a_1$ according to the policy \\ also i've modified below for new features}
\\
\\
From \ref{q_v} we have the following. In the below, $s_t$ represent global state at time t (Note it's not individual state), $\textbf{s}_t$. Similarly $a_t$ is global action at t. In the below, we ignore writing $k$ and $\theta$ in $\pi^k_{\theta}$ and $V^*_{\theta}$ to avoid clutter as it is understood in the context:

\begin{lalign} 

$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^*(s_1,a_1)] - V^* \\
= \mathbb{E}_{a_1 \sim \pi(s_1)}[c(s_1, a_1) + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}V^*(s_2)] - V^*(s_1)  $ \\
Using Bellman Equation and cost is 1
\\ 
$=  \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{  1 + \mathbb{E}_{s_2 \sim \mathbb{P}(.,s_1,a_1)}[V^*(s_2)] - V^*(s_1) \Big \}$
\\ Expand the Expectation $ \\
=   \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  P(s_1|s_1,a_1) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1) \Big \}
\\ $ Use expression of probability from above \ref{stay_at_init}$
 \\= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta +
  \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2)  - V^*(s_1) \Bigg \}
\\$ Rearranging the terms $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +  \Big \{ \frac{1-\delta}{2^{n-1}} - \Delta \Big \}  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*(s_2) - V^*(s_1)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n}     \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} . V^*(s_1) \Big\} 
\\ $ Notice from the general expression of probability from previous proof \ref{general_prob} $\\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ 1 +P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - V^*(s_1) \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} 
\\$ Expand V*(s_1) $ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Bigg\{ 1 + P(s_1|s_1,a_1^*)  V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1,a_1)V^*_{s_2} - \Big\{ 1 +  P(s_1|s_1,a_1^*) V^*(s_1) + \sum_{s_2 \neq s_1} P(s_2|s_1, a_1^*) V^*(s_2) \Big\} \Bigg \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p})\neq sgn(\theta_{i,p})\} V^*(s_1) \Big\} 
\\$   

Rearrange and combine  terms to have a  lower bound 

$ \\
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $
\end{lalign}
\label{q_v_simp}

\\



\subsubsection{\textit{Dealing with the sum of Probability differences above}} 

Recall from earlier \ref{q_v_simp}, \\ 
$\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)   
= \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2)  \Big \} + \\
 \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 The first term is problematic and it is not clear how to deal with it. Let's investigate the summation inside the expectation of the first term: \\ 
 $\sum_{s_2 \neq s_1} [P(s_2|s_1,a_1)-P(s_2|s_1, a_1^*)] V^*(s_2) \\ = \sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} [P(s'|s_1,a_1)-P(s'|s_1, a_1^*)] V^*(s') $ (Now, use results from above sections \ref{prob_diff_init}) \\
 = $\sum_{r\in[n-1]} \sum_{s' \in \mathcal{S}_{n,r}} \frac{2 \Delta}{n(d-1)} \sum_{p=1}^{d-1} \Big\{\sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p})\} \Big\} V^*_r $ \\
= $\frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{\sum_{s' \in \mathcal{S}_{n,r}} [\{   \sum_{m=1}^{r}   \mathbbm{1} \{sgn(a_{i_m,p}) \neq sgn(\theta_{i_m,p})\}   - \sum_{m=1}^{n-r}  \mathbbm{1} \{sgn(a_{j_m,p}) \neq sgn(\theta_{j_m,p}) \}]  \Big\}   \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n}   
 \sum_{s' \in \mathcal{S}_{n,r}} [ \mathbbm{1}\{s'_i = s_{init}\}   \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}   - \mathbbm{1}\{s'_i = goal\}  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \}]  \Big\} \\
= \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  
 \sum_{s' \in \mathcal{S}_{n,r}} \mathbbm{1}\{s'_i = s_{init}\}     -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \sum_{s' \in \mathcal{S}_{n,r}} 
 \mathbbm{1}\{s'_i = goal\} \Big\}  \Big\} 
 \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1} \Big\{ \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \binom{n-1}{r-1}    -  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p}) \} \binom{n-1}{r} \Big\}  \Big\} \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \{ \binom{n-1}{r-1}    -   \binom{n-1}{r} \} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)} \sum_{r\in[n-1]} V^*_r \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} V^*_r  \frac{2r-n}{n} \binom{n}{r} \Big\}   \\
 = \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} + V^*_{n-r}  \frac{2(n-r)-n}{n} \binom{n}{n-r} \} \Big\}   \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  \frac{2r-n}{n} \binom{n}{r} - V^*_{n-r}  \frac{2r-n}{n} \binom{n}{r} \} \Big\}  \\
= \frac{2 \Delta}{n(d-1)}  \sum_{p=1}^{d-1}  \sum_{i=1}^{n} \Big \{  \mathbbm{1} \{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \sum_{r\in[n-1]} 0.5 . \{V^*_r  - V^*_{n-r}   \} \frac{2r-n}{n} \binom{n}{r} \Big\} \geq 0. 
 $ \\
 \\
 Observe that when $r> n/2, V^*_r > V^*_{n-r}$ and vice-versa (refer result above) \\
 Hence we have established that, \\
 $\mathbb{E}_{a_1 \sim \pi(s_1)}[Q^{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1) \geq \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \label{q_v_further_simp} \\ \\
 In the above we showed the inequality for $s_1=(s_{init},s_{init},\dots, s_{init})$. Using similar arguments same inequality can be shown to hold for any $s_1 \in \mathcal{S}$. We will use this general result below.

 \subsection{\textit{Back to Lower Bound Proof}}
 From earlier \ref{eq_Q_V}, expected regret in the $k-th$ episode: \\
$R_{\theta,k} \\ = V^{\pi_\theta}(s_1) - V^*(s_1) 
\\ 
 = \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)}[Q_{\pi^*}(s_1,a_1)] - V^{\pi^*}(s_1)$ \\
\\ Using above result \ref{q_v_further_simp}, \\
 $R_{\theta,k} \\ \geq  \mathbb{E}_{a_1 \sim\ \pi(s_1), s_2 \sim\ \mathbb{P}(.|s_1,a_1)}[V^{\pi}(s_2) - V^*(s_2)] + \mathbb{E}_{a_1 \sim \pi(s_1)} \Big\{ \frac{2 \Delta}{n(d-1)} \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_1 \neq goal \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}V^*(s_1) \Big\} $ \\
 By recursion and the generalized result from the section above,
 we have: \\

 $R_{\theta,k} \\ \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{h=1}^{\infty} \mathbb{E}_{k} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_h \neq goal \} \mathbbm{1}\{sgn(a^h_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}  $ \\
 where, the Expectation is taken with respect to trajectory induced in the $k-th$ episode by the interaction of policy $\pi$ and transition kernel $P_{\theta}$. Now, the total expected regret over $K$ episodes is: \\
 $
 R_{\theta}(K) \\
 \geq   \frac{2 \Delta V^*_1}{n(d-1)} \sum_{t=1}^{\infty} \mathbb{E}_{\theta, \pi} \Big\{  \sum_{i = 1}^{n} \sum_{p=1}^{d-1} \mathbbm{1}\{s_t \neq goal \} \mathbbm{1}\{sgn(a^t_{i,p}) \neq sgn(\theta_{i,p})\} \Big\}
 $ \\
 Analogous to Min et al, Cohen et al, we define: \\
 $N = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} $ and for agent $i \in [n]$, $j \in [d-1]$,\\
$N_{i,j}(\theta) = \sum_{t=1}^{\infty} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta_{i,j})\} $  \\
Thus, $R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]} \sum_{j=1}^{d-1} N_{i,j}(\theta) \}$ \\
To use the standard Pinsker's Inequality, we need $N_{i,j}(\theta)$ to be bounded almost surely which is known to not hold for SSPs (Min et al, Cohen et al). Hence, we use the capping trick introduced by Cohen et al and also used by Min et al. In this trick, we cap the learning process to a predetermined T. If the learning process (i.e. $K-th$ episode) ends before this, the agents continue to remain at $goal$. In this case the summation for the actual process and the capped process is the same. On the other hand when K episodes end beyond T, we have a truncated sum. Due to non-negativity of each part, the sum for the capped process lower bounds the actual sum. \\ Define \\ $N^- = \sum_{t=1}^T\mathbbm{1}\{s_t \neq goal\} $ and for any agent $i \in [n] $ and $ j \in [d-1],$\\ $N^-_{i,j}(\theta) = \sum_{t=1}^{T} \mathbbm{1}\{s_t \neq goal\} \mathbbm{1}\{sgn(a^t_{i,j}) \neq sgn(\theta_{i,j})\} $ \\ 
It is easy to see that for any $i \in [n]$ and $j \in [d-1]$, $N^- =   N^-_{i,j}(\theta) + N^-_{i,j}(\theta^{j})  $ \\ where for every $\theta$, $\theta^j$ represents the vector that only differs at the $j-th$ index of every $\theta_i$ in $\theta = \{\theta_1,1,\theta_2,1,\dots,\theta_n,1\}$, where each $\theta_i \in \{\frac{-\Delta}{n(d-1)}, \frac{\Delta}{n(d-1)}\}^{d-1}$. \\  
Thus,  $R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}$n(d-1)} \mathbb{E}_{\theta, \pi}  \{ \sum_{i \in [n]}\sum_{j=1}^{d-1} N^-_{i,j}(\theta) \}$.  Notice that $\theta \in \Theta \iff \theta^{j} \in \Theta$ (This follows from definition of $\Theta$ \textcolor{red}{without this, following equation won't hold}). Then, we have: \\
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \{ \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi} [N^-_{i,j}(\theta^{j})] \} \\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^- - N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] + \mathbb{E}_{\theta^{j}, \pi}  [N^-] - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}
\\
= \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1}  \{  \mathbb{E}_{\theta, \pi}  [N^-] + \mathbb{E}_{\theta, \pi} [N^-_{i,j}(\theta)]   - \mathbb{E}_{\theta^{j}, \pi}[N^-_{i,j}(\theta)] \}

Generalisation of Lemma C2 in Cohen et al 2020: If $T \geq 2KB^*$, then $\mathbb{E}_{\theta}[N^-] \geq KB^*/4$  \\ Proof given below \ref{generalise_cohen}. We pick $T = 2KB_*$ \\
\textbf{Pinsker's Inequality(Min et al, Lemma E.3)} \pt{$TV(p,q) \leq \sqrt{KL(p,q)}$}

If $f:S^T\xrightarrow{}[0,D]$ then, 
$\mathbb{E}_{\mathcal{P}_1} (f(s)) - \mathbb{E}_{\mathcal{P}_2} (f(s))\leq D \sqrt{\frac{log(2)}{2}}. \sqrt{ KL(\mathcal{P}_2 || \mathcal{P}_1)}$  

\pt{Note that this will hold only if $|f(s)| \leq D \sqrt{\frac{log(2)}{2}}$?}
\textcolor{red}{I dont think so. $|f(.)|$ can be D}


\pt{don't use double back slash. These are not needed. just give one line spacing.}

Then, 
$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta V^*_1}{n(d-1)} \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  \mathbb{E}_{\theta, \pi}  [N^-] +  \{ \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] - \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] \} \Big \} \\ \geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{  \mathbb{E}_{\theta^{j}, \pi}  [  N^-_{i,j}(\theta)] - \mathbb{E}_{\theta, \pi}  [N^-_{i,j}(\theta)] \} \Big \} \\ 
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KB^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
$

\textcolor{blue}{to update the above relations, equalities and inequalities } \textcolor{red}{done}
\\
\\
\\
 We have the following for our case (proof:\ref{simplify_kld}): \\
For appropriate $\delta$ and $\Delta$:
$ KL(\mathcal{P_{\theta}||\mathcal{P_{\theta^j}}}) \leq  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-] $
\\


$ 2 \sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq \frac{2 \Delta V_1^*}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{log(2)/2} \sqrt{KL(\mathcal{P}_{\theta}||\mathcal{P}_{\theta^{j}})}  \} \Big \} \\
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{1/2} \sqrt{3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]}  \} \Big \} \\
= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{\mathbb{E}_{\theta}[N^-]} \Big \} \\
\geq \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -  \{ T \sqrt{3/2}   \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} . \sqrt{T} \Big \} \\
= \frac{2 \Delta V^*_1}{n(d-1)}  \sum_{\theta \in \Theta} \sum_{i \in [n]} \sum_{j=1}^{d-1} \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \} \\ 
$\\
Notice that the term in bracket is independent of $\theta, i$ or $j$. Thus, we have: \\
$\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq  \Delta V_1^* |\Theta| \Big \{  KV_1^*/4 -   (2KV_1^*)^{3/2} \sqrt{3/2} \frac{2^{n}.\Delta}{\sqrt{\delta} (d-1)} \Big \} \\
\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \\ \geq   V_1^*  \Big \{ \Delta  KV_1^*/4 -   (KV_1^*)^{3/2}  \frac{2^{n+2}.\Delta^2}{\sqrt{\delta} (d-1)} \Big \} \\ 
$ 
Specifically, pick, $\Delta^* = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}$. \\ At this value of delta,\\
$\frac{1}{|\Theta|}\sum_{\theta \in \Theta} R_{\theta}(K) \geq V_1^* \{  \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}}. \frac{KV_1^*}{4} - \frac{(KV_1^*)^{3/2}.2^{n+2}}{\sqrt{\delta}(d-1)}.  (\frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}})^2\} \\ 
= V_1^* \{\frac{(d-1) \sqrt{\delta.K.V_1^*}}{2^{n+7}} - \frac{(d-1)\sqrt{\delta.K.V_1^*}}{2^{n+8}}\}
\\
\geq  \frac{(d-1).\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+8}} \geq \frac{d.\sqrt{\delta}.\sqrt{KV_1^*}}{2^{n+9}} $ \\ \pt{This makes it independent of number of agents, a very strong result? Is this correct or do we need to incorporate the number of agents here.} \textcolor{red}{potentially the intermediate results I used directly without verifying depend on n. the term i argued to be $+ve$ and ignored in lower bound certainly depends on n but very difficult to simplify(needs closed form V*)} \\
\textcolor{red}{update : it depends on n}

Since the average over entire set is lower bounded by the RHS, there must exist some parameter in the set for which the RHS is a lower bound. Hence proved. \textcolor{blue}{ok we will discuss the proof}. \\ \\
It remains to show that the $\Delta$ picked above is valid. \\ Hence, need to ensure that $\Delta = \frac{(d-1) \sqrt{\delta}}{2^{n+5} \sqrt{KV_1^*}} < 2^{-n}.min\{\frac{3\delta-1}{n^2+n+1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2}\}$  \\ or, $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.min^2\{\frac{3\delta-1}{n^2+n+1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2}\}} $
\\ \\
\textcolor{blue}{updated later} \textcolor{red}{Although it is independent of $n$, it can be interpreted as a strong result in the sense that no matter how many agents are deployed to learn, this minimum regret will always hold. The independence also comes from ignoring the positive terms} \\ \textcolor{red}{(whose proof is as of now still incomplete )}. \\ \textcolor{red}{since now there is a dependence on $n$, the above para is not valid} 

\textcolor{blue}{we need to write the  statement that is proved, and also delineate that statement from the proof -- use macros provided in the style file} \textcolor{red}{This is not complete yet. Only if we can find the corresponding lemmas I've mentioned in the proof, it will be complete possibly with very different expression.} \\
\\
\textcolor{blue}{2/4/25} \textcolor{red}{The proof is now complete! Now we have one complete result!}
\\ 
\\
\textcolor{red}{3/4/25} \\
\tb{Theorem}: For any MASSP learning algorithm $\mathfrak{A}$, there exists a linear-mixture MASSP instance defined by appropriate parameters ($n, \delta, \Delta, \theta$) for whom the expected cumulated regret matches the reported upper bound $\widetilde{O}(\sqrt{K})$. \\ Specifically, the instance satisfies: \\ $\mathbb{E}_{\theta,\mathfrak{A}}[R(K)] \geq \frac{d.\sqrt{\delta}\sqrt{K.V^*_1}}{2^{n+9}}$ \\
for $K > \frac{(d-1)^2.\delta}{2^{10}V^*_1.min^2\{\frac{3\delta-1}{n^2+n+1}, \frac{2\delta}{3},\frac{1-2\delta}{1+n+n^2}\}} $

\subsection{ \label{generalise_cohen} \textit{Generalisation of Lemma C2 of Cohen et al for our case}-12/13-3-25}
\tb{Lemma:} For any deterministic learner, if $T\geq 2KV_1^*$, then, $\mathbb{E}[N_-]\geq KV^*_1/4$ \\ 

\textcolor{blue}{there is a relation between $B^\star$ and $V^\star_1$ and is given in the first half of this writeup }

\tb{Proof:} If capped process finishes before T, $N_-=N$. Else number of visits to goal state is less than $K$. \\Thus, $N_- \geq T-K$.\\ Thus, $\mathbb{E}[N_-] \geq \mathbb{E}[min\{T-K,N\}] \geq \mathbb{E}[\sum_{i=1}^Kmin\{T/K-1, N_k\}]$.\\
Since $T\geq2KV^*_1,$ and $V^*_1\geq1$ the lemma will hold for any policy (mapping of actions) if, $N_k \geq V^*_1$ with probability $\geq 1/4$ for any policy. Consider any policy. \\ We can lower bound the probability $\mathbb{P}[N_k \geq V^*_1]$ by the events that we transit to an $r=1$ state and stay there for next $\lceil V^*_r\rceil -1$ steps. \\Thus, \\
$\mathbb{P}[N_k \geq V^*_1] \\ = \mathbb{P}(s_2 \neq g|s_1=s_{init}).\mathbb{P}(s_3 \neq g|s_2).\mathbb{P}(s_4 \neq g|s_3)....\mathbb{P}(s_{\lceil V^*_1\rceil} \neq g|s_{\lceil V^*_1\rceil-1}) \\ = (1-p^{a(s_1)}_{n,0}).(1-p^{a(s_2)}_{s_2,0})...(1-p^{a(s_{\lceil V^*_1\rceil-1})}_{s_{\lceil V^*_1\rceil-1},0}) $ \\
For any state s, $1-p^{a(s)}_{n,0}$ is minimum when $p^{a(s)}_{n,0}$ is maximum. Check from line 1087 that this happens at $a^*$ which matches all signs with $\theta$. Further, $1-p^*_{s,0}$ when $s \neq g$ is minimum when $p^*_{s,0}$ is maximum at any $s \in \mathcal{S}_{n,1}$. Thus, we can lower bound the above product as: \\
$\mathbb{P}[N_k \geq V^*_1] \geq (1-p^*_{n,0}).(1-p^*_{s_2,0})...(1-p^*_{s_{\lceil V^*_1 \rceil -1},0}) \geq (1-p^*_{1,0})^{\lceil V^*_1 \rceil -1} \geq (1-p^*_{1,0})^{ V^*_1 -1} = (1-p^*_{1,0})^{ 1/{p^*_{1,0}} -1} \geq 1/e \geq 1/4$ \\
For the last second inequality, we use for $x\geq 1$, $(1-1/x)^{x-1}\geq 1/e$ \\
 Thus, $\mathbb{E}[N_-]  \geq \mathbb{E}[\sum_{i=1}^Kmin\{T/K-1, N_k\}] \geq KV^*_1/4$ \\


 
 \subsubsection{\textit{Alternate proof for dealing with $\mathbb{P}[N_k \geq V^*_1] \ge \frac{1}{4}}$ 13-3-25}
 
\textcolor{blue}{the result below a general one}
 
 Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](s)$ as the probability that starting at state $s \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in R^+$. Further, $\mathbb{P}[N_k \geq x] = \mathbb{P}[N_k \geq x](s_{init})$. \\
 \tb{Claim} Consider any $s \in S_{n,r}$ where $r \in [n]$. Then, for any policy it holds for our instances that $\mathbb{P}^{\pi}[N_k \geq x](s) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](s')$ for all $x \in R$ where $s' \in \mathcal{S}_{n,r'}(s)$ for any $r' \in \{0\} \cup [r]$ with equality holding only at $\pi = \pi^*$  and $r'=r $ i.e., $s'=s$ respectively. Here $\pi^*$ is the policy of taking action $a^*$(the one matching all signs with $\theta$) at every state $s \in \mathcal{S}$. The equality in the middle says that for any $s \in \mathcal{S}_{n,r}$ under $\pi^*$, $\mathbb{P}^{\pi^*}[N_k \geq V^*_1](s)$ happens to stay a constant independent of $s$ and only depends on $r$.\\
 Proof will be similar to $V^*$ proof \\
 Will work on this later if above proof is not satisfactory.\\
 \tb{Proof} We will prove this by induction. \\
 \tb{Base Case:} For r=1: 
 Consider any $s \in \mathcal{S}_{n,1}$ \\
 For any $x \in R^+$, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x\rceil-1}$ \\
 One can check from the general formula for transition probabilities that the above is uniquely minimum when $\pi(s) = a^*$. Hence equality only holds at $\pi=\pi^*$.  \\
 Hence, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x\rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x\rceil -1}$ \\
 Recall that for the same action $a^*$ at any $s \in \mathcal{S}_{n,1}$, $P(g|s,a^*)$ remains the same. Hence, \\
 $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x \rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) $ \\
 The only two possibilities for $s'$ are $s$ itself and $g$. \\
 Clearly for $s$ the equality holds and for $g$, $\mathbb{P}^{\pi^*}[N_k \geq x](s'=g) = 0$ \\ Hence, \\
  $\mathbb{P}^{\pi}[N_k \geq x](s) = (1-P(g|s,\pi(s)))^{\lceil x \rceil-1} \geq (1-P(g|s,\pi^*(s)))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s')  $
  \\ Finally we showed that for any $x \in R^+$ for any policy $\pi$, for any $s \in \mathcal{S}_{n,1}$ and $s' \in \cup_{r' \in \{0,1\}} \mathcal{S}_{n,r'}(s)$,  \\
  $\mathbb{P}^{\pi}[N_k \geq x](s)  \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](s')  $ \\
  where in the first inequality, equality holds only when $\pi = \pi^*$, the middle equality means that the probability is same for all $s \in \mathcal{S}_{n,1}$ and in the last inequality, equality holds only when $s' = s$. \\
  \\
  \tb{Generalization:} Assume the above holds for m = 1, 2,...,r i.e., for all $m \in [r]$ it holds that for any $x \in R^+$ for any $s \in \mathcal{S}_{n,m}$, for any policy $\pi$, for our instances, it holds that, $\mathbb{P}^{\pi}[N_k \geq x](s) \geq \mathbb{P}^{\pi^*}[N_k \geq x](s)=\mathbb{P}^{\pi^*}[N_k \geq x](m)\geq \mathbb{P}^{\pi^*}[N_k \geq x](s')$ where $\pi^*$ is the policy taking action $a^*$(the one matching signs with all components of $\theta$) at all states and $s' \in \cup_{m' \in \{\{0\} \cup [m] \}}\mathcal{S}_{n,m'}(s)$. Further, in the first inequality, equality only holds when $\pi =\pi^*$ and the middle equality implies that the probability is same for all states $s \in \mathcal{S}_{n,m}$ and in the last inequality, the equality only holds when $s' =s$.  \\
  Assuming this we need to show that the same holds for any $s \in \mathcal{S}_{n,r+1}$ \\
  Again consider any $x \in R^+$. \\
  Consider any $s \in \mathcal{S}_{n,r+1}$. \\
  We have, \\
  $\mathbb{P}^{\pi}[N_k \geq x](s) = \sum_{r' \in \{0,[r+1]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)} P(s'|s,\pi(s)) . \mathbb{P}^{\pi}[N_k \geq x-1](s') \\= P(s|s,\pi(s)). \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)). \mathbb{P}^{\pi}[N_k \geq x-1](s')$ \\ 
   If $x \leq 1$, then trivially, for all $s \neq g$, for all policies, $\mathbb{P}[N_k \geq x] =1$. Otherwise, we have the following:
  \\
$\mathbb{P}^{\pi}[N_k \geq x](s) \\ =  P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s') \\ 
  \geq P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \sum_{s' \in \mathcal{S}_{n,r'}(s)}  P(s'|s,\pi(s))  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') +  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  \Bigg\} \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Bigg \} + \\ \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{s' \in \mathcal{S}_{n,r'}(s)}  \frac{2 \Delta}{n(d-1)} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \sum_{p \in [d-1]} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}  
  \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0, [r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{s' \in \mathcal{S}_{n,r'}(s)} \sum_{i \in [n]}      \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \mathbbm{1}\{t \in \mathcal{T}\} . \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{i \in [n]}        \{ \binom{r}{r'-1} -  \binom{r}{r'} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}     
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in \{0,[r]\}} \sum_{i \in [n]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} 
   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in [r]} \sum_{i \in [n]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}  \Big \} \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{ \{ \binom{r}{r-r'} -  \binom{r}{r+1-r'} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big \} \Bigg \}   \\
  = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \{ \binom{r}{r'-1} -  \binom{r}{r'} \} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} \Big \} + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{ \{ \binom{r}{r'} -  \binom{r}{r'-1} \}. \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}\Big \} \Bigg \} \\
 = P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in [n]} \sum_{r' \in [r]} \Bigg \{ \Big \{ \binom{r}{r'-1} -  \binom{r}{r'} \Big \} \Big \{ \mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq V^*_1](r+1-r') \Big \}      \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\}        \Bigg \}$ \\ \\
 Notice that for $r' < (r+1)/2$, the binomial difference $\binom{r}{r'-1} - \binom{r}{r'}<0$ as well as probability difference $\mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r') < 0$ hence the product is $>0$. Similar argument holds for $r'>(r+1)/2$. For $r' = (r+1)/2$ it will be 0. Overall we can observe that the only terms dependent on action have non-negative coefficients for the sign matching indicator. Hence this term will be minimum when $a = a^*$.  Thus, we have, \\
 $\mathbb{P}^{\pi}[N_k\geq x](s) \geq   P(s|s,\pi^*(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} $\\ Also, \\
 $\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $ \\

Subtracting the above two equations, 
\\
$\mathbb{P}^{\pi}[N_k\geq x](s) - \mathbb{P}^{\pi^*}[N_k\geq x](s) \\ \geq P(s|s,\pi(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) - P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) \\ \geq P(s|s,\pi^*(s)) \mathbb{P}^{\pi}[N_k \geq x-1](s) - P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) \\ 
= P(s|s,\pi^*(s)) (\mathbb{P}^{\pi}[N_k \geq x-1](s) - \mathbb{P}^{\pi^*}[N_k \geq x-1](s))$ \\
By recursion,  \\
$\mathbb{P}^{\pi}[N_k\geq x](s) - \mathbb{P}^{\pi^*}[N_k\geq x](s) \\ \geq P(s|s,\pi^*(s))^{\lfloor x \rfloor} (\mathbb{P}^{\pi}[N_k \geq x-\lfloor x \rfloor](s) - \mathbb{P}^{\pi^*}[N_k \geq x-\lfloor x \rfloor](s)) = P(s|s,\pi^*(s))^{\lfloor x \rfloor} (1- 1) = 0$  \\
Thus, $\mathbb{P}^{\pi}[N_k\geq x](s) \geq \mathbb{P}^{\pi^*}[N_k\geq x](s)$ \\
Also note that for equality, it must hold for each above inequality. Effectively this will only happen at $\pi = \pi^*$ \\ 
Recall, for any $s \in \mathcal{S}_{n,r}$, \\
$\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $
 \\
From the probability expression one can verify that the term $P(s|s,\pi^*(s))$ only depends on $r$. The only term that may differ due to $s$ is $\mathbb{P}^{\pi^*}[N_k \geq x-1](s)$. \\We claim that this is same too. This can be dealt with by induction on x itself. \\
For base case, $m = x-\lfloor x \rfloor$, for any $s \in \mathcal{S}_{n,r}$, $\mathbb{P}^{\pi^*}[N_k \geq m](s)=1$ \\ Hence showed for base case. \\ Assuming true for $m = x - \lfloor x \rfloor,  x - \lfloor x \rfloor+1,  x - \lfloor x \rfloor+2, \dots,  x - \lfloor x \rfloor+p $, we need to show that it holds for $m =  x - \lfloor x \rfloor + p+1$ \\ We can write for any $s \in \mathcal{S}_{n,r}$ that: \\
$\mathbb{P}^{\pi^*}[N_k\geq m ](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq m-1](s) + \\ \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq m-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n.2^{r}} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 $ \\ Here the RHS doesn't depend on which $s \in \mathcal{S}_{n,r}$ is being chosen. Thus shown for m. \\
 Thus back in expression for $\mathbb{P}^{\pi^*}[N_k \geq x](s)$, $\mathbb{P}^{\pi^*}[N_k \geq x-1](s)$ is not dependent on $s \in \mathcal{S}_{n,r}$. Hence $\mathbb{P}^{\pi^*}[N_k \geq x](s)$ is same for all $s \in \mathcal{S}_{n,r}$.  \\
 Finally we need to show that, $\mathbb{P}^{\pi^*}[N_k \geq x](s) \geq \mathbb{P}^{\pi^*}[N_k \geq x](s') \forall s' \in \cup_{r' \in \{0,[r]\}}\mathcal{S}_{n,r'}$ with equality only at $s' = s$. \\
 Recall again, for any $s \in \mathcal{S}_{n,r+1}$, \\
 $\mathbb{P}^{\pi^*}[N_k\geq x](s) =   P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in [r]} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} (\binom{r}{r'}  .  p^*_{r,r'} - \delta_{r'})  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\binom{r}{r'}  .  p^*_{r,r'}+ \delta_{r'}  )\mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r')) + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') )  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \sum_{r' \in \{ 1,2, \dots , r \}} (\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') ) \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r'))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') )  \\ >  P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}(\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1))   + \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} (\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](\lfloor \frac{r+1}{2} \rfloor + 1)) \\ =  P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  ( \sum_{r' \in \{ 1,2, \dots , \lfloor \frac{r+1}{2} \rfloor \}}\delta_{r'} - \sum_{r' \in \{\lfloor \frac{r+1}{2} \rfloor +1, \lfloor \frac{r+1}{2} \rfloor +2,\dots, r\}} \delta_{r'}) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1)  \\ = P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  P(s|s,\pi^*(s)) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1) \\ > P(s|s,\pi^*(s)) \mathbb{P}^{\pi^*}[N_k \geq x-1](s) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  P(s|s,\pi^*(s)) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( r) 
 $ \\
 Thus, we have, \\
 $\mathbb{P}^{\pi^*}[N_k \geq x](s) - \mathbb{P}^{\pi^*}[N_k \geq x](r) \geq P(s|s,\pi^*(s)).(\mathbb{P}^{\pi^*}[N_k \geq x-1](s) - \mathbb{P}^{\pi^*}[N_k \geq x-1](r))$ \\ By recursion and same arguments as before, \\
 $\mathbb{P}^{\pi^*}[N_k \geq x](s) = \mathbb{P}^{\pi^*}[N_k \geq x](r+1) >  \mathbb{P}^{\pi^*}[N_k \geq x](r)$
\\
 
 Hence the overall main induction argument for r holds. \\ \\
 Now, given this general theorem, where $s_1 \in \mathcal{S}_{n,1}$, we have, \\$\mathbb{P}^{\pi}[N_k \geq V^*_1](s) \geq \mathbb{P}^{\pi^*}[N_k \geq V^*_1](s_1) = (1-p^*(g|s,a^*))^{\lceil V^*_1 \rceil -1} \geq (1-p^*(g|s,a^*))^{ V^*_1  -1}  \geq 1/e \geq 1/4$

\subsubsection{Ignore this and check next section: Simplification of KL Divergence term 14-3-25} 
By chain rule of KL-Divergence, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)]$
\\
where, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $

\\
Let's simplify $\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)})$


\pt{Before doing this upper bound, why can't I break it into two terms -- first one where $s_t = (g,g,...,g)$, and the other one when $s_t \neq (g,..., g)$. I think the terms will be simplified a lot if you do this. 
 Also, you can go one step ahead and look at all the impossible transitions -- the log term will vanish for all of them. So, you are left with the cases when the transitions are valid. Now, you can utilize the same notations, $r$ to $r'$ type of transitions. For all such transitions, the ratio inside the log can be written in terms of the features and corresponding $\theta$, and $\theta^j$. note that we might need to carefully use the conditions on $\delta$ and $\Delta$ you obtained earlier. } \textcolor{red}{i won't be able to use $s_{t+1} \neq g$ inside ln(.), I need to check when the ratio inside ln maximises here:$s_{max}$ to provide upper bound. $s_{min}$ is not strictly required and any global state can be used instead as for eg. you suggested $g,g,g...$. Also yes, i'm thinking of possible transitions only although once the $s_t$ is fixed from outer  summation. But notice that when $s_t=(s_{init},s_{init},...s_{init})$, we will need to optimize over all $s \in S$.}

 \pt{i am not talking about $s_{t+1}$, I am saying you can look at the summation for two cases separately, $s_t = g$, and $s_t \neq g$. That will lead to some simplifications. } \\ \textcolor{red}{i wouldn't even think about $s_t=g$: cz then $s_{t+1}$ has to be $g$ with probability 1 : independent of $\theta$ or $\theta_j$ hence ratio inside log is 1 and this term will be 0, for other $s_{t+1}$ probability is 0 hence all those terms are 0. problem is to deal with the general case}

 \pt{exactly, that's where we can now only use the features and then explicitly write them in terms of the other parameters. Also, why you are trying to maximize the term inside the log? We can just write the expressions for $\theta$ and $\theta^j$ and then finally use some other bounds at the later stage.} 

 \textcolor{red}{explicitly substituting the probabilities using features leads to a huge sum, each of those $2^{r}$ terms will have ratio inside ln that looks like line 1765. It would be desirable to simplify those terms without bounding earlier. The reason i want to maximise is to bound before simplifying. I'm just trying an approach as of now.  }


 \pt{Some results from the Jaksch et al 2010 paper can be used at the later stage.}

 \begin{figure}[h!]
     \centering
     \includegraphics[width=0.5\linewidth]{Jaksch.png}
     \caption{The result from Jaksch et al 2010 paper. This holds for some conditions on $\delta', \epsilon'$. Need to check if these conditions hold in our work. this type of result can be used for each term inside the summation, possibly for each $r$ to $r'$ transition. }
 \end{figure}
 \textcolor{red}{i have seen this, it can't be used for our case. in fact i want to get the sum over $2^r$ next states in this form thats why looking for maximum of that ratio. thats what motivated line 1756. also if you look carefully, the above result is not exactly from Jaksch, it is from Min. Jaksch result is bit different. Also Min made has made a typo in this above equation.}
 
 


Notice this can be upper bounded as follows: \\ 
$\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ \leq \mathcal{P}_{\theta}(s_{t+1}= s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s_{min}|\textbf{s}_{t-1}, s_t = s, a_t = a)}) + (1-\mathcal{P}_{\theta}(s_{t+1  }= s_{min}|\textbf{s}_{t-1},s_t = s, a_t = a)).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s_{max}|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s_{max}|\textbf{s}_{t-1}, s_t = s, a_t = a)})$ \\
where, \\ $s_{min} = arg min_{s' \in \mathcal{S}} \ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $ and, \\
$s_{max} = arg max_{s' \in \mathcal{S}} \ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ $ \\
Since, $s$ and $a$ are fixed in the outer summation, both $s_{min}$ and $s_{max}$ may depend on both $s$ and $a$. For any general transition, we investigate the behavior of the ratio above. Given $s_t$, we partition the set of agents at $s_{init}$, into $X$ and $Y$ based on action $a$. Suppose $a$ is such that agents in $X:$ $x_1,x_2,\dots,x_m$ have their $j-th$ components not matching signs with respective components of $\theta$. Hence, agents $x_1,x_2,\dots,x_m$ have their $j-th$ components matching signs with respective components of $\theta_j$. Similarly let agents in $Y: y_1,y_2,\dots, y_{r-m}$ be such that their $j-th$ components match with respective components in $\theta$. This means agents $y_1, y_2, \dots, y_{r-m}$ are such that their $j-th $ components do not match with $\theta_j$. Along with previous notations, the ratio can be analyzed as : \\ 
$
\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}  \\= \frac{\frac{(r'-0.5r)(1-2\delta) + 0.5n }{n.2^{r-1}}     +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)}\sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta_{i,p})\} -  \sum_{t \in \mathcal{T}} \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta_{t,p})\} \Big \}}{  \frac{(r'-0.5r)(1-2\delta) + 0.5n }{n.2^{r-1}}          +    \frac{\Delta}{n}  (r-2r') +  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{sgn(a_{i,p}) \neq sgn(\theta^j_{i,p})\} -  \sum_{t \in \mathcal{T}}  \mathbbm{1}\{sgn(a_{t,p}) \neq sgn(\theta^j_{t,p})\} \Big \}} \\ 
$\\ \\
To find the optimal values of this ratio, we first check what happens at fixed $r, r'$ and then optimize for $r'$. Notice that the ratio is maximum when maximum number of agents who stayed had signs matched with $\theta_j$ and maximum number of agents who transited had signs matched with $\theta$

\textcolor{blue}{we are looking at $\mathbb{E}_P[X] - \mathbb{E}_Q[X]$ for two probability measures $P$ and $Q$. we can use change of variable and write $\mathbb{E}_Q[X] = \mathbb{E}_P[X \frac{dQ}{dP}]$? }

\textcolor{blue}{policy is $\pi_\theta$ and does $\theta$ refer to something else? }

\textcolor{blue}{based on a call on Sat 10pm, 22/3}
\textcolor{red}{hi, i thought we weren't meeting yesterday} \\
\pt{\url{http://joschu.net/blog/kl-approx.html} -- we can use some ideas from here.} \textcolor{blue}{this unbaised estimator of KL with low variance (by John Shulmann of PPO fame) would be very good to use in computations} \textcolor{red}{Im very doubtful, this blog is about constructing suitable estimate of kl-div from samples. but we need to analytically express kl-div or its suitable upper bound}

\pt{The above blog is suitable for the computations, isn't it?} \textcolor{red}{if by computation u mean implementing learning algo for massp, then no. I dont know if you are referring to any other kind of computation}

\pt{can we make use of the indicator present in line 1775 and bound the entire term.}

\pt{Other possibility is to take out the smallest of $\sum_{i\in I \cap T'}$ and $\sum_{t\in T}$?} \\ \textcolor{red}{can u try these and update above?}

\pt{Just for clarity, what I remember is:}

\pt{$\mathcal{I}$: Set of all agent are $s_{init}$.}

\pt{$\mathcal{J}$: Set of all agents at $g$}

\pt{$\mathcal{T}$: Set of all agents from $\mathcal{I}$ who move from $s$ to $g$.}

\pt{$\mathcal{T}'$: set of all agents from $\mathcal{I}$ who stayed at $s$}


\pt{If the above is correct, then $\mathcal{I}\cap \mathcal{T}'$ and $T$ are disjoint?} \textcolor{red}{yes, also above is correct}


\pt{Alternatively, upper bound the numerator, and lower bound the denominator and vice-versa and then take the min.} 
\textcolor{red}{the bounding of individual ratio doesn't help later, then there would be $2^r$ type factor}  \\ \textcolor{blue}{we can use min of two bounds and see how it effects the regret bound}

\pt{Also, note that only the orders as of now with respect to $n$ are important, not the front constants. As long as we are able to get some order of the regret bound wrt $n$, we are good.}


\pt{Any updates after Saturday?} \textcolor{red}{no break thru yet}

\textcolor{blue}{$\delta$ and $\delta_j$ are vectors with entries +1s and -1s. When entries are  +1s and 0s the Hamming distance between them is the number of entries that differ. we can \emph{temporarily} take -1s as 0s. this may  help to bound the KL$(\delta|| \delta_j)$.}
\\
\textcolor{red}{I have an update : today I performed computation of the sum in line 1758 for many instances of n,a,$s_t$ and realized that it is maximum at $s_t = (s_{init},s_{init},...,s_{init})$ : contradictory to what i was hoping (max for states of type r=1). Turns out this can be explained by property of KL-divergence. So we can upper bound this summation for any $s_t$ by the summation at this initial state. As of now i don't know if the upper bound i wish to obtain (same/similar as given in Min) still holds. Im trying to see that via computations. Will update further soon.}

\pt{Wasn't this observation intuitive and follows from the fact that KL is positive, and  when I told you that for the case when $s_t = (g,g,g...g)$, then one term was getting zero?} \textcolor{red}{Pls explain us how this is intuitive from terms becoming 0 when st is all at g, in the next meeting. Also do respond to my earlier responses on your above remarks, its further confusing when you suggest something and not elaborate anything. Also next meeting pls come prepared to explain the steps in upper bound proof that i had asked in January. The note you send is unclear to me.}

\pt{What are the next steps in theory?}

Meeting link: \url{https://ucf.zoom.us/j/99575809604?pwd=dar1hN9fReFbU4yae8Bp4YGDKfaBeP.1}
\\ \\
Property of KL-Divergence: https://math.stackexchange.com/questions/4986295/partition-form-of-the-kl-divergence


\subsection{\textit{Simplifying KL-Divergence} \label{simplify_kld}}

By chain rule of KL-Divergence, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)]$
\\
where, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) $ \\
Notice that in the above, for any fixed $(s,a)$, the inner summation is itself a KL-divergence. \\ 
Let's simplify it first: \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\  = \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) $ \\
Hence we'll upper bound using the inner KL for any $\tb{s} \in \mathcal{S}$. \\
As $ KL(B|A) > 0$, $KL(A|B) \leq KL(A|B) + KL(B|A)$ for any distributions $A, B$. Thus: \\ \\
$\sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\ \leq   \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) + \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}) \\= \sum_{s' \in \mathcal{S}} (\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) ).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\
= \sum_{s' \in \mathcal{S}} (\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) ).\ln(1 + \frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) \\
\leq \sum_{s' \in \mathcal{S}} \frac{(\mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a) - \mathcal{P}_{\theta_j}(s_{t+1  }=s'|s_t = s, a_t = a) )^2}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)} \\
\leq 2^n . \frac{max_{s'}( \langle \phi(s'|s,a), \theta - \theta_j \rangle)^2}{ min_{s}\mathcal{P}_{\theta_j}(s_{t+1}=g|s_t = s, a_t = a)} \leq 2^n . \frac{(\frac{2 \Delta}{d-1})^2}{\frac{\delta}{2^{n-1}} - \Delta}
$ \\
Since $2/5<\delta<1/2$ and $\Delta<2^{-n}\frac{1-2\delta}{1+n+n^2}$, $\Delta < 2^{-n}. \frac{2\delta}{3} $. \\ Thus, \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)})  < 2^n. \frac{(\frac{4\Delta^2}{(d-1)^2})}{\frac{2\delta}{3.2^{n-1}}} = 3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $ \\ 
Hence, going back above: \\
$ \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\  = \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|s_t = s, a_t = a)}) < 3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $ \\
Thus, \\
$\sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s_{t+1} \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}} \mathcal{P}(\textbf{s}_t). \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_t).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_t)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_t)}) \\ = \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) \sum_{s' \in \mathcal{S}} \mathcal{P}_{\theta}(s_{t+1  }=s'|\textbf{s}_{t-1},s_t = s, a_t = a).\ln(\frac{\mathcal{P}_{\theta}(s_{t+1}=s'|\textbf{s}_{t-1},s_t = s, a_t = a)}{\mathcal{P}_{\theta_j}(s_{t+1}=s'|\textbf{s}_{t-1}, s_t = s, a_t = a)}) \\ < \sum_{\textbf{s}_{t-1} \in \mathcal{S}^{\times {t-1}}} \mathcal{P}(\textbf{s}_{t-1}). \sum_{s \in \mathcal{S}, a \in \mathcal{A}} \mathcal{P}(s_t = s, a_t = a|\textbf{s}_{t-1}) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} \\ =  \mathcal{P}({s}_{t} \neq g) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} $  \\ \\ Therefore from earlier, \\
$KL(\mathcal{P}_{\theta} || \mathcal{P}_{\theta_j}) = \sum_{t=1}^{T-1} \sum_{\textbf{s}_t \in \mathcal{S}^{\times t}}\mathcal{P}(\textbf{s}_t).KL[\mathcal{P}_{\theta}(s_{t+1}|\textbf{s}_t)||\mathcal{P}_{\theta_j}(s_{t+1}||\textbf{s}_t)] \\ <  \sum_{t=1}^{T-1} \mathcal{P}({s}_{t} \neq g) .  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} \leq  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} .  \sum_{t=1}^{T} \mathcal{P}({s}_{t} \neq g)  =  3. 2^{2n} \frac{\Delta^2}{\delta (d-1)^2} . \mathbb{E}_{\theta}[N^-]  $
\\
We use the above result in lower bound proof.

\pt{This seems good. Can you also write why the inequality in line 1847 holds} \\ \textcolor{red}{you meant the 1st line in the equations right? ive mentioned now in line 1848} \pt{yes, got it.}

\pt{Does that mean we now have a lower bound proof? I can see that the KL bound is exponential in $n$, will it lead to exponential bounds? or will it create some problems in the lower bound?}
\\
\textcolor{red}{yes we have a lower bound now. yes it looks exponential but from sufficient conditions, $\Delta$ is also of exponential order hence overall the bound is not exponentially large. from computations i've verified that this is quite tight(off by 1 order of magnitude for small n's and this difference decreases as n increases. hence we have a reasonably tight bound). ive updated and completed the lower bound proof(page 38). finally we get lower bound that scales as $1/2^n$. but we also get $\sqrt{K}$ }


\pt{Great!! So, we have the lower bound with $\sqrt{K}$, thus as tightest lower bound in terms of $K$, and can you explain what is the regret lower bound implication as $n$ increases? -- somehow not very clear to me. Particulary, i dond't understand this statement of yours  ``this difference decreases as n
increases. hence we have a reasonably tight bound''. } \textcolor{red}{yeah no problem, i will clear this in next meeting}

\pt{I think, now is the time to clean it and write the results in a nice format with all the details and explaination of each step. Can you explain the entire proof in our next meeting, and we can start writing it. }
\textcolor{red}{yes i wanted to explain everything too}
\pt{Let us connect on Friday evening 7:00 PM or Sat morning 9:00 AM India time, we can discuss this for a long time with all the details.} \textcolor{red}{sure, saturday 9am would be best}

Meeting link: \url{https://ucf.zoom.us/j/99575809604?pwd=dar1hN9fReFbU4yae8Bp4YGDKfaBeP.1}

\subsection{\textit{Upper Bound proof and Implementation}}
\begin{itemize}
    \item Simplification of T
    \item Min-max : convergence to best policy
    \item Appendix C3 line 3: $a_{m,h}$ is not the same as argmin_a $Q^i_{j_i}(s_{m,h},a)$ for this algo.
    \item Algorithm: V update-what about $a^{-i}$
\end{itemize}

\subsection{Related Work}
\label{subsec:related_work}

\input{Sections/extras}


\begin{corollary}\label{corollary:ps_s}
For any non-goal state $\tb{\ti{s}} \in \mathcal{S}_r$ of type $r$, the self-transition probability under action $\tb{\ti{a}}$ is
\begin{align}
    \mathbb{P}(\tb{\ti{s}} | \tb{\ti{s}}, \tb{\ti{a}}) = \frac{r(1-\delta)}{n \cdot 2^{r-1}} + \frac{n - r}{n \cdot 2^r} -  \frac{r \cdot \Delta}{n} + \frac{2\Delta}{n(d - 1)} \sum_{i \in \mathcal{I}} \sum_{p = 1}^{d - 1} \mathbbm{1}\{\sgn({a}_{i,p}) \neq \sgn(\theta_{i,p})\}.
\end{align}
This is minimized when $\tb{\ti{a}} = \tb{\ti{a}}_{\theta}$ and the resulting probability only depends on $r$.
\end{corollary}
% 





\begin{lemma} \label{lemma:episodelength} 
Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$ as the probability that starting at state $\tb{\ti{s}} \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in R^+$. Furthermore, $\mathbb{P}^{\pi}[N_k \geq x] = \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$. 
Consider any $\tb{\ti{s}} \in \mathcal{S}(r)$ where $r \in [n]$. Then, for any policy $\pi$, it holds for any instance as defined in (ref) that for any $x \in R^+$: \\ $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}')$ \\ where $\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})$ with equality holding (for all $x \in R^+$) only at $\pi = \pi^*$  and $r'=r $ (i.e., $\tb{\ti{s}}'=\tb{\ti{s}}$) respectively. \\  Here $\pi^*$ is the policy of taking action $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$ (optimal policy from Theorem \ref{thm:all_in_one}). The equality in the middle indicates that under $\pi^*$ (for any fixed $x \in R^+$), $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ stays constant depending only on $r$ for all $\tb{\ti{s}} \in \mathcal{S}(r)$.
\end{lemma}

\begin{corollary}
\label{corollary:pn_x}
An immediate corollary of the above lemma is that $\mathbb{P}^{\pi^*}[N_k \geq x](r)$ is ordered for any $x \in R^+$ i.e., $\mathbb{P}^{\pi^*}[N_k \geq x](n) \geq \mathbb{P}^{\pi^*}[N_k \geq x](n-1) \geq \cdots \geq \mathbb{P}^{\pi^*}[N_k \geq x](2) \geq \mathbb{P}^{\pi^*}[N_k \geq x](1) \geq \mathbb{P}^{\pi^*}[N_k \geq x](0) =0 $

\end{corollary}



\subsection{Proof of Lemma \ref{lemma:episodelength}}
Used in proof of Lemma 5.

\textbf{Recall the Lemma \ref{lemma:episodelength}. } 
% 
\textit{Let's define the notation $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$ as the probability that starting at state $\tb{\ti{s}} \in \mathcal{S}$ and following the policy $\pi$, the number of time steps to reach global goal $(N_k)$ is more than or equal to $x$ for any $x \in R^+$. Furthermore, $\mathbb{P}^{\pi}[N_k \geq x] = \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})$.} 

\textit{Consider any $\tb{\ti{s}} \in \mathcal{S}(r)$ where $r \in [n]$. Then, for any policy $\pi$, it holds for any instance as defined in (ref) that for any $x \in R^+$: \\ $\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r)  \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}')$ \\ where $\tb{\ti{s}}' \in \mathcal{S}(\tb{\ti{s}})$ with equality holding (for all $x \in R^+$) only at $\pi = \pi^*$  and $r'=r $ (i.e., $\tb{\ti{s}}'=\tb{\ti{s}}$) respectively. \\  Here $\pi^*$ is the policy of taking action $\tb{\ti{a}}^* = \tb{\ti{a}}_{\theta}$ at every state $\tb{\ti{s}} \in \mathcal{S}$ (optimal policy from Theorem \ref{thm:all_in_one}). The equality in the middle indicates that under $\pi^*$ (for any fixed $x \in R^+$), $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ stays constant depending only on $r$ for all $\tb{\ti{s}} \in \mathcal{S}(r)$.}


\begin{proof}
 
We will prove this by induction.
\\
 \tb{Base Case:} \\ For r=1: 
 Consider any $\tb{\ti{s}} \in \mathcal{S}(1)$ \\
 For any $x \in R^+$, 
 \begin{align}
     \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) = (1-\mathbb{P}(\tb{g}|\tb{\ti{s}},\pi(\tb{\ti{s}})))^{\lceil x\rceil-1}
 \end{align}
 One can check from Lemma \ref{lemma:general_tp} that the above is uniquely minimum when $\pi(\tb{\ti{s}}) = \tb{\ti{a}}^*$. Hence equality only holds at $\pi=\pi^*$.  \\
 Hence,
 \begin{align}\label{eqn:prob_n}
     \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) = (1-\mathbb{P}(\tb{g}|\tb{\ti{s}},\pi(\tb{\ti{s}})))^{\lceil x\rceil-1} \geq (1-\mathbb{P}(\tb{g}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})))^{\lceil x\rceil -1}
 \end{align}
 Recall that for the same action $\tb{\ti{a}}^*$ at any $\tb{\ti{s}} \in \mathcal{S}(1)$, $\mathbb{P}(\tb{g}|\tb{\ti{s}},\tb{\ti{a}}^*)$ remains the same (Corollary \ref{corollary:p_star}).\\
 Hence, we further have, 
 \begin{align}
     \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) = (1-\mathbb{P}(\tb{g}|\tb{\ti{s}},\pi(\tb{\ti{s}})))^{\lceil x \rceil-1} \geq (1-\mathbb{P}(\tb{g}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) 
 \end{align}
 The only two possibilities for next state $\tb{\ti{s}}'$ are $\tb{\ti{s}}$ itself and $\tb{g}$. \\
 Clearly for $\tb{\ti{s}}$ the equality holds and for $\tb{g}$, $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}'=\tb{\ti{g}}) = 0$ \\ Hence, 
 \begin{align}
     \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) = (1-\mathbb{P}(\tb{\ti{g}}|\tb{\ti{s}},\pi(\tb{\ti{s}})))^{\lceil x \rceil-1} \geq (1-\mathbb{P}(\tb{\ti{g}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})))^{\lceil x \rceil -1} = \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}') 
 \end{align}
  \\ To recap, we have shown above that for any $x \in R^+$ for any policy $\pi$, for any $\tb{\ti{s}} \in \mathcal{S}(1)$ and $\tb{\ti{s}}' \in \cup_{r' \in \{0,1\}} \mathcal{S}(r')(\tb{\ti{s}})$,  \\
  \begin{align}
      \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})  \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r=1) \geq  \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}') 
  \end{align}
  where in the first inequality, equality holds for all $x \in R^+$ only when $\pi = \pi^*$, the middle equality means that the probability is same for all $\tb{\ti{s}} \in \mathcal{S}(1)$ and in the last inequality, equality holds only when $\tb{\ti{s}}' = \tb{\ti{s}}$. \\
  \\
  \tb{Generalization:} \\ Assume the above holds for m = 1, 2,\dots,r i.e., for all $m \in [r]$ it holds that for any $x \in R^+$ for any $\tb{\ti{s}} \in \mathcal{S}(m)$, for any policy $\pi$, for our instances, 
  \begin{align}
   \mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})=\mathbb{P}^{\pi^*}[N_k \geq x](m)\geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}')   
  \end{align}
   where $\pi^*$ is the policy taking action $\tb{\ti{a}}^*=\tb{\ti{a}}_{\theta}$ at all states and $\tb{\ti{s}}' \in \cup_{m' \in \{\{0\} \cup [m] \}}\mathcal{S}(m')(\tb{\ti{s}}) = \mathcal{S}(\tb{\ti{s}})$. Further, in the first inequality, equality only holds for all $x \in R^+$ when $\pi =\pi^*$ and the middle equality implies that the probability is same for all states of same \emph{type} $\tb{\ti{s}} \in \mathcal{S}(m)$ and in the last inequality, the equality only holds when $\tb{\ti{s}}' = \tb{\ti{s}}$.  \\
  Assuming this, we need to show that the same holds for any $\tb{\ti{s}} \in \mathcal{S}(r+1)$ \\ 
  Now, consider any $x \in R^+$. \\
  Consider any $\tb{\ti{s}} \in \mathcal{S}(r+1)$. \\
  We have, 
  \begin{align}
      &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \\
      &= \sum_{r' \in \{0,[r+1]\}} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\pi(\tb{\ti{s}})) . \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}') \\
      &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})). \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' \in \{0,[r]\}} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})}  \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\pi(\tb{\ti{s}})). \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}')
  \end{align}
   If $x \leq 1$, then trivially, for all $\tb{\ti{s}} \neq \tb{g}$, for all policies, $\mathbb{P}[N_k \geq x] = 1$. However,in general, we have the following:
   \begin{align}
      &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})  \\
      &=  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' \in \{0,[r]\}} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})}  \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}') \\
      &\geq \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' \in \{0,[r]\}} \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})}  \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](r') 
      \end{align}
      The above follows from induction assumption. \\
      Thus,
      \begin{align}
      &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})  \\   
      &\geq  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})}  \mathbb{P}(\tb{\ti{s}}'|\tb{\ti{s}},\pi(\tb{\ti{s}})) \\
      &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) +  \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \times \\ 
      &\quad  \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}} +    \frac{\Delta}{n}  (r+1-2r') +  \\
    &\quad \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}   -\sum_{t \in \mathcal{T}}  \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}  \Bigg\} \\
    &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
    &\quad \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .  \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \Bigg\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Bigg \} + \\ 
    &\quad \sum_{r' \in \{0,[r]\}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \times \\
    &\quad   \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})}  \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \Big \{  \sum_{i \in \mathcal{I} \cap \mathcal{T'}}\mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}   -\sum_{t \in \mathcal{T}} \mathbbm{1}\{\sgn(a_{t,p}) \neq \sgn(\theta_{t,p})\} \Big \}  
  \end{align}
  In the first term, we observe that the term inside the inner summation over $s' \in \mathcal{S}(r')(\tb{\ti{s}}')$, the terms inside that summation do not depend on which $\tb{\ti{s}}'$ is being considered for a fixed $r'$ and $\tb{\ti{s}}$ and are the same. Hence, the whole summation simplifies to the product of this term and the cardinality of that set which is $\binom{r+1}{r'}$. Also, we realize that for the second term for any agent the coefficient of the indicator is $+1$ if he stays at node $s$ itself while it is $-1$ when he transits to node $g$. Hence we can simplify the above as following including some rearrangement of summation and using the fact that the probability terms vanish for state of \emph{type} 0, namely $\tb{\ti{g}}$ :
  \begin{align}
   &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})  \\   
  &\geq \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
  &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ 
  &\quad \frac{2 \Delta}{n(d-1)} \times \\
  &\sum_{p \in [d-1]} \sum_{r' \in  [r]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{\tb{\ti{s}}' \in \mathcal{S}(r')(\tb{\ti{s}})} \sum_{i \in \mathcal{I}}      \Big \{  \mathbbm{1}\{i \in \mathcal{I} \cap \mathcal{T'}\}.   - \mathbbm{1}\{i \in \mathcal{T}\}\Big \} . \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} 
   \\
   &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
   &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ 
   &\quad \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in [r]} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \sum_{i \in \mathcal{I}}      \Big  \{ \binom{r}{r'-1} -  \binom{r}{r'} \Big \}. \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}
   \end{align}
   The last step follows by taking the summation over $s'$ inside and observing that from any fixed $\tb{\ti{s}}$ of \emph{type} $r$, the number of states of \emph{type} $r'$ reachable from $\tb{\ti{s}}$ in which any agent at node $s$ stays at node $s$ is $\binom{r}{r'-1}$ and those in which he transits to node $g$ is $\binom{r}{r'}$. Thus, we have:
   \begin{align}
   &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}})  \\  
   &\geq \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
   &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ 
   &\quad \frac{2 \Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{r' \in [r]} \sum_{i \in \mathcal{I}} \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{  \binom{r}{r'-1} -  \binom{r}{r'}  \Big \} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}
   \\
   &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
   &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ 
   &\quad \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]} \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{ \binom{r}{r'-1} -  \binom{r}{r'}  \Big \}\mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}  \\
   &\quad + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{  \binom{r}{r-r'} -  \binom{r}{r+1-r'} \Big \}. \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Bigg \}   
   \end{align}
    In the last step, we use $\sum_{a\in[m]}f(a) = \sum_{a\in[m]} f(m+1-a)$ for any $f(\cdot)$ \\
    We simplify above as:
   \begin{align}
   &\mathbb{P}^{\pi}[N_k \geq x](\tb{\ti{s}}) \\    
   &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
   &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\ 
   &\quad \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]}  \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \Bigg \{  \mathbb{P}^{\pi^*}[N_k \geq x-1](r')         \Big \{  \binom{r}{r'-1} -  \binom{r}{r'} \Big \} \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}  \\
   &\quad + \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r')         \Big \{  \binom{r}{r'} -  \binom{r}{r'-1}\Big \}. \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\} \Bigg \} \\
   &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\
   &\quad \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} + \\
   &\quad \frac{\Delta}{n(d-1)} \sum_{p \in [d-1]}  \sum_{i \in \mathcal{I}} \sum_{r' \in [r]} \Bigg \{ \Big \{ \binom{r}{r'-1} -  \binom{r}{r'} \Big \} \Big \{ \mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq V^*_1](r+1-r') \Big \}   . \\
   &\quad \mathbbm{1}\{\sgn(a_{i,p}) \neq \sgn(\theta_{i,p})\}        \Bigg \}
   \end{align}
 Notice that for $r' \leq  (r+1)/2$, the binomial difference $\binom{r}{r'-1} - \binom{r}{r'} \leq 0$ as well as probability difference $\mathbb{P}^{\pi^*}[N_k \geq x-1](r') - \mathbb{P}^{\pi^*}[N_k \geq x-1](r+1-r') \leq  0$ due to induction assumption, hence the product is $ \geq 0$. Similar argument holds for $r'\geq (r+1)/2$.  \\
 Overall we can observe that the only terms dependent on action have non-negative coefficients for the sign matching indicator. Hence the overall summation will be minimum when this term will be minimum which happens at $a = a^*=a_{\theta}$.  \\
 Thus, we have, 
 \begin{align}
     &\mathbb{P}^{\pi}[N_k\geq x](\tb{\ti{s}}) \\
     &\geq   \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
     &\sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} 
 \end{align}
 Also, 
 \begin{align}
     & \mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}}) \\
     & =   \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) \\
     &\quad+  \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} + \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
 \end{align}
Subtracting the above two equations, 
\begin{align}
    &\mathbb{P}^{\pi}[N_k\geq x](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}}) \\ 
    &\geq \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) - \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) \\ 
    &\geq \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) - \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) \\ 
    &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) (\mathbb{P}^{\pi}[N_k \geq x-1](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}))
\end{align}
The last second step follows from Corollary \ref{corollary:ps_s}.\\
By recursion we have,  
\begin{align}\label{eqn:pnxnx}
    &\mathbb{P}^{\pi}[N_k\geq x](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}}) \\ 
    &\geq \mathbb{P}\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}}))^{\lfloor x \rfloor} \{\mathbb{P}^{\pi}[N_k \geq x-\lfloor x \rfloor](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k \geq x-\lfloor x \rfloor](\tb{\ti{s}})\} \\
    &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}}))^{\lfloor x \rfloor} (1- 1) \\
    &= 0
\end{align}
In the last second step, we use the fact that $x-[x]$ is a fractional value or equal to $0$ for any $x \in R^+$ hence for any $\tb{\ti{s}} \neq \tb{\ti{g}},$ certainly (w.p. 1), at least one time step is required to reach reach $\tb{\ti{g}}$. \\
Thus, 
\begin{align}
   \mathbb{P}^{\pi}[N_k\geq x](s) \geq \mathbb{P}^{\pi^*}[N_k\geq x](s) 
\end{align}
Also note that for equality for all $x \in R^+$, the equality must hold at every one of the above inequalities. Effectively this will only happen if $\pi = \pi^*$ \\ 


Recall, for any $\tb{\ti{s}} \in \mathcal{S}(r)$, 
\begin{align}\label{eqn:prob_nxs}
    &\mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}}) \\
    &=   \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \\ 
    &\sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq x-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \}
\end{align}
From the probability expression one can verify that the term $\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}}))$ only depends on $r$. The second term is independent of $\tb{\ti{s}} \in \mathcal{S}(\tb{\ti{r}})$ due to induction hypothesis and $r+1$ is same. \\Thus, the only term in the above expression that may differ due to $\tb{\ti{s}}$ is $\mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}})$. \\We claim that this is same too for all $\tb{\ti{s}} \in \mathcal{S}(r)$.\\ 
This can be dealt with by induction on $x$ itself.  \\
For base case, $m = x-\lfloor x \rfloor$, for any $\tb{\ti{s}} \in \mathcal{S}(r)$, $\mathbb{P}^{\pi^*}[N_k \geq m](\tb{\ti{s}})=1$ \\ 
Hence showed for base case. \\ 
Assuming true for $ x - \lfloor x \rfloor,  x - \lfloor x \rfloor+1,  x - \lfloor x \rfloor+2, \dots,  x - \lfloor x \rfloor+q $, we need to show that it holds for $m =  x - \lfloor x \rfloor + q+1$ \\ We can write for any $\tb{\ti{s}} \in \mathcal{S}(r)$ that: 
\begin{align}
   &\mathbb{P}^{\pi^*}[N_k\geq m ](\tb{\ti{s}}) \\
   &=\mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq m-1](\tb{\ti{s}}) \\
   &+  \sum_{r' \in [r]} \binom{r+1}{r'} \mathbb{P}^{\pi^*}[N_k \geq m-1](r') .   \Big\{ \frac{r' + (r+1-2r')\delta}{n \cdot 2^r} +   \frac{n-r-1}{n2^{r+1}}        +    \frac{\Delta}{n}  (r+1-2r') \Big \} 
\end{align}
 Here the RHS doesn't depend on which $\tb{\ti{s}} \in \mathcal{S}(r)$ is being chosen again due to induction assumption and Corollary \ref{corollary:p_star}. Thus shown for m. \textcolor{blue}{$m = x - \lfloor x \rfloor + q + 1$} ? \\
 Thus, back in expression for $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ in Equation \eqref{eqn:prob_nxs}, $\mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}})$ is also not dependent on $\tb{\ti{s}} \in \mathcal{S}(r)$. Therefore, $\mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}})$ is same for all $\tb{\ti{s}} \in \mathcal{S}(r)$.  \\

 
 Finally we need to show that, 
    \begin{align}
        \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) \geq \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}') \forall \tb{\ti{s}}' \in \cup_{r' \in \{0,[r]\}}\mathcal{S}(r')
    \end{align}
 with equality only at $\tb{\ti{s}}' = \tb{\ti{s}}$. \\
 Recall again, for any $\tb{\ti{s}} \in \mathcal{S}(r+1)$, 
 \begin{align}
     &\mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}})\\
     &=   \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' \in [r]} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\ 
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' = 1}^{ \lfloor \frac{r+1}{2} \rfloor } \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\
     &\quad + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{ r} \binom{r+1}{r'}  .  p^*_{r+1,r'}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') 
     \end{align}
     In the above, we just split the summation and below, we use the fact that Claim \ref{claim:probability_inequality} is true for our instances.\\
     In the below all $\delta_{r'}$ are all positive. Note that for different $r$, these will be different and technically we must write $\delta_{r,r'}$ but we let it be to avoid notational overhead. \textcolor{red}{we can use $\delta_{r,r'}$. for now im leaving it as it is}
     
     \begin{align}
     &\mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}})\\
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r'= 1}^{ \lfloor \frac{r+1}{2} \rfloor } \Big\{\binom{r}{r'}  .  p^*_{r,r'} - \delta_{r'} \Big\}  \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \\
     &\quad + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{ r} \Big \{\binom{r}{r'}  .  p^*_{r,r'}+ \delta_{r'}  \Big\}\mathbb{P}^{\pi^*}[N_k \geq x-1](r')  \\ 
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' = 1}^{ \lfloor \frac{r+1}{2} \rfloor } \Big\{\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\} \\
     &\quad -  \sum_{r' = 1}^{\lfloor \frac{r+1}{2} \rfloor }\Big\{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r')\Big\}   + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{ r} \Big\{\binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r')\Big\} \\
     &\quad + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{r} \Big\{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\}  \\ 
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \sum_{r' = 1}^{ r} \Big\{ \binom{r}{r'}  .  p^*_{r,r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\} \\
     &\quad -  \sum_{r' =1}^{ \lfloor \frac{r+1}{2} \rfloor}\Big\{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\}   + \sum_{r' = \lfloor \frac{r+1}{2} \rfloor +1}^{ r} \Big\{ \delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\} \\ 
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  \\
     &\quad -  \sum_{r' = 1}^{ \lfloor \frac{r+1}{2} \rfloor }\Big\{ \delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\}  + \sum_{r'= \lfloor \frac{r+1}{2} \rfloor +1}^{r} \Big\{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](r') \Big\}  
     \end{align}
    The last step is using the definition of $\mathbb{P}^{\pi^*}[N_k \geq x](r)$. \\
    Below we use Corollary \ref{corollary:pn_x}:
     \begin{align}
     &\mathbb{P}^{\pi^*}[N_k\geq x](\tb{\ti{s}})\\
     &\geq  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \sum_{r'=1}^{ \lfloor \frac{r+1}{2} \rfloor } \Big \{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1)\Big\} \\
     &\quad+ \sum_{r' =\lfloor \frac{r+1}{2} \rfloor +1}^{r} \Big\{\delta_{r'} . \mathbb{P}^{\pi^*}[N_k \geq x-1](\lfloor \frac{r+1}{2} \rfloor + 1)\Big\} \\ 
     &=  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \Big\{ \sum_{r'= 1}^{ \lfloor \frac{r+1}{2} \rfloor }\delta_{r'} - \sum_{r'= \lfloor \frac{r+1}{2} \rfloor +1}^{r} \delta_{r'} \Big\} . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1)  \\ 
     &= \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( \lfloor \frac{r+1}{2} \rfloor + 1) \\ 
     &> \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) \mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) + \mathbb{P}^{\pi^*}[N_k \geq x](r)  -  \mathbb{P}(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})) . \mathbb{P}^{\pi^*}[N_k \geq x-1]( r) 
 \end{align}
 In the last second step, we used the result and the discussion that leads to Equation \eqref{eqn:prr}.\\
 For the last step, we further use Corollary \ref{corollary:pn_x}.\\
 Thus, we have, 
 \begin{align}
     \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k \geq x](r) \geq P(\tb{\ti{s}}|\tb{\ti{s}},\pi^*(\tb{\ti{s}})).(\mathbb{P}^{\pi^*}[N_k \geq x-1](\tb{\ti{s}}) - \mathbb{P}^{\pi^*}[N_k \geq x-1](r))
 \end{align}
 By recursion and same arguments as before that follows Equation \eqref{eqn:pnxnx}, \\
 \begin{align}
     \mathbb{P}^{\pi^*}[N_k \geq x](\tb{\ti{s}}) = \mathbb{P}^{\pi^*}[N_k \geq x](r+1) >  \mathbb{P}^{\pi^*}[N_k \geq x](r)
 \end{align}
 Hence the overall main induction argument for $r$ holds.     
\end{proof}

==> Sections/intro_old.tex <==
\pt{what is our problem, and what are challenges, what is novelty, why it is significant, and how is the flow of the entire thing. If not, can you try to think of how to take care of these important points. }.

...

\pt{Something along these lines has to be written in the intro.}

At the heart of this paper lies the following central question, which we state clearly:

\begin{center} \emph{``What is the fundamental difficulty of decentralized learning in multi-agent stochastic shortest path problems under linear function approximation?''} \end{center}

Multi-agent stochastic systems are ubiquitous -- appearing in domains like swarm robotics, traffic networks, and distributed control systems. In many such settings, agents must act collaboratively while having access to only partial, local information, and without centralized coordination. Understanding the inherent hardness of learning in these decentralized environments is therefore crucial: it informs the limits of achievable performance and guides the design of more efficient algorithms.

In particular, linear function approximation is an essential modeling tool to overcome the curse of dimensionality, but it also complicates the learning task by introducing generalization errors. Thus, quantifying the true difficulty in decentralized linear MDPs and SSPs is not only of theoretical importance but also necessary for building scalable, robust multi-agent systems.


Furthermore, the problem of establishing a \emph{regret lower bound} is crucial in evaluating the performance of decentralized learning algorithms. Specifically, we wish to understand how the performance of decentralized agents compares to that of an oracle following the optimal policy $\pi^*$ over $K$ episodes. The regret lower bound provides a benchmark against which the efficiency of the learning algorithms can be measured. A lower bound on regret helps establish the limits of what is achievable by decentralized agents when trying to minimize the total cost in the MA-SSP problem. 



A popular class of problems studied under the literature on Markov Decision Problems is the Stochastic Shortest Path (SSP) Problem \citep{eaton},\citep{berttsit}\citep{yu2013boundedness}\citep{yu2013q}\citep{bert_prop_pol}\citep{guillot2017stochasticshortestpathproblem}. It is also known as total reward undiscounted MDP \citep{puterman2014markov}, \citep{bertsekas2012dynamic}. It generalizes from the well-known Shortest Path (SP) Problem where one has to chose the best links at every node to traverse from one node to another on a \textit{known} network. To model various uncertainties, under SSP, costs are treated as stochastic, actions are represented as more abstract quantities, and there exists conditional probability distributions associated over \textit{next states} for any \textit{state-action} pair. Depending on how many agents are to traverse, the problem may be single or multi-agent. When cost and transition structures are known to the agent(s), the problem is that of searching the right strategy of chosing actions. When either of these are not available, the agent(s) must \textit{explore} and learn the environment over time and pick the \textit{best} actions. A line of works has recently emerged studying the learning version of SSP problem with single agent with finite state and action spaces \citep{tarbouriech2020no} \citep{rosenberg2020near} \citep{tarbouriech2021stochastic}\citep{cohen2021minimax}. 
To extend above works for large number of state and action spaces, \citep{min2022learning}
 and \citep{vial2022regret} use linear function approximations. While \citep{min2022learning} approximates only the transition dynamics and assumes the knowledge of costs, \citep{vial2022regret}'s model assumes approximation of costs as well. In summary, these works propose algorithms motivated by existing works in other classes of MDP and Bandit Literature. Additionally, the optimality of these algorithms has also been well established through tight lower bounds. 
 Many real world goal oriented settings however, involve interaction of multiple independent decision makers. To incorporate such settings, \citep{trivedi2023massp} introduce the problem of Decentralised Learning of Stochastic Shortest Path. The paper provides an algorithm for this setting and report an upper bound on regret of $\widetilde{O}({B^*}^{1.5}d \sqrt{nK/c_{min}})$ where $B^*$ is the maximum expected cost to reach goal from any state, $n$ is the number of agents, $d$ is related to the feature dimensions and $K$ is the number of episodes. The paper, however, does not comment on its optimality. Are better learning algorithms possible in this setting? If yes, what are the optimality gaps that new algorithms can fill? Can we comment on tightness of regret bounds with respect to number of agents? To answer such questions, it is important to obtain good lower bounds for this setting. Typical lower bound proofs in the literature of single-agent SSP \citep{rosenberg2020near}, \citep{min2022learning} or that of multi-armed bandits \citep{auer2002nonstochastic} or in general RL \citep{jaksch2010near} are generally based on hard to learn instances. 

The transition from single agent SSP to Multi-Agent SSP, leads to the following complications: 
\begin{itemize}
    \item The state and action space explodes (exponentially in number of agents $n$). Due to exponentially large number of states and actions, it is challenging to create and analyze such an instance for regret lower bound. Further, it is desirable to create generalizable instance in the number of agents in order to have analyses for all $n \geq 1$.  
    \item Next state transition probabilities and costs of individual agents (and thus of the system as a whole) depends not only on individual current state and action but also on that of others.
    \item Cost information is available only locally and needs to be shared with other agents to meet global objective. However, there may be privacy, security and scaling issues \citep{zhang2018fully}. 
    \item Existing lower bound proofs for previously studied settings typically consider only two node networks. For single agent cases, it corresponds to only two states. Both the optimal policies as well as values are easily characterizable. But, in a multi-agent (n agents) set up, even a two node network corresponds to $2^n$ states. It is unclear whether tractable optimal policies exist. Further, tractable closed form expression of optimal value function is no longer easy to obtain to use it in lower-bound regret analysis. We circumvent this issue by ignoring a non-exactly simplifiable summation of not neccesarily all positive terms, by showing that the entire summation is itself positive (\ref{lemma:sum_diff_prob_v}).
    \item In our analysis, we observe another similar challenge when simplifying a KL-divergence term that arises due to information theoretic bound on difference between expectations over different measures of the same random variable (\ref{eqn:exp_diff}) that captures the number of times sub-optimal component of action is taken similar in spirit to proofs in \citep{auer2002nonstochastic}. Instead of exact simplification, a suitably tight upper bounding technique that exploits symmetry of probability distrubution arising due to symmetry in state-space to simplify KL-divergence works for us.
 \end{itemize}

 
 
Major contribution of our work are 

\begin{itemize}

\item \textbf{Novel Feature Design.}  Design of new features generalizable to any number of agents to use in creating hard to learn LM-MASSP instance
\item Provide and study classes of valid LM-MASSP instances that are hard to learn to prove matching $\sqrt{K}$ lower bound. Such a lower bound analysis is first-of-its kind for exponential number of states and actions arising here due to muli-agent setting and can be generalizable to other multi state, multi action settings.

\item We characterize optimal policies for any 2-node instance as proposed in \ref{subsec:problem_instance} and show that its very tractable. Further, these instances have an interesting partition of state space based on number of agents at a given node - all states lying the same partition set have same optimum value function implying that under optimal policy, states with same number distribution of agents across the two nodes are equivalent as value function is independent of who is present and only dependent on how many are present

\end{itemize}

% \pt{I feel this is not needed in the conference papers.}

% In \ref{subsec:relatedwork} we provide a brief background on this line of literature. \\
% In \ref{subsec:prelims} we introduce the problem setting and necessary definitions. \\
% In \ref{subsec:problem_formulation} we formulate our problem. \\
% In \ref{subsec:problem_instance} we provide details of our instances. \\
% In \ref{subsec:features} we provide the features to use in the function approximation of transition probabilities. \\
% \ref{sec:theory} discusses major results with proof overviews.\\
% In \ref{sec:discussion} we summarize our contribution and suggest some interesting open problems arising from our work.\\
% All the detailed analyses and proofs leading to the key results are deferred to the appendix \ref{sec:appendix}

\subsection{Related Works}\label{subsec:relatedwork}


% \pt{If these are incorporated, we can remove this itemize list.} \textcolor{red}{d/one}


\paragraph{Shortest Path Problems.} The shortest path problems are one of the classical problems studied in the fields of computer science and operations research. The first evidence of stochastic shortest path problem may be traced back to 
\cite{eaton}. They studied the problem in pursuit evasion games. \cite{berttsit} proved the natural generalization of results for deterministic shortest path to the stochastic setting. Recently there has been a growing interest in studying the learning version of the problem \cite{tarbouriech2020no}, \cite{tarbouriech2021stochastic}, \cite{cohen2021minimax},\cite{rosenberg2020near}, \cite{vial2022regret}, \cite{min2022learning}. \\
\citep{tarbouriech2020no} provides first no-regret SSP learning algorithm UC-SSP whose regret bound scales as $\widetilde{O}(DS\sqrt{ADK/c_{min}})$ after K episodes for any tabular SSP with $S$ states, $A$ actions, positive costs bounded above $c_{min}>0$ and $D$ diameter of SSP defined as the smallest expected hitting time from any state to goal. In a follow-up work, \cite{rosenberg2020near} provide an algorithm whose regret upper bound gets rid of the $c_{min}$ dependence and scales as $\widetilde{O}(B^*S\sqrt{AK})$ where $B^*$ is analogous to $D$ above but in terms of cost rather than time. Importantly, they provide a lower bound scaling as $\Omega(B^*\sqrt{SAK})$ showing that their algorithm is optimal to a factor of $\sqrt{S}$. 

\paragraph{Learning in SSP.} \citep{tarbouriech2021stochastic} provide EP-SSP, a model based SSP learning algorithm whose regret upper bound scales as $\widetilde{O}(B^*\sqrt{SAK})$ achieving the previously reported lower bound. EP-SSP does not require prior knowledge of $B^*$. The paper also dicusses various cases that lead to first-nearly horizon-free regret bound beyond the finite horizon MDP setting. \citep{cohen2021minimax} assumed costs to be i.i.d and unknown while previous works assumed it to be known and deterministic and provided an algorithm based on reducing the SSP to finite horizon MDPs whose regret upper bound also achieves the reported lower bound. \\
The above works were for tabular SSPs. To deal with higher number of states and actions, \citep{min2022learning} and \citep{vial2022regret} assumed slightly different linear function approximation models for transition probabilities. \citep{vial2022regret} provides an algorithm that, under minimal assumption, obtains sublinear regret, is computationally efficient, and uses stationary policies. \citep{min2022learning} first proposes an algorithm with Hoeffding-type confidence sets that attains $\widetilde{O}(d{B^*}^{1.5}\sqrt{K/c_{min}})$
 regret for positive costs. A further improvement of the regret bound to  $\widetilde{O}(d{B^*}\sqrt{K/c_{min}})$ is achieved for another proposed algorithm using refined Bernstien-type confidence sets. Additionally provided lower bound of $\Omega(dB^*\sqrt{K})$ suggests that their algorithm is optimal to a $\sqrt{c_{min}}$ factor. \\
 All the above works consider that there is just a single traversing agent. \citep{trivedi2023massp} extend the problem to a decentralized multi-agent setup and provide a MACCM algorithm with a MAEVI subroutine whose regret scales as $\widetilde{O}({B^*}^{1.5}d\sqrt{nK/c_{min}})$. The paper does not comment on how tight the bound is. Hence the optimality of proposed algorithm is not well-established. \\
 \citep{zhang2021decentralized} propose two fully decentralized actor-critic algorithms for large scale MARL problems with convergence guarantees when value functions can be approximated by linear functions.

 
% \pt{let us keep the flow of the paper as it is now, this is very standard flow in the ML community.} \textcolor{red}{ok}

==> Sections/outline.tex <==
\section{Outline of the Paper}

Here is the first attempt to the outline of the paper. We need to change or modify it as we write the paper. 

\begin{abstract}
We investigate the theoretical foundations of the multi-agent stochastic shortest path (MA-SSP) problem from a regret minimization perspective. While single-agent SSP has been well-studied with established regret upper and lower bounds, the multi-agent version remains under-explored. Recent work has extended regret upper bounds to the MA-SSP setting, but fundamental questions remain unresolved. In this paper, we derive the first regret lower bounds for MA-SSP and analyze how the number of agents impacts the complexity of learning. Our results bridge a critical gap in the literature and provide new insights into the design of efficient multi-agent learning algorithms.
\end{abstract}

\section{Introduction}

Briefly describe SSP, transition to RL version
Gaps in literature: lower bounds, agent scaling. And finally our major  contributions.
\begin{itemize}
    \item Start with the importance of the Stochastic Shortest Path (SSP) problem in planning and decision-making.
    \item Mention that Single-Agent SSP is well studied; cite foundational RL results with known upper and lower bounds.
    \item Emphasize that the multi-agent extension (MA-SSP) is less explored; mention \cite{trivedi2023massp} as a recent attempt.
    \item Point out the gaps in literature: No lower bounds for regret in MA-SSP.
    \item The effect of the number of agents on regret is poorly understood.
\end{itemize}

\textbf{Major Contributions:}

First regret lower bounds for MA-SSP.

Analysis of agent scaling in regret.

Matching (or near-matching) lower and upper bounds.

Novel intermediate theoretical insights (e.g., feature design).

Some additional results that can be of interest to the  ML community in other domains.

\subsection{Related Work}

SSP in RL: single-agent case. 
MARL literature, MA-SSP work. 
Prior bounds.  Highlight novelty Mention that to the best of our knowledge, these results are novel. Divide the entire section into 3-4 sub parts and dostinguish our work with the existing and also highlight the challenges and novelty. 

\begin{itemize}
    \item Classical SSP in RL: key algorithms, upper/lower bounds.
    \item Regret analysis in online RL (e.g., UCRL2, UBEV).
    \item Multi-agent RL and planning: MARL challenges, coordination, scalability.  
    \item \cite{trivedi2023massp} as the most relevant prior work on MA-SSP (upper bounds only).
    \item Lower bounds in MARL (mention scarcity).
    \item Highlight the novelty of your contributions in contrast.
\end{itemize}


\section{Problem Formulation}

Notations and Prelims -- Define MA-SSP setup: states, joint actions, dynamics, cost. Define regret. 
Key assumptions -- policy class, etc.



\begin{itemize}
    \item Formal definition of the MA-SSP setting: State space, action space, transitions, cost structure.
    \item Agents act in a shared environment to reach a terminal state.
    \item \textbf{Objective}: minimize cumulative cost  over episodes.
    \item Define regret formally over $K$ episodes.
    \item In detail explain assumptions: decentralized learning, linear MDP, feature design (complex process) etc. The linear MDP transitions can't be decomposed as a separate agents. 
    \item Highlight complexity due to joint actions and decentralized learning constraints (if any).
    \item Policy class restriction etc. 
\end{itemize}

\section{Our Approach}

High-level strategy to prove lower bounds. Intuition: why MA-SSP is harder. How to design the hard instances? Why they are hard. Major challanges, and how we address them. 

\begin{itemize}
    \item High-level outline of how you study the regret lower bounds in MA-SSP.
    \item Intuition: Construct ``hard'' MA-SSP instances.
    \item Show how agent interactions increase complexity
    \item Describe what makes SSP harder in the multi-agent case vs. single-agent.
    \item Brief overview of feature design techniques used in analysis.
    \item Clearly highlight the challenges and then how they are addressed. 
\end{itemize}

\section{Theoretical Results}

Theorem: regret lower bound. Sketch of proof. Dependence on number of agents. Matching to known upper bounds. Feature-related insights. Other key results in the form of lemma, corollary and propositions, remarks etc. 



\section{Experiments (If available)}

Toy MA-SSP setup. Regret vs. agents graph if possible. Empirical support for theory

\begin{itemize}
    \item Simple MA-SSP instances with n=3, 4, etc?
    \item Plot regret vs. number of agents.
    \item Show alignment between theory and practice (at least qualitatively).
    \item Highlight how coordination and joint action space increase learning complexity.
\end{itemize}

\section{Conclusion/Discussion}

Recap contributions. Importance of theoretical results. Future work directions.

==> Sections/updated_features.tex <==
\section*{Updated Features}




